General supervised learning as change propagation with delta lenses

Delta lenses are an established mathematical framework for modelling and designing bidirectional model transformations. Following the recent observations by Fong et al, the paper extends the delta lens framework with a a new ingredient: learning over a parameterized space of model transformations seen as functors. We define a notion of an asymmetric learning delta lens with amendment (ala-lens), and show how ala-lenses can be organized into a symmetric monoidal (sm) category. We also show that sequential and parallel composition of well-behaved ala-lenses are also well-behaved so that well-behaved ala-lenses constitute a full sm-subcategory of ala-lenses.

==> cameraReadyStuff.tex <==
Paper:   84
Authors: Zinovy Diskin
Title:   Supervised learning as change propagation with delta lenses

-------------------------------------------------------

Dear Zinovy,

concerning the preparation of the camera-ready papers, we were asked
for more details about

> 5. Please do not forget to clearly mark the corresponding author.

First, please always include the corresponding author's email address.

Second, you can mark the corresponding author by putting an envelope
(in brackets) behind the name of the corresponding author (as it is
done in the PDFs typeset by Springer). For this you can for instance
use "\Letter" from the marvosym package.

Please remember that the final paper and the signed copyright form are
due on

  February 22, 2020.

We are sorry for all the extra instructions, but the publication
process for ETAPS has changed due to a new contract with Springer,
which causes some hiccups.

Regards,

Barbara & Jean

==> content4arxive-OLD.tex <==
% -- these guys are in the main file
%\maketitle
%\input{abstract}
%\pagestyle{plain}	
	\newcommand\figrplane{FigrPlane}
	
	\newcommand\figro{\figref{policyfun-ml1}}
	\newcommand\figroo{\figref{policyfun-ml2}}
	\renewcommand\figrii{\figref{policyfun-brief}}

 	  %\input{ll-sections/intro-foss20} 
%--->  this is the right backgr sect	      	  
	      	  \input{ll-sections/intro-act2foss}
%-------
	        %\input{ll-sections/ml=bx}  outdated
	\renewcommand\figri{\figref{bxmlPut}}
	\renewcommand\figrii{\figref{policyfun-brief}}
	         %\input{ll-sections/backgr} outdated 
	          % changed name form ..backgr-new to overview
\input{ll-sections/backgr-act2foss}
       %%--> this is useful section toi be used later but not in this paper
       %\input{ll-sections/backgr--views-via-monads}
        %%   \input{ll-sections/prelimiaries}
%\input{ll-sections/overview-act2foss}
%\input{ll-sections/arrowDiags-to-use}
\renewcommand\figriii{\figref{policyfun}}
 %-----
 \input{ll-sections/learn4bx}
%%--> the next sect went into the sect above!
% \input{ll-sections/functOfLearning-act2foss}
    %\clearpage
%\dend
	
	%%%\input{ll-sections/horiz-compose-new} outdated
	%%% => comment only for debugging <===
	%%%-- sect apalens def
	\newcommand\figari{\figref{apa-arity}} %arity
	\newcommand\defri{\defref{def:aalens-arity}}
	\renewcommand\ppgB{\ensuremath{\putl^B}}
	\renewcommand\ppgB{\ensuremath{\putps}}
	\input{ll-sections/apalensdefs-act2foss}
%	\dend
	
	%%-- sect aplenscat
	\renewcommand\kl{\ensuremath{\ekk;\ell}} 
		\renewcommand\figrii{\figref{kl-lens}}
	\input{ll-sections/apalenscat}
	%\dend
	
		\input{ll-sections/relWork}
	\input{ll-sections/concl}
%	\dend

\bibliographystyle{splncs} 
%\bibliographystyle{splncs04} 
\bibliographystyle{abbrv}
\bibliography{refsGrand17}

% 
%\clearpage
%\input{ll-sections/arrowDiags-to-use}

\clearpage
\medskip
	\noindent{\Large\sc Appendices} 
	\appendix
	
	\input{ll-sections/pcat}
	%\dend
	%==========
	\newcommand\ideny{identity}
	% renewcommm from Append B are copied here \renewcommand\kl{\enma{\ekk\ell}}
	\renewcommand\lm{\enma{\ell\emm}}
	\renewcommand\klbr{\enma{(\ekk\ell)}}
	\renewcommand\lmbr{\enma{(\ell\emm)}}
	\renewcommand\putekel[2]{\putUL{\kl.#1}{#2}}
	\renewcommand\putelem[2]{\putUL{\lm.#1}{#2}}
	%--
	\input{ll-sections/proof-th1}
	%==========
	
	%\dend
	%%%%%%%%%%%
	\newcommand\figkl{\figref{kl-lens}}
	\renewcommand\figrii{\figkl} %ref{kl-lens}}
	\newcommand\defrii{\defref{def:aalens-hComp}}
	
	\renewcommand\kl{\ensuremath{\ekk;\ell}} % this one maybe in aworng place
	\renewcommand\lm{\enma{\ell;\emm}}
	\renewcommand\lmbr{\enma{(\ell;\emm)}}
	%
	\renewcommand\kl{\enma{\ekk\ell}}
	\renewcommand\lm{\enma{\ell\emm}}
	\renewcommand\klbr{\enma{(\ekk\ell)}}
	\renewcommand\lmbr{\enma{(\ell\emm)}}
	\renewcommand\putekel[2]{\putUL{\kl.#1}{#2}}
	\renewcommand\putelem[2]{\putUL{\lm.#1}{#2}}
	%--
	\input{ll-sections/proof-assoc-seq}
%	%%%%%%%%%
%	\input{ll-sections/lenses-as-mm}
%%	\clearpage
%%	\input{ll-sections/accat-symLensAppendix}
%%	\input{ll-sections/arrowDiagsToUse}

	       		%\clearpage
%\input{ll-sections/todo}
	\dend


%	%\dend
%	\input{ll-sections/actions}
%	\input{ll-sections/derivatives-as-functors}
%	\input{ll-sections/bits-i-pieces-2}
	% -- old wordy def
	
			\clearpage
			\noindent{\LARGE Aux and OLd sections} 
				\input{ll-sections/intro}
				\input{ll-sections/overview-act2foss}
			%	\input{ll-sections/backgr--views-via-monads}
	\input{ll-sections/intro-foss20} 
	\input{ll-sections/backgr--views-via-monads}
	

	 
	\clearpage
	\input{ll-sections/bits-i-pieces}
	\input{ll-sections/arrowDiags-to-use}
	\input{ll-sections/todo}


==> ll-figures/diags/aalens-arity.tex <==
	\begin{figure}
%	\begin{equation}
\begin{tabular}{c@\qquad c}
	% column 1
	\begin{diagram}[w=5em,h=2em]
		% row 11
		 \dbox{A} & \rMapsto^{{:}\get_p} & \dbox{B}
		\\  % row 12
		&&\dTo>v
		\\ % row 13
	\dDashto>u&
		\swseTilearrowAB{{:}\putpa}{}
		%\seTilearrowAB{}{}
	%	\Downarrow %{:}\putpa
		&B'
			\\ % 14
		&&\dDashto>{\amex{v}}
		\\ % 15
A' &\rDermapsto^{{:}\get_{p'}} & B''
	\end{diagram}
%------------
& % column 2	
%--------------
	\begin{diagram}[w=5em,h=5ex]
		% row 21
	\dbox{A} &\rMapsto^{{:}\get_p} & \dbox{B} & \rMapsto^{{:}\get_q} & \dbox{C}
	\\  % row 22
	&&&&\dTo>w
	\\ % row 23
	&	\swseTilearrowAB{~~2{:}\putpa}{}&\dDashto>v&
	     \swseTilearrowAB{~~1{:}\putqb}{}&C'
	\\ % 24
	&&&&\dDashto>{\amex{w}}
	\\ % 25
	\dDashto<u &
%	\swTilearrowAB{}{~~~{:}\putpa}{}
		& B' &\rDermapsto^{{:}\get^{(1)}_{q'}} & C''
	\\  % row 26
	&&\dDashto>{\amex{v}}& \stackrel{3{:}\get_{q'}}{\Longrightarrow}&\dDashto>{\get^{}_{q'}(\amex{v})}
	\\  % row 27
	A' &\rDermapsto^{\get^{(2)}_{p'}} & B''&\rDermapsto^{{:}\get^{(3)}_{q'}}& C''''
	\end{diagram}
\\  [10pt] % End OF TABULAR ROW 1
(a)  & (b)
\end{tabular}
	%	\end{equation}
	\caption{Schemas of update propagation: (a) the arity of \putl, and (b) composition. Input elements are boxed (nodes) and solid (arrows), output elements are not boxed and dashed.
	\label{fig:ppg-schema}}
\end{figure}
A target update \frar{v}{\get(B)}{A'} is called {\em closed} if %$\putl^B_\inda(v)=\id_{A'}$. 
$\amex{v}=\id_{A'}$, and an aa-lens is {\em closed} if all its target updates are closed.  \qed
\end{defin}
%The following is a specialization of Def.~\ref{def:wblens}, in which consistency between a base $B$ and a view $A$ is understood as equality $\get(B)=A$.


==> ll-figures/diags/al-lens-as-mealy-apply.tex <==
{%\renewcommand\app{{}}
\begin{figure}
	%	\begin{wrapfigure}{R}{0.5\columnwidth}
	%		\vspace{-0.5cm}
	\centering
	\begin{tabular}{l}%@{\quad}l}
\begin{diagram}[w=2.5em,h=2.5em]%[small]
% -------------------------------> row 1
%\Inget&\rEQ&
&&\Inget&&&&
\rTo^{\get} % = \{ \get^\readd\orr\get^\app\}  }
%	begin{\cases}
%	\get^\app\\ 
%	\get^\readd 
%	\end{cases} 
%}
%\pile{
%	\rTo^{\hspace{0em}\get^\app}%_{\footnotesize{\orr}} 
%%	\\ 
%%	\rTo~{\get=%\left\{ \right.
%%		\hspace{4em} }
%		\\
%	\rTo_{\hspace{0em}\get^\readd}
% } % end pile 
&&&&	
\Outget &&
\\ %%%%%%%%------- ---> row 2 
%\dTo<{\igai}
%DIAGONALS
          & \ldTo(2,2)^{\igai} \ruDotto(2,4) ~{\oisim}%\ldTo>{\igai}
          & \dTo~{\igpi} %&\rdTo(2,2)<{\igpi} 
          &
          \rdTo(2,2)~{\igpo}
           \rdTo(6,2)^{\igao}
          &&& %\pmb{\puncture} 
          &&&  
          \ldDertoda(8,2)^{~\ogpi} 
          \ldDertoda(6,2)~{\ogpo
%          	\begin{array}{c}
%          		\\ [-17.5pt]
%          		\ogpo
%          		\\
%          		\pmb{\puncture}
%          	\end{array}
}
        %    	\ogpo}  %
           \ldDertoda(2,2)~{\ogao} 
          &&\rdTo>{\ogbi}
\\ %%%%%%%%%%%%%-----------> row 3 for the asymmetric case
%\uDashto<{\oiiso}
\sparra &&
\ppi %\uDashto~{\oiiso}
&
  \pile{%\rTo^{\qquad_\ta} 
	%\rTo^{\hspace{3em}_\so}
	\rTo%~{\so}
	\\
	%       \lDashto
	%       \\
	%	\rTo_{\hspace{3em}^\ta}
	\rTo%~{\ta} 
}
& \po %	\sparrp
&   \lTo~\pr 
%\pile{%\rTo^{\qquad_\ta} 
%	%\rTo^{\hspace{3em}_\so}
%		\rTo%~{\so}
%       \\
%%       \lDashto
%%       \\
%       %	\rTo_{\hspace{3em}^\ta}
%       	\rTo%~{\ta} 
%}
& (\po %{\lefteqn{\hspace{2.5em}\times}}}
%	\begin{array}{c}
%%		\smash{\pmb{\puncture}}
%%		\\
%	\spobp
%\end{array}
	&{\times\hspace{0em}
	}&
\stackrel{\puncture}{\spoba)}
	 &\rTo^{~~\get_{00}}_{\text{~~from$\timm$}}%\spobR&\rTo_{b}
	&\spobb
	&
	\pile{\lTo~{_\ta} \\  \lTo~{_\so}} % pile end
	&\sparrb
	&
\\ %%%%%%%%% -------------========> ROW 4 DIAGONALS 
\uTo<{\opai} &    %\luTo<{\opai}
	& %\ruImplies(2,2)<{_{\oppi^\sim}}_{^\oppi}
%\color{blue} 
\uTo<{\oppi^\sim}\uDertodo~{\oppi}
    &
	%&&
	\luTo(8,2)_{\ippi}
	%&&
	\ruDertodo(2,2)~{\oppo}
	&& 
	\luTo(6,2)~{\ippo}
	&&
	\ruDertodo(6,2) _{\opao}
	&&\luTo(2,2)~{\ipao}
	&
	&
	\ruTo>{\ipbi} %\luTo(1,2)>{\ipi} &
\\%  --------------------------------------------->row 5
\Output&\rEQ&\Output&&&&
%\pile{\lTo^{\hspace{0em}\putl_0} \\ \lTo_{\hspace{0em}\putl} }
\lTo_{\putl}
&&&&	\Input &&
\\
&&&& &&&& &&&&
\end{diagram}
%\\ [30pt]
\\ [25pt]
(to avoid clutter,  
%the fragment $\sparrp\pile{\rTo \\  \rTo}\spobp$ is used a shorthand for $\sparrp\pile{\rTo \\  \rTo}\spobp\lTo^{\pr_2}(\spoba\times\spobp)$
%\\ and 
the fragment $\sparra\pile{\rTo \\  \rTo}\spoba$ is not shown
)
%not shown to avoid clutter)
\end{tabular}
\begin{myeq}{eqmmgetP}
	%	\eqmmgetP  % was a macro but now is a direct encoding below
	\begin{array}{| l@{\quad}l |}
		\hline
		\multicolumn{2}{|l|}{
			\mbox{Definition of a learning $\get$  machine over given \spabpgetoo: }} 
		\\ [3pt]
		\text{(Alphabets)} &	\ainx{\get}=\sparra, \aoutx{\get}=\sparrb,
		\\ 
			\text{(State space)} &\stt^\get=\paoios\eqdef\pois\timm\ao 
			%\\	& \phantom{\stt^\get}
			\cong \apoois\eqdef\ao\timm\pois
			%= (\po\timm_\so\ppi)\timm\ao
			%\pois\timm\ao\sqcup\poit\timm\ao~
			%\cong~\ao\timm\poit\sqcup\ao\timm\pois
		\\
		%\mbox{Input alphabet is $\spA_1$} &\\
		\text{(Eff. Input)} &	\Inget = \pois\timm\aois %\sqcup\poit\timm\aois
		\\
		\text{(Eff. Output)} & \Outget =\spB_1~{}_\ta\timm_\param~ \stt^\get
		             = \bapioot ~{}_\param\timm_\so~\ppi
		            \\
		           & \phantom{\Outget }= \compr{(v,A',p',e')}{(A',p',v)\models\gethit~\&~p'=e'.\so}
		            \\
		            & \phantom{\Outget }= \compr{(v,A',p',e')}{A'.\get_{00}(p')=v.\ta ~\&~ p'=e'.\so}
		         		\\ [3pt]
		\multicolumn{2}{|l|}{
					\mbox{Equational Laws (to hold for any $(p,e,A,u)\in\Inget$) %...
					
						%$p\in\po$, $A \in\ao$, $e\inn\ppi,u\inn\ai$ such that $p=e^\so \text{ or } p=e^\ta$, $A=u^\so$
}} 	\\ %[5pt]
			\multicolumn{2}{|l|}{\mbox{Basic (in addition to \gethit):}}
\\
		\text{ (Incidence)}%_{(A,u)\in\Inget} 
		& (p,e,A,u).\get.\ogbi.\so= A.\get_{00}(p) 
		% the arrow version (\get^\readd.\ogbi.\so= \igao.\get_{0}) 
		\\
		\text{ (Increm)}_{\ao} 
		&	(p,e,A,u).\get.\ogao=u.\ta ~~(= A' \text{ in Eff. Output})
		\\
				\text{ (Increm)}_{\po} 
		&	(p,e,A,u).\get.\ogpo=e.\ta~~ (=p' \text{ in Eff. Output})
			\\
		\text{ (Increm)}_{\ppi} 
		&	(p,e,A,u).\get.\ogpi=\id_{e.\ta}~~  (=e' \text{ in Eff. Output})
%		\begin{cases}
%			e, \text{ if } p=e^\so,\\
%			id_{e^\ta} \textit{ if } p=e^\ta
%		\end{cases}
%		\\
%				\text{ (histIgnore)}
%		&	(p,e1,A,u).\get.\ogbi=(p,e2,A,u).\get.\ogbi\ 
%		\\
%		&\text{ for any $e1 \neq e2$ as soon as $e1^\ta = e2^\ta = p$}
%		\\
%	\text{ (Nat) }	&	(u,e,p,A).\get =(\id_A,e,p,A).\get~; (u,p,A).\get_{00} \\
%	& \hspace{6.25em}= (u,p',A).\get_0~; (\id_{A'},e, p', A').\get  
		\\[2.5pt]
			\multicolumn{2}{|l|}{\mbox{Monoidal (to hold for any \frar{e1}{e.\ta}{\_}, \frar{u1}{u.\ta}{\_})  )}:}
		\\
		\text{ (GetId)}%_A	
		& 			(p,\id_p,A,\id_A).\get.\ogbi=\id_{A.\get(p)} 
		%(u, A).\get.\ogbi=(u,A).\get_0
		\\
		\text{ (GetGet)}%_{(u^\ta,u')\in\Inget} 
		&	(p,e;e1, A,u;u1).\get.\ogbi        =         (p,e,A,u).\get.\ogbi ; 
		\\ 	 & \phantom{(p,e;e', A,u;u').\get.\ogbi=} 
		(e.\ta, e1, u.\ta,u1).\get.\ogbi
		\\ [3pt]
		\hline
	\end{array}
\end{myeq}
%  --- NOW PUT
\begin{myeq}{eqmmputP}
	%	\eqmmgetP  % was a macro but now is a direct encoding below
	\begin{array}{| l@{\quad}l |}
		\hline
		\multicolumn{2}{|l|}{
			\mbox{Definition of a learning $\putl$  machine over given \spabpgetoo: }} 
		\\ [3pt]
		\text{(Alphabets)} &	\ain^\putl=\bi, \aout^\putl=\ai,
		\\ 
		\text{(State space)} &\stt^\putl=\stt^\get %= \paoios\eqdef\pois\timm\ao 
	%\\ & 
	\phantom{\stt^\get}\cong \apoois\eqdef\ao\timm\pois
				\\
		\text{(Eff.Input)} & \Input =\stt^\putl{}_\param\timm_\so~ \spB_1
		%= \abpoos ~{}_\param\timm_\so~\ppi
			%\\ 	& \phantom{\Input }
			= \compr{(A,p,e,v)}{A.\get_{00}(p)=v.\so ~\&~ p=e.\so}
					\\
		\text{(Eff.Output)} &	\Output =\spA_1\timm\spP_1\timm\stt^\putl =
		   \\
		   		   	& %\phantom{\Output }
		   		   	= \compr{(u,e^\sim,e', A',p')}{(u,e',A',p')\models \text{(Incr)}_{\ao,\po,\ppi}
		   		     ~\&~p'=e'.\so}
		   \\
		   	& %\phantom{\Output }
		   	= \compr{(u,e^\sim,e', A',p')}%
		   	    {A'=u.\ta,\; p'= e^\sim.\ta,\; e'=\id_{e.\ta}~\&~p'=e'.\so}
		   	\\ [4pt]
		\multicolumn{2}{|l|}{
			\mbox{Equational Laws (to hold for any $(p,e,A,v)\in\Inget$)
				%$p\in\po$, $A \in\ao$, $e\inn\ppi,u\inn\ai$ such that $p=e^\so \text{ or } p=e^\ta$, $A=u^\so$
		}} 
		\\ [2.5pt]
		\text{ (Incidence)}%_{(A,u)\in\Inget} 
		& (p,e,A,u).\get.\ogbi.\so= A.\get_{00}(p) 
		% the arrow version (\get^\readd.\ogbi.\so= \igao.\get_{0}) 
%		\\
%		\text{ (Increm)}_{\ao} 
%		&	(p,e,A,u).\get.\ogao=u.\ta ~~(= A' \text{ in Eff. Output})
%		\\
%		\text{ (Increm)}_{\po} 
%		&	(p,e,A,u).\get.\ogpo=e.\ta~~ (=p' \text{ in Eff. Output})
%		\\
%		\text{ (Increm)}_{\ppi} 
%		&	(p,e,A,u).\get.\ogpi=\id_{e.\ta}~~  (=e' \text{ in Eff. Output})
          \\
          \text{ (PutHit)}
          & (A,p,e,v).\putl.\opao.\get_{00}(\oppo)=\ipbi.\ta~~ (\text{a.k.a. (PutGet)$_0$ law})
			\\[2.5pt]
			\multicolumn{2}{|l|}{
			\mbox{ (Unitality (a.k.a Stability) %any \frar{e1}{e.\ta}{\_}, \frar{u1}{u.\ta}{\_})   
		               }}
		\\
		\text{ (PutId)}%_A	
		& 			(p,\id_p,A,\id_A).\get.\ogbi=\id_{A.\get(p)} 
		%(u, A).\get.\ogbi=(u,A).\get_0
		\\ [3pt]
		\hline
	\end{array}
\end{myeq}
%
%\begin{myeq}{eqmmputP}
%%	\eqmmputP
%%	\eqmmgetP  % was a macro but now is a direct encoding below
%	\begin{array}{|ll|}
%	\hline
%	\multicolumn{2}{|c|}{
%		\mbox{Definition of a parametrized $\putl$ machine over given \spabpgetoo}}
%	\\ [3pt]
%			\text{(Alphabets)} & \ain^\putl=\bi, \aout^\putl=\ai,
%			\stt^\putl
%	\\ 
%	\Input=\compr{(A,p,v)}{(A,p).\get_{00}=\so(v)} &\\
%	\Output=\compr{(e,u,A,p)}{\ta(e)=p, \ta(u)=A} &\\
%	\putl.\opi.\so=\ipo &\text{ (Inc.)}\\
%	%		    \putl.\opi.\ta.\get_0=\ipi.\ta   \text{ (Putget for objects)  }  &\\
%	%\putl.\opo=\putl.\opi.\ta  \text{ (state update) }&\\ 		[3pt]
%	%		\mbox{\putgetlaw{} law:~} &\nonumber\\
%	\putl.\opo.\get_0 =\ipi.\ta & \text{ (PutOk) }\\
%	(A, \id_{A.\get_0}).\putl.\opi=\id_{A}  &\text{ (PutId) } \\
%	\textcolor{red}{(A, v;v').\putl.\opi=(A,v).\putl.\opi ; (A',v').\putl.\opi} &\textcolor{red}{~~ (PutPut) } \\
%	\hline
%\end{array}	
%\end{myeq}
%%
\begin{myeq}{eqmmputget}
	\begin{array}{|ll|}
		\hline
		\multicolumn{2}{|l|}{
			\mbox{Definition of a coupled $(\putl,\get)$-machine (a lens) over given \spabpgetoo}}
		\\ [3pt]
		\multicolumn{2}{|l|}{\mbox{Basic equational Law (to hold for any $(A,p)\inn\spA_0\timm\spP_0$ and \frar{v}{A.\get_{00}(p)}{\_}):  }}
		\\ [3pt]	
		\text{(Def. of \oisim) } & \oisim(u,e^\sim, e',u.\ta, e^\sim.\ta) = (e^\sim.\so, e,u.\so, u) 
		\\
		\text{(PutGet)}%_{(A,v)\in\Input} 
		& (A,p,e,v).\putl.\oisim.\get.\ogbi=v ~~(\text{or } \putl.\oisim.\get.\ogbi=\ipbi)
		\\ \hline
	\end{array}
\end{myeq}
	\caption{NEW Definition of an asymmetric coupled \mema\ with learning}
\label{fig:al-lensmm}
%\end{wrapfigure}
\end{figure}
} % end renew command for \app=idle

==> ll-figures/diags/al-lens-as-mealy-big.tex <==
\newcommand\eqmmgetP{\enma{
	%	\begin{IEEEeqnarray}{ll}
	\begin{array}{| l@{\quad}l |}
		\hline
		\multicolumn{2}{|c|}{
			\mbox{Definition of learning $\get$  machine (over given $\get_{00}$)}} 
		\\ [3pt]
		%\mbox{Input alphabet is $\spA_1$} &\\
		\text{Def.1} &	\Inget =\compr{(e,u,A,p)}{\so(e)=p, \so(u)=A}  
			\\
		\text{Def.2}  & \Outget=\compr{(A,p,v)}{(A, p).\get_{00} =\ta(v)} 
		\\	
				\text{ (Nat) }	&	(e,u,A,p).\get =(e,\id_A,A,p).\get ; (u,A,p).\get_0 \\
		& \hspace{6.25em}= (u,A,p').\get_0 ; (e, \id_A', A',p').\get  
		\\
		\text{ (GetId)}_A	&	(\id_p,u, A,p).\get.\ogbi=(u,A,p).\get_0
				\\
	\text{ (GetGet)}_A &			(e;e', \id_A, A, p).\get.\ogbi= \\
		&	\hspace{5em} =(e,\id_A,A,p).\get.\ogbi ; (e',\id_A, A, p').\get.\ogbi 
				\\ [3pt]
	\text{}	&		\Inget_0=\compr{(u,A,p)}{\so(u)=A}  
					\\  
		\text{ (Inc) }&\get_0.\ogbi.\so=(\igao,\igpo).\get_{00} 
			\\
		\text{ (GetOk)}_p &	\get_0.(\ogao, \ogpo).\pr=\igai.\ta  
			\\
	\text{ (GetId)}_p &		(\id_A, A,p).\get_0.\ogbi=\id_{(A,p).\get_{00}}  
			\\
\text{ (GetGet)}_p  &			(u;u', A, p).\get_0.\ogi=(u,A,p).\get_0.\ogbi ; (u',A',p).\get_0.\ogbi \\ [3pt]
		\hline
	\end{array}
	%	\end{IEEEeqnarray}
}}

\newcommand\eqmmputP{\enma{
	%	\begin{IEEEeqnarray}{ll}
	\begin{array}{|ll|}
		\hline
		\multicolumn{2}{|c|}{
			\mbox{Definition of learning $\putl$ machine (over given $\get_{00}$ )}}
		\\ [3pt]
		\Input=\compr{(A,p,v)}{(A,p).\get_{00}=\so(v)} &\\
		\Output=\compr{(e,u,A,p)}{\ta(e)=p, \ta(u)=A} &\\
		\putl.\opi.\so=\ipo &\text{ (Inc.)}\\
		%		    \putl.\opi.\ta.\get_0=\ipi.\ta   \text{ (Putget for objects)  }  &\\
		%\putl.\opo=\putl.\opi.\ta  \text{ (state update) }&\\ 		[3pt]
		%		\mbox{\putgetlaw{} law:~} &\nonumber\\
		\putl.\opo.\get_0 =\ipi.\ta & \text{ (PutOk) }\\
		(A, \id_{A.\get_0}).\putl.\opi=\id_{A}  &\text{ (PutId) } \\
		\textcolor{red}{(A, v;v').\putl.\opi=(A,v).\putl.\opi ; (A',v').\putl.\opi} &\textcolor{red}{~~ (PutPut) } \\
		\hline
	\end{array}	}
	%\end{IEEEeqnarray}
}

\begin{figure}
	%	\begin{wrapfigure}{R}{0.5\columnwidth}
	%		\vspace{-0.5cm}
	\centering
	\begin{tabular}{c}%@{\quad}l}
\begin{diagram}[small]
	% row 00
\Inget^{11}&&&& &&&& &&&&
\\ % row 0
&
\luDashto(2,6) ~{\oiiso}
\rdTo(2,2)>{\pr} 
\rdTo(10,2)^{\get}
&&& &&&& &&&&
\\%  row 1
\dTo<{\igpi}
%& %\rdTo(2,1)
&&\Inget_0&&&
\pile{
	\rTo^{\hspace{4em}\get_0} 
%	\\ 
%	\rTo_{\hspace{4em}\get} 
} % end pile 
&&&&&	
\Outget &&
\\ % ---> row 2 
%\dTo<{\igai}
%DIAGONALS
          &    %\ldTo>{\igai}
          & \dTo(2,2)>{\igai} &
          \rdTo(4,2)~{\igao}
           \rdTo(6,2)^{\igpo}
          &&& &&&  
          \ldTo(4,2)^{\ogao}  %\ldTo(2,2)>{\ogi} 
           \ldTo(2,2)~{\ogpo} 
          &&\rdTo>{\ogbi}
\\ % row 3 for the asymmetric case
%\uDashto<{\oiiso}
\sparrp &&
%\uDashto~{\oiiso}
\sparra
	&
	\pile{\rTo^{\so~~~
}
	 \\  \rTo_{\ta~~~}} % pile end
	&\spoba&\lTo~{\pr_1}&(\spoba&{\times\qquad\quad}&\spobp)
	 &\rTo^{~~\get_{00}}%\spobR&\rTo_{b}
	&\spobb
	&
	\pile{\lTo^{\ta
		}
	 \\ \lTo_\so} % pile end
	&\sparrb
	&
\\ % ROW 4 DIAGONALS 
&\luTo<{\opai}
	&\uTo(2,2)>{\oppi}&
	&
	&\ruTo(4,2)~{\opao}
	& &\luTo(4,2)_{\ipao}
	\ruTo(6,2) _{\oppo}
	&&\luTo(2,2)~{\ippo}
	&
	&
	\ruTo>{\ipbi} %\luTo(1,2)>{\ipi} &
\\%  row 5
&&\Output&&&&\lTo^{\qquad\quad\putl}&&&&	\Input &&
%\\
%&&&& &&&& &&&&
\end{diagram}
\\ [25pt]
(mappings 
$\spP_1\pile{\rTo \\  \rTo}\spP_0\lTo^{\pr_2}(\spA_0\times\spP_0)$ not shown to avoid clutter)
\\ [2.5pt]
\end{tabular}
\begin{myeq}{eqmmgetP}
	\eqmmgetP
\end{myeq}
\begin{myeq}{eqmmputP}
	\eqmmputP
\end{myeq}
\begin{myeq}{eqmmputget}
	\fbox{\putgetlaw{} law:~ $\putl.\oiiso.\get.\ogbi~=~\ipbi$} 
\end{myeq}
	\caption{BIGGG Categorically learning asymmetric lens as a special Mealy machine couple: the two common state spaces are $S_0=\spA_0\timm\spP_0$ and $S_1=S_0\timm\spP_1$}
\label{fig:al-lens-mealy}

%\end{wrapfigure}
\end{figure}

==> ll-figures/diags/al-lens-as-mealy-nice.tex <==
\begin{figure}
	%	\begin{wrapfigure}{R}{0.5\columnwidth}
	%		\vspace{-0.5cm}
	\centering
	\begin{tabular}{l}%@{\quad}l}
\begin{diagram}%[small]
% -------------------------------> row 1
&&\Inget&&&&
\pile{
	\rTo^{\hspace{3em}\get} 
	\\ 
	\rTo_{\hspace{3em}\get_0} } % end pile 
&&&&	
\Outget &&
\\ %%%%%%%%------- ---> row 2 
%\dTo<{\igai}
%DIAGONALS
          & \ldTo>{\igai}
          &&\rdTo(2,2)<{\igpi} 
          \rdDashto(4,2)~{\igpo}
           \rdTo(6,2)^{\igao}
          &&& &&&  
          \ldTo(6,2)^{\ogpi} 
          \ldDashto(4,2)~{\ogpo}  %
           \ldTo(2,2)~{\ogao} 
          &&\rdTo>{\ogbi}
\\ %%%%%%%%%%%%%-----------> row 3 for the asymmetric case
%\uDashto<{\oiiso}
\sparra &&
\uDashto~{\oiiso}
&&	\sparrp
	& \pile{\rTo^{\qquad_\ta} \\ \rTo_{\qquad^\so}}
	&\spobp&{\times\qquad\quad}&\spoba)
	 &\rTo^{~~\get_{00}}_{\text{~~from$\timm$}}%\spobR&\rTo_{b}
	&\spobb
	&
	\pile{\lTo~{_\ta} \\  \lTo~{_\so}} % pile end
	&\sparrb
	&
\\ %%%%%%%%% -------------========> ROW 4 DIAGONALS 
&\luTo<{\opai}
	&&\ruTo(2,2)<{\oppi}
	&&\luTo(6,2)_{\ippi}
	%&
	\ruDashto(4,2)~{\oppo}
	& 
	&\luDashto(4,2)~{\ippo}
	\ruTo(6,2) _{\opao}
	&&\luTo(2,2)~{\ipao}
	&
	&
	\ruTo>{\ipbi} %\luTo(1,2)>{\ipi} &
\\%  --------------------------------------------->row 5
&&\Output&&&&
\pile{\lTo^{\hspace{1.5em}\putl_0} \\ \lTo_{\hspace{1.5em}\putl} }
&&&&	\Input &&
\\
&&&& &&&& &&&&
\end{diagram}
%\\ [30pt]
\\ [25pt]
(to avoid clutter,  
the fragment $\sparrp\pile{\rTo \\  \rTo}\spobp$ is used a shorthand for 
$\sparrp\pile{\rTo \\  \rTo}\spobp\lTo^{\pr_2}(\spoba\times\spobp)$
\\
and the fragment $\sparra\pile{\rTo \\  \rTo}\spoba$ is not shown
)
%not shown to avoid clutter)
\end{tabular}
\begin{myeq}{eqmmgetP}
%	\eqmmgetP  % was a macro but now is a direct encoding below
	\begin{array}{| l@{\quad}l |}
	\hline
	\multicolumn{2}{|l|}{
		\mbox{Definition of learning $\get$  machine (over given $\get_{00}$)}} 
	\\ [3pt]
	%\mbox{Input alphabet is $\spA_1$} &\\
	\text{(PB1)} &	\Inget \eqdef\compr{(u,e,p,A)}{\so(u)=A, \so(e)=p}  
	\\
	\text{(PB2)}  & \Outget\eqdef\compr{(e,p,A,v)}{(A, p).\get_{00} =\ta(v)} 
		\\ [3pt]
	\multicolumn{2}{|l|}{
		\mbox{Equational Laws: }}
	\\ [3pt]
	\text{ (Inc) }&\get_0.\ogbi.\so=(\igao,\igpo).\get_{00} 
	\\
	\text{ (Nat) }	&	(u,e,p,A).\get =(\id_A,e,p,A).\get~; (u,p,A).\get_0 \\
	& \hspace{6.25em}= (u,p',A).\get_0~; (\id_{A'},e, p', A').\get  
\\
	\text{ (GetId)}_A	&	(\id_p,u, A,p).\get.\ogbi=(u,A,p).\get_0
	\\
	\text{ (GetGet)}_A &			(e;e', \id_A, A, p).\get.\ogbi= \\
	&	\hspace{5em} =(e,\id_A,A,p).\get.\ogbi ; (e',\id_A, A, p').\get.\ogbi 
	\\ [3pt]
	\text{}	&		\Inget_0=\compr{(u,A,p)}{\so(u)=A}  
%	\\
%	\text{ (GetOk)}_p &	\get_0.(\ogao, \ogpo).\pr=\igai.\ta  
	\\
	\text{ (GetId)}_p &		(\id_A, A,p).\get_0.\ogbi=\id_{(A,p).\get_{00}}  
	\\
	\text{ (GetGet)}_p  &			(u;u', A, p).\get_0.\ogi=(u,A,p).\get_0.\ogbi ; (u',A',p).\get_0.\ogbi \\ [3pt]
	\hline
\end{array}
\end{myeq}
\begin{myeq}{eqmmputP}
%	\eqmmputP
%	\eqmmgetP  % was a macro but now is a direct encoding below
	\begin{array}{|ll|}
	\hline
	\multicolumn{2}{|c|}{
		\mbox{Definition of learning $\putl$ machine (over given $\get_{00}$ )}}
	\\ [3pt]
	\Input=\compr{(A,p,v)}{(A,p).\get_{00}=\so(v)} &\\
	\Output=\compr{(e,u,A,p)}{\ta(e)=p, \ta(u)=A} &\\
	\putl.\opi.\so=\ipo &\text{ (Inc.)}\\
	%		    \putl.\opi.\ta.\get_0=\ipi.\ta   \text{ (Putget for objects)  }  &\\
	%\putl.\opo=\putl.\opi.\ta  \text{ (state update) }&\\ 		[3pt]
	%		\mbox{\putgetlaw{} law:~} &\nonumber\\
	\putl.\opo.\get_0 =\ipi.\ta & \text{ (PutOk) }\\
	(A, \id_{A.\get_0}).\putl.\opi=\id_{A}  &\text{ (PutId) } \\
	\textcolor{red}{(A, v;v').\putl.\opi=(A,v).\putl.\opi ; (A',v').\putl.\opi} &\textcolor{red}{~~ (PutPut) } \\
	\hline
\end{array}	
\end{myeq}
%
\begin{myeq}{eqmmputget}
%	\fbox{\putgetlaw{} law:~ $\putl.\oiiso.\get.\ogbi~=~\ipbi$} 
	\begin{array}{|l@{~~}l|}
	\hline
	\mbox{\putgetlaw{} law:~} &\\
	\oiiso(u,e,A',p') \eqdef(u,e,A,p) &\\
	\putl.\oiiso.\get.\ogbi =\ipbi &\\
	\hline
	\end{array}
\end{myeq}
	\caption{Categorically learning asymmetric lens as a special Mealy machine couple: the two common state spaces are $S_0=\spA_0\timm\spP_0$ and $S_1=S_0\timm\spP_1$}
\label{fig:al-lens-mealy}
%\end{wrapfigure}
\end{figure}

==> ll-figures/diags/al-lens-as-mealy-read.tex <==
\begin{figure}
	%	\begin{wrapfigure}{R}{0.5\columnwidth}
	%		\vspace{-0.5cm}
	\centering
	\begin{tabular}{l}%@{\quad}l}
\begin{diagram}%[small]
% -------------------------------> row 1
&&\Ingetread&&&&
\pile{
	\rTo^{\hspace{3em}\get^\readd} 
	\\ 
	\rTo_{\hspace{3em}\get^\readd_0} } % end pile 
&&&&	
\Outgetread &&
\\ %%%%%%%%------- ---> row 2 
%\dTo<{\igai}
%DIAGONALS
          & \ldTo>{\igai}
          &&\rdTo(2,2)<{\igpi} 
          \rdDashto(4,2)~{\igpo}
           \rdTo(6,2)^{\igao}
          &&& %\puncture 
          &&&  
          \ldTo(6,2)^{\ogpi} 
          \ldDashto(4,2)_{
          \begin{array}{c}
          	\\ [-17.5pt]
          	\ogpo
          	\\
          \pmb{\puncture}
          \end{array}
          }  %
           \ldTo(2,2)~{\ogao} 
          &&\rdTo>{\ogbi}
\\ %%%%%%%%%%%%%-----------> row 3 for the asymmetric case
%\uDashto<{\oiiso}
\sparra &&
\uDashto~{\oiiso}
&&	\sparrp
	& \pile{\rTo^{\hspace{3em}_\ta} 
		%\\  %\rTo_{\qquad^\so}
	}
	&\spobp&{\times\qquad\quad}
	& \begin{array}{c}
%		\smash{\puncture}
%		\\ %[3pt]
		\spoba)
	\end{array}
	 &\rTo^{~~\get_{00}}_{\text{~~from$\timm$}}%\spobR&\rTo_{b}
	&\spobb
	&
	\pile{\lTo~{_\ta} \\  \lTo~{_\so}} % pile end
	&\sparrb
	&
\\ %%%%%%%%% -------------========> ROW 4 DIAGONALS 
&\luTo<{\opai}
	&&\ruTo(2,2)<{\oppi}
	&&\luTo(6,2)_{\ippi}
	%&
	\ruDashto(4,2)~{\oppo}
	& 
	&\luDashto(4,2)~{\ippo}
	\ruTo(6,2) _{\opao}
	&&\luTo(2,2)~{\ipao}
	&
	&
	\ruTo>{\ipbi} %\luTo(1,2)>{\ipi} &
\\%  --------------------------------------------->row 5
&&\Output&&&&
\pile{\lTo^{\hspace{1.5em}\putl_0} \\ \lTo_{\hspace{1.5em}\putl} }
&&&&	\Input &&
\\
&&&& &&&& &&&&
\end{diagram}
%\\ [30pt]
\\ [25pt]
(to avoid clutter,  
the fragment $\sparrp\pile{\rTo \\  \rTo}\spobp$ is used a shorthand for 
$\sparrp\pile{\rTo \\  \rTo}\spobp\lTo^{\pr_2}(\spoba\times\spobp)$
\\
and the fragment $\sparra\pile{\rTo \\  \rTo}\spoba$ is not shown
)
%not shown to avoid clutter)
\end{tabular}
\begin{myeq}{eqmmgetP}
%	\eqmmgetP  % was a macro but now is a direct encoding below
	\begin{array}{| l@{\quad}l |}
	\hline
	\multicolumn{2}{|l|}{
		\mbox{Definition of the learning $\get^\readd$  machine (over given $\get_{00}$)}} 
	\\ [3pt]
	%\mbox{Input alphabet is $\spA_1$} &\\
	\text{(PB1)} &	\Ingetread \eqdef\compr{(u,e,p,A)}{\so(u)=A, \ta(e)=p}  
	\\
	\text{(PB2)}  & \Outgetread\eqdef\compr{(e,p,A,v)}{p=\ta(e), (A, p).\get_{00} =\ta(v)} 
		\\ [3pt]
	\multicolumn{2}{|l|}{
		\mbox{Equational Laws: }}
	\\ [3pt]
		\text{ (ReadOnly)$_1$ }&\get^\readd.\ogpi=\igpi
	\\
		\text{ (ReadOnly)$_0$ }&\get^\readd.\ogpo=\igpo
	\\
	\text{ (Inc) }&\get^\readd_0.\ogbi.\so=(\igao,\igpo).\get_{00} 
	\\
	\text{ (Nat) }	&	(u,e,p,A).\get^\readd =(\id_A,e,p,A).\get~; (u,p,A).\get_0 \\
	& \hspace{6.25em}= (u,p',A).\get_0~; (\id_{A'},e, p', A').\get  
\\
	\text{ (GetId)}_A	&	(\id_p,u, A,p).\get.\ogbi=(u,A,p).\get_0
	\\
	\text{ (GetGet)}_A &			(e;e', \id_A, A, p).\get.\ogbi= \\
	&	\hspace{5em} =(e,\id_A,A,p).\get.\ogbi ; (e',\id_A, A, p').\get.\ogbi 
	\\ [3pt]
	\text{}	&		\Inget_0=\compr{(u,A,p)}{\so(u)=A}  
%	\\
%	\text{ (GetOk)}_p &	\get_0.(\ogao, \ogpo).\pr=\igai.\ta  
	\\
	\text{ (GetId)}_p &		(\id_A, A,p).\get_0.\ogbi=\id_{(A,p).\get_{00}}  
	\\
	\text{ (GetGet)}_p  &			(u;u', A, p).\get_0.\ogi=(u,A,p).\get_0.\ogbi ; (u',A',p).\get_0.\ogbi \\ [3pt]
	\hline
\end{array}
\end{myeq}
\begin{myeq}{eqmmputP}
%	\eqmmputP
%	\eqmmgetP  % was a macro but now is a direct encoding below
	\begin{array}{|ll|}
	\hline
	\multicolumn{2}{|c|}{
		\mbox{Definition of learning $\putl$ machine (over given $\get_{00}$ )}}
	\\ [3pt]
	\Input=\compr{(A,p,v)}{(A,p).\get_{00}=\so(v)} &\\
	\Output=\compr{(e,u,A,p)}{\ta(e)=p, \ta(u)=A} &\\
	\putl.\opi.\so=\ipo &\text{ (Inc.)}\\
	%		    \putl.\opi.\ta.\get_0=\ipi.\ta   \text{ (Putget for objects)  }  &\\
	%\putl.\opo=\putl.\opi.\ta  \text{ (state update) }&\\ 		[3pt]
	%		\mbox{\putgetlaw{} law:~} &\nonumber\\
	\putl.\opo.\get_0 =\ipi.\ta & \text{ (PutOk) }\\
	(A, \id_{A.\get_0}).\putl.\opi=\id_{A}  &\text{ (PutId) } \\
	\textcolor{red}{(A, v;v').\putl.\opi=(A,v).\putl.\opi ; (A',v').\putl.\opi} &\textcolor{red}{~~ (PutPut) } \\
	\hline
\end{array}	
\end{myeq}
%
\begin{myeq}{eqmmputget}
%	\fbox{\putgetlaw{} law:~ $\putl.\oiiso.\get.\ogbi~=~\ipbi$} 
	\begin{array}{|l@{~~}l|}
	\hline
	\mbox{\putgetlaw{} law:~} &\\
	\oiiso(u,e,A',p') \eqdef(u,e,A,p) &\\
	\putl.\oiiso.\get.\ogbi =\ipbi &\\
	\hline
	\end{array}
\end{myeq}
	\caption{Categorically learning asymmetric lens as a special Mealy machine couple: the two common state spaces are $S_0=\spA_0\timm\spP_0$ and $S_1=S_0\timm\spP_1$}
\label{fig:al-lens-mealy}
%\end{wrapfigure}
\end{figure}

==> ll-figures/diags/al-lens-as-mealy-twoPuts.tex <==
{%\renewcommand\app{{}}
\begin{figure}
	%	\begin{wrapfigure}{R}{0.5\columnwidth}
	%		\vspace{-0.5cm}
	\centering
	\begin{tabular}{l}%@{\quad}l}
\begin{diagram}[w=2.5em,h=2.5em]%[small]
% -------------------------------> row 1
%\Inget&\rEQ&
&&\Inget&&&&
\rTo^{\get} % = \{ \get^\readd\orr\get^\app\}  }
%	begin{\cases}
%	\get^\app\\ 
%	\get^\readd 
%	\end{cases} 
%}
%\pile{
%	\rTo^{\hspace{0em}\get^\app}%_{\footnotesize{\orr}} 
%%	\\ 
%%	\rTo~{\get=%\left\{ \right.
%%		\hspace{4em} }
%		\\
%	\rTo_{\hspace{0em}\get^\readd}
% } % end pile 
&&&&	
\Outget &&
\\ %%%%%%%%------- ---> row 2 
%\dTo<{\igai}
%DIAGONALS
          & \ldTo(2,2)^{\igai} \ruDotto(2,4) ~{\oisim}%\ldTo>{\igai}
          & \dTo~{\igpi} %&\rdTo(2,2)<{\igpi} 
          &
          \rdTo(2,2)~{\igpo}
           \rdTo(6,2)^{\igao}
          &&& %\pmb{\puncture} 
          &&&  
          \ldDertoda(8,2)^{~\ogpi} 
          \ldDertoda(6,2)~{\ogpo
%          	\begin{array}{c}
%          		\\ [-17.5pt]
%          		\ogpo
%          		\\
%          		\pmb{\puncture}
%          	\end{array}
}
        %    	\ogpo}  %
           \ldDertoda(2,2)~{\ogao} 
          &&\rdTo>{\ogbi}
\\ %%%%%%%%%%%%%-----------> row 3 for the asymmetric case
%\uDashto<{\oiiso}
\sparra &&
\ppi %\uDashto~{\oiiso}
&
  \pile{%\rTo^{\qquad_\ta} 
	%\rTo^{\hspace{3em}_\so}
	\rTo%~{\so}
	\\
	%       \lDashto
	%       \\
	%	\rTo_{\hspace{3em}^\ta}
	\rTo%~{\ta} 
}
& \po %	\sparrp
&   \lTo~\pr 
%\pile{%\rTo^{\qquad_\ta} 
%	%\rTo^{\hspace{3em}_\so}
%		\rTo%~{\so}
%       \\
%%       \lDashto
%%       \\
%       %	\rTo_{\hspace{3em}^\ta}
%       	\rTo%~{\ta} 
%}
& (\po %{\lefteqn{\hspace{2.5em}\times}}}
%	\begin{array}{c}
%%		\smash{\pmb{\puncture}}
%%		\\
%	\spobp
%\end{array}
	&{\times\hspace{0em}
	}&
\stackrel{\puncture}{\spoba)}
	 &\rTo^{~~\get_{00}}_{\text{~~from$\timm$}}%\spobR&\rTo_{b}
	&\spobb
	&
	\pile{\lTo~{_\ta} \\  \lTo~{_\so}} % pile end
	&\sparrb
	&
\\ %%%%%%%%% -------------========> ROW 4 DIAGONALS 
\uTo<{\opai} &    %\luTo<{\opai}
	& %\ruImplies(2,2)<{_{\oppi^\sim}}_{^\oppi}
%\color{blue} 
\uTo<{\oppi^\sim}\uDertodo~{\oppi}
    &
	%&&
	\luTo(8,2)_{\ippi}
	%&&
	\ruDertodo(2,2)~{\oppo}
	&& 
	\luTo(6,2)~{\ippo}
	&&
	\ruDertodo(6,2) _{\opao}
	&&\luTo(2,2)~{\ipao}
	&
	&
	\ruTo>{\ipbi} %\luTo(1,2)>{\ipi} &
\\%  --------------------------------------------->row 5
\Output&\rEQ&\Output&&&&
%\pile{\lTo^{\hspace{0em}\putl_0} \\ \lTo_{\hspace{0em}\putl} }
\lTo_{\putl}
&&&&	\Input &&
\\
&&&& &&&& &&&&
\end{diagram}
%\\ [30pt]
\\ [25pt]
(to avoid clutter,  
%the fragment $\sparrp\pile{\rTo \\  \rTo}\spobp$ is used a shorthand for $\sparrp\pile{\rTo \\  \rTo}\spobp\lTo^{\pr_2}(\spoba\times\spobp)$
%\\ and 
the fragment $\sparra\pile{\rTo \\  \rTo}\spoba$ is not shown
)
%not shown to avoid clutter)
\end{tabular}
\begin{myeq}{eqmmgetP}
	%	\eqmmgetP  % was a macro but now is a direct encoding below
	\begin{array}{| l@{\quad}l |}
		\hline
		\multicolumn{2}{|l|}{
			\mbox{Definition of a learning $\get$  machine over given \spabpgetoo: }} 
		\\ [3pt]
		\text{(Alphabets)} &	\ainx{\get}=\sparra, \aoutx{\get}=\sparrb,
		\\ 
			\text{(State space)} &\stt^\get=\paoios\eqdef\pois\timm\ao 
			%\\	& \phantom{\stt^\get}
			\cong \apoois\eqdef\ao\timm\pois
			%= (\po\timm_\so\ppi)\timm\ao
			%\pois\timm\ao\sqcup\poit\timm\ao~
			%\cong~\ao\timm\poit\sqcup\ao\timm\pois
		\\
		%\mbox{Input alphabet is $\spA_1$} &\\
		\text{(Eff. Input)} &	\Inget = \pois\timm\aois %\sqcup\poit\timm\aois
		\\
		\text{(Eff. Output)} & \Outget =\spB_1~{}_\ta\timm_\param~ \stt^\get
		             = \bapioot ~{}_\param\timm_\so~\ppi
		            \\
		           & \phantom{\Outget }= \compr{(v,A',p',e')}{(A',p',v)\models\gethit~\&~p'=e'.\so}
		            \\
		            & \phantom{\Outget }= \compr{(v,A',p',e')}{A'.\get_{00}(p')=v.\ta ~\&~ p'=e'.\so}
		         		\\ [3pt]
		\multicolumn{2}{|l|}{
					\mbox{Equational Laws (to hold for any $(p,e,A,u)\in\Inget$) %...
					
						%$p\in\po$, $A \in\ao$, $e\inn\ppi,u\inn\ai$ such that $p=e^\so \text{ or } p=e^\ta$, $A=u^\so$
}} 	\\ %[5pt]
			\multicolumn{2}{|l|}{\mbox{Basic (in addition to \gethit):}}
\\
		\text{ (Incidence)}%_{(A,u)\in\Inget} 
		& (p,e,A,u).\get.\ogbi.\so= A.\get_{00}(p) 
		% the arrow version (\get^\readd.\ogbi.\so= \igao.\get_{0}) 
		\\
		\text{ (Increm)}_{\ao} 
		&	(p,e,A,u).\get.\ogao=u.\ta ~~(= A' \text{ in Eff. Output})
		\\
				\text{ (Increm)}_{\po} 
		&	(p,e,A,u).\get.\ogpo=e.\ta~~ (=p' \text{ in Eff. Output})
			\\
		\text{ (Increm)}_{\ppi} 
		&	(p,e,A,u).\get.\ogpi=\id_{e.\ta}~~  (=e' \text{ in Eff. Output})
%		\begin{cases}
%			e, \text{ if } p=e^\so,\\
%			id_{e^\ta} \textit{ if } p=e^\ta
%		\end{cases}
%		\\
%				\text{ (histIgnore)}
%		&	(p,e1,A,u).\get.\ogbi=(p,e2,A,u).\get.\ogbi\ 
%		\\
%		&\text{ for any $e1 \neq e2$ as soon as $e1^\ta = e2^\ta = p$}
%		\\
%	\text{ (Nat) }	&	(u,e,p,A).\get =(\id_A,e,p,A).\get~; (u,p,A).\get_{00} \\
%	& \hspace{6.25em}= (u,p',A).\get_0~; (\id_{A'},e, p', A').\get  
		\\[2.5pt]
			\multicolumn{2}{|l|}{\mbox{Monoidal (to hold for any \frar{e1}{e.\ta}{\_}, \frar{u1}{u.\ta}{\_})  )}:}
		\\
		\text{ (GetId)}%_A	
		& 			(p,\id_p,A,\id_A).\get.\ogbi=\id_{A.\get(p)} 
		%(u, A).\get.\ogbi=(u,A).\get_0
		\\
		\text{ (GetGet)}%_{(u^\ta,u')\in\Inget} 
		&	(p,e;e1, A,u;u1).\get.\ogbi        =         (p,e,A,u).\get.\ogbi ; 
		\\ 	 & \phantom{(p,e;e', A,u;u').\get.\ogbi=} 
		(e.\ta, e1, u.\ta,u1).\get.\ogbi
		\\ [3pt]
		\hline
	\end{array}
\end{myeq}
%  --- NOW PUT
\begin{myeq}{eqmmputP}
	%	\eqmmgetP  % was a macro but now is a direct encoding below
	\begin{array}{| l@{\quad}l |}
		\hline
		\multicolumn{2}{|l|}{
			\mbox{Definition of a learning $\putl$  machine over given \spabpgetoo: }} 
		\\ [3pt]
		\text{(Alphabets)} &	\ain^\putl=\bi, \aout^\putl=\ai,
		\\ 
		\text{(State space)} &\stt^\putl=\stt^\get %= \paoios\eqdef\pois\timm\ao 
	%\\ & 
	\phantom{\stt^\get}\cong \apoois\eqdef\ao\timm\pois
				\\
		\text{(Eff.Input)} & \Input =\stt^\putl{}_\param\timm_\so~ \spB_1
		%= \abpoos ~{}_\param\timm_\so~\ppi
			%\\ 	& \phantom{\Input }
			= \compr{(A,p,e,v)}{A.\get_{00}(p)=v.\so ~\&~ p=e.\so}
					\\
		\text{(Eff.Output)} &	\Output =\spA_1\timm\spP_1\timm\stt^\putl =
		   \\
		   		   	& %\phantom{\Output }
		   		   	= \compr{(u,e^\sim,e', A',p')}{(u,e',A',p')\models \text{(Incr)}_{\ao,\po,\ppi}
		   		     ~\&~p'=e'.\so}
		   \\
		   	& %\phantom{\Output }
		   	= \compr{(u,e^\sim,e', A',p')}%
		   	    {A'=u.\ta,\; p'= e^\sim.\ta,\; e'=\id_{e.\ta}~\&~p'=e'.\so}
		   	\\ [4pt]
		\multicolumn{2}{|l|}{
			\mbox{Equational Laws (to hold for any $(p,e,A,v)\in\Inget$)
				%$p\in\po$, $A \in\ao$, $e\inn\ppi,u\inn\ai$ such that $p=e^\so \text{ or } p=e^\ta$, $A=u^\so$
		}} 
		\\ [2.5pt]
		\text{ (Incidence)}%_{(A,u)\in\Inget} 
		& (p,e,A,u).\get.\ogbi.\so= A.\get_{00}(p) 
		% the arrow version (\get^\readd.\ogbi.\so= \igao.\get_{0}) 
%		\\
%		\text{ (Increm)}_{\ao} 
%		&	(p,e,A,u).\get.\ogao=u.\ta ~~(= A' \text{ in Eff. Output})
%		\\
%		\text{ (Increm)}_{\po} 
%		&	(p,e,A,u).\get.\ogpo=e.\ta~~ (=p' \text{ in Eff. Output})
%		\\
%		\text{ (Increm)}_{\ppi} 
%		&	(p,e,A,u).\get.\ogpi=\id_{e.\ta}~~  (=e' \text{ in Eff. Output})
          \\
          \text{ (PutHit)}
          & (A,p,e,v).\putl.\opao.\get_{00}(\oppo)=\ipbi.\ta~~ (\text{a.k.a. (PutGet)$_0$ law})
			\\[2.5pt]
			\multicolumn{2}{|l|}{
			\mbox{ (Unitality (a.k.a Stability) %any \frar{e1}{e.\ta}{\_}, \frar{u1}{u.\ta}{\_})   
		               }}
		\\
		\text{ (PutId)}%_A	
		& 			(p,\id_p,A,\id_A).\get.\ogbi=\id_{A.\get(p)} 
		%(u, A).\get.\ogbi=(u,A).\get_0
		\\ [3pt]
		\hline
	\end{array}
\end{myeq}
%
%\begin{myeq}{eqmmputP}
%%	\eqmmputP
%%	\eqmmgetP  % was a macro but now is a direct encoding below
%	\begin{array}{|ll|}
%	\hline
%	\multicolumn{2}{|c|}{
%		\mbox{Definition of a parametrized $\putl$ machine over given \spabpgetoo}}
%	\\ [3pt]
%			\text{(Alphabets)} & \ain^\putl=\bi, \aout^\putl=\ai,
%			\stt^\putl
%	\\ 
%	\Input=\compr{(A,p,v)}{(A,p).\get_{00}=\so(v)} &\\
%	\Output=\compr{(e,u,A,p)}{\ta(e)=p, \ta(u)=A} &\\
%	\putl.\opi.\so=\ipo &\text{ (Inc.)}\\
%	%		    \putl.\opi.\ta.\get_0=\ipi.\ta   \text{ (Putget for objects)  }  &\\
%	%\putl.\opo=\putl.\opi.\ta  \text{ (state update) }&\\ 		[3pt]
%	%		\mbox{\putgetlaw{} law:~} &\nonumber\\
%	\putl.\opo.\get_0 =\ipi.\ta & \text{ (PutOk) }\\
%	(A, \id_{A.\get_0}).\putl.\opi=\id_{A}  &\text{ (PutId) } \\
%	\textcolor{red}{(A, v;v').\putl.\opi=(A,v).\putl.\opi ; (A',v').\putl.\opi} &\textcolor{red}{~~ (PutPut) } \\
%	\hline
%\end{array}	
%\end{myeq}
%%
\begin{myeq}{eqmmputget}
	\begin{array}{|ll|}
		\hline
		\multicolumn{2}{|l|}{
			\mbox{Definition of a coupled $(\putl,\get)$-machine (a lens) over given \spabpgetoo}}
		\\ [3pt]
		\multicolumn{2}{|l|}{\mbox{Basic equational Law (to hold for any $(A,p)\inn\spA_0\timm\spP_0$ and \frar{v}{A.\get_{00}(p)}{\_}):  }}
		\\ [3pt]	
		\text{(Def. of \oisim) } & \oisim(u,e^\sim, e',u.\ta, e^\sim.\ta) = (e^\sim.\so, e,u.\so, u) 
		\\
		\text{(PutGet)}%_{(A,v)\in\Input} 
		& (A,p,e,v).\putl.\oisim.\get.\ogbi=v ~~(\text{or } \putl.\oisim.\get.\ogbi=\ipbi)
		\\ \hline
	\end{array}
\end{myeq}
	\caption{NEW Definition of an asymmetric coupled \mema\ with learning}
\label{fig:al-lensmm}
%\end{wrapfigure}
\end{figure}
} % end renew command for \app=idle

==> ll-figures/diags/al-lens-as-mealy-twoState.tex <==
{%\renewcommand\app{{}}
\begin{figure}
	%	\begin{wrapfigure}{R}{0.5\columnwidth}
	%		\vspace{-0.5cm}
	\centering
	\begin{tabular}{l}%@{\quad}l}
\begin{diagram}[w=2.5em,h=2.5em]%[small]
% -------------------------------> row 1
%\Inget&\rEQ&
&&\Inget&&&&
\rTo^{\get} % = \{ \get^\readd\orr\get^\app\}  }
%	begin{\cases}
%	\get^\app\\ 
%	\get^\readd 
%	\end{cases} 
%}
%\pile{
%	\rTo^{\hspace{0em}\get^\app}%_{\footnotesize{\orr}} 
%%	\\ 
%%	\rTo~{\get=%\left\{ \right.
%%		\hspace{4em} }
%		\\
%	\rTo_{\hspace{0em}\get^\readd}
% } % end pile 
&&&&	
\Outget &&
\\ %%%%%%%%------- ---> row 2 
%\dTo<{\igai}
%DIAGONALS
          & \ldTo(2,2)^{\igai} \ruDotto(2,4) ~{\oisim}%\ldTo>{\igai}
          & \dTo~{\igpi} %&\rdTo(2,2)<{\igpi} 
          &
          \rdTo(2,2)~{\igpo}
           \rdTo(6,2)^{\igao}
          &&& %\pmb{\puncture} 
          &&&  
          \ldDertoda(8,2)^{~\ogpi} 
          \ldDertoda(6,2)~{\ogpo
%          	\begin{array}{c}
%          		\\ [-17.5pt]
%          		\ogpo
%          		\\
%          		\pmb{\puncture}
%          	\end{array}
}
        %    	\ogpo}  %
           \ldDertoda(2,2)~{\ogao} 
          &&\rdTo>{\ogbi}
\\ %%%%%%%%%%%%%-----------> row 3 for the asymmetric case
%\uDashto<{\oiiso}
\sparra &&
\ppi %\uDashto~{\oiiso}
&
  \pile{%\rTo^{\qquad_\ta} 
	%\rTo^{\hspace{3em}_\so}
	\rTo%~{\so}
	\\
	%       \lDashto
	%       \\
	%	\rTo_{\hspace{3em}^\ta}
	\rTo%~{\ta} 
}
& \po %	\sparrp
&   \lTo~\pr 
%\pile{%\rTo^{\qquad_\ta} 
%	%\rTo^{\hspace{3em}_\so}
%		\rTo%~{\so}
%       \\
%%       \lDashto
%%       \\
%       %	\rTo_{\hspace{3em}^\ta}
%       	\rTo%~{\ta} 
%}
& (\po %{\lefteqn{\hspace{2.5em}\times}}}
%	\begin{array}{c}
%%		\smash{\pmb{\puncture}}
%%		\\
%	\spobp
%\end{array}
	&{\times\hspace{0em}
	}&
\stackrel{\puncture}{\spoba)}
	 &\rTo^{~~\get_{00}}_{\text{~~from$\timm$}}%\spobR&\rTo_{b}
	&\spobb
	&
	\pile{\lTo~{_\ta} \\  \lTo~{_\so}} % pile end
	&\sparrb
	&
\\ %%%%%%%%% -------------========> ROW 4 DIAGONALS 
\uTo<{\opai} &    %\luTo<{\opai}
	& %\ruImplies(2,2)<{_{\oppi^\sim}}_{^\oppi}
%\color{blue} 
\uTo<{\oppi^\sim}\uDertodo~{\oppi}
    &
	%&&
	\luTo(8,2)_{\ippi}
	%&&
	\ruDertodo(2,2)~{\oppo}
	&& 
	\luTo(6,2)~{\ippo}
	&&
	\ruDertodo(6,2) _{\opao}
	&&\luTo(2,2)~{\ipao}
	&
	&
	\ruTo>{\ipbi} %\luTo(1,2)>{\ipi} &
\\%  --------------------------------------------->row 5
\Output&\rEQ&\Output&&&&
%\pile{\lTo^{\hspace{0em}\putl_0} \\ \lTo_{\hspace{0em}\putl} }
\lTo_{\putl}
&&&&	\Input &&
\\
&&&& &&&& &&&&
\end{diagram}
%\\ [30pt]
\\ [25pt]
(to avoid clutter,  
%the fragment $\sparrp\pile{\rTo \\  \rTo}\spobp$ is used a shorthand for $\sparrp\pile{\rTo \\  \rTo}\spobp\lTo^{\pr_2}(\spoba\times\spobp)$
%\\ and 
the fragment $\sparra\pile{\rTo \\  \rTo}\spoba$ is not shown
)
%not shown to avoid clutter)
\end{tabular}
\begin{myeq}{eqmmgetP}
	%	\eqmmgetP  % was a macro but now is a direct encoding below
	\begin{array}{| l@{\quad}l |}
		\hline
		\multicolumn{2}{|l|}{
			\mbox{Definition of a learning $\get$  machine over given \spabpgetoo: }} 
		\\ [3pt]
		\text{(Alphabets)} &	\ainx{\get}=\sparra, \aoutx{\get}=\sparrb,
		\\ 
			\text{(State space)} &\stt^\get=\paoios\eqdef\pois\timm\ao 
			%\\	& \phantom{\stt^\get}
			\cong \apoois\eqdef\ao\timm\pois
			%= (\po\timm_\so\ppi)\timm\ao
			%\pois\timm\ao\sqcup\poit\timm\ao~
			%\cong~\ao\timm\poit\sqcup\ao\timm\pois
		\\
		%\mbox{Input alphabet is $\spA_1$} &\\
		\text{(Eff. Input)} &	\Inget = \pois\timm\aois %\sqcup\poit\timm\aois
		\\
		\text{(Eff. Output)} & \Outget =\spB_1~{}_\ta\timm_\param~ \stt^\get
		             = \bapioot ~{}_\param\timm_\so~\ppi
		            \\
		           & \phantom{\Outget }= \compr{(v,A',p',e')}{(A',p',v)\models\gethit~\&~p'=e'.\so}
		            \\
		            & \phantom{\Outget }= \compr{(v,A',p',e')}{A'.\get_{00}(p')=v.\ta ~\&~ p'=e'.\so}
		         		\\ [3pt]
		\multicolumn{2}{|l|}{
					\mbox{Equational Laws (to hold for any $(p,e,A,u)\in\Inget$) %...
					
						%$p\in\po$, $A \in\ao$, $e\inn\ppi,u\inn\ai$ such that $p=e^\so \text{ or } p=e^\ta$, $A=u^\so$
}} 	\\ %[5pt]
			\multicolumn{2}{|l|}{\mbox{Basic (in addition to \gethit):}}
\\
		\text{ (Incidence)}%_{(A,u)\in\Inget} 
		& (p,e,A,u).\get.\ogbi.\so= A.\get_{00}(p) 
		% the arrow version (\get^\readd.\ogbi.\so= \igao.\get_{0}) 
		\\
		\text{ (Increm)}_{\ao} 
		&	(p,e,A,u).\get.\ogao=u.\ta ~~(= A' \text{ in Eff. Output})
		\\
				\text{ (Increm)}_{\po} 
		&	(p,e,A,u).\get.\ogpo=e.\ta~~ (=p' \text{ in Eff. Output})
			\\
		\text{ (Increm)}_{\ppi} 
		&	(p,e,A,u).\get.\ogpi=\id_{e.\ta}~~  (=e' \text{ in Eff. Output})
%		\begin{cases}
%			e, \text{ if } p=e^\so,\\
%			id_{e^\ta} \textit{ if } p=e^\ta
%		\end{cases}
%		\\
%				\text{ (histIgnore)}
%		&	(p,e1,A,u).\get.\ogbi=(p,e2,A,u).\get.\ogbi\ 
%		\\
%		&\text{ for any $e1 \neq e2$ as soon as $e1^\ta = e2^\ta = p$}
%		\\
%	\text{ (Nat) }	&	(u,e,p,A).\get =(\id_A,e,p,A).\get~; (u,p,A).\get_{00} \\
%	& \hspace{6.25em}= (u,p',A).\get_0~; (\id_{A'},e, p', A').\get  
		\\[2.5pt]
			\multicolumn{2}{|l|}{\mbox{Monoidal (to hold for any \frar{e1}{e.\ta}{\_}, \frar{u1}{u.\ta}{\_})  )}:}
		\\
		\text{ (GetId)}%_A	
		& 			(p,\id_p,A,\id_A).\get.\ogbi=\id_{A.\get(p)} 
		%(u, A).\get.\ogbi=(u,A).\get_0
		\\
		\text{ (GetGet)}%_{(u^\ta,u')\in\Inget} 
		&	(p,e;e1, A,u;u1).\get.\ogbi        =         (p,e,A,u).\get.\ogbi ; 
		\\ 	 & \phantom{(p,e;e', A,u;u').\get.\ogbi=} 
		(e.\ta, e1, u.\ta,u1).\get.\ogbi
		\\ [3pt]
		\hline
	\end{array}
\end{myeq}
%  --- NOW PUT
\begin{myeq}{eqmmputP}
	%	\eqmmgetP  % was a macro but now is a direct encoding below
	\begin{array}{| l@{\quad}l |}
		\hline
		\multicolumn{2}{|l|}{
			\mbox{Definition of a learning $\putl$  machine over given \spabpgetoo: }} 
		\\ [3pt]
		\text{(Alphabets)} &	\ain^\putl=\bi, \aout^\putl=\ai,
		\\ 
		\text{(State space)} &\stt^\putl=\stt^\get %= \paoios\eqdef\pois\timm\ao 
	%\\ & 
	\phantom{\stt^\get}\cong \apoois\eqdef\ao\timm\pois
				\\
		\text{(Eff.Input)} & \Input =\stt^\putl{}_\param\timm_\so~ \spB_1
		%= \abpoos ~{}_\param\timm_\so~\ppi
			%\\ 	& \phantom{\Input }
			= \compr{(A,p,e,v)}{A.\get_{00}(p)=v.\so ~\&~ p=e.\so}
					\\
		\text{(Eff.Output)} &	\Output =\spA_1\timm\spP_1\timm\stt^\putl =
		   \\
		   		   	& %\phantom{\Output }
		   		   	= \compr{(u,e^\sim,e', A',p')}{(u,e',A',p')\models \text{(Incr)}_{\ao,\po,\ppi}
		   		     ~\&~p'=e'.\so}
		   \\
		   	& %\phantom{\Output }
		   	= \compr{(u,e^\sim,e', A',p')}%
		   	    {A'=u.\ta,\; p'= e^\sim.\ta,\; e'=\id_{e.\ta}~\&~p'=e'.\so}
		   	\\ [4pt]
		\multicolumn{2}{|l|}{
			\mbox{Equational Laws (to hold for any $(p,e,A,v)\in\Inget$)
				%$p\in\po$, $A \in\ao$, $e\inn\ppi,u\inn\ai$ such that $p=e^\so \text{ or } p=e^\ta$, $A=u^\so$
		}} 
		\\ [2.5pt]
		\text{ (Incidence)}%_{(A,u)\in\Inget} 
		& (p,e,A,u).\get.\ogbi.\so= A.\get_{00}(p) 
		% the arrow version (\get^\readd.\ogbi.\so= \igao.\get_{0}) 
%		\\
%		\text{ (Increm)}_{\ao} 
%		&	(p,e,A,u).\get.\ogao=u.\ta ~~(= A' \text{ in Eff. Output})
%		\\
%		\text{ (Increm)}_{\po} 
%		&	(p,e,A,u).\get.\ogpo=e.\ta~~ (=p' \text{ in Eff. Output})
%		\\
%		\text{ (Increm)}_{\ppi} 
%		&	(p,e,A,u).\get.\ogpi=\id_{e.\ta}~~  (=e' \text{ in Eff. Output})
          \\
          \text{ (PutHit)}
          & (A,p,e,v).\putl.\opao.\get_{00}(\oppo)=\ipbi.\ta~~ (\text{a.k.a. (PutGet)$_0$ law})
			\\[2.5pt]
			\multicolumn{2}{|l|}{
			\mbox{ (Unitality (a.k.a Stability) %any \frar{e1}{e.\ta}{\_}, \frar{u1}{u.\ta}{\_})   
		               }}
		\\
		\text{ (PutId)}%_A	
		& 			(p,\id_p,A,\id_A).\get.\ogbi=\id_{A.\get(p)} 
		%(u, A).\get.\ogbi=(u,A).\get_0
		\\ [3pt]
		\hline
	\end{array}
\end{myeq}
%
%\begin{myeq}{eqmmputP}
%%	\eqmmputP
%%	\eqmmgetP  % was a macro but now is a direct encoding below
%	\begin{array}{|ll|}
%	\hline
%	\multicolumn{2}{|c|}{
%		\mbox{Definition of a parametrized $\putl$ machine over given \spabpgetoo}}
%	\\ [3pt]
%			\text{(Alphabets)} & \ain^\putl=\bi, \aout^\putl=\ai,
%			\stt^\putl
%	\\ 
%	\Input=\compr{(A,p,v)}{(A,p).\get_{00}=\so(v)} &\\
%	\Output=\compr{(e,u,A,p)}{\ta(e)=p, \ta(u)=A} &\\
%	\putl.\opi.\so=\ipo &\text{ (Inc.)}\\
%	%		    \putl.\opi.\ta.\get_0=\ipi.\ta   \text{ (Putget for objects)  }  &\\
%	%\putl.\opo=\putl.\opi.\ta  \text{ (state update) }&\\ 		[3pt]
%	%		\mbox{\putgetlaw{} law:~} &\nonumber\\
%	\putl.\opo.\get_0 =\ipi.\ta & \text{ (PutOk) }\\
%	(A, \id_{A.\get_0}).\putl.\opi=\id_{A}  &\text{ (PutId) } \\
%	\textcolor{red}{(A, v;v').\putl.\opi=(A,v).\putl.\opi ; (A',v').\putl.\opi} &\textcolor{red}{~~ (PutPut) } \\
%	\hline
%\end{array}	
%\end{myeq}
%%
\begin{myeq}{eqmmputget}
	\begin{array}{|ll|}
		\hline
		\multicolumn{2}{|l|}{
			\mbox{Definition of a coupled $(\putl,\get)$-machine (a lens) over given \spabpgetoo}}
		\\ [3pt]
		\multicolumn{2}{|l|}{\mbox{Basic equational Law (to hold for any $(A,p)\inn\spA_0\timm\spP_0$ and \frar{v}{A.\get_{00}(p)}{\_}):  }}
		\\ [3pt]	
		\text{(Def. of \oisim) } & \oisim(u,e^\sim, e',u.\ta, e^\sim.\ta) = (e^\sim.\so, e,u.\so, u) 
		\\
		\text{(PutGet)}%_{(A,v)\in\Input} 
		& (A,p,e,v).\putl.\oisim.\get.\ogbi=v ~~(\text{or } \putl.\oisim.\get.\ogbi=\ipbi)
		\\ \hline
	\end{array}
\end{myeq}
	\caption{NEW Definition of an asymmetric coupled \mema\ with learning}
\label{fig:al-lensmm}
%\end{wrapfigure}
\end{figure}
} % end renew command for \app=idle

==> ll-figures/diags/al-lens-as-mealy-twoStates.tex <==
{%\renewcommand\app{{}}
\begin{figure}
	%	\begin{wrapfigure}{R}{0.5\columnwidth}
	%		\vspace{-0.5cm}
	\centering
	\begin{tabular}{l}%@{\quad}l}
\begin{diagram}[w=2.5em,h=2.5em]%[small]
% -------------------------------> row 1
%\Inget&\rEQ&
&&\Inget&&&&
\rTo^{\get} % = \{ \get^\readd\orr\get^\app\}  }
%	begin{\cases}
%	\get^\app\\ 
%	\get^\readd 
%	\end{cases} 
%}
%\pile{
%	\rTo^{\hspace{0em}\get^\app}%_{\footnotesize{\orr}} 
%%	\\ 
%%	\rTo~{\get=%\left\{ \right.
%%		\hspace{4em} }
%		\\
%	\rTo_{\hspace{0em}\get^\readd}
% } % end pile 
&&&&	
\Outget &&
\\ %%%%%%%%------- ---> row 2 
%\dTo<{\igai}
%DIAGONALS
          & 
          \ldTo(2,2)^{\igai}
          %\ruDotto(2,4) ~{\oisim}%\ldTo>{\igai}
          &       %\dTo~{\igpi} %&\rdTo(2,2)<{\igpi} 
          &
          \rdTo(2,2)~{\igpi}
          \rdTo(4,2)~{\igpo}
           \rdTo(6,2)^{\igao}
          &&& %\pmb{\puncture} 
          &&&  
          %\ldDertoda(8,2)^{~\ogpi} 
          \ldDertoda(6,2)~{\ogpi
%          	\begin{array}{c}
%          		\\ [-17.5pt]
%          		\ogpo
%          		\\
%          		\pmb{\puncture}
%          	\end{array}
}
        %    	\ogpo}  %
          \ldDertoda(4,2)~{\ogpo} 
           \ldDertoda(2,2)~{\ogao} 
          &&\rdTo>{\ogbi}
\\ %%%%%%%%%%%%%-----------> row 3 for the asymmetric case
%\uDashto<{\oiiso}
\ai%\sparra 
&&
%  \pile{%\rTo^{\qquad_\ta} 
%	%\rTo^{\hspace{3em}_\so}
%	\rTo%~{\so}
%	\\
%	%       \lDashto
%	%       \\
%	%	\rTo_{\hspace{3em}^\ta}
%	\rTo%~{\ta} 
%}
&& \ppi %	\sparrp
&   \timm_{\so{+}\ta}
& (\po %{\lefteqn{\hspace{2.5em}\times}}}
%	\begin{array}{c}
%%		\smash{\pmb{\puncture}}
%%		\\
%	\spobp
%\end{array}
	&{\times\hspace{0em}
	}&
\stackrel{\puncture}{\spoba)}
	 &\rTo^{~~\get_{00}}_{\text{~~from$\timm$}}%\spobR&\rTo_{b}
	&\spobb
	&
	\pile{\lTo~{_\ta} \\  \lTo~{_\so}} % pile end
	&\sparrb
	&
\\ %%%%%%%%% -------------========> ROW 4 DIAGONALS 
& \luTo<{\opai} %&    %\luTo<{\opai}
& %\ruImplies(2,2)<{_{\oppi^\sim}}_{^\oppi}
%\color{blue} 
%\uTo<{\oppi^\sim}
\uDertodo~{\oisim}
    &
	%&&
	%\luTo(8,2)_{\ippi}
	%&&
	\ruDertodo(2,2)~{\oppi}
	&& 
	\luTo(6,2)~{\ippi}
		\ruDertodo(4,2) ~{\oppo}
	&&
	\luTo(4,2)~{\ippo}
	%&
	\ruDertodo(6,2) _{\opao}
	&&\luTo(2,2)~{\ipao}
	&
	&
	\ruTo>{\ipbi} %\luTo(1,2)>{\ipi} &
\\%  --------------------------------------------->row 5
%\Output&\rEQ
&&\Output&&&&
%\pile{\lTo^{\hspace{0em}\putl_0} \\ \lTo_{\hspace{0em}\putl} }
\lTo_{\putl}
&&&&	\Input &&
\\
&&&& &&&& &&&&
\end{diagram}
%\\ [30pt]
\\ [25pt]
(to avoid clutter,  
%the fragment $\sparrp\pile{\rTo \\  \rTo}\spobp$ is used a shorthand for $\sparrp\pile{\rTo \\  \rTo}\spobp\lTo^{\pr_2}(\spoba\times\spobp)$
%\\ and 
the fragment $\sparra\pile{\rTo \\  \rTo}\spoba$ is not shown
)
%not shown to avoid clutter)
\end{tabular}
\begin{myeq}{eqmmgetP}
	%	\eqmmgetP  % was a macro but now is a direct encoding below
	\begin{array}{| l@{\quad}l |}
		\hline
		\multicolumn{2}{|l|}{
			\mbox{Definition of a learning $\get$  machine over given \spabpgetoo: }} 
		\\ [3pt]
		\text{(Alphabets)} & \ainx{\get}=\ai, \aoutx{\get}=\bi,
		\\ 
			\text{(State space)} &
			\stt_\get=\pois\timm\ao \sqcup\poit\timm\ao%
			=\stt_\get^\app\sqcup\stt_\get^\readd
			\\	& \phantom{\stt^\get}
			\cong .... %\apoois\eqdef\ao\timm\pois
			%= (\po\timm_\so\ppi)\timm\ao
			%\pois\timm\ao\sqcup\poit\timm\ao~
			%\cong~\ao\timm\poit\sqcup\ao\timm\pois
		\\
		%\mbox{Input alphabet is $\spA_1$} &\\
		\text{(Eff. Input)} &	\Inget = \pois\timm\aois \sqcup\poit\timm\aois=\Ingetapp\sqcup\Ingetread
		\\
		\text{(Eff. Output)} & \Outget =\bi\timm\stt_\get
		%\spB_1~{}_\ta\timm_\param~ \stt^\get
		            % = \bapioot ~{}_\param\timm_\so~\ppi
		            \\
		           & \phantom{\Outget }= \compr{(v,A',p',e')}{(A',p',v)\models\gethit~\&~p'=e'.\so}
		            \\
		            & \phantom{\Outget }= \compr{(v,A',p',e')}{A'.\get_{00}(p')=v.\ta ~\&~ p'=e'.\so}
		         		\\ [3pt]
		\multicolumn{2}{|l|}{
					\mbox{Equational Laws (to hold for any $(p,e,A,u)\in\Inget$) %...
					
						%$p\in\po$, $A \in\ao$, $e\inn\ppi,u\inn\ai$ such that $p=e^\so \text{ or } p=e^\ta$, $A=u^\so$
}} 	\\ %[5pt]
			\multicolumn{2}{|l|}{\mbox{Basic (in addition to \gethit):}}
\\
		\text{ (Incidence)}%_{(A,u)\in\Inget} 
		& (p,e,A,u).\get.\ogbi.\so= A.\get_{00}(p) 
		% the arrow version (\get^\readd.\ogbi.\so= \igao.\get_{0}) 
		\\
		\text{ (Increm)}_{\ao} 
		&	(p,e,A,u).\get.\ogao=u.\ta ~~(= A' \text{ in Eff. Output})
		\\
				\text{ (Increm)}_{\po} 
		&	(p,e,A,u).\get.\ogpo=e.\ta~~ (=p' \text{ in Eff. Output})
			\\
		\text{ (Increm)}_{\ppi} 
		&	(p,e,A,u).\get.\ogpi=\id_{e.\ta}~~  (=e' \text{ in Eff. Output})
%		\begin{cases}
%			e, \text{ if } p=e^\so,\\
%			id_{e^\ta} \textit{ if } p=e^\ta
%		\end{cases}
		\\
				\text{ (histIgnore)}
		&	(p,e1,A,u).\get.\ogbi=(p,e2,A,u).\get.\ogbi\ 
		\\
		&\text{ for any $e1 \neq e2$ as soon as $e1^\ta = e2^\ta = p$}
%		\\
%	\text{ (Nat) }	&	(u,e,p,A).\get =(\id_A,e,p,A).\get~; (u,p,A).\get_{00} \\
%	& \hspace{6.25em}= (u,p',A).\get_0~; (\id_{A'},e, p', A').\get  
		\\[2.5pt]
			\multicolumn{2}{|l|}{\mbox{Monoidal (to hold for any \frar{e1}{e.\ta}{\_}, \frar{u1}{u.\ta}{\_})  )}:}
		\\
		\text{ (GetId)}%_A	
		& 			(p,\id_p,A,\id_A).\get.\ogbi=\id_{A.\get(p)} 
		%(u, A).\get.\ogbi=(u,A).\get_0
		\\
		\text{ (GetGet)}%_{(u^\ta,u')\in\Inget} 
		&	(p,e;e1, A,u;u1).\get.\ogbi        =         (p,e,A,u).\get.\ogbi ; 
		\\ 	 & \phantom{(p,e;e', A,u;u').\get.\ogbi=} 
		(e.\ta, e1, u.\ta,u1).\get.\ogbi
		\\ [3pt]
		\hline
	\end{array}
\end{myeq}
%  --- NOW PUT
\begin{myeq}{eqmmputP}
	%	\eqmmgetP  % was a macro but now is a direct encoding below
	\begin{array}{| l@{\quad}l |}
		\hline
		\multicolumn{2}{|l|}{
			\mbox{Definition of a learning $\putl$  machine over given \spabpgetoo: }} 
		\\ [3pt]
		\text{(Alphabets)} &	\ain^\putl=\bi, \aout^\putl=\ai,
		\\ 
		\text{(State space)} &\stt^\putl=\stt^\get %= \paoios\eqdef\pois\timm\ao 
	%\\ & 
	\phantom{\stt^\get}\cong \apoois\eqdef\ao\timm\pois
				\\
		\text{(Eff.Input)} & \Input =\stt^\putl{}_\param\timm_\so~ \spB_1
		%= \abpoos ~{}_\param\timm_\so~\ppi
			%\\ 	& \phantom{\Input }
			= \compr{(A,p,e,v)}{A.\get_{00}(p)=v.\so ~\&~ p=e.\so}
					\\
		\text{(Eff.Output)} &	\Output =\spA_1\timm\spP_1\timm\stt^\putl =
		   \\
		   		   	& %\phantom{\Output }
		   		   	= \compr{(u,e^\sim,e', A',p')}{(u,e',A',p')\models \text{(Incr)}_{\ao,\po,\ppi}
		   		     ~\&~p'=e'.\so}
		   \\
		   	& %\phantom{\Output }
		   	= \compr{(u,e^\sim,e', A',p')}%
		   	    {A'=u.\ta,\; p'= e^\sim.\ta,\; e'=\id_{e.\ta}~\&~p'=e'.\so}
		   	\\ [4pt]
		\multicolumn{2}{|l|}{
			\mbox{Equational Laws (to hold for any $(p,e,A,v)\in\Inget$)
				%$p\in\po$, $A \in\ao$, $e\inn\ppi,u\inn\ai$ such that $p=e^\so \text{ or } p=e^\ta$, $A=u^\so$
		}} 
		\\ [2.5pt]
		\text{ (Incidence)}%_{(A,u)\in\Inget} 
		& (p,e,A,u).\get.\ogbi.\so= A.\get_{00}(p) 
		% the arrow version (\get^\readd.\ogbi.\so= \igao.\get_{0}) 
%		\\
%		\text{ (Increm)}_{\ao} 
%		&	(p,e,A,u).\get.\ogao=u.\ta ~~(= A' \text{ in Eff. Output})
%		\\
%		\text{ (Increm)}_{\po} 
%		&	(p,e,A,u).\get.\ogpo=e.\ta~~ (=p' \text{ in Eff. Output})
%		\\
%		\text{ (Increm)}_{\ppi} 
%		&	(p,e,A,u).\get.\ogpi=\id_{e.\ta}~~  (=e' \text{ in Eff. Output})
          \\
          \text{ (PutHit)}
          & (A,p,e,v).\putl.\opao.\get_{00}(\oppo)=\ipbi.\ta~~ (\text{a.k.a. (PutGet)$_0$ law})
			\\[2.5pt]
			\multicolumn{2}{|l|}{
			\mbox{ (Unitality (a.k.a Stability) %any \frar{e1}{e.\ta}{\_}, \frar{u1}{u.\ta}{\_})   
		               }}
		\\
		\text{ (PutId)}%_A	
		& 			(p,\id_p,A,\id_A).\get.\ogbi=\id_{A.\get(p)} 
		%(u, A).\get.\ogbi=(u,A).\get_0
		\\ [3pt]
		\hline
	\end{array}
\end{myeq}
%
%\begin{myeq}{eqmmputP}
%%	\eqmmputP
%%	\eqmmgetP  % was a macro but now is a direct encoding below
%	\begin{array}{|ll|}
%	\hline
%	\multicolumn{2}{|c|}{
%		\mbox{Definition of a parametrized $\putl$ machine over given \spabpgetoo}}
%	\\ [3pt]
%			\text{(Alphabets)} & \ain^\putl=\bi, \aout^\putl=\ai,
%			\stt^\putl
%	\\ 
%	\Input=\compr{(A,p,v)}{(A,p).\get_{00}=\so(v)} &\\
%	\Output=\compr{(e,u,A,p)}{\ta(e)=p, \ta(u)=A} &\\
%	\putl.\opi.\so=\ipo &\text{ (Inc.)}\\
%	%		    \putl.\opi.\ta.\get_0=\ipi.\ta   \text{ (Putget for objects)  }  &\\
%	%\putl.\opo=\putl.\opi.\ta  \text{ (state update) }&\\ 		[3pt]
%	%		\mbox{\putgetlaw{} law:~} &\nonumber\\
%	\putl.\opo.\get_0 =\ipi.\ta & \text{ (PutOk) }\\
%	(A, \id_{A.\get_0}).\putl.\opi=\id_{A}  &\text{ (PutId) } \\
%	\textcolor{red}{(A, v;v').\putl.\opi=(A,v).\putl.\opi ; (A',v').\putl.\opi} &\textcolor{red}{~~ (PutPut) } \\
%	\hline
%\end{array}	
%\end{myeq}
%%
\begin{myeq}{eqmmputget}
	\begin{array}{|ll|}
		\hline
		\multicolumn{2}{|l|}{
			\mbox{Definition of a coupled $(\putl,\get)$-machine (a lens) over given \spabpgetoo}}
		\\ [3pt]
		\multicolumn{2}{|l|}{\mbox{Basic equational Law (to hold for any $(A,p)\inn\spA_0\timm\spP_0$ and \frar{v}{A.\get_{00}(p)}{\_}):  }}
		\\ [3pt]	
		\text{(Def. of \oisim) } & \oisim(u,e^\sim, e',u.\ta, e^\sim.\ta) = (e^\sim.\so, e,u.\so, u) 
		\\
		\text{(PutGet)}%_{(A,v)\in\Input} 
		& (A,p,e,v).\putl.\oisim.\get.\ogbi=v ~~(\text{or } \putl.\oisim.\get.\ogbi=\ipbi)
		\\ \hline
	\end{array}
\end{myeq}
	\caption{TWO State spaces diag Definition of an asymmetric coupled \mema\ with learning}
\label{fig:al-lensmm}
%\end{wrapfigure}
\end{figure}
} % end renew command for \app=idle

==> ll-figures/diags/al-lens-as-mealy.tex <==
\begin{figure}
	%	\begin{wrapfigure}{R}{0.5\columnwidth}
	%		\vspace{-0.5cm}
	\centering
	\begin{tabular}{l}%@{\quad}l}
\begin{diagram}%[small]
% -------------------------------> row 1
&&\Inget&&&&
\pile{
	\rTo^{\hspace{3em}\get} 
	\\ 
	\rTo_{\hspace{3em}\get_0} } % end pile 
&&&&	
\Outget &&
\\ %%%%%%%%------- ---> row 2 
%\dTo<{\igai}
%DIAGONALS
          & \ldTo>{\igai}
          &&\rdTo(2,2)<{\igpi} 
          \rdDashto(4,2)~{\igpo}
           \rdTo(6,2)^{\igao}
          &&& &&&  
          \ldTo(6,2)^{\ogpi} 
          \ldDashto(4,2)~{\ogpo}  %
           \ldTo(2,2)~{\ogao} 
          &&\rdTo>{\ogbi}
\\ %%%%%%%%%%%%%-----------> row 3 for the asymmetric case
%\uDashto<{\oiiso}
\sparra &&
\uDashto~{\oiiso}
&&	\sparrp
	& \pile{\rTo^{\qquad_\ta} \\ \rTo_{\qquad^\so}}
	&\spobp&{\times\qquad\quad}&\spoba)
	 &\rTo^{~~\get_{00}}_{\text{~~from$\timm$}}%\spobR&\rTo_{b}
	&\spobb
	&
	\pile{\lTo~{_\ta} \\  \lTo~{_\so}} % pile end
	&\sparrb
	&
\\ %%%%%%%%% -------------========> ROW 4 DIAGONALS 
&\luTo<{\opai}
	&&\ruTo(2,2)<{\oppi}
	&&\luTo(6,2)_{\ippi}
	%&
	\ruDashto(4,2)~{\oppo}
	& 
	&\luDashto(4,2)~{\ippo}
	\ruTo(6,2) _{\opao}
	&&\luTo(2,2)~{\ipao}
	&
	&
	\ruTo>{\ipbi} %\luTo(1,2)>{\ipi} &
\\%  --------------------------------------------->row 5
&&\Output&&&&
\pile{\lTo^{\hspace{1.5em}\putl_0} \\ \lTo_{\hspace{1.5em}\putl} }
&&&&	\Input &&
\\
&&&& &&&& &&&&
\end{diagram}
%\\ [30pt]
\\ [25pt]
(to avoid clutter,  
the fragment $\sparrp\pile{\rTo \\  \rTo}\spobp$ is used a shorthand for 
$\sparrp\pile{\rTo \\  \rTo}\spobp\lTo^{\pr_2}(\spoba\times\spobp)$
\\
and the fragment $\sparra\pile{\rTo \\  \rTo}\spoba$ is not shown
)
%not shown to avoid clutter)
\end{tabular}
\begin{myeq}{eqmmgetP}
%	\eqmmgetP  % was a macro but now is a direct encoding below
	\begin{array}{| l@{\quad}l |}
	\hline
	\multicolumn{2}{|l|}{
		\mbox{Definition of learning $\get$  machine (over given $\get_{00}$)}} 
	\\ [3pt]
	%\mbox{Input alphabet is $\spA_1$} &\\
	\text{(PB1)} &	\Inget \eqdef\compr{(u,e,p,A)}{\so(u)=A, \so(e)=p}  
	\\
	\text{(PB2)}  & \Outget\eqdef\compr{(e,p,A,v)}{(A, p).\get_{00} =\ta(v)} 
		\\ [3pt]
	\multicolumn{2}{|l|}{
		\mbox{Equational Laws: }}
	\\ [3pt]
	\text{ (Inc) }&\get_0.\ogbi.\so=(\igao,\igpo).\get_{00} 
	\\
	\text{ (Nat) }	&	(u,e,p,A).\get =(\id_A,e,p,A).\get~; (u,p,A).\get_0 \\
	& \hspace{6.25em}= (u,p',A).\get_0~; (\id_{A'},e, p', A').\get  
\\
	\text{ (GetId)}_A	&	(\id_p,u, A,p).\get.\ogbi=(u,A,p).\get_0
	\\
	\text{ (GetGet)}_A &			(e;e', \id_A, A, p).\get.\ogbi= \\
	&	\hspace{5em} =(e,\id_A,A,p).\get.\ogbi ; (e',\id_A, A, p').\get.\ogbi 
	\\ [3pt]
	\text{}	&		\Inget_0=\compr{(u,A,p)}{\so(u)=A}  
%	\\
%	\text{ (GetOk)}_p &	\get_0.(\ogao, \ogpo).\pr=\igai.\ta  
	\\
	\text{ (GetId)}_p &		(\id_A, A,p).\get_0.\ogbi=\id_{(A,p).\get_{00}}  
	\\
	\text{ (GetGet)}_p  &			(u;u', A, p).\get_0.\ogi=(u,A,p).\get_0.\ogbi ; (u',A',p).\get_0.\ogbi \\ [3pt]
	\hline
\end{array}
\end{myeq}
\begin{myeq}{eqmmputP}
%	\eqmmputP
%	\eqmmgetP  % was a macro but now is a direct encoding below
	\begin{array}{|ll|}
	\hline
	\multicolumn{2}{|c|}{
		\mbox{Definition of learning $\putl$ machine (over given $\get_{00}$ )}}
	\\ [3pt]
	\Input=\compr{(A,p,v)}{(A,p).\get_{00}=\so(v)} &\\
	\Output=\compr{(e,u,A,p)}{\ta(e)=p, \ta(u)=A} &\\
	\putl.\opi.\so=\ipo &\text{ (Inc.)}\\
	%		    \putl.\opi.\ta.\get_0=\ipi.\ta   \text{ (Putget for objects)  }  &\\
	%\putl.\opo=\putl.\opi.\ta  \text{ (state update) }&\\ 		[3pt]
	%		\mbox{\putgetlaw{} law:~} &\nonumber\\
	\putl.\opo.\get_0 =\ipi.\ta & \text{ (PutOk) }\\
	(A, \id_{A.\get_0}).\putl.\opi=\id_{A}  &\text{ (PutId) } \\
	\textcolor{red}{(A, v;v').\putl.\opi=(A,v).\putl.\opi ; (A',v').\putl.\opi} &\textcolor{red}{~~ (PutPut) } \\
	\hline
\end{array}	
\end{myeq}
%
\begin{myeq}{eqmmputget}
%	\fbox{\putgetlaw{} law:~ $\putl.\oiiso.\get.\ogbi~=~\ipbi$} 
	\begin{array}{|l@{~~}l|}
	\hline
	\mbox{\putgetlaw{} law:~} &\\
	\oiiso(u,e,A',p') \eqdef(u,e,A,p) &\\
	\putl.\oiiso.\get.\ogbi =\ipbi &\\
	\hline
	\end{array}
\end{myeq}
	\caption{Categorically learning asymmetric lens as a special Mealy machine couple: the two common state spaces are $S_0=\spA_0\timm\spP_0$ and $S_1=S_0\timm\spP_1$}
\label{fig:al-lens-mealy}
%\end{wrapfigure}
\end{figure}

==> ll-figures/diags/al0-lens-as-mealy.tex <==

\begin{figure}
	%	\begin{wrapfigure}{R}{0.5\columnwidth}
	%		\vspace{-0.5cm}
	\centering
	\begin{tabular}{l@{\quad}l}
\begin{diagram}[small]
%  row 1
\Inget&&&&&\rTo^\get &&&	
\Outget &&
\\ % ---> row 2 DIAGONALS
          &\rdTo(2,2)<{\igai} 
          \rdTo(4,2)~{\igao}
           \rdTo(6,2)^{\igpo}
          &&& &&&  
          \ldTo(4,2)^{\ogao}  %\ldTo(2,2)>{\ogi} 
           \ldTo(2,2)~{\ogpo} 
          &&\rdTo>{\ogbi}
%\\ % row 3 foir the symmetric case
%&	\sparra
%	&\pile{\rTo^\so \\  \rTo_\ta}
%	&\spoba &\lTo_{a}&\spobR&\rTo_{b}&\spobb
%	&\pile{\lTo^\ta \\ \lTo_\so}
%	&\sparrb
%	&
%===================
\\ % row 3 for the asymmetric case
\uDashto<{\oiiso}
%\dDashto>{\sim_{io}}
&&	\sparra
	&\pile{\rTo^{\so~~~
}
	 \\  \rTo_{\ta~~~
}}
	&(\spoba&{\times}&\spobp)
	 &\rTo^{~~\get_0}%\spobR&\rTo_{b}
	&\spobb
	&\pile{\lTo^{\ta
		}
	 \\ \lTo_\so}
	&\sparrb
	&
\\ % ROW 4 DIAGONALS 
	&\ruTo(2,2)<{\opai}
	&
	&\ruTo(4,2)~{\opao}
	& &\luTo(4,2)_{\ipao}
	\ruTo(6,2) _{\oppo}
	&&\luTo(2,2)~{\ippo}
	&
	&
	\ruTo>{\ipbi} %\luTo(1,2)>{\ipi} &
\\%  row 5
\Output&&&&&\lTo^\putl&&&	\Input &&
\end{diagram}
&
\mbox{$
\begin{array}{|l@{~~}l|}
\hline
\mbox{Definitions of state machines  \get:} &\\
\Inget=\compr{(u,A,p)}{\so(u)=A}%\igi.\so =\igo
 & \\
 \Outget=\compr{(A,p,v)}{\ta(v)=A}
 &\\
 \get.\ogpo = \igpo
 &\\
 \ldots ... &\\
% \get.\ogbi.\ta=(\igai.\ta, \igpo).\get_0& \\
%\get.\ogbi.\so=(\igai.\so, \igpo).\get_0& \\[3pt]
%\mbox{Incidence/totality  for \putl:} &\\
\Input=\compr{(A,p,v)}{(A, p).\get_0=\so(v)}
&\\
\Output=\compr{(u,A,p)}{\xxxx }
%\ipi.\so=\ipo.\get_0
& \\
\putl.\opai.\so=\ipao &\\[3pt]
%
\mbox{\putgetlaw{} law:~}
\putl.\oiiso.\get.\ogbi =\ipbi &\\
\hline
\end{array}
$}
\end{tabular}
	\caption{Codiscrtely learning asym. lens as a Mealy machine couple: The common state space is $\spA_0\timm\spP_0$}
\label{fig:al-lens-mealy}
%\end{wrapfigure}
\end{figure}

==> ll-figures/diags/alens-as-mealy.tex <==
%
%\newcommand\eqmmget{\enma{
%%	\begin{IEEEeqnarray}{ll}
%		 \begin{array}{| ll |}
%		\hline
%\multicolumn{2}{|c|}{
%             \mbox{Definition of $\get$  machine (over given $\get_0$)}} 
%         \\ [3pt]
%		   %\mbox{Input alphabet is $\spA_1$} &\\
%		       	\Inget=\compr{(u,A)}{\so(u)=A}  & \\
%		    \Outget=\compr{(A,v)}{A.\get_0=\ta(v)} &	\\  
%		%[3pt] 		\mbox{\get\ transitions} &\nonumber \\
%		\get.\ogi.\so=\igo.\get_0 &\text{ (Inc.) } \\
%		%\get.\ogi.\ta=\igi.\ta.\get_0 \text{ () }  &\\
%		\get.\ogo=\igi.\ta  &\text{ (GetOk) } \\
%		(\id_A, A).\get.\ogi=\id_{A.\get_0} &\text{ (GetId) } \\
%		(u;u', A).\get.\ogi=(u,A).\get.\ogi ; (u',A').\get.\ogi &\text{ (GetGet) } \\
%			\hline
%	\end{array}
%%	\end{IEEEeqnarray}
%}}
%
%
%\newcommand\eqmmput{
%%	\begin{IEEEeqnarray}{ll}
%\begin{array}{|ll|}
%\hline
%\multicolumn{2}{|c|}{
%\mbox{Definition of $\putl$ machine (over given $\get_0$ )}}
%\\ [3pt]
%		\Input=\compr{(A,v)}{A.\get_0=\so(v)} &\\
%		\Output=\compr{(u,A)}{\ta(u)=A} &\\
%	     	\putl.\opi.\so=\ipo &\text{ (Inc.)}\\
%%		    \putl.\opi.\ta.\get_0=\ipi.\ta   \text{ (Putget for objects)  }  &\\
%		    %\putl.\opo=\putl.\opi.\ta  \text{ (state update) }&\\ 		[3pt]
%%		\mbox{\putgetlaw{} law:~} &\nonumber\\
%		\putl.\opo.\get_0 =\ipi.\ta & \text{ (PutOk) }\\
%			(A, \id_{A.\get_0}).\putl.\opi=\id_{A}  &\text{ (PutId) } \\
%				\textcolor{red}{(A, v;v').\putl.\opi=(A,v).\putl.\opi ; (A',v').\putl.\opi} &\textcolor{red}{~~ (PutPut) } \\
%		\hline
%	\end{array}	
%	%\end{IEEEeqnarray}
%}

%\newcommand\Inx[1]{\enma{\mathit{In}_{{#1}}}}
%\newcommand\Outx[1]{\enma{\mathit{Out}_{{#1}}}}
%\newcommand\InA{\Inx{\spA}}
%\newcommand\InB{\Inx{\spB}}
%\newcommand\Inget{\Inx{\get}}
%\newcommand\Input{\Inx{\putl}}
%\newcommand\Outget{\Outx{\get}}
%\newcommand\Output{\Outx{\putl}}
%
%\newcommand\igpxy[2]{\enma{\mathit{i}\mathit{#1}_{\mathsf{#2}}}}
%    \newcommand\igo{\igpxy{g}{0}}
%	\newcommand\igi{\igpxy{g}{1}}
%\newcommand\ogpxy[2]{\enma{\mathit{o}\mathit{#1}_{\mathsf{#2}}}}
%	\newcommand\ogo{\ogpxy{g}{0}}
%	\newcommand\ogi{\ogpxy{g}{1}}
%	
%%\newcommand\igpxy[2]{\enma{\mathit{i}_{\mathsf{#1#2}}}}
%   \newcommand\ipo{\igpxy{p}{0}}
%   \newcommand\ipi{\igpxy{p}{1}}
%%\newcommand\ogpxy[2]{\enma{\mathit{o}_{\mathsf{#1#2}}}}
%   \newcommand\opo{\ogpxy{p}{0}}
%    \newcommand\opi{\ogpxy{p}{1}}
%\newcommand\oiiso{\enma{\iota_\sim}}
%
%\newcommand\spobx[1]{\enma{#1_0}}
%\newcommand\sparrx[1]{\enma{#1_1}}
%\newcommand\spoba{\spobx{\spA}}
%\newcommand\spobb{\spobx{\spB}}
%\newcommand\sparra{\sparrx{\spA}}
%\newcommand\sparrb{\sparrx{\spB}}
%\newcommand\spobR{\spobx{\spR}}
%\newcommand\sparrR{\sparrx{\spR}}

\begin{figure}
	%	\begin{wrapfigure}{R}{0.5\columnwidth}
	\centering
	\begin{tabular}{l@{\quad}l}
\begin{diagram}%[small]
%  ------------------------------------------- >row 1
\Inget&&&&\rTo^\get &&&&	
\Outget
\\ % -----------------------------------------> row 2 DIAGONALS
 &\rdTo(2,2)<{\igai} \rdTo(4,2)>{\igao}
 &&& \puncture &&&\ldDertoda(4,2)<{\ogao}  %\ldTo(2,2)>{\ogi} 
 &\dTo>{\ogbi}
%\\ ---------> % row 3 foir the symmetric case
%&	\sparra
%	&\pile{\rTo^\so \\  \rTo_\ta}
%	&\spoba &\lTo_{a}&\spobR&\rTo_{b}&\spobb
%	&\pile{\lTo^\ta \\ \lTo_\so}
%	&\sparrb
%	&
\\ % ------------------------>      row 3 for the asymmetric case
\uDashto<{\oiiso}
%\dDashto>{\sim_{io}}
& %[=]\hspace{1ex}
\pmb{\puncture_{\spA_0}}
&	\sparra
	&\pile{\rTo^{\so~~}
	          \\  \rTo_{\ta~~}} % end pile }
	&\spoba &\rTo^{\get_0}%\spobR&\rTo_{b}
	&\spobb
	&\pile{\lTo^{\ta
%			\begin{array}{cc}
%			&	(3) \\
%			~~~~~~~~\ta &\\
%					\end{array}	
		}
	 \\ \lTo_\so}
	&\sparrb
	&
\\ % ROW 4 DIAGONALS 
	&\ruTo(2,2)<{\opai}&&\ruDertoda(4,2)>{\opao}
	&\puncture & \luTo(4,2)_{\ipao}&&&\uTo>{\ipbi} %\luTo(1,2)>{\ipi} 
\\%  row 5
\Output&&&&\lTo^\putl&&&&	\Input
\end{diagram}
&
\end{tabular}
{\renewcommand\readd{{}}
\begin{myeq}{eqmmget}
	%	\eqmmgetP  % was a macro but now is a direct encoding below
	\begin{array}{| l@{\quad}l |}
		\hline
		\multicolumn{2}{|l|}{
		\mbox{Definition of a \get\  machine over given \spabgeto: }
			} 
		\\ [3pt]
			\text{(The base)} &	%\ainx{\get}=\ai, \aoutx{\get}=\bi, \sttx{\get}=\ao
			\ain^{\get}=\ai, \aout^{\get}=\bi, \stt^{\get}=\ao
		\\
		%\mbox{Input alphabet is $\spA_1$} &\\
		\text{(Eff. Input)} &	\Inget=\aois\eqdef\compr{(A,u)}{u.\so=A},
		\\
		\text{(Eff. Output)}& 
		\Outget=\baiot\eqdef\compr{(v,A')}{(v,A')\models\gethit} 
		\\
		& \phantom{Outget=\baiot}= \compr{(v,A')}{A'.\get_{0}=v.\ta}  % GetHit condition 
		%  \Outget=\baiot\eqdef\compr{(v,A')}{(A,u).\get.\ogbi.\so= A.\get_0 }  % Incidence
		%				\text{(Def. of \Outget)}  & \Outgetread\eqdef\compr{(v,A)}{A.\get_{0}=v^\ta} 
		\\ [5pt]
		\multicolumn{2}{|l|}{
%			\mbox{Equational Laws (to hold for any $A\in\spA_0$, $(A,u)\inn\Inget$, and \frar{u'}{u^\ta}{\_}): }}
			\mbox{Equational Laws (to hold for any $A\in\spA_0$, \frar{u}{A}{\_}, and \frar{u'}{u^\ta}{\_}): }}
		\\ %[3pt]
			\multicolumn{2}{|l|}{\mbox{Basic (in addition to \gethit):}}
			\\
		\text{ (Incidence)}%_{(A,u)\in\Inget} 
		&  (A,u).\get.\ogbi.\so= A.\get_0  % Incidence 
			% the arrow version (\get^\readd.\ogbi.\so= \igao.\get_{0}) 
			\\
		\text{ (Increm)}%_{(A,u)\in \Inget} 
		&	(A,u).\get.\ogao=u.\ta~~ (= A' \text{ in Eff. Output})
		\\
%		\text{ (Nat) }	&	(u,e,p,A).\get^\readd =(\id_A,e,p,A).\get~; (u,p,A).\get_0 \\
%		& \hspace{6.25em}= (u,p',A).\get_0~; (\id_{A'},e, p', A').\get  
			\multicolumn{2}{|l|}{\mbox{Monoidal (a.k.a. ``well-behaved''):}}
			\\
		\text{ (GetId)}%_A	
		& 			(A,\id_A).\get.\ogbi=\id_{A.\get} 
				%(u, A).\get.\ogbi=(u,A).\get_0
		\\
		\text{ (GetGet)}%_{(u^\ta,u')\in\Inget} 
		&	(A,u;u').\get.\ogbi=(A,u).\get.\ogbi ; (u^\ta,u').\get.\ogbi
			%(\id_A, A).\get.\ogbi= \\
		%&	\hspace{5em} =(\id_A,A).\get.\ogbi ; (\id_A, A).\get.\ogbi 
		\\ [3pt]
		\hline
	\end{array}
\end{myeq}
} % end renew command readd
%\begin{myeq}{eqmmget}
%	\eqmmget
%\end{myeq}
%
\begin{myeq}{eqmmput}
%	\eqmmput replaced by the body of the macros
\begin{array}{|ll|}
	\hline
	\multicolumn{2}{|l|}{
		\mbox{Definition of a $\putl$ machine over given \spabgeto}}
\\ [3pt]
		\text{(The base)} &	\ainx{\putl}=\sparrb, \aoutx{\putl}=\sparra, \stt^\putl=\spoba
\\
	%\mbox{Input alphabet is $\spA_1$} &\\
	\text{(Eff. Input)} &	\Input=\abois\eqdef\compr{(A,v)}{A.\get_0=v^\so}, 
	\\
% \text{(Eff. Output)} &	\Output=\aiot\eqdef\compr{(u,A)}{u^\ta=A} 
%\\ [3pt]
		\text{(Eff. Output)}& 
\Output=\aiot\eqdef\compr{(u,A')}{(u,A')\models\text{ (Increm)} } 
\\
& \phantom{Output=\aiot}= \compr{(u,A')}{A'=u.\ta}  % GetHit condition 
%  \Outget=\baiot\eqdef\compr{(v,A')}{(A,u).\get.\ogbi.\so= A.\get_0 }  % Incidence
%				\text{(Def. of \Outget)}  & \Outgetread\eqdef\compr{(v,A)}{A.\get_{0}=v^\ta} 
\\ [5pt]
  	\multicolumn{2}{|l|}{
			\mbox{Equational Laws (to hold for any $A\in\spA_0$, \frar{v}{A.\get_0}{\_}, and \frar{v'}{v^\ta}{\_}): }}
\\ %[3pt]
  	\multicolumn{2}{|l|}{\mbox{Basic (in addition to Increm):}}
\\
\text{ (Incidence)}%_{(A,v)\inn\Input} 
&  (A,v).\putl.\opai.\so = A
\\
 \text{ (PutHit)}%_{A,v} 
 &	(A,v).\putl.\opao.\get_0 =v.\ta~~ (\text{a.k.a. (PutGet)$_0$ law})
 %\\
 %\textcolor{red}{otherDir ~ version }& \textcolor{red}{(\opao.\putl.(A,v)).\get_0=\ta(v)}
	\\ %[3pt]
		\multicolumn{2}{|l|}{\mbox{Monoidal:}}
		\\
\text{ (PutId)}%_A 
&	(A, \id_{A.\get_0}).\putl.\opai=\id_{A}  
\\
  	\multicolumn{2}{|l|}{
	\mbox{For reference only (not required to hold) %Equational Laws (to hold for any $A\in\spA_0$, \frar{v}{A.\get_0}{\_}, and \frar{v'}{v^\ta}{\_}): 
}}
\\
\textcolor{red}{(PutPut)}%_{A,v,v'} 
&	\textcolor{red}{(A, v;v').\putl.\opi=(A,v).\putl.\opi ; (A',v').\putl.\opi}  
\\ 	\hline
\end{array}	
\end{myeq}
%\end{array}$
%\end{tabular}
%\eqalensmm
\begin{myeq}{eqmmputget}
	\begin{array}{|ll|}
		\hline
		\multicolumn{2}{|l|}{
			\mbox{Definition of a coupled $(\putl,\get)$-machine (a lens) over given \spabgeto}}
		\\ [3pt]
\multicolumn{2}{|l|}{\mbox{Basic equational Law (to hold for any $A\in\spA_0$, \frar{v}{A.\get_0}{\_}):  }}
\\ [3pt]	
\text{(Def. of \oiiso) } & \oiiso(u, u^\ta) = (u^\so, u) 
\\
\text{(PutGet)}%_{(A,v)\in\Input} 
& (A,v).\putl.\oiiso.\get.\ogbi~=~v
\\ \hline
\end{array}
\end{myeq}
		\caption{A coupled Mealy machine definition}
	\label{fig:alensmm}
	%\end{wrapfigure}
\end{figure}


==> ll-figures/diags/bigPIcture-wSym.tex <==
\begin{figure}[t]
	\centering
\begin{diagram}[small]
	%\pcatcat&\lMonic&\ptracat &\pile{
	%	\rTo^{{+}\putl(\prpol)}\\ \lTo_{{-}\putl}}
	%&\aplenscat
	%\\
	%\uMonic &&\uMonic &&\uMonic
	%\\
	(\psetcat,\times)&\lMonic&\paracatcon&\pile{
		\rTo^{{+}\Grd(\eps,\err)}\\ \lTo_{{-}\Grd}
	} &\learncat &\rTo^{\sym_0}&\slenscat_0 &\mathrm{\quad Codicrete~Setting}~\citefst,\citefjbx
	\\
	\dMonic &&\dMonic &&\dMonic&?&\dMonic
	&\mbox{$\mathit{Hom}(x,y)$ is $(x,y)$}
	\\
	(\pcatcat,\times)&\lMonic&\ptracat &\pile{
		\rTo^{{+}\Put(\prpol)}\\ \lTo_{{-}\Put}}
	&\aplenscat&\rTo^{\sym?}&\slenscat &\mathrm{Learning~Lenses}
	\\
	\uMonic &&\uMonic &&\uMonic&& %?&\uMonic
	&\mbox{Parameter space is \tcat}
	\\
	(\catcat,\times)&\lMonic&\tracat&\pile{
		\rTo^{{+}\putl(\prpol)}\\ \lTo_{{-}\putl}}
	&\alenscat&& &\mbox{Ordinary~Lenses}
\end{diagram}
\caption{Compositional learning and lenses: nodes are sm-categories and arrows are sm-functors; arrows with triangle tail denote embedding. All functors are identical on objects.  
	\psetcat\ is the codiscrete version of \pcatcat.
}
	\label{fig:bigpic}
\end{figure}

==> ll-figures/diags/bigPicture.tex <==
\begin{figure}[t]
	\centering
\begin{diagram}[h=3em,w=2em]
	% row 0
	&& (1) &(2)&(3)&(4)&(5)
		\\ % row 1
	%(\psetcat,\times)&\lMonic&
(1)&&	&&\paracat&\pile{
		\rTo^{{+}\gdbp(\eps,\err)}\\ \lTo_{{-}\gdbp}
	} &\learncat &\parbox{4.5cm}{\small Learning by Gradient~descent \& Back~prop.~\citefst}
	\\ % row 2
(2)&&	&&\dMapsto &\mboxsmall{paper \citefst} &\dEQ %&?&\dMonic
	&\mboxsmall{\small Instantiation}
	\\ % row 3
(3)&&	\psetcat&\lMonic&\pviewcat_0&\pile{
		\rTo^{{+}\Put_0(\Pol)}\\ \lTo_{{-}\Put_0}
	} &\allenscat_0 &\mboxsmall{\small  Abstract Codiscr. Learning Lenses}~\citefst
	\\ % row 4
(4)&&	\dMonic>\fu &&\dMonic>\fu &
\mboxsmall{the present paper} 
&\dMonic>\fu %&?&\dMonic
	&\mbox{\small Embed via setting $\mathit{Hom}(x,y)=(x,y)$}
	\\ % row 5
(5)	&&\pcatcat&\lMonic&\pviewcat &\pile{
		\rTo^{{+}\Put(\Pol)}\\ \lTo_{{-}\Put}}
	&\allenscat &\mboxsmall{\small Abstract Learning Lenses}
	\\ % row 6
(6)	&&\uMonic>\wi &&\uMonic>\wi &
\mboxsmall{the present paper} 
&\uMonic>\wi %?&\uMonic
	&\mboxsmall{Embed via setting $\spP = \tcat$}
	\\  % row 7
(7)	&&\catcattimm&\lMonic&\viewcat&\pile{
		\rTo^{{+}\putl(\pol)}\\ \lTo_{{-}\putl}}
	&\alenscat&\mboxsmall{Ordinary Abstract Lenses}
		\\ % row 7
(8)	&& &&\uMapsto &
\mboxsmall{future work} 
&\uMapsto %?&\uMonic
	&\mboxsmall{Instantiation}
	\\  % row 8
(9)	&&&&\viewcattgg&\pile{
		\rTo^{{+}\bprules(\nmf{tggBp})}\\ \lTo_{{-}\bprules}}
	&\alenscattgg&\parbox{3.5cm}{\small Update propagation via View~TGG \cite{tony-viewtgg-ecmfa14}}
\end{diagram}
\caption{Compositional learning and lenses: nodes are sm-categories and arrows are sm-functors; arrows with triangle tail denote embedding (full or wide, if labelled with \fu\ or \wi\ resp.). All functors are identical on objects.  
	\psetcat\ is the codiscrete version of \pcatcat.
}
	\label{fig:bigpic}
\end{figure}

==> ll-figures/diags/bxmlPut-act19.tex <==
%\newcommand\Uml{\enma{\mathcal{U}}}
%=====
\newcommand\arI{
	\begin{array}{c}
		a'= \\ [-5pt]
		r_I(p,a,b)	
	\end{array}
}
%====
\newcommand\bxdiag{
	\begin{diagram}%[small]
		% row 01
		\spA &\rTo^{\get_p}_{p\in\spP}&\spB&&
		\\ % row 02
		&& &&
			\\ % row 1
		\dbox{A}& \rDashmapsto^{{:}\get_p}& {B}&
		\\ % row 2
		&& & \rdTo>{v}&
		\\ % row 3
		\dDotto<{u^{}} &\swssseTilearrowAB{{:}\putl}{}&\dDashto>{u.\get_{e}}&&\dbox{B'}
		\\ % row 4
		&&&\ldDotto>{v^{@}}&
		\\ % row 5
		A' &\rDermapsto^{{:}\get_{p'}}&B'^@_{}&&	
	\end{diagram}
}
%=====  mldiag new
\newcommand\mldiagnew{
	\begin{diagram}%[small]
		% row 01
		\rcat^m &\rTo^{I(p,\_)}_{p\in\rcat^k}&\rcat^n&&
		\\ % row 02
		&& &&
		\\ % row 1
		\dbox{a}& \rDashmapsto^{I(p,-)}& {I(p,a)}&
		\\ % row 2
		&& & \rdTo>{\del{=}\del_{I}(p,a,b)} %=(\del_i{-}a_i)_{i\le n}}
		&
		\\ % row 3
		\dDotto<{\della} &\swssseTilearrowAB{{:}\putl}{}%\swssTilearrowAB{{:}\putl}{}
		&\dDashto>{\della_{pp'}}&&\dbox{b}
		\\ % row 4
		&&&\ldDotto>{\del^@}%{\del_{I}^@(p,a,b)}
		&
		\\ % row 5
		\arI &\rDermapsto^{I(p',-)}_{p'=\Uml_I(p,a,b)}
		&I(p',a')&&	
	\end{diagram}
}
%===== \mldiag old
%\newcommand\mldiag{
%	\begin{diagram}
%		% row 1
%		(\Reals^m, \DDel^m) &\rTo^{I(p,-)}_{p\in\Reals^k} &(\Reals^n, \DDel^n)
%		\\ % row 2
%		&&
%		\\ % row 3
%		\dbox{a}& \rDermapsto^{I(p,-)} & I(p,a)
%		\\ % row 4
%		&& \dTo<{E_I(p,a,b)}
%		\\ % row 5
%		\dDashto>{E(a,a')} &\swssTilearrowAB{{:}\putl}{}&\dbox{b}
%		\\ % row 6
%		&&\dDashto<{} %<{E_I^@}
%		\\ % row 7
%	\arI &\rDermapsto^{I(p',-)}_{p'=\Uml_I(p,a,b)}& I(p',a')
%	\end{diagram}
%}

%\renewcommand\mldiag{}
\begin{figure}
%\begin{wrapfigure}{R}{0.65\columnwidth}
\vspace{-0.5cm}
\centering
\begin{tabular}{c@{\qquad\qquad}c}
	\bxdiag & %\mldiag
	               \mldiagnew
	\\  [25ex]

	a) \frar{e}{p}{p'} is not shown & b) $\dellp=p'-p$ is not shown
\end{tabular}
\caption{Change propagation in \alalens es. Derived/computed elements are specially visualized: nodes are not framed, arrows are dashed. % Given nodes are framed, given arrows are solid
}
\label{fig:bxmlPut}
%\vspace{-10mm}
%\end{wrapfigure}
\end{figure}

==> ll-figures/diags/bxmlPut.tex <==
\newcommand\Uml{\enma{\mathcal{U}}}
%=====
\newcommand\arI{
	\begin{array}{c}
		a'= \\ [-5pt]
		r_I(p,a,b)	
	\end{array}
}
%====
\newcommand\bxdiag{
	\begin{diagram}%[small]
		% row 01
		\spA &\rTo^{\get_p}_{p\in\spP}&\spB&&
		\\ % row 02
		&& &&
			\\ % row 1
		\dbox{A}& \rDashmapsto^{{:}\get_p}& {B}&
		\\ % row 2
		&& & \rdTo>{v}&
		\\ % row 3
		\dDotto<{u^{}} &\swssseTilearrowAB{{:}\putl}{}&\dDashto>{u.\get_{e}}&&\dbox{B'}
		\\ % row 4
		&&&\ldDotto>{v^{@}}&
		\\ % row 5
		A' &\rDermapsto^{{:}\get_{p'}}&B'^@_{}&&	
	\end{diagram}
}
%=====  mldiag new
\newcommand\mldiagnew{
	\begin{diagram}%[small]
		% row 01
		\rcat^m &\rTo^{I(p,\_)}_{p\in\rcat^k}&\rcat^n&&
		\\ % row 02
		&& &&
		\\ % row 1
		\dbox{a}& \rDashmapsto^{I(p,-)}& {I(p,a)}&
		\\ % row 2
		&& & \rdTo>{\del{=}\del_{I}(p,a,b)} %=(\del_i{-}a_i)_{i\le n}}
		&
		\\ % row 3
		\dDotto<{\della} &\swssseTilearrowAB{{:}\putl}{}%\swssTilearrowAB{{:}\putl}{}
		&\dDashto>{\della_{pp'}}&&\dbox{b}
		\\ % row 4
		&&&\ldDotto>{\del^@}%{\del_{I}^@(p,a,b)}
		&
		\\ % row 5
		\arI &\rDermapsto^{I(p',-)}_{p'=\Uml_I(p,a,b)}
		&I(p',a')&&	
	\end{diagram}
}
%===== \mldiag old
%\newcommand\mldiag{
%	\begin{diagram}
%		% row 1
%		(\Reals^m, \DDel^m) &\rTo^{I(p,-)}_{p\in\Reals^k} &(\Reals^n, \DDel^n)
%		\\ % row 2
%		&&
%		\\ % row 3
%		\dbox{a}& \rDermapsto^{I(p,-)} & I(p,a)
%		\\ % row 4
%		&& \dTo<{E_I(p,a,b)}
%		\\ % row 5
%		\dDashto>{E(a,a')} &\swssTilearrowAB{{:}\putl}{}&\dbox{b}
%		\\ % row 6
%		&&\dDashto<{} %<{E_I^@}
%		\\ % row 7
%	\arI &\rDermapsto^{I(p',-)}_{p'=\Uml_I(p,a,b)}& I(p',a')
%	\end{diagram}
%}

%\renewcommand\mldiag{}
\begin{figure}
%\begin{wrapfigure}{R}{0.65\columnwidth}
\vspace{-0.5cm}
\centering
\begin{tabular}{c@{\qquad\qquad}c}
	\bxdiag & %\mldiag
	               \mldiagnew
	\\  [25ex]

	a) \frar{e}{p}{p'} is not shown & b) $\dellp=p'-p$ is not shown
\end{tabular}
\caption{Change propagation in \alalens es. Derived/computed elements are specially visualized: nodes are not framed, arrows are dashed. % Given nodes are framed, given arrows are solid
}
\label{fig:bxmlPut}
%\vspace{-10mm}
%\end{wrapfigure}
\end{figure}

==> ll-figures/diags/codifun-last-withPara.tex <==
%\par\textcolor{red}{DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%}
%\endinput
{
	\renewcommand\grt[1]{#1}
\begin{figure}
	\centering
\begin{diagram}%[small]
(1)\quad&&&\alalenscatdif&&&&&&&
\\ % row 2
(2)\quad&&
\ldTo^{{-}\lens}
\ruDashto(2,6)^{\grgrt{\leefunovr}\qquad\qquad\qquad\qquad}
&%\mbox{[j-monic]}
&
\rdTo^{{-}\dif}
\rdTo(5,2)^\codiscr_{
\begin{array}{c}
	{}_{[\noteq^?]}
\end{array}
}& &&&&&
\\ % row 3 -------
(3)\quad&
\pspadifcat
&&\uDashto~{\blt{[\plusx{\ponix},\!\plusx{\ponix}]}}
%\pile{\rTo^{}}
&&\qquad\alalenscat&
&\lEmbed
&\alalenscatcodi&\grgrt{~=\learncat}	
\\ % row 4----------------
(4)\quad&&
\rdTo^{\minusdif}
\luTo(2,4)<{\grt{\qquad\qquad\plusxdif}}
&&
\ldTo^{\minusput}
\ruTo(2,4)>{\plusxput\qquad\qquad}<{(*)\qquad\qquad}%\ruTo(5,2)^\codiscr
&&%[\noteq]
&
\ruDashto(5,4)<{\qquad\qquad\plusxput}_{(**)\qquad}
\ldTo(1,2)_{\minusputcodi}
%\ruDashto(2,4)>{\blt{{\plusxput^0}}}
&\ruDashto(2,4)>{\grgrt{L_{\eps,\err}}}
&
\\ % row 5
(5)\quad&&&\pcatcat%_{(*)}
&
&\lEmbed%\rTo^{{-}\mathsf{arrows}}
&&\psetcat&&&&
\\ % row 6 ===
(6)\quad &&& \uTo<{{-}\nix\!\!}
&&&
\ruDashto(4,2)>{\minusnixcodi}
\ruTo(1,2)>{\minusnixcodi}
&&&&
\\ % row 7
(7)\quad&
\grgrt{\paracatrcat}
&\grgrt{=\!=\!=\!=}%\rEQ
&
\grt{\pgetcat_\nix}&& 
%\pile{\rTo^{\grt{\minusxdel}\quad}_{\grt{\congx{\nix}}}
%	\\
%	\lTo_{\grt{\plusxdel}~~}}
\lEmbed_{\congx{\nix}}%^{\grt{\plusxdel}~~}
&\grt{\pgetcat^0_\nix}&\grgrt{~=\paracat_\reals}&&&
\end{diagram}
\caption{Building codiscrete lenses}\label{fig:codifun-big}
\end{figure}
}


==> ll-figures/diags/codifun-new-withPara.tex <==
%\par\textcolor{red}{DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%}
%\endinput
{
	\renewcommand\grt[1]{#1}
\begin{figure}
	\centering
\begin{diagram}%[small]
(1)\quad&&&\alalenscatdif&&&&&&&
\\ % row 2
(2)\quad&&
\ldTo^{{-}\lens}
\ruDashto(2,6)^{\grgrt{\leefunovr}\qquad\qquad\qquad\qquad}
&%\mbox{[j-monic]}
&
\rdTo^{{-}\dif}
\rdTo(5,2)^\codiscr_{
\begin{array}{c}
	{}_{[\noteq^?]}
\end{array}
}& &&&&&
\\ % row 3 -------
(3)\quad&
\pspadifcat
&&\uDashto~{\blt{[\plusx{\ponix},\!\plusx{\ponix}]}}
%\pile{\rTo^{}}
&&\qquad\alalenscat&
&\lEmbed
&\alalenscatcodi&\grgrt{~=\learncat}	
\\ % row 4----------------
(4)\quad&&
\rdTo^{{-}\dif}
\luTo(2,4)<{\grt{\qquad\qquad\plusxdif}}
&&
\ldTo^{{-}\putl}
\ruTo(2,4)>{\plusxput\qquad\qquad}<{(*)\qquad\qquad}%\ruTo(5,2)^\codiscr
&&%[\noteq]
&\ldTo(2,2)^{{-}\putl^0}
\ruDashto(2,4)>{\blt{{\plusxput^0}}}
&\ruDashto(2,4)>{\grgrt{L_{\eps,\err}}}
&
\\ % row 5
(5)\quad&&&\pcatcat%_{(*)}
&
&\lEmbed%\rTo^{{-}\mathsf{arrows}}
&\psetcat&&&&
\\ % row 6
(6)\quad &&& \uTo<{{-}\nix\!\!}
&&&
\uTo<{({-}\nix)^0}
&&&&
\\ % row 7
(7)\quad&
\grgrt{\paracatrcat}
&\grgrt{=\!=\!=\!=}%\rEQ
&
\grt{\pgetcat_\nix}&& 
%\pile{\rTo^{\grt{\minusxdel}\quad}_{\grt{\congx{\nix}}}
%	\\
%	\lTo_{\grt{\plusxdel}~~}}
\lEmbed_{\congx{\nix}}^{\grt{\plusxdel}~~}
&\grt{\pgetcat^0_\nix}&\grgrt{~=\paracat_\reals}&&&
\end{diagram}
\caption{Building codiscrete lenses}\label{fig:codifun-big}
\end{figure}
}


==> ll-figures/diags/codifun-new.tex <==
%\par\textcolor{red}{DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%}
%\endinput

\begin{figure}
	\centering
\begin{diagram}%[small]
(1)\quad&&&\alalenscatdif&&&&&&&
\\ % row 2
(2)\quad&&
\ldTo^{{-}\lens}
\ruDashto(2,6)^{\grt{\leefunovr}\qquad\qquad\qquad\qquad}
&%\mbox{[j-monic]}
&
\rdTo^{{-}\dif}
\rdTo(5,2)^\codiscr_{
\begin{array}{c}
	{}_{[\noteq^?]}
\end{array}
}& &&&&&
\\ % row 3
(3)\quad&
\pspadifcat
&&\uDashto~{\blt{[\plusx{\nix},\!\plusx{\nix}]}}
%\pile{\rTo^{}}
&&\qquad\alalenscat&
&\lEmbed
&\alalenscatcodi&~=\learncat	
\\ % row 4
(4)\quad&&\rdTo^{{-}\dif}\luTo(2,4)<{\grt{\qquad\qquad\plusxdif}}
&&\ldTo^{{-}\putl}\ruTo(2,4)>{\grt{\plusxput\qquad\qquad}}%\ruTo(5,2)^\codiscr
&&%[\noteq]
&\ldTo(2,2)^{{-}\putl^0}
\ruDashto(2,4)>{\blt{{\plusxput^0}}}
&\ruDashto(2,4)>{\grt{L_{\eps,\err}}}
&
\\ % row 5
(5)\quad&&&\pcatcat&
&\lEmbed%\rTo^{{-}\mathsf{arrows}}
&\psetcat&&&&
\\ % row 6
(6)\quad &&& \uTo<{{-}\nix\!\!}
&&&
\uTo<{({-}\nix)^0}
&&&&
\\ % row 7
(7)\quad&
\grt{\paracatrcat}&\rEQ&
\grt{\pgetcat_\nix}&& 
\pile{\rTo^{\grt{\minusxdel}\quad}_{\grt{\congx{\nix}}}
	\\
	\lTo_{\grt{\plusxdel}~~}}
&\grt{\pgetcat^0_\nix}&~=\grt{\paracat_\reals}&&&
\end{diagram}
\caption{Building codiscrete lenses}\label{fig:codifun-big}
\end{figure}



==> ll-figures/diags/codifun-small-noteq-learner.tex <==
%\par\textcolor{red}{DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%}
%\endinput
{
	\renewcommand\grt[1]{#1}
\begin{figure}[h]
	\centering
\begin{diagram}[w=2ex,h=2em]%[small] %[w=2ex,h=4ex]%[small]
	 % row 1
	&&%\quad
\alalenscatdif%_{{-}\difputlaw}\quad
	&&& &&&
	\\ % row 2
	&%\quad
	\ldTo(2,5)^{\qquad\qquad\minusput}
&&
    \rdTo(2,5)^{\minusdif\qquad\qquad}
    \rdTo(4,5)^{\codifun}_{(2)} %{\redt{\mbox{not a functor}}}
	&&& &&
	\\ % row 2+
	&&\dEmbedDashed>{!}&& &&&&
\\	% row 3 ----
&&%\quad
\begin{array}{c}
	%\\	
	\alalenscatdif_{{-}\difputlaw}
%	\\ [-7.5pt]
%	\footnotesize{\text{without}\difputlaw}
\end{array} %{\mbox{-}} %wbdif}}\quad %\alalenscatdif\quad
 &&& &&&
\\ % row 4 -----
&
\ldDashto
%--\ruDashto(2,6)^{\grgrt{\leefunovr}\qquad\qquad\qquad\qquad}
& %\mbox{\footnotesize\sf [j-monic]}
&
\rdDashto
\rdDotto(4,2)~{\redt{\langle\text{not a functor}\rangle} %\redt{(3)}
%\begin{array}{c}
%	\\ [-15.5pt]
%	{\redt{\footnotesize\text{not a functor}}}
%\end{array}
}
& &&
\\ % row 5 -------
%\qquad
\pgetdifcat
&& 
(1)   
&&\alalenscat
&\lEmbed_{\plusx{\pairing}\deltas\qqquad}
&\alalenscatcodi
&\pile{
\rTo^{{-}\putl^0(\id)} 
\\
\lTo_{{+}\putl^0(\id)}
}
&\learncat
%	
\\ % row 6----------------
&
\rdTo(2,2)^{~~\minusdif}
%---\luTo(2,4)<{\grt{\qquad\qquad\plusxdif}}
&&
\ldTo(2,2)^{\minusput~~}
%_{\mbox{\footnotesize
%	\qquad\begin{tabular}{l}
%		\\ [-17.5pt]
%		also~forgets 
%		\\ [-7.5pt]
%		model space 
%			\\ [-7.5pt]
%		properties
%	\end{tabular}
%}}
%---\ruTo(2,4)>{\plusxput\qquad\qquad}<{(*)\qquad\qquad}%\ruTo(5,2)^\codiscr
&\qqquad\qquad (3) &%[\noteq]
\ldTo(1,2)_{\minusputcodi}
& &%----\ruDashto(2,4)>{\grgrt{L_{\eps,\err}}}
\ldTo(1,2)>{{-}\putl^L}
&
\\ % row 7 ----------
&&\pgetcat%_{(*)}
&
&\lEmbed_{\plusx{\pairing}\deltas\qqquad} 
& \pgetcat^0
&\pile{
	\lTo^{all=} \\ \lTo_{all\sim}
}
&\psetcat&&
\\ % row 8 ===
&&
\dEmbed<{\minusspaprop}>{\qqquad(4)}
%%  \mbox{\footnotesize
%%			\qquad\begin{tabular}{l}
%%				\\ [-17.5pt]
%%				also~forgets 
%%				\\ [-7.5pt]
%%				model space 
%%					\\ [-7.5pt]
%%				properties
%%			\end{tabular}
%\begin{array}{l}
%	{-}\mathsf{space}
%	\\ [-7.5pt]
%	\mathsf{properties}
%\end{array}
%		}>{\qqquad(4)}
&&
\ldEmbedDashed(3,2)_{\plusx{\pairing}\arrows}
&
\dTo>{\minusspaprop}
&&
\\ % row 9
&&\pcatcat&&&
\pcatcat^0
&
\end{diagram}
\vspace{-0.5cm}
\caption{From lenses with diff to codiscrete lenses}
\label{fig:codifun-1}
\end{figure}
}  % end renew grt


==> ll-figures/diags/codifun-small.tex <==
%\par\textcolor{red}{DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%	DRAWING THE  diagram is not enabled
%}
%\endinput
{
	\renewcommand\grt[1]{#1}
\begin{figure}[h]
	\centering
\begin{diagram}[w=8ex,h=4ex]%[small]
	 % row 1
	&&%\quad
	\alalenscatdif%_{{-}\difputlaw}\quad
	&&& &&&
	\\ % row 2
	&%\quad
	\ldTo(2,5)^{\qquad\qquad\minusput}
&&
    \rdTo(2,5)^{\minusdif\qquad\qquad}
    \rdTo(4,5)^{\codifun}_{(2)} %{\redt{\mbox{not a functor}}}
	&&& &&
	\\ % row 2+
	&&\dEmbedDashed>{!}&& &&&&
\\	% row 3 ----
&&%\quad
\begin{array}{c}
	%\\	
	\alalenscatdif_{{-}\difputlaw}
%	\\ [-7.5pt]
%	\footnotesize{\text{without}\difputlaw}
\end{array} %{\mbox{-}} %wbdif}}\quad %\alalenscatdif\quad
 &&& &&&
\\ % row 4 -----
&
\ldDashto
%--\ruDashto(2,6)^{\grgrt{\leefunovr}\qquad\qquad\qquad\qquad}
& %\mbox{\footnotesize\sf [j-monic]}
&
\rdDashto
\rdDotto(4,2)~{\redt{\langle\text{not a functor}\rangle} %\redt{(3)}
%\begin{array}{c}
%	\\ [-15.5pt]
%	{\redt{\footnotesize\text{not a functor}}}
%\end{array}
}
& &&
\\ % row 5 -------
%\qquad
\pgetdifcat
&& 
(1)   &&\alalenscat
&\lEmbed_{\plusx{\pairing}\deltas\qqquad}
&\alalenscatcodi
&(\grt{\mbox{a.k.a. \learncat}})	
\\ % row 6----------------
&
\rdTo^{~~\minusdif}
%---\luTo(2,4)<{\grt{\qquad\qquad\plusxdif}}
&&
\ldTo^{\minusput~~}
%_{\mbox{\footnotesize
%	\qquad\begin{tabular}{l}
%		\\ [-17.5pt]
%		also~forgets 
%		\\ [-7.5pt]
%		model space 
%			\\ [-7.5pt]
%		properties
%	\end{tabular}
%}}
%---\ruTo(2,4)>{\plusxput\qquad\qquad}<{(*)\qquad\qquad}%\ruTo(5,2)^\codiscr
&\qqquad\qquad (3) &%[\noteq]
\ldTo(1,2)_{\minusputcodi}
%\ruDashto(2,4)>{\blt{{\plusxput^0}}}
& %----\ruDashto(2,4)>{\grgrt{L_{\eps,\err}}}
&
\\ % row 7
&&\pgetcat%_{(*)}
&
&\lEmbed_{\plusx{\pairing}\deltas\qqquad} 
&\psetcat&&&&
\\ % row 8 ===
&&\dEmbed<{
%  \mbox{\footnotesize
%			\qquad\begin{tabular}{l}
%				\\ [-17.5pt]
%				also~forgets 
%				\\ [-7.5pt]
%				model space 
%					\\ [-7.5pt]
%				properties
%			\end{tabular}
\begin{array}{l}
	{-}\mathsf{space}
	\\ [-7.5pt]
	\mathsf{properties}
\end{array}
		}>{\qqquad(4)}
&&
\ldEmbedDashed(3,2)_{\plusx{\pairing}\arrows}
&&&
\\ % row 9
&&\pcatcat&&&&
\end{diagram}
\vspace{-0.5cm}
\caption{From lenses with diff to codiscrete lenses}
\label{fig:codifun-1}
\end{figure}
}  % end renew grt


==> ll-figures/diags/codifun-triangle.tex <==
%\begin{figure}
\begin{wrapfigure}{R}{0.425\textwidth}
	\renewcommand\grt[1]{#1}
\vspace{-1.75cm}
	\centering
\[
\begin{diagram}%[small]
\\ % row 1
\grt{\aladlenscat}
&&\rTo^{\codifun}
&&\alalenscatcodi
\\ % row 2
&\rdTo<{{-}\dif}
&\textcolor{red}{[=]^?}%{[\noteq^?]}
&\ldEmbed>{\plusx{\pairing}\deltas}
& 
\\ % row 3
&&\alalenscat
&&
\end{diagram}
\]
\vspace{-0.55cm}
\caption{%\parbox{0.3\textwidth}{}
From alad-lenses to codiscrete ala-lenses}
\label{fig:codifun-triangle}
\end{wrapfigure}
%\end{figure}
%\vspace{-0.55cm}

==> ll-figures/diags/codifun.tex <==
% colors
\newcommand\differ{\enma{\diagopername{differ}}}
\newcommand\lens{\enma{\diagopername{lens}}}
\newcommand\grt[1]{\textcolor{caribbeangreen}{#1}}
\newcommand\blt[1]{\textcolor{blue}{#1}}
\begin{figure}
	\centering
\begin{diagram}%[small]
(1)\quad&&&\alalenscatdif&&&&&&&
\\ % row 2
(2)\quad&&\ldTo^\differ&%\mbox{[j-monic]}
&\rdTo^{\lens}\rdTo(5,2)^\codiscr& &&&&&
\\ % row 3
(3)\quad&\pcatcatdif&&\uDashto>{\blt{\plusx{\nix}\!\!\plusx{\nix}}}
%\pile{\rTo^{}}
&&\alalenscat&&&\alalenscatcodi&~=\learncat	
\\ % row 4
(4)\quad&&\rdTo^{{-}\dif}\luTo(2,4)<{\grt{\qquad\qquad\plusxdif}}
&&\ldTo^{{-}\putl}\ruTo(2,4)>{\grt{\plusxput\qquad\qquad}}%\ruTo(5,2)^\codiscr
&&&
\ldTo(2,2)^{{-}\putl^0}
\ruDashto(2,4)>{\blt{{\plusxput^0}}}
&\ruDashto(2,4)>{\grt{L_{\eps,\err}}}
&
\\ % row 5
(5)\quad&&&\pcatcat&&\rTo^{{-}\mathsf{arrows}}&\psetcat&&&&
\\ % row 6
(6)\quad &&& \uTo<{{-}\nix\!\!}
&&&\uTo<{{-}^0\nix}
&&&&
\\ % row 7
%(5)\quad&&&\pcatcat&&\rTo^{{-}\mathsf{arr.}}&\psetcat&&&&
(7)\quad&&&\grt{\pgetcat_\nix}&& \pile{\rTo^{\grt{{-}\deltas}\quad}
	\\
	\lTo_{\grt{\plusxdel}~~}}
&\grt{\pgetcat^0_\nix}&~=\grt{\paracat}&&&
\end{diagram}
\caption{Building codiscrete lenses}\label{fig:codi}
\end{figure}



==> ll-figures/diags/diag-aalens-compose.tex <==
%\begin{figure}
	\begin{wrapfigure}{R}{0.375\columnwidth}
		\vspace{-0.75cm}
		\centering


{ % begin group
%	\renewcommand\geti{\enma{\get1}}
%	\newcommand\getii{\enma{\get2}}
	\newcommand\getio{\enma{\get1_0}}
	\newcommand\getiio{\enma{\get2_0}}
\begin{tabular}{c}%{c@\quad c}
%\begin{diagram}[w=1.05\cellW,h=1.1\cellH] %(a)
%\dbox{A} & \rCorrto^r     & \dbox{B} & \rCorrto^{r} & \dbox{A}%
%               &  \rCorrto^{r} & \dbox{B}
%\\%
%\dCorrto<a & \seTilearrow{\fppg}~~~ & \dDercorrto>b %
%                 & \seTilearrow{\bppg}~~~ & \dDercorrto>{a_1}
%                  & \seTilearrow{\fppg}~~~ & \dDercorrto>b
%\\%
%\dbox{A'} & \rDercorrto^{r'}  & %
%B'            & \rDercorrto^{r_1'} & A_1' %
%               & \rDercorrto^{r_1'} & B'
%\end{diagram}%
% &
\begin{diagram}[w=1.1\cellW,h=1.1\cellH] %(a)
\dbox{A} 
& \rMapsto^{{:}\getio}  & \dbox{B} 
& \rMapsto^{{:}\getiio} &  \dbox{C}%
\\% row 2
\dDashto<u & \swTilearrow{\putl{1}_A}~~~ & \dDerupdto>{v} %
                 & \swTilearrow{\putl2_B} ~~~& \dDerupdto>{w} 
\\% row 3
{A'} & \rDermapsto_{{:}\getio}  & %
 B'            & \rDermapsto_{{:}\getiio} & C' %
\end{diagram}%
\\[30pt]
%(a) \fbfppglaw\ law  & (b) \bfbppglaw\ law
\end{tabular}
} % end group
\caption{Lens composition} %
\label{fig:alens-compose}%
\end{wrapfigure}
%\end{figure}


==> ll-figures/diags/diag-monotonPpgPpg.tex <==
\newarrow{Updto}----{>}
\newarrow{Derupdto}{}{dash}{}{dash}{>}

%-- version with letters A,B
\begin{wrapfigure}{R}{0.45\textwidth}
\vspace{-0.1cm}%
%\centering
\begin{tabular}{c@{\qquad}c} %@{\qquad}c@{\qquad}c}
%\multirow{2}{*}{%
    \begin{diagram}[w=\cellW,h=\cellH] %(a)
\dbox{A} & \rCorrto^r &\dbox{B}\\%
\dUpdto<a & \seTilearrow{\fppg}~~~
            & \dDerupdto>b \\%
\dbox{A'} & \rDercorrto^{r'} & B'  \\%
\dUpdto<{a'} & \seTilearrow{\fppg}~~~
            & \dDerupdto>b'\\%
            \dbox{A''} & \rDercorrto^{r''} & B''%
             &&\\
\end{diagram}%
% }%
  & %
%\multirow{2}{*}{%
    \begin{diagram}[w=\cellW,h=\cellH] %(a)
\dbox{A} & \rCorrto^r &\dbox{B}\\%
\uUpdto<a & \seTilearrow{\fppg}~~~
            & \uDerupdto>b \\%
\dbox{A'} & \rDercorrto^{r'} & B'  \\%
\uUpdto<{a'} & \seTilearrow{\fppg}~~~
            & \uDerupdto>b'\\%
            \dbox{A''} & \rDercorrto^{r''} & B''%
            &&\\
\end{diagram}%
% }%
\end{tabular}
\caption{Monotonic (\ppgppglaw) laws \label{fig:monot-PpgPpg}}%
\vspace{-0.1cm}
\end{wrapfigure}

\endinput


%%== version with bullets and \circ s =beginFigure
%\begin{wrapfigure}{l}{.25\textwidth}%
%\vspace{-2ex}%
\begin{figure}
\centering
\begin{tabular}{c@{\quad}c@{\quad}c@{\quad}c}
\begin{diagram}[w=\cellW,h=\cellH] %(a)
\bullet & \rCorrto &\bullet\\%
\dUpdto & %\ruDercorrto_{} &\\%
            & \dDerupdto \\%
\bullet & \rDercorrto^{} & \circ
\end{diagram}%
&%
\begin{diagram}[w=\cellW,h=\cellH] %(b)
\bullet & \rCorrto &\bullet\\%
\dDerupdto & %\ruDercorrto_{} &\\%
            & \dUpdto \\%
\circ & \rDercorrto^{} & \bullet
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (c) was (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dUpdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dDerupdto>{\ide{}{}} \\%
\bullet & \rDercorrto^{r} & \circ
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dDerupdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dUpdto>{\ide{}{}} \\%
\circ & \rDercorrto^{r} & \bullet
\end{diagram}%
\\[30pt]
(a) \fppg{} & (b) \bppg{} & %
%(c) f-commutativity &
\multicolumn{2}{c}{(c) (\idppglaw) law}
\end{tabular}
\caption{Update propagation operations (a,b)
and their laws \label{fig:lens-oper}}%
\end{figure}
%\vspace{-7ex}
%\end{wrapfigure}
%===EndFigure


==> ll-figures/diags/diag-trafoGetPut.tex <==
\newarrow{Viewto}===={=>}
\newarrow{Derviewto}{=}{}{=}{}{=>}
\newarrow{Updto}{<}---{>}
\newarrow{Derupdto}{<}{dash}{}{dash}{>}
%
\begin{wrapfigure}{R}{.375\textwidth}
\vspace{-0.5cm}%
%\centering%
\begin{tabular}{c}
% metarow
\begin{diagram}[w=1.1\cellW,h=1.1\cellH] %(a)[small]
\dbox{M} &\lViewto^{m} & \dbox{MN} &\rViewto^{n}&\dbox{N}\\%
\end{diagram}   %
\\[25pt]
 %
\begin{diagram}[w=1.1\cellW,h=1.1\cellH] %(a)
\dbox{A} & \lViewto^{\cartliarr{m}{A}}  & \dbox{R} %
               & \rViewto^{\cartliarr{n}{B}} & \dbox{B}%
            \\%
\dUpdto<a & \seTilearrow{\get{m}}~~~ & \dDerupdto>{} %
                 & \seTilearrow{\put{n}}~~~ & \dDerupdto>{b}
             \\%
\dbox{A'} & \lDerviewto^{\cartliarr{m}{A}'}  & R' %
               & \rDerviewto^{\cartliarr{n}{B}'}   & B' %
\end{diagram}%
\end{tabular}  %
%\vspace{-1ex}%
\caption{Model transformation via GetPut-decomposition%
\label{fig:trafo-as-getput}}%
%\vspace{-0.2cm}
\end{wrapfigure}%

\endinput
% old version with pptx figures
\begin{wrapfigure} {R}{0.326\textwidth}%
\vspace{-0.5cm}%
\includegraphics[width=0.325\columnwidth]{trafo-as-get-put}%
\caption{Model transformation via GetPut-decomposition}%
\label{fig:trafo-as-getput}%
\vspace{-0.2cm}%
\end{wrapfigure}%
%\end{figure}


==> ll-figures/diags/dif-space-triangle.tex <==
%\begin{figure}
\begin{wrapfigure}{R}{0.45\textwidth}
	\renewcommand\grt[1]{#1}
\vspace{-1.75cm}
	\centering
\[
\begin{diagram}%[small]
\\ % row 1
\grt{\pspadifcat}
&&\rTo^{{-}\dif}
&&\pcatcat%\alalenscat
\\ % row 2
&\luTo<{\plusx{\pairing}\dif}
&%(*)
&\ruEmbed>{\plusx{\pairing}\arrows}
& 
\\ % row 3
&&\psetcat
&&
\end{diagram}
\]
\vspace{-0.55cm}
%\caption{%\parbox{0.3\textwidth}{
%}}
\label{fig:difspa-triangle}
\end{wrapfigure}
%\end{figure}
%\vspace{-0.55cm}

==> ll-figures/diags/funofput.tex <==
%\begin{figure}
\begin{wrapfigure}{R}{0.5\textwidth}
\vspace{-1cm}
	\centering
\[
\begin{diagram}[h=2.5em]%[small]
% row 00
%&\spP_1&&\spP_2&&\spP_3&
\\  % row 01
  \spA_1&\rTo_{\get^1_{p_1}}^{{p_1\in\spP_1}}
&\spA_2&\rTo_{\get^2_{p_2}}^{{p_2\in\spP_2}} 
&\spA_3&\rTo_{\get^3_{p_3}}^{{p_3\in\spP_3}} 
& \spA_4
\\ % row 02
&&& &&&
\\ %row 1
   \dbox{A_1}&\rDermapsto^{{:}\get^1_{p_1}}
&A_2&\rDermapsto^{{:}\get^2_{p_2}}
&A_3&\rDermapsto^{{:}\get^3_{p_3}}
&A_4
\\ % row 2
&&&&&
%--begin triple arrow label
&\dTo>{u_4}
\\ % row 3
&&&&\dDotto<{u_3}&
%--begin triple arrow label
\swssseTilearrowAB{1{:}\putl^3}{}
&\dbox{A'_4}
\\ % row 4
&&\dDotto<{u_2}&
&&&\dDotto<{u_4^@}
\\ % row 5
&&&
% begin triple arrow label
\swssseTilearrowAB{2{:}\putl^2}{}
&A'_3
&\rDashmapsto^{{:}\get^3_{p'_3}}&{A'}_4^@
\\ %row 6
\dDotto<{u_1}&&&&\dDotto<{u_3^@}&\stackrel{4{:}\get^3_{e_3}}{\Rightarrow}&\dDashto
\\ % row 7
&\swssseTilearrowAB{3{:}\putl^1}{}&A'_2&\rDashmapsto^{{:}\get^2_{p'_2}}&{A'}_3^@&\rDashmapsto^{{:}\get^3_{p'_3}}&\circ
\\ % row 8
&&\dDotto<{u_2^@}&\stackrel{5_1{:}\get^2_{e_2}}{\Rightarrow}
&\dDashto&\stackrel{5_2{:}\get^3_{e_3}}{\Rightarrow}&\dDashto
\\ % row 9
A'_1&\rDermapsto^{{:}\get^1_{p'_1}}&{A'}_2^@&\rDashmapsto^{{:}\get^2_{p'_2}}
&\circ
	&\rDashmapsto^{{:}\get^3_{p'_3}}&\circ
\end{diagram}
\]
%\end{document}
\caption{Functoriality of update propagation policies}
\label{fig:funofput}
\end{wrapfigure}
%\end{figure}

==> ll-figures/diags/horCompose.tex <==
\begin{figure}
	\centering
\[
\begin{diagram}%[small]
% row 00
%&\spP_1&&\spP_2&&\spP_3&
\\  % row 01
  \spA_1&\rTo_{\get1_{p_1}}^{{p_1\in\spP_1}}
&\spA_2&\rTo_{\get2_{p_2}}^{{p_2\in\spP_2}} 
&\spA_3&\rTo_{\get3_{p_3}}^{{p_3\in\spP_3}} 
& \spA_4
\\ % row 02
&&& &&&
\\ %row 1
   A_1&\rDermapsto^{{:}\get1_{p_1}}
&A_2&\rDermapsto^{{:}\get2_{p_2}}
&A_3&\rDermapsto^{{:}\get3_{p_3}}
&A_4
\\ % row 2
&&&&&
%--begin triple arrow label
&\dTo>{u_4}
\\ % row 3
&&&&\dDotto<{u_3}&
%--begin triple arrow label
\swssseTilearrowAB{1{:}\putl3}{}
&A'_4
\\ % row 4
&&\dDotto<{u_2}&
&&&\dDotto<{u_4^@}
\\ % row 5
&&&
% begin triple arrow label
\swssseTilearrowAB{2{:}\putl2}{}
&A'_3
&\rDotto^{{:}\get3_{p'_3}}&{A'}_4^@
\\ %row 6
\dDotto<{u_1}&&&&\dDotto<{u_3^@}&\stackrel{4{:}\get3_{p'_3}}{\Rightarrow}&\dDashto
\\ % row 7
&\swssseTilearrowAB{3{:}\putl1}{}&A'_2&\rDotto^{{:}\get2_{p'_2}}&{A'}_3^@&\rDashto^{{:}\get3_{p'_3}}&\bullet
\\ % row 8
&&\dDotto<{u_2^@}&\stackrel{5_1{:}\get_{p'_2}}{\Rightarrow}
&\dDashto&\stackrel{5_2{:}\get_{p'_3}}{\Rightarrow}&\dDashto
\\ % row 9
A'_1&\rDotto^{{:}\get1_{p'_1}}&{A'}_2^@&\rDashto^{{:}\get2_{p'_2}}&\bullet
	&\rDashto^{{:}\get3_{p'_3}}&\bullet
\end{diagram}
\]
%\end{document}
\caption{Functoriality of update propagation policies}
\label{fig:funofput}
\end{figure}


==> ll-figures/diags/lawvereLensSquare.tex <==
%\begin{figure}
\begin{wrapfigure}{R}{0.375\columnwidth}
	\vspace{-0.5cm}
	\centering
	\begin{diagram}[small]
		\paracaterr&\rMonic^{\mathsf{wide}}&\paracat \\
		\dTo<{L_{\eps,\pol(\err)}}&&\dTo>{L_{\eps,\err}} \\
		\allenscat(\lmp)&\rTo^{\tfun}&
		\begin{array}{c}
			\mbox{$\allenscat(\tcat)$} \atop
			\mbox{=\learncat}
		\end{array}
		\end{diagram} 
	%\caption{}
	\label{fig:metricSq}
	\vspace{-5mm}
\end{wrapfigure}
%\end{figure}
%


\endinput
%\begin{figure}
\begin{wrapfigure}{R}{0.31\columnwidth}
\vspace{-0.5cm}
\centering


%\caption{}
\label{fig:lawvereLensSq}
\vspace{-10mm}
\end{wrapfigure}
%\end{figure}

==> ll-figures/diags/lens-as-mealy.tex <==
\newcommand\Inx[1]{\enma{\mathit{In}_{{#1}}}}
\newcommand\Outx[1]{\enma{\mathit{Out}_{{#1}}}}
\newcommand\InA{\Inx{\spA}}
\newcommand\InB{\Inx{\spB}}
\newcommand\Inget{\Inx{\get}}
\newcommand\Input{\Inx{\putl}}
\newcommand\Outget{\Outx{\get}}
\newcommand\Output{\Outx{\putl}}

\newcommand\igpxy[2]{\enma{\mathit{i}_{\mathsf{#1#2}}}}
    \newcommand\igo{\igpxy{g}{0}}
	\newcommand\igi{\igpxy{g}{1}}
\newcommand\ogpxy[2]{\enma{\mathit{o}_{\mathsf{#1#2}}}}
	\newcommand\ogo{\ogpxy{g}{0}}
	\newcommand\ogi{\ogpxy{g}{1}}
	
%\newcommand\igpxy[2]{\enma{\mathit{i}_{\mathsf{#1#2}}}}
   \newcommand\ipo{\igpxy{p}{0}}
   \newcommand\ipi{\igpxy{p}{1}}
%\newcommand\ogpxy[2]{\enma{\mathit{o}_{\mathsf{#1#2}}}}
   \newcommand\opo{\ogpxy{p}{0}}
    \newcommand\opi{\ogpxy{p}{1}}
	

%\newcommand\ogx[1]{\enma{In_{{#1}}}}
%\newcommand\{\Inx{\spA}}
%\newcommand\InB{\Inx{\spB}}


\newcommand\spobx[1]{\enma{#1_0}}
\newcommand\sparrx[1]{\enma{#1_1}}
\newcommand\spoba{\spobx{\spA}}
\newcommand\spobb{\spobx{\spB}}
\newcommand\sparra{\sparrx{\spA}}
\newcommand\sparrb{\sparrx{\spB}}
\newcommand\spobR{\spobx{\spR}}
\newcommand\sparrR{\sparrx{\spR}}


\begin{diagram}
%  row 1
\Inget&&&&\rTo^\get &&&&	\Outget
\\ % ---> row 2 DIAGONALS
          &\rdTo(1,2)<{\igi} \rdTo(3,2)>{\igo}
          &&(1)& &&&\ldTo(5,2)<{\ogo} \ldTo(1,2)>{\ogi} 
          &
%\\ % row 3 foir the symmetric case
%&	\sparra
%	&\pile{\rTo^\so \\  \rTo_\ta}
%	&\spoba &\lTo_{a}&\spobR&\rTo_{b}&\spobb
%	&\pile{\lTo^\ta \\ \lTo_\so}
%	&\sparrb
%	&
\\ % row 3 for the asymmetric case
&	\sparra
	&\pile{\rTo^{\so
%	\begin{array}{cc}
%		(1) &~~~~~~~~\\
%		\so &
%	\end{array}
}
	 \\  \rTo_{\ta
%	\begin{array}{cc}
%\ta &\\
%		(6) &~~~~~~~~
%\end{array}	 
}}
	&\spoba &\rTo^{\get_0}%\spobR&\rTo_{b}
	&\spobb
	&\pile{\lTo^{\ta
%			\begin{array}{cc}
%			&	(3) \\
%			~~~~~~~~\ta &\\
%					\end{array}	
		}
	 \\ \lTo_\so}
	&\sparrb
	&
\\ % ROW 4 DIAGONALS 
	\ruTo(1,2)<{\opi}&&\ruTo(3,2)>{\opo}
	&(2)& \luTo(5,2)_{\ipo}&&&& \luTo(1,2)>{\ipi} 
\\%  row 5
\Output&&&&\lTo^\putl&&&&	\Input
\end{diagram}

==> ll-figures/diags/lens-compose_a+aa_.tex <==

%\begin{figure}
%\begin{wrapfigure}{R}{0.55\textwidth}
%\vspace{-0.4cm}
%	\centering
\begin{tabular}{l}
%	$
%   \begin{diagram}[w=1.1\cellW,h=0.9\cellH] %(a)
%	\dbox{A} 
%	& \rMapsto^{{:}\getio}  & {B} 
%	& \rMapsto^{{:}\getiio} &  {C}%
%	\\% row 2
%	\dDotto<u & \swTilearrow{\putl{1}_A}~~~ & \dDotto>{v} %
%	& \swTilearrow{\putl2_B} ~~~& \dTo>{w} 
%	\\% row 3
%	{A'} & \rDermapsto_{{:}\getio}  & %
%	B'            & \rDermapsto_{{:}\getiio} & \dbox{C'} %
%\end{diagram}%
%$
%\\ [7.5ex]
%(a) ordinary lens composition
%\\ [10pt]
$
\begin{diagram}[h=2.em]%[small]
 %row 1
\dbox{A}&\rDermapsto^{{:}\get1_{0}}
&B&\rDermapsto^{{:}\get2_{0}}
&C
\\ % row 2
&&&& \dTo>{w}
\\ % row 3
&& %\dDotto<{v}
&
%--begin triple arrow label
\swseTilearrowABx{1{:}\putl2_{B}}{}
&\dbox{C'}
\\ % row 4
%\dDotto<{u}
&&
\dDotto>{v}
&&\dDotto<{w^@}
\\ % row 5
%&&
&
% begin triple arrow label
\swseTilearrowABx{2{:}\putl1_{A} }{}
&B'
&\rDashmapsto^{{:}\get2_{0}}&{C'}^@
\\ %row 6
\dDotto>{u} 
&&\dDotto<{v^@}&\stackrel{3{:}\get2}{\Rightarrow}&\dDashto>{v^@.\get2}
\\ % row 7
%&\swssseTilearrowABx{3{:}\putl^1_{A_1,p_1}}{e_1}&
A'&\rDashmapsto^{{:}\get1_{0}}&{B'}^@&\rDashmapsto^{{:}\get2_{0}}
&C'^{@@}%\circ
\end{diagram}
$
%\\ [15ex]
%(b)  lenses with amendment 
\end{tabular}
%%\end{document}
%\caption{Composition of lenses}
%\label{fig:aaalenscompose}
%\end{wrapfigure}
%\end{figure}

==> ll-figures/diags/policyfun-2triangles.tex <==

%\begin{figure}
\begin{wrapfigure}{R}{0.35\textwidth}
%\vspace{-1cm}
	\centering
\[
\begin{diagram}%[small]
% row 1----
&&&&&& 
\alalenscat^0
\\ % row--- 2===
&&&&&
\ruDashto(6,2)^{\plusxputcodi}
\ldEmbed(2,2)<{\fu}
\ldTo(4,6)>{{-}\putl^0} 
&
\\ % row--- 3
 \pgetcatnix
&&
\rTo^{~~~~\plusxput}_%
	{\begin{array}{c}
		\\ [-20pt]
	\minusnixbra
%	\\ [-3.5pt]
%	~~{}_{(*)}
	\end{array}}
&&
\alalenscat~~
&&
\\ %--- row 4
&
\rdDashto(2,4)_{\minusnixcodi}%<{({-}\nix)^0}
\rdTo(2,2)>{\minusnix}
& (1) &
\ldTo(2,2)<{\minusput}_{
	\begin{array}{c}
	(2)
\end{array}
}
&&&
\\ %-- row 5
&&\pcatcat&&&&
\\ %--- row 6
&& 
\uEmbed>\fu 
&&&&
\\  %--- row 7
%&&
&&\psetcat&&&&
\end{diagram}
\]
\caption{Change propagation systems}
\label{fig:policyfun}
\end{wrapfigure}
%\end{figure}


==> ll-figures/diags/policyfun-2tringles.tex <==

%\begin{figure}
\begin{wrapfigure}{R}{0.6\textwidth}
%\vspace{-1cm}
	\centering
\[
\begin{diagram}%[small]
% row 1----
%\pgetnixcatcodi
&&&&
%\rDotto(8,2)^{\plusxput^0}_{\minusnixcodibra}%{[({-}\nix)^0]}
&&
&%\rEQ
& \alalenscat^0
\\ % row 2===
%\dEQ 
&  
%\rdDotto(4,6)<{\minusnixcodi} %{({-}\nix)^0}
%\rdFEmbDot(3,2)^{\congx{\nix}}  %\rdEQ %\rdFEmbDash(2,2) 
&&&&
&&
%\ruDotto(8,1)^{\plusxput^0~[({-}\nix)^0]}
%\ruDotto(8,2)^{\plusxput^0~[({-}\nix)^0]}
%&&
\ruDashto(5,2)^{\plusxput^0}%^{\plusxput^0~[({-}\nix)^0]}  
\ldEmbed(2,2)<{\fu}
\ldTo(4,6)>{{-}\putl^0} 
&
\\ % row 3
 &&&
\pgetcat_\nix
&%&
\rTo^{~~~~\plusxput}_%
	{\begin{array}{c}
		\\ [-20pt]
	\minusnixbra
	\\ [-3.5pt]
	~~{}_{(*)}
	\end{array}}
&&
\alalenscat~~
&&
\\ % row 4
&%\rdDotto(4,4)<{({-}\nix)^0}
&&&
\rdDashto(1,4)_{\minusnixcodi}%<{({-}\nix)^0}
\rdTo(1,2)>{{-}\nix}
& 
\ldTo(2,2)<{{-}\putl}
&
\\ % row 5
&&&&\pcatcat&&&&
\\ % row 6
&&&& 
\uEmbed>\fu 
&&&&
\\  % row 7
&&&&\psetcat&&&&
\end{diagram}
\]
\caption{Functoriality of update propagation policies}
\label{fig:policyfun}
\end{wrapfigure}
%\end{figure}


==> ll-figures/diags/policyfun-3tringles.tex <==

%\begin{figure}
\begin{wrapfigure}{R}{0.6\textwidth}
%\vspace{-1cm}
	\centering
\[
\begin{diagram}%[small]
% row 1----
\pgetnixcatcodi
&&&&\rDotto(8,2)^{\plusxput^0}_{\minusnixcodibra}%{[({-}\nix)^0]}
&&
&%\rEQ
& \alalenscat^0
\\ % row 2
%\dEQ 
&  
\rdDotto(4,6)<{\minusnixcodi} %{({-}\nix)^0}
\rdFEmbDot(3,2)^{\congx{\nix}}  %\rdEQ %\rdFEmbDash(2,2) 
&&&&
&&
%\ruDotto(8,1)^{\plusxput^0~[({-}\nix)^0]}
%\ruDotto(8,2)^{\plusxput^0~[({-}\nix)^0]}
%&&
\ruDashto(5,2)^{\plusxput^0}%^{\plusxput^0~[({-}\nix)^0]}  
\ldEmbed(2,2)<{\fu}
\ldTo(4,6)>{{-}\putl^0} 
&
\\ % row 3
 &&&
\pgetcat_\nix
&%&
\rTo^{~~~~\plusxput}_%
	{\begin{array}{c}
		\\ [-20pt]
	\minusnixbra
	\\ [-3.5pt]
	~~{}_{(*)}
	\end{array}}
&&
\alalenscat~~
&&
\\ % row 4
&%\rdDotto(4,4)<{({-}\nix)^0}
&&&
\rdDashto(1,4)_{\minusnixcodi}%<{({-}\nix)^0}
\rdTo(1,2)>{{-}\nix}
& 
\ldTo(2,2)<{{-}\putl}
&
\\ % row 5
&&&&\pcatcat&&&&
\\ % row 6
&&&& 
\uEmbed>\fu 
&&&&
\\  % row 7
&&&&\psetcat&&&&
\end{diagram}
\]
\caption{Functoriality of update propagation policies}
\label{fig:policyfun}
\end{wrapfigure}
%\end{figure}


==> ll-figures/diags/policyfun-bigTri-OLD_defVersion_.tex <==

%\begin{figure}
\begin{wrapfigure}{R}{0.5\textwidth}
%\vspace{-1cm}
	\centering
\[
\begin{diagram}%[small]
%\pgetcat_\nix &&&\rDashto^{\plusxput_0} &&& \alalenscat_0
&&&& &&&& \alalenscat^0
\\ % row 2
&%\rdEQ %\rdFEmbDash(2,2) 
&&&&&&\ruDashto(6,2)^{\plusxput^0}  \ldWEmbDot(2,2)<{\fu}\ldDashto(4,6)>{{-}\putl^0} &
\\ % row 3
&&\pgetcat_\nix&&\rTo^{\plusx{\nix}\putl} &&\alalenscat&&
\\ % row 4
&&&\rdDashto(2,4)<{{-}^0\nix}\rdTo(2,2)>{{-}\nix}&(*)&\ldTo(2,2)<{{-}\putl}&
\\ % row 5
&&&&\pcatcat&&&&
\\ % row 6
&&&& \uWEmbDot>\fu &&&&
\\  % row 7
&&&&\psetcat&&&&
\end{diagram}
\]
\caption{Functoriality of update propagation policies}
\label{fig:policyfun}
\end{wrapfigure}
%\end{figure}


==> ll-figures/diags/policyfun-bigTri.tex <==

%\begin{figure}
\begin{wrapfigure}{R}{0.6\textwidth}
%\vspace{-1cm}
	\centering
\[
\begin{diagram}%[small]
% row 1----
\pgetnixcatcodi
&&&&\rDotto(8,2)^{\plusxput^0}_{\minusnixcodibra}%{[({-}\nix)^0]}
&&
&%\rEQ
& \alalenscat^0
\\ % row 2
%\dEQ 
&  
\rdDotto(4,6)<{\minusnixcodi} %{({-}\nix)^0}
\rdFEmbDot(3,2)^{\congx{\nix}}  %\rdEQ %\rdFEmbDash(2,2) 
&&&&
&&
%\ruDotto(8,1)^{\plusxput^0~[({-}\nix)^0]}
%\ruDotto(8,2)^{\plusxput^0~[({-}\nix)^0]}
%&&
\ruDashto(5,2)^{\plusxput^0}%^{\plusxput^0~[({-}\nix)^0]}  
\ldEmbed(2,2)<{\fu}
\ldTo(4,6)>{{-}\putl^0} 
&
\\ % row 3
 &&&
\pgetcat_\nix
&%&
\rTo^{~~~~\plusxput}_%
	{\begin{array}{c}
		\\ [-20pt]
	\minusnixbra
	\\ [-3.5pt]
	~~{}_{(*)}
	\end{array}}
&&
\alalenscat~~
&&
\\ % row 4
&%\rdDotto(4,4)<{({-}\nix)^0}
&&&
\rdDashto(1,4)_{\minusnixcodi}%<{({-}\nix)^0}
\rdTo(1,2)>{{-}\nix}
& 
\ldTo(2,2)<{{-}\putl}
&
\\ % row 5
&&&&\pcatcat&&&&
\\ % row 6
&&&& 
\uEmbed>\fu 
&&&&
\\  % row 7
&&&&\psetcat&&&&
\end{diagram}
\]
\caption{Functoriality of update propagation policies}
\label{fig:policyfun}
\end{wrapfigure}
%\end{figure}


==> ll-figures/diags/policyfun-ml-diamond.tex <==

\newcommand\mlpenta{\enma{
\begin{diagram}%[small]
\\ % row 1 ML
&& \psetcat && % &&
\\ % row 2 ML
&\ruEmbed(2,2)<{\minusrr}  %&\ruTo(4,2)^{L_{\eps,\err}} &
&&  \luTo^{\minusupdreq}      %\luEmbdot(2,2)>{\minusee} 
&
\\ % row 3  ML
\grt{\paracatrr}
&&\rTo^{\grt{L_{\eps,\err}} }
&&
\grt{\begin{array}{c}
	\learncat=
	\\ [-2.5pt]
	\allenscatcodi
\end{array}
}
%{\begin{array}{c}
%	\allenscat^{\codiind}_{\grdee}
%	\\ [-2.5pt]
%	=\learncat_{\grdee}
%	\end{array}
%}
\\ % row 4  ML
&\rdTo<{\grt{par}}
&%(*)
&\ldTo>{par'}
& 
\\ % row 5 ML
&&|\psetcat|^*
&&
\end{diagram}
}}

% ---> now the bx version
\newcommand\bxpenta{\enma{
		\begin{diagram}%[small]
			\\ % row 1 bx
		&&	\pcatcat &&  
			\\ % ---- > row 2 bx
			&\ruEmbed^{{-}\mtl} 
			&& \luTo^{\minusput}    %\ruTo(4,2)^{L_{\eps,\err}} 
			& % \uEmbed>{\minusnixhat} %<{[\img]} 
					\\ % row 3 bx
			\grt{\pgetcat_\mtl}
			&&\rTo^{\grt{\plusx{\mtl}\putl}} 
			&&
				\begin{array}{c}
				\allenscatwbx{}
				%				\\ [-2.5pt]
				%				=\learncat
			\end{array}
			\\ % row 4 bx
			&\rdTo<{\grt{par}}
			&%(*)
			&\ldTo>{par'}
			& 
			\\ % row 6
			&&|\pcatcat|^*
			&&
		\end{diagram}
}}
% end diag defins

\begin{figure}
%\begin{wrapfigure}{R}{0.275\textwidth}
	\renewcommand\grt[1]{#1}
%\vspace{-0.5cm}
	\centering
	\begin{tabular}{c@{\qquad\qquad}c}
%\vspace{-0.55cm}
\mlpenta & \bxpenta
\\ [8em]
\parbox{4.5 cm}{(a) {ML~setting}: asymmetric {\em discrete}  learning lenses (=learners)} 
& \parbox{6 cm}{(b) \Bx setting: asymmetric ({\em well-behaved})  learning {\em delta} lenses with {\em amendments}} % (= (wb) learning lenses)}
\end{tabular}
\caption{%\parbox{0.3\textwidth}{
	Functoriality of learning algorithms: 
}
\label{fig:policyfun-ml1}
%\end{wrapfigure}
\end{figure}
%\vspace{-0.55cm}

==> ll-figures/diags/policyfun-ml-pentagon.tex <==

\newcommand\mlpenta{\enma{
\begin{diagram}%[small]
\\ % row 1 ML
\psetcat && \lTo^{\minusput} &&
\begin{array}{c}
\allenscatcodi
\\ [-2.5pt]
=\learncat
\end{array}
\\ % row 2 ML
\uEmbed<{\minusR} &&&\ruTo(4,2)^{L_{\eps,\err}} &
\uEmbdot>{\minusee} 
&&
\\ % row 3  ML
\grt{\paracatre}
&&\rDotto^{%{\grt{L'_{\eps,\err}}
\begin{array}{cc}
	& \quad[\img]
	\\
	\qquad\grt{L'_{\eps,\err}} %
\end{array}
}
&&
\grt{
	\begin{array}{c}
	\allenscat^{\codiind}_{\grdee}
	\\ [-2.5pt]
	=\learncat_{\grdee}
	\end{array}
}
\\ % row 4  ML
&\rdTo<{\grt{par}}
&%(*)
&\ldTo>{par}
& 
\\ % row 6
&&|\psetcat|^*
&&
\end{diagram}
}}

% ---> now the bx version
\newcommand\bxpenta{\enma{
		\begin{diagram}%[small]
			\\ % row 1 bx
			\pcatcat && \lTo^{\minusput} &&
			\begin{array}{c}
				\alalenscatwbx{}
%				\\ [-2.5pt]
%				=\learncat
			\end{array}
			\\ % ---- > row 2 bx
			\uEmbed>{\minusnix} &&& %\ruTo(4,2)^{L_{\eps,\err}} 
			& \uEmbed>{\minusnixhat} %<{[\img]} 
			&&
			\\ % row 3 bx
			\grt{\pgetcat_\nix}
			&&\rTo^{\grt{\plusxput}} 
			&&
			\grt{
				\begin{array}{c}
					\alalenscatwbXhat
%					\\ [-2.5pt]
%					=\learncat_{\grdee}
				\end{array}
			}
			\\ % row 4 bx
			&\rdTo<{\grt{par}}
			&%(*)
			&\ldTo>{par}
			& 
			\\ % row 6
			&&|\pcatcat|^*
			&&
		\end{diagram}
}}
% end diag defins

\begin{figure}
%\begin{wrapfigure}{R}{0.275\textwidth}
	\renewcommand\grt[1]{#1}
%\vspace{-0.5cm}
	\centering
	\begin{tabular}{c@{\qquad\qquad}c}
%\vspace{-0.55cm}
\mlpenta & \bxpenta
\\ [8em]
\parbox{2.75cm}{(a) ML setting: {\em discrete} asymmetric lenses (=learners)} 
& \parbox{5cm}{(b) \Bx setting: asymmetric ({\em well-behaved}) {\em delta} lenses with {\em amendments}}
\end{tabular}
\caption{%\parbox{0.3\textwidth}{
	Functoriality of learning algorithms: 
}
\label{fig:policyfun-ml1}
%\end{wrapfigure}
\end{figure}
%\vspace{-0.55cm}

==> ll-figures/diags/policyfun-ml-rectangle.tex <==

\newcommand\mlrectangle{\enma{
\begin{diagram}%[small]
\\ % row 1  ML
\grt{\paracatrr}
&&\rTo^{\grt{L_{\eps,\err}}}_{\grt{( \plusx{\eps,\err}\putl^{\codiindd})  }}
&&
\grt{\begin{array}{c}
	\learncat=
	\\ [-2.5pt]
	~~\allenscatcodicodi
\end{array}
}
%{\begin{array}{c}
%	\allenscat^{\codiind}_{\grdee}
%	\\ [-2.5pt]
%	=\learncat_{\grdee}
%	\end{array}
%}
\\ % row 2  ML
\dEmbed<{\minusrr}  %\rdTo<{\grt{par}}
&&&
\ldTo(4,2)_{\minusput^\codiindd}%{\minusupdreq} 
&\dDashto>{par'}
\\ % row 3 ML
\psetcat&&\rTo_{\parname^\codiind}&&\iaset
\end{diagram}
}}
%--> the bx rectangle
\newcommand\bxrectangle{\enma{
		\begin{diagram}%[small]
			\\ % row 1  Bx
			\grt{\pgetcat_\mtl}
			&&\rTo^{L_\mtl}
			_{(\plusx{\mtl}\putl)}
			&&\alalenscatwbind
			\\ % row 2  ML
			\dEmbed<{{-}\mtl}  %\rdTo<{\grt{par}}
			&&&
			\ldTo(4,2)_{\minusput} 
			&\dDashto>{par'}
			\\ % row 3 ML
			\pcatcat&&\rTo_{\parname}&&\iacat
		\end{diagram}
}}



% end diag defins

\begin{figure}
%\begin{wrapfigure}{R}{0.275\textwidth}
	\renewcommand\grt[1]{#1}
%\vspace{-0.5cm}
	\centering
	\begin{tabular}{c@{\qquad\qquad}c}
%\vspace{-0.55cm}
\mlrectangle & \bxrectangle
\\ [8em]
\parbox{4.5 cm}{(a) {ML~setting}: asymmetric {\em codiscrete}  learning lenses (=learners)} 
& \parbox{6 cm}{(b) \Bx setting: asymmetric ({\em well-behaved})  learning {\em delta} lenses with {\em amendments}} % (= (wb) learning lenses)}
\end{tabular}
\caption{%\parbox{0.3\textwidth}{
	Functoriality of learning algorithms and policies
}
\label{fig:policyfun}
%\end{wrapfigure}
\end{figure}
%\vspace{-0.55cm}

==> ll-figures/diags/policyfun-ml-small.tex <==
\begin{figure}
%\begin{wrapfigure}{R}{0.5\textwidth}
\vspace{-1cm}
	\centering
\[
\begin{diagram}%[small]
%\\ % row -2   
%\grt{\paracat_\reals}&\rFEmb_\cong^{\grt{\plusdelx{\diff}}}
%&\grt{\paracatrcat}
%%&\rTo^{[\plusx{Gd(\eps,\err)}\putl, \plusx{\nix}\dif]}
%&\rTo^{\grt{\plusx{Gd(\eps,\err)}\putl}} %, \plusx{\nix}\dif]}
%&\alalensdifcat&\rTo^{\codiscr}&\learncat%=\alenscatcodi
%\\ % row -1   
%\grt{\paracat_\reals}&\rFEmb_\cong^{\grt{\plusdelx{\diff}}}
%&\grt{\paracatrcat}
%%&\rTo^{[\plusx{Gd(\eps,\err)}\putl, \plusx{\nix}\dif]}
%&\rTo^{\grt{\plusx{Gd(\eps,\err)}\putl}} %, \plusx{\nix}\dif]}
%&\alalensdifcat&\rTo^{\codiscr}&\learncat%=\alenscatcodi
\\ %========  row 1   =========
\grt{\paracat_\reals}&\rFEmb_\cong^{\grt{\plusdelx{\diff}}}
&\grt{\paracatrcat}
%&\rTo^{[\plusx{Gd(\eps,\err)}\putl, \plusx{\nix}\dif]}
 &\rTo^{\grt{\plusx{Gd(\eps,\err)}\putl}} %, \plusx{\nix}\dif]}
&\alalensdifcat&\rTo^{\codiscr}&\learncat%=\alenscatcodi
\\ % row 2
&%(1)
&\dTo>{\grt{{-}\rcat}}
&{}_{(2)} 
&\dTo<{{-}\dif}
&\luFEmb(2,4)^{\plusx{\pairing}(\deltas,\dif)} %(3)
&\dEQ<{{}^{(3)}\quad} 
\\ % row 3
\dTo<{\grt{{-}\reals}}&{}^{(1)}&\pcatcat&\lTo_{{-}\putl}
&\alalenscat^{\quad(4)}
&%\textcolor{red}{{}^{(3)}}
&
\\ % row 4
&\ruFEmb_{\plusarrx{\pairing}}&&
{}_{(5)}
&&
\luFEmbDash_{\plusdelx{\pairing}}
&
\\ % row 5
\psetcat&&&\lTo_{{-}\putl^0}
&&&\alalenscatcodi
\end{diagram}
\]
%\vspace{-0.5cm}
\caption{Functoriality of learning algorithms}
\label{fig:policyfun-ml}
%\end{wrapfigure}
\end{figure}

==> ll-figures/diags/policyfun-ml.tex <==
\begin{figure}[h]
%\begin{wrapfigure}{R}{0.5\textwidth}
\vspace{-1cm}
	\centering
\[
\begin{diagram}%[small]
\\ % row -2   
\grt{\paracat_\reals}
& %\rFEmb_\cong^{\grt{\plusdelx{\diff}}}
& %\grt{\paracatrcat}
&  \rDashto^{\grt{L_{\eps,\err}}} %\rTo^{\grt{\plusx{Gd(\eps,\err)}\putl}} 
&  %\alalensdifcat 
&  %\rTo^{\codiscr}
&  \learncat%=\alenscatcodi
\\ % row -1   
&\rdFEmb_\cong^{\grt{\plusdelx{\dif}}}   
    %\rdTo(4,2)^{\grt{\ovr{\leefun}}}  
&    %\grt{\paracatrcat}
&   {}^{(*)}   %\rTo^{\grt{\plusx{Gd(\eps,\err)}\putl}} %, \plusx{\nix}\dif]}
&     %\alalensdifcat
&  \ruTo^{\codiscr}
&      %\learncat%=\alenscatcodi
\\ %========  row 1   =========
&   %\rFEmb_\cong^{\grt{\plusdelx{\diff}}}
&\grt{\paracatrcat}
%&\rTo^{[\plusx{Gd(\eps,\err)}\putl, \plusx{\nix}\dif]}
&\rTo^{\grt{\plusx{Gd(\eps,\err)}\putl}} %, \plusx{\nix}\dif]}
&\alalensdifcat
&  %\rTo^{\codiscr}
&   %\learncat%=\alenscatcodi
\\ % row 2
&%(1)
&\dTo>{\grt{{-}\rcat}}
&{}_{(2)} 
&\dTo<{{-}\dif}
&\luFEmb(2,4)^{\plusx{\pairing}(\deltas,\dif)} %(3)
&\dEQ<{{}^{(3)}\quad} 
\\ % row 3
\dTo<{\grt{{-}\reals}}&{}^{(1)}&\pcatcat&\lTo_{{-}\putl}
&\alalenscat^{~(4)}
&%\textcolor{red}{{}^{(3)}}
&
\\ % row 4
&\ruFEmb_{\plusarrx{\pairing}}&&
{}_{(5)}
&&
\luFEmbDash_{\plusdelx{\pairing}}
&
\\ % row 5
\psetcat&&&\lTo_{{-}\putl^0}
&&&\alalenscatcodi
\end{diagram}
\]
\vspace{-0.5cm}
\caption{Functoriality of learning algorithms, 3}
\label{fig:policyfun-ml3}
%\end{wrapfigure}
\end{figure}

==> ll-figures/diags/policyfun-new.tex <==
%\begin{figure}
\begin{wrapfigure}{R}{0.5\textwidth}
%\vspace{-1cm}
	\centering
\[
\begin{diagram}[small]
\pgetcat_\nix &&&\rDashto^{\plusxput_0} &&& \alalenscat_0
\\ % row 2
&\rdEQ %\rdFEmbDash(2,2) 
&&&& \ldWEmbDash(2,2)^{\fu} &
\\ % row 3
&&\pgetcat_\nix&\rTo^{\plusx{\nix}\putl} &\alalenscat&&
\\ % row 4
\dDashto>{{-}_0\nix}&& \dTo>{{-}\nix}&(*)&\dTo<{{-}\putl}
&&\dDashto<{{-}\putl_0}
\\ % row 5
&& \pcatcat&\rEQ&\pcatcat&&
\\ % row 6
&\ruFEmbDash(2,2)<\fu &&&&\luFEmbDash(2,2)>\fu &
\\  % row 7
\psetcat&&&\rEQ&&&\psetcat
\end{diagram}
\]
\caption{Functoriality of update propagation policies}
\label{fig:policyfun}
\end{wrapfigure}
%\end{figure}

==> ll-figures/diags/policyfun-smallTri.tex <==
%\begin{figure}
\begin{wrapfigure}{R}{0.5\textwidth}
%\vspace{-1cm}
	\centering
\[
\begin{diagram}%[small]
%\pgetcat^0_\nix &&&&&\rDashto^{\plusxput^0} &&&&& \alalenscat^0
%\\ % row 2
%&\rdTo(5,4)<{{-}\nix}\rdWEmbed(3,2) && &&&&
\\ % row 3
\pgetcat_\nix&\rTo^{\plusx{\nix}\putl} &\alalenscat
\\ % row 4
&\rdTo(1,2)>{{-}\nix}\ldTo(1,2)>{{-}\putl}& 
\\ % row 5
&\pcatcat&
\end{diagram}
\]
\caption{Functoriality of update propagation policies}
\label{fig:policyfun}
\end{wrapfigure}
%\end{figure}

==> ll-figures/diags/policyfun-tripleLane.tex <==

%\begin{figure}
\begin{wrapfigure}{R}{0.5\textwidth}
\vspace{-1cm}
	\centering
\[
\begin{diagram}[h=2.5em]%[small]
% row 00
%&\spP_1&&\spP_2&&\spP_3&
\\  % row 00
\nia_1&\rTo_{\nivv^1_{p_1}}^{{p_1\in\spP_1}}
&\nia_2&\rTo_{\nivv^2_{p_2}}^{{p_2\in\spP_2}} 
&\nia_3&\rTo_{\nivv^3_{p_3}}^{{p_3\in\spP_3}} 
& \nia_4
\\ &&& &&&
\\  % row 01
  \spA_1&\rTo_{\get^1_{p_1}}^{{p_1\in\spP_1}}
&\spA_2&\rTo_{\get^2_{p_2}}^{{p_2\in\spP_2}} 
&\spA_3&\rTo_{\get^3_{p_3}}^{{p_3\in\spP_3}} 
& \spA_4
\\ % row 02
&&& &&&
\\ %row 1
   \dbox{A_1}&\rDermapsto^{{:}\get^1_{p_1}}
&A_2&\rDermapsto^{{:}\get^2_{p_2}}
&A_3&\rDermapsto^{{:}\get^3_{p_3}}
&A_4
\\ % row 2
&&&&&
%--begin triple arrow label
&\dTo>{u_4}
\\ % row 3
&&&&\dDotto<{u_3}&
%--begin triple arrow label
\swssseTilearrowABx{1{:}\putl^3_{A_3,p_3}}{e_3}
&\dbox{A'_4}
\\ % row 4
&&\dDotto<{u_2}&
&&&\dDotto<{u_4^@}
\\ % row 5
&&&
% begin triple arrow label
\swssseTilearrowABx{2{:}\putl^2_{A2, p_2} }{e_2}
&A'_3
&\rDashmapsto^{{:}\get^3_{p'_3}}&{A'}_4^@
\\ %row 6
\dDotto<{u_1}&&&&\dDotto<{u_3^@}&\stackrel{4{:}\get^3_{e_3}}{\Rightarrow}&\dDashto
\\ % row 7
&\swssseTilearrowABx{3{:}\putl^1_{A_1,p_1}}{e_1}&A'_2&\rDashmapsto^{{:}\get^2_{p'_2}}&{A'}_3^@&\rDashmapsto^{{:}\get^3_{p'_3}}&\circ
\\ % row 8
&&\dDotto<{u_2^@}&\stackrel{5_1{:}\get^2_{e_2}}{\Rightarrow}
&\dDashto&\stackrel{5_2{:}\get^3_{e_3}}{\Rightarrow}&\dDashto
\\ % row 9
A'_1&\rDermapsto^{{:}\get^1_{p'_1}}&{A'}_2^@&\rDashmapsto^{{:}\get^2_{p'_2}}
&\circ
	&\rDashmapsto^{{:}\get^3_{p'_3}}&\circ
\end{diagram}
\]
%\end{document}
\caption{Functoriality of update propagation policies: tripleLane}
\label{fig:policyfun-tripleLane}
\end{wrapfigure}
%\end{figure}

==> ll-figures/diags/policyfun-twoRectangles.tex <==

\newcommand\mlrectangle{\enma{
\begin{diagram}%[small]
\\ % row 1  ML
\grt{\paracatrr}
&&\rTo^{\grt{L_{\eps,\err}}}_{\grt{( \plusx{\eps,\err}\putl^{\codiindd})  }}
&&
\grt{\begin{array}{c}
	\learncat=
	\\ [-2.5pt]
	~~\allenscatcodicodi
\end{array}
}
%{\begin{array}{c}
%	\allenscat^{\codiind}_{\grdee}
%	\\ [-2.5pt]
%	=\learncat_{\grdee}
%	\end{array}
%}
\\ % row 2  ML
\dEmbed<{\minusrr}  %\rdTo<{\grt{par}}
&&&
\ldTo(4,2)_{\minusput^\codiindd}%{\minusupdreq} 
&\dDashto>{par'}
\\ % row 3 ML
\psetcat&&\rTo_{\parname^\codiind}&&\iaset
\end{diagram}
}}
%--> the bx rectangle
\newcommand\bxrectangle{\enma{
		\begin{diagram}%[small]
			\\ % row 1  Bx
			\grt{\pgetcat_\mtl}
			&&\rTo^{L_\mtl}
			_{(\plusx{\mtl}\putl)}
			&&\alalenscatwbind
			\\ % row 2  ML
			\dEmbed<{{-}\mtl}  %\rdTo<{\grt{par}}
			&&&
			\ldTo(4,2)_{\minusput} 
			&\dDashto>{par'}
			\\ % row 3 ML
			\pcatcat&&\rTo_{\parname}&&\iacat
		\end{diagram}
}}



% end diag defins

\begin{figure}
%\begin{wrapfigure}{R}{0.275\textwidth}
	\renewcommand\grt[1]{#1}
%\vspace{-0.5cm}
	\centering
	\begin{tabular}{c@{\qquad\qquad}c}
%\vspace{-0.55cm}
\mlrectangle & \bxrectangle
\\ [8em]
\parbox{4.5 cm}{(a) {ML~setting}: asymmetric {\em codiscrete}  learning lenses (=learners)} 
& \parbox{6 cm}{(b) \Bx setting: asymmetric ({\em well-behaved})  learning {\em delta} lenses with {\em amendments}} % (= (wb) learning lenses)}
\end{tabular}
\caption{%\parbox{0.3\textwidth}{
	Functoriality of learning algorithms and policies
}
\label{fig:policyfun}
%\end{wrapfigure}
\end{figure}
%\vspace{-0.55cm}

==> ll-figures/diags/policyfun-twoTriangles.tex <==


\begin{figure}
%\begin{wrapfigure}{R}{0.275\textwidth}
	\renewcommand\grt[1]{#1}
%\vspace{-0.5cm}
	\centering
	\begin{tabular}{c@{\qquad}c}
%\vspace{-0.55cm}
%\ml triangle goes
\begin{diagram}%[small]
	\\ % row 1  ML
	\grt{\paracatrr}
	&&\rTo^{\grt{L_{\eps,\err}}}_{\grt{( \plusx{\eps,\err}\putl^{\codiindd})  }}
	&&
	\grt{\begin{array}{c}
			\learncat=
			\\ [-2.5pt]
			~~\allenscatcodicodi
		\end{array}
	}
	%{\begin{array}{c}
	%	\allenscat^{\codiind}_{\grdee}
	%	\\ [-2.5pt]
	%	=\learncat_{\grdee}
	%	\end{array}
	%}
	\\ % -------------->       row 2  ML
	%\dEmbed<{\minusrr}  %\rdTo<{\grt{par}}
	&\rdEmbed(2,2)<{\minusrr} 
	&
	&
	\ldTo(2,2)_{\minusput^\codiindd}%{\minusupdreq} 
	&%\dDashto>{par'}
	\\ % ------------------>        row 3 ML
	&&\psetcat&&%\rTo_{\parname^\codiind}&&\iaset
\end{diagram}
& 
%\bx triangle goes
\begin{diagram}%[small]
	% row -2
	&&&& &&\alalenscatwbind
	\\ % row -1
	&&&& &
	\ruTo(6,2)^{L_{\mtlwb}}%_{(\plusx{\mtlwb}\putl)}
	\ldEmbed(2,2)>{{-}\wbind}&
	\\ % row 1  Bx
	\grt{\pgetcat_\mtl}
	&&\rTo^{L_\mtl}
	_{(\plusx{\mtlwb}\putl)}
	&&\alalenscat
	\\ % -------------------->        row 2  ML
	%\dEmbed<{{-}\mtl}  %\rdTo<{\grt{par}}
	&
	\rdEmbed(2,2)<{{-}\mtl}
	&&
	\ldTo(2,2)_{\minusput} 
	& %\dDashto>{par'}
	\\ % ---------------------->         row 3 ML
	&&\pcatcat&& %\rTo_{\parname}&&\iacat
\end{diagram}
\\ [5em]
\parbox{4.5 cm}{(a) {ML~setting}: asymmetric {codiscretely}  learning codiscrete lenses (=learners)} 
& \parbox{6 cm}{(b) \Bx\ setting: asymmetric ({\em well-behaved})  categorically learning {\em delta} lenses with {\em amendments}} % (= (wb) learning lenses)}
\end{tabular}
\caption{%\parbox{0.3\textwidth}{NEW
 Functoriality of learning algorithms and policies
}
\label{fig:policyfun}
%\end{wrapfigure}
\end{figure}
%\vspace{-0.55cm}

==> ll-figures/diags/policyfun.tex <==
%\begin{figure}
\begin{wrapfigure}{R}{0.35\textwidth}
\vspace{-1cm}
	\centering
\[
\begin{diagram}[small]
%\pgetcat^0_\nix &&&&&\rDashto^{\plusxput^0} &&&&& \alalenscat^0
%\\ % row 2
%&\rdTo(5,4)<{{-}\nix}\rdWEmbed(3,2) && &&&&
\\ % row 3
\pgetcat_\nix&&\rTo^{\plusx{\nix}\putl} &&\alalenscat
\\ % row 4
&\rdTo>{{-}\nix}&(*)&\ldTo>{{-}\putl}& 
\\ % row 5
&&\pcatcat&&
\end{diagram}
\]
%\caption{Functoriality of update propagation policies}
\label{fig:policyfun}
\end{wrapfigure}
%\end{figure}

==> ll-figures/pdfs/classPlane.tex <==
\begin{figure}
%	\begin{wrapfigure}{R}{0.5\columnwidth}	
\vspace{-0.25cm}
	\centering
	   \includegraphics[width=0.7\textwidth]%
	{ll-figures/pdfs/classPlane-pic}
	\caption{The universe of categories of learning delta lenses
		}
	\label{fig:classPlane}
	\vspace{-0.25cm}
%\end{wrapfigure}
\end{figure}

==> ll-figures/pdfs/ex-whyDL-bigbig.tex <==
%\newlength{\twomodwid}
\setlength{\twomodwid}{\textwidth}

\begin{figure}
%\agmargin{[w=2.5] in Fig. 2? Should that be removed?\\Additionally, I changed the \textbackslash{}twomodwid width from 0.32\textbackslash{}textwidth to 0.3\textbackslash{}textwidth. That makes the figures only few milimetres narrower (3--4mm) and saves a lot of space and fixes lots of ``overfull'' errors.}
%\begin{wrapfigure}{r}{2.1\twomodwid}
    \vspace{-0.25cm}
       \centering
    %\begin{tabular}{|@\quad c@\quad|@\quad c@\quad|}
   %\hline\\[5pt]
    \includegraphics[width=\twomodwid]% try 1.75 for wrap
    {ll-figures/pdfs/ex-whyDLbigbig-pic.pdf}
       %    \\[5pt] \hline
   %\end{tabular}
%   \vspace{-0.65cm}
    \caption{Example of update propagation}
    \label{fig:ex-whyDLbigbig}
   \vspace{-0.5cm}
%\end{wrapfigure}
\end{figure}


==> ll-figures/pdfs/getAmend-inR.tex <==
%\begin{figure}
	\begin{wrapfigure}{R}{0.5\columnwidth}
		\vspace{-0.5cm}
		\centering
	\centering
	   \includegraphics[width=0.5\textwidth]%
	{ll-figures/pdfs/getAmend-inR-pic}
	\caption{Differentiation of a parameterized function}
	\label{fig:getamend-inR}
\end{wrapfigure}
%\end{figure}

==> ll-sections/ML-with-deltas.tex <==
\section{%Future work: 
	Enriching ML with deltas: A sketch for future work}\label{sec:deltas4ml}

\renewcommand\xxx{\enma{\mathsf{xxx}}}
\newcommand\paracatx[1]{\enma{\paracat_{#1}}}


%We discuss (somewhat speculatively) three unconventional options for compositional ML suggested by the delta-based \bx. The discussion is purely theoretical as no attempt to evaluate %The present author does not have any knowledge of the ML literature and is not aware whether these possibilities are already realized, or how difficult an algorithmic realization of these options could be (or whether they are reasonable indeed). 
%

Learners defined in \citefst\ are codiscrete learning lenses, and in this section we will  semi-formally discuss enriching them with deltas. Subsection~\ref{sec:codi} is a general lens theory piece: we show that codiscrete lenses actually hide delta lenses inside them and describe a general schema of building a codiscrete lens from a delta lens with an additional differencing operation. The other three subsections are specifically for ML. In  \sectref{difasfun}, we present learners as an instance of the general schema built in \sectref{codi}. Sect.~\ref{sec:del4ml-nonmetr} discusses non-metrical deltas that lead to adaptive learning algorithms, in which learning can include restructuring the neural network . In short \sectref{del4ml-amend}, we discuss amendments in the context of ML. 


%\input{ll-sections/ml-metric}
\input{ll-sections/ml-delta}
\input{ll-sections/ml-amend}

\endinput

What could be deltas for pairs of values?

1)  Metrics like in Lawvere's metric spaces

2) Labels (men/women, students, professors, mathematician and poets)

3) Restruct the architecture!! Look at the discussion at \citefst


\endinput


==> ll-sections/aLens-indexed.tex <==
\section{Lenses for learners}\label{sec:lego-spans2lens}

\input{ll-sections/modSpaces-short}
%\input{ll-sections/aa-lensDef-semiDiscrete}

\begin{defin}[Indexed Asymmetric Lenses, cf. \cite{me-fase18}]
	Let \spaA\ and \spB\ be model spaces, \ie, categories with compatibility relation \Kupd. 
	An {\em indexed asymmetric lens  with amendment (indexed aa-lens)} from \spA\ to \spB\ is given by the following data. 
	
	a) A category \spP\ of {\em parameters} (think about function/view definitions). We will denote objects of \spP\ by small letters $p,p',..$ rather than capital ones to avoid confusion with paper \cite{ll-bx19}. 

	b) A functor \frar{\get}{\spP}{[\spA,\spB]}. We will write $\get_p$ or even shorter $p^*$ for $\get(p)$. For any $A\in\xob{\spA}$, the pair $(A,p^*(A))$ will be shown in diagrams as an arrow $A\rMapsto^{\#p}p^*(A)$ with a bulleted tail by the technical reason of pptx.%
	\footnote{In the fibered version, $\#p$ will be a chosen opcartesian lifting of arrow $p$ at object $A$.} 
	
	c) A family of operations $\putpa$ indexed by pairs $(p\in P, A\in\xob{\spA})$ %(read ``put the view update back'') 
	of the following arity. 
	
	Provided with a target update \frar{v}{p^*(A)}{B'} at the input, operation $\putpa$ outputs three elements as illustrated by diagram in \figref{fig:ppg-schema}(a)
	
	b1) a source update \frar{u=\putpa_\indb(v)}{A}{A'} 
	
	b2) a parameter update  $p'=\putpa_\upd(v)$
	
	b3) an amendment to the target update, %$\putpa_{\self}(v)$ or 
	\frar{\amex{v}=\putpa_{\self}(v)}{A'}{A''}. 
	%such that $v;\amex{v}=\get(u')$. 
	
	\begin{figure}
%	\begin{equation}
\begin{tabular}{c@\qquad c}
	% column 1
	\begin{diagram}[w=5em,h=2em]
		% row 11
		 \dbox{A} & \rMapsto^{{:}\get_p} & \dbox{B}
		\\  % row 12
		&&\dTo>v
		\\ % row 13
	\dDashto>u&
		\swseTilearrowAB{{:}\putpa}{}
		%\seTilearrowAB{}{}
	%	\Downarrow %{:}\putpa
		&B'
			\\ % 14
		&&\dDashto>{\amex{v}}
		\\ % 15
A' &\rDermapsto^{{:}\get_{p'}} & B''
	\end{diagram}
%------------
& % column 2	
%--------------
	\begin{diagram}[w=5em,h=5ex]
		% row 21
	\dbox{A} &\rMapsto^{{:}\get_p} & \dbox{B} & \rMapsto^{{:}\get_q} & \dbox{C}
	\\  % row 22
	&&&&\dTo>w
	\\ % row 23
	&	\swseTilearrowAB{~~2{:}\putpa}{}&\dDashto>v&
	     \swseTilearrowAB{~~1{:}\putqb}{}&C'
	\\ % 24
	&&&&\dDashto>{\amex{w}}
	\\ % 25
	\dDashto<u &
%	\swTilearrowAB{}{~~~{:}\putpa}{}
		& B' &\rDermapsto^{{:}\get^{(1)}_{q'}} & C''
	\\  % row 26
	&&\dDashto>{\amex{v}}& \stackrel{3{:}\get_{q'}}{\Longrightarrow}&\dDashto>{\get^{}_{q'}(\amex{v})}
	\\  % row 27
	A' &\rDermapsto^{\get^{(2)}_{p'}} & B''&\rDermapsto^{{:}\get^{(3)}_{q'}}& C''''
	\end{diagram}
\\  [10pt] % End OF TABULAR ROW 1
(a)  & (b)
\end{tabular}
	%	\end{equation}
	\caption{Schemas of update propagation: (a) the arity of \putl, and (b) composition. Input elements are boxed (nodes) and solid (arrows), output elements are not boxed and dashed.
	\label{fig:ppg-schema}}
\end{figure}
A target update \frar{v}{\get(B)}{A'} is called {\em closed} if %$\putl^B_\inda(v)=\id_{A'}$. 
$\amex{v}=\id_{A'}$, and an aa-lens is {\em closed} if all its target updates are closed.  \qed
\end{defin}
%The following is a specialization of Def.~\ref{def:wblens}, in which consistency between a base $B$ and a view $A$ is understood as equality $\get(B)=A$.

%{ %---> version with put^B_indv(v) rather than v^@
%\renewcommand\ppgB{\ensuremath{\putl^B}}
%\begin{defin}[Well-behavedness]\label{def:wbalens}
%An a-lens is {\em well-behaved (wb)} if it satisfies the following laws for all $B\in\xob{\spaB}$, \frar{v}{\get(B)}{A'}, and \frar{u}{B}{B'}:
%%
%\\[1ex]
%\lawgap=1ex
%\noindent \begin{tabular}{l@{\quad}l}
%%		\lawnamebr{Hippocr1}{
%%        \frar{u}{B}{B'}
%%		} & 
%%		if $\get(B) = \get(B')$, then $\get(u) = \id_{\get(B)}$
%%		\\ [\lawgap]\lawnamebr{Hippocr2}{
%%		\frar{v}{\get(B)}{A'}
%%		}	& 
%%			if $A'=\get{B}$, then $\ppgB_\indb(v) = \id_B$,   $\ppgB_\inda(v)=\id_{\get(B)}$
%%		%$\ppgB_{\indb}(\id_{\get(B)})=\id_{B}$
%%		\\
%%		& \parbox{15em}{\textcolor{red}{the two laws above are just a reminder of a path that was rejected} }
%%		\\
%\lawnamebr{Stability}{
%	%\frar{v}{\get(B)}{A'}
%}	& 
%if %\frar{v}{\get(B)}{A'} is identity, 
%   $v=\id_{\get(B)}$, then $\ppgB_\indb(v) = \id_B$ and  $\ppgB_\inda(v)=\id_{\get(B)}$
%%$\ppgB_{\indb}(\id_{\get(B)})=\id_{B}$
%		\\  [\lawgap] \lawnamebr{\reflectzero}{
%		    % \frar{v}{\get(B)}{A'}
%		} &	
%		%$\ppgB_{\inda}(v)\noteq \id_{A'}$ implies 
%		%$A'\noteq \get(X)$ for all $X\in\xob{\spaB}$
%		if $A'=\get(X)$ for some $X\inn\xob{\spB}$, then $\ppgB_{\inda}(v)=\id_{A'}$
%		\\  [\lawgap] \lawnamebr{Reflect1}{
%		%\frar{v}{\get(B)}{A'}
%		} &	
%		$(v, \ppgB_{\inda}(v))\in \Kupd_{A'}$ %for all $u_i$ 
%		\\  [\lawgap] \lawnamebr{Reflect2}{
%		%\frar{v}{\get(B)}{A'}
%		} &
%		$\ppgB_{\indb}(v;\ppgB_{\inda}(v)) = \ppgB_{\indb}(v)$
%		\\ [\lawgap] \lawnamebr{PutGet}{
%		%\frar{v}{\get(B)}{A'}
%		} & %$_{~~~~~~}$
%			%$v;v'=\get(v.\putl_\indb^B) $	% dot version
%		$v;\putl^B_\inda(v)=\get(\putl_\indb^B(v)) $   % bracket version 
%\end{tabular} \\
%\rule{0mm}{0mm}\qed
%\end{defin}
%}

{ % --> version with v^@ rather than put^B_indv(v) @
	\renewcommand\ppgB{\ensuremath{\putl^B}}
	\renewcommand\ppgB{\ensuremath{\putpa}}
	\begin{defin}[Well-behavedness]\label{def:wbalens}
		An aa-lens is {\em well-behaved for learning (wbl)} if it satisfies the following laws for all $p\in P$, $A\in\xob{\spaB}$ and \frar{v}{B}{B'} where $B$ denotes $\get_p(A)$:
		%, and \frar{u}{B}{B'}:
			\\[1ex]
		\lawgap=1ex
		\noindent \begin{tabular}{l@{\quad}l}
			%		\lawnamebr{Hippocr1}{
			%        \frar{u}{B}{B'}
			%		} & 
			%		if $\get(B) = \get(B')$, then $\get(u) = \id_{\get(B)}$
			%		\\ [\lawgap]\lawnamebr{Hippocr2}{
			%		\frar{v}{\get(B)}{A'}
			%		}	& 
			%			if $A'=\get{B}$, then $\ppgB_\indb(v) = \id_B$,   $\ppgB_\inda(v)=\id_{\get(B)}$
			%		%$\ppgB_{\indb}(\id_{\get(B)})=\id_{B}$
			%		\\
			%		& \parbox{15em}{\textcolor{red}{the two laws above are just a reminder of a path that was rejected} }
			%		\\
			\lawnamebr{Stability}{
			}	& 
			if $v=\id_B$, then $p'=p$, $\putpa_\req(v) = \id_A$ and  
			$\amex{v}=\id_B$ %{\get_p(A)}$
%							\\  [\lawgap] \lawnamebr{\reflectzero}{
%			} &	
%			if $v=\get(u)$ for some \frar{u}{A}{A'}, then $\amex{v}=\id_{B'}$
			\\  [\lawgap] \lawnamebr{Reflect1}{
			} &	
			$(v, \amex{v})\in \Kupd_{B'}$ %for all $u_i$ 
%			\\  [\lawgap] \lawnamebr{Reflect2}{
%			} &
%			$\ppgB_{\indb}(v;\amex{v}) = \ppgB_{\indb}(v)$
			\\ [\lawgap] \lawnamebr{PutGet}{
				} & %$_{~~~~~~}$
			$\get_p(\putpa_\req(v)) =v;\amex{v} $ \qed
			\end{tabular} \\
		%\rule{0mm}{0mm}\qed
	\end{defin}
}


In contrast to the general lens case, a wb a-lens features \lawname{\reflectzero} --- a sort of a self-Hippocratic law regulating the necessity of amendments: the latter is not allowed as soon as consistency can be restored without amendment. Another distinction is inclusion of an invertibility law \lawname{PutGet} into the definition of well-behavedness: 
 %due to historical traditions. %Subsequent results will also provide some justification for this. 
\lawname{PutGet}{} together with \lawname{Reflect2} provide (weak) invertibility: $\putl^B_\indb(\get(\putl^B_\indb(v)))=\putl^B_\indb(v)$.   
\lawname{Reflect3} is omitted as it is implied by \lawname{Reflect0} and \lawname{PutGet}.  

Any a-lens $\ebb^{\preccurlyeq} =(\spaA,\spaB,\get, \putl)$ gives rise to a binary symmetric lens $\ebb$. Its carrier consists of model spaces $\spaA$ and $\spB$, for which we assume $\Kupd$ and $\Kdisj{}$ to be defined such that the spaces are well-behaved, cf.\ Def.~\ref{def:wbspace}. The set of corrs of a pair $(A,B)\in \xob{\spA}\times \xob{\spB}$ is the singleton $\{\etosing{(A,B)}\}$ with $\prt_\spA\etosing{(A,B)}=A$ and $\prt_\spB\etosing{(A,B)}=B$, 
%the boundary mappings are the projections, 
\zdmodtok{realignment is thus trivial,}{}{ALIGH} and consistent corrs are exactly those \etosing{(A,B)}, for which $A = \get(B)$.

For a consistent corr $\etosing{B}={(\get(B), B)}$, we need to define six operations $\ebb.\ppghB_{\_\_}$. Below we will write the upper index as $B$ rather than $\hat B$ to ease the notation. For a  view update \frar{v}{A}{A'} and the corr \etosing{B}, we define 
 $$
\ppgB_{\spA\spB}(v)=\putl^B_\indb(v){:}\, B\to B'', \;
%
\ppgB_{\spA\spA}(v)=\putl^B_\inda(v){:}\, A'\to A'', \;
% \mbox{ and }
\ppgB_{\spA\star}(v)=\etosing{B''}
$$
 The condition $A''=\get(B'')$ for $\ebb^\preccurlyeq$ means that \etosing{B''} is again a consistent corr with the desired boundaries. For a base update \frar{u}{B}{B'} and the corr \etosing{B}, we define
$$\ppgB_{\spB\spA}(u)=\get(u),\;
\ppgB_{\spB\spB}(u)=\id_{B'},\; %and
\ppgB_{\spB\star}(u)=\etosing{B'}
$$ Functoriality of $\get$ yields consistency of $\widehat{B'}$.

\begin{defin}[Very well-behaved a-lenses] \label{def:putput_a}
		A wb a-lens is called {\em very well behaved (very wb)}, if the \corring\ binary symmetric lens is such.  %additionally fulfills \lawnamebr{PutPut}, 
		cf.  Def.~\ref{def:putput}.
Of course, this definition restricts the behaviour only for the $\putl$-part of the a-lens (hence the name of the law), since functor $\get$ is compositional anyway. \qed
\end{defin}

\begin{lemma}\label{lemma:asymm_symm} Let $\ebb^\preccurlyeq$ be a (very) wb a-lens and $\ebb$ the corresponding symmetric lens. Then all base updates of $\ebb$ are closed, and $\ebb$ is (very) wb and invertible. 
 \end{lemma}
 \begin{proof}
 Base updates are closed by the definition of $\ppg_{\spB\spB}$. Well-behavedness follows from wb-ness of $\ebb^\preccurlyeq$. Invertibility has to be proved in two directions: $\ppg_{\spaB\spaA};\ppg_{\spaA\spaB};\ppg_{\spaB\spaA} = \ppg_{\spaB\spaA}$ follows from \lawnamebr{PutGet}{} and \lawnamebr{Reflect0}, the other direction follows from \lawnamebr{PutGet}{} and \lawnamebr{Reflect2}, see the remark after Def.\ref{def:wbalens}. The ''vwb''-implication follows directly from Def.\ref{def:putput_a}. 
 \qed
 \end{proof}
\begin{remark}[A-lenses as view transformation engines]\newpii{
	In terms of Varr\'o et al \cite{dvarro-models18}, a wb a-lens can be seen as an abstract algebraic model of a bidirectional view transformation engine. This engine is assumed to be a) consistent: it is a basic lens law that propagation must always produce a consistent corr, b) incremental, as lenses propagate changes rather than create the target models from scratch, c) validating, as the result of propagation is always assumed to satisfy the target metamodel constraints (either by considering the entire model space to be only populated by valid models, or by introducing a subclass of valid models and require the result of the propagation to get into that subclass). Reactiveness, \ie, whether the engine executes on-demand or in response to changes, is beyond the lens \fwk. To address this and similar concerns, we need a richer \fwk\ of lenses augmented with organizational structure introduced in \cite{me-jss15,me-grand17}. }{1}{-15em}
\end{remark}

  \begin{theorem}[Lenses from Spans]\label{thm:LensesFromSpans} An $n$-ary span of (very) wb asymmetric lenses $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$, $i=1..n$ with a common base \spaB\ of all $\ebb_i^{\preccurlyeq}$ gives rise to a (very) wb symmetric lens denoted by $\Sigma_{i=1.. n}^\spB\ebb_i^{\preccurlyeq}$. 
\end{theorem}
\begin{proof}
An $n$-ary span of a-lenses $\ebb_i^{\preccurlyeq}$ (all of them interpreted as symmetric lenses $\ebb_i$ as explained above) is a construct equivalent to the star-composition of Def.~\ref{def:star-comp}.3, in which lens $\ekk=\idlensnb$ (cf. Ex.~\ref{ex:idLens}) and peripheral lenses are lenses $\ebb_i$. The junction condition is satisfied as all base updates are $\ebb_i$-closed for all $i$ by Lemma \ref{lemma:asymm_symm}, and also trivially closed for any identity lens. The theorem thus follows from Theorem~\ref{th:star-comp}. The ``very wb''-part follows directly from Def.~\ref{def:putput_a}. Note that a corr in $\Corrx{\Sigma_{i=1.. n}^\spB\ebb_i^{\preccurlyeq}}$ 
 is nothing but a single model $B\in\xob{\spaB}$ with boundaries being the respective $\get_i$-images.
\end{proof}
The theorem shows that combining a-lenses in this way yields an $n$-ary symmetric lens, whose properties can automatically be inferred from the binary a-lenses.
\input{figures/pdfs/mergedMetamultimod-uml}

\exIntro. Figure~\ref{fig:mergedMetamod-uml} shows a metamodel $M^+$ obtained by merging the three metamodels $M_{1,2,3}$ from \figri\ without loss and duplication of information. In addition, for persons and companies, the identifiers of their  original model spaces can be traced back via attribute ''spaces'' 
(\Commute-objects are known to appear in space $\spA_3$ and hence do not need such an attribute). As shown in \cite{me-ecmfa17}, any consistent multimodel $(A_1...A_n, R)$ can be merged into a comprehensive model $A^+$ instantiating $M^+$. Let 
$\spB$ be the space of such together with their comprehensive updates \frar{u^+}{A^+}{A'^+}. 

For a given $i\le 3$, we can define the following a-lens $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$:
$\get_i$ takes update $u^+$ as above and outputs its restriction to the model containing only objects recorded in space $\spA_i$. Operation $\putl_i$ takes an update \frar{v_i}{A_i}{A'_i} and first propagates it to all directions as discussed in \sectref{sec:example}, then merges these propagated local updates into a comprehensive  \spaB-update between comprehensive models. This yields a span of a-lenses that implements the same \syncon\ behaviour as the symmetric lens discussed in \sectref{sec:example}.

\noindent {\em\bf  From (symmetric) lenses to spans of a-lenses.} There is also a backward transformation of (symmetric) lenses to spans of a-lenses. Let $\ell=(\mspaA, \ppg)$ be a (very) wb lens. It gives rise to the following span of (very) wb a-lenses $\ell_i^\preccurlyeq=(\prtbf_i(\mspaA),\spaB,\get_i, \putl_i)$   
where space $\spaB$ has objects $(A_1\ldots A_n,R)$ with $R\in \Corrx{A_1...A_n}$ a consistent corr, and arrows are the update tuples of $\mspA$. Functors $\get_i:\spaB\to \spaA_i$ are projection functors. Given $B = (\tupleAWOB, R)$ and local update \frar{u_i}{A_i}{A'_i}, let

%\noindent 
\frar{\putl^B_{i\indb}(u_i)\eqdef(u_1',..,u'_{i-1}, (u_i;u_i'), u'_{i+1},..,u_n')}
{(A_1... A_n,R)}{(A''_1... A''_n,R'')}
\\[1ex] 
where $u_j' \eqdef \ppg^R_{ij}(u_i)$ (all $j$) and $R'' = \ppg_{i\star}^R(u_i)$. Finally, $\putl^B_{i\inda}(v_i)\eqdef\ppg^R_{ii}(v_i)$, \ie, 
$v_i^{@B}=v_i^{@R}$. 
Validity of \zdmodtok{\lawname{Hippocr1-2}}{\lawname{Stability}}{}, \lawname{Reflect0-2}, \lawname{PutGet} and \kputputlaw\ directly follows from the above definitions. This yields 
\begin{theorem}\label{theo:lens2span}
Let $\ell = (\mspA, \ppg)$ be a (very) wb symmetric lens. Then the multi-span 
\[(\ell_i^\preccurlyeq=(\prtbf_i(\mspaA),\spaB,\get_i, \putl_i) \mid i=1..n)\]
of (very) wb a-lenses (where \spB\ is defined as specified above) has the same synchronisation behaviour w.r.t.\ model spaces $(\prtbf_i(\mspaA)\mid i=1..n)$.  
\qed
\end{theorem}

\newpii{
An open question is whether the span-to-lens transformation in Thm.\ref{thm:LensesFromSpans} and the lens-to-span transformation of Thm.~\ref{theo:lens2span} are mutually inverse. It is easy to see that the chain 
\begin{equation}\label{eq:lens2span2lens}
\mbox{symmetric lens $\rightarrow$ wide span $\rightarrow$ symmetric lens} 
\end{equation}
results in a lens isomorphic to the initial one, but the chain 
\begin{equation}
\mbox{wide span $\rightarrow$ symmetric lens $\rightarrow$ wide span} 
\end{equation}
ends with a different span as the first transformation above loses information about updates in the head of the span. 
 The results for the binary case in \cite{jr-jot17} show that the two spans can only be shown to be equivalent modulo certain equivalence relation, and an equivalence relation between lenses is also needed to tune all constructs into harmony. These equivalences may be different for our multiary lenses with amendments, and we leave this important question for future research.  
}{1}{-17em}
 \endinput
 
%============= Old Version ========= 
 \begin{theorem}[Lenses from Spans]\label{thm:LensesFromSpans} An $n$-ary span of wb a-lenses $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$, $i=1..n$ (note the common base \spaB\ of all $\ebb_i$) gives rise to a wb  (symmetric) lens $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$.
% 	
  	Moreover, $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$ is invertible as soon as the span satisfies the following condition%
 	\footnote{Found for the binary case by Bob Rosebrugh \cite{bob-invert}}: 
% 	$$
% 	\putl^B_{\indb i}
% 	$$
$\PP^B_i=\PP^B_j$ for all $B\in\xob{\spaB}$ and $i,j\le n$, where for given $B$ and $i$,  $\PP^B_i$ is the inverse image of 
$\xarr{\spaB}(\get_i(B),\_)$, \ie,  the set $\compr{\putl^B_{\indb i}(v_i)}{\frar{v_i}{\get_i(B)}{\_}}$. %, then $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$ is invertible.
\end{theorem}
\shortlong{}{%}
\begin{proof}
An $n$-ary span of a-lenses $\ebb_i^{\preccurlyeq}$ (all of them interpreted as symmetric lenses $\ebb_i$ as explained above) is a construct equivalent%
\footnote{To make it precise, we need to introduce a simple notion of lens equivalence, which identify lenses with the same propagation behavior but, perhaps, different sets of corrs -- see. \eg, \cite{jr-jot17}} to the star-composition of Def.~\ref{def:star-comp}, in which lens $\ekk=\idlensna$ and peripheral lenses are lenses $\ebb_i$. The junction condition is satisfied as all base updates are $\ebb_i$-closed for all $i$ by Lemma \ref{lemma:asymm_symm}, and also trivially closed for any identity lens. The theorem thus follows from Theorem~\ref{th:star-comp}. Note that a corr in $\xstar{(\Sigma_{i=1}^n\ebb_i^{\preccurlyeq})}$ 
 is nothing but a single model $B\in\xob{\spaB}$ with boundaries the respective $\get_i$-images. \qed
 \end{proof} 
}
For the backward transformation of lenses to spans of a-lenses, we use our observation in footnote~\ref{ft:mspa-as-cat} on p.~\pageref{ft:mspa-as-cat}.
\begin{theorem}[Spans from lenses] \label{th:lens2span}Any {(not necessarily invertible) }wb lens $\ell=(\mspaA, \ppg)$ gives rise to a span of wb a-lenses $\ell_i^\preccurlyeq=(\spaA_i,\spaB,\get_i, \putl_i)$. \\
%{\color{red}We should say already here, how $\ell$ is related to the resulting construction of Thm \ref{thm:LensesFromSpans} for $\ell_i^\preccurlyeq$, see below}
\end{theorem}
\shortlong{}{%}
\begin{proof} Let $\mspA$ have model spaces $\spaA_i$ and corr set $\R$ with corresponding boundary functions $\partial_i$. Let 
\[\spaB = \{(A_1, \ldots, A_n, R)\mid \partial_i(R) = A_i \mbox{ for all }i\}\] 
be the set of all aligned consistent multimodels and $\get_i:\spaB\to \spaA_i$ be projections, \ie\ $\get_i(A_1, \ldots, A_n, R)= A_i$ and $\get_i(u_1, \ldots, u_n)= u_i$\footnote{
Recall the definition of multimodel updates in Def.\ref{def:multispace}: There is no update component for $R$ 
}. Given $B = (A_1, \ldots, A_n, R)$ and update \frar{u_i}{A_i}{A'_i}, we define
\[\putl^B_{i\indb}(u_i)=(u_1', \ldots, u'_{i-1}, u_i;u_i', u'_{i+1} \ldots, u_n'): (A_1, \ldots, A_n, R)\to (A_1'', \ldots, A_n'', R''),\]
where $u_j' \eqdef \ppg^R_{ij}(u_i)$ for all $j$, $R'' = \ppg_{i\star}^R(u_i)$ and $\putl^B_{i\inda}(v_i)=\ppg^R_{ii}(u_i)$. 

That well-behavedness carries over from $\ell$ to the a-lenses is an direct consequence of the respective definitions. 
 \qed
\end{proof} 
}
%An important issue is how the two transformations, lenses to spans and spans to lenses, interact. To manage this, we need an $n$-ary counterpart of the theory of lens equivalence developed by Johnson and Rosebrugh in \cite{jr-jot17} for the binary case.  We leave it for future work. 
It is easy to see that $\Sigma_{i\in I_\ell}\ell_i^\preccurlyeq = \ell$ for any lens $\ell$, but if we begin with a span of a-lenses $\ebb_i$, $i\in I$ build a lens $\Sigma_{i\in I}\ebb_i$ and then build the span $(\Sigma_{i\in I}\ebb_i)^\preccurlyeq_i$, the two spans are different. This difference could disappear with a suitable notion of span equivalence, which we conjecture should be a straightforward generalization of the equivalence developed by Johnson and Rosebrugh in \cite{jr-jot17} for the binary case.  %which we think should be generalizable for the $n$-ary case. We leave it for future work. 
%
%\begin{example}
%Running
%\end{example}

\endinput
\begin{theorem}[Sequential composition]
	Let \lensar{\aekk}{\spaA}{\spaB} and  \lensar{\aell}{\spaB}{\spaC} be two wb a-lenses satisfying the following {\em junction condition}: all updates in $\spaB$ obtained by $\ekk$-propagation from \spaA\ are $\ell$-closed. Then there is a uniquely defined wb a-lens \lensar{\aekk;\aell}{\spaA}{\spaC}. %The composition is associative with identity lenses \lensar{\ell_{\id_{\spaB}}}{\spaB}{\spaB} being its units. 
\end{theorem}
 \input{figures/diags/seq-comp} 
 \textit{Proof.} Obviously, composition of \Kupd-preserving functors  
\flar{\get^\ekk}{\spaA}{\spaB} and \flar{\get^\ell}{\spaB}{\spaC} is a \Kupd-preserving functor: $\get^{\ekk;\ell}=\get^\ekk\circ\get^\ell$. Now we define $\putl^{\ekk;\ell}$. 
Let $u$ be an update as shown in \figref{fig:seq-comp} where horizontal lines are \get-corrs. Let $v=\putl^{\ekk B}_\indb(u)$, $u'=\putl^{\ekk B}_\inda(u)$, and $w=\putl^{\ell C}_\indb(v)$ (by the junction condition $v'=\id_{B''}$).  
%Finally, $u^*{=}\,\get^\ekk(v')$.  
Define $\putl^{C~\ekk;\ell}_\indb(u)=w$ and $\putl^{C~\ekk;\ell}_\inda(u)=u'$. Laws \lawname{Reflect1,2, 3} for $\ell;\ekk$ are obvious. %To prove idempotency \lawname{Reflect2}, we note that as $(v, v')\in\Kupd{B''}$ by $\ell.\lawname{Reflect}$, $u''\Kupd_{A''}u^*$ as $u''=u;u'=\get^\ekk(v)$ owing to $\Kupd$-preservation by $\get^\ekk$. Hence, by $\ekk.\lawname{PutPut}$, $\pult^{B \ekk}(u'';u^*)=\putl(u'');\putl(u^*)$
Stability and Putput are obvious too. 



==> ll-sections/aa-lensDef-semiDiscrete.tex <==
\begin{defin}[Indexed Asymmetric Lenses, cf. \cite{me-fase18}]
	Let \spaA\ and \spB\ be model spaces, \ie, categories with compatibility relation \Kupd. 
	An {\em indexed asymmetric lens  with amendment (indexed aa-lens)} from \spA\ to \spB\ is given by the following data. 
	
	a) A family of functors \frar{\get_p}{\spA}{\spB}, $p\in P$ whose indexes are called {\em parameters}
	

	b) A family of operations $\putpa$ indexed by pairs $(p\in P, A\in\xob{\spA})$ %(read ``put the view update back'') 
	of the following arity. Provided with a target update \frar{v}{\get_p(A)}{B'} at the input, operation $\putpa$ outputs three elements as illustrated by diagram in \figref{fig:ppg-schema}(a)
	
	b1) a source update \frar{u=\putpa_\indb(v)}{A}{A'} 
	
	b2) a parameter update  $p'=\putpa_\upd(v)$
	
	b3) an amendment to the target update, %$\putpa_{\self}(v)$ or 
	\frar{\amex{v}=\putpa_{\self}(v)}{A'}{A''}. 
	%such that $v;\amex{v}=\get(u')$. 
	
	\begin{figure}
%	\begin{equation}
\begin{tabular}{c@\qquad c}
	% column 1
	\begin{diagram}[w=5em,h=2em]
		% row 11
		 \dbox{A} & \rMapsto^{{:}\get_p} & \dbox{B}
		\\  % row 12
		&&\dTo>v
		\\ % row 13
	\dDashto>u&
		\swseTilearrowAB{{:}\putpa}{}
		%\seTilearrowAB{}{}
	%	\Downarrow %{:}\putpa
		&B'
			\\ % 14
		&&\dDashto>{\amex{v}}
		\\ % 15
A' &\rDermapsto^{{:}\get_{p'}} & B''
	\end{diagram}
%------------
& % column 2	
%--------------
	\begin{diagram}[w=5em,h=5ex]
		% row 21
	\dbox{A} &\rMapsto^{{:}\get_p} & \dbox{B} & \rMapsto^{{:}\get_q} & \dbox{C}
	\\  % row 22
	&&&&\dTo>w
	\\ % row 23
	&	\swseTilearrowAB{~~2{:}\putpa}{}&\dDashto>v&
	     \swseTilearrowAB{~~1{:}\putqb}{}&C'
	\\ % 24
	&&&&\dDashto>{\amex{w}}
	\\ % 25
	\dDashto<u &
%	\swTilearrowAB{}{~~~{:}\putpa}{}
		& B' &\rDermapsto^{{:}\get^{(1)}_{q'}} & C''
	\\  % row 26
	&&\dDashto>{\amex{v}}& \stackrel{3{:}\get_{q'}}{\Longrightarrow}&\dDashto>{\get^{}_{q'}(\amex{v})}
	\\  % row 27
	A' &\rDermapsto^{\get^{(2)}_{p'}} & B''&\rDermapsto^{{:}\get^{(3)}_{q'}}& C''''
	\end{diagram}
\\  [10pt] % End OF TABULAR ROW 1
(a)  & (b)
\end{tabular}
	%	\end{equation}
	\caption{Schemas of update propagation: (a) the arity of \putl, and (b) composition. Input elements are boxed (nodes) and solid (arrows), output elements are not boxed and dashed.
	\label{fig:ppg-schema}}
\end{figure}
A target update \frar{v}{\get(B)}{A'} is called {\em closed} if %$\putl^B_\inda(v)=\id_{A'}$. 
$\amex{v}=\id_{A'}$, and an aa-lens is {\em closed} if all its target updates are closed.  \qed
\end{defin}


==> ll-sections/aalens-wblaws-bulkyNotation.tex <==


%=== bulk notation 
{ 
\renewcommand\ppgB{\ensuremath{\putl^B}}
\begin{defin}[Well-behavedness]\label{def:wbalens}
An a-lens is {\em well-behaved (wb)} if it satisfies the following laws for all $B\in\xob{\spaB}$, \frar{v}{\get(B)}{A'}, and \frar{u}{B}{B'}:
%
\\[1ex]
\lawgap=1ex
\noindent \begin{tabular}{l@{\quad}l}
%		\lawnamebr{Hippocr1}{
%        \frar{u}{B}{B'}
%		} & 
%		if $\get(B) = \get(B')$, then $\get(u) = \id_{\get(B)}$
%		\\ [\lawgap]\lawnamebr{Hippocr2}{
%		\frar{v}{\get(B)}{A'}
%		}	& 
%			if $A'=\get{B}$, then $\ppgB_\indb(v) = \id_B$,   $\ppgB_\inda(v)=\id_{\get(B)}$
%		%$\ppgB_{\indb}(\id_{\get(B)})=\id_{B}$
%		\\
%		& \parbox{15em}{\textcolor{red}{the two laws above are just a reminder of a path that was rejected} }
%		\\
\lawnamebr{Stability}{
	%\frar{v}{\get(B)}{A'}
}	& 
if %\frar{v}{\get(B)}{A'} is identity, 
   $v=\id_{\get(B)}$, then $\ppgB_\indb(v) = \id_B$ and  $\ppgB_\inda(v)=\id_{\get(B)}$
%$\ppgB_{\indb}(\id_{\get(B)})=\id_{B}$
		\\  [\lawgap] \lawnamebr{\reflectzero}{
		    % \frar{v}{\get(B)}{A'}
		} &	
		%$\ppgB_{\inda}(v)\noteq \id_{A'}$ implies 
		%$A'\noteq \get(X)$ for all $X\in\xob{\spaB}$
		if $A'=\get(X)$ for some $X\inn\xob{\spB}$, then $\ppgB_{\inda}(v)=\id_{A'}$
		\\  [\lawgap] \lawnamebr{Reflect1}{
		%\frar{v}{\get(B)}{A'}
		} &	
		$(v, \ppgB_{\inda}(v))\in \Kupd_{A'}$ %for all $u_i$ 
		\\  [\lawgap] \lawnamebr{Reflect2}{
		%\frar{v}{\get(B)}{A'}
		} &
		$\ppgB_{\indb}(v;\ppgB_{\inda}(v)) = \ppgB_{\indb}(v)$
		\\ [\lawgap] \lawnamebr{PutGet}{
		%\frar{v}{\get(B)}{A'}
		} & %$_{~~~~~~}$
			%$v;v'=\get(v.\putl_\indb^B) $	% dot version
		$v;\putl^B_\inda(v)=\get(\putl_\indb^B(v)) $   % bracket version 
\end{tabular} \\
\rule{0mm}{0mm}\qed
\end{defin}
}

==> ll-sections/aalens-wblaws.tex <==
%\zd{TO BE COMPLETED!!!!}
%Note red commutativity symbol in the triangle $T_p T_{p'}T^@$, whcih implies commutativity of the adjoint triangle; equivalently, commutativity of the latter implies commutaivity of the former). For \bx, Putget is a fundamental requirement.....
%\begin{remark}
%====
%\begin{remark}	
%If \spS, \spT, and \spP\ are codiscrete categories (sets), then an apa-lens is nothing but a learner as defined in \citefst. Operations $\putps^\upd(v)$ and $\putps^\req(v)$ correspond to theirs update $\mathcal{U}(p,S,T')$ and request $r(p,S,T')$ operations; amendment $\putps^\self$ is new but for the codiscrete case. we can define $T^@$ to be $\get_{p'}(S')$ so that PutGet automatically holds (see however Remark \ref{rem:?}). % degenerates into juts a notation for $\get_{p'}(S')$.
%\end{remark}


{ % --> version with v^@ rather than put^B_indv(v) @
	\renewcommand\ppgB{\ensuremath{\putl^B}}
	\renewcommand\ppgB{\ensuremath{\putps}}
	\begin{defin}[Well-behavedness]\label{def:wbalens}
		%In addition to the Putget law above, consider two more equational laws
		%he following two list of requirements (laws) that an apa-lens could satisfy. 
		An apa-lens is called {\em well-behaved (wb)} if it satisfies the following three laws specified by equations to hold for all $p\in P$, $S\in\xob{\spS}$ and \frar{v}{T_p}{T'} where $T_p$ denotes $\get_p(S)$:
		%, and \frar{u}{B}{B'}:
		\\[1ex]
		\lawgap=1 ex
				\noindent \begin{tabular}{l@{\quad}l}
			%		\lawnamebr{Hippocr1}{
			%        \frar{u}{B}{B'}
			%		} & 
			%		if $\get(B) = \get(B')$, then $\get(u) = \id_{\get(B)}$
			%		\\ [\lawgap]\lawnamebr{Hippocr2}{
			%		\frar{v}{\get(B)}{A'}
			%		}	& 
			%			if $A'=\get{B}$, then $\ppgB_\indb(v) = \id_B$,   $\ppgB_\inda(v)=\id_{\get(B)}$
			%		%$\ppgB_{\indb}(\id_{\get(B)})=\id_{B}$
			%		\\
			%		& \parbox{15em}{\textcolor{red}{the two laws above are just a reminder of a path that was rejected} }
			%		\\
			\lawnamebr{Stability}{
			}	& 
			if $v=\id_{T_p}$ %where $B=p^*(S)$, 
			then all three propagated updates 
			%\\  & 
			$e,u,\amex{v}$ are identities: 
			\\
			& $\putps^\upd(\id_{T_p})=\id_p$, \quad%
			   $\putps^\req(\id_{T_p}) = \id_S$, \quad%    
			   $\putps^\self(\id_{T_p})=\id_{T_p}$
%			%\\  [\lawgap] \lawnamebr{\reflectzero}{
%			%			} &	
%			%			if $v=\get(u)$ for some \frar{u}{A}{A'}, then $\amex{v}=\id_{B'}$
%			\\  [\lawgap] \lawnamebr{K{-}amendment}{
%			} &	
%			$(v, \amex{v})\in \Kupd_{B'}$ %for all $u_i$ 
			\\  [\lawgap] \lawnamebr{Closure}{
						} &
						$\ppgB^{\indb}(v;\amex{v}) = \ppgB^{\indb}(v)$
					 \mbox{\em 	where $\amex{v}$ denotes $\putps^\self(v)$}
			\\ [\lawgap] \lawnamebr{weakPutget}{
			} & %$_{~~~~~~}$
			$v;\amex{v}=(v.\putps^\upd.\get_S)\,;\,(v.\putps^\req.\get_{p'})$, 
%			%
%			\mbox{\em or, equivalently}, 
%			\\ [\lawgap] \lawnamebr{Putget}{'
%		}&$v;\amex{v}=(v.\putps^\req.\get_{p})\,;\,(v.\putps^\upd.\get_{S'})$
	\\ [\lawgap] \lawnamebr{Putget}{
	} & %$_{~~~~~~}$
	$%e_S\eqdef 
	v.\putUL{\upd}{p,S}.\get_S= \id_{T_p} \mbox{  and }
		v;\amex{v}=v.\putps^\req.\get_{p'}$, 
		\\ [\lawgap]
				\end{tabular} \\
		%\rule{0mm}{0mm}\qed
			%When we will need to refer to compliance to these laws separately, we will 
			We call a lens {\em stable} if it satisfies Stability, and an {\em SPg-lens} if it satisfies Stability and Putget.  
			
			We call delta $v$ {\em closed} if $\amex{v}=\id_{T}$; an apa-lens is {\em closed} if each target delta is closed. %or {\em spgc-lens} if it also satisfies Putget and Closure resp. 
			% it satisfies, resp., the laws of stabiluty  with {\em  K-amendments}, with {\em closed amendments}, and a {\em Putget-lens} if it satisfies the respective law. 
			%
		%	We say a lens is {\em well-behaved (wb)} if it is a stable PutGet-lens with K-amendments,  and a wb-lens is called {\em wb+-lens} if it also has closed amendments. 
	\end{defin}
Note that condition Closure only requires full amendment deltas $v;v^@$ to be closed, which is  much weaker than the defining condition of closed lens, which requires {\em each} delta to be closed. %as to be fulfilled in closed lenses.  
%\begin{remark}\label{rema:putget}%\zd{to be reworked}
%	The Putget law may seem a notational trick rather than a law: indeed, operation $\putps^\req$  provides delta $u$, and functor $\get_{p'}$ sends it to a delta  $\get_{p'}(u)$ targeting at some model $T''$ anyway. However, the Putget law requires much more certainty about $T''$ and precisely specifies the relationship between $T'$ and $T''$, namely, it says that they are related by a specified update $\amex{v}$.
%\end{remark}
\begin{example}[Identity lenses]\label{ex:idlens} %$\mathcal{id}$
	Any skeletal category \spA\ gives rise to an apa-lens $\idl_\spA$ with the following components. The source and target spaces are equal to \spA, and the parameter space is \tcat\ (a category with a single object * and a single arrow $\id_*)$. Functor $\get_{*}$ is the identity functor and all puts are identities. Obviously, this lens is wb.
\end{example}
\begin{example}[Iso-lenses]\label{ex:isolens}
	Let \frar{\iota}{\spA}{\spB} be an isomorphism between model spaces. It gives rise to a simple wb apa-lens \frar{\ell(\iota)}{\spA}{\spB} with $\spP^{\ell(\iota)}=\tcat$ as follows. Given any $A$ in \spA and \frar{v}{\iota(A)}{B'} in \spB, we define $\putl^{\ell(\iota).\req}_{*,A}(v) = \iota^{-1}(v)$ and the two other put operations send $v$ to identities. 
\end{example}
\begin{example}[Bx lenses]\label{ex:bxlens} Examples of SPg and wb aa-lenses can be found in \cite[ext.version]{me-fase18}: they all can be considered as apa-lenses with a trivial parameter space \tcat. 
\end{example}
\begin{example}[Learners (borrowed from \citefst\ but rearranged)]\label{ex:mlasbx}
	Let \frar{\err(x,y)}{\Reals\timm\Reals}{\Reals} be a differentiable  {\em error} function such that \frar{\prtfrac{\err}{x}(x_0,-)}{\Reals}{\Reals} is invertible for any given $x_0$. For an $n$-dimensional Euclidean space $\reals^n$, we define the {\em total} error function \frar{\Err}{\rreals}{\reals} by $\Err(a,a')=\sum_{i\le n}\err(a_i, a'_i)$. This converts space $\reals^n$ into a category (Lawvere's metric space) \brealsx{n}. 
	%
	A {\em \parrd\ function} from \realsx{m} to \realsx{n} is a differentiable function \frar{I}{\realsx{k}\timm\realsx{m}}{\realsx{n}} (and hence a functor \frar{I}{\brealsx{k}\timm\brealsx{m}}{\brealsx{n}}). 
	
	It is shown in \citefst\ that, given a {\em step size} $\eps\in(0,\infty)$,  any parameterized function \frar{I}{\realsx{m}}{\realsx{n}} gives rise to an ap-lens \frar{\ell_\eps(I)}{\brealsx{m}}{\brealsx{n}} called in \citefst\ a {\em learner}.%
	%\footnote{Warning: our models $S$ (for source) and $T'$ (target) are theirs $a$ and $b$ rather than $b'$.}
	\footnote{Moreover, they show the functoriality of the construction.} To make it an apa-lens, we need to add amendments by defining $T^@=b'=I(p',a')$; then Putget trivially holds as there is only one arrow (distance/error) between any two objects. 
    
    Any learner $\ell_\eps(I)$ can be made stable if we direct it to do nothing when $\Err(I(p,a),b)=0$. 
\end{example}
}

\endinput
%The following result is straightforward.
%\begin{propo}[Codiscrete \lner s]
%	(a) Learners defined in \citefjbx\ are codiscrete lenses without amendment. 
%	%
%	(b) Any codiscrete lens without \amend\ \zdmod{gives rise to a codiscrete Putget-lens with \amend\ in a unique way.}{enjoys Putget and K-amendment....}{}
%\end{propo}
%\begin{discuss}[Why non-trivial updates?]
%\end{discuss}

\zd{what is below is simply copied from the faoc paper. probably, it's not needed. }

==> ll-sections/aboutDefLens.tex <==
\subsubsection{Defining asymmetric learning delta lenses (al-lenses) and their composition  (sequential and parallel).
	% with amendment, \alalenscat.
} 
It could be called categorification of the learning lens notion: we will work with {\em delta} lenses,  in which a change/delta between objects $x,x'$ is an arrow \frar{u}{x}{x'} rather than a pair $(x,x')$; moreover, multiple different updates/deltas are possible between the same objects $x,x'$ so that $\Hom(x,x')$ is a set (non-empty for a typical \bx\ application in MDE). Each species of a delta lens has its codiscrete version, in which $\Hom(x,x')=\{(x,x')\}$, and learners defined in \citefst\ are exactly codiscrete al-lenses.%
\footnote{In detail, the category of learners \learncat\ defined in \citefst\ coincides with the category of codiscrete al-lenses \allenscatcodi, which is a  full sm-subcategory of the sm-category of al-lenses \allenscat.}
In this paper, a lens will always mean a delta lens by default.  
%The original lenses of then become the codiscrete specialization of delta lenses. %, whose only arrows are pairs $(x,x')$ and any such a pair is an arrow (in \bx, any object $x$ can be updated to any other object $x'$ so that categories of objects of interests are bidirectionally connected: $\mathit{Hom}(x,x')\noteq\varnothing$ for any pair $x,x'$). In this paper, a lens will always mean a delta lens while lenses employed in \citefetal\ are referred to as codiscrete. 

In the MDE context, objects $x,x'$ are complex structures so that their delta/update \frar{u}{x}{x'} is a complex structure too. Its ignorance in the codiscrete lens formalism may create fundamental problems for applying codiscrete lenses to practical problems (see \cite{me-jot11}). The role of deltas in the ML context, where objects $x,x'$ are tuples of real numbers, is probably less fundamental but still important---we will briefly discuss it below in \sectref{ddlens-1}. %and continue  in \sectref{deltas4ml}. 




==> ll-sections/actions.tex <==
\section{View systems and lenses with edits}

%======
%\input{figures/diags/difasfun1}
\input{figures/diags/difasfun-edit-lens}
%\input{figures/diags/difasfun3}
%====
%\input{figures/pdfs/getAmend-inR}
%====

{
\renewcommand\ovre{\ovr{u}}
\begin{defin}[model spaces with edits]\label{def:editmodspace}
	An {\em model space} is a triple is given by a skeletal category \spX\ and a monoid \DDel\ of {\em deltas} (also called {\em edits} or {\em updates}) acting on \spXX: for any $u\in \DDel$ and $X\in|\spXX|$, there is defined an arrow \frar{X\odash u}{X}{X'} in \spXX. We will write this arrow as \frar{\ovre}{X}{X'} and call action \odash\ {\em lifting}, and sometimes denote $X'$ by $X\cdot u$ so that $\odot$ denotes the object action determined by \odash-action. Lifting is required to be unital: $X\odash 1=\id_X$, and be compatible with composition: given edits $u, u'$, $X\odash ee'=(X\odash u);(X\odot u\;\odash u')$, that is, $\ovr{uu'}=\ovre;\ovr{u'}$. 
\end{defin}
\begin{defin}[incremental view system with edits]\label{def:editviewsys}
	Let \spS\ and \spT\ be model spaces (with edits. An {\em (incremental parametrized) view system with edits} 	from \spS\ (the {\em source} of the view) to \spT\ (the {\em target}) is given by 
	
	i) a model space \spP\ of {\em parameters},
	
	ii) an object function \frar{|\get|}{|\spP|\timm|\spS|}{|\spT|},
	
	iii) for any pair $p\in|\spP|$, $S\in |\spS|$, a monoid morphism \frar{\prt^\get_\spS(p,S)}{\DDel_\spS}{\DDel_\spT} endowed with a mapping \frar{@^\get_\spS(p,S)}{\DDel_\spS}{\spT(S_{pu}, \_)} (see diagram \eqref{difasfun-edits} for the meaning of $S_{pu}$) such that for any $u\in\spS(S,\_$, the target of $u.@^\get_\spS(P,S)$ equals to $S'_p$ as shown in the diagram. 
	
	iv) for any pair $p\in|\spP|$, $S\in |\spS|$, a monoid morphism \frar{\prt^\get_\spP(p,S)}{\DDel_\spP}{\DDel_\spT} endowed with a mapping \frar{@^\get_\spP(p,S)}{\DDel_\spP}{\spT(S_{pe}, \_)} with all conditions shown in diagram \eqref{difasfun-edits} but with delta $e\in\spP(p,\_)$ rather than $u\in\spS(p,\_)$
\end{defin}
}
It is easy to see that any view system with edits as defined above gives rise to a view system as defined in \defref{viewsys}


Metrics is given by some differentiable function \frar{\err}{\reals\times\reals}{\reals} and for any $a,a'\in\reals^m$, the distance  %\frar{\ovr{\del}=\Err(a,a')}{a}{a'} 
is computed by summation: $\Err(a,a') :=\sum_{i\le m}\err(a_i,a'_i)$ (we follow \citefst).
%$=\sum_{i\le m}\err(a_i,a_i+\del_i)$. 
We consider the metric space $(\reals^m, \Err)$ as a category $\rcat^m$ enriched over Lawvere's posetal monoid $\nil=(\reals_{\ge 0}, +, 0, \ge)$ (the composition being the triangle inequality). Next we introduce monoid $\DDel^m=(\reals^m, +, 0)$ with $+$ and $0$ defined componentwise, and this monoid acts on $\rcat^m$ in an obvious way: given $\del\in\DDel^m$ and $a\in\reals^m$, $a\oplus\del\eqdef a+\del=(a_i+\del_i, i\le m)$ (with $\oplus$ denoting action) is uniquely defined. We can consider this action as a discrete opfibration as shown by the leftmost square in diagram \eqref{difasfun}, where the lift \ovr{\del} is the distance $\Err(a, a+\del)$.  Given a differentiable function \frar{r}{\reals^m}{\reals^n} and point  $a\in\reals^m$, we have a monoid homomorphism \frar{\prtf_a}{\DDel^m}{\DDel^n} such that for any $\del\in\DDel^m$
\begin{equation}\label{eq:getamend}
(a\oplus \del).f = a.f\oplus\ \del.\prtf_a + o(\del) 
\end{equation}
where $o(\del)$ denotes the higher-order part of the difference (given by the sum of the higher-order terms in the Taylor series for analytic $f$) which converges to 0 if \del\ converges to 0. The right part of \eqref{getamend} can be seen as arrow composition in $\rcat^n$ as shown in diagram \eqref{difasfun}.


The chain rule nicely fits in this treatment: given \frar{f}{\reals^m}{\reals^n} and \frar{g}{\reals^n}{\reals^o}, for any $a\in\reals^m$, we have $\prtx{(f;g)}_a=\prtx{f}_a;\prtx{g}_{a.f}$. % if we have functions \frar{f, g}{\reals}{\reals}, then it's straightforward to check that $\widehat{f;g}=\hat f;\hat g$.


==> ll-sections/apalensdefs.tex <==
%\clearpage
\section{Asymmetric Learning Lenses (with Amendments) (ALA-Lenses)} %and their laws}
\label{sec:alalens}

%\input{ll-sections/modSpaces-short}
%\input{ll-sections/aa-lensDef-semiDiscrete}

%\subsection{Apa-lenses}
%Given a category \spC, its collection of objects is denoted by $|\spC|$. An arrow with domain $A\in|\spC|$ will often be denoted by \frar{u}{A}{\_} and similarly \frar{u}{\_}{B} is an arrow with codomain $B$. 
\begin{defin}[Model spaces]
	A {\em model space} is a small category, in which all isomorphisms are identities (which is stronger than being skeletal). Objects are called {\em models} and arrows are {\em deltas} or {\em updates}. %with compatibility relation \Kupd. 
\end{defin}
\vspace{-0.5cm}
\begin{defin}[\alalens es]% cf. \cite{me-fase18}]\label{def:aalens-arity}
	Let \spS\ and \spT\ be categories. An {\em \alalens}
	from \spS\ (the {\em source} of the lens) to \spT\ (the {\em target}) is 
	a pair $\ell=(\get, \putl)$ whose first component is a p-functor \fprar{\get}{\spS}{\spT}{\spP} and the second component is a triple of operations 
	$\putl=(\putps^\upd,\putps^\req,\putps^\self) $
	indexed by pairs $p\in|\spP|$, $S\in|\spS|$. We will write such a lens as an arrow \fprar{\ell=(\get,\putl)}{\spS}{\spT}{\spP}
	
	given by the following three components a-c.
 \begin{enumerate}[label={\bf  \alph*)}, %Step 
	%\arabic{enumi}., ref=Step \arabic{enumi},% 
	wide=0pt]
\item[{\bf a) Parameters:}] A small category \spP\ of {\em parameters} (think about function/view definitions \parrd\ by objects of \spP). We denote objects of \spP\ by small letters $p,p',..$ rather than capital ones to avoid confusion with \citefst, in which capital $P$ is used for the entire parameter set.  

\item[{\bf b) Gets:}] 
A functor \frar{\get}{\spP}{[\spS,\spT]}, where $[\spS,\spT]$ is the category of functors from \spS\ to \spT\ and their natural transformations. For a parameter  $p\in|\spP|$, we write %$\get(p,\_)$ or 
$\get_p$ % or even shorter ${\_}_p$ 
for the functor \frar{\get(p)}{\spS}{\spT} (read ``get \spT-views of \spS''), and if $S\in|\spS|$ is a source model, its $\get_p$-view is denoted by $\get_p(S)$ or $S.\get_p$ or even $S_p$ (so that ${\_}_p$ becomes yet another notation for functor $\get_p$). 

Given a parameter delta \frar{e}{p}{p'} and a source model $S\in|\spS|$, the model delta \frar{\get(e)}{\get_p(S)}{\get_{p'}(S)} will be denoted by $\get_e(S)$ or $e_S$ (rather than $S_e$ as we would like to keep capital letters for objects). %although a more consistent discipline would require $S_e$).%

Since $\get_e$ is a natural transformation, for any delta \frar{u}{S}{S'}, we have a commutative square $e_S;u_{p'}=u_p;e_{S'}$. We will denote the diagonal of this square by $u.\get_e$ or \frar{u_e}{S_p}{S'_{p'}}.  Thus, we use notation
      %\begin{equation}\label{eq:u.gete}
\begin{enumerate}[label={\bf  \alph*)}, %Step 
	%\arabic{enumi}., ref=Step \arabic{enumi},% 
	wide=5pt]
\item[{\bf (b*)}]	
~~~~~~\frar{u_e\eqdef u.\get_e \eqdef e_S;u_{p'}=u_p;e_{S'}}{S_p}{S'_{p'}}
\end{enumerate}
	%\end{equation}

	\item[{\bf c) Puts:}] A family of operations $\putps$ indexed by pairs $(p\in\xob{\spP}, S\in\xob{\spS})$. %(read ``put the view update back'') 
	Each operation in the family takes a delta \frar{v}{S_p}{T'} as its input, and outputs three deltas 
	$\comprfam{\putps^{\x}(v)}%
		            {\x\in\{\req,\upd,\self\}}$ 
    specified below (names \req\ and \upd\ are chosen to match the terminology in \citefst).
	%Given a pair $(p,S)$, operation $\putpa$ takes  an update \frar{v}{p^*(S)}{T'} as its input and outputs three arrows c1-c3 as specified below and illustrated by diagram in \figref{fig:aalens-arity}
\begin{enumerate}[label={\bf  \alph*)}, %Step 
	%\arabic{enumi}., ref=Step \arabic{enumi},% 
	wide=5pt]
\item[{\bf (c1) }%$\putl_\upd$:
	]  \frar{e=\putps^\upd(v)}{p}{p'} 	is a parameter update (or transformation {\em evolution}, hence name $e$).
\item[{\bf (c2)}%$\putl_\req$:
]  \frar{u=\putps^\indb(v)}{S}{S'} is a {\em source} update (read ``put the view update $v$ back'')
\item[{\bf (c3) }%$\putl_\self$:
]
	\frar{\amex{v}=\putps^{\self}(v)}{T'}{S'_{p'}} is an {\em amendment} to the original update. 
	%where $T^@$ denotes the codomain of $u_e$
	Note that the domain and the codomain of this arrow are determined by previously defined operations so that $\putps^{\self}$ maps $v$ to an arrow in a already defined Hom-set. 
	%$\putpa_{\self}(v)$ or }
	%such that $v;\amex{v}=\get(u')$. 
\end{enumerate}
\end{enumerate}
			A lens is called {\em codiscrete} if categories \spS, \spT, \spP\ are codiscrete.
\end{defin}

%  notation4diags explained
%\input{ll-sections/notation4diags}
\input{ll-figures/pdfs/aalens-arity}
Diagram in \figari\ shows how these operations are interrelated. The upper part shows an arrow \frar{e}{p}{p'} in category \spP\ and two corresponding functors from \spS\ to \spT. The lower part is to be seen as a 3D-prism with visible front face $SS_{p'}S'_{p'}S'$ and visible upper face $SS_pS_{p'}$, the bottom and  two back faces are invisible and the \corring\ arrows are dashed. The prism denotes an algebraic term (workflow): given elements are shown with black fill and white font, while derived elements are blue (recalls being mechanically computed) and blank (double-body arrows are considered as ``blank''). The two pairs of arrows originating from $S$ and $S'$ are not blank because they denote pairs of nodes (the UML says {\em links}) rather than mappings/deltas between nodes ---we explained this notation in the previous section (where derived arrows were dashed but now we use dashing for 3D-drawing). %Link-arrows now have bulleted rather than bar tails like in $\mapsto$ due to limitations of Powerpoint used for building the diagram).
%As in diagram \figri(a), we again use numeric names for links to convey the order of operations, but now we write $i{:}p$ rather than $i{:}\get_p$ for the pair $(S, S.\get_p)$ to ease reading (below we will see diagrams that have more such arrows). By the same reason, we omit numeric scripts near vertical and diagonal arrows (deltas), and label the deltas realizing natural transformations very briefly, \eg, $e_S$ for the full name  $\get(e,S)$-- the latter will also be written in formulas as $\get_S(e)$. % or $e.\get_S$. 
%Two callouts near $1{:}p$ and $e_S$ recall these notational tricks. 
%
%}{\get(p,S)}{\get(p',S)})  . 
% For example, link labelled $1{:}\get_p$ denotes application of functor $\get_p$ to object $S$ that results in an object $T_p=\get_p(S)$.%
%\footnote{Notation with colon is suggested by UML: $1$ is the name of the link whereas $\get_p$ is its type. In a refined setting with the names \spS, \spT, $\get_p$ organized into a syntactic category, the Grothendieck construction can be seen here, but we don't need this in the present paper.}    
%In the other three link-arrows we write $i{:}p$ rather than $i{:}\get_p$ to ease reading (below we will have more such arrows). 

%\input{ll-figures/pdfs/aalens-arity}
%\spT-arrows (deltas rather than links) realizing natural transformations (such as \frar{\get(e,S)}{\get(p,S)}{\get(p',S)}) are labelled as $ij{:}e_S$ where $i,j$ are indexes of the \corring\ links to the source and target of $\get(e,S)$. %Similarly to diagram \figri(a), link indexes convey the order of operations from which the entire workflow is built, but now we skip numeric indexes on updates to ease reading (below we will have more such arrows).  The label of invoking operation \putl\ in the third step of the scenario is omitted, but instead, the 
Equational definitions of deltas $e,u,v^@$ are written up in three callouts near them. 
%
%We begin with 1) computing $T_p$, then 2) apply delta $v$ and compute three deltas $e=\putps^\upd(v)$, $u=\putps^\req(v)$, and $v^@=\putps^\self(v)$ (upper indexes near puts are not shown in the diagram; %) as Powerpoint doesn't allow having upper and lower indexing together; 
%subscripting $e$, $u$, $v^@$ with 2 would make notation heavy and we omitted it). 
Four derived deltas forming the right back face of the prism: 
$u_p=u.\get_p$, $u_{p'}=u.\get_{p'}$, and two matching them deltas $e_S=\get(e,S)$, $e_{S'}=\get(e,S')$, which together form a commutative square due to naturality of $\get(e)$ as explained earlier (see notation b*)).
%== the piece below is now outdatwd. it was about Putget law for objects/nodes====
%Finally, the diagram also shows the coincidence of  $S'_{p'}$ node  and the target $T^@$ of the amendment $v^@$ shown as an inner circle node. The equality of two objects is a special requirement (a constraint) that does not  hold automatically and to be specially postulated (the reddish  filler in-between the square and the circle recalls a constraint). Thus, the arity schema of put operations includes the following \putgeto\ equation for any given $S, p, v$
%\noindent \begin{tabular}{l@{\quad}l}
%	%\\[0.5ex] 
%	\lawnamebr{Putget}{$_0$
%	} & %$_{~~~~~~}$
% $
% \codd((\putps^\req.v).\get_{e}) =\codd(\putps^\self.v)
% $
%	\\ [\lawgap]
%\end{tabular}
%where $S'$ stands for $\codd(\putps^\req.v)$, the left equality is a constraint (red) %included into the arity schema while the right one is automatic (blue). The ``co-discreteness'' index 0 recalls that the constraint equates objects (nodes) rather than arrows. Equating arrows is the subject of a special Putget law stated below together with two other requirements to \alalens es, which would allow MDE practitioners  to call them  ``well-behaved''. 
%====  
%note the interplay between red and blue in the diagram). The constraint is named Putget$_0$ and is a prerequisite for an important delta lens law called Putget, which requires the commutativity of the triangles in the right back face of the prism (it'd be enough to require one, then the other is derived -- note a red and a blue labels [=] in the diagram, which do not belong the arity schema) --- it will formally be stated below. % is a special and important requirement called the Putget law (see the definition below). 
% =========  the law piece begins
%\input{ll-sections/aalens-wblaws}

\renewcommand\ppgB{\ensuremath{\putl^B}}
\renewcommand\ppgB{\ensuremath{\putps}}
\begin{defin}[\shortlong{Equational laws} {Well-behavedness}]\label{def:wbalens}{\emno 
		A {\em (lens) equational law} is an equation to hold for all values of three bound variables: $p\in \xob{\spP}$, $S\in\xob{\spS}$ and \frar{v}{S_p}{T'}} (as in the laws below). The following \shortlong{two}{three} laws are important: 
%		
	%The following two laws are important:}{An \alalens\ is called {\em well-behaved (wb)} if it satisfies the following {three} laws specified by equations to hold for all $p\in \xob{\spP}$, $S\in\xob{\spS}$ and \frar{v}{S_p}{T'}}
	\\[1ex]
	\lawgap=1 ex
	\noindent \begin{tabular}{l@{\quad}l}
		%		\lawnamebr{Hippocr1}{
		%        \frar{u}{B}{B'}
		%		} & 
		%		if $\get(B) = \get(B')$, then $\get(u) = \id_{\get(B)}$
		%		\\ [\lawgap]\lawnamebr{Hippocr2}{
		%		\frar{v}{\get(B)}{A'}
		%		}	& 
		%			if $A'=\get{B}$, then $\ppgB_\indb(v) = \id_B$,   $\ppgB_\inda(v)=\id_{\get(B)}$
		%		%$\ppgB_{\indb}(\id_{\get(B)})=\id_{B}$
		%		\\
		%		& \parbox{15em}{\textcolor{red}{the two laws above are just a reminder of a path that was rejected} }
		%		\\
		\lawnamebr{Stability}{
		}	& \mbox{\em 
		if $v=\id_{T_p}$ %where $B=p^*(S)$, 
		then all three propagated updates 
		%\\  & 
		$e,u,\amex{v}$ are identities:} 
		\\
		& $\putps^\upd(\id_{T_p})=\id_p$, \quad%
		$\putps^\req(\id_{T_p}) = \id_S$, \quad%    
		$\putps^\self(\id_{T_p})=\id_{T_p}$
%		%			%\\  [\lawgap] \lawnamebr{\reflectzero}{
%		%			%			} &	
%		%			%			if $v=\get(u)$ for some \frar{u}{A}{A'}, then $\amex{v}=\id_{B'}$
%		%			\\  [\lawgap] \lawnamebr{K{-}amendment}{
%		%			} &	
%		%			$(v, \amex{v})\in \Kupd_{B'}$ %for all $u_i$ 
%		\\  [\lawgap] \lawnamebr{Closure1}{
%		} &
%		$\putUL{\x}{p,S}(v;\amex{v}) = \putUL{\x}{p,S}(v) $
%		\mbox{\em  where $v^@$ denotes $\putps^\self(v)$
%		and $\x\inn\{\upd,\req\}$ }
%			\\  [\lawgap] \lawnamebr{Closure2}{
%	} &
%	$\putUL{\self}{p,S}(v;\amex{v}) = \id_{T^@}$ %\putUL{\x}{p,S}(v) $
%	%\mbox{\em  where $v^@$ denotes $\putps^\self(v)$
%	%	and $\x\inn\{\upd,\req\}$ }
%%		\\ [\lawgap] \lawnamebr{weakPutget}{
%%		} & %$_{~~~~~~}$
%%		$v;\amex{v}=(v.\putps^\upd.\get_S)\,;\,(v.\putps^\req.\get_{p'})$, 
%%		%			%
%%		%			\mbox{\em or, equivalently}, 
%%		%			\\ [\lawgap] \lawnamebr{Putget}{'
%%		%		}&$v;\amex{v}=(v.\putps^\req.\get_{p})\,;\,(v.\putps^\upd.\get_{S'})$
		\\ [\lawgap] \lawnamebr{Putget}{
		} & %$_{~~~~~~}$
	\mbox{ 
		 $(\putps^\req.v).\get_{e} = v; v^@$ %\putps^\self.v)
%				$v;\amex{v} = u_e \eqdef (\putps^\req.v).\get_{p};(\putps^\upd.v)_{S'} =
%		(\putps^\upd.v)_{S};(\putps^\req.v).\get_{p'})
%		$,
		 where $e=\putps^\upd(v)$ and $v^@= \putps^\self(v)$
	 } % end \em 
 \shortlong{}{
	 	\\ [\lawgap]
				\lawnamebr{Hippocr}{
		}	& \mbox{\em 
			if $\get_p(u)=v$ for some \frar{u}{S}{S'}, 
			then $v^@=\id_{T'}$
	                       }
                   } %end long 
	\end{tabular} \\[10pt] 
	%\rule{0mm}{0mm}\qed
	%When we will need to refer to compliance to these laws separately, we will 
{\emno A lens is {\em stable} if it satisfies Stability, and an {\em SPg-lens} if it satisfies Stability and Putget.  \shortlong{}{A lens is called {\em Hippocratic} if the (Hippocr) law holds.%
	\footnote{The term Hippocratic and its derivatives were coined for Bx by Perdita Stevens \cite{stevens-sosym10} to refer to a family of requirements sharing a common intention of doing nothing if consistency is not violated, which 
	can be seen as an application of a major medical principle ``First, do no harm'' usually attributed to the Hippocratic oath --- see Wikipedia {\tt https://en.wikipedia.org/wiki/Hippocratic\_Oath} for details.} 
An SPg Hippocratic lens is called {\em well-behaved (wb)}
}  % end of long
%	
%	A target delta $v$, is {\em closed} if $v^@=\id_{T'}$; an \alalens\ is {\em closed} if each target delta is closed. %or {\em SPg-lens} if it also satisfies Putget and Closure resp. 
}
\end{defin}  %}
\begin{remark}{\emno 
%a) Condition Closure only requires full amendment deltas $v;v^@$ to be closed, which is  much weaker than the defining condition of closed lens requiring  {\em each} delta to be closed. %as to be fulfilled in closed lenses. 
a) Stability says that the lens does nothing if nothing happens on the target side (no trigger--no action, hence, the name of the law) 

b) Putget requires the goal of update propagation to be achieved after the propagation act is finished. 
%\begin{remark}\label{rema:putget}%\zd{to be reworked}
%	The Putget law 
It may seem a notational trick rather than a law as operation:  $\putps^\req$  provides delta $u$, and functor $\get_{p'}$ sends it to a delta  $\get_{p'}(u)$ targeting at some model $S'_{p'}$ anyway. However, in general, there are many possible deltas between models $T'$ and $S'_{p'}$, whereas the Putget law states the existence of some special delta \frar{v^@}{T'}{S'_{p'}} such that equation (\putget) holds. %Note also that Putget implies commutativity of the lower triangle in the right back face as the upper one is commutative by Putget. %much more certainty about $T''$ and precisely specifies the relationship between $T'$ and $T''$, namely, it says that they are related by a specified update $\amex{v}$.

\shortlong{
c) Besides Stability and Putget, the MDE context for ala-lenses suggests other important laws, \eg, Hippocraticness described in the longer version \cite{me-act19-long}.
}{
c) Hippocraticness prohibits amending delta $v$ if consistency can be achieved for $v$ without amendment (hence, the name).  Note that neither equality $\putUL{\upd}{p,S}(v)=p$ nor $\putUL{\req}{p,S}(v)=u$ are required: the lens can improve consistency by changing $p$ and $u$ but changing $v$ is disallowed.  
}} % end \em; end long
\end{remark}

%==== the law pieces ends 
%=== Examples begin

\begin{example}[Identity lenses]\label{ex:idlens} %$\mathcal{id}$
	Any skeletal category \spA\ gives rise to an \alalens\ $\idl_\spA$ with the following components. The source and target spaces are equal to \spA, and the parameter space is \tcat\ (a category with a single object * and a single arrow $\id_*)$. Functor $\get_{*}$ is the identity functor and all puts are identities. Obviously, this lens is wb.
\end{example}
\begin{example}[Iso-lenses]\label{ex:isolens}
	Let \frar{\iota}{\spA}{\spB} be an isomorphism between model spaces. It gives rise to a wb \alalens\ \frar{\ell(\iota)}{\spA}{\spB} with $\spP^{\ell(\iota)}=\tcat$ as follows. Given any $A$ in \spA\ and \frar{v}{\iota(A)}{B'} in \spB, we define $\putl^{\ell(\iota).\req}_{*,A}(v) = \iota^{-1}(v)$ and the two other put operations send $v$ to identities. 
\end{example}
\begin{example}[Bx lenses]\label{ex:bxlens} Examples of SPg and wb aa-lenses modelling a Bx can be found in \cite{me-fase18}: they all can be considered as \alalens es with a trivial parameter space \tcat. 
\end{example}

\endinput 

\begin{example}[Learners: borrowed from \citefst\ but rearranged]\label{ex:mlasbx}
	Let \frar{\err(x,y)}{\Reals\timm\Reals}{\Reals} be a differentiable  {\em error} function such that \frar{\prtfrac{\err}{y}(x_0,y)}{\Reals}{\Reals} is invertible for any given $x_0$. For an $n$-dimensional Euclidean space $\reals^n$, we define the {\em total} error function \frar{\Err}{\reals^n}{\reals^n} by $\Err(a,a')=\sum_{i\le n}\err(a_i, a'_i)$. This converts space $\reals^n$ into a category (Lawvere's metric space) \brealsx{n}. 
	%
	A {\em \parrd\ function} from \realsx{m} to \realsx{n} is a differentiable function \frar{I}{\realsx{k}\timm\realsx{m}}{\realsx{n}} (and hence a functor \frar{I}{\brealsx{k}\timm\brealsx{m}}{\brealsx{n}}). 
	
	It is shown in \citefst\ that, given a {\em step size} $\eps\in(0,\infty)$,  any parameterized function \frar{I}{\realsx{k}\timm\realsx{m}}{\realsx{n}} gives rise to an ap-lens \frar{\ell_\eps(I)}{\brealsx{m}}{\brealsx{n}} called in \citefst\ a {\em learner}.%
	%\footnote{Warning: our models $S$ (for source) and $T'$ (target) are theirs $a$ and $b$ rather than $b'$.}
	\footnote{Moreover, they show the functoriality of the construction.} To make it an \alalens, we need to add amendments by defining $T^@=b'=I(p',a')$; then Putget trivially holds as there is only one arrow (distance/error) between any two objects. 
	
	%Any learner $\ell_\eps(I)$ can be made stable if we direct it to do nothing when $\Err(I(p,a),b)=0$. 
	Paper \citefjbx\ says that neither of the laws necessarily holds in the anarchic world of ML. % Putget nor Hippocraticness 
\end{example}

%==== the end of example




\endinput 




%In \citefst, Fong \etal\ prove that the category of codiscrete \alalenses is sm by showing that the required monoidal structure is borrowed from Cartesian sm-category $(\setcat, \times)$. We can do the same with \catcat\ instead of \setcat.




\endinput
We need to prove associativity: $(\ekk;\ell);\emm=\ekk;(\ell;\emm)$ for any three consecutive lenses 
\frar{\ekk}{\spA}{\spB}, \frar{\ell}{\spB}{\spC}, \frar{\emm}{\spC}{\spD} with \ekk\ and $\ell$ as shown in \figkl, and \emm\ having the parameter space \spR.   
We easily have associativity for the get part of the construction: $(\spP\timm\spQ)\timm\spR\cong\spP\timm(\spQ\timm\spR)$ (to be identified for equivalence classes), and $(\get^\ekk_p;\get^\ell_q);\get^\emm_r=\get^\ekk_p;(\get^\ell_q;\get^\emm_r)$.

\clearpage
Associativity of puts is more involved. 
Suppose that we extended the diagram in \figkl\ with lens \emm\ data on the right, \ie, with a triangle prism (say, purple) whose right face is a square $D_{pqr}D_{r'}D^@D'_r$ with diagonal \frar{\ome;\ome^@}{D_{pqr}}{D^@} where $r\in\spR$ is a parameter, $D_{pqr}=\get^\emm_r(C_{pq}$ and \frar{\ome}{D_{pqr}}{D'} is an arbitrary delta to be propagated to $\spP$ and \spA, and reflected as amendment $\ome^@=\putxyz{\emm.\self}{r}{C_{pq}}(\ome)$. 
We begin with rewriting \eqref{kldef2} by 
substituting the term for $v$ from \eqref{kldef1} 
\begin{eqnarray}\label{eqna:kldef2}
	% row 5
		\frar{w.\putl^{\klbr.\upd}_{pq,A} &= &%
		((w.\putxy{q}{B_p}^{\ell.\req}).\putxy{p}{A}^{\ekk.\upd}}{p}{p'})
	\paar (w.\putl^{\ell.\upd}_{q,B_p}{:}~q\rightarrow q') \label{eq:eqna4}
	\\
	\frar{w.\putl^{\klbr.\req}_{pq,A}&=&w.\putxy{q}{B}^{\ell.\req}.\putxy{p}{A}^{\ekk.\req}}{A}{A'}, \label{eq:eqna5}
	\\
	% \mbox{ and }
	\frar{w.\putl^{\klbr.\self}_{pq,A}&=&(w.\putl^{\ell.\self});(w.\putl^{\ell.\req}_{q,B}.%
		        \putl^{\ekk.\self}_{p,A}.\get^{\ell}_{q'})
	}{C'}{C^{@}}\rightarrow C^{@@} \label{eq:eqna6}
\end{eqnarray}
which shows the interplay between different puts. Now we do the same for the lens \klbr;\emm\ (recall that pairs $(x,y)$ can also be denoted by $x\paar y$. 
\begin{eqnarray}   %\label{eqna:klm-proof}
\ome.\putl^{\klbr;\emm.\upd}_{(pq)r,A}
&=& % row 7
(\ome.\putl^{\emm.\req}_{r,C}.\putl^{\kl.\upd}_{pq,A}{:}~pq\rightarrow p'q')
\paarrx{(a)}
 (\ome.\putl^{\emm.\upd}_{r,C}{:}~r\rightarrow r')
\mbox{~~~~~by \eqref{eqna4}}
\\ &=& % row 8
\left((\ome.\putl^{\emm.\req}_{r,C}.\putl^{\ell.\req}_{q,B}).\putl^{\ekk.\upd}_{p,A} %
\right)\paarrx{(a1)}\left(
\ome.\putl^{\emm.\req}_{r,C}.\putl^{\ell.\upd}_{q,B}
\paarrx{(a)} \ldots\right)
%\ome.\putl^{\emm.\upd}_{r,C} 
\mbox{~~by \eqref{eqna4}\paar\ same}
\\ &=& % row 9
\ome.\putl^{\lmbr.\req}_{qr,B}.\putl^{\ekk.\upd}_{p,A}
\paarr 
\ome.\putl^{\lmbr.\upd}_{qr,B}
\mbox{~~~~by \eqref{eqna5} \paarr\ by \eqref{eqna4}}
\\ &=& % row 10
\ome.\putl^{\ekk;\lmbr.\upd}_{p(qr),A}
\mbox{~~~~by \eqref{eqna4}}
\end{eqnarray}
Associativity of $\putl^{\ekk;\ell;\emm.\req}_{pqr,A}$ and $\putl^{\ekk;\ell;\emm.\self}_{pqr,A}$ can be proved in a similar manner (using sequential associativity rather than monoidal associativity above)  

\endinput


We also have %$w=\putxyz{\emm.\req}{}{}$
$w=\putxyz{\emm.\req}{r}{C_{pq}}(\ome)$ and 
$\frar{\eps=\putxyz{\emm.\upd}{r}{C_{pq}}(\ome)}{r}{r'}$. 
Then we extend the purple prism with the required fill-in arrows produced by functors $\get^\mu_r$ and $\get^\mu_{r'}$ as required. 



, \eg, the full diagonal on the right face will be %$\ome;\ome^@;\get^\mu_{r'}(w^{\ekk;\ell.@})=
$\ome;\ome^@; $



\endinput
In contrast to the general lens case, a wb a-lens features \lawname{\reflectzero} --- a sort of a self-Hippocratic law regulating the necessity of amendments: the latter is not allowed as soon as consistency can be restored without amendment. Another distinction is inclusion of an invertibility law \lawname{PutGet} into the definition of well-behavedness: 
 %due to historical traditions. %Subsequent results will also provide some justification for this. 
\lawname{PutGet}{} together with \lawname{Reflect2} provide (weak) invertibility: $\putl^B_\indb(\get(\putl^B_\indb(v)))=\putl^B_\indb(v)$.   
\lawname{Reflect3} is omitted as it is implied by \lawname{Reflect0} and \lawname{PutGet}.  

Any a-lens $\ebb^{\preccurlyeq} =(\spaA,\spaB,\get, \putl)$ gives rise to a binary symmetric lens $\ebb$. Its carrier consists of model spaces $\spaA$ and $\spT$, for which we assume $\Kupd$ and $\Kdisj{}$ to be defined such that the spaces are well-behaved, cf.\ Def.~\ref{def:wbspace}. The set of corrs of a pair $(A,B)\in \xob{\spS}\times \xob{\spT}$ is the singleton $\{\etosing{(A,B)}\}$ with $\prt_\spS\etosing{(A,B)}=A$ and $\prt_\spT\etosing{(A,B)}=B$, 
%the boundary mappings are the projections, 
\zdmodtok{realignment is thus trivial,}{}{ALIGH} and consistent corrs are exactly those \etosing{(A,B)}, for which $A = \get(B)$.

For a consistent corr $\etosing{B}={(\get(B), B)}$, we need to define six operations $\ebb.\ppghB_{\_\_}$. Below we will write the upper index as $B$ rather than $\hat B$ to ease the notation. For a  view update \frar{v}{A}{A'} and the corr \etosing{B}, we define 
 $$
\ppgB_{\spS\spT}(v)=\putl^B_\indb(v){:}\, B\to B'', \;
%
\ppgB_{\spS\spS}(v)=\putl^B_\inda(v){:}\, A'\to A'', \;
% \mbox{ and }
\ppgB_{\spS\star}(v)=\etosing{B''}
$$
 The condition $A''=\get(B'')$ for $\ebb^\preccurlyeq$ means that \etosing{B''} is again a consistent corr with the desired boundaries. For a base update \frar{u}{B}{B'} and the corr \etosing{B}, we define
$$\ppgB_{\spT\spS}(u)=\get(u),\;
\ppgB_{\spT\spT}(u)=\id_{B'},\; %and
\ppgB_{\spT\star}(u)=\etosing{B'}
$$ Functoriality of $\get$ yields consistency of $\widehat{B'}$.

\begin{defin}[Very well-behaved a-lenses] \label{def:putput_a}
		A wb a-lens is called {\em very well behaved (very wb)}, if the \corring\ binary symmetric lens is such.  %additionally fulfils \lawnamebr{PutPut}, 
		cf.  Def.~\ref{def:putput}.
Of course, this definition restricts the behaviour only for the $\putl$-part of the a-lens (hence the name of the law), since functor $\get$ is compositional anyway. \qed
\end{defin}

\begin{lemma}\label{lemma:asymm_symm} Let $\ebb^\preccurlyeq$ be a (very) wb a-lens and $\ebb$ the corresponding symmetric lens. Then all base updates of $\ebb$ are closed, and $\ebb$ is (very) wb and invertible. 
 \end{lemma}
 \begin{proof}
 Base updates are closed by the definition of $\ppg_{\spT\spT}$. Well-behavedness follows from wb-ness of $\ebb^\preccurlyeq$. Invertibility has to be proved in two directions: $\ppg_{\spaB\spaA};\ppg_{\spaA\spaB};\ppg_{\spaB\spaA} = \ppg_{\spaB\spaA}$ follows from \lawnamebr{PutGet}{} and \lawnamebr{Reflect0}, the other direction follows from \lawnamebr{PutGet}{} and \lawnamebr{Reflect2}, see the remark after Def.\ref{def:wbalens}. The ''vwb''-implication follows directly from Def.\ref{def:putput_a}. 
 \qed
 \end{proof}
\begin{remark}[A-lenses as view transformation engines]\newpii{
	In terms of Varr\'o et al \cite{dvarro-models18}, a wb a-lens can be seen as an abstract algebraic model of a bidirectional view transformation engine. This engine is assumed to be a) consistent: it is a basic lens law that propagation must always produce a consistent corr, b) incremental, as lenses propagate changes rather than create the target models from scratch, c) validating, as the result of propagation is always assumed to satisfy the target metamodel constraints (either by considering the entire model space to be only populated by valid models, or by introducing a subclass of valid models and require the result of the propagation to get into that subclass). Reactiveness, \ie, whether the engine executes on-demand or in response to changes, is beyond the lens \fwk. To address this and similar concerns, we need a richer \fwk\ of lenses augmented with organizational structure introduced in \cite{me-jss15,me-grand17}. }{1}{-15em}
\end{remark}

  \begin{theorem}[Lenses from Spans]\label{thm:LensesFromSpans} An $n$-ary span of (very) wb asymmetric lenses $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$, $i=1..n$ with a common base \spaB\ of all $\ebb_i^{\preccurlyeq}$ gives rise to a (very) wb symmetric lens denoted by $\Sigma_{i=1.. n}^\spT\ebb_i^{\preccurlyeq}$. 
\end{theorem}
\begin{proof}
An $n$-ary span of a-lenses $\ebb_i^{\preccurlyeq}$ (all of them interpreted as symmetric lenses $\ebb_i$ as explained above) is a construct equivalent to the star-composition of Def.~\ref{def:star-comp}.3, in which lens $\ekk=\idlensnb$ (cf. Ex.~\ref{ex:idLens}) and peripheral lenses are lenses $\ebb_i$. The junction condition is satisfied as all base updates are $\ebb_i$-closed for all $i$ by Lemma \ref{lemma:asymm_symm}, and also trivially closed for any identity lens. The theorem thus follows from Theorem~\ref{th:star-comp}. The ``very wb''-part follows directly from Def.~\ref{def:putput_a}. Note that a corr in $\Corrx{\Sigma_{i=1.. n}^\spT\ebb_i^{\preccurlyeq}}$ 
 is nothing but a single model $B\in\xob{\spaB}$ with boundaries being the respective $\get_i$-images.
\end{proof}
The theorem shows that combining a-lenses in this way yields an $n$-ary symmetric lens, whose properties can automatically be inferred from the binary a-lenses.
\input{figures/pdfs/mergedMetamultimod-uml}

\exIntro. Figure~\ref{fig:mergedMetamod-uml} shows a metamodel $M^+$ obtained by merging the three metamodels $M_{1,2,3}$ from \figri\ without loss and duplication of information. In addition, for persons and companies, the identifiers of their  original model spaces can be traced back via attribute ''spaces'' 
(\Commute-objects are known to appear in space $\spS_3$ and hence do not need such an attribute). As shown in \cite{me-ecmfa17}, any consistent multimodel $(A_1...A_n, R)$ can be merged into a comprehensive model $A^+$ instantiating $M^+$. Let 
$\spT$ be the space of such together with their comprehensive updates \frar{u^+}{A^+}{A'^+}. 

For a given $i\le 3$, we can define the following a-lens $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$:
$\get_i$ takes update $u^+$ as above and outputs its restriction to the model containing only objects recorded in space $\spS_i$. Operation $\putl_i$ takes an update \frar{v_i}{A_i}{A'_i} and first propagates it to all directions as discussed in \sectref{sec:example}, then merges these propagated local updates into a comprehensive  \spaB-update between comprehensive models. This yields a span of a-lenses that implements the same \syncon\ behaviour as the symmetric lens discussed in \sectref{sec:example}.

\noindent {\em\bf  From (symmetric) lenses to spans of a-lenses.} There is also a backward transformation of (symmetric) lenses to spans of a-lenses. Let $\ell=(\mspaA, \ppg)$ be a (very) wb lens. It gives rise to the following span of (very) wb a-lenses $\ell_i^\preccurlyeq=(\prtbf_i(\mspaA),\spaB,\get_i, \putl_i)$   
where space $\spaB$ has objects $(A_1\ldots A_n,R)$ with $R\in \Corrx{A_1...A_n}$ a consistent corr, and arrows are the update tuples of $\mspA$. Functors $\get_i:\spaB\to \spaA_i$ are projection functors. Given $B = (\tupleAWOB, R)$ and local update \frar{u_i}{A_i}{A'_i}, let

%\noindent 
\frar{\putl^B_{i\indb}(u_i)\eqdef(u_1',..,u'_{i-1}, (u_i;u_i'), u'_{i+1},..,u_n')}
{(A_1... A_n,R)}{(A''_1... A''_n,R'')}
\\[1ex] 
where $u_j' \eqdef \ppg^R_{ij}(u_i)$ (all $j$) and $R'' = \ppg_{i\star}^R(u_i)$. Finally, $\putl^B_{i\inda}(v_i)\eqdef\ppg^R_{ii}(v_i)$, \ie, 
$v_i^{@B}=v_i^{@R}$. 
Validity of \zdmodtok{\lawname{Hippocr1-2}}{\lawname{Stability}}{}, \lawname{Reflect0-2}, \lawname{PutGet} and \kputputlaw\ directly follows from the above definitions. This yields 
\begin{theorem}\label{theo:lens2span}
Let $\ell = (\mspA, \ppg)$ be a (very) wb symmetric lens. Then the multi-span 
\[(\ell_i^\preccurlyeq=(\prtbf_i(\mspaA),\spaB,\get_i, \putl_i) \mid i=1..n)\]
of (very) wb a-lenses (where \spT\ is defined as specified above) has the same synchronization behaviour w.r.t.\ model spaces $(\prtbf_i(\mspaA)\mid i=1..n)$.  
\qed
\end{theorem}

\newpii{
An open question is whether the span-to-lens transformation in Thm.\ref{thm:LensesFromSpans} and the lens-to-span transformation of Thm.~\ref{theo:lens2span} are mutually inverse. It is easy to see that the chain 
\begin{equation}\label{eq:lens2span2lens}
\mbox{symmetric lens $\rightarrow$ wide span $\rightarrow$ symmetric lens} 
\end{equation}
results in a lens isomorphic to the initial one, but the chain 
\begin{equation}
\mbox{wide span $\rightarrow$ symmetric lens $\rightarrow$ wide span} 
\end{equation}
ends with a different span as the first transformation above loses information about updates in the head of the span. 
 The results for the binary case in \cite{jr-jot17} show that the two spans can only be shown to be equivalent modulo certain equivalence relation, and an equivalence relation between lenses is also needed to tune all constructs into harmony. These equivalences may be different for our multiary lenses with amendments, and we leave this important question for future research.  
}{1}{-17em}
 \endinput
 
%============= Old Version ========= 
 \begin{theorem}[Lenses from Spans]\label{thm:LensesFromSpans} An $n$-ary span of wb a-lenses $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$, $i=1..n$ (note the common base \spaB\ of all $\ebb_i$) gives rise to a wb  (symmetric) lens $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$.
% 	
  	Moreover, $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$ is invertible as soon as the span satisfies the following condition%
 	\footnote{Found for the binary case by Bob Rosebrugh \cite{bob-invert}}: 
% 	$$
% 	\putl^B_{\indb i}
% 	$$
$\PP^B_i=\PP^B_j$ for all $B\in\xob{\spaB}$ and $i,j\le n$, where for given $B$ and $i$,  $\PP^B_i$ is the inverse image of 
$\xarr{\spaB}(\get_i(B),\_)$, \ie,  the set $\compr{\putl^B_{\indb i}(v_i)}{\frar{v_i}{\get_i(B)}{\_}}$. %, then $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$ is invertible.
\end{theorem}
\shortlong{}{%}
\begin{proof}
An $n$-ary span of a-lenses $\ebb_i^{\preccurlyeq}$ (all of them interpreted as symmetric lenses $\ebb_i$ as explained above) is a construct equivalent%
\footnote{To make it precise, we need to introduce a simple notion of lens equivalence, which identify lenses with the same propagation behaviour but, perhaps, different sets of corrs -- see. \eg, \cite{jr-jot17}} to the star-composition of Def.~\ref{def:star-comp}, in which lens $\ekk=\idlensna$ and peripheral lenses are lenses $\ebb_i$. The junction condition is satisfied as all base updates are $\ebb_i$-closed for all $i$ by Lemma \ref{lemma:asymm_symm}, and also trivially closed for any identity lens. The theorem thus follows from Theorem~\ref{th:star-comp}. Note that a corr in $\xstar{(\Sigma_{i=1}^n\ebb_i^{\preccurlyeq})}$ 
 is nothing but a single model $B\in\xob{\spaB}$ with boundaries the respective $\get_i$-images. \qed
 \end{proof} 
}
For the backward transformation of lenses to spans of a-lenses, we use our observation in footnote~\ref{ft:mspa-as-cat} on p.~\pageref{ft:mspa-as-cat}.
\begin{theorem}[Spans from lenses] \label{th:lens2span}Any {(not necessarily invertible) }wb lens $\ell=(\mspaA, \ppg)$ gives rise to a span of wb a-lenses $\ell_i^\preccurlyeq=(\spaA_i,\spaB,\get_i, \putl_i)$. \\
%{\color{red}We should say already here, how $\ell$ is related to the resulting construction of Thm \ref{thm:LensesFromSpans} for $\ell_i^\preccurlyeq$, see below}
\end{theorem}
\shortlong{}{%}
\begin{proof} Let $\mspA$ have model spaces $\spaA_i$ and corr set $\R$ with corresponding boundary functions $\partial_i$. Let 
\[\spaB = \{(A_1, \ldots, A_n, R)\mid \partial_i(R) = A_i \mbox{ for all }i\}\] 
be the set of all aligned consistent multimodels and $\get_i:\spaB\to \spaA_i$ be projections, \ie\ $\get_i(A_1, \ldots, A_n, R)= A_i$ and $\get_i(u_1, \ldots, u_n)= u_i$\footnote{
Recall the definition of multimodel updates in Def.\ref{def:multispace}: There is no update component for $R$ 
}. Given $B = (A_1, \ldots, A_n, R)$ and update \frar{u_i}{A_i}{A'_i}, we define
\[\putl^B_{i\indb}(u_i)=(u_1', \ldots, u'_{i-1}, u_i;u_i', u'_{i+1} \ldots, u_n'): (A_1, \ldots, A_n, R)\to (A_1'', \ldots, A_n'', R''),\]
where $u_j' \eqdef \ppg^R_{ij}(u_i)$ for all $j$, $R'' = \ppg_{i\star}^R(u_i)$ and $\putl^B_{i\inda}(v_i)=\ppg^R_{ii}(u_i)$. 

That well-behavedness carries over from $\ell$ to the a-lenses is an direct consequence of the respective definitions. 
 \qed
\end{proof} 
}
%An important issue is how the two transformations, lenses to spans and spans to lenses, interact. To manage this, we need an $n$-ary counterpart of the theory of lens equivalence developed by Johnson and Rosebrugh in \cite{jr-jot17} for the binary case.  We leave it for future work. 
It is easy to see that $\Sigma_{i\in I_\ell}\ell_i^\preccurlyeq = \ell$ for any lens $\ell$, but if we begin with a span of a-lenses $\ebb_i$, $i\in I$ build a lens $\Sigma_{i\in I}\ebb_i$ and then build the span $(\Sigma_{i\in I}\ebb_i)^\preccurlyeq_i$, the two spans are different. This difference could disappear with a suitable notion of span equivalence, which we conjecture should be a straightforward generalization of the equivalence developed by Johnson and Rosebrugh in \cite{jr-jot17} for the binary case.  %which we think should be generalizable for the $n$-ary case. We leave it for future work. 
%
%\begin{example}
%Running
%\end{example}

\endinput
\begin{theorem}[Sequential composition]
	Let \lensar{\aekk}{\spaA}{\spaB} and  \lensar{\aell}{\spaB}{\spaC} be two wb a-lenses satisfying the following {\em junction condition}: all updates in $\spaB$ obtained by $\ekk$-propagation from \spaA\ are $\ell$-closed. Then there is a uniquely defined wb a-lens \lensar{\aekk;\aell}{\spaA}{\spaC}. %The composition is associative with identity lenses \lensar{\ell_{\id_{\spaB}}}{\spaB}{\spaB} being its units. 
\end{theorem}
 \input{figures/diags/seq-comp} 
 \textit{Proof.} Obviously, composition of \Kupd-preserving functors  
\flar{\get^\ekk}{\spaA}{\spaB} and \flar{\get^\ell}{\spaB}{\spaC} is a \Kupd-preserving functor: $\get^{\ekk;\ell}=\get^\ekk\circ\get^\ell$. Now we define $\putl^{\ekk;\ell}$. 
Let $u$ be an update as shown in \figref{fig:seq-comp} where horizontal lines are \get-corrs. Let $v=\putl^{\ekk B}_\indb(u)$, $u'=\putl^{\ekk B}_\inda(u)$, and $w=\putl^{\ell C}_\indb(v)$ (by the junction condition $v'=\id_{B''}$).  
%Finally, $u^*{=}\,\get^\ekk(v')$.  
Define $\putl^{C~\ekk;\ell}_\indb(u)=w$ and $\putl^{C~\ekk;\ell}_\inda(u)=u'$. Laws \lawname{Reflect1,2, 3} for $\ell;\ekk$ are obvious. %To prove idempotency \lawname{Reflect2}, we note that as $(v, v')\in\Kupd{B''}$ by $\ell.\lawname{Reflect}$, $u''\Kupd_{A''}u^*$ as $u''=u;u'=\get^\ekk(v)$ owing to $\Kupd$-preservation by $\get^\ekk$. Hence, by $\ekk.\lawname{PutPut}$, $\pult^{B \ekk}(u'';u^*)=\putl(u'');\putl(u^*)$
Stability and Putput are obvious too. 



==> ll-sections/back-act2foss.tex <==
\subsection{Background}\label{sec:back}
Connections between learners and lenses appear much less surprising in the light of the Mealy machine view of lenses: a lens can  be understood as a couple of two Mealy machines working over the same space in the opposite directions (if the lens is asymmetric, one machine is stateless while the other is stateful, and for symmetric lenses, both machines are stateful). In this sense, learners are just lenses whose states are enriched with parameters (we will call the procedure {\em parameterization}) so that a state update includes a parameter update. This enrichment has a clear practical sense for Bx. Indeed, classical (non-enriched) \bx\ lenses specify \syncon\ of a pair of models $(A,B)$ connected by a transformation, say, $F(A)=B$.%
\footnote{Think, \eg, of $A$ as a UML model and $B$ as a Java program generated from it, or $A$ may be a Java program and $B$ is its bytecode, or $A$ can be an object model and $B$ is its relational storage, see \cite{me-jss15} for a variety of such examples.} If the target model $B$ is updated to $B'$ and consistency between the two sides is violated, the lens ``sitting'' over $F$ 
prescribes how the source model $A$ is to be updated to $A'$ such that $F(A')=B'$ and consistency is restored. (In the \bx\ jargon, one also says that the change \sqarr{B}{B'} is propagated to \sqarr{A}{A'}.) Now the learning lens idea allows us in search of consistency restoration to update the very transformation too so that the final result is $F'(A')=B'$. To  manage the extended search possibiities, it makes sense to parameterize the space of transformations to be searched as a family of mappings \frar{F_p}{\spA}{\spB} (with bold letters denoting spaces of $A$s and $B$s resp.)  indexed over some parameter space $p\in\spP$. Then we have two interrelated propagation  operations: backpropagation that maps \sqarr{B}{B'} to \sqarr{A}{A'} and update mapping \sqarr{B}{B'} to \sqarr{p}{p'} (update).  Formally, this is exactly the ML setting considered above up to the currying/uncurring equivalence (but note that $b$ is now written as an updated artifact and hence primed). The possibility to update the transformation appears to be so natural in so many \bx\ contexts (indeed, designing and debugging a model \trafon\ is well-known to be challenging, \eg, see \citemtbe) that we perhaps should be more puzzled by why the ``surprising links'' between learning and \bx\ were not discovered much earlier. 

\newcommand\john{\enma{\mathsf{John}}}
\newcommand\jon{\enma{\mathsf{Jon}}}
\newcommand\mary{\enma{\mathsf{Mary}}}

Thus, porting the learning idea into the \bxmde\ \fwk\ appears to be theoretically reasonable and practically useful. There is, however, a challenge to manage. For learners, a change \sqarr{b}{b'} is just  a pair $(b,b')$, while in \bxmde, the situation is different. \Bx-lenses first appeared in the work on file \syncon, and if we have two sets of strings, say, $B=\{\john, \mary\}$ and $B'=\{\jon, \mary\}$, we can readily see the difference: $\john\noteq\jon$ and $\mary=\mary$. There is a structure in-between $B$ and $B'$ (that maybe rather complex for big files), but this structure can be recovered by matching (the same in ML) and thus updates can be identified with pairs. (This is exactly the procedure that converts any set into a co-discrete category, hence the name {\em codiscrete} for lenses propagating such updates.) The situation dramatically changes if $B$ and $B'$ are object structures, \eg, $B=\{o_1, o_2\}$ with $\name(o_1)=\john$, $\name(o_2)=\mary$ and similarly  $B'=\{o'_1, o'_2\}$ with $\name(o'_1)=\jon$, $\name(o'_2)=\mary$. Now string matching does not say too much: it may happen that $o_1$ and $o'_1$ are the same (think of as typo in the dataset), while $o_2$ and $o'_2$ are different (although have the same name). Of course, for better matching we could use full names or ID numbers or something similar (called, in the database parlance, primary keys) but absolutely reliable keys are rare, and typos and bugs can compromise them anyway. Thus, for object structures that \bxmde\ needs to keep in sync, changes or updates, or {\em deltas} need to be independently specified. For example, a relational delta $u\subset B\timm B"$ with $u=\{o_1, o_1'\}$ unambiguously says that $\john@B$ and $\jon@B'$ are the same person while $\mary@B$ and $\mary@B'$ are not. Hence, model spaces in \bxmde\ are categories (objects are models and arrows are update/delta specifications) rather than sets (codiscrete categories). The transition from codiscrete lenses to delta-based lenses originated in \cite{me-jot11} was not unclouded and seamless, but after delta lenses were implemented with triple graph grammars (TGG) \citedlenstgg, they are gaining more attention in both industry and academia. 



\endinput
Indeed, lenses are devices specifying change propagation, and learning can be seen as a special change propagation case. For example, given (i) sets $A, B, P$ and  a family of functions 
$f=\comprfam{p\in P}{\frar{f_p}{A}{B}}$ as the learning space, and (ii) a training datum $(a,b')$ with $b'\noteq b=f_p(a)$ for an initially given parameter value $p$, we can interpret it as a change from a consistent state of the system $(a,p,b)$ to an inconsistent state $(a,p,b')$ caused by the change \warrbb. \Bx would fix this inconsistency by changing the input data \warraa\ so that the state $(a',p,b')$ is consistent, \ie, $f_p(a')=b'$; this action is often described as {\em propagating} change \warrbb\ to change \warraa. ML would call the original change \warrbb\ an error, and fix it by changing the parameter value \warrpp\ so that the state $(a,p',b')$ is either consistent, 
%\ie, $f_{p'}(a)=b'$, 
or at least less inconsistent than $(a,p,b')$ w.r.t. some metrics, \eg, we can add  metrics to set $B$ and require that $||f_{p'}(a), b'|| < ||f_p(a),b'||$. In ML terms, the system has {\em learnt} a better approximation $f_{p'}$ of the function; in \Bx terms, change \warrbb\ is propagated to \warrpp.  


Abstract learners defined in \citefst\ do both propagations so that the updated/learnt state is $(a',p',b')$. The story is schematically described in the inset figure, in which the horizontal dashed arrow shows ML's evolution towards having back propagation (Bp) and the vertical arrow shows \bx's evolution towards \Bx with learning (\bxl, still to be developed; the work on deriving model transformations from examples \citemtex\ can be seen as \bxl). In the lens \fwk\ developed for \bx, point (1,1) corresponds to the idea of a learning lens, % defined in the present paper, 
which covers both ML and \bx. In the paper, %the notion of a learning lens allows us to work
we will work with asymmetric rather than symmetric learning lenses, which is a) technically much simpler and b) conceptually justified: compositional ML considered in \citefst\ is about composing functions rather than relations, and an asymmetric model seems to be more appropriate.  The main result of \citefjbx\ can then be seen as an ``internal lens business'': it says that any codiscrete al-lens can be encoded by a special symmetric non-learning lens. In the present paper, a lens always means an asymmetric lens.
% == nice piece !
%As asymmetric lenses are simpler than symmetric, and ordinary lenses are simpler than learning lenses, this results says that we can trade asymmetry for unparameterization, which is unexpected and nice, but can be encapsulated as an internal lens business not immediately related to interactions between ML and BX (of course, such observations are much easier to make after connections between ML and lenses were noticed in \citefjbx). 

Thus, the notion  of a codiscrete al-lens was actually discovered in \citefst.  The present paper makes three contributions to the learning lens idea consecutively described in three subsections below, after which we outline the structure of the rest of the paper. 


==> ll-sections/backgr-new.tex <==
\section{Overview of delta lenses with amendment and their compositionality%Background: \bx\ world of model spaces and delta lenses
}\label{sec:backgr}

%\input{ll-figures/diags/bxmlPut}

\renewcommand\figri{\figref{bxmlPut}}
\subsection{Background: \bx\ world of model spaces and delta lenses}
In the (delta-based) \bx, the counterpart of values in Euclidean spaces dealt with in ML are complex artifacts called \bfem{models}. They can be seen as models of logical theories (of the first- or even higher-order) called \bfem{metamodels}. A typical way of specifying metamodels is to use graphs and constraints; in fact, metamodels can be seen as Makkai's generalized sketches \citemakkai, see also \cite{me-entcs08} for definitions and discussion in the MDE context. For our current discussion, it's enough to think about models as graphs with some (unspecified) extra structure, which behaves well enough to ensure the required categorical properties (the reader can think about {\em attributed typed graphs} as defined in \cite{ehrig-book06}); we will call them 'graphs'. In MDE applications, it normally does not make sense to distinguish isomorphic 'graphs' (indeed, objects identifiers are invisible) and thus we identify models with isomorphisms  classes of 'graphs' and assume categories of models to be strongly skeletal: the only isomorphisms are identity loops.  

Let \spG\ be a category of 'graphs'/models, $G, G'\in |\spG|$ are two objects, and \wrar{\tilde u}{G}{G'} is some informal notion of a model update (delta, change). We can formalize it by a span of monics $u=(G\lTo^i O\rTo^{i'} G')$ whose head $O$ specifies what part of $G$ is preserved in $G'$ so that the elements of $G$ beyond the image $i(O)$ are deleted, and the elements of $G'$ beyond $i'(O)$ are added during the update. % \frar{u}{G}{G'}.  
We assume that \spG\ has pullbacks so that spans are composable (and produce spans of monics), and we obtain a strongly skeletal category $\Span_{\mathsf{mon}}(\spG)$, %  (recall that \spG\ is skeletal and hence \Span(\spG) is a category rather than a bicategory), 
whose arrows are called \bfem{updates} or \bfem{deltas}. %Another way to specify informal updates $\tilde u$ is to use edit sequences describing what should be done with model $G$ to obtain model $G'$ step-by-step; such sequences are associatively composable and also produce a category (see, \eg, \citeeditlenses). 
The delta lens \fwk\ abstracts away these details and simply identifies model spaces with strongly skeletal categories and forward \trafon s between model spaces with functors; the latter are usually called \bfem{get functors}  or just \bfem{get}s (read `` get the view''): a detailed discussion and examples can be found in \cite{me-jot11}.%
\footnote{Not all useful \trafon s are functors, but many are, and it is a standard assumption in the delta lens \fwk.} 

Now we will schematically discuss how \alalens es work (and then will relate them to the ML setting in \citefst). %; precise definitions will be given in Sect.3. 
While an ordinary asymmetric  lens ``inverts'' a given functor \frar{\get}{\spA}{\spB} between model spaces, an \alalens\ ``inverts''  {\bf\em and} ``learns'' over a family of get functors \frar{\get_p}{\spA}{\spB} with $p$ being a parameter from a set $P$. We will actually consider a more general case with the parameter space also being a small category \spP, and the get family being a functor \frar{\get}{\spP}{[\spA, \spB]} into the category of functors from \spA\ to \spB\ and their natural transformations. %  (later we will consider a small category of parameters \spP\ whose set of objects is $P$). 
This implies that for \frar{e}{p}{p'} in \spP, and any two objects $A,A' \in \spA$, there is a mapping \frar{\get_e}{\spA(A,A')}{\spB(A.\get_p, A'.\get_{p'})} provided by the naturality of transformation $\get(e)$ (in the next section we will consider this in detail). 
We describe the data above in the top row of diagram \figri a, which provides the  ``types'' of the story, while the story itself is unravelled on the level of instances shown by the rectangular diagram below.   

Suppose given a model $A\in\spA$ and its view, model $A.\get_p= B \in\spB$, so that the state $(A,p,B)$ is consistent. 
Note our notation for the fact $A.\get_p=B$: bulleted arrows $x \rMapsto y$ don't have an internal structure and just visualize pairs $(x,y)$ --- the UML calls them {\em links}. The label over link $(A,B)$ in \figri(a) says that the link is an instance of function $\get_p$ (note the colon symbol), in more detail, this instance is fully determined by object $A$: it is the result of executing function  $\get_p$ at object $A$.%
\footnote{\label{fnote:storywithdefs} In a fuller version of the story with the type side explicitly given by a category \defcat\ of metamodels and \trafon\ definitions, over which a category of models is fibred,  link $(A,B)$ would be the Cartesian lifting of \trafon\ definition \flar{\niget_p}{\nim}{\nin} at object $A$ living in fibre \spA\ over metamodel \nim, and arriving at $B$ in the fibre \spB\ over \nin. Although the syntactical side is important for applications, lenses traditionally ignore it and we follow this style in the paper. 
}

\input{ll-figures/diags/bxmlPut}
Now suppose that $B$ is updated to $B'$ with delta (update) $\vii\in\spB(B,B')$ as shown. 
%We use numeric indexes for elements of the diagram to additionally convey the order of operations producing them, \eg, 1 means that production of link 1 by operation $\get_p$ is the first step of the story, and update $\vii$ is the second step. There is no intention to make this notation fully consistent (the more so formal); it is a syntactic sugar with some semantic connotations useful for reading complex diagrams further in the paper. %
%=== important remark for future thought
%\footnote{ 
%In the operational setting for updates (like in edit lenses), we would have a (partially defined) \trafon\ \frar{\vbf}{\spB}{\spB} so that update $\vii$ would be an instance of \vbf\ denoted by $2{:}\vbf$, but in the delta lens version used in this paper, vertical arrows are....}
In the asymmetric lens setting, any change of view $B$ destroys consistency (it's not so for the symmetric version of lenses), and an \alalens\ restores it by calling an operation \putl\ which a) changes the parameter with delta/update \frar{e}{p}{p'} (where $e$ refers to the {\em evolution} of the get), %from $p$ to $p'$, 
b) changes the source model $A$ with update \uiii,  and c) amends the update-violator $v$ with an {\em amendment} update $v^@$  so that the result of these changes is a consistent system $A'.\get_{p'}=B'^@$ as shown in the diagram (note the dashed arrows and index $p'$ near the bottom arrow). Thus, \putl\ is a triple of operations $(\putl^\upd, \putl^\req, \putl^\self)$, which for a given pair $(A,v)$ return a corresponding triple of updates \frar{e=\putl^\upd(A,v)}{p}{p'} (not shown in the diagram), \frar{u=\putl^\req(A,v)}{A}{A'}, \frar{v^@=\putl^\self(A,v)}{B'}{B'^@}; the superscripts \upd, \req\ abbreviate the corresponding names used in \citefst.   
%$u$, $v^@$.%and $\putl^\self$ that given $(A,v)$ 
%\footnote{Actually we will define even more categorical version in which the parameter space \spP\ is also a category and $\putl^\upd$ returns a parameter update \frar{e}{p}{p'}.}

Moreover, to ensure that operations \putl\ really invert functors \get, we require a much stronger consistency condition to hold:  %. Given  \frar{e}{p}{p'}, for any two objects $A,A' \in \spA$, there is a mapping \frar{\get_e}{\spA(A,A')}{\spB(A.\get_p, A'.\get_{p'})} provided by the naturality of transformation $\get(e)$ (in the next section we will consider this in detail). Now, 
for any $v$ as above, we require the equality $u.\get_{e}= v;v^@$ between updates---because it is update/delta $v;v^@$ that gives model $B'^@$ its real meaning in a typical MDE scenario.  
In the lens parlance, the last equation and its versions are called the Putget law: if we substitute $\putl(v)$ for $u$, we obtain equality $(\putl.v).\get_{p'} =v;v^@$ to hold for any $v$, hence, the name of the law. Another important law is {\em Stability}: if $v=\id_B$, then all three deltas, $e,u,v^@$ are also identities. A lens satisfying Stablity and Putget laws is called an {\em SP-alaLens}. 

Thus, an (SP) ala-lens is a pair $\ell=(\get,\putl)$ specified above, and we will write it as an arrow $\ell=(\get,\putl){:}\, \spA\stackrel{\spP}{\longrightarrow}\spB$ or just \frar{\ell=(\get,\putl)}{\spA}{\spB} keeping the parameter space \spP\ implicit. In the next section, we will show that SP-lenses can be composed sequentially and in parallel, and form an sm-category $\alalenscat$. 

An ala-lens \frar{\ell}{\spA}{\spB} is called {\em (elementarily) codiscrete} if all categories $\spA,\spP, \spB$ are codiscrete (below we will also consider non-elementarily codiscrete lenses). The full subcategory of (SP) codiscrete lenses will be denoted by $\alalenscat_0$ (and we have a full embedding $\alalenscat_0\rFEmb\alalenscat$).  

\subsection{Learners in the delta lens setting, I}

Diagram \figri(b) shows a specialization of the general ala-lens scenario in \figri(a) for ML-learners as defined in \citefst. Euclidean spaces are turned into categories whose arrows are differences: for any pair of tuples $a,a'\in\reals^m$, we have their componentwise difference $\del=(\del_i)_{i\le m}$, $\del_i=a'_i-a_i$, considered as an arrow \frar{\del}{a}{a'}.  Composition and identity are obvious, and any function \frar{f}{\reals^m}{\reals^n} gives rise to a functor \frar{\pmb f}{\rcat^m}{\rcat^n}.%
\footnote{A more refined model would be to consider monoids of differences as acting on values, say, monoid $\reals^m$ acts on $\reals^m$ so that given a value $a\in\reals^m$ and a difference (\textit{edit}, in the lens parlance) $\del\in\reals^m$, we compute $a'=a\odot\del$ where action $\odot$ is given by summation: $a\odot\del :=a+\del$. Thus, we have a monoid $\DDel^m=(\reals^m,+,0)$ that acts on $\reals^m$ by  \frar{\odot}{\DDel^m\timm\reals^m}{\reals^m}, and if function\frar{f}{\reals^m}{\reals^n} is differentiable, then its Jacobian matrix at point  $a$ can be seen as a monoid morphism \frar{\jacobf_a}{\DDel^m}{\DDel^n} so that for sufficiently small deltas, $f(a\odot\del)\approx f(a)\odot\jacobf_a(\del)$. Then functoriality of $f$ is based on its differentiability. We consider this model in more detail in \sectref{?}.
}
 The notation in diagram \figri(b) is borrowed from \citefst\ to ease seeing the parallelism (but note a discrepancy: $B'$ in \figri(a) corresponds to $b$  without prime in \figri(b)). Also note that for defining \putl, a special metrics is used: first, a differentiable error function \frar{\err}{\reals\timm\reals}{\reals} is defined, and then the total error is given by summation, $E_I(p,a,b):=\sum_{j\le n}\err(I_j(p,a), b_j)$ (see \citefst) so that $E_I(p,a,b)$ is a function of $\del_I(p,a,b)$ seen as an arrow. Finally, we can define update arrows using the gradient descent idea: \frar{\dellp}{p}{p'} with $\dellp=-\eps\nabla_p E_I(p,a,b)$ and \frar{\della}{a}{a'} with $\della=-\eps\nabla_a E_I(p,a,b)$ (of course, we can use different step sizes \eps\ for \dellp\ and \della).%
 \footnote{In \citefst, they define \della\ differently. First, function \frar{\prt_x\err(x_0,\_)}{\reals}{\reals} is considered invertible for all $x_0$, and let \flar{\rre_{x_0}}{\reals}{\reals} be its inverse (symbol \rre\ is the inversely read \err). Then for an $a\in\reals^m$, we have \flar{\rre_a}{\reals^m}{\reals^m}. Now  $\della$ can be defined as $\rre_a(\nabla_a E_I(p,a,b))$.} 
 Amendment is defined by differencing $\del^@=I(p',a')-b$. It easy to see that if $\del=0=\id_{I(p,a)}$, then $E_I(p,a,b)=0$ achieves its minimum and thus  $\dellp=\della=\del^@=0$ as well so that Stability holds. The Putget law trivially holds due to the definition of $\del^@$. Thus, learning based on the gradient descent gives us an SP-alaLens. 
 
 
\clearpage
 \subsection{Functoriality of update policies}
  \renewcommand\figrii{\figref{funofput}}
 \input{ll-figures/diags/funofput}
 The diagram in \figrii\ illustrates compositionality of operations \get\ (trivial) and \putl\ (non-trivial) (nodes $\circ$ denote objects without names). Given a sequence of parameterized functors \frar{\get^i_{p_i}}{\spA_i}{\spA_{i+1}}, $p_i\in\spP_i$, $i\le n$ ($n=3$ in the diagram), it is easy to define their composition \frar{\get_p}{\spA_1}{\spA_n} for $p=(p_1...p_n)\in\spP{=}\spP_1\timm\ldots\timm\spP_n$ as $A.\get_p=(...(A.\get^1_{p_1}).\;\ldots\;).\get^n_{p_n}$, and show that it is associative (when functors are considered up to a suitable equivalence). Composition of $\putl^i$, $i\le n$ is more interesting: the diagram shows a simple projection of story, in which  arrows \frar{e_i{=}\putl^{i\,\upd}}{p_i}{p'_i} are not shown. Triple-arrow symbols $j{:}\putl^i$ denote three consecutive applications ($j=1,2,3$) of operations $\putl^i$. Double-arrows labelled $j{:}\get^i_{e_i}$ denote application of the corresponding \get-functors to arrows to demonstrate that the Putget law holds. 
 
 
 A pair $\ell_i=(\get^i,\putl^i)$ is an ala-lens \frar{\ell_i}{\spA_i}{\spA_{i+1}}, and the construction shown in the figure defines lens composition \frar{\ell_1;\ell_2;\ell_3}{A_1}{A_4} (in \sectref{alalenscat} it will be formally defined). %, we will prove that ala-lenses make an sm-category. 
 However, it's not the end of the story developed in \citefst. 
 %
 So far, in the lens formalism as such, two components of a lens $\ell=(\get, \putl)$ are considered given independently (although their interaction is regulated by lens laws ensuring a weaker or stronger sense of \putl\ being an inverse to \get ) while in practice of both BX and ML, the \putl-component is built based on the \get-component. As there are many ways of inverting a {\bf general} functor, finding reasonable single-valued operation \putl\ (a so called {\em update policy})  is normally based on the {\bf specific} form of \get\ so that \putl\ is carefully ``tuned'' for a given specific \get. In other words, for a given specific domain context \nix, model spaces $\spA_i$ are special categories and functors \get s are special functors for which a reasonable single-valued operations \putl\ can be defined. For example, ML provides a special context, in which model spaces are Euclidean spaces (considered as categories $\rcat^m$), \get s are differentiable mappings \frar{f}{\rcat^k\timm\rcat^m}{\rcat^n}, and the gradient descent idea Gd provides a reasonable definition of \putl s. We will return for this discussion in \sectref{policyfun}
 
 \endinput
 
 \renewcommand\fu{}
 \renewcommand\wi{}
 
 % \input{ll-figures/diags/policyfun}
 %  \input{ll-figures/diags/policyfun-smallTri}
  %\input{ll-figures/diags/policyfun-bigTri-OLD(defVersion)} % future work
      \input{ll-figures/diags/policyfun-bigTri}
 %   \input{ll-figures/diags/policyfun-new}
 
 We can model the notion of a context \nix\ as an %sm-subcategory $\pgetcat_\nix$ of the sm-category of parametrized functors \pcatcat\ (see Appendix \sectref{pcatcat}) or, better, as an 
 sm-category $\pgetcat_\nix$ equipped with a faithful forgetful functor \frar{{-}\nix}{\pgetcat_\nix}{\pcatcat} (read symbol `${-}\nix$' as ``forget the \nix-structure'') into the category \pcatcat\ of all small categories and (equivalence classes of) parameterized functors between them (see Appendix \sectref{pcatcat}).  Now the process of building \putl\ based on \get\ can be formalized as a graph morphism \frar{\plusxput}{\pgetcat_\nix}{\alalenscat} from (the graph underlying) category $\pgetcat_\nix$ of parameterized \nix-functors to (the graph underlying) category of ala-lenses such that the internal triangle (*) in \figref{policyfun} commutes  %$({+}_\nix\putl);({-}\putl)={-}\nix$ 
 (read symbol `$\plusx{\nix}\putl$' as ``add \nix-determined operation \putl'' and `${-}\putl$' as ``forget operation \putl'' in a lens $\ell=(\get, \putl)$). 
 
 A central question of defining an update policy is whether it is functorial, that is, whether the graph morphism \plusxput\ is a functor. For example, a central result of \citefst\ is functoriality of \frar{\plusputx{Gd(\eps,\err)}}{\diffcat}{\learncat} where Gd refers to defining \putl\ via gradient descent with step size $\eps$ and  error function \err\ (see above), \diffcat\ denotes the category of (equivalence classes of) parameterized differentiable functions between Euclidean spaces, and \learncat\ is the category of codiscrete ala-lenses. The discussion above motivates the following formal definition.
 %\begin{defin}\label{def:policyfun}
 \par
 \smallskip\noindent
 {\bf Definition (Change propagation systems).}
 	An {\em asymmetric (parameterized, compositional) change propagation system (CPS)} is a triple $\nix=(\pgetcat_\nix, {-}\nix, \plusxput)$ with \pgetcat\ being an sm-category  equipped with two sm-functors, ${-}\nix$ and \plusxput\ as shown in \figref{policyfun}, such that ${-}\nix$ is faithful, and the triangle (*) commutes. % functor commutative diagram of functors 
 	
 	A CPS is called {\em codiscrete} if functor ${-}\nix$ factors through \psetcat\ and functor \plusxput\ factors through $\alalenscat_0$ as shown in \figref{policyfun}, where arrows with triangle tails denote full embeddings. Thus, a codiscrete CPS is a triple $\nix=(\pgetcat_\nix,{-}_0\nix, \plusxput_0)$ such that the external triangle (dashed arrows) in \figref{policyfun} commutes.
 %\end{defin}

One may think that ML-motivated CPS considered in \citefst\ is codiscrete  but .......

\zd{TWO sections are commented below:
	\\
ll-sections/ml-diff
\\
ll-sections/policyfun-ml2-piece
\\
but they are used elsewhere
}

\endinput

\input{ll-sections/ml-diff}
\input{ll-sections/policyfun-ml2-piece}

==> ll-sections/backgr.tex <==
\section{Background: Model spaces}
\endinput
\input{ll-sections/modSpaces-short}

==> ll-sections/bigPic.tex <==
\section{Propagation policy as  a functor
	%Functoriality of learning and back propagation
}

\input{ll-figures/diags/bigPicture}

==> ll-sections/bits-i-pieces-2.tex <==
\section{BITS AND PIECES}

%\input{ll-sections/policyfun-ml2-piece}
\input{ll-sections/vert-compose}

\subsection{Outdated DD-lens piece}
In more detail, we assume that model spaces are equipped with an operation \dif\ %\frar{\dif}{|\spX|\times|\spX|}{\spX} =>  this fomula doesn't work!!! hence commented
that assigns to each pair of objects $X, X'\in|\spXX|$ an arrow $\frar{\dif(X,X')}{X}{X'} \in \spXX(X,X')$ between them, and $\dif(X,X)=\id_X$ for all $X\in|\spXX|$. Then having a delta ala-lens \frar{\ell=(\get,\putl)}{\spS}{\spT}, we can build a codiscrete ala-lens \frar{\ell0=(\get0,\putl0)}{|\spS|}{|\spT|} (\ie, a learner as defined in \citefst) as follows: 
%, by defining its operation as follows: 
%%%so that codiscrete \putl-operations (denoted by \putl0) are actually composed, 
%\eg, the updated source state $S'=\putl0^\req_{p,S}(T')$ computed for a source state $S$ and a target state $T'$ is defined as the codomain of delta $\putl^\req_{p,S}(v)$ where $v=\dif(S.\get_p, T')$. %
%
%Thus, 
\renewcommand\xxx{\enma{\mathsf{xxx}}}
for any source $S$, target $T'$, and $\xxx \in \{\req, \upd, \self\}$, we define
\begin{align}
%\tag{(putDef)$^{xxx}$}
%\label{eq:codi-build}
%&\quad 
%%\begin{cases}
%\putl0^{\xxx}(v):=
%\mathsf{codomain}(
%\putl^{xxx}_{p,S}(v)
%)
%\\
%\mathcal{F}_{\wh}(\qb,\qt) \noteq 0 %\hfill \\
%\end{cases}
\tag{get0Def}
\label{get0def}
&\qquad \get0_p(S) :=\get_p(S) 
\\
\tag{put0Def}
\label{eq:put0def}
&\qquad \putl0^{\xxx}_{p}(S,T'):=
\mathsf{codomain}(
\putl^{\xxx}_{p,S}(v)) 
\mbox{ where $v=\dif(S.\get_p\,, T')$}
\end{align}
This construction gives us a reflexive graph morphism 
\begin{equation}\label{eq:codifun}
\frar{\codifun}{\alalenscatdif}{\alalenscatcodi}
\end{equation}
between (reflexive graphs underlying) the following categories: 
%whose domain is the following category: its 
objects of \alalenscatdif\ are model spaces (categories) equipped with operation \dif, and arrows are delta ala-lenses described in the paper, %satisfying conditions above, 
while \alalenscatcodi\ is the category whose objects are sets and arrows are codiscrete ala-lenses, \ie, learners defined in \citefst. %We will refer to arrows in \alalenscatdif\ as dd-lenses (= ala-lenses with differencing).

To ensure functoriality of \codifun,  we need to require compatibility of $\putl^\req$ and \dif:
\begin{equation}\label{eq:difputreq}
\putl^\req_{p,S}(v) = \dif(S,S')
\end{equation}
so that sequential composition of codiscrete lenses will be compatible with sequential composition of the underlying delta lenses. Preservation of condition \eqref{difputreq} by sequential and parallel composition is straightforward, and we thus have category \alalenscatdif\ of delta lenses with differencing satisfying \eqref{difputreq} (further called {\em dd-lenses}), and an sm-functor \eqref{codifun}. Note that Stability and Putget without amendment for the delta lens imply Getput and Putget for the codiscrete lens.

To ensure that the two structures of a dd-lens smoothly interact, we require the following conditions: %make the Putget law for codiscrete lenses stronger and delta-oriented, we also require
compatibility of the other two \putl\ operations with \dif:  
\begin{equation}\label{eq:difputupdself}
\begin{array}{c}
\putl^\upd_{p,S}(v) = \dif(p,p')
\\
\putl^\self_{p,S}(v) = \dif(T', S'.\get_{p'}) 
\end{array}
\end{equation}
(in the equations above, there are three different \dif-operations acting in their model spaces), and 
%and similarly for $\putl^\upd$ and $\putl^\self$. 
%We also require 
compatibility of \get\ and \dif: 
\begin{equation}\label{eq:difget}
\begin{array}{c}
\dif(S,S').\get_p=\dif(S.\get_p, S'.\get_p) \mbox{ for any $p, S, S'$}
\\
\dif(p,p').\get_S = \dif(S.\get_p, S.\get_{p'})\mbox{  for any $S, p, p'$} %\label{eq:difgets}
\end{array}
\end{equation}
In addition, we may want to require the Difdif law for \dif-operation:
\begin{equation}\label{eq:difdif}
\dif(X,X');\dif(X',X'') = \dif(X,X''),
\end{equation}
and then the Putput law for the delta lens implies Putput for the codiscrete lens (see %some discussion of Difdif law and its relation to Putput law can be found in 
\cite[Sect. 4.4]{me-jot11} for details).
Equations above look mathematically natural  and regulate the notion of a well-behaved dd-lens. They do also need a detailed discussion of their practical meaning, which we leave for future work. Further on, we assume that all dd-lenses satisfy the conditions above. 

\subsubsection{Structure preserved by functor \codifun %Preservation of the delta-free structure.
}
Specification of building a codiscrete lens from a dd-lens by a functor \eqref{codifun} is incomplete as it leaves  unspecified that the delta-free  part of a dd-lens is preserved in the corresponding codiscrete lens. This is fixed by the commutative diagram in \figrcodi\ in which nodes are sm-categories and arrows are sm-functors: for a while, only consider rows (1..5) of the digram and ignore  arrows starting at objects in row 7 (the vertical bang arrow $!$ (dashed) also originates at node $\pcatcat(\nix)$ but its lower part is screened by the inclusion arrow $i$).
%\input{ll-figures/diags/codifun}
%\input{ll-figures/diags/codifun-new}

Category \pcatcat\ is the category of all small categories and (equivalence classes of) parameterized functors between them (see Appendix \sectref{pcatcat} for a precise definition), and category \pcatcatdif\ is the category of small categories equipped with differencing and parameterized functors compatible with them as prescribed by equations  \eqref{difget}. We thus have a forgetful functor ${-}\dif$ in row (4) of the diagram. We will use this notational discipline below: functors forgetting a part $\xxx$ of the source category structure are denoted by ${-}\xxx$ (read ``minus \xxx'') while functors adding the part by ${+}\xxx$ (``plus \xxx''). For example, we have a forgetful functor ${-}\putl$ from lenses to parameterized functors as shown in the diagram. Any lens with differencing \elll\ consists of its \dif-compatible family of \get-functors $\ell.\differ$, and a delta lens $\ell.\lens$ as shown by the span of jointly monic functors in the diagram. By forgetting \dif\ on the left and \putl\ on the right, we obtain the same family of parameterized functors (\get s) so that the square commutes. %
%\footnote{There are other functors and commutativity conditions for the categories involved, which we omitted as our goao is to understand the construction of building codiscrete lenses.} 
Finally, codiscretization construction is given by functor \codiscr\ specified above together with two forgetful functors into the category of sets and parameterized functions \psetcat\ so that the ``trapezoid'' commutes: $\codiscr;({-}\putl_0) = \lens;({-}\putl);({-}\mathsf{deltas})$, where ${-}\mathsf{deltas}$ maps a small category to its set of objects with codiscrete arrows. % (recall that deltas are arrows of model spaces, \ie, the source and target categories for lenses).


%% the end of  the piece

\subsection{Unknown 2}
\begin{defin}[incremental view system]% cf. \right) 
The definition is illustrated by \figrgetamend b). 
			
		, where sets $|\spS|$ and $|\spT|$ are considered as dicrete categories. That is, we have a family of functions \frar{\getobp}{|\spS|}{|\spT|} indexed by $p\in|\spP|$ and for any arrow \frar{e}{p}{p'} in \spP\ and object $S\in\spS$, an arrow \frar{\get0_S(e)}{S.\getobp}{S.\getobx{p'}}.  a family of functions \frar{\get}{}{} and then $[|\spS|,|\spT|]$ is the category of functors from \spS\ to \spT\ and their natural transformations. For a parameter  $p\in|\spP|$, we write %$\get(p,\_)$ or 
		$\get_p$ or even shorter ${\_}_p$ for the functor \frar{\get(P)}{\spS}{\spT} (read ``get \spT-views of \spS''), and if $S\in|\spS|$ is a source model, its $\get_p$-view is denoted by $\get_p(S)$ or $S.\get_p$ or $S_p$. Given a parameter delta \frar{e}{p}{p'} and a source model $S\in|\spS|$, the model delta \frar{\get(e)}{\get_p(S)}{\get_{p'}(S)} will be denoted by $\get_e(S)$ or $e_S$ (rather than $S_e$ as we would like to keep capital letters for objects). %although a more consistent discipline would require $S_e$).%
		
		Since $\get_e$ is a natural transformation, for any delta \frar{u}{S}{S'}, we have a commutative square $e_S;u_{p'}=u_p;e_{S'}$. We will denote the diagonal of this square by $u.\get_e$ or \frar{u_e}{S_p}{S'_{p'}}.  Thus, we use notation
		%\begin{equation}\label{eq:u.gete}
		\begin{enumerate}[label={\bf  \alph*)}, %Step 
			%\arabic{enumi}., ref=Step \arabic{enumi},% 
			wide=5pt]
			\item[{\bf (b*)}]	
			~~~~~~\frar{u_e\eqdef u.\get_e \eqdef e_S;u_{p'}=u_p;e_{S'}}{S_p}{S'_{p'}}
		\end{enumerate}
		%\end{equation}
\end{defin}
Some work needs to be done to make the above sketch formally accurate, but it seems to be very well specifiable in terms of the get-part of the dd-lens \fwk\ with the following reservations:
\begin{itemize}
	\item we work with categories enriched over \nil\ rather than \setcat.
	\item we work with so called {\em edit} lenses, in which model spaces are equipped with monoids acting on them, and whose elements are called {\em edits}; thus, differentials map edits to edits.
	\item \get\ is a functor up to an amendment ($o(\del)$ in our setting)
\end{itemize}
It is easy to show that any edit lens gives rise to a delta lens (see \cite[sect.3]{me-jot11} for the idea and practical examples, and \citejrunified\ and \citeaotrx{Appendix F} for accurate formal definitions).

 ===== an old piece
 
 
We convert \reals\ into a category \rcat\ with $Hom(a,a')=\{(a, a'-a, a')\}$ and write the only element of the Hom as $(a'-a)$. Composition is defined by $(a'-a);(a''-a')$ := $ (a'-a)+(a''-a')=(a''-a)$, and the identity on $a$ is $(a-a)$, \ie, $(a,0,a)$. Monoid $\DDela=\DDel:=(\reals, +, 0)$ acts on this category in the obvious way, and we can treat this action as a discrete opfibration as shown by the leftmost square in the diagram, where * denotes the only object of category \DDel, and the dashed arrows are produced by lifting; following the lens parlance, we can call elements of \DDel\ {\em edits}. The derivative is then a monoid homomorphism mapping edits to edits, and the entire construction specified by diagram \eqref{difasfun} can be seen as the (incrementally defined) get-part of an asymmetric edit lens as defined in \citejrunified. That is,  pair $(f,\prt f)$ gives rise to a functor \frar{\ffun}{\rcat}{\rcat} with $a.\ffun :=a.f$ and 
\frar{(a'-a).\ffun = (a'-a)*\prt f(a)}{a.f}{a'.f}. %(recall that $a$ is the domain of arrow \del). % 
%We will also write $\prt f_a(\del)$ for \ffun(\del) to recall the origin of the arrow part of \ffun. 
 

Having a family of differentiable functions \frar{f_p}{\reals}{\reals} indexed by $p\in\reals$, we obtain a family of functors \frar{\ffun_p}{\rcat}{\rcat} and, moreover, for a parameter delta \frar{e=p'-p}{p}{p'}, we have a natural transformation $\ffun(e)$ that for any $a$ provides delta $f_{p'}(a)-f_p(a)$:  naturality of the transformation and conditions \eqref{difget} trivially hold. 
An accurate formal account of this treatment can be found in paper \citeao{Appendix F} about abstract differentiability.%
\footnote{In the lens jargon, their setting should be termed as (asymmetric) {\em edit lenses} (cf. \citeeditlenses) rather then delta lenses as such, but edit lenses can be seen as a special case of delta lenses as shown in \cite{jr-unified}.}

Generalization for multiple variables and parameterization is straightforward based on the functions \frar{f}{\reals^m}{\reals^n} is provided by the gradient vector construct. Having function \frar{f}{\reals^m}{\reals^n}, we consider $f$ as an $n$-tuple of functions \frar{f_j}{\reals^m}{\reals}, $j=1...n$, each having a derivative functor given by the gradient $\nabla f_j$ that maps  delta $a'-a = (a'_1-a_1,\ldots,a'_m-a_m)$ to delta $b'_j - b_j$, where $b_j=a.f_j$, $b'_j=a'.f_j$, computed %with error _1...a'_n)-f(a_1...a_n)$ 
by scalar multiplication: $b'_j-b_j=(a'-a)*\nabla f_j(a)$. Finally,  $b'-b = (b'_1-b_1,\ldots,b'_n-b_n)$.  


==> ll-sections/buffer.tex <==
\subsection{Change propagation systems}

\renewcommand\fu{}
\renewcommand\wi{}

% \input{ll-figures/diags/policyfun}
%\input{ll-figures/diags/policyfun-smallTri}
%\input{ll-figures/diags/policyfun-bigTri-OLD(defVersion)} % future work
%\input{ll-figures/diags/policyfun-3triangles} % includes \pgetcatnixcodi
\input{ll-figures/diags/policyfun-2triangles} % only has \pgetcatnix
%  \input{ll-figures/diags/policyfun-new}

%\endinput
We continue the discussion in ....
We can model the notion of a context \nix\ as an %sm-subcategory $\pgetcat_\nix$ of the sm-category of parametrized functors \pcatcat\ (see Appendix \sectref{pcatcat}) or, better, as an 
sm-category $\pgetcat_\nix$ equipped with a forgetful functor \frar{{-}\nix}{\pgetcat_\nix}{\pcatcat} (read symbol `${-}\nix$' as ``forget the \nix-structure'') into the category \pcatcat\ of all small categories and (equivalence classes of) parameterized functors between them (see Appendix \sectref{pcatcat}).  The process of building \putl\ based on \get\ can be formalized as a 
%bijective on objects (bo) 
graph morphism \frar{\plusxput}{\pgetcat_\nix}{\alalenscat} from (the graph underlying) category $\pgetcat_\nix$ of parameterized \nix-functors to (the graph underlying) category of ala-lenses such that the internal triangle (*) in \figref{policyfun} on p.~\pageref{fig:policyfun} commutes. %$({+}_\nix\putl);({-}\putl)={-}\nix$ 
Read symbol `$\plusx{\nix}\putl$' as ``add \nix-determined operation \putl'' and `${-}\putl$' as ``forget operation \putl'' in a lens $\ell=(\get, \putl)$. The label $[{-}\nix]$ below arrow \plusxput\ is not a part of the functor name: it's a reminder that alongside with adding \putl, the functor also forgets the context/structure \nix. 

%\endinput
A central question of defining an update policy is whether it is functorial, that is, whether the graph morphism \plusxput\ is a functor. For example, a central result of \citefst\ is functoriality of \frar{\plusputx{Gd(\eps,\err)}}{\paracatre}{\learncat} where Gd refers to defining \putl\ via gradient descent with step size $\eps$ and  error function \err\ (see above), \paracatre\ denotes the category of (equivalence classes of) parameterized differentiable functions between Euclidean spaces, and \learncat\ is the category of codiscrete ala-lenses. The discussion above motivates the following formal definition.
%\begin{defin}\label{def:policyfun}
\par
\smallskip\noindent
{\bf Definition (Change propagation systems).}
An {\em asymmetric (parameterized, compositional) change propagation system with learning (a CP-system in short)} is a triple $\nix=(\pgetcat_\nix, {-}\nix, \plusxput)$ with \pgetcatnix\ being an sm-category  equipped with two sm-functors, ${-}\nix$ and \plusxput\ as shown in \figref{policyfun}, such that ${-}\nix$ is \zdmod{faithful}{forgetful??}{}, and the triangle (1) commutes. % functor commutative diagram of functors 

A CPS is called {\em codiscrete} if functor ${-}\nix$ factors through \psetcat\ and functor \plusxput\ factors through $\alalenscat_0$ as shown in \figref{policyfun}, where arrows with triangle tails denote obvious embeddings (and hence the factorizations are unique so that a codiscrete CPS can be seens  as a triple $\nix=(\pgetcat_\nix,{-}_0\nix, \plusxput_0)$ such that the external triangle (dashed arrows) in \figref{policyfun} commutes: as square (2) is always commutative, commutativity of (1) is derived).
%\end{defin}

One may think that ML-motivated CPS considered in \citefst\ is codiscrete  but .......

\begin{defin}[CPS with differencing]
	A {\em CPS with differencing (CPD-system, CPDS)}  is a quadruple 
	$\nix=(\pgetcatnix,\plusxput, \plusxdif, \minusnix)$ 
	where the triple $((\pgetcatnix,\plusxput, \minusnix)$ is a CPS, and \plusxdif\ is a functor as shown in diagram (rows 3-7 left) such that triangle (2) commutes.
\end{defin}



==> ll-sections/buffer2.tex <==
\subsection{Delta lenses with differencing: their disassembling and assembling} 
%\input{ll-figures/diags/codifun}
\input{ll-figures/diags/codifun-last%
	-withPara%
}

Codiscrete lenses appearing in BX practice are delta lenses equipped with an additional {\em differencing} operation that automatically computes deltas (rather than delta lenses with forgotten deltas as is common to think about codiscrete lenses). We will sketch the corresponding formal \fwk. 
\subsubsection{Main definitions and facts}
\begin{defin}[Model spaces with differencing, dif-spaces]
	A {\em model space with differencing} is a pair $\spX=(|\spX|, \dif)$ with $|\spXX|$ a model space (= a strongly skeletal category) and \dif\ an operation that assigns to each pair of objects $X, X'\in||\spXX||$ an arrow $\frar{\dif(X,X')}{X}{X'} \in |\spXX|(X,X')$ between them, such that 
	
	\noindent\begin{tabular}{ll}
		\lawnamebr{DifId}{}
		& \mbox{$\dif(X,X)=\id_X$ for all $X\in|\spXX|$}
		\\
		\lawnamebr{DifDif}{}
		& \mbox{$\dif(X,X');\dif(X',X'')=\dif(X,X'')$ for all $X, X', X''\in|\spXX|$}
		\end{tabular}

\noindent By a typical abuse of notation, we will denote a dif-space \spXX\ and its carrier category by the same symbol \spXX. 
	
	A {\em dif-functor} between dif-spaces  is a functor \frar{\get}{\spS}{\spT} such that conditions Difget$_0$ below holds for any $S,S'$ in \spS. 
	%A natural dif-\trafon\ between two dif-functors \frar{\get_i}{\spS}{\spT}, $i=1,2$ is a natural \trafon\ \drar{\tau}{\get_1}{\get_2} such that condition Difget below holds.
	Dif-functors and their natural transformations form a category  denoted by $[\spS, \spT]$. 
	
		A {\em parametrized} dif-functor between dif-spaces  is given by a small category \spP\ of parameters, and a functor \frar{\get}{\spP}{[\spS, \spT]} such that conditions DifGet holds for any \frar{e}{p}{p'}. 
	
\noindent
\begin{tabular}{ll}
	\lawnamebr{DifGet}{$_0$}
	  &\mbox{$(S, S').\dif^\spS.\get =(S.\get, S'.\get).\dif^\spT$ }
	  \\
%	\lawnamebr{DifGet}{$_\tau$}
%      &\mbox{$(S, S').\dif^\spS.\tau =(S.\get, S'.\get).\dif^\spT$}
      	\lawnamebr{DifGet}{}
      &\mbox{$(S, S').\dif^\spS.\get_e =(S.\get, S'.\get).\dif^\spT$ 
  }
\end{tabular}
	\end{defin}

\input{ll-figures/diags/dif-space-triangle}
It is easy to see that similarly to \pcatcat, parameterized dif-functors between dif-spaces form an sm-category \pspadifcat, and the inset diagram commutes.
%It is easy to see that similarly to \pcatcat, parameterized dif-functors between dif-spaces form an sm-category \pspadifcat, and the inset diagram trivially commutes.




%
\begin{defin}[ala-lenses with differencing, alad-lenses]
	An {\em (well-behaved) alad-lens} from a dif-space \spS\ to a dif-space \spT\ is an ala-lens \frar{\ell=(\spP, \get, \putl)}{\spS}{\spT}, in which  %where \spP\ is a smal category of {\em parameters}, 
	\get\ is a parameterized dif-functor from \spS\ tp \spT, and condition DigPut holds for any $S$, $p$ and $T'$ in \spS, \spP, and \spT\ resp. (and where $S'$ denotes the target of $\putl^\req_{S,p}.\dif^\spT(S_p,T') $): %\putl\ operations are  compatible with differencing in the following sense:
		
		\noindent\begin{tabular}{ll}
		\lawnamebr{DifPut}{}
		&\mbox{$\dif^\spS(S, S') =\putl^\req_{S,p}.\dif^\spT(S_p,T')$ 
		}
	\end{tabular}
\end{defin}


\input{ll-figures/diags/codifun-triangle}

Alad-lenses form an sm-category \aladlenscat\ equipped with a forgetful functor ${-}\dif$ as shown in the diagram \figcodifun. What is special about alad-lenses is that any alad-lens \frar{\ell=(\spP,\get,\putl)}{\spS}{\spT} gives rise to a codiscrete lens  \frar{\ell^0=(\spP^0,\get^0,\putl^0)}{\spS^0}{\spT^0}, in which
$S.\get^0_p \eqdef S.\get_p$ and 
$\putl^{0\xyz}_{p}(S,T')\eqdef \cod.\putl^{\xyz}_{p,S}.\dif^\spT(S_p, T')$ 
for all $\xyz\in \{\req,\upd,\self\}$. Due to condition DifPut, this construction gives rise to a functor shown by the horizontal arrow in the triangle in \figcodifun. Importantly, for a general alad-lens the triangle does not commute as \codifun\ does not fully use the underlying delta lens structure: commuting only holds for thin dif-spaces whose Hom-sets are singletons. A more detailed story is given by rows (1-5) of the diagram \figcodifunbig\ (the vertical dashed arrow $[\plusx{\nix},\plusx{\nix}]$ actually originates at node $\pcatcat(\nix)$ and does not belong to rows (1-5) (its lower part is screened by arrow ${-}\nix$). Note that the pair of firgetful functors $({-}\lens, {-}\dif)$ is jointly monic.



Now we can continue our discussion of compositionality of update policies, which we began on p.\pageref{fig:policyfun} with the notion of change propagation systems. 

%\endinput
\subsubsection{Building delta lenses.}

\zd{Fix outdated names of functors and revise}

Rows (1-5) of diagram \figcodifun\ show decomposition of dd-lenses and structure deletion, but in practice we need to go in the opposite direction and build lenses (and their codiscrete variants) by structure addition. That is, we  start with categories and functors (or sets and functions), \ie, the \get\ part, and then add to them  operations \putl s (and \dif\ if finally we want to build a codiscrete lens). This is a challenging task as there are many possibilities of adding  \dif s and \putl s so that the resulting dd-lens is well-behaved and, as a rule, there are no universal solutions amongst those possibilities. Hence, given a concrete context \nix\ in which \get s are defined (formally, a subcategory $\pcatcat(\nix)$ or $\psetcat(\nix)$ for the codiscrete case), we need a {\em selection policy} that would allow us to choose reasonable \dif s and \putl s so that the result would be a dd-lens suitable for the context \nix. 


If \nix\ is some model-to-model transformation context (BX), then category $\pcatcat(\nix)$ is roughly sketched in \sectref{backgr}, and operations \dif\ and \putl\ are to be carefully selected depending on the needs of a particular change propagation problem at hand---hence, names ${+}\dif(\pol)$ and ${+}\putl(\pol)$ for the corresponding arrows in the diagram \figrcodi, where \pol\ refers to the propagation policy. 


Similarly, if the context is ML, then we begin building dd-lenses from $\psetcat(\nix)$ being the category of Euclidean spaces and parameterized differentiable mappings between them (denoted \paracat\ in \citefst), \dif\ is the ordinary difference of reals, and a typical ML propagation policy is based on the gradient descent idea  (Gd). % and back-propagation (Bp) constructs. 
We will discuss this in more detail in the next section. Perhaps, connections between open games (OG) and lenses can be treated similarly by considering OG as a special case of context \nix. 


==> ll-sections/buffer3.tex <==
\subsection{An example of change propagation system: Learners as alad-lenses}

 %%==
\input{ll-figures/diags/policyfun-ml}
%%===


In this diagram, \pcatcat\ is the category of all small categories as objects and (equivalence classes of) parameterized functors between them as arrows.%
\footnote{The latter are functors \frar{f}{\spP\timm\spA}{\spB} or, equivalently, functors \frar{f}{\spP}{[\spA, \spB]} from some small category \spP\ into the category of functors $\spA\rightarrow\spB$ and their natural transformations; see \sectref{pcatcat} for details.}



The category of (small) sets and (equivalence classes of) parameterized functions, \psetcat, is fully embedded into \pcatcat\ by considering any set as a codiscrete category.  We name this embedding as \plusarrx{\pairing} to be read as ``add arrows by pairing'', \ie, by considering a pair $(a,a')\in A\timm A$ as an arrow $a\rightarrow a'$, which makes set $A$ a (codiscrete) category \spA.  Similarly, on the right side, we have a full embedding of the category of codiscrete ala-lenses into the category of delta ala-lenses. Finally, as any ala-lens is basically a pair $\get, \putl$ with \get\ a parameterized functor and \putl\ is its inversion in some special sense, we have a forgetful functor ${-}\putl$ (read ``forget \putl'') as shown in the diagram.  

Now we consider the upper row of the diagram. We can convert any Euclidean space $\reals^n$ into a category $\rcat^n$ whose arrows, \frar{\del}{a}{a'}, are deltas defined componentwise: $a=(a_i)_{i\le n}$, $a'=(a'_i)_{i\le n}$, and $\del=(\del_i)_{i\le n}$ with $\del_i=a'_i-a_i$. Functors \frar{\pmb f}{\rcat^n}{\rcat^n} and functions \frar{f}{\reals^m}{\reals^n} are in bijective correspondence. This gives us the commutative square (1) in which $\paracatrcat$ is the category of parameterized differentiable maps considered as functors, the upper arrow is an isomorphism, and vertical arrows are functors that forget the rich structure of \reals\ and consider it as either a set (the left edge) or a category (the right edge).  The central part of the story is given by the central square (2). The gradient descent idea (Gd) allows us to add to any parameterized functor \fbf\  in \paracatrcat\ with its inverse (in a certain sense)  mapping \putl\ so that the pair $(\fbf,\putl)$ makes an ala-lens with an additional operation of differencing, which for any two objects $x,y$ in a general category \spXX\ selects an arrow/delta \frar{\dif(x,y)}{x}{y} %called adelta between $x$ and $y$ 
(an accurate definition will be given in \sectref{codilens}). Forgetting first \dif\ and then \putl\ gives us a commutative square (2). Finally, a typical way of building codiscrete lenses in applications is to begin with a delta lens with differencing, which gives rise to a codiscrete lens in a functorial way--this gives us a general functor \codiscr\ (the right most edge in the diagram denotes equality: two different names for the same category). Note that square (actually, triangle) (3) is not %necessarily commutative and is not 
commutative for a general delta lens with diff, whose underlying lens is not codiscrete. However, the lenses in the image of functor $\plusx{Gd(\eps,\err)}\putl$ relate thin categories, so that the rectangle (2)+(3) is commutative. 


==> ll-sections/cpsystems.tex <==
\subsection{Change propagation systems}

\renewcommand\fu{}
\renewcommand\wi{}

% \input{ll-figures/diags/policyfun}
%\input{ll-figures/diags/policyfun-smallTri}
%\input{ll-figures/diags/policyfun-bigTri-OLD(defVersion)} % future work
%\input{ll-figures/diags/policyfun-3triangles} % includes \pgetcatnixcodi
\input{ll-figures/diags/policyfun-2triangles} % only has \pgetcatnix
%  \input{ll-figures/diags/policyfun-new}

%\endinput
We continue the discussion in ....
We can model the notion of a context \nix\ as an %sm-subcategory $\pgetcat_\nix$ of the sm-category of parametrized functors \pcatcat\ (see Appendix \sectref{pcatcat}) or, better, as an 
sm-category $\pgetcat_\nix$ equipped with a forgetful functor \frar{{-}\nix}{\pgetcat_\nix}{\pcatcat} (read symbol `${-}\nix$' as ``forget the \nix-structure'') into the category \pcatcat\ of all small categories and (equivalence classes of) parameterized functors between them (see Appendix \sectref{pcatcat}).  The process of building \putl\ based on \get\ can be formalized as a 
%bijective on objects (bo) 
graph morphism \frar{\plusxput}{\pgetcat_\nix}{\alalenscat} from (the graph underlying) category $\pgetcat_\nix$ of parameterized \nix-functors to (the graph underlying) category of ala-lenses such that the internal triangle (*) in \figref{policyfun} on p.~\pageref{fig:policyfun} commutes. %$({+}_\nix\putl);({-}\putl)={-}\nix$ 
Read symbol `$\plusx{\nix}\putl$' as ``add \nix-determined operation \putl'' and `${-}\putl$' as ``forget operation \putl'' in a lens $\ell=(\get, \putl)$. The label $[{-}\nix]$ below arrow \plusxput\ is not a part of the functor name: it's a reminder that alongside with adding \putl, the functor also forgets the context/structure \nix. 

%\endinput
A central question of defining an update policy is whether it is functorial, that is, whether the graph morphism \plusxput\ is a functor. For example, a central result of \citefst\ is functoriality of \frar{\plusputx{Gd(\eps,\err)}}{\paracatre}{\learncat} where Gd refers to defining \putl\ via gradient descent with step size $\eps$ and  error function \err\ (see above), \paracatre\ denotes the category of (equivalence classes of) parameterized differentiable functions between Euclidean spaces, and \learncat\ is the category of codiscrete ala-lenses. The discussion above motivates the following formal definition.
%\begin{defin}\label{def:policyfun}
\par
\smallskip\noindent
{\bf Definition (Change propagation systems).}
An {\em asymmetric (parameterized, compositional) change propagation system with learning (a CP-system in short)} is a triple $\nix=(\pgetcat_\nix, {-}\nix, \plusxput)$ with \pgetcatnix\ being an sm-category  equipped with two sm-functors, ${-}\nix$ and \plusxput\ as shown in \figref{policyfun}, such that ${-}\nix$ is \zdmod{faithful}{forgetful??}{}, and the triangle (1) commutes. % functor commutative diagram of functors 

A CPS is called {\em codiscrete} if functor ${-}\nix$ factors through \psetcat\ and functor \plusxput\ factors through $\alalenscat_0$ as shown in \figref{policyfun}, where arrows with triangle tails denote obvious embeddings (and hence the factorizations are unique so that a codiscrete CPS can be seens  as a triple $\nix=(\pgetcat_\nix,{-}_0\nix, \plusxput_0)$ such that the external triangle (dashed arrows) in \figref{policyfun} commutes: as square (2) is always commutative, commutativity of (1) is derived).
%\end{defin}

One may think that ML-motivated CPS considered in \citefst\ is codiscrete  but .......

\begin{defin}[CPS with differencing]
	A {\em CPS with differencing (CPD-system, CPDS)}  is a quadruple 
	$\nix=(\pgetcatnix,\plusxput, \plusxdif, \minusnix)$ 
	where the triple $((\pgetcatnix,\plusxput, \minusnix)$ is a CPS, and \plusxdif\ is a functor as shown in diagram (rows 3-7 left) such that triangle (2) commutes.
\end{defin}


==> ll-sections/ddlenses.tex <==
\subsection{Delta lenses with differencing: their disassembling and assembling} 
%\input{ll-figures/diags/codifun-small}  wnet below 
\input{ll-figures/diags/codifun-last%
	-withPara%
}

Codiscrete lenses appearing in BX practice are delta lenses equipped with an additional {\em differencing} operation that automatically computes deltas (rather than delta lenses with forgotten deltas as is common to think about codiscrete lenses). We will sketch the corresponding formal \fwk. 
\subsubsection{Main definitions and facts}
\begin{defin}[Model spaces with differencing, dif-spaces]
	A {\em model space with differencing} is a pair $\spXX=(|\spXX|, \dif)$ with $|\spXX|$ a model space (= a strongly skeletal category) and \dif\ an operation that assigns to each pair of objects $X, X'\in||\spXX||$ an arrow $\frar{\dif(X,X')}{X}{X'} \in |\spXX|(X,X')$ between them, such that 
	
	\noindent\begin{tabular}{ll}
%		\lawnamebr{DifId}{}
%		& \mbox{$\dif(X,X)=\id_X$ for all objects $X\in||\spXX||$}
	\lawnamebr{DifId}{}
		& \mbox{$\dif(X,X)\noteq\id_X$ for all objects $X\in||\spXX||$}
		\\
		\lawnamebr{DifDif}{}
		& \mbox{$\dif(X,X');\dif(X',X'')\le\dif(X,X'')$ for all $X, X', X''\in|\spXX|$}
		\end{tabular}


\noindent By a typical abuse of notation, we will often denote a dif-space \spXX\ and its carrier category by the same symbol \spXX, but write \spXXcodi\ for the set of objects to avoid confusion. %  $||\spXX||$. 
	
	A {\em dif-functor} between dif-spaces  is a functor \frar{\get}{\spS}{\spT} such that conditions Difget$_0$ below holds for any $S,S'$ in \spS. 
	%A natural dif-\trafon\ between two dif-functors \frar{\get_i}{\spS}{\spT}, $i=1,2$ is a natural \trafon\ \drar{\tau}{\get_1}{\get_2} such that condition Difget below holds.
	Dif-functors and their natural transformations form a category  denoted by $[\spS, \spT]$. 
	
		A {\em parametrized dif-functor} between dif-spaces  is given by a small category \spP\ of parameters, and a functor \frar{\get}{\spP}{[\spS, \spT]} (that we write as \fprar{f}{\spS}{\spT}{\spP}) such that two conditions Difget hold for any \frar{e}{p}{p'}. 

\noindent
\begin{tabular}{ll}
	\lawnamebr{DifGet}{$_0$}
	  &\mbox{$(S, S').\dif^\spS.\get =(S.\get, S'.\get).\dif^\spT$ }
	  \\
%	\lawnamebr{DifGet}{$_\tau$}
%      &\mbox{$(S, S').\dif^\spS.\tau =(S.\get, S'.\get).\dif^\spT$}
      	\lawnamebr{DifGet}{}
      &\mbox{$(S, S').\dif^\spS.\get_e =(S.\get, S'.\get).\dif^\spT$ 
  }
\end{tabular}
\end{defin}
%  a triablge diagram not needed now
%\input{ll-figures/diags/dif-space-triangle}
It is easy to see that similarly to \pcatcat, parameterized dif-functors between dif-spaces form an sm-category \pspadifcat\ equipped with a faithful forgetful functor \frar{~~\minusdif}{\pspadifcat}{\pcatcat~~} (read ``minus \dif, \ie, forget \dif) into the category of small categories and parametrized functors defined in Appendix \sectref{pcatcat}. With the axiom of choice, this functor is surjective on objects (soo). % if the axiom of choice holds. 
For a dif-space \spXX, we will write $\spXX_\minusdif$ for the category $\quad\minusdif(\spXX)$
%, and the inset diagram commutes.
%It is easy to see that similarly to \pcatcat, parameterized dif-functors between dif-spaces form an sm-category \pspadifcat, and the inset diagram trivially commutes.




%
\begin{defin}[ala-lenses with differencing, alad-lenses]
	An {\em (well-behaved) alad-lens} from a dif-space \spS\ to a dif-space \spT\ is an ala-lens \fprar{\ell=(\get, \putl)}{\spS}{\spT}{\spP}, in which  %where \spP\ is a smal category of {\em parameters}, 
	\get\ is a parameterized dif-functor from \spS\ tp \spT, and condition \difputlaw\ below holds for any $S\inn\spS$, $p\inn\spP$ and $T'\inn\spT$
	% in \spS, \spP, and \spT\ resp. 
	(and where $S'$ denotes the target of $\putl^\req_{S,p}.\dif^\spT(S_p,T') $): %\putl\ operations are  compatible with differencing in the following sense:
		
		\noindent\begin{tabular}{ll}
		\lawnamebr{\difputlaw}{}
		&\mbox{$\dif^\spS(S, S') =\putl^\req_{S,p}.\dif^\spT(S_p,T')$ 
		}
	\end{tabular}
\end{defin}
Sequential and parallel composition of alad-lenses is defined in exactly the same way as for ala-lenses, and in the same way we can make from alad-lenses an sm-category
\aladlenscat. Facts about this category that we need are presented by diagram in \figcodifuni, in which nodes are sm-categories and arrows are sm-functors (so that \figcodifuni\ presents a diagram in \smcatcat). %\figref{codifun-1}

\clearpage
%\input{ll-figures/diags/codifun-triangle}
%\input{ll-figures/diags/codifun-small}
\input{ll-figures/diags/codifun-small-noteq-learner}
Let us begin with the diamond (1). The left upper arrow \minusput\ is an identity on objects (ioo) functor that forgets the \putl-components of arrows and maps an alad-lens \fprar{\ell{=}(\get,\putl)}{\spS}{\spT}{\spP} to a parameterized dif-functor 
\fprar{\get}{\spS}{\spT}{\spP}. It is not faithful as there are many ways of inverting a \get, and is full if the axiom of choice holds.%
%
\footnote{Non-faithfulness does not contradicts to the \fwk\ described by John Baez in \citebaezncat: although  functor \minusput\ forgets an operation,  this operation can be see as ``some stuff'' in the arrows of the source category rather than some structure over its objects.} The left lower arrow \minusdif\ is an soo (with the axiom of choice) faithful forgetful functor mentioned above (it forgets a part of the object structure and maps an arrow 
\fprar{\get}{\spS}{\spT}{\spP} to arrow \fprar{\get}{\spS_\minusdif}{\spT_\minusdif}{\spP}
). The right upper functor \minusdif\ is a %bijective on objects (boo) 
soo faithful forgetful functor, and the right lower \putl\ is an injective on objects (ioo) full functor forgetting \putl\ (and the space properties). The diamond commutes: an alad lens 
\fprar{\ell{=}(\get, \putl)}{\spS}{\spT}{\spP}
is mapped to a p-functor
\fprar{\get}{\spS_\minusdif}{\spT_\minusdif}{\spP}.
%
The pullback of the lower cospan (note the dashed span) gives us the category of alad-lenses not necessarily satisfying condition \difputlaw. Commutativity of (1) now implies a unique functor {!} which is a property forgetting embedding. 
%Finally, the pair of upper functors is jointly monic: alad-lenses constitute a subcategory of the product $\pspadifcat\times\alalenscat$ defined by equations . 

What is special about alad-lenses is that any alad-lens \fprar{\ell{=}(\get,\putl)}{\spS}{\spT}{\spP} gives rise to a codiscrete ala-lens  \fprar{\ell^0{=}(|\get|,\putl^0)}{||\spS||}{||\spT||}{|\spP|}, in which
\begin{equation}\label{eq:codifundef}
S.|\get_p| \eqdef S.\get_p
 \mbox{ and }
\putl^{0\xyz}_{p}(S,T')\eqdef \cod.\putl^{\xyz}_{p,S}.\dif^\spT(S_p, T')
\end{equation}
for each $\xyz\in \{\req,\upd,\self\}$. This construction gives rise to a graph morphism shown by the dotted arrow labelled ``not a functor'' because to ensure functoriality, we need to require \difputlaw, which provides functor \codifun\ as shown in the diagram. Importantly, for a general alad-lens, the triangle (2) does not commute as \codifun\ does not fully use the underlying delta lens structure (but commuting holds for thin dif-spaces whose Hom-sets are singletons). %A more detailed story is given by rows (1-5) of the diagram \figcodifunbig\ (the vertical dashed arrow $[\plusx{\nix},\plusx{\nix}]$ actually originates at node $\pcatcat(\nix)$ and does not belong to rows (1-5) (its lower part is screened by arrow ${-}\nix$). Note that the pair of firgetful functors $({-}\lens, {-}\dif)$ is jointly monic.
%%\input{ll-figures/diags/codifun-triangle}
%\input{ll-figures/diags/codifun-small}


Finally, to complete the picture, we tile diamonds (1) and (2) with another commutative diamond (3), in which %\alalenscatcodi\ is the subcategory of codiscrete ala-lenses with an obvious forgetful functor 
\minusputcodi\ is an obvious forgetfulinto \psetcat\ defined in Appendix \sectref{pcatcat}.


Now we can continue our discussion of compositionality of update policies, which we began on p.\pageref{fig:policyfun} with the notion of change propagation systems. 

%\endinput
\subsubsection{Building delta lenses.}

\zd{Fix outdated names of functors and revise}

Rows (1-5) of diagram \figcodifun\ show decomposition of dd-lenses and structure deletion, but in practice we need to go in the opposite direction and build lenses (and their codiscrete variants) by structure addition. That is, we  start with categories and functors (or sets and functions), \ie, the \get\ part, and then add to them  operations \putl s (and \dif\ if finally we want to build a codiscrete lens). This is a challenging task as there are many possibilities of adding  \dif s and \putl s so that the resulting dd-lens is well-behaved and, as a rule, there are no universal solutions amongst those possibilities. Hence, given a concrete context \nix\ in which \get s are defined (formally, a subcategory $\pcatcat(\nix)$ or $\psetcat(\nix)$ for the codiscrete case), we need a {\em selection policy} that would allow us to choose reasonable \dif s and \putl s so that the result would be a dd-lens suitable for the context \nix. 


If \nix\ is some model-to-model transformation context (BX), then category $\pcatcat(\nix)$ is roughly sketched in \sectref{backgr}, and operations \dif\ and \putl\ are to be carefully selected depending on the needs of a particular change propagation problem at hand---hence, names ${+}\dif(\pol)$ and ${+}\putl(\pol)$ for the corresponding arrows in the diagram \figrcodi, where \pol\ refers to the propagation policy. 


Similarly, if the context is ML, then we begin building dd-lenses from $\psetcat(\nix)$ being the category of Euclidean spaces and parameterized differentiable mappings between them (denoted \paracat\ in \citefst), \dif\ is the ordinary difference of reals, and a typical ML propagation policy is based on the gradient descent idea  (Gd). % and back-propagation (Bp) constructs. 
We will discuss this in more detail in the next section. Perhaps, connections between open games (OG) and lenses can be treated similarly by considering OG as a special case of context \nix. 


==> ll-sections/derivatives-as-functors.tex <==
\section{Learners as delta lenses %: Functoriality of differentiation
}\label{sec:derifun}
%\newcommand\leefun{\enma{L_{\eps,\err}}}


In this section, we sketch  how the functor \frar{\leefun}{\paracat}{\learncat} specified in \citefst\ could be derived along the dd-lens lines described above as the composition $\leefun=({+}
\mathsf{deltas});!;\codifun$, where $!$ is the unique functor determined by pair $({+}\dif(pol), {+}\putl(pol))$ due to the universal property of products and the fact that the image of $!$ satisfies the condition of being a well-behaved dd-lens. 

\newcommand\figrcomp{\figref{difasfun}}
\subsubsection{Derivative as a functor.} Our first observation is that differentiability can be seen as functoriality. 
Let \frar{f}{\reals}{\reals} be a differentiable function, whose derivative is denoted by $\prt f$, $a,a'$ are two reals and $\del=a'-a$ is their difference treated as an arrow \frar{\del}{a}{a'}. %---subindex $a$ is used to suggest that we consider $a'-a$ as an action (we will also say {\em edit}) applied to value $a$ so that $(\reals, +, 0)$ becomes a monoid acting on \reals. 
%%(The difference $a'-a$ plays yet another role of a distance between $a$ and $a'$, below we will discuss it in more detail.) 
If \del\ is small enough, then $f(a')-f(a)\approx \del\cdot\prt f(a)$ and we can say that $\prt f(a)$ maps arrow \del\ to arrow \frar{\del.\prt f(a)}{a.f}{a'.f}. If function $f$ maps from the left to the right, we will often use the dot notation for function application so that \frar{\del.\prt f_a}{a.f}{a'.f}, where $\prt f_a$ denotes $\prtf(a)$. %the value of the differential $\prt f(a)$ at point $a$.

%-- the gradient version ---
%Let \frar{f}{\reals^m}{\reals} be a differentiable function, whose gradient is denoted by $\nabla f$, $a,a'$ are two $m$-tuples of real numbers, and $\del=(\del_1...\del_m)$ %a'-a=(a'_1-a-1,....,a'_m-a_m) is their componentwise difference, $\del_i=a'_i-a_i$, $i\le m$, treated as an arrow \frar{\del}{a}{a'}. If all $\del_i$ are small enough, then $f(a')-f(a)\approx \nabla f(a)\cdot\del$ (where $\cdot$ denotes the scalar product) and we can say that $\nabla f(a)$ maps arrow \del\ to arrow \frar{\nabla f(a)(\del)}{f(a)}{f(a')}. The generalization for the case \frar{f}{\reals^m}{\reals^n} is straightforward by considering $f$ a tuple $f_j, j\le n$ and Jacobian matrix $\jacobf=(\prt_if_j: i\le m, j\le n)$ replacing the gradient. To encompass all cases, we will call a linear operator mapping deltas from $a$ to deltas from $f(a)$ a {\em differential} and write  $\prtf(a)$ or often $\prtf_a$. If function $f$ maps from the left to the right, we will often use the dot notation for function application so that \frar{\del.\prt f_a}{a.f}{a'.f}, where $\prt f_a$ denotes the value of the differential $\prt f(a)$ at point $a$.

If deltas are not infinitely small, then $a'.f=a.f+\del.\prtf_a+o(\del)$ as shown by square (1) in diagram \figrcomp a, where \medadx{f} denotes $a.f+\del.\prtf_a$, and term $o(\del)$ converges to $0$ if \del\ converges to $0$. (If \frar{f}{\reals}{\reals} is an analytic function, then $o(\del)$ is the part of its Taylor series representation starting with the second order derivative, $o(\del)=\prt^2f_a\cdot\del^2/2!+\prt^3f_a\cdot\del^2/3!+\ldots$). If we consider \reals\ as a category \rcat\ whose arrows are triples $(a,\del,a')$ such that $a'=a+\del$, and composition $\del;\del'$ is given by addition, then differentiation becomes a functor-like mapping as shown by diagram  \figrcomp a. Diagram \figrcomp b, in which commutative ``rectangles'' (12) and (12') define $\prt(f;g)$, specifies the chain rule. 
\begin{remark}\label{rem:del-as-act}
	Commutativity of rectangle (11) in \figrcomp a is trivial as \rcat\ is a thin category. We can make it more interesting if....
\end{remark}
Generalization for the case \frar{f}{\reals^m}{\reals^n} is straightforward with $a,a'$ being $m$-tuples of real numbers, $\del=(\del_1...\del_m)$ %a'-a=(a'_1-a-1,....,a'_m-a_m) is 
their componentwise difference, Jacobian matrix $\jacobf=(\prt_i f_j: i\le m, j\le n)$ being the differential and $\jacobf\cdot\del$ is matrix-vector multiplication. If $n=1$, then \jacobf\ is gradient $\nabla f$. %, whose value at vector $a$ will be denoted by $\nabla_a$. 
To encompass all cases, we will call a linear operator mapping $m$-dimensional deltas from $a$ to $n$-dimensional deltas from $f(a)$ a {\em differential} and write  $\prtf(a)$ or often $\prtf_a$. 
%
An $m$-dimensional space $\reals^m$ is converted into category $\rcat^m$ componentwise. 

%======
%\input{figures/diags/difasfun1}
\input{figures/diags/difasfun3}
%====
%\input{figures/pdfs/getAmend-inR}
%====

\newcommand\couplarr[1]{\enma{#1^{\gg}}}
Now we define an abstract version of the above. %Given a category \spXX\ and an object $X\in|\spXX|$, we write $\spXX(X,\_)$ and $\spXX(\_,X)$ for classes \compr{\frar{u}{X}{X'}}{X'\in|\spXX|} and \compr{\frar{u}{X'}{X}}{X'\in|\spXX|} resp. 
Given a category \spXX\ and objects $X,X'\in|\spXX|$, we write $\couplarr{\spXX}(X,X')$ for the set of pairs of arrows 
%
\compr{(u,u')\in\spXX(X,Y)\timm\spXX(Y,X')}{Y\in|\spXX|} 
%
\noindent determined by the obvious pullback. 
\begin{defin}[Quasi-functors]\label{def:qfun}
Given categories \spA, \spB, a {\em quasi-functor} 
%$\spA\rightarrow\spB$ 
\frar{f^\gg}{\spA}{\spB} is given by i) an object function \frar{|f|}{|\spA|}{|\spB|} and ii) for any $A,A'\in|\spA|$, a mapping \frar{f^\gg_{AA'}}{\spA(A,A')}{\spB^\gg(B,B')} where $B=|f|(A)$, $B'=|f|(A')$. Given \frar{u}{A}{A'}, we consider the first component of pair $f^\gg_{AA'}(u)$ as the main value and denote it by $f_{AA'}(u)$ while the second component is called an {\em amendment} and denoted by $f_{AA'}^@(u)$. We say quasi-functor $f$ is {\em functorial at $u$} if $f_{AA'}^@(u)=\id_{B'}$, and {\em functorial at $A,A'$} if it is functorial at all \frar{u}{A}{A'}.  As a rule, we will omit indexes and write $f(u)$ for the main value and $f^@(u)$ for its amendments. %By an abuse of notation, 
The composition of pair $f^\gg_{AA'}(u)$, \ie, arrow $f(u);f^@(u)$, will be  denoted by $f^\gg(u)$. All this abuses notation but the context should make it clear.


Moreover, the following two functoriality conditions are required to hold for quasi-functors: unitality, \ie, for any $A$, $f(\id_A)=f^@(\id_A)=\id_{|f|(A)}$, and composition preservation  (cf. diagram \figrcomp a), which requires for any \frar{u}{A}{A'}, \frar{u'}{A'}{A''}, the following equation:
\begin{equation}\label{eq:qfun}
       f^\gg(u;u')=f^\gg(u);f^\gg(u') 
\end{equation}
%And for any $A$, $f(\id_A)=f^@(\id_A)=\id_{|f|(A)}$.
If $f$ maps from the left to the right, we will use the dot notation $u.f$, $u.f^@$. 
\end{defin}

The intuition that in the pair $u.f^\gg_{AA'}$, the component $u.f$ is the main value while $u.f^@$ is its amendment is formalized by the following definition of quasi-functor composition. Given two quasi-functors \frar{f}{\spA}{\spB} and \frar{g}{\spB}{\spC}, their {\em composition} $f;g$ or just $fg$ is defined by the following triple of mappings:  $|fg|:=|f|;|g|$ and, for any \frar{u}{A}{A'}, $u. fg := u.f .g$ and $u.(fg)^@:=(u.f.g^@);(u.f^@.g^\gg)$ (cf. diagram \figrcomp b). %Note that it is the definition of composition, which formalizes the intuition of the second component of a quasi-functor as an amendment.

Obviously, if $f$ and $g$ are unital, then $fg$ is such, and it is straightforward to check by multiple substitution, that if $f$ and $g$ preserve composition according to \eqref{qfun}, then $fg$ preserves composition too. Hence, $fg$ is a quasi-functor as soon as $f$ and $g$ are such. The identity functor on \spA\ is also the identity quasi-functor on \spA, and we thus have a category \qcatcat. Moreover, componentwise paring equips this category with an sm-structure: given parallel quasi-functors \frar{f_i}{\spA_i}{\spB_i}, $i=1,2$, we define $u_1\paar u_2.\,f_1\paar f_2=u_1. f_1\paar u_2.f_2$ and $u_1\paar u_2.\,(f_1\paar f_2)^@=u_1. f_1^@\paar u_2.f_2^@$. Checking sm-category axioms is straightforward. 
%\begin{lemma} The collection of all small categories and quasi-functors between them is a category \qcatcat. %Condition \eqref{qfun} holds for the above triple, and hence the latter determines a quasi-functor \frar{f;g}{\spA}{\spC}
%\end{lemma}

\subsubsection{Differentiating parameterized functions}
%====
\input{ll-figures/pdfs/getAmend-twoFig}
%====

Consider \frar{f}{\spP\timm\reals^m}{\reals^n}, where $\spP=\reals^k$ is a parameter space. Differentiating over parameters for a fixed $a\in\reals^m$, gives us an operator $\prt_p f(p,a)$ mapping parameter deltas \frar{e}{p}{p'} from $p$ into $\reals^n$-deltas from $a.f_p:=f(p,a)$ (as usual, we use symbol $p$ in two roles: as a variable running over \spP\ in $\prt_p f$ and as a fixed parameter value in other expressions). Similarly, differentiating over variables in $\reals^m$  for a fixed parameter $p\in\reals^k$, gives us an operator $\prt_a f(p,a)$ mapping deltas \frar{\del}{a}{a'} from $a$ into $\reals^n$-deltas from $a.f_p$. Diagram in \figgetam a describes the ingredients of the story as arrows. Intermediate vertical arrow from $a.e\prt_p$ has the same label as its counterpart on the left as we consider the delta $\hat \del :=\del.\prt_af(p,a)$ as acting on values in $\reals^n$, and we label the result of applying $\hat \del$ to $b\in \reals^n$ by $\hat \del$ so that different arrows from different $b$s get the same label. Similarly, two different horizontal arrows from $a.f_p$ and $a.\del\prt_a$ have the same action label too. 

An abstract delta lens formulation of the story is given by the following definition illustrated by diagram \figgetam b. 
\begin{defin}[incremental view system]\label{def:viewsys}
	Let \spS\ and \spT\ be model spaces. An {\em (incremental parametrized) view system} 	from \spS\ (the {\em source} of the view) to \spT\ (the {\em target}) is given by i) a category \spP\ of {\em parameters} (think about function/view definitions \parrd\ by objects of \spP) and ii) a quasi-functor \frar{\get}{\spP\timm\spA}{\spB}. A view system is called {\em codiscrete} if categories \spS, \spT, \spP\ are codiscrete.
\end{defin}

In the parametrized setting,  we have a differentiable function \frar{f}{P\times\reals^m}{\reals^n} with $P=\reals^k$ being the parameter space. %, and a differentiable error function \frar{\Err}{\reals^m}{\reals}, whose composition gives us differentiable  function \frar{E}{P\times\reals^m}{\reals}. 
We can convert this data into a double-indexed family of functors-as-monoid- homomorphisms  \frar{\get_{p,a}}{\DDel^m}{\DDel^n}, $p\in P, a\in \reals^m$ %, by, first, converting all Euclidean spaces into categories as described above, and then, 
by the two upper equations in \eqref{mlgetdef}: %as follows: for a given parameter $p$, parameter delta \frar{\Delp=(p'-p)}{p}{p'}, m-tuple of reals $a$ and input variables delta \frar{\Dela=(a'-a)}{a}{a'}, we define%
\footnote{as usual, by the abuse of notation we will denote variable and its fixed value by the same symbol $a$} 
%\begin{minipage}[t]{0.5\textwidth}
\begin{equation}\label{eq:mlgetdef}
\begin{array}{c}
\get_p(a)=f(p,a)
\\
\get_{p,a}(\dela)=\Dela*\nabla_af(p,a)
\\
\get_a(\Delp)=\Delp*\nabla_pf(p,a)
\end{array}
\end{equation}
%\end{minipage}
(where the last equation specifies natural transformation  $\get(\Delp)$). Thus, we have a parameterized functor or the \get-part of a dd-lens: the differencing operation is uniquely defined so that Difdif holds, and it is straightforward to check conditions \eqref{difget}.  In terms of diagram \figrcodi, we have built functors ${+}\mathsf{deltas(\pol)}$ and ${+}\dif(\pol)$.


\subsubsection{Gradient descent as an update propagation policy
	%Model spaces as metric spaces.
}
Metrics, \ie, setting a distance between values considered as an {\em error} is an important part of the story. %We will need also some metrics on differences considered as errors. 
Following \citefst, we assume that some  differentiable function \frar{\err}{\reals\times\reals}{\reals} is given, and %actions of monoid $\DDel=(\reals,+,0)$ are considered as opliftings: 
then given $a\in\reals$ and edit $\delta \in\DDel$, the result of applying $\delta$ to $a$ is an arrow \frar{\ovr{\delta}=\err(a,a')}{a}{a'}. For the multiple variables case $\reals^m$, a delta is a vector $\del=(\del_1,...,\del_m)$ acting componentwise, and the result of applying it to value $a=(a_1...a_m)$ is an arrow/distrance  \frar{\ovr{\del}=\Err(a,a')}{a}{a'} computed by summation: $\Err(a,a') :=\sum_{i\le m}\err(a_i,a'_i)=\sum_{i\le m}\err(a_i,a_i+\del_i)$.  
%considered as an arrow \frar{\ovr{\delb}}{b}{b'}
with $b=f(a)$ and $b'=f(a')$. Thus, an accurate setting would be to consider an asymmetric edit delta lens (see \cite{jr-unified} for a definition for the codiscrete case) whose model spaces are Lawvere categories (metric spaces). However, delta lenses subsume edit lenses (see \cite[sect.??]{me-jot11} for the idea and examples, and \cite{jr-unified} for formal results), and below we will work in the delta lens setting, in which deltas are pairs $(\del,\ovr{\del})$ where $\del=a'-a$ and $\ovr{\del}=\err(\del)$.  %As it was shown in \cite{jr-unified}, 

In the setting of \citefst,

For defining the \putl-part, we need a policy, and the gradient descent method gives us one. We can treat formulas in \citefst\ for computing the updated parameter $p'$ (for a given step size \eps) and updated input value $a'$ as $\putl^\upd$ and $\putl^\req$ operations mapping delta $\Del_b=b-E(p,a)$ to deltas $p'-p$ and $a'-a$ resp. (and conditions \eqref{difputupdself} (upper) and \eqref{difputreq} are automatically satisfied). We can also set $\putl^\self(\Del_b)=E(p',a') - b$ so that condition \eqref{difputupdself}(bottom) is also satisfied. Moreover, the Putget laws holds too. Thus, we have a (well-behaved) dd-lens. In terms of diagram in \figrcodi, we built functor ${+}\putl(\pol)$ and showed that the universal arrow $!=[{+}\dif(\pol), {+}\putl(\pol)]$ targets at the category of well-behaved dd-lenses as shown in the diagram.
%
%Probably, the entire construction would be more transparent and manageable (\eg, with respect to generalizations) if we consider this dd-lens as sequentially composed from two dd-lenses: \frar{\ell_\eps(f)}{\reals^m}{\reals^n} and \frar{\ell(\err)}{\reals^n}{\reals} (whose parameter space is \tcat). This elaboration is also left for future work. 

Finally, by applying the codiscretization functor, we arrive at the category of codiscrete ala-lenses, which gives us derived functor ${+}\putl0(\pol)$.   

%An Euclidean space $\reals^n$ can be seen as a category $\rcat^n$ enriched in $\niv=(\reals^n, +)$: given two tuples $a, a' \in \reals^n$, we define $\rcat^n(a,a')= (a'- a)$. A differentiable function \frar{f}{\reals^m}{\reals^n} can then be seen as a functor \frar{\get}{\rcat^m}{\rcat^n} whose object part is $f$, and the arrow part is the derivative: $\get(a'-a)=$

==> ll-sections/editSpaces.tex <==
\section{Functoriality of DPO}


\newcommand\dpo{\enma{\mathsf{DPO}}}
\newcommand\tr{\enma{\mathsf{tr}}}
\newcommand\tracecat{\catname{Trace}}
\renewcommand\span{\enma{\mathsf{Span}}}

The subject of our discussions can be formulated in a quite general way without mentioning updates etc. in terms of adhesive cats. As I am not sure do we need adhesive or weakly adhesive cats, or something of this kind, I'll call them adh cats. 
\begin{defin}[adh cats] An {\em adh} cat is a pair $C=(|C|, \nim)$ where $|C|$ is a cat called the carrier of $C$ and $\nim$ a class of morphisms such that...
	
	By an abuse of notation, we will often omit vert bars and thus symbol $C$ will mean either a cat $|C|$ or a pair $(|C|,\nim)$ depending on the context.
	\end{defin}
What we discussed today is the following construction. For any given adhcat $C$, we can build:

-- a dagger category $\span(C)$ of spans in $|C|$ whose legs are from \nim

-- a dagger category $\dpo(C)$ of DPOs as discussed 

-- a dagger opfibration \frar{\tr_C}{\dpo(C)}{\span(C)}

 For applications and just categorically, it's important to know that this construction is functorial 
 \begin{theorem}[so far conjecture]
 	Let \frar{f}{C}{D} is an adh functor between adhcats. Then it gives rise to an opfibration morphism $(f_\span, f_\dpo)$
 	\begin{diagram}[small]
 		\dpo(C) & \rTo^{f_\dpo} & \dpo(D) \\
 		\dTo<{\tr_C}  & &\dTo>{\tr_D}\\
 		\span(C) & \rTo_{f_\span} & \span(D)
 		 	\end{diagram}
 	 	\end{theorem}
  To apply the above in the context of updates, we need to  quotient everything with strong skeletality. 
  \begin{lemma}Any cat $C$ gives rise to a surj on objects full functor \frar{q_{\cong}}{C}{C_{\cong}} with $C_{\cong}$ being strongly skel., and any functor \frar{f}{C}{D} gives rise to \frar{f_{\cong}}{C_{\cong}}{D_{\cong}} so that the square commutes. (check pls)
  \end{lemma}
We need also the quotient version of the opfibration %$[\span(C)]_{\cong}$, $$ and opfibration 
\frar{[\tr_C]_{\cong}}{\dpo_{\cong}(C)}{\span_{\cong}(C)} (note that we quotient both objects of $C$ and spans so that the functor \frar{q_{\cong}}{\span(C)}{\span_{\cong}(C)} is {\bf  not} identity on objects).

Then, if all notions are properly defined, we should have
\begin{theorem}Any adh cat $C$ gives rise to  an edit space $\spE(C)$ with $\tracecat_{\spE(C)}=\span_{\cong}(C)$ etc. Moreover, an adh functor \frar{f}{C}{D} gives rise to an edit space morphism \frar{f_\spE}{\spE(C)}{\spE(D)}. Moreover, we have a functor \frar{\spE}{\catname{adhCat}}{\catname{editSp}}
\end{theorem}	
 	 	

==> ll-sections/functOfLearning-act2foss.tex <==

\subsection{Functoriality of learning algorithms in the {\em delta} lens setting: An overview}\label{sec:ddlens-1}

\renewcommand\figri{\figref{policyfun}}

In general, all lenses we will be dealing with can be uniformly described as a pair of operations \fprar{(\get, \putl)}{\spA}{\spB}{\spP} between two categories (perhaps, codiscrete) \spA, \spB. Operation \get\ is a mapping (functor or function) that maybe parametrized by a category \spP\ (perhaps, codiscrete), or be unparameterized, which is parameterization 
with a singleton category \spP. Operation \putl\ is actually a family of multivalued mappings (\ie, a tuple of families of single-valued mappings) that inverts mapping \get\ in some specified way. For example, for learners, \spA, \spB, \spP\ are sets, \get\ is a \paramed\  function, and \putl\ consists of two families of discrete operations described in \citefst: $\putl^\upd$ updates the parameter and $\putl^\req$ updates the source value thus making a request to the previous layer. Learning delta lenses is a categorification of learners, in which all spaces are categories, \get s are functors, and families $\putl^\upd$, $\putl^\req$ are functorial operations. % (\sectref{classPalne} provides more detailss). 
Lenses with amendments add one more family of functorial operations $\putl^\self$, which reflectively update deltas on the \spB\ side.


%\subsection{Learning functors over their contextual bases}
%==
%\input{ll-figures/diags/policyfun}
%\input{ll-figures/diags/policyfun-ml-triangle}
%\input{ll-figures/diags/policyfun-ml-pentagon}
%\input{ll-figures/diags/policyfun-ml-diamond}
\input{ll-figures/diags/policyfun-ml-rectangle}
%\input{ll-figures/diags/policyfun-smallTri}
The learning functor \eqref{lfunee} (see p.~\pageref{eq:lfunee})  is equipped with a constraint (obvious but implicit in \citefst) explicated in diagram \figri(a), whose nodes are sm-\cats\ and arrows are sm-functors (further we will omit the prefix sm). Objects of \psetcat\ are all small sets and arrows are all (equivalence classes of) parametrized functions (p-functions, see \sectref{pcatcat} for details). This \cat\ is equipped with an obvious functor into a big one-object sm-category \iaset\ freely generated by the class of all small sets with the (the equivalence class of the ) singleton set being the tensor unit (see \sectref{pcatcat}). Functor \minusrr\ embeds (non-fully) \paracatrr\ into \psetcat\ and forgets the Euclidean structure, hence the notation \minusrr\ ``minus structure'' (we will use this notational trick further on). Similarly, if a functor adds a structural component $X$, we denote it by a ${+} X$ symbol (note this notation for \lfunee\ below the arrow). 
%
The diagonal functor $\minusput^\codiind$ takes a leaner and forgets its \putl-components $\putl^\upd$ and $\putl^\req$,  thus arriving at \psetcat\ and commuting the upper triangle. The vertical $par'$ is just the composition of $\minusput^\codiind$ with \parname\ (similar composition with \minusrr\ is not shown). The diagram clearly shows that learners live in the  \psetcat\ universe. 



Delta learning lenses is a direct categorification of learners specified in diagram \figri(b) (we show the version for lenses with amendments). Euclidean spaces are replaced by model spaces definable by a model \trafon\ language \mtl, differentiable p-functions by \mtl-definable p-functors, and discrete operations $\putl^\codiind$s by functorial operations \putl\ s. Functor $L_\mtl$ from \eqref{mtlfun} p.~\pageref{eq:mtlfun} is synonymously denoted by $\plusx{\mtl}\putl$.  The big one-object sm-category \iacat\ is specified in \sectref{pcatcat}. We thus have a structurally similar diagram over \pcatcat--- the foundation of the ala-lens building. %
%\footnote{\label{fnote:partcateg}
In the next section, we consider the path from (a) to (b) in more detail. 
%On the path from \figri(a) to (b), there are two intermediate points of partial categorification described in the TR \cite{myTR-foss20}.}

%Figure~\ref{fig:classPlane} shows the categorification path in more detail.  






 




==> ll-sections/horiz-compose-new.tex <==
\section{Category of Asymmetric \Parrd\ Lenses with Amendment (APA-Lenses)}\label{sec:lego-spans2lens}

%\input{ll-sections/modSpaces-short}
%\input{ll-sections/aa-lensDef-semiDiscrete}
\newcommand\figari{\figref{apa-arity}} %arity
\newcommand\defri{\defref{def:aalens-arity}}


\subsection{Apa-lenses}
Given a category \spC, its collection of objects is denoted by $|\spC|$.
\begin{defin}[Model spaces]
	A {\em model space} is a small skeletal category whose objects and arrows are called, resp., {\em models} and {\em deltas} (or {\em updates}). %with compatibility relation \Kupd. 
\end{defin}
\vspace{-0.5cm}
\begin{defin}[apa-lenses]% cf. \cite{me-fase18}]\label{def:aalens-arity}
	Let \spS\ and \spT\ be model spaces. An {\em apa-lens%indexed asymmetric lens  with amendment (indexed aa-lens)
	} from \spS\ (the {\em source} of the lens) to \spT\ (the {\em target}) is given by the following three components a-c.
 \begin{enumerate}[label={\bf  \alph*)}, %Step 
	%\arabic{enumi}., ref=Step \arabic{enumi},% 
	wide=0pt]
\item[{\bf a) Parameters:}] A category \spP\ of {\em parameters} (think about function/view definitions \parrd\ by objects of \spP). We denote objects of \spP\ by small letters $p,p',..$ rather than capital ones to avoid confusion with \citefst, in which capital $P$ is used for the entire parameter set.  

\item[{\bf b) Gets:}] A functor \frar{\get}{\spP}{[\spS,\spT]}, where $[\spS,\spT]$ is the category of functors from \spS\ to \spT\ and their natural transformations. We will write $\get(p,\_)$ or $\get_p$ or (or even shorter $p^*$) for the functor \frar{\get(p)}{\spS}{\spT} (read ``get \spT-views of \spS''). Given a parameter delta \frar{e}{p}{p'} and a source model $S\in|\spS|$, the model delta \frar{\get(e)}{\get_p(S)}{\get_{p'}(S)} will be denoted in formulas by $e.\get_S$ (rather than $\get_e(S)$) to smoothly use the dot notation for substitution; i n diagrams, we write $e_S$.

	\item[{\bf c) Puts:}] A family of operations $\putps$ indexed by pairs $(p\in P, S\in\xob{\spS})$. %(read ``put the view update back'') 
	Each operation in the family takes a delta \frar{v}{\get_p(S)}{T'} as its input, and outputs three deltas 
	$\comprfam{\putps^{\x}(v)}%
		            {\x\in\{\req,\upd,\self\}}$ 
    specified below (names \req\ and \upd\ are chosen to match the terminology in \citefst).
	%Given a pair $(p,S)$, operation $\putpa$ takes  an update \frar{v}{p^*(S)}{T'} as its input and outputs three arrows c1-c3 as specified below and illustrated by diagram in \figref{fig:aalens-arity}
\begin{enumerate}[label={\bf  \alph*)}, %Step 
	%\arabic{enumi}., ref=Step \arabic{enumi},% 
	wide=5pt]
\item[{\bf c1)}%$\putl_\req$:
]  \frar{u=\putps^\indb(v)}{S}{S'} is a {\em source} update (read ``put the view update $v$ back'')
	\item[{\bf c2) }%$\putl_\upd$:
]  \frar{e=\putps^\upd(v)}{p}{p'} 	is a parameter update or transformation {\em evolution}.
\item[{\bf c3) }%$\putl_\self$:
]
	\frar{\amex{v}=\putps^{\self}(v)}{T'}{T^@} is an {\em amendment} to the original update, %$\putpa_{\self}(v)$ or }
	%such that $v;\amex{v}=\get(u')$. 
\end{enumerate}
\end{enumerate}
			A lens is called {\em codiscrete} if categories \spS, \spT, \spP\ are codiscrete.
\end{defin}

%  notation4diags explained
%\input{ll-sections/notation4diags}
%\input{ll-figures/pdfs/aalens-arity}
Diagram in \figari\ shows how these operations are interrelated. The upper part shows an arrow \frar{e}{p}{p'} in category \spP\ and two corresponding functors from \spS\ to \spT. The lower part is to be seen as a 3D-prism with visible front $ST_{p'}T^@S'$ and upper $ST_pT_{p'}$ faces, the bottom and  back side faces are invisible and the \corring\ arrows are dashed. The prism denotes an algebraic term (workflow): given elements are shown with black fill and white font, while derived elements are blue (recalls being mechanically computed) and blank (double-body arrows are considered to be blank). The two pairs of arrows originating from $S$ and $S'$ are not blank because they denote pairs of nodes (the UML says {\em links}) rather than mappings/deltas between nodes ---we explained this notation in the previous section (where derived arrows were dashed but now we use dashing for 3D-drawing. Link-arrows now have bulleted rather than bar tails like in $\mapsto$ due to limitations of Powerpoint used for building the diagram).
As in diagram \figri(a), we again use numeric names for links to convey the order of operations, but now we write $i{:}p$ rather than $i{:}\get_p$ to ease reading (below we will diagrams that have more such arrows). By the same reason, we omit numeric scripts near vertical and diagonal arrows (deltas), and label the deltas realizing natural transformations very briefly, \eg, $e_S$ for the full name  $\get(e,S)$-- the latter will also be written in formulas as $\get_S(e)$ or $e.\get_S$. Two callouts near $1{:}p$ and $E_S$ recall these notational tricks. 
%
%}{\get(p,S)}{\get(p',S)})  . 
% For example, link labelled $1{:}\get_p$ denotes application of functor $\get_p$ to object $S$ that results in an object $T_p=\get_p(S)$.%
%\footnote{Notation with colon is suggested by UML: $1$ ia the name of the link whereas $\get_p$ is its type. In a refined setting with the names \spS, \spT, $\get_p$ organized into a syntactic category, the Grothendieck construction can be seen here, but we don't need this in the present paper.}    
%In the other three link-arrows we write $i{:}p$ rather than $i{:}\get_p$ to ease reading (below we will have more such arrows). 

\input{ll-figures/pdfs/aalens-arity}
%\spT-arrows (deltas rather than links) realizing natural transformations (such as \frar{\get(e,S)}{\get(p,S)}{\get(p',S)}) are labelled as $ij{:}e_S$ where $i,j$ are indexes of the \corring\ links to the source and target of $\get(e,S)$. %Similarly to diagram \figri(a), link indexes convey the order of operations from which the entire workflow is built, but now we skip numeric indexes on updates to ease reading (below we will have more such arrows). 
The label of invoking operation \putl\ in the third step of the scenario is omitted, but instead, the equational definitions of deltas $e,u,v^@$ are written (note the three callouts near them). 
%
%We begin with 1) computing $T_p$, then 2) apply delta $v$ and compute three deltas $e=\putps^\upd(v)$, $u=\putps^\req(v)$, and $v^@=\putps^\self(v)$ (upper indexes near puts are not shown in the diagram; %) as Powerpoint doesn't allow having upper and lower indexing together; 
%subscripting $e$, $u$, $v^@$ with 2 would make notation heavy and we omitted it). 
The diagram also shows four derived deltas forming the right back face of the prism: 
$v_p=\get_p(u)$, $v_{p'}=\get_{p'}(u)$, and two matching them deltas $e_S=\get_S(e)$, $e_{S'}=\get_{S'}(e)$, which together form a commutative square due to naturality of $\get(e)$ (note the common target of $e_{S'}$ and $v_{p'}$, \ie, $S'.\get_{p'}$, shown as a rounded square). Finally, the diagram also shows coincidence of this ``square'' object and the target $T^@$ of the amendment $v^@$ 
(the inner circle), which is a special requirement (a constraint) that does not  hold automatically and to be specially postulated (the red filler in-between the square and the circle refers to this constraint). Thus, the arity schema of put operations includes the following \putgeto\ equations:
% Specifically, the diagram shows that three derived objects, $T^@$ (the target of $v^@$ shown a circle node), the target of $v_{p'}=\get(p',u)$   (shown as a rounded square node) and the target of $e_{S'}$ (the same square node), coincide. While the coincidence of the two square nodes (and the commutativity of the right back face of the prism) follow from the naturality of $\get(e)$, the coincidence of the common square and the circle nodes is a special requirements specified by the following equation 
%\begin{equation}\label{eq:putget0}

\noindent \begin{tabular}{l@{\quad}l}
	%\\[0.5ex] 
	\lawnamebr{Putget}{$_0$
	} & %$_{~~~~~~}$
 $
 \codd(v.\putps^\self) \mbox{ \textcolor{red}{=} }
    \codd(v.\putps^\req.\get_{p'}) 
    \mbox{ \textcolor{blue}{=} } \codd(v.\putps^\upd.\get_{S'})
    %\mbox{ where } \frar{e=v.\putps^\upd}{p}{p'}
 $
	\\ [\lawgap]
\end{tabular}
%\end{equation}
\\
where the left equality is a constraint (red) %included into the arity schema 
while the right one is automatic (blue). The ``co-discreteness'' index 0 recalls that the constraint equates objects (nodes) rather than arrows. Equating arrows is the subject of a special Putget law stated below together with two other requirements to apa-lenses, which would allow MDE practitioners  to call them  ``well-behaved''. %Weak Putget asserts commutativity of the triangles in the right back face (it's enough to require one, \eg, the upper as shown in the diagram with the red [=], the other one then follows --- note the blue [=]). Strong Putget or just Putget requires delta $e_S$ to be an identity and, moreover, the equality $v;\amex{v}=v.\putps^\req.\get_{p'}$
% --- the latter are discussed below.  
%note the interplay between red and blue in the diagram). The constraint is named Putget$_0$ and is a prerequisite for an important delta lens law called Putget, which requires the commutativity of the triangles in the right back face of the prism (it'd be enough to require one, then the other is derived -- note a red and a blue labels [=] in the diagram, which do not belong the arity schema) --- it will formally be stated below. % is a special and important requirement called the Putget law (see the definition below). 
% =========  the law piece begins
%\input{ll-sections/aalens-wblaws}
\renewcommand\ppgB{\ensuremath{\putl^B}}
\renewcommand\ppgB{\ensuremath{\putps}}
\begin{defin}[Well-behavedness]\label{def:wbalens}{\em 
	An apa-lens is called {\em well-behaved (wb)} if it satisfies the following three laws specified by equations to hold for all $p\in P$, $S\in\xob{\spS}$ and \frar{v}{T_p}{T'} where $T_p$ denotes $\get_p(S)$:}
	%, and \frar{u}{B}{B'}:
	\\[1ex]
	\lawgap=1 ex
	\noindent \begin{tabular}{l@{\quad}l}
		%		\lawnamebr{Hippocr1}{
		%        \frar{u}{B}{B'}
		%		} & 
		%		if $\get(B) = \get(B')$, then $\get(u) = \id_{\get(B)}$
		%		\\ [\lawgap]\lawnamebr{Hippocr2}{
		%		\frar{v}{\get(B)}{A'}
		%		}	& 
		%			if $A'=\get{B}$, then $\ppgB_\indb(v) = \id_B$,   $\ppgB_\inda(v)=\id_{\get(B)}$
		%		%$\ppgB_{\indb}(\id_{\get(B)})=\id_{B}$
		%		\\
		%		& \parbox{15em}{\textcolor{red}{the two laws above are just a reminder of a path that was rejected} }
		%		\\
		\lawnamebr{Stability}{
		}	& \mbox{\em 
		if $v=\id_{T_p}$ %where $B=p^*(S)$, 
		then all three propagated updates 
		%\\  & 
		$e,u,\amex{v}$ are identities:} 
		\\
		& $\putps^\upd(\id_{T_p})=\id_p$, \quad%
		$\putps^\req(\id_{T_p}) = \id_S$, \quad%    
		$\putps^\self(\id_{T_p})=\id_{T_p}$
%		%			%\\  [\lawgap] \lawnamebr{\reflectzero}{
%		%			%			} &	
%		%			%			if $v=\get(u)$ for some \frar{u}{A}{A'}, then $\amex{v}=\id_{B'}$
%		%			\\  [\lawgap] \lawnamebr{K{-}amendment}{
%		%			} &	
%		%			$(v, \amex{v})\in \Kupd_{B'}$ %for all $u_i$ 
%		\\  [\lawgap] \lawnamebr{Closure1}{
%		} &
%		$\putUL{\x}{p,S}(v;\amex{v}) = \putUL{\x}{p,S}(v) $
%		\mbox{\em  where $v^@$ denotes $\putps^\self(v)$
%		and $\x\inn\{\upd,\req\}$ }
%			\\  [\lawgap] \lawnamebr{Closure2}{
%	} &
%	$\putUL{\self}{p,S}(v;\amex{v}) = \id_{T^@}$ %\putUL{\x}{p,S}(v) $
%	%\mbox{\em  where $v^@$ denotes $\putps^\self(v)$
%	%	and $\x\inn\{\upd,\req\}$ }
%%		\\ [\lawgap] \lawnamebr{weakPutget}{
%%		} & %$_{~~~~~~}$
%%		$v;\amex{v}=(v.\putps^\upd.\get_S)\,;\,(v.\putps^\req.\get_{p'})$, 
%%		%			%
%%		%			\mbox{\em or, equivalently}, 
%%		%			\\ [\lawgap] \lawnamebr{Putget}{'
%%		%		}&$v;\amex{v}=(v.\putps^\req.\get_{p})\,;\,(v.\putps^\upd.\get_{S'})$
		\\ [\lawgap] \lawnamebr{Putget}{
		} & %$_{~~~~~~}$
	\mbox{\em  
		$v.\putUL{\upd}{p,S}.\get_S= \id_{T_p}$
		and 
		$v;\amex{v}= %(v.\putps^\upd.\get_S)\,;\,(
		v.\putps^\req.\get_{p'}$,
		 where $v^@$ denotes $\putps^\self(v)$} 
	 	\\ [\lawgap]
				\lawnamebr{Hippocr}{
		}	& \mbox{\em 
			if $u.\get_p=v$ for some \frar{u}{S}{S'}, 
			then $v^@=\id_{T'}$
	                       } 
	\end{tabular} \\[10pt] 
	%\rule{0mm}{0mm}\qed
	%When we will need to refer to compliance to these laws separately, we will 
{\em A lens is {\em stable} if it satisfies Stability, and an {\em SPg-lens} if it satisfies Stability and Putget.  
%	
%	A target delta $v$, is {\em closed} if $v^@=\id_{T'}$; an apa-lens is {\em closed} if each target delta is closed. %or {\em spgc-lens} if it also satisfies Putget and Closure resp. 
}
\end{defin}  %}
\begin{remark}{\em 
%a) Condition Closure only requires full amendment deltas $v;v^@$ to be closed, which is  much weaker than the defining condition of closed lens requiring  {\em each} delta to be closed. %as to be fulfilled in closed lenses. 
a) Stability says that the lens does nothing if nothing happens on the target side (no trigger--no action, hence, the name of the law) 

b) Putget requires the goal of update propagation is to be achieved after the propagation act is finished. 
%\begin{remark}\label{rema:putget}%\zd{to be reworked}
%	The Putget law 
It may seem a notational trick rather than a law as operation $\putps^\req$  provides delta $u$, and functor $\get_{p'}$ sends it to a delta  $\get_{p'}(u)$ targeting at some model $T^@$ anyway. However, in general, there are many possible deltas between models $T'$ and $T^@$, whereas the Putget law b1) states the existence of some special delta \frar{v^@}{T}{T^@} and, moreover, b2) requires equations (\putget) to hold. Note also that Putget implies commutativity of the lower triangle in the right back face as the upper one is commutative by Putget. %much more certainty about $T''$ and precisely specifies the relationship between $T'$ and $T''$, namely, it says that they are related by a specified update $\amex{v}$.

c) Hippocraticness%
\footnote{the term introduced in Bx by Perdita Stevens \cite{stevens-sosym10} for a family of requirements sharing a common intention ``do not do harm''}
prohibits amending delta $v$ if consistency can be achieved for $v$ without amendment. Note that equalities $\putUL{\upd}{p,S}(v)=p$ nor $\putUL{\req}{p,S}(v)=u$ are not required: the lens can improve consistency by changing $p$ and $u$ but changing $v$ is disallowed.  
}\end{remark}

%==== the law pieces ends 
%=== Examples begin

\begin{example}[Identity lenses]\label{ex:idlens} %$\mathcal{id}$
	Any skeletal category \spA\ gives rise to an apa-lens $\idl_\spA$ with the following components. The source and target spaces are equal to \spA, and the parameter space is \tcat\ (a category with a single object * and a single arrow $\id_*)$. Functor $\get_{*}$ is the identity functor and all puts are identities. Obviously, this lens is wb.
\end{example}
\begin{example}[Iso-lenses]\label{ex:isolens}
	Let \frar{\iota}{\spA}{\spB} be an isomorphism between model spaces. It gives rise to a simple wb apa-lens \frar{\ell(\iota)}{\spA}{\spB} with $\spP^{\ell(\iota)}=\tcat$ as follows. Given any $A$ in \spA and \frar{v}{\iota(A)}{B'} in \spB, we define $\putl^{\ell(\iota).\req}_{*,A}(v) = \iota^{-1}(v)$ and the two other put operations send $v$ to identities. 
\end{example}
\begin{example}[Bx lenses]\label{ex:bxlens} Examples of SPg and wb aa-lenses can be found in \cite[ext.version]{me-fase18}: they all can be considered as apa-lenses with a trivial parameter space \tcat. 
\end{example}
\begin{example}[Learners (borrowed from \citefst\ but rearranged)]\label{ex:mlasbx}
	Let \frar{\err(x,y)}{\Reals\timm\Reals}{\Reals} be a differentiable  {\em error} function such that \frar{\prtfrac{\err}{x}(x_0,-)}{\Reals}{\Reals} is invertible for any given $x_0$. For an $n$-dimensional Euclidean space $\reals^n$, we define the {\em total} error function \frar{\Err}{\rreals}{\reals} by $\Err(a,a')=\sum_{i\le n}\err(a_i, a'_i)$. This converts space $\reals^n$ into a category (Lawvere's metric space) \brealsx{n}. 
	%
	A {\em \parrd\ function} from \realsx{m} to \realsx{n} is a differentiable function \frar{I}{\realsx{k}\timm\realsx{m}}{\realsx{n}} (and hence a functor \frar{I}{\brealsx{k}\timm\brealsx{m}}{\brealsx{n}}). 
	
	It is shown in \citefst\ that, given a {\em step size} $\eps\in(0,\infty)$,  any parameterized function \frar{I}{\realsx{m}}{\realsx{n}} gives rise to an ap-lens \frar{\ell_\eps(I)}{\brealsx{m}}{\brealsx{n}} called in \citefst\ a {\em learner}.%
	%\footnote{Warning: our models $S$ (for source) and $T'$ (target) are theirs $a$ and $b$ rather than $b'$.}
	\footnote{Moreover, they show the functoriality of the construction.} To make it an apa-lens, we need to add amendments by defining $T^@=b'=I(p',a')$; then Putget trivially holds as there is only one arrow (distance/error) between any two objects. 
	
	%Any learner $\ell_\eps(I)$ can be made stable if we direct it to do nothing when $\Err(I(p,a),b)=0$. 
	Paper \citefjbx\ says that neither of the laws necessarily holds in the anarchic world of ML. % Putget nor Hippocraticness 
\end{example}

%==== the end of example

\input{ll-sections/apacat}


\endinput 




%In \citefst, Fong \etal\ prove that the category of codiscrete apa-lenses is sm by showing that the required monoidal structure is borrowed from Cartesian sm-category $(\setcat, \times)$. We can do the same with \catcat\ instead of \setcat.




\endinput
We need to prove associativity: $(\ekk;\ell);\emm=\ekk;(\ell;\emm)$ for any three consecutive lenses 
\frar{\ekk}{\spA}{\spB}, \frar{\ell}{\spB}{\spC}, \frar{\emm}{\spC}{\spD} with \ekk\ and $\ell$ as shown in \figkl, and \emm\ having the parameter space \spR.   
We easily have associativity for the get part of the construction: $(\spP\timm\spQ)\timm\spR\cong\spP\timm(\spQ\timm\spR)$ (to be identified for equivalence classes), and $(\get^\ekk_p;\get^\ell_q);\get^\emm_r=\get^\ekk_p;(\get^\ell_q;\get^\emm_r)$.

\clearpage
Associativity of puts is more involved. 
Suppose that we extended the diagram in \figkl\ with lens \emm\ data on the right, \ie, with a triangle prism (say, purple) whose right face is a square $D_{pqr}D_{r'}D^@D'_r$ with diagonal \frar{\ome;\ome^@}{D_{pqr}}{D^@} where $r\in\spR$ is a parameter, $D_{pqr}=\get^\emm_r(C_{pq}$ and \frar{\ome}{D_{pqr}}{D'} is an arbitrary delta to be propagated to $\spP$ and \spA, and reflected as amendment $\ome^@=\putxyz{\emm.\self}{r}{C_{pq}}(\ome)$. 
We begin with rewriting \eqref{kldef2} by 
substituting the term for $v$ from \eqref{kldef1} 
\begin{eqnarray}\label{eqna:kldef2}
	% row 5
		\frar{w.\putl^{\klbr.\upd}_{pq,A} &= &%
		((w.\putxy{q}{B_p}^{\ell.\req}).\putxy{p}{A}^{\ekk.\upd}}{p}{p'})
	\paar (w.\putl^{\ell.\upd}_{q,B_p}{:}~q\rightarrow q') \label{eq:eqna4}
	\\
	\frar{w.\putl^{\klbr.\req}_{pq,A}&=&w.\putxy{q}{B}^{\ell.\req}.\putxy{p}{A}^{\ekk.\req}}{A}{A'}, \label{eq:eqna5}
	\\
	% \mbox{ and }
	\frar{w.\putl^{\klbr.\self}_{pq,A}&=&(w.\putl^{\ell.\self});(w.\putl^{\ell.\req}_{q,B}.%
		        \putl^{\ekk.\self}_{p,A}.\get^{\ell}_{q'})
	}{C'}{C^{@}}\rightarrow C^{@@} \label{eq:eqna6}
\end{eqnarray}
which shows the interplay between different puts. Now we do the same for the lens \klbr;\emm\ (recall that pairs $(x,y)$ can also be denoted by $x\paar y$. 
\begin{eqnarray}   %\label{eqna:klm-proof}
\ome.\putl^{\klbr;\emm.\upd}_{(pq)r,A}
&=& % row 7
(\ome.\putl^{\emm.\req}_{r,C}.\putl^{\kl.\upd}_{pq,A}{:}~pq\rightarrow p'q')
\paarrx{(a)}
 (\ome.\putl^{\emm.\upd}_{r,C}{:}~r\rightarrow r')
\mbox{~~~~~by \eqref{eqna4}}
\\ &=& % row 8
\left((\ome.\putl^{\emm.\req}_{r,C}.\putl^{\ell.\req}_{q,B}).\putl^{\ekk.\upd}_{p,A} %
\right)\paarrx{(a1)}\left(
\ome.\putl^{\emm.\req}_{r,C}.\putl^{\ell.\upd}_{q,B}
\paarrx{(a)} \ldots\right)
%\ome.\putl^{\emm.\upd}_{r,C} 
\mbox{~~by \eqref{eqna4}\paar\ same}
\\ &=& % row 9
\ome.\putl^{\lmbr.\req}_{qr,B}.\putl^{\ekk.\upd}_{p,A}
\paarr 
\ome.\putl^{\lmbr.\upd}_{qr,B}
\mbox{~~~~by \eqref{eqna5} \paarr\ by \eqref{eqna4}}
\\ &=& % row 10
\ome.\putl^{\ekk;\lmbr.\upd}_{p(qr),A}
\mbox{~~~~by \eqref{eqna4}}
\end{eqnarray}
Associativity of $\putl^{\ekk;\ell;\emm.\req}_{pqr,A}$ and $\putl^{\ekk;\ell;\emm.\self}_{pqr,A}$ can be proved in a similar manner (using sequential associativity rather than monoidal associativity above)  

\endinput


We also have %$w=\putxyz{\emm.\req}{}{}$
$w=\putxyz{\emm.\req}{r}{C_{pq}}(\ome)$ and 
$\frar{\eps=\putxyz{\emm.\upd}{r}{C_{pq}}(\ome)}{r}{r'}$. 
Then we extend the purple prism with the required fill-in arrows produced by functors $\get^\mu_r$ and $\get^\mu_{r'}$ as required. 



, \eg, the full diagonal on the right face will be %$\ome;\ome^@;\get^\mu_{r'}(w^{\ekk;\ell.@})=
$\ome;\ome^@; $



\endinput
In contrast to the general lens case, a wb a-lens features \lawname{\reflectzero} --- a sort of a self-Hippocratic law regulating the necessity of amendments: the latter is not allowed as soon as consistency can be restored without amendment. Another distinction is inclusion of an invertibility law \lawname{PutGet} into the definition of well-behavedness: 
 %due to historical traditions. %Subsequent results will also provide some justification for this. 
\lawname{PutGet}{} together with \lawname{Reflect2} provide (weak) invertibility: $\putl^B_\indb(\get(\putl^B_\indb(v)))=\putl^B_\indb(v)$.   
\lawname{Reflect3} is omitted as it is implied by \lawname{Reflect0} and \lawname{PutGet}.  

Any a-lens $\ebb^{\preccurlyeq} =(\spaA,\spaB,\get, \putl)$ gives rise to a binary symmetric lens $\ebb$. Its carrier consists of model spaces $\spaA$ and $\spT$, for which we assume $\Kupd$ and $\Kdisj{}$ to be defined such that the spaces are well-behaved, cf.\ Def.~\ref{def:wbspace}. The set of corrs of a pair $(A,B)\in \xob{\spS}\times \xob{\spT}$ is the singleton $\{\etosing{(A,B)}\}$ with $\prt_\spS\etosing{(A,B)}=A$ and $\prt_\spT\etosing{(A,B)}=B$, 
%the boundary mappings are the projections, 
\zdmodtok{realignment is thus trivial,}{}{ALIGH} and consistent corrs are exactly those \etosing{(A,B)}, for which $A = \get(B)$.

For a consistent corr $\etosing{B}={(\get(B), B)}$, we need to define six operations $\ebb.\ppghB_{\_\_}$. Below we will write the upper index as $B$ rather than $\hat B$ to ease the notation. For a  view update \frar{v}{A}{A'} and the corr \etosing{B}, we define 
 $$
\ppgB_{\spS\spT}(v)=\putl^B_\indb(v){:}\, B\to B'', \;
%
\ppgB_{\spS\spS}(v)=\putl^B_\inda(v){:}\, A'\to A'', \;
% \mbox{ and }
\ppgB_{\spS\star}(v)=\etosing{B''}
$$
 The condition $A''=\get(B'')$ for $\ebb^\preccurlyeq$ means that \etosing{B''} is again a consistent corr with the desired boundaries. For a base update \frar{u}{B}{B'} and the corr \etosing{B}, we define
$$\ppgB_{\spT\spS}(u)=\get(u),\;
\ppgB_{\spT\spT}(u)=\id_{B'},\; %and
\ppgB_{\spT\star}(u)=\etosing{B'}
$$ Functoriality of $\get$ yields consistency of $\widehat{B'}$.

\begin{defin}[Very well-behaved a-lenses] \label{def:putput_a}
		A wb a-lens is called {\em very well behaved (very wb)}, if the \corring\ binary symmetric lens is such.  %additionally fulfills \lawnamebr{PutPut}, 
		cf.  Def.~\ref{def:putput}.
Of course, this definition restricts the behaviour only for the $\putl$-part of the a-lens (hence the name of the law), since functor $\get$ is compositional anyway. \qed
\end{defin}

\begin{lemma}\label{lemma:asymm_symm} Let $\ebb^\preccurlyeq$ be a (very) wb a-lens and $\ebb$ the corresponding symmetric lens. Then all base updates of $\ebb$ are closed, and $\ebb$ is (very) wb and invertible. 
 \end{lemma}
 \begin{proof}
 Base updates are closed by the definition of $\ppg_{\spT\spT}$. Well-behavedness follows from wb-ness of $\ebb^\preccurlyeq$. Invertibility has to be proved in two directions: $\ppg_{\spaB\spaA};\ppg_{\spaA\spaB};\ppg_{\spaB\spaA} = \ppg_{\spaB\spaA}$ follows from \lawnamebr{PutGet}{} and \lawnamebr{Reflect0}, the other direction follows from \lawnamebr{PutGet}{} and \lawnamebr{Reflect2}, see the remark after Def.\ref{def:wbalens}. The ''vwb''-implication follows directly from Def.\ref{def:putput_a}. 
 \qed
 \end{proof}
\begin{remark}[A-lenses as view transformation engines]\newpii{
	In terms of Varr\'o et al \cite{dvarro-models18}, a wb a-lens can be seen as an abstract algebraic model of a bidirectional view transformation engine. This engine is assumed to be a) consistent: it is a basic lens law that propagation must always produce a consistent corr, b) incremental, as lenses propagate changes rather than create the target models from scratch, c) validating, as the result of propagation is always assumed to satisfy the target metamodel constraints (either by considering the entire model space to be only populated by valid models, or by introducing a subclass of valid models and require the result of the propagation to get into that subclass). Reactiveness, \ie, whether the engine executes on-demand or in response to changes, is beyond the lens \fwk. To address this and similar concerns, we need a richer \fwk\ of lenses augmented with organizational structure introduced in \cite{me-jss15,me-grand17}. }{1}{-15em}
\end{remark}

  \begin{theorem}[Lenses from Spans]\label{thm:LensesFromSpans} An $n$-ary span of (very) wb asymmetric lenses $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$, $i=1..n$ with a common base \spaB\ of all $\ebb_i^{\preccurlyeq}$ gives rise to a (very) wb symmetric lens denoted by $\Sigma_{i=1.. n}^\spT\ebb_i^{\preccurlyeq}$. 
\end{theorem}
\begin{proof}
An $n$-ary span of a-lenses $\ebb_i^{\preccurlyeq}$ (all of them interpreted as symmetric lenses $\ebb_i$ as explained above) is a construct equivalent to the star-composition of Def.~\ref{def:star-comp}.3, in which lens $\ekk=\idlensnb$ (cf. Ex.~\ref{ex:idLens}) and peripheral lenses are lenses $\ebb_i$. The junction condition is satisfied as all base updates are $\ebb_i$-closed for all $i$ by Lemma \ref{lemma:asymm_symm}, and also trivially closed for any identity lens. The theorem thus follows from Theorem~\ref{th:star-comp}. The ``very wb''-part follows directly from Def.~\ref{def:putput_a}. Note that a corr in $\Corrx{\Sigma_{i=1.. n}^\spT\ebb_i^{\preccurlyeq}}$ 
 is nothing but a single model $B\in\xob{\spaB}$ with boundaries being the respective $\get_i$-images.
\end{proof}
The theorem shows that combining a-lenses in this way yields an $n$-ary symmetric lens, whose properties can automatically be inferred from the binary a-lenses.
\input{figures/pdfs/mergedMetamultimod-uml}

\exIntro. Figure~\ref{fig:mergedMetamod-uml} shows a metamodel $M^+$ obtained by merging the three metamodels $M_{1,2,3}$ from \figri\ without loss and duplication of information. In addition, for persons and companies, the identifiers of their  original model spaces can be traced back via attribute ''spaces'' 
(\Commute-objects are known to appear in space $\spS_3$ and hence do not need such an attribute). As shown in \cite{me-ecmfa17}, any consistent multimodel $(A_1...A_n, R)$ can be merged into a comprehensive model $A^+$ instantiating $M^+$. Let 
$\spT$ be the space of such together with their comprehensive updates \frar{u^+}{A^+}{A'^+}. 

For a given $i\le 3$, we can define the following a-lens $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$:
$\get_i$ takes update $u^+$ as above and outputs its restriction to the model containing only objects recorded in space $\spS_i$. Operation $\putl_i$ takes an update \frar{v_i}{A_i}{A'_i} and first propagates it to all directions as discussed in \sectref{sec:example}, then merges these propagated local updates into a comprehensive  \spaB-update between comprehensive models. This yields a span of a-lenses that implements the same \syncon\ behaviour as the symmetric lens discussed in \sectref{sec:example}.

\noindent {\em\bf  From (symmetric) lenses to spans of a-lenses.} There is also a backward transformation of (symmetric) lenses to spans of a-lenses. Let $\ell=(\mspaA, \ppg)$ be a (very) wb lens. It gives rise to the following span of (very) wb a-lenses $\ell_i^\preccurlyeq=(\prtbf_i(\mspaA),\spaB,\get_i, \putl_i)$   
where space $\spaB$ has objects $(A_1\ldots A_n,R)$ with $R\in \Corrx{A_1...A_n}$ a consistent corr, and arrows are the update tuples of $\mspA$. Functors $\get_i:\spaB\to \spaA_i$ are projection functors. Given $B = (\tupleAWOB, R)$ and local update \frar{u_i}{A_i}{A'_i}, let

%\noindent 
\frar{\putl^B_{i\indb}(u_i)\eqdef(u_1',..,u'_{i-1}, (u_i;u_i'), u'_{i+1},..,u_n')}
{(A_1... A_n,R)}{(A''_1... A''_n,R'')}
\\[1ex] 
where $u_j' \eqdef \ppg^R_{ij}(u_i)$ (all $j$) and $R'' = \ppg_{i\star}^R(u_i)$. Finally, $\putl^B_{i\inda}(v_i)\eqdef\ppg^R_{ii}(v_i)$, \ie, 
$v_i^{@B}=v_i^{@R}$. 
Validity of \zdmodtok{\lawname{Hippocr1-2}}{\lawname{Stability}}{}, \lawname{Reflect0-2}, \lawname{PutGet} and \kputputlaw\ directly follows from the above definitions. This yields 
\begin{theorem}\label{theo:lens2span}
Let $\ell = (\mspA, \ppg)$ be a (very) wb symmetric lens. Then the multi-span 
\[(\ell_i^\preccurlyeq=(\prtbf_i(\mspaA),\spaB,\get_i, \putl_i) \mid i=1..n)\]
of (very) wb a-lenses (where \spT\ is defined as specified above) has the same synchronisation behaviour w.r.t.\ model spaces $(\prtbf_i(\mspaA)\mid i=1..n)$.  
\qed
\end{theorem}

\newpii{
An open question is whether the span-to-lens transformation in Thm.\ref{thm:LensesFromSpans} and the lens-to-span transformation of Thm.~\ref{theo:lens2span} are mutually inverse. It is easy to see that the chain 
\begin{equation}\label{eq:lens2span2lens}
\mbox{symmetric lens $\rightarrow$ wide span $\rightarrow$ symmetric lens} 
\end{equation}
results in a lens isomorphic to the initial one, but the chain 
\begin{equation}
\mbox{wide span $\rightarrow$ symmetric lens $\rightarrow$ wide span} 
\end{equation}
ends with a different span as the first transformation above loses information about updates in the head of the span. 
 The results for the binary case in \cite{jr-jot17} show that the two spans can only be shown to be equivalent modulo certain equivalence relation, and an equivalence relation between lenses is also needed to tune all constructs into harmony. These equivalences may be different for our multiary lenses with amendments, and we leave this important question for future research.  
}{1}{-17em}
 \endinput
 
%============= Old Version ========= 
 \begin{theorem}[Lenses from Spans]\label{thm:LensesFromSpans} An $n$-ary span of wb a-lenses $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$, $i=1..n$ (note the common base \spaB\ of all $\ebb_i$) gives rise to a wb  (symmetric) lens $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$.
% 	
  	Moreover, $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$ is invertible as soon as the span satisfies the following condition%
 	\footnote{Found for the binary case by Bob Rosebrugh \cite{bob-invert}}: 
% 	$$
% 	\putl^B_{\indb i}
% 	$$
$\PP^B_i=\PP^B_j$ for all $B\in\xob{\spaB}$ and $i,j\le n$, where for given $B$ and $i$,  $\PP^B_i$ is the inverse image of 
$\xarr{\spaB}(\get_i(B),\_)$, \ie,  the set $\compr{\putl^B_{\indb i}(v_i)}{\frar{v_i}{\get_i(B)}{\_}}$. %, then $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$ is invertible.
\end{theorem}
\shortlong{}{%}
\begin{proof}
An $n$-ary span of a-lenses $\ebb_i^{\preccurlyeq}$ (all of them interpreted as symmetric lenses $\ebb_i$ as explained above) is a construct equivalent%
\footnote{To make it precise, we need to introduce a simple notion of lens equivalence, which identify lenses with the same propagation behavior but, perhaps, different sets of corrs -- see. \eg, \cite{jr-jot17}} to the star-composition of Def.~\ref{def:star-comp}, in which lens $\ekk=\idlensna$ and peripheral lenses are lenses $\ebb_i$. The junction condition is satisfied as all base updates are $\ebb_i$-closed for all $i$ by Lemma \ref{lemma:asymm_symm}, and also trivially closed for any identity lens. The theorem thus follows from Theorem~\ref{th:star-comp}. Note that a corr in $\xstar{(\Sigma_{i=1}^n\ebb_i^{\preccurlyeq})}$ 
 is nothing but a single model $B\in\xob{\spaB}$ with boundaries the respective $\get_i$-images. \qed
 \end{proof} 
}
For the backward transformation of lenses to spans of a-lenses, we use our observation in footnote~\ref{ft:mspa-as-cat} on p.~\pageref{ft:mspa-as-cat}.
\begin{theorem}[Spans from lenses] \label{th:lens2span}Any {(not necessarily invertible) }wb lens $\ell=(\mspaA, \ppg)$ gives rise to a span of wb a-lenses $\ell_i^\preccurlyeq=(\spaA_i,\spaB,\get_i, \putl_i)$. \\
%{\color{red}We should say already here, how $\ell$ is related to the resulting construction of Thm \ref{thm:LensesFromSpans} for $\ell_i^\preccurlyeq$, see below}
\end{theorem}
\shortlong{}{%}
\begin{proof} Let $\mspA$ have model spaces $\spaA_i$ and corr set $\R$ with corresponding boundary functions $\partial_i$. Let 
\[\spaB = \{(A_1, \ldots, A_n, R)\mid \partial_i(R) = A_i \mbox{ for all }i\}\] 
be the set of all aligned consistent multimodels and $\get_i:\spaB\to \spaA_i$ be projections, \ie\ $\get_i(A_1, \ldots, A_n, R)= A_i$ and $\get_i(u_1, \ldots, u_n)= u_i$\footnote{
Recall the definition of multimodel updates in Def.\ref{def:multispace}: There is no update component for $R$ 
}. Given $B = (A_1, \ldots, A_n, R)$ and update \frar{u_i}{A_i}{A'_i}, we define
\[\putl^B_{i\indb}(u_i)=(u_1', \ldots, u'_{i-1}, u_i;u_i', u'_{i+1} \ldots, u_n'): (A_1, \ldots, A_n, R)\to (A_1'', \ldots, A_n'', R''),\]
where $u_j' \eqdef \ppg^R_{ij}(u_i)$ for all $j$, $R'' = \ppg_{i\star}^R(u_i)$ and $\putl^B_{i\inda}(v_i)=\ppg^R_{ii}(u_i)$. 

That well-behavedness carries over from $\ell$ to the a-lenses is an direct consequence of the respective definitions. 
 \qed
\end{proof} 
}
%An important issue is how the two transformations, lenses to spans and spans to lenses, interact. To manage this, we need an $n$-ary counterpart of the theory of lens equivalence developed by Johnson and Rosebrugh in \cite{jr-jot17} for the binary case.  We leave it for future work. 
It is easy to see that $\Sigma_{i\in I_\ell}\ell_i^\preccurlyeq = \ell$ for any lens $\ell$, but if we begin with a span of a-lenses $\ebb_i$, $i\in I$ build a lens $\Sigma_{i\in I}\ebb_i$ and then build the span $(\Sigma_{i\in I}\ebb_i)^\preccurlyeq_i$, the two spans are different. This difference could disappear with a suitable notion of span equivalence, which we conjecture should be a straightforward generalization of the equivalence developed by Johnson and Rosebrugh in \cite{jr-jot17} for the binary case.  %which we think should be generalizable for the $n$-ary case. We leave it for future work. 
%
%\begin{example}
%Running
%\end{example}

\endinput
\begin{theorem}[Sequential composition]
	Let \lensar{\aekk}{\spaA}{\spaB} and  \lensar{\aell}{\spaB}{\spaC} be two wb a-lenses satisfying the following {\em junction condition}: all updates in $\spaB$ obtained by $\ekk$-propagation from \spaA\ are $\ell$-closed. Then there is a uniquely defined wb a-lens \lensar{\aekk;\aell}{\spaA}{\spaC}. %The composition is associative with identity lenses \lensar{\ell_{\id_{\spaB}}}{\spaB}{\spaB} being its units. 
\end{theorem}
 \input{figures/diags/seq-comp} 
 \textit{Proof.} Obviously, composition of \Kupd-preserving functors  
\flar{\get^\ekk}{\spaA}{\spaB} and \flar{\get^\ell}{\spaB}{\spaC} is a \Kupd-preserving functor: $\get^{\ekk;\ell}=\get^\ekk\circ\get^\ell$. Now we define $\putl^{\ekk;\ell}$. 
Let $u$ be an update as shown in \figref{fig:seq-comp} where horizontal lines are \get-corrs. Let $v=\putl^{\ekk B}_\indb(u)$, $u'=\putl^{\ekk B}_\inda(u)$, and $w=\putl^{\ell C}_\indb(v)$ (by the junction condition $v'=\id_{B''}$).  
%Finally, $u^*{=}\,\get^\ekk(v')$.  
Define $\putl^{C~\ekk;\ell}_\indb(u)=w$ and $\putl^{C~\ekk;\ell}_\inda(u)=u'$. Laws \lawname{Reflect1,2, 3} for $\ell;\ekk$ are obvious. %To prove idempotency \lawname{Reflect2}, we note that as $(v, v')\in\Kupd{B''}$ by $\ell.\lawname{Reflect}$, $u''\Kupd_{A''}u^*$ as $u''=u;u'=\get^\ekk(v)$ owing to $\Kupd$-preservation by $\get^\ekk$. Hence, by $\ekk.\lawname{PutPut}$, $\pult^{B \ekk}(u'';u^*)=\putl(u'');\putl(u^*)$
Stability and Putput are obvious too. 



==> ll-sections/horiz-compose.tex <==
\section{Horizontal composition}\label{sec:lego-spans2lens}

%\input{ll-sections/modSpaces-short}
%\input{ll-sections/aa-lensDef-semiDiscrete}

\renewcommand\figri{\figref{fig:aalens-arity}}
\newcommand\defri{\defref{def:aalens-arity}}

\begin{defin}[Indexed Asymmetric Lenses with Amendment, cf. \cite{me-fase18}]\label{def:aalens-arity}
	Let \spS\ and \spT\ be model spaces, \ie, categories with compatibility relation \Kupd. 
	
	An {\em indexed asymmetric lens  with amendment (indexed aa-lens)} from \spS\ (the {\em source} space of the lens) to \spT\ (the {\em target} space) is given by the following three components a-c.
 \begin{enumerate}[label={\bf  \alph*)}, %Step 
	%\arabic{enumi}., ref=Step \arabic{enumi},% 
	wide=0pt]
\item[{\bf a) Parameters:}] A category \spP\ of {\em parameters} (think about function/view definitions). We will denote objects of \spP\ by small letters $p,p',..$ rather than capital ones to avoid confusion with paper \cite{ll-bx19}. 

\item[{\bf b) Get:}] A functor \frar{\get}{\spP}{[\spS,\spT]}, where $[\spS,\spT]$ is the category of functors from \spS\ to \spT\ and their natural transformations. We will write $\get_p$ or even shorter $p^*$ for the functor \frar{\get(p)}{\spS}{\spT}.% $\get(p)$. 
\\	
	For any $S\in\xob{\spS}$, the pair $(S,p^*(S))$ will be shown in diagrams as an arrow $S\rBMapsto^{\#p}p^*(S)$ with a bulleted tail%
	\footnote{rather than $A\rMapsto^{\#p}p^*(S)$ by the technical reasons related to Powerpoint limitations}. 
	{In the future fibered version of the story, parameters will be arrows in a suitable category, and  $\#p$ will be a chosen opcartesian lifting of arrow $p$ at object $S$.} 
	
	The third component of an aa-lens is
	
	\item[{\bf c) Put:}] A family of operations $\putps$ indexed by pairs $(p\in P, S\in\xob{\spS})$ %(read ``put the view update back'') 
	Each operation in the family takes an update arrow as its input and outputs three arrows as specified below.  
	
	Given a pair $(p,S)$, operation $\putpa$ takes  an update \frar{v}{p^*(S)}{T'} as its input and outputs three arrows c1-c3 as specified below and illustrated by diagram in \figref{fig:aalens-arity}
\begin{enumerate}[label={\bf  \alph*)}, %Step 
	%\arabic{enumi}., ref=Step \arabic{enumi},% 
	wide=5pt]
	
\item[{\bf c1) }$\putl_\req$:] A source update \frar{u=\putps_\indb(v)}{S}{S'} 
	
\item[{\bf c2) }$\putl_\upd$:]	A parameter update ({\em evolution})  \frar{e=\putps_\upd(v)}{p}{p'}
	
\item[{\bf c3) }$\putl_\self$:]	An amendment to the target update, %$\putpa_{\self}(v)$ or 
	\frar{\amex{v}=\putps_{\self}(v)}{T'}{T''}. 
	%such that $v;\amex{v}=\get(u')$. 
\end{enumerate}
\end{enumerate}
\end{defin}
%%\endinput
%\input{ll-figures/diags/aalens-arity} -- earlier diagr. version with \spP\ being a set
%=====
%\input{ll-figures/pdfs/aalens-arity}
%===


\begin{lemma}
	If \spS, \spT, and \spP\ are co-discrete categories, then an aa-lens is nothing but a learner as defined in \cite{fj-bx19}
\end{lemma}
	
%---> version with put^B_indv(v) rather than v^@
%\input{ll-sections/aalens-wblaws-bulkyNotation}

\input{ll-sections/aalens-wblaws}

\renewcommand\figrii{\figref{fig:aalens-hComp}}
\renewcommand\defrii{\defref{def:aalens-hComp}}
\renewcommand\kl{\ensuremath{\ekk;\ell}}

%\input{ll-figures/pdfs/aalens-hComp}
\begin{defin}[(Horizontal) composition of aa-lenses] \label{def:aalens-hcomp}
	Let \frar{\ekk}{\spA}{\spB} and \frar{\ell}{\spB}{\spC} be two aa-lenses with parameter spaces \spP\ and \spQ\ resp. Their {\em composition}  is the following lens \kl.
	
	Its parameter space is the product $\spP\times\spQ$, and the \get-family is defined as follows: for any pair of parameters $(p,q)$, %$\get^{(p,q)}$ or 
	functor $\#(p,q)$ is the composed functor %\frar{\get^p;\get^q}{\spA}{\spC}, 
	\frar{\#p;\#q}{\spA}{\spC}, and given a pair of parameter updates $(e,o)$ in $\xar{\spP}\times\xar{\spQ}$, their \get-image is the Godement product of natural transformations. 
	
	The most interesting is, of course, the definition of propagation operations \putl s. Let $(A,p,q, C)$ with $A\in\xob{\spA}$, $p\in\spP$, $q\in\spQ$ be a \zdmod{state}{corr}{} of lens \kl, and  \frar{w}{C}{C'} is a target update as shown in \figrii\ with bold black lines.  %All stages of the definition are accurately described in \figrii. 
	For the first propagation step, we run lens $\ell$ as shown in \figrii\ with the blue colour: this is just an instantiation of the pattern of \figri\ with $(q,B)$, where $B=\#p(A))$, being a given state of  lens $\ell$,  $w$ a given target update, and \frar{v=\putxy{q}{B}_\req}{B}{B'}, 
	\frar{o=\putxy{q}{B}_\upd}{q}{q'}, and
	\frar{\amex{w}=\putxy{q}{B}_\self}{C'}{C''} three propagated updates. 
	%
	Next we run lens $\ekk$ at state $(p,A)$ and the target update $v$: it is yet another instantiation of pattern \figri\ (this time with the green colour for derived elements), which produces three propagated updates
	\frar{u=\putxy{p}{A}_\req}{A}{A'}, 
	\frar{e=\putxy{p}{A}_\upd}{p}{p'}, and
	\frar{\amex{v}=\putxy{p}{A}_\self}{B'}{B''}.
	
	Having these data and using functoriality of \get s, we produce a system of ``fill-in'' arrows shown in \figrii\ in orange (where we have chosen one of the two equivalent ways of forming Godement product).
By composing appropriate green and orange arrows, we obtain yet another instantiation of the pattern in \figri,\ie, an aa-lens, which we denote by \kl.
\end{defin}
%====
%\input{ll-figures/pdfs/aalens-hComp}
%===
\begin{propo} [Composition and lens laws] a) Lens \kl\ is wb (and closed) as soon as lenses $\ekk$ and $\ell$ are wb (and closed). b) Moreover, lens \kl\ is wb+ as soon as lenses $\ekk$ and $\ell$ are such {\em and} all functors $p^*$ preserve closedness of updates: if update \frar{v}{B}{B'} is closed for lens $\ekk$ (\ie, $\amex{v}=\id_{B'}$), then update $q^*(v)$ is closed for lens $\ell$.
\end{propo}
\zd{the prop aboe is to be carefully checked, esp. closedness condition}
\begin{defin}[Aa-lens Equaivalence]
	Two parallel aa-lenses \frar{\ell, \hat\ell}{\spS}{\spT} are called {\em (definitionally) equivalent} if their parameter spaces are isomorphic via a functor \frar{f}{\spP}{\hat\spP} together with an isomorphic natural transformation \dlar{i}{\#}{f;\hat\#} such that %$f;\hat\#=\#$ 
	for all propagation operations $\putl_\x$, $x\in\{\upd,\req,\self\}$, and any \zdmod{state}{???}{} $(p,S)$, equality $$\putxy{p}{S}_x(v) = \puthatxy{\hat p}{S}_x(i_S;v)$$ holds for any target update \frar{v}{T}{T'} where $T=p^*(S)$, $\hat p=f(p)$, and  $\hat T=\hat p^*(S)$ (so that \flar{i_S}{T}{\hat T}). 
	\zd{$\putl_\x$, $x\in\{\upd,\req,\self\}$ is to be intriduced earlier!!}
\end{defin}
\begin{remark}\zd{Just for the record}A more categorically plausible definition would require just isomorphisms rather than equalities, but then we need 2-arrows between updates.
\end{remark}
\begin{propo}[Category of aa-lenses]
	a) Model spaces as objects and equivalence classes of aa-lenses as arrows form a category denoted by \aalenscat. 
	b) 	If \defri\ (\figri) is enriched with Cartesian monoidal product ($S_1\otimes S_2=(S_1, S_2)$ for objects and similarly for arrows), then  \aalenscat\ becomes a symmetric monoidal category. 
\end{propo}
\zd{the proof is a direct gen of that on ein FJ-bx19, or not????}

\endinput
In contrast to the general lens case, a wb a-lens features \lawname{\reflectzero} --- a sort of a self-Hippocratic law regulating the necessity of amendments: the latter is not allowed as soon as consistency can be restored without amendment. Another distinction is inclusion of an invertibility law \lawname{PutGet} into the definition of well-behavedness: 
 %due to historical traditions. %Subsequent results will also provide some justification for this. 
\lawname{PutGet}{} together with \lawname{Reflect2} provide (weak) invertibility: $\putl^B_\indb(\get(\putl^B_\indb(v)))=\putl^B_\indb(v)$.   
\lawname{Reflect3} is omitted as it is implied by \lawname{Reflect0} and \lawname{PutGet}.  

Any a-lens $\ebb^{\preccurlyeq} =(\spaA,\spaB,\get, \putl)$ gives rise to a binary symmetric lens $\ebb$. Its carrier consists of model spaces $\spaA$ and $\spT$, for which we assume $\Kupd$ and $\Kdisj{}$ to be defined such that the spaces are well-behaved, cf.\ Def.~\ref{def:wbspace}. The set of corrs of a pair $(A,B)\in \xob{\spS}\times \xob{\spT}$ is the singleton $\{\etosing{(A,B)}\}$ with $\prt_\spS\etosing{(A,B)}=A$ and $\prt_\spT\etosing{(A,B)}=B$, 
%the boundary mappings are the projections, 
\zdmodtok{realignment is thus trivial,}{}{ALIGH} and consistent corrs are exactly those \etosing{(A,B)}, for which $A = \get(B)$.

For a consistent corr $\etosing{B}={(\get(B), B)}$, we need to define six operations $\ebb.\ppghB_{\_\_}$. Below we will write the upper index as $B$ rather than $\hat B$ to ease the notation. For a  view update \frar{v}{A}{A'} and the corr \etosing{B}, we define 
 $$
\ppgB_{\spS\spT}(v)=\putl^B_\indb(v){:}\, B\to B'', \;
%
\ppgB_{\spS\spS}(v)=\putl^B_\inda(v){:}\, A'\to A'', \;
% \mbox{ and }
\ppgB_{\spS\star}(v)=\etosing{B''}
$$
 The condition $A''=\get(B'')$ for $\ebb^\preccurlyeq$ means that \etosing{B''} is again a consistent corr with the desired boundaries. For a base update \frar{u}{B}{B'} and the corr \etosing{B}, we define
$$\ppgB_{\spT\spS}(u)=\get(u),\;
\ppgB_{\spT\spT}(u)=\id_{B'},\; %and
\ppgB_{\spT\star}(u)=\etosing{B'}
$$ Functoriality of $\get$ yields consistency of $\widehat{B'}$.

\begin{defin}[Very well-behaved a-lenses] \label{def:putput_a}
		A wb a-lens is called {\em very well behaved (very wb)}, if the \corring\ binary symmetric lens is such.  %additionally fulfills \lawnamebr{PutPut}, 
		cf.  Def.~\ref{def:putput}.
Of course, this definition restricts the behaviour only for the $\putl$-part of the a-lens (hence the name of the law), since functor $\get$ is compositional anyway. \qed
\end{defin}

\begin{lemma}\label{lemma:asymm_symm} Let $\ebb^\preccurlyeq$ be a (very) wb a-lens and $\ebb$ the corresponding symmetric lens. Then all base updates of $\ebb$ are closed, and $\ebb$ is (very) wb and invertible. 
 \end{lemma}
 \begin{proof}
 Base updates are closed by the definition of $\ppg_{\spT\spT}$. Well-behavedness follows from wb-ness of $\ebb^\preccurlyeq$. Invertibility has to be proved in two directions: $\ppg_{\spaB\spaA};\ppg_{\spaA\spaB};\ppg_{\spaB\spaA} = \ppg_{\spaB\spaA}$ follows from \lawnamebr{PutGet}{} and \lawnamebr{Reflect0}, the other direction follows from \lawnamebr{PutGet}{} and \lawnamebr{Reflect2}, see the remark after Def.\ref{def:wbalens}. The ''vwb''-implication follows directly from Def.\ref{def:putput_a}. 
 \qed
 \end{proof}
\begin{remark}[A-lenses as view transformation engines]\newpii{
	In terms of Varr\'o et al \cite{dvarro-models18}, a wb a-lens can be seen as an abstract algebraic model of a bidirectional view transformation engine. This engine is assumed to be a) consistent: it is a basic lens law that propagation must always produce a consistent corr, b) incremental, as lenses propagate changes rather than create the target models from scratch, c) validating, as the result of propagation is always assumed to satisfy the target metamodel constraints (either by considering the entire model space to be only populated by valid models, or by introducing a subclass of valid models and require the result of the propagation to get into that subclass). Reactiveness, \ie, whether the engine executes on-demand or in response to changes, is beyond the lens \fwk. To address this and similar concerns, we need a richer \fwk\ of lenses augmented with organizational structure introduced in \cite{me-jss15,me-grand17}. }{1}{-15em}
\end{remark}

  \begin{theorem}[Lenses from Spans]\label{thm:LensesFromSpans} An $n$-ary span of (very) wb asymmetric lenses $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$, $i=1..n$ with a common base \spaB\ of all $\ebb_i^{\preccurlyeq}$ gives rise to a (very) wb symmetric lens denoted by $\Sigma_{i=1.. n}^\spT\ebb_i^{\preccurlyeq}$. 
\end{theorem}
\begin{proof}
An $n$-ary span of a-lenses $\ebb_i^{\preccurlyeq}$ (all of them interpreted as symmetric lenses $\ebb_i$ as explained above) is a construct equivalent to the star-composition of Def.~\ref{def:star-comp}.3, in which lens $\ekk=\idlensnb$ (cf. Ex.~\ref{ex:idLens}) and peripheral lenses are lenses $\ebb_i$. The junction condition is satisfied as all base updates are $\ebb_i$-closed for all $i$ by Lemma \ref{lemma:asymm_symm}, and also trivially closed for any identity lens. The theorem thus follows from Theorem~\ref{th:star-comp}. The ``very wb''-part follows directly from Def.~\ref{def:putput_a}. Note that a corr in $\Corrx{\Sigma_{i=1.. n}^\spT\ebb_i^{\preccurlyeq}}$ 
 is nothing but a single model $B\in\xob{\spaB}$ with boundaries being the respective $\get_i$-images.
\end{proof}
The theorem shows that combining a-lenses in this way yields an $n$-ary symmetric lens, whose properties can automatically be inferred from the binary a-lenses.
\input{figures/pdfs/mergedMetamultimod-uml}

\exIntro. Figure~\ref{fig:mergedMetamod-uml} shows a metamodel $M^+$ obtained by merging the three metamodels $M_{1,2,3}$ from \figri\ without loss and duplication of information. In addition, for persons and companies, the identifiers of their  original model spaces can be traced back via attribute ''spaces'' 
(\Commute-objects are known to appear in space $\spS_3$ and hence do not need such an attribute). As shown in \cite{me-ecmfa17}, any consistent multimodel $(A_1...A_n, R)$ can be merged into a comprehensive model $A^+$ instantiating $M^+$. Let 
$\spT$ be the space of such together with their comprehensive updates \frar{u^+}{A^+}{A'^+}. 

For a given $i\le 3$, we can define the following a-lens $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$:
$\get_i$ takes update $u^+$ as above and outputs its restriction to the model containing only objects recorded in space $\spS_i$. Operation $\putl_i$ takes an update \frar{v_i}{A_i}{A'_i} and first propagates it to all directions as discussed in \sectref{sec:example}, then merges these propagated local updates into a comprehensive  \spaB-update between comprehensive models. This yields a span of a-lenses that implements the same \syncon\ behaviour as the symmetric lens discussed in \sectref{sec:example}.

\noindent {\em\bf  From (symmetric) lenses to spans of a-lenses.} There is also a backward transformation of (symmetric) lenses to spans of a-lenses. Let $\ell=(\mspaA, \ppg)$ be a (very) wb lens. It gives rise to the following span of (very) wb a-lenses $\ell_i^\preccurlyeq=(\prtbf_i(\mspaA),\spaB,\get_i, \putl_i)$   
where space $\spaB$ has objects $(A_1\ldots A_n,R)$ with $R\in \Corrx{A_1...A_n}$ a consistent corr, and arrows are the update tuples of $\mspA$. Functors $\get_i:\spaB\to \spaA_i$ are projection functors. Given $B = (\tupleAWOB, R)$ and local update \frar{u_i}{A_i}{A'_i}, let

%\noindent 
\frar{\putl^B_{i\indb}(u_i)\eqdef(u_1',..,u'_{i-1}, (u_i;u_i'), u'_{i+1},..,u_n')}
{(A_1... A_n,R)}{(A''_1... A''_n,R'')}
\\[1ex] 
where $u_j' \eqdef \ppg^R_{ij}(u_i)$ (all $j$) and $R'' = \ppg_{i\star}^R(u_i)$. Finally, $\putl^B_{i\inda}(v_i)\eqdef\ppg^R_{ii}(v_i)$, \ie, 
$v_i^{@B}=v_i^{@R}$. 
Validity of \zdmodtok{\lawname{Hippocr1-2}}{\lawname{Stability}}{}, \lawname{Reflect0-2}, \lawname{PutGet} and \kputputlaw\ directly follows from the above definitions. This yields 
\begin{theorem}\label{theo:lens2span}
Let $\ell = (\mspA, \ppg)$ be a (very) wb symmetric lens. Then the multi-span 
\[(\ell_i^\preccurlyeq=(\prtbf_i(\mspaA),\spaB,\get_i, \putl_i) \mid i=1..n)\]
of (very) wb a-lenses (where \spT\ is defined as specified above) has the same synchronisation behaviour w.r.t.\ model spaces $(\prtbf_i(\mspaA)\mid i=1..n)$.  
\qed
\end{theorem}

\newpii{
An open question is whether the span-to-lens transformation in Thm.\ref{thm:LensesFromSpans} and the lens-to-span transformation of Thm.~\ref{theo:lens2span} are mutually inverse. It is easy to see that the chain 
\begin{equation}\label{eq:lens2span2lens}
\mbox{symmetric lens $\rightarrow$ wide span $\rightarrow$ symmetric lens} 
\end{equation}
results in a lens isomorphic to the initial one, but the chain 
\begin{equation}
\mbox{wide span $\rightarrow$ symmetric lens $\rightarrow$ wide span} 
\end{equation}
ends with a different span as the first transformation above loses information about updates in the head of the span. 
 The results for the binary case in \cite{jr-jot17} show that the two spans can only be shown to be equivalent modulo certain equivalence relation, and an equivalence relation between lenses is also needed to tune all constructs into harmony. These equivalences may be different for our multiary lenses with amendments, and we leave this important question for future research.  
}{1}{-17em}
 \endinput
 
%============= Old Version ========= 
 \begin{theorem}[Lenses from Spans]\label{thm:LensesFromSpans} An $n$-ary span of wb a-lenses $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$, $i=1..n$ (note the common base \spaB\ of all $\ebb_i$) gives rise to a wb  (symmetric) lens $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$.
% 	
  	Moreover, $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$ is invertible as soon as the span satisfies the following condition%
 	\footnote{Found for the binary case by Bob Rosebrugh \cite{bob-invert}}: 
% 	$$
% 	\putl^B_{\indb i}
% 	$$
$\PP^B_i=\PP^B_j$ for all $B\in\xob{\spaB}$ and $i,j\le n$, where for given $B$ and $i$,  $\PP^B_i$ is the inverse image of 
$\xarr{\spaB}(\get_i(B),\_)$, \ie,  the set $\compr{\putl^B_{\indb i}(v_i)}{\frar{v_i}{\get_i(B)}{\_}}$. %, then $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$ is invertible.
\end{theorem}
\shortlong{}{%}
\begin{proof}
An $n$-ary span of a-lenses $\ebb_i^{\preccurlyeq}$ (all of them interpreted as symmetric lenses $\ebb_i$ as explained above) is a construct equivalent%
\footnote{To make it precise, we need to introduce a simple notion of lens equivalence, which identify lenses with the same propagation behavior but, perhaps, different sets of corrs -- see. \eg, \cite{jr-jot17}} to the star-composition of Def.~\ref{def:star-comp}, in which lens $\ekk=\idlensna$ and peripheral lenses are lenses $\ebb_i$. The junction condition is satisfied as all base updates are $\ebb_i$-closed for all $i$ by Lemma \ref{lemma:asymm_symm}, and also trivially closed for any identity lens. The theorem thus follows from Theorem~\ref{th:star-comp}. Note that a corr in $\xstar{(\Sigma_{i=1}^n\ebb_i^{\preccurlyeq})}$ 
 is nothing but a single model $B\in\xob{\spaB}$ with boundaries the respective $\get_i$-images. \qed
 \end{proof} 
}
For the backward transformation of lenses to spans of a-lenses, we use our observation in footnote~\ref{ft:mspa-as-cat} on p.~\pageref{ft:mspa-as-cat}.
\begin{theorem}[Spans from lenses] \label{th:lens2span}Any {(not necessarily invertible) }wb lens $\ell=(\mspaA, \ppg)$ gives rise to a span of wb a-lenses $\ell_i^\preccurlyeq=(\spaA_i,\spaB,\get_i, \putl_i)$. \\
%{\color{red}We should say already here, how $\ell$ is related to the resulting construction of Thm \ref{thm:LensesFromSpans} for $\ell_i^\preccurlyeq$, see below}
\end{theorem}
\shortlong{}{%}
\begin{proof} Let $\mspA$ have model spaces $\spaA_i$ and corr set $\R$ with corresponding boundary functions $\partial_i$. Let 
\[\spaB = \{(A_1, \ldots, A_n, R)\mid \partial_i(R) = A_i \mbox{ for all }i\}\] 
be the set of all aligned consistent multimodels and $\get_i:\spaB\to \spaA_i$ be projections, \ie\ $\get_i(A_1, \ldots, A_n, R)= A_i$ and $\get_i(u_1, \ldots, u_n)= u_i$\footnote{
Recall the definition of multimodel updates in Def.\ref{def:multispace}: There is no update component for $R$ 
}. Given $B = (A_1, \ldots, A_n, R)$ and update \frar{u_i}{A_i}{A'_i}, we define
\[\putl^B_{i\indb}(u_i)=(u_1', \ldots, u'_{i-1}, u_i;u_i', u'_{i+1} \ldots, u_n'): (A_1, \ldots, A_n, R)\to (A_1'', \ldots, A_n'', R''),\]
where $u_j' \eqdef \ppg^R_{ij}(u_i)$ for all $j$, $R'' = \ppg_{i\star}^R(u_i)$ and $\putl^B_{i\inda}(v_i)=\ppg^R_{ii}(u_i)$. 

That well-behavedness carries over from $\ell$ to the a-lenses is an direct consequence of the respective definitions. 
 \qed
\end{proof} 
}
%An important issue is how the two transformations, lenses to spans and spans to lenses, interact. To manage this, we need an $n$-ary counterpart of the theory of lens equivalence developed by Johnson and Rosebrugh in \cite{jr-jot17} for the binary case.  We leave it for future work. 
It is easy to see that $\Sigma_{i\in I_\ell}\ell_i^\preccurlyeq = \ell$ for any lens $\ell$, but if we begin with a span of a-lenses $\ebb_i$, $i\in I$ build a lens $\Sigma_{i\in I}\ebb_i$ and then build the span $(\Sigma_{i\in I}\ebb_i)^\preccurlyeq_i$, the two spans are different. This difference could disappear with a suitable notion of span equivalence, which we conjecture should be a straightforward generalization of the equivalence developed by Johnson and Rosebrugh in \cite{jr-jot17} for the binary case.  %which we think should be generalizable for the $n$-ary case. We leave it for future work. 
%
%\begin{example}
%Running
%\end{example}

\endinput
\begin{theorem}[Sequential composition]
	Let \lensar{\aekk}{\spaA}{\spaB} and  \lensar{\aell}{\spaB}{\spaC} be two wb a-lenses satisfying the following {\em junction condition}: all updates in $\spaB$ obtained by $\ekk$-propagation from \spaA\ are $\ell$-closed. Then there is a uniquely defined wb a-lens \lensar{\aekk;\aell}{\spaA}{\spaC}. %The composition is associative with identity lenses \lensar{\ell_{\id_{\spaB}}}{\spaB}{\spaB} being its units. 
\end{theorem}
 \input{figures/diags/seq-comp} 
 \textit{Proof.} Obviously, composition of \Kupd-preserving functors  
\flar{\get^\ekk}{\spaA}{\spaB} and \flar{\get^\ell}{\spaB}{\spaC} is a \Kupd-preserving functor: $\get^{\ekk;\ell}=\get^\ekk\circ\get^\ell$. Now we define $\putl^{\ekk;\ell}$. 
Let $u$ be an update as shown in \figref{fig:seq-comp} where horizontal lines are \get-corrs. Let $v=\putl^{\ekk B}_\indb(u)$, $u'=\putl^{\ekk B}_\inda(u)$, and $w=\putl^{\ell C}_\indb(v)$ (by the junction condition $v'=\id_{B''}$).  
%Finally, $u^*{=}\,\get^\ekk(v')$.  
Define $\putl^{C~\ekk;\ell}_\indb(u)=w$ and $\putl^{C~\ekk;\ell}_\inda(u)=u'$. Laws \lawname{Reflect1,2, 3} for $\ell;\ekk$ are obvious. %To prove idempotency \lawname{Reflect2}, we note that as $(v, v')\in\Kupd{B''}$ by $\ell.\lawname{Reflect}$, $u''\Kupd_{A''}u^*$ as $u''=u;u'=\get^\ekk(v)$ owing to $\Kupd$-preservation by $\get^\ekk$. Hence, by $\ekk.\lawname{PutPut}$, $\pult^{B \ekk}(u'';u^*)=\putl(u'');\putl(u^*)$
Stability and Putput are obvious too. 



==> ll-sections/intro-act19.tex <==
\section{Introduction}\label{sec:intro}

	In a seminal paper \citefst, Fong, Spivak and Tuy\'eras showed how to compose supervised machine learning (ML) algorithms so that the latter form a symmetric monoidal (sm) category \learncat, and built an sm-functor %\frar{L_{\eps,\err}}{\paracat}{\learncat}, 
\frar{L}{\paracat}{\learncat}, 
which maps a parameterized differentiable function 
%$f=\comprfam{p\in P}{\frar{f_p}{A}{B}}$ (where $A,B,P$ are sets)
\frar{f}{P\times\reals^m}{\reals^n} (with the parameter space $P=\reals^k$)
%or, via currying, a parameterized function \frar{I}{P\timm A}{B}%
%\footnote{{\em I} refers to {\em implementation}: we're trying to be close to the notation in \citefst} 
to a learning algorithm %$L_{\eps,\err}(f)$ %$\ptol_{\eps,e}(I)(f)$ 
that improves an initially  given function \frar{f(p_0, \_)}{\reals^m}{\reals^n} 
%(with $p_0$ being some initial value of the parameter \pind) 
by learning from a set of training pairs $(a,b)\in \reals^m\timm \reals^n$. %(where the {\em step size} $0<\eps\in\reals$ and the {\em error function} \frar{\err}{\reals\timm\reals}{\reals} are parameters of $L$). 
Recently, Fong and Johnson noticed in \citefjbx\ (quoting them directly) ``surprising links between two apparently disparate areas'': %a compositional treatment of supervised learning algorithms, called learners, and and a mathematical treatment of bidirectional transformations, called lenses.'' 
ML (treated compositionally as above) and bidirectional model \trafon s or \Bx (also treated compositionally in a \fwk\ of mathematical structures called {\em lenses} \cite{bpierce-popl05}), whereas ``naively at least, there seemed to be little reason to expect them to be closely related mathematically''.%
%introduced by Pierce \etal\ \citepiercetr\ and categorificied by Diskin \etal\ \cite{me-jot11,me-models11}}{}{}), 
\footnote{
	Term {\em \Bx} abbreviates ``bidirectional $X$ (something)'' and refers to bidirectional change propagation in different contexts in different domains: file \syncon\ in versioning, data exchange in databases, model \syncon\ and model transformation in Model-Driven software Engineering (MDE), 
	%and virtually everywhere in engineering, 
	see \cite{bx-cross} for some of these contexts. What makes \Bx a special and united community amongst many circles studying \syncon\ and change propagation, is a foundational lens-based algebraic \fwk.  Nevertheless, within \Bx the application context can vary, sometimes significantly, and in the present paper, \Bx will mainly refer to \Bx in the MDE context --- the author's area of expertize in \Bx. %\textcolor{red}{trafos are views}
}   
Fong and Johnson also built an sm-functor %\frar{\sym_0}{\learncat}{\slenscat},
$\learncat\rightarrow\slenscat$
which maps learning algorithms to so called symmetric lenses.%{\em co-discrete} lens. Such lenses can be seen as a trivial version of delta lenses, in which deltas \frar{\Delta}{x}{y} are degenerated into source-target pairs $(x,y)$.

The main goal of the present paper is to introduce a \fwk\ in which similarities between ML and \Bx become apparent. We will see that by abstracting away some details and ignoring the contextual differences, both problems can be seen as two different instantiations of the same algebraic structure defined in the paper and called \bfem{asymmetric learning lens, al-lens}. Indeed, lenses are devices specifying change propagation, and learning can be seen as a special change propagation case. For example, given (i) sets $A, B, P$ and  a family of functions 
$f=\comprfam{p\in P}{\frar{f_p}{A}{B}}$ as the learning space, and (ii) a training datum $(a,b')$ with $b'\noteq b=f_p(a)$ for an initially given parameter value $p$, we can interpret it as a change from a consistent state of the system $(a,p,b)$ to an inconsistent state $(a,p,b')$ caused by the change \warrbb. \Bx would fix this inconsistency by changing the input data \warraa\ so that the state $(a',p,b')$ is consistent, \ie, $f_p(a')=b'$; this action is often described as {\em propagating} change \warrbb\ to change \warraa. ML would call the original change \warrbb\ an error, and fix it by changing the parameter value \warrpp\ so that the state $(a,p',b')$ is either consistent, 
%\ie, $f_{p'}(a)=b'$, 
or at least less inconsistent than $(a,p,b')$ w.r.t. some metrics, \eg, we can add  metrics to set $B$ and require that $||f_{p'}(a), b'|| < ||f_p(a),b'||$. In ML terms, the system has {\em learnt} a better approximation $f_{p'}$ of the function; in \Bx terms, change \warrbb\ is propagated to \warrpp.  

\input{ll-figures/pdfs/mlbx-plane}
Abstract learners defined in \citefst\ do both propagations so that the updated/learnt state is $(a',p',b')$. The story is schematically described in the inset figure, in which the horizontal dashed arrow shows ML's evolution towards having back propagation (Bp) and the vertical arrow shows \bx's evolution towards \Bx with learning (\bxl, still to be developed; the work on deriving model transformations from examples \citemtex\ can be seen as \bxl). In the lens \fwk\ developed for \bx, point (1,1) corresponds to the idea of a learning lens, % defined in the present paper, 
which covers both ML and \bx. In the paper, %the notion of a learning lens allows us to work
we will work with asymmetric rather than symmetric learning lenses, which is a) technically much simpler and b) conceptually justified: compositional ML considered in \citefst\ is about composing functions rather than relations, and an asymmetric model seems to be more appropriate.  The main result of \citefjbx\ can then be seen as an ``internal lens business'': it says that any codiscrete al-lens can be encoded by a special symmetric non-learning lens. In the present paper, a lens always means an asymmetric lens.
% == nice piece !
%As asymmetric lenses are simpler than symmetric, and ordinary lenses are simpler than learning lenses, this results says that we can trade asymmetry for unparameterization, which is unexpected and nice, but can be encapsulated as an internal lens business not immediately related to interactions between ML and BX (of course, such observations are much easier to make after connections between ML and lenses were noticed in \citefjbx). 

Thus, the notion  of a codiscrete al-lens was actually discovered in \citefst.  The present paper makes three contributions to the learning lens idea consecutively described in three subsections below, after which we outline the structure of the rest of the paper. 

\subsection{Defining asymmetric learning delta lenses (al-lenses) and their composition  (sequential and parallel).
	% with amendment, \alalenscat.
} 
It could be called categorification of the learning lens notion: we will work with {\em delta} lenses,  in which a change/delta between objects $x,x'$ is an arrow \frar{u}{x}{x'} rather than a pair $(x,x')$; moreover, multiple different updates/deltas are possible between the same objects $x,x'$ so that $\Hom(x,x')$ is a set (non-empty for a typical \bx\ application in MDE). Each species of a delta lens has its codiscrete version, in which $\Hom(x,x')=\{(x,x')\}$, and learners defined in \citefst\ are exactly codiscrete al-lenses.%
\footnote{In detail, the category of learners \learncat\ defined in \citefst\ coincides with the category of codiscrete al-lenses \allenscatcodi, which is a  full sm-subcategory of the sm-category of al-lenses \allenscat.}
 In this paper, a lens will always mean a delta lens by default.  
%The original lenses of then become the codiscrete specialization of delta lenses. %, whose only arrows are pairs $(x,x')$ and any such a pair is an arrow (in \bx, any object $x$ can be updated to any other object $x'$ so that categories of objects of interests are bidirectionally connected: $\mathit{Hom}(x,x')\noteq\varnothing$ for any pair $x,x'$). In this paper, a lens will always mean a delta lens while lenses employed in \citefetal\ are referred to as codiscrete. 

In the MDE context, objects $x,x'$ are complex structures so that their delta/update \frar{u}{x}{x'} is a complex structure too. Its ignorance in the codiscrete lens formalism may create fundamental problems for applying codiscrete lenses to practical problems (see \cite{me-jot11}). The role of deltas in the ML context, where objects $x,x'$ are tuples of real numbers, is probably less fundamental but still important---we will briefly discuss it below in \sectref{ddlens-1}. %and continue  in \sectref{deltas4ml}. 

\subsection{%The second technical contribution of the paper is s
	Specification of algebraic laws for learning lenses and studying their preservation under lens composition. Building an sm-category \alalenscat\ of al-lenses with amendment.} 

For \bx, this is a crucial aspect: it says that if several synchronization modules satisfy some laws (are {\em well-behaved} in the lens parlance), then their composition is automatically well-behaved and hence the (usually expensive) integration testing is not needed. However, a major asymmetric BX lens law that requires consistency of the system after change propagation (called the PutGet law in the lens parlance) does not always hold in practice and needs to be relaxed \cite{me-fase18}. The relaxed PutGet is based on the idea of self-propagation: the change \warrbb\ is amended by a consecutive change \warrxy{b'}{b'^@:=f_{p'}(a')} so that the resulting state $(a',p',b'^@)$ is consistent.   Thus, \bx\ needs lenses with amendment, and the main construct of the paper is the notion of an \bfem{asymmetric learning lens with amendment, \alalens}, for which we will formulate \shortlong{two}{three} basic laws. We will define sequential and parallel composition of \alalens es, study their compatibility with the laws, and build an sm-category of well-behaved \alalens es, \alalenscat. The role of algebraic laws in the ML context is an intriguing subject left for future work. 

%Finally, yet another feature of the lens perspective on ML developed in this paper is to consider lenses with {\em amendments} recently defined in the \Bx context \cite{me-fase18} but, as we will see, having a natural ML motivation as well. Thus, lenses to be considered are al-lenses with amendments or {\em \alalens es}. 
%%and our compositional ML-\Bx story becomes a cospan of sm-functors
%%\begin{equation}\label{eq:mlbxcospan}
%% \paracat\rTo^{\learnfun_{\eps,\err}}\apalenscat\lTo^{\bxfun_\prpol}\bxcat
%%\end{equation}
%In the paper, we will define the category \alalenscat\ and prove it is \smm. We will also see that category \learncat\ of \citefst\ is nothing but the codiscrete version of \alalenscat. 
%%  We also reinterpret the functorial result of \citefst\ as shown in \eqref{mlbxcospan} by treating Euclidean spaces as Lawvere's metric spaces. The right part of (1) is left for future work.

%%==
%%\input{ll-figures/diags/policyfun}
%\input{ll-figures/diags/policyfun-ml-triangle}
%%\input{ll-figures/diags/policyfun-smallTri}

\subsection{Functoriality of learning algorithms in the {\em delta} lens setting}\label{sec:ddlens-1}
We will reconsider a major result in \citefst---compositionality of the mapping from learning spaces to learning algorithms, in the light of {\em delta} rather than {\em codiscrete} lenses. The compositionality above is specified by the commutative triangle in \figro,  in which nodes are sm-categories and arrows are sm-functors (and below we will omit the prefix sm). 

%==
%\input{ll-figures/diags/policyfun}
\input{ll-figures/diags/policyfun-ml-triangle}
%\input{ll-figures/diags/policyfun-smallTri}

Node $\paracatre$ denotes the category of (equivalence classes of) parameterized differentiable mappings $P\times\reals^m\rightarrow\reals^n$ (with the parameter space $P=\reals^k$), which is denoted by \paracat\ in \citefst\ but we add subindex \reals\ to recall the context, which will be important in our setting.
Arrow  \leefun\ is the functor built in \citefst\ with \eps\ and \err\ referring to parameters of the gradient descent learning (a step size and an error function $\reals\timm\reals\rightarrow\reals$ resp.), and ${-}\reals$ and ${-}\putl$ are two forgetful functors into the category of sets and (equivalence classes of) parameterized functors, \psetcat\ (%\footnote{C
considering parameterized functions up to some equivalence is needed to ensure associativity of their composition -- see \sectref{pcatcat} for details). Here and below we will denote a functor forgetting a part $X$ of its source objects' or/and arrows' structure by symbol ${-}X$. Similarly, functors adding a structural piece $X$ are denoted by $\plusx{\xyz}X$ with index \xyz\ referring to the mechanism by which this addition is realized.
%}

%\input{ll-figures/diags/policyfun-ml-topPart}
Our main observation is that functor \leefun\ is actually composed from two components %each having its own special role 
as shown by commutative square  (1) in \figroo, in which \alalensdifcat\ is the category of ala-lenses whose source and target model spaces are equipped with an operation \dif\ that given two objects $x, x'$ (\eg, two tuples in \realsx{n}), produces a delta between them, \ie, an arrow \frar{\dif(x,x')}{x}{x'} (\eg, for $x,x'\in\realsx{n}$, $\dif(x,x')=(x'_i-x_i)_{i\le n}$), and lens operations are compatible with \dif. Each delta lens with differencing gives rise (in fact, collapses) into a codiscrete lens, whose operation $\putlcodi$ works by, first, computing the required delta and then applying to it the delta lens \putl. We consider this construction in \sectref{codifun} and show that this construction amounts to a functor \frar{\codiscr}{\alalensdifcat}{\alalenscatcodi}.% 
\footnote{Importantly, as functor \codiscr\ forgets structural information about its source lenses,  its composition  with the obvious  full forgetful embedding of \alalenscatcodi\ into \alalensdifcat\ (see triangle (4) in the diagram, where this embedding is denoted by $\plusx{\pairing}(\deltas,\dif)$ as it adds necessary deltas and differencing by employing pairing of objects) is not identity on \alalensdifcat\ (but the converse composition $(\plusx{\pairing}(\deltas,\dif));\codiscr$ is the identity functor $\id_\alalenscatcodi$).}

\input{ll-figures/diags/policyfun-ml-topPart}
In comparison with functor \leefun\ considered in \citefst, the idea of gradient descent learning is more accurately described by functor \leefunovr\ because it does not include the forgetful functor \codifun\ into  the story (see triangle (1) in the diagram). Moreover, \leefunovr\ is itself composed as shown by triangle (2) of the diagram: the first component (the left edge) is an isomorphic representation of functions between Euclidean spaces-as-sets (denoted \realsx{n}) as functors between Euclidean spaces-as-categories (\rcatx{n}), whose arrows are componentwise differences, and the second component (the horizontal edge) is augmenting these functors with their special inverses called \putl s in the lens parlance. Building operations \putl s is essentially based on the gradient descent idea, hence, the notation 
$\plusx{Gd(\eps,\err)}\putl$ for this functor.  Adding \putl\ does not change the original functors \get s and triangle (3) formed with two obvious forgetful functors into \pcatcat\ commutes (category \pcatcat\ is the category of (equivalence classes of ) parametrized functors between small categories specified in \sectref{pcatcat}). Note that while commutativity of forgetting for functor \leefun\ is considered over \psetcat\ (see \figro), the context for \leefunovr\ is \pcatcat\ so that we have a consistent delta setting for the gradient descent learning. (The triangle from \figro\ can be restored in \figroo\ as well by a suitable combination of embeddings --- see \sectref{codifun}).  


%, in which nodes are sm-categories and arrows are sm-functors. 
 %%%%%
 %\input{ll-figures/diags/policyfun-bigTri-OLD(defVersion)} % future work
 %\input{ll-figures/diags/policyfun-bigTri}
 %   \input{ll-figures/diags/policyfun-new}
%We will describe this diagram later in the paper, but for now note ....



\subsection{Our plan for the paper} %is as follows. 

The next section 
%is  motivational (why delta lenses can be useful in ML) and semi-formal; 
semi-formally explains delta lenses and relates them to abstract learners from \citefst. Formal results are presented next: Sect.~\ref{sec:alalens} defines ala-lenses, and several algebraic laws for them motivated by the MDE context; 
Sect.~\ref{sec:alalenscat} defines sequential and parallel composition of ala-lenses and proves two important results: a) preservation of lens laws by lens compositions, and b) the possibility to organize \alalens es into an sm-category (proofs are placed into the Appendix). 
%in Sect.~\ref{sec:alalens} and \ref{sec:alalenscat}:
 %(with proofs placed in Appendix), 
\zdmod{How the full-fledged delta lens \fwk\ can possibly be applied in ML is discussed in \sectref{deltas4ml}.}{REPHRASE!!}{rephrase}
and in \sectref{future} we discuss future work. %In more detail, \sectref{backgr} is a short primer on delta lenses with amendments, and in \sectref{deltas4ml} we discuss possible roles of metric and even non-metric deltas in ML. 
% meaning and role of deltas in ML. 
%Section~\ref{sec:alalens}  defines \alalens es and several algebraic laws for them motivated by the MDE context.  

\subsection{%Several remarks about the notation used in the paper. 
	About the notation used in the paper.}
	
	In general, an application of function $f$ to argument $x$ will be denoted by $f(x)$. But many formulas in the paper will specify terms built from two operations going in the opposite directions (this is in the nature of the lens formalism), and in our diagrams,  operation \get\ maps from the left to the right while operation \putl\ maps in the opposite direction. To minimize the number of brackets,  and relate a formula to its supporting diagram, we will also use the dot notation in the following way: %denote the application of function $f$ to argument $x$ by either $f(x)$, $f.x$ or $x.f$, and sometimes we will even use different ways within the same formula.  For example, if operation \get\ maps from the left to the right, operation \putl\ maps in the opposite direction, 
if $x$ is an argument in the domain of \get, we tend to write formula $x'=\putl(\get(x))$ as $x'=\putl(x.\get)$ while if $y$ is an argument in the domain of \putl, we tend to write the formula $y'=\get(\putl(y))$ as  $(\putl.y).\get=y'$ or $(\putl.y)\get=y'$.
% would perhaps be even more visually suggestive), 
Unfortunately, this discipline is not always well aligned with the in-fix notation for sequential (;) and parallel (||) composition of functions, %was recognized too late in the process of writing, and thus is not always followed % (especially when it requires writing $\putl.y$) 
so that some notational mix remained. 

Given a category \spA, its objects are denoted by capital letters $A$, $A'$, etc. to recall that in MDE applications, objects are complex structures (\eg, they can even be databases); the collection of all objects of \spA\ is denoted by $|\spA|$. An arrow with domain $A\in|\spA|$ is denoted by \frar{u}{A}{\_} and similarly \frar{u}{\_}{A'} is an arrow with codomain $A'$. A subcategory $\spB\subset\spA$ is called {\em wide} if it has the same objects. % (but fewer arrows). 
%Many formulas specify terms built from operations going in the opposite directions (this is in the nature of the lens formalism). To ease parsing of these formulas, the application of function $f$ to argument $x$ is denoted by either $y=f(x)$ or $x.f=y$ depending on where $f$ is directed in the related diagram: $y\lTo^f x$ for the former and $x\rTo^f y$ for the latter. This idea often conflicts with other useful requirements to formula writing: minimize the number of brackets and make reading intuitive (whatever that means). Bracket minimization and conformance to direction could be reconciled with the notation $y=f.x$ for $y=f(x)$, but it was realized too lately in the process of writing and is used in the paper for just few times. 

%\zd{write the colour piece better!}
%Colours in diagrams help to restore the scope of groups of operations, and partially their order (workflow), various sub- and super-scripts aim at helping this too.%
%\footnote{This resulted in perhaps excessive indexing but, again, it was understood too lately in the process of writing.} Yet another means to facilitate understanding the workflow underlying a complex diagram is to use animation (unfortunately, only applicable for presentations): the present author's experience in presenting complex diagrammatic terms (typical for categorical reasoning) for non-categorical audiences shows that animation can be quite useful, hence the use of Powerpoint for complex diagrams in the paper. 




%\input{ll-figures/diags/bigPicture}

\endinput

The second major technical  distinction from \citefjbx\ is that we model ML by {\em a}symmetric rather than symmetric lenses. Indeed, compositional ML considered in \citefetal\ is about composing functions rather than relations, and thus an asymmetric model seems to be more appropriate. In fact, symmetric lenses appear in \citefjbx\ as a means to model \parn\ within an ordinary lens \fwk, while we model \parn\ directly by adding a new ingredient to the \fwk; we will see that asymmetric \pard\ lenses (ap-lenses) are indeed a natural model for evolution (of model transformations in \bx) and learning (in the compositional ML). Moreover, we will use alenses with amendment....

Finally, we rearrange the methodological \fwk, in which ML and \Bx are considered. We introduce an abstract mathematical structure called an {\em abstract supervised learner (ASL)} and show that the compositional perspective on ML developed in \citefetal\ and \Bx are two different instances of the ASL structure.%
\footnote{As an analogy, think of mechanical or electrical or biological oscillation cases as instances of an abstract oscillation model given by the differential equation $ax''+bx'+c=r$} 
Perhaps, it makes sense to outline the main definition right away. An ASL is given by the following data: a sub-2-category \xcatcat{} (not necessary full) of \catcat\ and a pair of functors 
\begin{equation}
\end{equation}
where \xcatcat{p} is the category whose objects are categories from \xcatcat{} and arrows from a category \spA\ to a category \spB\ are parameterized functors, \ie, functors \frar{f}{\spP}{\xcatcat{}(\spA,\spB)} for some category \spP\ of {\em parameters} 

Specifically, the functor \ptol\ described above becomes a functor \frar{\learnfun_{\eps,\err}}{\paracat}{\aplenscat}, where two crucial learning  parameters: step size $0<\eps\in\Reals$ and an error function \frar{\err}{\Reals\timm\Reals}{\Reals}, are made explicit. % necessary to build the lens. 
Similarly, evolutionary \Bx should be modelled by a functor \frar{\Bxfun_\prpol}{\Bxcat}{\aplenscat}, where \Bxcat\ is a category of \pard\ model \trafon s (an analog of \paracat) and $\Bxfun_\prpol$ models the procedure of building a lens (\ie, a change/delta propagation device) based on some change propagation {\em policy}---a crucial ingredient making the backward propagation deterministic (analogous to the role of $(\eps,\err)$ in ML). 
We did not build such a functor in the paper -- it is a whole story left for future work, but the idea itself seems to be an accurate formalization of the notion of policy seen in the compositional perspective so that \Bxcat\ and \Bxfun\ should be sm. Thus, ML-\Bx interrelations can be formally specified by a cospan of functors above. %$\paracat\rTo^{\learnfun_{\eps,\err}}\aplenscat\lTo^{\Bxfun_\prpol}\Bxcat$ 

\endinput



==> ll-sections/intro-new.tex <==
\section{Introduction}\label{sec:intro}
	Modelling normally results in a set of inter-related models presenting different views of a single system at different stages of development. The former differentiation is usually referred to as {\em horizontal} (different views on the same abstraction level) and the latter as {\em vertical} (different abstraction levels beginning from the most general requirements down to design and further on to implementation). A typical modelling environment in a complex project is thus a collection of models inter-related and inter-dependant along and across the horizontal and the vertical dimensions of the network. We will call the entire collection a {\em multimodel}, and refer to its component as to {\em local} models.  

%	The system integrating local models can exist either materially (\eg, with UML modelling, a single UML model whose views are specified by UML diagrams, is physically stored by the UML tool) or virtually (\eg, several databases integrated into a federal database), or in a mixed way (\eg, in a complex modelling environment encompassing several UML models).  Irrespective of the type of integration (material, virtual, mixed), the most fundamental property of a multimodel is its  {\em global}, or {\em joint, consistency}: if local models do not contradict each other in their viewing of the system, then at least one system satisfying {\em all} local models exists; otherwise, we say local models are (globally) inconsistent.

If one of the local models changes and their joint consistency is violated, the related models should also be changed to restore consistency. This task of model \syncon\ 
is obviously of paramount importance for Model-Driven Engineering (MDE), but its theoretical underpinning is inherently difficult and reliable automatic synchronization solutions are rare in practice. %There are working solutions for file \syncon\ in systems like Git, but they are not applicable in the UML/EMF world of diagrammatic models.  For the latter, 
Much theoretical work partially supported by implementation has been done for the binary case (synchronizing two models) by the bidirectional transformation community (bx) in the \fwk\ of so called lenses -- algebraic structures specifying sync of two models via change propagation  %\cite{stevens-sosym10}, 
%specifically, by its TGG sub-community, see, \eg, \cite{hermann2012:concurrent}), and  the {\em delta lens}  sub-community on a more abstract level (delta lenses \cite{me-models11} can be seen as an abstract algebraic interface to TGG based \syncon\ \cite{frank-models11}). % , within the \fwk\ of so called {\em delta lenses} \cite{me-models11} that can be seen as , 
\footnote{
	Term {\em \Bx} abbreviates ``bidirectional $X$ (something)'' and refers to bidirectional change propagation in different contexts in different domains: file \syncon\ in versioning, data exchange in databases, model \syncon\ and model transformation in Model-Driven software Engineering (MDE), 
	%and virtually everywhere in engineering, 
	see \cite{bx-cross} for some of these contexts. What makes \Bx a special and united community amongst many circles studying \syncon\ and change propagation, is a foundational lens-based algebraic \fwk.  Nevertheless, within \Bx the application context can vary, sometimes significantly, and in the present paper, \Bx will mainly refer to \Bx in the MDE context --- the author's area of expertize in \Bx. %\textcolor{red}{trafos are views}
}   


The main goal of the present paper is to introduce a \fwk\ in which similarities between ML and \Bx become apparent. We will see that by abstracting away some details and ignoring the contextual differences, both problems can be seen as two different instantiations of the same algebraic structure defined in the paper and called \bfem{asymmetric learning lens, al-lens}. Indeed, lenses are devices specifying change propagation, and learning can be seen as a special change propagation case. For example, given (i) sets $A, B, P$ and  a family of functions 
$f=\comprfam{p\in P}{\frar{f_p}{A}{B}}$ as the learning space, and (ii) a training datum $(a,b')$ with $b'\noteq b=f_p(a)$ for an initially given parameter value $p$, we can interpret it as a change from a consistent state of the system $(a,p,b)$ to an inconsistent state $(a,p,b')$ caused by the change \warrbb. \Bx would fix this inconsistency by changing the input data \warraa\ so that the state $(a',p,b')$ is consistent, \ie, $f_p(a')=b'$; this action is often described as {\em propagating} change \warrbb\ to change \warraa. ML would call the original change \warrbb\ an error, and fix it by changing the parameter value \warrpp\ so that the state $(a,p',b')$ is either consistent, 
%\ie, $f_{p'}(a)=b'$, 
or at least less inconsistent than $(a,p,b')$ w.r.t. some metrics, \eg, we can add  metrics to set $B$ and require that $||f_{p'}(a), b'|| < ||f_p(a),b'||$. In ML terms, the system has {\em learnt} a better approximation $f_{p'}$ of the function; in \Bx terms, change \warrbb\ is propagated to \warrpp.  

\input{ll-figures/pdfs/mlbx-plane}
Abstract learners defined in \citefst\ do both propagations so that the updated/learnt state is $(a',p',b')$. The story is schematically described in the inset figure, in which the horizontal dashed arrow shows ML's evolution towards having back propagation (Bp) and the vertical arrow shows \bx's evolution towards \Bx with learning (\bxl, still to be developed; the work on deriving model transformations from examples \citemtex\ can be seen as \bxl). In the lens \fwk\ developed for \bx, point (1,1) corresponds to the idea of a learning lens, % defined in the present paper, 
which covers both ML and \bx. In the paper, %the notion of a learning lens allows us to work
we will work with asymmetric rather than symmetric learning lenses, which is a) technically much simpler and b) conceptually justified: compositional ML considered in \citefst\ is about composing functions rather than relations, and an asymmetric model seems to be more appropriate.  The main result of \citefjbx\ can then be seen as an ``internal lens business'': it says that any codiscrete al-lens can be encoded by a special symmetric non-learning lens. In the present paper, a lens always means an asymmetric lens.
% == nice piece !
%As asymmetric lenses are simpler than symmetric, and ordinary lenses are simpler than learning lenses, this results says that we can trade asymmetry for unparameterization, which is unexpected and nice, but can be encapsulated as an internal lens business not immediately related to interactions between ML and BX (of course, such observations are much easier to make after connections between ML and lenses were noticed in \citefjbx). 

Thus, the notion  of a codiscrete al-lens was actually discovered in \citefst.  The present paper makes three contributions to the learning lens idea consecutively described in three subsections below, after which we outline the structure of the rest of the paper. 

\subsection{Defining asymmetric learning delta lenses (al-lenses) and their composition  (sequential and parallel).
	% with amendment, \alalenscat.
} 
It could be called categorification of the learning lens notion: we will work with {\em delta} lenses,  in which a change/delta between objects $x,x'$ is an arrow \frar{u}{x}{x'} rather than a pair $(x,x')$; moreover, multiple different updates/deltas are possible between the same objects $x,x'$ so that $\Hom(x,x')$ is a set (non-empty for a typical \bx\ application in MDE). Each species of a delta lens has its codiscrete version, in which $\Hom(x,x')=\{(x,x')\}$, and learners defined in \citefst\ are exactly codiscrete al-lenses.%
\footnote{In detail, the category of learners \learncat\ defined in \citefst\ coincides with the category of codiscrete al-lenses \allenscatcodi, which is a  full sm-subcategory of the sm-category of al-lenses \allenscat.}
 In this paper, a lens will always mean a delta lens by default.  
%The original lenses of then become the codiscrete specialization of delta lenses. %, whose only arrows are pairs $(x,x')$ and any such a pair is an arrow (in \bx, any object $x$ can be updated to any other object $x'$ so that categories of objects of interests are bidirectionally connected: $\mathit{Hom}(x,x')\noteq\varnothing$ for any pair $x,x'$). In this paper, a lens will always mean a delta lens while lenses employed in \citefetal\ are referred to as codiscrete. 

In the MDE context, objects $x,x'$ are complex structures so that their delta/update \frar{u}{x}{x'} is a complex structure too. Its ignorance in the codiscrete lens formalism may create fundamental problems for applying codiscrete lenses to practical problems (see \cite{me-jot11}). The role of deltas in the ML context, where objects $x,x'$ are tuples of real numbers, is probably less fundamental but still important---we will briefly discuss it below in \sectref{ddlens-1}. %and continue  in \sectref{deltas4ml}. 

\subsection{%The second technical contribution of the paper is s
	Specification of algebraic laws for learning lenses and studying their preservation under lens composition. Building an sm-category \alalenscat\ of al-lenses with amendment.} 

For \bx, this is a crucial aspect: it says that if several synchronization modules satisfy some laws (are {\em well-behaved} in the lens parlance), then their composition is automatically well-behaved and hence the (usually expensive) integration testing is not needed. However, a major asymmetric BX lens law that requires consistency of the system after change propagation (called the PutGet law in the lens parlance) does not always hold in practice and needs to be relaxed \cite{me-fase18}. The relaxed PutGet is based on the idea of self-propagation: the change \warrbb\ is amended by a consecutive change \warrxy{b'}{b'^@:=f_{p'}(a')} so that the resulting state $(a',p',b'^@)$ is consistent.   Thus, \bx\ needs lenses with amendment, and the main construct of the paper is the notion of an \bfem{asymmetric learning lens with amendment, \alalens}, for which we will formulate \shortlong{two}{three} basic laws. We will define sequential and parallel composition of \alalens es, study their compatibility with the laws, and build an sm-category of well-behaved \alalens es, \alalenscat. The role of algebraic laws in the ML context is an intriguing subject left for future work. 

%Finally, yet another feature of the lens perspective on ML developed in this paper is to consider lenses with {\em amendments} recently defined in the \Bx context \cite{me-fase18} but, as we will see, having a natural ML motivation as well. Thus, lenses to be considered are al-lenses with amendments or {\em \alalens es}. 
%%and our compositional ML-\Bx story becomes a cospan of sm-functors
%%\begin{equation}\label{eq:mlbxcospan}
%% \paracat\rTo^{\learnfun_{\eps,\err}}\apalenscat\lTo^{\bxfun_\prpol}\bxcat
%%\end{equation}
%In the paper, we will define the category \alalenscat\ and prove it is \smm. We will also see that category \learncat\ of \citefst\ is nothing but the codiscrete version of \alalenscat. 
%%  We also reinterpret the functorial result of \citefst\ as shown in \eqref{mlbxcospan} by treating Euclidean spaces as Lawvere's metric spaces. The right part of (1) is left for future work.

%%==
%%\input{ll-figures/diags/policyfun}
%\input{ll-figures/diags/policyfun-ml-triangle}
%%\input{ll-figures/diags/policyfun-smallTri}

\subsection{Functoriality of learning algorithms in the {\em delta} lens setting}\label{sec:ddlens-1}
We will reconsider a major result in \citefst---compositionality of the mapping from learning spaces to learning algorithms, in the light of {\em delta} rather than {\em codiscrete} lenses. The compositionality above is specified by the commutative triangle in \figro,  in which nodes are sm-categories and arrows are sm-functors (and below we will omit the prefix sm). 

%==
%\input{ll-figures/diags/policyfun}
\input{ll-figures/diags/policyfun-ml-triangle}
%\input{ll-figures/diags/policyfun-smallTri}

Node $\paracatre$ denotes the category of (equivalence classes of) parameterized differentiable mappings $P\times\reals^m\rightarrow\reals^n$ (with the parameter space $P=\reals^k$), which is denoted by \paracat\ in \citefst\ but we add subindex \reals\ to recall the context, which will be important in our setting.
Arrow  \leefun\ is the functor built in \citefst\ with \eps\ and \err\ referring to parameters of the gradient descent learning (a step size and an error function $\reals\timm\reals\rightarrow\reals$ resp.), and ${-}\reals$ and ${-}\putl$ are two forgetful functors into the category of sets and (equivalence classes of) parameterized functors, \psetcat\ (%\footnote{C
considering parameterized functions up to some equivalence is needed to ensure associativity of their composition -- see \sectref{pcatcat} for details). Here and below we will denote a functor forgetting a part $X$ of its source objects' or/and arrows' structure by symbol ${-}X$. Similarly, functors adding a structural piece $X$ are denoted by $\plusx{\xyz}X$ with index \xyz\ referring to the mechanism by which this addition is realized.
%}

%\input{ll-figures/diags/policyfun-ml-topPart}
Our main observation is that functor \leefun\ is actually composed from two components %each having its own special role 
as shown by commutative square  (1) in \figroo, in which \alalensdifcat\ is the category of ala-lenses whose source and target model spaces are equipped with an operation \dif\ that given two objects $x, x'$ (\eg, two tuples in \realsx{n}), produces a delta between them, \ie, an arrow \frar{\dif(x,x')}{x}{x'} (\eg, for $x,x'\in\realsx{n}$, $\dif(x,x')=(x'_i-x_i)_{i\le n}$), and lens operations are compatible with \dif. Each delta lens with differencing gives rise (in fact, collapses) into a codiscrete lens, whose operation $\putlcodi$ works by, first, computing the required delta and then applying to it the delta lens \putl. We consider this construction in \sectref{codifun} and show that this construction amounts to a functor \frar{\codiscr}{\alalensdifcat}{\alalenscatcodi}.% 
\footnote{Importantly, as functor \codiscr\ forgets structural information about its source lenses,  its composition  with the obvious  full forgetful embedding of \alalenscatcodi\ into \alalensdifcat\ (see triangle (4) in the diagram, where this embedding is denoted by $\plusx{\pairing}(\deltas,\dif)$ as it adds necessary deltas and differencing by employing pairing of objects) is not identity on \alalensdifcat\ (but the converse composition $(\plusx{\pairing}(\deltas,\dif));\codiscr$ is the identity functor $\id_\alalenscatcodi$).}

\input{ll-figures/diags/policyfun-ml-topPart}
In comparison with functor \leefun\ considered in \citefst, the idea of gradient descent learning is more accurately described by functor \leefunovr\ because it does not include the forgetful functor \codifun\ into  the story (see triangle (1) in the diagram). Moreover, \leefunovr\ is itself composed as shown by triangle (2) of the diagram: the first component (the left edge) is an isomorphic representation of functions between Euclidean spaces-as-sets (denoted \realsx{n}) as functors between Euclidean spaces-as-categories (\rcatx{n}), whose arrows are componentwise differences, and the second component (the horizontal edge) is augmenting these functors with their special inverses called \putl s in the lens parlance. Building operations \putl s is essentially based on the gradient descent idea, hence, the notation 
$\plusx{Gd(\eps,\err)}\putl$ for this functor.  Adding \putl\ does not change the original functors \get s and triangle (3) formed with two obvious forgetful functors into \pcatcat\ commutes (category \pcatcat\ is the category of (equivalence classes of ) parametrized functors between small categories specified in \sectref{pcatcat}). Note that while commutativity of forgetting for functor \leefun\ is considered over \psetcat\ (see \figro), the context for \leefunovr\ is \pcatcat\ so that we have a consistent delta setting for the gradient descent learning. (The triangle from \figro\ can be restored in \figroo\ as well by a suitable combination of embeddings --- see \sectref{codifun}).  


%, in which nodes are sm-categories and arrows are sm-functors. 
 %%%%%
 %\input{ll-figures/diags/policyfun-bigTri-OLD(defVersion)} % future work
 %\input{ll-figures/diags/policyfun-bigTri}
 %   \input{ll-figures/diags/policyfun-new}
%We will describe this diagram later in the paper, but for now note ....



\subsection{Our plan for the paper} %is as follows. 

The next section 
%is  motivational (why delta lenses can be useful in ML) and semi-formal; 
semi-formally explains delta lenses and relates them to abstract learners from \citefst. Formal results are presented next: Sect.~\ref{sec:alalens} defines ala-lenses, and several algebraic laws for them motivated by the MDE context; 
Sect.~\ref{sec:alalenscat} defines sequential and parallel composition of ala-lenses and proves two important results: a) preservation of lens laws by lens compositions, and b) the possibility to organize \alalens es into an sm-category (proofs are placed into the Appendix). 
%in Sect.~\ref{sec:alalens} and \ref{sec:alalenscat}:
 %(with proofs placed in Appendix), 
\zdmod{How the full-fledged delta lens \fwk\ can possibly be applied in ML is discussed in \sectref{deltas4ml}.}{REPHRASE!!}{rephrase}
and in \sectref{future} we discuss future work. %In more detail, \sectref{backgr} is a short primer on delta lenses with amendments, and in \sectref{deltas4ml} we discuss possible roles of metric and even non-metric deltas in ML. 
% meaning and role of deltas in ML. 
%Section~\ref{sec:alalens}  defines \alalens es and several algebraic laws for them motivated by the MDE context.  

\subsection{%Several remarks about the notation used in the paper. 
	About the notation used in the paper.}
	
	In general, an application of function $f$ to argument $x$ will be denoted by $f(x)$. But many formulas in the paper will specify terms built from two operations going in the opposite directions (this is in the nature of the lens formalism), and in our diagrams,  operation \get\ maps from the left to the right while operation \putl\ maps in the opposite direction. To minimize the number of brackets,  and relate a formula to its supporting diagram, we will also use the dot notation in the following way: %denote the application of function $f$ to argument $x$ by either $f(x)$, $f.x$ or $x.f$, and sometimes we will even use different ways within the same formula.  For example, if operation \get\ maps from the left to the right, operation \putl\ maps in the opposite direction, 
if $x$ is an argument in the domain of \get, we tend to write formula $x'=\putl(\get(x))$ as $x'=\putl(x.\get)$ while if $y$ is an argument in the domain of \putl, we tend to write the formula $y'=\get(\putl(y))$ as  $(\putl.y).\get=y'$ or $(\putl.y)\get=y'$.
% would perhaps be even more visually suggestive), 
Unfortunately, this discipline is not always well aligned with the in-fix notation for sequential (;) and parallel (||) composition of functions, %was recognized too late in the process of writing, and thus is not always followed % (especially when it requires writing $\putl.y$) 
so that some notational mix remained. 

Given a category \spA, its objects are denoted by capital letters $A$, $A'$, etc. to recall that in MDE applications, objects are complex structures (\eg, they can even be databases); the collection of all objects of \spA\ is denoted by $|\spA|$. An arrow with domain $A\in|\spA|$ is denoted by \frar{u}{A}{\_} and similarly \frar{u}{\_}{A'} is an arrow with codomain $A'$. A subcategory $\spB\subset\spA$ is called {\em wide} if it has the same objects. % (but fewer arrows). 
%Many formulas specify terms built from operations going in the opposite directions (this is in the nature of the lens formalism). To ease parsing of these formulas, the application of function $f$ to argument $x$ is denoted by either $y=f(x)$ or $x.f=y$ depending on where $f$ is directed in the related diagram: $y\lTo^f x$ for the former and $x\rTo^f y$ for the latter. This idea often conflicts with other useful requirements to formula writing: minimize the number of brackets and make reading intuitive (whatever that means). Bracket minimization and conformance to direction could be reconciled with the notation $y=f.x$ for $y=f(x)$, but it was realized too lately in the process of writing and is used in the paper for just few times. 

%\zd{write the colour piece better!}
%Colours in diagrams help to restore the scope of groups of operations, and partially their order (workflow), various sub- and super-scripts aim at helping this too.%
%\footnote{This resulted in perhaps excessive indexing but, again, it was understood too lately in the process of writing.} Yet another means to facilitate understanding the workflow underlying a complex diagram is to use animation (unfortunately, only applicable for presentations): the present author's experience in presenting complex diagrammatic terms (typical for categorical reasoning) for non-categorical audiences shows that animation can be quite useful, hence the use of Powerpoint for complex diagrams in the paper. 




%\input{ll-figures/diags/bigPicture}

\endinput

The second major technical  distinction from \citefjbx\ is that we model ML by {\em a}symmetric rather than symmetric lenses. Indeed, compositional ML considered in \citefetal\ is about composing functions rather than relations, and thus an asymmetric model seems to be more appropriate. In fact, symmetric lenses appear in \citefjbx\ as a means to model \parn\ within an ordinary lens \fwk, while we model \parn\ directly by adding a new ingredient to the \fwk; we will see that asymmetric \pard\ lenses (ap-lenses) are indeed a natural model for evolution (of model transformations in \bx) and learning (in the compositional ML). Moreover, we will use alenses with amendment....

Finally, we rearrange the methodological \fwk, in which ML and \Bx are considered. We introduce an abstract mathematical structure called an {\em abstract supervised learner (ASL)} and show that the compositional perspective on ML developed in \citefetal\ and \Bx are two different instances of the ASL structure.%
\footnote{As an analogy, think of mechanical or electrical or biological oscillation cases as instances of an abstract oscillation model given by the differential equation $ax''+bx'+c=r$} 
Perhaps, it makes sense to outline the main definition right away. An ASL is given by the following data: a sub-2-category \xcatcat{} (not necessary full) of \catcat\ and a pair of functors 
\begin{equation}
\end{equation}
where \xcatcat{p} is the category whose objects are categories from \xcatcat{} and arrows from a category \spA\ to a category \spB\ are parameterized functors, \ie, functors \frar{f}{\spP}{\xcatcat{}(\spA,\spB)} for some category \spP\ of {\em parameters} 

Specifically, the functor \ptol\ described above becomes a functor \frar{\learnfun_{\eps,\err}}{\paracat}{\aplenscat}, where two crucial learning  parameters: step size $0<\eps\in\Reals$ and an error function \frar{\err}{\Reals\timm\Reals}{\Reals}, are made explicit. % necessary to build the lens. 
Similarly, evolutionary \Bx should be modelled by a functor \frar{\Bxfun_\prpol}{\Bxcat}{\aplenscat}, where \Bxcat\ is a category of \pard\ model \trafon s (an analog of \paracat) and $\Bxfun_\prpol$ models the procedure of building a lens (\ie, a change/delta propagation device) based on some change propagation {\em policy}---a crucial ingredient making the backward propagation deterministic (analogous to the role of $(\eps,\err)$ in ML). 
We did not build such a functor in the paper -- it is a whole story left for future work, but the idea itself seems to be an accurate formalization of the notion of policy seen in the compositional perspective so that \Bxcat\ and \Bxfun\ should be sm. Thus, ML-\Bx interrelations can be formally specified by a cospan of functors above. %$\paracat\rTo^{\learnfun_{\eps,\err}}\aplenscat\lTo^{\Bxfun_\prpol}\Bxcat$ 

\endinput



==> ll-sections/learners2lenses.tex <==
\subsection{An example of change propagation system: Learners as alad-lenses}

 %%==
\input{ll-figures/diags/policyfun-ml}
%%===


In this diagram, \pcatcat\ is the category of all small categories as objects and (equivalence classes of) parameterized functors between them as arrows.%
\footnote{The latter are functors \frar{f}{\spP\timm\spA}{\spB} or, equivalently, functors \frar{f}{\spP}{[\spA, \spB]} from some small category \spP\ into the category of functors $\spA\rightarrow\spB$ and their natural transformations; see \sectref{pcatcat} for details.}



The category of (small) sets and (equivalence classes of) parameterized functions, \psetcat, is fully embedded into \pcatcat\ by considering any set as a codiscrete category.  We name this embedding as \plusarrx{\pairing} to be read as ``add arrows by pairing'', \ie, by considering a pair $(a,a')\in A\timm A$ as an arrow $a\rightarrow a'$, which makes set $A$ a (codiscrete) category \spA.  Similarly, on the right side, we have a full embedding of the category of codiscrete ala-lenses into the category of delta ala-lenses. Finally, as any ala-lens is basically a pair $\get, \putl$ with \get\ a parameterized functor and \putl\ is its inversion in some special sense, we have a forgetful functor ${-}\putl$ (read ``forget \putl'') as shown in the diagram.  

Now we consider the upper row of the diagram. We can convert any Euclidean space $\reals^n$ into a category $\rcat^n$ whose arrows, \frar{\del}{a}{a'}, are deltas defined componentwise: $a=(a_i)_{i\le n}$, $a'=(a'_i)_{i\le n}$, and $\del=(\del_i)_{i\le n}$ with $\del_i=a'_i-a_i$. Functors \frar{\pmb f}{\rcat^n}{\rcat^n} and functions \frar{f}{\reals^m}{\reals^n} are in bijective correspondence. This gives us the commutative square (1) in which $\paracatrcat$ is the category of parameterized differentiable maps considered as functors, the upper arrow is an isomorphism, and vertical arrows are functors that forget the rich structure of \reals\ and consider it as either a set (the left edge) or a category (the right edge).  The central part of the story is given by the central square (2). The gradient descent idea (Gd) allows us to add to any parameterized functor \fbf\  in \paracatrcat\ with its inverse (in a certain sense)  mapping \putl\ so that the pair $(\fbf,\putl)$ makes an ala-lens with an additional operation of differencing, which for any two objects $x,y$ in a general category \spXX\ selects an arrow/delta \frar{\dif(x,y)}{x}{y} %called adelta between $x$ and $y$ 
(an accurate definition will be given in \sectref{codilens}). Forgetting first \dif\ and then \putl\ gives us a commutative square (2). Finally, a typical way of building codiscrete lenses in applications is to begin with a delta lens with differencing, which gives rise to a codiscrete lens in a functorial way--this gives us a general functor \codiscr\ (the right most edge in the diagram denotes equality: two different names for the same category). Note that square (actually, triangle) (3) is not %necessarily commutative and is not 
commutative for a general delta lens with diff, whose underlying lens is not codiscrete. However, the lenses in the image of functor $\plusx{Gd(\eps,\err)}\putl$ relate thin categories, so that the rectangle (2)+(3) is commutative. 


==> ll-sections/lenses-as-mm.tex <==
\clearpage
\section{Delta lenses as Mealy Machines}\label{lensesasmm}

% \begin{minipage}[t]{0.55\textwidth}
%\subsection{Delta lenses as coupled \mema s}
Presenting delta lenses in terms of \mema\ may be seen as a more ``physical'' view of mathematical constructs. In this section, we will begin with a notion of view as a function that, given a pair a categories, maps objects of the first to the objects of the second. We call such a function a {\em coupled space}. Then we define an incremental view computation as a forward \mema\ over a coupled space and see that it is nothing but a functor, while a backward update propagation defined as a backward \mema\ over a coupled space is nothing but a special case of the lifting construction called {\em cofunctor} by some authors \cite{?,?}. Finally, an (incrementally) updatable view is a coupled \mema\ consisting of a forward and a backward ones over the same coupled space, and it is nothing but an asymmetric delta lens. 
\begin{defin}[Mealy machines]
	A {\em (partial) Mealy machine (without an initial state)} is given by diagram \nim\ of sets and functions specified in \figref{mmdef}:
	\begin{figure}
		\begin{diagram}[small]
			\ineff && \rTo^{f} && \outeff
			\\  % row 2
			\dTo<{i}>{_{\jmm}}
			&\rdTo(2,2)>{i_S}
			&\pmb{\puncture}&\ldTo(2,2)<{o_S} 
			& \dTo>{o}<{_{\jmm}}
			\\ % row 3
			\ain && \stt && \aout
		\end{diagram}
		\caption{Defining diagram of Mealy machines, \nim}\label{fig:mmdef}
	\end{figure}
	%\zd{Draw the diagram in the order $In\subset \stt\timm\ain$ and make it a figure to ref?}
	Element of set  \stt\ are called {\em states}, sets \ain\ and \aout\ are {\em input {\em and} output alphabets}, function $f$ is the {\em transition function}, and pairs $\left((a,s), (s',b)\right)\in \ineff\timm\outeff$ related by $f$ are {\em transitions} (often written as arrows $ts\rTo^{a/b}s'$ with  $a$ called the trigger and $b$ the action of the transition).  
	%\end{minipage}~~
	% \begin{minipage}[t]{0.35\textwidth}
	%\end{minipage}
	The triangle is not required to be commutative (note the puncture symbol) so that a transition can update the state. If the triangle is commutative, the machine is called {\em stateless} (otherwise it is {\em stateful}). Pairs of functions %$(p_A,i_S)$ and $(o_S, p_B)$ 
	labelled by a predicate symbol \jmm\ are required to be jointly monic, (note the label \jmm),  hence, $\ineff\subseteq \stt\timm \ain$ and $\outeff \subseteq \aout \timm \stt$ (we prefer to order components of the products in this way), and the case $\ineff=\varnothing$ is not excluded. 
	%consider the state space as the first component in both products). 
	This is a major distinction from the ordinary definition, in which $\ineff=\stt\timm \ain$ and $\outeff=\aout\timm\stt$. We call sets \ineff\ and \outeff\ {\em effective} input and output sets resp. The triple $(\ain, \stt, \aout)$ is called the {\em base} of the \mema.
\end{defin} 

We will denote a \mema\ with an input alphabets \spA, output alphabet \spB,  and state space \spS\ by an arrow \fprar{m}{\spA}{\spB}{\spS}.%
\footnote{Formally, a Mealy machine is a (generalized \cite{makkai-ske}) sketch morphism \frar{m}{\nim}{\setcat} that sends pairs of arrows labelled \jmm\ into jointly monic pairs of functions in \setcat. When we refer to a \mema\ with input/output alphabets \spA, \spB\ and state space \spS, %and input/output sets \setin\ and \setout, 
	we mean that $m(\ain)=\spA$, $m(\aout)=\spB$, and $m(\stt)=\spS$ while sets  $m(\ineff)$ %=\setin$ 
	and $m(\outeff)$ %=\setout$ 
	are left implicit. 
}
\mema s can be composed: given \fprar{m1}{\spA}{\spB}{\spS_1} and \fprar{m2}{\spB}{\spC}{\spS_2}, we define \fprar{m1;m2}{\spA}{\spC}{\spS_1\timm\spS_2} by an obvious diagram chasing  (we begin with pullback of $o^{m1}$ and $i^{m2}$) that needs pullbacks and image factorization (and thus can be done in any regular \cat\ \zd{check with Freyd Scedrov}). To get associativity, we need to consider \mema s up to equivalence wrt. isomorphic state spaces. Two parallel \mema s \fprar{m_i}{\spA}{\spB}{\spS_i}, $i=1,2$ are called {\em equivalent} if there are isomorphisms \frar{\iota_{in}}{\ineff^{m_1}}{\ineff^{m_2}} and 
\frar{\iota_{out}}{\outeff^{m_2}}{\outeff^{m_1}} such that $f^{m_1}=\iota_{in};f^{m_2};\iota_{out}$ (and hence  $f^{m_2}=\iota_{in}^{-1};f^{m_1};\iota_{out}^{-1}$). It can be shown that 
\mema s considered up to equivalence can be equipped with a structure of an sm-category. We will not need this result in the paper, but it is paradigmatic for what we are going to do with lenses. 
%in the following way. First, we take the pullback of $o^{m2}$ and $i^{m2}$, let span \flar{\ovr{i}}{\setout^{m1}}{X}, \frar{\ovr{o}}{X}{\setin^{m2}} be the result. Then we define  $\setin^{m1;m2}\eqdef f1^{-1}(X_{12})$ and $\setout^{m1;m2}\eqdef $

\subsubsection{Notation.}  For the rest of this section, we will use the following notation: given a small category \spXX, let $\spXX_0$ and $\spXX_1$ denote sets of its objects and arrows resp. %of a category \spXX, 
The two functions giving the source and the target of an arrow are denoted by \frar{\so,\ta}{\spXX_1}{\spXX_0}, and the identity arrows of object $X\in\spXX_0$ is $\id_X$. %graph structure underlying \spXX\ is specified by 
Also, the (apex of the) pulback of  $\spXX_1\rTo^{\so}\spXX_0\lTo^{\id}\spXX_0$ will be denoted by $\spXX_1~{}_\so\timm_\id~\spXX_0$, or shorter $\spXX_1~{}_\so\timm\spXX_0$, or even shorter $\spXX_{10}^\so$, and its isomorphic dual from the PB of the inverse cospan is denoted by $\spXX_0\timm_\so\spXX_1$ or $\spXX_{01}^\so$. That is, we write up indexes identifying the left and the right feet, and the non-identity leg (\so\ in this case).  Similarly, we have isomorphic sets $\spXX_{01}^\ta$ and $\spXX_{10}^\ta$.

We model the notion of view by the construct of a coupled space.
\begin{defin}[Coupled spaces]
	A {\em coupled (asymmetric) space} is a triple $(\spA, \spB, \get_0)$ with \spA, \spB\ being small categories and \frar{\get_0}{\spA_0}{\spB_0} a function between their object sets. By an abuse of notation, we will refer to the entire coupled spaced by the same symbol $\get_0$ and denote it by an arrow \spabgeto. %\spabgeto
	%\trisprar{\get_0}{\spA}{\spB}
\end{defin}
For a given coupled space, we can extend our indexed notation, \eg, $\abois$ will denote the pullback of $\spA_0\rTo^{\get_0}\spB_0\lTo^\so\spB_1$ (where $\get_0$ is omitted like \id\ is omitted when we consider pullbacks withing a given model space \spXX), or \baiot\ is the pullback of $\spB_1\rTo^\ta\spB_0\lTo^{\get_0}\spA_0$

\input{ll-figures/diags/alens-as-mealy}
While a coupled space is a model of a view computation, an {\em incremental} view computation is modelled by the notion of a {\em forward} \mema\ over a coupled space.
\begin{defin}[Forward Mealy machine] % over a coupled space]
	A {\em forward Mealy machine} over a coupled space \spabgeto\    
	%	\trisprar{\get_0}{\spA}{\spB} 
	is given by (sets and functions in) the upper part of the diagram in \figref{alensmm}, which are required to satisfy equations (GetHit, Incidence, Increm) in  \eqref{eqmmget}. % for any value of their indexes in the specified domain. 
	The machine is called {\em functorial} if the monoidal axioms also hold. %{\em well-behaved (wb)} if the other two equations in \eqref{eqmmget} hold.  %Equation (Inc) regulates incidence between nodes and arrows,  and (GetOk) is a correctness requirement. Equation (GetId) says that identities are propagated to identities, and (GetGet) says that propagation of arrows is compositional.
\end{defin}
%\input{ll-figures/diags/alens-as-mealy}

It is easy to see that a forward machine is nothing but a graph-morphism, and monoidal laws make it a functor. %Note that  different functoriality conditions play different roles in our context. First of all, we consider arrows of a category as actions so that a category acts on its set fo objects, and a functor maps actions to actions. Then equation (Incidence) is a ``hygienic'' syntactical condition regulating incidence between nodes and arrows,  while (Increm) is a correctness requirement assuring the consistency of the system after update propagation. Equation (GetId) says that identities are propagated to identities, and (GetGet) says that propagation of arrows is compositional. 

\begin{defin}[Backward \mema]	 
	A {\em backward Mealy machine} over a coupled space \spabgeto\ is given by the lower part of the diagram in \figref{alensmm}, which are required to satisfy basic equations (Increm, Incidence, PutHit) in  \eqref{eqmmput}. The machine is called {\em Stable} (or {\em unital}) if the (PutId) equation in \eqref{eqmmput} holds.
	%	A {\em backward Mealy machine} over a coupled space $\get_0$ is given by the lower part of the diagram in \figref{alensmm} together with equation (Inc) in \eqref{eqmmput}. The machine is called {\em wb} if  equations (PutOk) and (PutId) in \eqref{eqmmput} (except PutPut!) hold as well.  Note that (PutOk) is also known as the PutGet law for objects. % Equation (Inc) regulates incidence between nodes and arrows, equation (GetId) says that identities are propagated to identities, and (GetOk) is a correctness requirement.
\end{defin}
\begin{lemma}
	A unital backward \mema\ is a unital semi-cofunctor as defined in \cite{?}
\end{lemma}

\begin{defin}[Coupled machine]
	A {\em coupled Mealy machine} over a coupled space \spabgeto\ is a pair $(\get,\putl)$ of Mealy machines sharing the same state space and alphabets (but swapping their roles) as specified in \figref{alensmm}; both machines are required to satisfy their basic laws, the forward machine is functorial and the backward is unital. A coupled machine is called {\em wb} if, in addition,  the PutGet law \eqref{eqmmputget} relating \get\ and \putl\ holds. %(The bijection \oiiso\ used in the formulation is defined by $\oiiso(u,A')=(u,A)$ for any \frar{u}{A}{A'} in \spA.) %
	%\footnote{Note that the definition can be internalized in any category that has pullbacks in a straightforward way (pullbacks are needed to define spans \Inget, \Input, \Outget\ and \Output, all the rest .} 
\end{defin}
Note the packaging of equations to make a machine well-behaved: GetGet is needed for wb-ness of both forward and coupled machines (the latter also require PutGet) while Putput is excluded. 
%\newcommand\cmealycat{\catname{cMealy}}
It is easy to see that a lens \frar{\ell=(\get, \putl)}{\spA}{\spB} is nothing but a coupled Mealy machine over the coupled space given by the object part of \get. The lens is wb iff the couple is wb. We can define sequential composition of forward Mealy machines as functors, and backward machines as shown in \figref{alens-compose}, which gives us a category of coupled machines \cmealycat\ and its subcategory of wb couples $\cmealycat_\wbind$. Obviously,
\begin{lemma}Categories of asymmetric (wb) lenses and (wb) coupled Mealy machines are isomorphic. 
\end{lemma}  

\subsection{Coupled \mema s with learning
	\footnote{In progress: To be revised}
}
%\input{ll-figures/diags/al0-lens-as-mealy}
%----
Now we have guidelines for incorporating the supervised learning idea into the lens \fwk. %straightforward (REALLY? :)
Given a set of parameters $\spP_0$, we make the state space a product $\spA_0\times\spP_0$ as shown in \figref{al-lens-mealy}. Parameterization of \get\ means that $\get.\ogpo=\igpo$ (but commutativity $\get.\ogao=\igao$ is not required). In contrast, neither of the two triangles for \putl\ is required to be commutative as the learning lens can update the parameter as well (and thus we have a single learning lens rather than a family of lenses). If the parameter space is a set, we will say that the lens learns {\em codicretely}: from any parameter $p$, any other parameter $p'$ is reachable in the learning process. Such unbounded learning  may not always be a good idea. \zd{To complete.....}

%\input{ll-figures/diags/alens-as-mealy}
\input{ll-figures/diags/al-lens-as-mealy-twoStates}
\input{ll-figures/diags/al-lens-as-mealy-twoPuts}
%\input{ll-figures/diags/al-lens-as-mealy-read}
%\input{ll-figures/diags/al-lens-as-mealy-big}


\begin{defin}[Asymmetric parametrized coupled spaces]
	A {\em parameterized coupled (asymmetric) space} is a quadruple  $(\spA, \spB, \spP, \get_{00})$ with \spA, \spB\ being small categories called the source and the target of the space, \spP\ a small \cat\ of {\em parameters}, and 
	\frar{\get_{00}}{\spP_0\timm\spA_0}{\spB_0} a function that we also consider (via Currying) 	as a family of functions \frar{\get_{00}}{\spP_0}{\spB_0^{\spA_0}}, whose application to an object $A\in\spA_0$ will be written as $A.\get_{00}(p)$ or $A.\get_{00p}$. 
	%$$	\comprfam{ 
	%		\frar{\get_{00}(p)=\get_{00p}}{\spA_0}{\spB_0}}
	%	{p\in\spP_0} $$
	%   % between the source and target object sets. %indexed by the object set of \spP. 
	%    %We will write its currying equivalent as a function . 
	We will denote such a space by an arrow 
	%	By an abuse of notation, we will 
	%	refer to a parameterized coupled spaced by $\get_0$ and write it as an arrow 	
	\pspabpgetoo. %\trispprar{\get_0}{\spA}{\spB}{\spP}.
	
	%A {\em parametrized functor (p-functor)} \fprar{\get}{\spA}{\spB}{\spP} over \pspabpgetoo\ is a functor \frar{\get}{\spP}{[\spA,\spB]} such that for any $p\in\spP_0$, $|\get_p|=\get_{00p}$. We will also say that functor \get\ extends $\get_{00}$.
\end{defin}
We again extend our indexing notation and, \eg, \bapioot\ is the pullback of $\spB_1\rTo^\ta\spB_0\lTo^{~\get_{00}}\spA_0\timm\spP_0$

\begin{defin}[Forward learning Mealy machine] % over a coupled space]
	A {\em forward learning Mealy machine} over a coupled space \pspabpgetoo\    
	%	\trisprar{\get_0}{\spA}{\spB} 
	is given by (sets and functions specified in) the upper part of the diagram in \figref{al-lensmm}, which is required to satisfy Basic Equations in  \eqref{eqmmgetP}. 
	The machine is {\em functorial} if monoidal laws also hold. 
\end{defin}
\begin{lemma}A forward learning \mema\ over coupled space \spabpgetoo\ gives rise to a functor \frar{\get}{\spP\timm\spA}{\spB} extending $\get_{00}$ and conversely, any such functor is a forward learning machine. Moreover, the categories of (equivalence classes of ) forward \mema\ and (eq. classes of) p-functors are isomorphic. 
\end{lemma}
%\begin{defin}[Forward learning Mealy machine]
%	A {\em forward learning Mealy machine} over a coupled space \pspabpget\ is given by the following two pieces of data.
%	
%	a) A family of forward Mealy machines over $\get_{0p}$, $p\inn\spP_0$, \ie, a family of functors \frar{\get_p}{\spA}{\spB} extending functions $\get_{00}$, and 
%	
%	b) For any arrow \frar{e}{p}{p'} in \spP, a natural transformation \drar{\get_e}{\get_p}{\get_{p'}} between functors. he following defini the upper part of the diagram in \figref{alensmm}, which is required to satisfy equations (Incidence, StateUpd) in the set \eqref{eqmmget}. % for any value of their indexes in the specified domain. 
%	The machine is called {\em well-behaved (wb)} if other three equations in \eqref{eqmmget} hold.  %Equation (Inc) regulates incidence between nodes and arrows,  and (GetOk) is a correctness requirement. Equation (GetId) says that identities are propagated to identities, and (GetGet) says that propagation of arrows is compositional.
%\end{defin}
%It is easy to see that a forward wb machine is nothing but a functor, but different functoriality conditions play different roles in our context. First of all, we consider arrows of a category as actions so that a category acts on its set fo objects, and a functor maps actions to actions. Then equation (Inc) is a ``hygienic'' syntactical condition regulating incidence between nodes and arrows,  while (GetOk) is a correctness requirement assuring the consistency of the system after update propagation. Equation (GetId) says that identities are propagated to identities, and (GetGet) says that propagation of arrows is compositional. 
\begin{defin}[Backward \& coupled Mealy machines]	 A {\em backward learning Mealy machine} over a coupled p-space \pspabpgetoo\ is given by the lower part of the diagram in \figref{alensmm} together with Basic Equation in \eqref{eqmmput}. The machine is called {\em unital semi-functorial} if  equations (PutId) in \eqref{eqmmput} (except PutPut!) hold as well.  %Note that (PutOk) is also known as the PutGet law for objects. % Equation (Inc) regulates incidence between nodes and arrows, equation (GetId) says that identities are propagated to identities, and (GetOk) is a correctness requirement.
	
	A {\em coupled Mealy machine} over a coupled space $\get_0$ is a pair $(\get,\putl)$ of Mealy machines sharing the same state space and alphabets (but swapping their roles) as specified by deiagram \figref{alensmm}. It is  {\em wb} if both machines are wb and, moreover, the PutGet law \eqref{eqmmputget} relating \get\ and \putl\ holds. %(The bijection \oiiso\ used in the formulation is defined by $\oiiso(u,A')=(u,A)$ for any \frar{u}{A}{A'} in \spA.) %
	%\footnote{Note that the definition can be internalized in any category that has pullbacks in a straightforward way (pullbacks are needed to define spans \Inget, \Input, \Outget\ and \Output, all the rest .} 
\end{defin}
Note the packaging of equations to make a machine well-behaved: GetGet is needed for wb-ness of both forward and coupled machines (the latter also require PutGet) while Putput is excluded. 

It is easy to see that a lens \frar{\ell=(\get, \putl)}{\spA}{\spB} is nothing but a coupled Mealy machine over the coupled space given by the object part of \get. The lens is wb iff the couple is wb. We can define sequential composition of forward Mealy machines as functors, and backward machines as shown in \figref{alens-compose}, which gives us a category of coupled machines \cmealycat\ and its subcategory of wb couples $\cmealycat_\wbind$.
\begin{lemma} Categories of (equivalence classes of ) (wb)) \mema\ and (eq. classes of) (wb) learning delta lenses are isomorphic. 
\end{lemma}
%\begin{lemma}Categories of asymmetric (wb) lenses and (wb) coupled Mealy machines are isomorphic. 
%\end{lemma}  

%\clearpage


==> ll-sections/ml-amend.tex <==
\subsection{ML with amendments}\label{sec:del4ml-amend}
Backward propagation to the input neuron layer does not make sense as input data are given, but backward propagation to an internal layer turned out a fruitful idea. Dually, it does not make sense to consider amendment to the output  layer as output data are also given, but amendments to an internal layer may turn out useful. In fact, backward propagation and amendments can be seen as two versions of basically the same idea: an intelligent optimization should be given the possibility to change the internal layer data irrespective to whether this layer is the input or the output of the training cell (= delta lens square as shown in \figri(a).  

==> ll-sections/ml-delta.tex <==
{\renewcommand\spP{\enma{P}}
\subsection{Non-metric deltas} \label{sec:del4ml-nonmetr}

In this section, we consider (somewhat speculatively) possibilities of non-metrical deltas between values in Euclidean spaces. The parameter space $\spP$ %=(\reals^k, E)$ 
is determined by the learning object --- a neural network \nin, and the gradient descent algorithm (Gd) optimizes the parameter value  $p\in\Reals^k=\spP$ built from biases of neurons in internal layers and weights of connections to and from them; the number $k$ is determined  by the network configuration and remains constant. Suppose, however, that on the learning path determined by Gd and back propagation (Bp), some internal layer neuron $X$ always fires; then it makes sense to remove it from the internal layer but add an input neuron constantly producing the \corring\ input data. Then numbers $k$ and $m$ (the number of input variables) change. Or, an intelligent learning algorithm can detect that learning improvement goes slowly due to the data from the same input neuron $Y$ so that removal of $Y$ and its connections significantly decreases the total error (\eg, think of a broken pixel in an image recognition scenario). This removal will change $m$ and $k$ (which depends on the number of connections). In general, we can assume intelligent learning algorithms that restructure the network \nin\ and change the number of variables in the input $\Reals^m$, parameter $\Reals^k$, and output $\reals^n$, spaces. To make intelligent decisions related to restructuring of the network, the learning algorithm should have a richer notion of deltas at the input and at the output. Below is a sketch of what such deltas could be as suggested by delta lenses.

\newcommand\nx{\enma{n_X}}
Consider a model space to be $\Reals^X$ with $X$ a finite set of variables $\{x_1...x_\nx\}$ (with \nx\ the cardinality of $X$). An object of the space is a  valuation \frar{a}{X}{\Reals}. % with $a_i=a(x_i)$. 
An updated object is a valuation \frar{a'}{X'}{\Reals} where $X'=\{x'_1...x'_{\nx'}\}$ is an updated set of variables, which, in general, somehow overlaps with $X$. The overlap is specified by a span of inclusions $X\lTo^{\iota_u} O_u\rTo^{\iota'_u} X'$, where index $u$ refers to the update/delta arrow \frar{u}{a}{a'}. A delta thus consists of three parts: set of deleted variables $X\setminus \iota_u(O_u)$, set of inserted variables $X'\setminus \iota'_u(O_u)$, and an error $E_u=\sum_{x\in O_u}|| a(\iota.x), a'(x.\iota')||$.
%(see \exref{mlasbx}). % for details).  
} %END GROUP

==> ll-sections/ml-diff.tex <==
\section{Functoriality of update policies
	%Codiscrete lenses as Delta Lenses with Differencing 
}\label{sec:policyfun-2}

In this section, we discuss.....

\subsection{Change propagation systems}

\renewcommand\fu{}
\renewcommand\wi{}

% \input{ll-figures/diags/policyfun}
%  \input{ll-figures/diags/policyfun-smallTri}
%\input{ll-figures/diags/policyfun-bigTri-OLD(defVersion)} % future work
\input{ll-figures/diags/policyfun-bigTri}
%   \input{ll-figures/diags/policyfun-new}

%\endinput
We continue the discussion in ....
We can model the notion of a context \nix\ as an %sm-subcategory $\pgetcat_\nix$ of the sm-category of parametrized functors \pcatcat\ (see Appendix \sectref{pcatcat}) or, better, as an 
sm-category $\pgetcat_\nix$ equipped with a forgetful functor \frar{{-}\nix}{\pgetcat_\nix}{\pcatcat} (read symbol `${-}\nix$' as ``forget the \nix-structure'') into the category \pcatcat\ of all small categories and (equivalence classes of) parameterized functors between them (see Appendix \sectref{pcatcat}).  The process of building \putl\ based on \get\ can be formalized as a 
%bijective on objects (bo) 
graph morphism \frar{\plusxput}{\pgetcat_\nix}{\alalenscat} from (the graph underlying) category $\pgetcat_\nix$ of parameterized \nix-functors to (the graph underlying) category of ala-lenses such that the internal triangle (*) in \figref{policyfun} on p.~\pageref{fig:policyfun} commutes. %$({+}_\nix\putl);({-}\putl)={-}\nix$ 
Read symbol `$\plusx{\nix}\putl$' as ``add \nix-determined operation \putl'' and `${-}\putl$' as ``forget operation \putl'' in a lens $\ell=(\get, \putl)$. The label $[{-}\nix]$ below arrow \plusxput\ is not a part of the functor name: it's a reminder that alongside with adding \putl, the functor also forgets the context/structure \nix. 

%\endinput
A central question of defining an update policy is whether it is functorial, that is, whether the graph morphism \plusxput\ is a functor. For example, a central result of \citefst\ is functoriality of \frar{\plusputx{Gd(\eps,\err)}}{\paracatre}{\learncat} where Gd refers to defining \putl\ via gradient descent with step size $\eps$ and  error function \err\ (see above), \paracatre\ denotes the category of (equivalence classes of) parameterized differentiable functions between Euclidean spaces, and \learncat\ is the category of codiscrete ala-lenses. The discussion above motivates the following formal definition.
%\begin{defin}\label{def:policyfun}
\par
\smallskip\noindent
{\bf Definition (Change propagation systems).}
An {\em asymmetric (parameterized, compositional) change propagation system with learning (CPS)} is a triple $\nix=(\pgetcat_\nix, {-}\nix, \plusxput)$ with \pgetcat\ being an sm-category  equipped with two sm-functors, ${-}\nix$ and \plusxput\ as shown in \figref{policyfun}, such that ${-}\nix$ is faithful, and the triangle (*) commutes. % functor commutative diagram of functors 

A CPS is called {\em codiscrete} if functor ${-}\nix$ factors through \psetcat\ and functor \plusxput\ factors through $\alalenscat_0$ as shown in \figref{policyfun}, where arrows with triangle tails denote full embeddings. Thus, a codiscrete CPS is a triple $\nix=(\pgetcat_\nix,{-}_0\nix, \plusxput_0)$ such that the external triangle (dashed arrows) in \figref{policyfun} commutes.
%\end{defin}

One may think that ML-motivated CPS considered in \citefst\ is codiscrete  but .......

%\endinput

\subsection{Delta lenses with differencing: their disassembling and assembling} 

Codiscrete lenses appearing in BX practice are delta lenses equipped with an additional {\em differencing} operation that automatically computes deltas (rather than delta lenses with forgotten deltas as is common to think about codiscrete lenses). We will sketch the corresponding formal \fwk. 
\subsubsection{Main definitions and facts}
\begin{defin}[Model spaces with differencing, dif-spaces]
	A {\em model space with differencing} is a pair $\spX=(|\spX|, \dif)$ with $|\spXX|$ a model space (= a strongly skeletal category) and \dif\ an operation that assigns to each pair of objects $X, X'\in||\spXX||$ an arrow $\frar{\dif(X,X')}{X}{X'} \in |\spXX|(X,X')$ between them, such that 
	
	\noindent\begin{tabular}{ll}
		\lawnamebr{DifId}{}
		& \mbox{$\dif(X,X)=\id_X$ for all $X\in|\spXX|$}
		\\
		\lawnamebr{DifDif}{}
		& \mbox{$\dif(X,X');\dif(X',X'')=\dif(X,X'')$ for all $X, X', X''\in|\spXX|$}
		\end{tabular}

\noindent By a typical abuse of notation, we will denote a dif-space \spXX\ and its carrier category by the same symbol \spXX. 
	
	A {\em dif-functor} between dif-spaces  is a functor \frar{\get}{\spS}{\spT} such that conditions Difget$_0$ below holds for any $S,S'$ in \spS. 
	%A natural dif-\trafon\ between two dif-functors \frar{\get_i}{\spS}{\spT}, $i=1,2$ is a natural \trafon\ \drar{\tau}{\get_1}{\get_2} such that condition Difget below holds.
	Dif-functors and their natural transformations form a category  denoted by $[\spS, \spT]$. 
	
		A {\em parametrized} dif-functor between dif-spaces  is given by a small category \spP\ of parameters, and a functor \frar{\get}{\spP}{[\spS, \spT]} such that conditions DifGet holds for any \frar{e}{p}{p'}. 
	
\noindent
\begin{tabular}{ll}
	\lawnamebr{DifGet}{$_0$}
	  &\mbox{$(S, S').\dif^\spS.\get =(S.\get, S'.\get).\dif^\spT$ }
	  \\
%	\lawnamebr{DifGet}{$_\tau$}
%      &\mbox{$(S, S').\dif^\spS.\tau =(S.\get, S'.\get).\dif^\spT$}
      	\lawnamebr{DifGet}{}
      &\mbox{$(S, S').\dif^\spS.\get_e =(S.\get, S'.\get).\dif^\spT$ 
  }
\end{tabular}
	\end{defin}

\input{ll-figures/diags/dif-space-triangle}
It is easy to see that similarly to \pcatcat, parameterized dif-functors between dif-spaces form an sm-category \pspadifcat, and the inset diagram commutes.
%It is easy to see that similarly to \pcatcat, parameterized dif-functors between dif-spaces form an sm-category \pspadifcat, and the inset diagram trivially commutes.




%
\begin{defin}[ala-lenses with differencing, alad-lenses]
	An {\em (well-behaved) alad-lens} from a dif-space \spS\ to a dif-space \spT\ is an ala-lens \frar{\ell=(\spP, \get, \putl)}{\spS}{\spT}, in which  %where \spP\ is a smal category of {\em parameters}, 
	\get\ is a parameterized dif-functor from \spS\ tp \spT, and condition DigPut holds for any $S$, $p$ and $T'$ in \spS, \spP, and \spT\ resp. (and where $S'$ denotes the target of $\putl^\req_{S,p}.\dif^\spT(S_p,T') $): %\putl\ operations are  compatible with differencing in the following sense:
		
		\noindent\begin{tabular}{ll}
		\lawnamebr{DifPut}{}
		&\mbox{$\dif^\spS(S, S') =\putl^\req_{S,p}.\dif^\spT(S_p,T')$ 
		}
	\end{tabular}
\end{defin}


\input{ll-figures/diags/codifun-triangle}
Alad-lenses form an sm-category \aladlenscat\ equipped with a forgetful functor ${-}\dif$ as shown in the diagram \figcodifun. What is special about alad-lenses is that any alad-lens \frar{\ell=(\spP,\get,\putl)}{\spS}{\spT} gives rise to a codiscrete lens  \frar{\ell^0=(\spP^0,\get^0,\putl^0)}{\spS^0}{\spT^0}, in which
$S.\get^0_p \eqdef S.\get_p$ and 
$\putl^{0\xyz}_{p}(S,T')\eqdef \cod.\putl^{\xyz}_{p,S}.\dif^\spT(S_p, T')$ 
for all $\xyz\in \{\req,\upd,\self\}$. Due to condition DifPut, this construction gives rise to a functor shown by the horizontal arrow in the triangle in \figcodifun. Importantly, for a general alad-lens the triangle does not commute as \codifun\ does not fully use the underlying delta lens structure: commuting only holds for thin dif-spaces whose Hom-sets are singletons. A more detailed story is given by rows (1-5) of the diagram \figcodifunbig\ (the vertical dashed arrow $[\plusx{\nix},\plusx{\nix}]$ actually originates at node $\pcatcat(\nix)$ and does not belong to rows (1-5) (its lower part is screened by arrow ${-}\nix$). Note that the pair of firgetful functors $({-}\lens, {-}\dif)$ is jointly monic.

%\input{ll-figures/diags/codifun}
\input{ll-figures/diags/codifun-new%
-withPara%
}

Now we can continue our discussion of compositionality of update policies, which we began on p.\pageref{fig:policyfun} with the notion of change propagation systems. 

%\endinput
\subsubsection{Building delta lenses.}

\zd{Fix outdated names of functors and revise}

Rows (1-5) of diagram \figcodifun\ show decomposition of dd-lenses and structure deletion, but in practice we need to go in the opposite direction and build lenses (and their codiscrete variants) by structure addition. That is, we  start with categories and functors (or sets and functions), \ie, the \get\ part, and then add to them  operations \putl s (and \dif\ if finally we want to build a codiscrete lens). This is a challenging task as there are many possibilities of adding  \dif s and \putl s so that the resulting dd-lens is well-behaved and, as a rule, there are no universal solutions amongst those possibilities. Hence, given a concrete context \nix\ in which \get s are defined (formally, a subcategory $\pcatcat(\nix)$ or $\psetcat(\nix)$ for the codiscrete case), we need a {\em selection policy} that would allow us to choose reasonable \dif s and \putl s so that the result would be a dd-lens suitable for the context \nix. 


If \nix\ is some model-to-model transformation context (BX), then category $\pcatcat(\nix)$ is roughly sketched in \sectref{backgr}, and operations \dif\ and \putl\ are to be carefully selected depending on the needs of a particular change propagation problem at hand---hence, names ${+}\dif(\pol)$ and ${+}\putl(\pol)$ for the corresponding arrows in the diagram \figrcodi, where \pol\ refers to the propagation policy. 


Similarly, if the context is ML, then we begin building dd-lenses from $\psetcat(\nix)$ being the category of Euclidean spaces and parameterized differentiable mappings between them (denoted \paracat\ in \citefst), \dif\ is the ordinary difference of reals, and a typical ML propagation policy is based on the gradient descent idea  (Gd). % and back-propagation (Bp) constructs. 
We will discuss this in more detail in the next section. Perhaps, connections between open games (OG) and lenses can be treated similarly by considering OG as a special case of context \nix. 

\subsection{An example of change propagation system: Learners as alad-lenses}

 %%==
\input{ll-figures/diags/policyfun-ml}
%%===


In this diagram, \pcatcat\ is the category of all small categories as objects and (equivalence classes of) parameterized functors between them as arrows.%
\footnote{The latter are functors \frar{f}{\spP\timm\spA}{\spB} or, equivalently, functors \frar{f}{\spP}{[\spA, \spB]} from some small category \spP\ into the category of functors $\spA\rightarrow\spB$ and their natural transformations; see \sectref{pcatcat} for details.}



The category of (small) sets and (equivalence classes of) parameterized functions, \psetcat, is fully embedded into \pcatcat\ by considering any set as a codiscrete category.  We name this embedding as \plusarrx{\pairing} to be read as ``add arrows by pairing'', \ie, by considering a pair $(a,a')\in A\timm A$ as an arrow $a\rightarrow a'$, which makes set $A$ a (codiscrete) category \spA.  Similarly, on the right side, we have a full embedding of the category of codiscrete ala-lenses into the category of delta ala-lenses. Finally, as any ala-lens is basically a pair $\get, \putl$ with \get\ a parameterized functor and \putl\ is its inversion in some special sense, we have a forgetful functor ${-}\putl$ (read ``forget \putl'') as shown in the diagram.  

Now we consider the upper row of the diagram. We can convert any Euclidean space $\reals^n$ into a category $\rcat^n$ whose arrows, \frar{\del}{a}{a'}, are deltas defined componentwise: $a=(a_i)_{i\le n}$, $a'=(a'_i)_{i\le n}$, and $\del=(\del_i)_{i\le n}$ with $\del_i=a'_i-a_i$. Functors \frar{\pmb f}{\rcat^n}{\rcat^n} and functions \frar{f}{\reals^m}{\reals^n} are in bijective correspondence. This gives us the commutative square (1) in which $\paracatrcat$ is the category of parameterized differentiable maps considered as functors, the upper arrow is an isomorphism, and vertical arrows are functors that forget the rich structure of \reals\ and consider it as either a set (the left edge) or a category (the right edge).  The central part of the story is given by the central square (2). The gradient descent idea (Gd) allows us to add to any parameterized functor \fbf\  in \paracatrcat\ with its inverse (in a certain sense)  mapping \putl\ so that the pair $(\fbf,\putl)$ makes an ala-lens with an additional operation of differencing, which for any two objects $x,y$ in a general category \spXX\ selects an arrow/delta \frar{\dif(x,y)}{x}{y} %called adelta between $x$ and $y$ 
(an accurate definition will be given in \sectref{codilens}). Forgetting first \dif\ and then \putl\ gives us a commutative square (2). Finally, a typical way of building codiscrete lenses in applications is to begin with a delta lens with differencing, which gives rise to a codiscrete lens in a functorial way--this gives us a general functor \codiscr\ (the right most edge in the diagram denotes equality: two different names for the same category). Note that square (actually, triangle) (3) is not %necessarily commutative and is not 
commutative for a general delta lens with diff, whose underlying lens is not codiscrete. However, the lenses in the image of functor $\plusx{Gd(\eps,\err)}\putl$ relate thin categories, so that the rectangle (2)+(3) is commutative. 


\zd{A HUGE outdated PIECE IS END-INPUTED}

\zd{But it seems that it is in the APPENDIX E now}

\endinput


\endinput
\input{ll-sections/derivatives-as-functors}
\section{Learners as delta lenses %: Functoriality of differentiation
}\label{sec:derifun}
%\newcommand\leefun{\enma{L_{\eps,\err}}}


In this section, we sketch  how the functor \frar{\leefun}{\paracat}{\learncat} specified in \citefst\ could be derived along the dd-lens lines described above as the composition $\leefun=({+}
\mathsf{deltas});!;\codifun$, where $!$ is the unique functor determined by pair $({+}\dif(pol), {+}\putl(pol))$ due to the universal property of products and the fact that the image of $!$ satisfies the condition of being a well-behaved dd-lens. 

\newcommand\figrcomp{\figref{difasfun}}
\subsubsection{Derivative as a functor.} Our first observation is that differentiability can be seen as functoriality. 
Let \frar{f}{\reals}{\reals} be a differentiable function, whose derivative is denoted by $\prt f$, $a,a'$ are two reals and $\del=a'-a$ is their difference treated as an arrow \frar{\del}{a}{a'}. %---subindex $a$ is used to suggest that we consider $a'-a$ as an action (we will also say {\em edit}) applied to value $a$ so that $(\reals, +, 0)$ becomes a monoid acting on \reals. 
%%(The difference $a'-a$ plays yet another role of a distance between $a$ and $a'$, below we will discuss it in more detail.) 
If \del\ is small enough, then $f(a')-f(a)\approx \del\cdot\prt f(a)$ and we can say that $\prt f(a)$ maps arrow \del\ to arrow \frar{\del.\prt f(a)}{a.f}{a'.f}. If function $f$ maps from the left to the right, we will often use the dot notation for function application so that \frar{\del.\prt f_a}{a.f}{a'.f}, where $\prt f_a$ denotes $\prtf(a)$. %the value of the differential $\prt f(a)$ at point $a$.

%-- the gradient version ---
%Let \frar{f}{\reals^m}{\reals} be a differentiable function, whose gradient is denoted by $\nabla f$, $a,a'$ are two $m$-tuples of real numbers, and $\del=(\del_1...\del_m)$ %a'-a=(a'_1-a-1,....,a'_m-a_m) is their componentwise difference, $\del_i=a'_i-a_i$, $i\le m$, treated as an arrow \frar{\del}{a}{a'}. If all $\del_i$ are small enough, then $f(a')-f(a)\approx \nabla f(a)\cdot\del$ (where $\cdot$ denotes the scalar product) and we can say that $\nabla f(a)$ maps arrow \del\ to arrow \frar{\nabla f(a)(\del)}{f(a)}{f(a')}. The generalization for the case \frar{f}{\reals^m}{\reals^n} is straightforward by considering $f$ a tuple $f_j, j\le n$ and Jacobian matrix $\jacobf=(\prt_if_j: i\le m, j\le n)$ replacing the gradient. To encompass all cases, we will call a linear operator mapping deltas from $a$ to deltas from $f(a)$ a {\em differential} and write  $\prtf(a)$ or often $\prtf_a$. If function $f$ maps from the left to the right, we will often use the dot notation for function application so that \frar{\del.\prt f_a}{a.f}{a'.f}, where $\prt f_a$ denotes the value of the differential $\prt f(a)$ at point $a$.

If deltas are not infinitely small, then $a'.f=a.f+\del.\prtf_a+o(\del)$ as shown by square (1) in diagram \figrcomp a, where \medadx{f} denotes $a.f+\del.\prtf_a$, and term $o(\del)$ converges to $0$ if \del\ converges to $0$. (If \frar{f}{\reals}{\reals} is an analytic function, then $o(\del)$ is the part of its Taylor series representation starting with the second order derivative, $o(\del)=\prt^2f_a\cdot\del^2/2!+\prt^3f_a\cdot\del^2/3!+\ldots$). If we consider \reals\ as a category \rcat\ whose arrows are triples $(a,\del,a')$ such that $a'=a+\del$, and composition $\del;\del'$ is given by addition, then differentiation becomes a functor-like mapping as shown by diagram  \figrcomp a. Diagram \figrcomp b, in which commutative ``rectangles'' (12) and (12') define $\prt(f;g)$, specifies the chain rule. 
\begin{remark}\label{rem:del-as-act}
	Commutativity of rectangle (11) in \figrcomp a is trivial as \rcat\ is a thin category. We can make it more interesting if....
\end{remark}
Generalization for the case \frar{f}{\reals^m}{\reals^n} is straightforward with $a,a'$ being $m$-tuples of real numbers, $\del=(\del_1...\del_m)$ %a'-a=(a'_1-a-1,....,a'_m-a_m) is 
their componentwise difference, Jacobian matrix $\jacobf=(\prt_i f_j: i\le m, j\le n)$ being the differential and $\jacobf\cdot\del$ is matrix-vector multiplication. If $n=1$, then \jacobf\ is gradient $\nabla f$. %, whose value at vector $a$ will be denoted by $\nabla_a$. 
To encompass all cases, we will call a linear operator mapping $m$-dimensional deltas from $a$ to $n$-dimensional deltas from $f(a)$ a {\em differential} and write  $\prtf(a)$ or often $\prtf_a$. 
%
An $m$-dimensional space $\reals^m$ is converted into category $\rcat^m$ componentwise. 

%======
%\input{figures/diags/difasfun1}
\input{figures/diags/difasfun3}
%====
%\input{figures/pdfs/getAmend-inR}
%====

\newcommand\couplarr[1]{\enma{#1^{\gg}}}
Now we define an abstract version of the above. %Given a category \spXX\ and an object $X\in|\spXX|$, we write $\spXX(X,\_)$ and $\spXX(\_,X)$ for classes \compr{\frar{u}{X}{X'}}{X'\in|\spXX|} and \compr{\frar{u}{X'}{X}}{X'\in|\spXX|} resp. 
Given a category \spXX\ and objects $X,X'\in|\spXX|$, we write $\couplarr{\spXX}(X,X')$ for the set of pairs of arrows 
%
\compr{(u,u')\in\spXX(X,Y)\timm\spXX(Y,X')}{Y\in|\spXX|} 
%
\noindent determined by the obvious pullback. 
\begin{defin}[Quasi-functors]\label{def:qfun}
Given categories \spA, \spB, a {\em quasi-functor} 
%$\spA\rightarrow\spB$ 
\frar{f^\gg}{\spA}{\spB} is given by i) an object function \frar{|f|}{|\spA|}{|\spB|} and ii) for any $A,A'\in|\spA|$, a mapping \frar{f^\gg_{AA'}}{\spA(A,A')}{\spB^\gg(B,B')} where $B=|f|(A)$, $B'=|f|(A')$. Given \frar{u}{A}{A'}, we consider the first component of pair $f^\gg_{AA'}(u)$ as the main value and denote it by $f_{AA'}(u)$ while the second component is called an {\em amendment} and denoted by $f_{AA'}^@(u)$. We say quasi-functor $f$ is {\em functorial at $u$} if $f_{AA'}^@(u)=\id_{B'}$, and {\em functorial at $A,A'$} if it is functorial at all \frar{u}{A}{A'}.  As a rule, we will omit indexes and write $f(u)$ for the main value and $f^@(u)$ for its amendments. %By an abuse of notation, 
The composition of pair $f^\gg_{AA'}(u)$, \ie, arrow $f(u);f^@(u)$, will be  denoted by $f^\gg(u)$. All this abuses notation but the context should make it clear.


Moreover, the following two functoriality conditions are required to hold for quasi-functors: unitality, \ie, for any $A$, $f(\id_A)=f^@(\id_A)=\id_{|f|(A)}$, and composition preservation  (cf. diagram \figrcomp a), which requires for any \frar{u}{A}{A'}, \frar{u'}{A'}{A''}, the following equation:
\begin{equation}\label{eq:qfun}
       f^\gg(u;u')=f^\gg(u);f^\gg(u') 
\end{equation}
%And for any $A$, $f(\id_A)=f^@(\id_A)=\id_{|f|(A)}$.
If $f$ maps from the left to the right, we will use the dot notation $u.f$, $u.f^@$. 
\end{defin}

The intuition that in the pair $u.f^\gg_{AA'}$, the component $u.f$ is the main value while $u.f^@$ is its amendment is formalized by the following definition of quasi-functor composition. Given two quasi-functors \frar{f}{\spA}{\spB} and \frar{g}{\spB}{\spC}, their {\em composition} $f;g$ or just $fg$ is defined by the following triple of mappings:  $|fg|:=|f|;|g|$ and, for any \frar{u}{A}{A'}, $u. fg := u.f .g$ and $u.(fg)^@:=(u.f.g^@);(u.f^@.g^\gg)$ (cf. diagram \figrcomp b). %Note that it is the definition of composition, which formalizes the intuition of the second component of a quasi-functor as an amendment.

Obviously, if $f$ and $g$ are unital, then $fg$ is such, and it is straightforward to check by multiple substitution, that if $f$ and $g$ preserve composition according to \eqref{qfun}, then $fg$ preserves composition too. Hence, $fg$ is a quasi-functor as soon as $f$ and $g$ are such. The identity functor on \spA\ is also the identity quasi-functor on \spA, and we thus have a category \qcatcat. Moreover, componentwise paring equips this category with an sm-structure: given parallel quasi-functors \frar{f_i}{\spA_i}{\spB_i}, $i=1,2$, we define $u_1\paar u_2.\,f_1\paar f_2=u_1. f_1\paar u_2.f_2$ and $u_1\paar u_2.\,(f_1\paar f_2)^@=u_1. f_1^@\paar u_2.f_2^@$. Checking sm-category axioms is straightforward. 
%\begin{lemma} The collection of all small categories and quasi-functors between them is a category \qcatcat. %Condition \eqref{qfun} holds for the above triple, and hence the latter determines a quasi-functor \frar{f;g}{\spA}{\spC}
%\end{lemma}

\subsubsection{Differentiating parameterized functions}
%====
\input{ll-figures/pdfs/getAmend-twoFig}
%====

Consider \frar{f}{\spP\timm\reals^m}{\reals^n}, where $\spP=\reals^k$ is a parameter space. Differentiating over parameters for a fixed $a\in\reals^m$, gives us an operator $\prt_p f(p,a)$ mapping parameter deltas \frar{e}{p}{p'} from $p$ into $\reals^n$-deltas from $a.f_p:=f(p,a)$ (as usual, we use symbol $p$ in two roles: as a variable running over \spP\ in $\prt_p f$ and as a fixed parameter value in other expressions). Similarly, differentiating over variables in $\reals^m$  for a fixed parameter $p\in\reals^k$, gives us an operator $\prt_a f(p,a)$ mapping deltas \frar{\del}{a}{a'} from $a$ into $\reals^n$-deltas from $a.f_p$. Diagram in \figgetam a describes the ingredients of the story as arrows. Intermediate vertical arrow from $a.e\prt_p$ has the same label as its counterpart on the left as we consider the delta $\hat \del :=\del.\prt_af(p,a)$ as acting on values in $\reals^n$, and we label the result of applying $\hat \del$ to $b\in \reals^n$ by $\hat \del$ so that different arrows from different $b$s get the same label. Similarly, two different horizontal arrows from $a.f_p$ and $a.\del\prt_a$ have the same action label too. 

An abstract delta lens formulation of the story is given by the following definition illustrated by diagram \figgetam b. 
\begin{defin}[incremental view system]\label{def:viewsys}
	Let \spS\ and \spT\ be model spaces. An {\em (incremental parametrized) view system} 	from \spS\ (the {\em source} of the view) to \spT\ (the {\em target}) is given by i) a category \spP\ of {\em parameters} (think about function/view definitions \parrd\ by objects of \spP) and ii) a quasi-functor \frar{\get}{\spP\timm\spA}{\spB}. A view system is called {\em codiscrete} if categories \spS, \spT, \spP\ are codiscrete.
\end{defin}

In the parametrized setting,  we have a differentiable function \frar{f}{P\times\reals^m}{\reals^n} with $P=\reals^k$ being the parameter space. %, and a differentiable error function \frar{\Err}{\reals^m}{\reals}, whose composition gives us differentiable  function \frar{E}{P\times\reals^m}{\reals}. 
We can convert this data into a double-indexed family of functors-as-monoid- homomorphisms  \frar{\get_{p,a}}{\DDel^m}{\DDel^n}, $p\in P, a\in \reals^m$ %, by, first, converting all Euclidean spaces into categories as described above, and then, 
by the two upper equations in \eqref{mlgetdef}: %as follows: for a given parameter $p$, parameter delta \frar{\Delp=(p'-p)}{p}{p'}, m-tuple of reals $a$ and input variables delta \frar{\Dela=(a'-a)}{a}{a'}, we define%
\footnote{as usual, by the abuse of notation we will denote variable and its fixed value by the same symbol $a$} 
%\begin{minipage}[t]{0.5\textwidth}
\begin{equation}\label{eq:mlgetdef}
\begin{array}{c}
\get_p(a)=f(p,a)
\\
\get_{p,a}(\dela)=\Dela*\nabla_af(p,a)
\\
\get_a(\Delp)=\Delp*\nabla_pf(p,a)
\end{array}
\end{equation}
%\end{minipage}
(where the last equation specifies natural transformation  $\get(\Delp)$). Thus, we have a parameterized functor or the \get-part of a dd-lens: the differencing operation is uniquely defined so that Difdif holds, and it is straightforward to check conditions \eqref{difget}.  In terms of diagram \figrcodi, we have built functors ${+}\mathsf{deltas(\pol)}$ and ${+}\dif(\pol)$.


\subsubsection{Gradient descent as an update propagation policy
	%Model spaces as metric spaces.
}
Metrics, \ie, setting a distance between values considered as an {\em error} is an important part of the story. %We will need also some metrics on differences considered as errors. 
Following \citefst, we assume that some  differentiable function \frar{\err}{\reals\times\reals}{\reals} is given, and %actions of monoid $\DDel=(\reals,+,0)$ are considered as opliftings: 
then given $a\in\reals$ and edit $\delta \in\DDel$, the result of applying $\delta$ to $a$ is an arrow \frar{\ovr{\delta}=\err(a,a')}{a}{a'}. For the multiple variables case $\reals^m$, a delta is a vector $\del=(\del_1,...,\del_m)$ acting componentwise, and the result of applying it to value $a=(a_1...a_m)$ is an arrow/distrance  \frar{\ovr{\del}=\Err(a,a')}{a}{a'} computed by summation: $\Err(a,a') :=\sum_{i\le m}\err(a_i,a'_i)=\sum_{i\le m}\err(a_i,a_i+\del_i)$.  
%considered as an arrow \frar{\ovr{\delb}}{b}{b'}
with $b=f(a)$ and $b'=f(a')$. Thus, an accurate setting would be to consider an asymmetric edit delta lens (see \cite{jr-unified} for a definition for the codiscrete case) whose model spaces are Lawvere categories (metric spaces). However, delta lenses subsume edit lenses (see \cite[sect.??]{me-jot11} for the idea and examples, and \cite{jr-unified} for formal results), and below we will work in the delta lens setting, in which deltas are pairs $(\del,\ovr{\del})$ where $\del=a'-a$ and $\ovr{\del}=\err(\del)$.  %As it was shown in \cite{jr-unified}, 

In the setting of \citefst,

For defining the \putl-part, we need a policy, and the gradient descent method gives us one. We can treat formulas in \citefst\ for computing the updated parameter $p'$ (for a given step size \eps) and updated input value $a'$ as $\putl^\upd$ and $\putl^\req$ operations mapping delta $\Del_b=b-E(p,a)$ to deltas $p'-p$ and $a'-a$ resp. (and conditions \eqref{difputupdself} (upper) and \eqref{difputreq} are automatically satisfied). We can also set $\putl^\self(\Del_b)=E(p',a') - b$ so that condition \eqref{difputupdself}(bottom) is also satisfied. Moreover, the Putget laws holds too. Thus, we have a (well-behaved) dd-lens. In terms of diagram in \figrcodi, we built functor ${+}\putl(\pol)$ and showed that the universal arrow $!=[{+}\dif(\pol), {+}\putl(\pol)]$ targets at the category of well-behaved dd-lenses as shown in the diagram.
%
%Probably, the entire construction would be more transparent and manageable (\eg, with respect to generalizations) if we consider this dd-lens as sequentially composed from two dd-lenses: \frar{\ell_\eps(f)}{\reals^m}{\reals^n} and \frar{\ell(\err)}{\reals^n}{\reals} (whose parameter space is \tcat). This elaboration is also left for future work. 

Finally, by applying the codiscretization functor, we arrive at the category of codiscrete ala-lenses, which gives us derived functor ${+}\putl0(\pol)$.   

%An Euclidean space $\reals^n$ can be seen as a category $\rcat^n$ enriched in $\niv=(\reals^n, +)$: given two tuples $a, a' \in \reals^n$, we define $\rcat^n(a,a')= (a'- a)$. A differentiable function \frar{f}{\reals^m}{\reals^n} can then be seen as a functor \frar{\get}{\rcat^m}{\rcat^n} whose object part is $f$, and the arrow part is the derivative: $\get(a'-a)=$

==> ll-sections/ml-metric.tex <==
\subsection{Metric deltas
	%Euclidean spaces as Lawvere's metric spaces and ML 
	%ML over distance non-increasing functions
} 



The main result of \citefst\ states the existence of an sm-functor \frar{L_{\eps, \err}}{\paracat}{\learncat}, where \paracat\ is the category whose objects are Euclidean spaces $\reals^n$, $n\in\ints$, and arrows are differentiable parameterized functions between them, \ie, (equivalence classes of) differentiable functions \frar{f}{P\times\reals^m}{\reals^n} with the parameter space $P=\reals^k$. Functor $L_{\eps, \err}$ is determined by two parameters: a {\em step size} $0<\eps\in\reals$ and an {\em error function}  \frar{\err(x,y)}{\Reals\timm\Reals}{\Reals} such that \frar{\prtfrac{\err}{x}(x_0,\_)}{\Reals}{\Reals} is invertible for any given $x_0\inn\reals$. In \bx\ terms, \eps\ and \err\ determine a {\em propagation policy} necessary to determine the \putl\ operations in the lens $L_{\eps,\err}(f)$. Importantly, while \err\ is needed for all \putl\ operations as it determines the cost function, \ie, the {\em total error} function $E_I(p,a,b)= \sum_{i\le n}\err(I_i(p,a),b_i)$ to be minimized by changes in $(p,a,b)$, the step size \eps\ is only needed for computing the change of $p$ while changing $a$ is based on a predefined idea of invertibility (see \citefstx{Sect.III} for details). In this light, a more suggestive notation for $L$ would be $L_{\err,\eps,\inv}$. 

The delta lens \fwk, gives us a somewhat different interpretation. Given an {\em error} function  \frar{\err}{\Reals\timm\Reals}{\Reals}, an $n$-dimensional Euclidean space $\reals^n$ can be converted into a metric space by  defining the {\em total} error  \frar{\Err}{\reals^n\times\reals^n}{\reals} by $\Err(x,x')=\sum_{i\le n}\err(x_i, x'_i)$. This also makes space $\reals^n$ a category enriched over Lawvere's monoidal poset $([0,\infty],\ge,+,0)$ (Lawvere's metric space) $\rcat^n_\err$, and get-view functors \frar{f_p}{\rcat^m_\err}{\rcat^n_\err} are exactly non-expanding (\ie, distance non-increasing) functions. It gives us a category \paracaterr, which is widely embedded into \paracat\ but has fewer arrows: only non-expanding functions from \paracat\ occur into \paracaterr. Now the learning functors  \frar{L_{\err,\eps,\inv}}{\paracat}{\learncat} are reshaped as functors \frar{L_{\eps,\inv}}{\paracaterr}{\learncat}. %% where  \paracaterr\ is the category whose objects are Euclidean spaces and arrows are differentiable distance-non-increasing differentiable parameterized functions 
%Note the commutativity $\emb;L_{\err,\eps,\inv}=L_{\eps,\inv}$ where \frar{\emb}{\paracaterr}{\paracat} is the embedding described above. 

\newcommand\lmp{\enma{[0,\infty]}}
The invertibility condition for \err\ is essential for the above formulation as it ensures definability of $\putl^\req$ via the policy \inv. In a more general setting, function \err\ can be not invertible at some points, \eg, cross entropy distance is such  (see \citefstx{Sect.VIIA}). If this more general \err\ is ``good enough'',  we can still define $\putl^\req$ by using a trickier  propagation policy $\pol(\err)$ but, importantly, it must be compositional and give rise to an sm-functor \frar{L_{\eps,\pol(\err)}}{\paracaterr}{\allenscat({\lmp})}, where $\allenscat(\lmp)$ denotes the category of \lmp-enriched al-lenses, \ie, lenses defined for 
%metric spaces and their morphisms as 
model spaces and get-functors being categories and functors enriched over \lmp\ rather than \setcat\ (and hence being metric spaces and non-expanding maps). Actually, the existence of a compositional policy \pol(\err) can serve as a formal definition of being ``good enough''.  

\input{ll-figures/diags/lawvereLensSquare}
The discussion above is summarized by the commutative diagram on the right, in which the following constructs are used. We first note that a codiscrete al-lens, \ie, a learner, can be seen as an al-lens defined for categories and functors enriched over a singleton category $\tcat=\{*\}$, which is also a monoidal poset in a trivial way. Then, the canonic morphisms \frar{\tfun}{\lmp}{\tcat} of monoidal posets gives rise to the change of base functor \frar{\tfun}{\catcat(\lmp)}{\catcat(\tcat) } between enriched categories and functors and, similarly, to a functor \frar{\tfun}{\allenscat(\lmp)}{\allenscat(\tcat)(=\learncat)
}. %\footnote
{That is, we assume that we have a general definition of an al-lens, whose ingredients are categories and functors and operations enriched over an sm-category \niv\  (this definition is still to be developed --- see remarks in Future work section~\ref{sec:future}), and thus we have a category of such lenses $\allenscat(\niv)$. If \niv\ is not mentioned, it is assumed to be \setcat\ (and \allenscat\ will be defined and shown to be sm in Sect.3-4). Note that $\catcat(\tcat)\cong\setcat$ and $\allenscat(\tcat)\cong\allenscat_0$ with 0 meaning codiscreteness. %Enrichment over \setcat\ is by default.
}


. %Hence, the general format of a Thus, for a general error function \frar{\errx}{\reals\times\reals}{\reals}, we should invent a 

\endinput
Given an  differentiable  {\em error} function  \frar{\err(x,y)}{\Reals\timm\Reals}{\Reals} be such that \frar{\prtfrac{\err}{x}(x_0,\_)}{\Reals}{\Reals} is invertible for any given $x_0$. For an $n$-dimensional Euclidean space $\reals^n$, we define the {\em total} error function \frar{\Err}{\reals^n}{\reals^n} by $\Err(a,a')=\sum_{i\le n}\err(a_i, a'_i)$. This converts space $\reals^n$ into a category (Lawvere's metric space) \brealsx{n}. 
	%
	A {\em \parrd\ function} from \realsx{m} to \realsx{n} is a differentiable function \frar{I}{\realsx{k}\timm\realsx{m}}{\realsx{n}} (and hence a functor \frar{I}{\brealsx{k}\timm\brealsx{m}}{\brealsx{n}}). 
	
	It is shown in \citefst\ that, given a {\em step size} $\eps\in(0,\infty)$,  any parameterized function \frar{I}{\realsx{k}\timm\realsx{m}}{\realsx{n}} gives rise to an ap-lens \frar{\ell_\eps(I)}{\brealsx{m}}{\brealsx{n}} called in \citefst\ a {\em learner}.%
	%\footnote{Warning: our models $S$ (for source) and $T'$ (target) are theirs $a$ and $b$ rather than $b'$.}
	\footnote{Moreover, they show the functoriality of the construction.} To make it an \alalens, we need to add amendments by defining $T^@=b'=I(p',a')$; then Putget trivially holds as there is only one arrow (distance/error) between any two objects. 
	
	%Any learner $\ell_\eps(I)$ can be made stable if we direct it to do nothing when $\Err(I(p,a),b)=0$. 
	Paper \citefjbx\ says that neither of the laws necessarily holds in the anarchic world of ML. % Putget nor Hippocraticness 


==> ll-sections/ml=bx.tex <==



\input{ll-sections/backgr-new}

\endinput
\input{ll-sections/ML-with-deltas}
\subsection{Enriching ML with deltas}\label{sec:deltas4ml}
%\zd{A phrase is to be added to the intro about the role of this section!!!!}

%We discuss (somewhat speculatively) three unconventional options for compositional ML suggested by the delta-based \bx. The discussion is purely theoretical as no attempt to evaluate %The present author does not have any knowledge of the ML literature and is not aware whether these possibilities are already realized, or how difficult an algorithmic realization of these options could be (or whether they are reasonable indeed). 
%
%Our goal is to demonstrate the possibilities of the \bx-ML interaction within the delta lens \fwk.  

\input{ll-sections/ml-metric}
\input{ll-sections/ml-delta}
\input{ll-sections/ml-amend}

\endinput

What could be deltas for pairs of values?

1)  Metrics like in Lawvere's metric spaces

2) Labels (men/women, students, professors, mathematician and poets)

3) Restruct the architecture!! Look at the discussion at \citefst


\endinput



==> ll-sections/mlbx-plane.tex <==

\subsection{From being orthogonal to united %From compositional ML to evolutionary BX
}\label{sec:mlbx-plane}


Let's fix a parameter $p\in P$ for a \parrd\ function \frar{f_p}{A}{B} as above, and consider a training datum $(a,b)$ with $b\noteq f_p(a)$. ML would call this inequality an error, %(and measure it by value $E(p,a,b)\eqdef e(f_p(a),b)\inn \Reals$), while 
Bx would call it an``inconsistency between artifacts $a$ and $b$''. 

\input{ll-figures/pdfs/mlbx-plane}
To fix an error, the ``no-back-propagation ML'' says ``change the function'', \ie, change the parameter from $p$ to $p'$ so that $f_{p'}(a)$ is closer to $b$ than $f_p(a)$. To recover consistency, the current/non-evolutionary Bx says ``change the input data'', \ie, find $a'$ such that $f_{p}(a')=b$ or, at least, closer to $b$ than $f_p(a)$ (note the inset figure with two opposite points 01 and 10). 
%\input{ll-figures/pdfs/mlbx-plane}


The modern ML (with back propagation) %Compositional ML (cML) considered in \citefst\ 
integrates the two approaches and fixes an error by modifying both, the function and the input data. The {\em evolutionary} Bx (still to be developed) goes along an orthogonal path but to the same point. Various scenarios involving changing the model \trafon\ definition (MDE usually says ``evolution'') are practically important and had been considered in the literature (mainly in the context of coevolution of a \trafon\ and its source or target (or both) metamodels) but not in the Bx-context. %   integrated approach that allows consistency restoration by modifying both the input data and the model \trafon\ definition. Although we are not aware of such a scenario in the context of MDE but it makes sense and will find its place in a plethora of works on coevolutions... \cite{?}    
Thus, \mlbp\ and \bxev\ should be different instances of basically the same formal model, but in their current realization there is an essential difference:  \mlbp\ is codiscrete/set-based while \bxo\ and (to be developed) \bxev\ should be  delta-based if we are serious about their MDE applications. Hence, the general goal of the present paper --- building a common delta-based model for ML and \bxev\ and looking for what interesting can we extract from it. The main ideas of the delta-based Bx, and whether it can be useful for ML, are discussed in \sectref{bx2ml} after a primer on delta lenses. 

==> ll-sections/modSpaces-short.tex <==
\subsection{Model Spaces and updates}% and Correspondences}
\label{sec:modelspaces}
Basically, a {\em model space} is a category, whose nodes are called {\em model states} or just {\em models}, and arrows are {\em (directed) deltas} or {\em updates}. For an arrow \frar{u}{A}{A'}, we treat $A$ as the state of the model before update $u$, $A'$ as the state after the update, and $u$ as an update specification.  Structurally, it is a specification of correspondences between $A$ and $A'$. Operationally, it is an edit sequence (edit log) that changed $A$ to $A'$. The formalism does not prescribe what updates are, but assumes that they form a category, \ie, there may be different updates from state $A$ to state $A'$; updates are composable; and idle updates \frar{\id_A}{A}{A} (doing nothing) are the units of the composition. 
\hkmodok{
It is also useful to have a more concrete notion of a model space as based on a category \spE\ of models and model embeddings, and then define an update \frar{u}{A}{A'} as a span of embeddings \flar{u_l}{A}{K}  and \frar{u_r}{K}{A'} where $K$ is a submodel of $A$ consisting of all elements preserved by $u$ so that embeddings $u_l$ and $u_r$ specify the deleted and the inserted elements resp. Then a model space \spA\ appears as the category $\Span(\spE)$ for some given \spE. Two ``extreme'' cases for the latter are a) the category of graphs and their inclusions, $\gracat_\subset$, which does not distinguish between objects/references and primitive values/attributes, and b) the Object-Slot-Value model developed in \cite[Sect.3]{me-gttse09} , which does make the distinction between objects and values but does not consider references/links between objects. Integrating a) and b) gives us the category of attributed graphs \cite{gtbook06}. Some of the notions that we axiomatically define below can be given formal definitions for a concrete choice of the category \spE, and we refer to paper \cite{orejas-bx13}, in which some of these definitions can be found for $\spE=\gracat_\subset$.
}{A prominent example of model spaces is the category of graphs where updates are encoded as (certain equivalence classes of) binary spans between them. They are heaviliy used in the theory of Graph Transformations \cite{gtbook06}. In this way an update $u:A\to A'$ can be a deletion or an addition or a combination of both.}{Thus updates as spans are at least mentioned informally. The formal treatment of the span cat with equivalences and so on is too much here! }
%\zd{In general, I agree, but let's keep this piece for some and finally decide later -- I mean that a systematic use of viewing \spA\ as \Span(\spE) is not assumed but maybe there will be a place where having it will be a useful thing.}
\par
We require every model space $\spA$ to be endowed with an additional construct of update compatibility. %described in the two consecutive subsections below.  
%of update {\em merging}
%
%\mysubsubsection{Sequential compatibility of updates} 
We assume a family $(\Kupd_A)_{A\inn\xob{\spaA}}$ of binary relations %$\comprfam{\Kupd_{A}\subset\spaA(\_,A)\timm\spaA(A,\_)}{A\in\xob{\spaA}}$,
{\renewcommand\xarr[1]{{#1}}
$\Kupd_{A}\subset\xarr{\spaA}(\_,A)\timm\xarr{\spaA}(A,\_) $
}
indexed by objects of \spaA, and 
specifying {\em non-conflicting} or {\em compatible} consecutive updates. Intuitively, an update %\frar{u}{\_}{A} 
$u$ into $A$ is compatible with update %\frar{u'}{A}{\_} 
$u'$ from $A$, if $u'$ does not revert/undo anything done by $u$, \eg, it does not delete/create objects created/deleted by $u$, or re-modify attributes modified by $u$. 
%For example, one could add Mary's employment at IBM ($\frar{u}{A_1}{A_1'}$) and subsequently add Ann ($\frar{u'}{A_1'}{A_1''}$) to $A'_1$ yielding a pair $(u,u')\in \Kupd_{A_1'}$ (see \cite{orejas-bx13} for a detailed discussion). Later we will specify several formal requirements to the compatibility (see \defref{def:wbspace} below). %Formally, we only require $(u,\id_A)\inn\Kupd_A$ and  $(\id_A,u')\inn\Kupd_A$ for all $A\in\xob{\spaA}$, $u\inn\xarr{\spaA}(\_,A)$ and $u'\inn\xarr{\spaA}(A,\_)$. 
%Now we can define model spaces.
\begin{defin}[Model Spaces] \label{def:mspace}
	A {\em model space} is a pair 
	$\spaA=(|\spaA|, \Kupd) %\Kdisj{}, \merge)
	$
	where |\spaA| is the {\em carrier} category of {\em models} and {\em updates}. We adopt a notational convention to omit the bars $|$ and denote a space and its carrier category by the same symbol \spA. The second component is a family 
	\[\Kupd=\comprfam{\Kupd_A\subset \spA(\_,A)\timm\spaA(A,\_)}{A\inn\xob{\spA}}\]	
of {\em sequential compatibility} relations  for sequential update pairs as described above. 
%The third and forth component are tightly coupled:
%	\[\Kdisj{}=\comprfam{\Kdisj{}_A\subset \spA(A, \_)\timm\spA(A,\_)}{A\inn\xob{\spA}}\]
%is a family of {\em concurrently compatible} or {\em mergeable} spans of updates, and 
%\[\merge =\comprfam{ \merge_A}
%	%\frar{\merge^k_A}{\Kdisj{k}_A}{\spA(A,\_)\times\Cospan^k}}
%	{A\inn\xob{\spA}}\]
%is a family of merge operations as shown in \eqref{eq:mergeDef}. The domain of operation $\merge_A$ is exactly the set $\Kdisj{}_A$. 
%We will denote the components of merge by $\merge_{A,i}$ with $i=1,2$ and omit index $A$ if they are clear from the context or not important. Writing $\merge_A(u,v)$ implicitly assumes $(u,v) \in \Kdisj{}_A$. 

A {\em functor} between model spaces \frar{f}{\spA}{\spB} is a functor between their carriers \frar{f}{|\spA|}{|\spB|} compatible with \Kupd: for any two arrow $u\Kupd v$ in \spA, we have $f(u) \Kupd f(v)$ in \spB. 
\qed
\end{defin}
%
\begin{defin}[Well-behaved Model Spaces]\label{def:wbspace}
	\noindent 
\newpii{A model space is {\em well-behaved (wb)} if the following conditions hold for all $A\in\xob{\spaA}$:
}{1: conditions $\Kupd_{1,2}$ below are added}{-2em}
\begin{center}
\begin{tabular}{l@{\quad}l}
	\lawnamebr{\Kupd\ and~ Id}{} &	
	For all $u\inn{\spA}(\_,A)$, $u'\inn{\spaA}(A,\_)$: $(u,\id_A), (\id_A,u')\inn\Kupd_A$, 
	\\ [1ex]
		%\lawnamebr{\Kupd\Kupd }{} 
		&	
For any three consecutive updates $u,v,w$, we require: 
	\\ [1ex] 
	%\begin{tabular}{l@{\quad}l}
		\lawnamebr{\Kupd\Kupd }{1}&
			$u\Kupd\,vw$ $\&$ $v\Kupd w$ imply $u\Kupd v$ $\&$ $uv\, \Kupd w$,
			\\
		\lawnamebr{\Kupd\Kupd }{2} &
		 $uv\,\Kupd w$ $\&$ $u\Kupd v$ imply $v\Kupd w$ $\&$ $u\Kupd\,vw$,
			 \\
		 & where composition is denoted by concatenation ($uv$ for $u;v$ etc). %and consider compositing binding stronger than \Kupd.
%%	\end{tabular}
%	\\ [1ex]
%		\lawnamebr{\Kdisj{}~and ~\Kupd}{} &
%	For all $(u_1,u_2)\in\Kdisj{}_A$: $(u_i,\merge_{A,i}(u_1,u_2))\in\Kupd_{A'_i}$, $i=1..2$
%	\\ [1ex]
%	\lawnamebr{Merge\ and~ Id}{}& For all $\frar{u}{A}{A'}$: $\merge_A(u,\id_A) = (\id_{A'},u)$    
\end{tabular} 
\end{center} \qed
%A {\em model space functor} from $\spaA$ to $\spaB$ is a functor $F:|\spaA|\to |\spaB|$, such that $(u,u')\hspace{-0.1em}\in \hspace{-0.1em}\Kupd_A$ implies $(F(u),F(u'))\hspace{-0.1em}\in\hspace{-0.1em}\Kupd_B$. We will denote model spaces and their carriers by the same symbol and often omit explicit mentioning of $\Kupd$.\qed  % (cf. Sect.\ref{sec:modelspaces}). 
\end{defin}
%Whereas the first condition is the already discussed natural property for sequential compatibility, the second requires complementing updates not to revert anything done by the other update. \footnote{
% that we do not claim the converse, namely the existence of a concurrently compatible partner in a sequentially compatible pair.} The third requirement is again self-evident. 
 We assume all our model spaces to be wb and, as a rule, will omit explicit mentioning. 
 %Each of the metamodels $M_1$..$M_3$ in the running example gives rise to a (wb) model space of its instances as discussed above.
%\input{figures/diags/mergeDef}


==> ll-sections/notation4diags.tex <==
% notation4diags piece
Diagram in \figari\ shows how these operations are interrelated. The upper part shows an arrow \frar{e}{p}{p'} in category \spP\ and two corresponding functors from \spS\ to \spT. The lower part is to be seen as a 3D-prism with visible front $ST_{p'}T^@S'$ and upper $ST_pT_{p'}$ faces, the bottom and side faces are invisible and the respective arrows are dashed. The prism denotes an algebraic term (workflow): given elements are shown with black fill and white font, while derived elements are blue (recalls being mechanically computed) and blank (double-body arrows are considered to be blank). The two pairs of arrows originating from $S$ and $S'$ are not blank because they denote pairs of nodes (UML says links) rather than mappings between nodes (like double-body arrows). For example, link labelled $1{:}\get_p$ denotes application of functor $\get_p$ to object $S$ that results in an object $T_p=\get_p(S)$.%
\footnote{Notation with colon is suggested by UML: $1$ ia the name of the link whereas $\get_p$ is its type. In a refined setting with the names \spS, \spT, $\get_p$ organized into a syntactic category, the Grothendieck construction can be seen here, but we don't need this in the present paper.}    
In the other three link-arrows we write $i{:}p$ rather than $i{:}\get_p$ to ease reading (below we will have more such arrows). Link-arrows have bulleted tails rather than usual $\mapsto$ due to limitations of Powerpoint, with which the diagram is built. In a similar style, \spT-arrows (deltas rather than links) such as \frar{\get(e,S)}{\get(p,S)}{\get(p',S)} are labelled as $ij{:}e_S$ where $i,j$ are indexes of the \corring\ links. Finally, link indexes convey the order of operations from which the entire workflow is built. We begin with 1) computing $T_p$, then 2) apply delta $v$ and compute three deltas $e=\putps_\upd(v)$, $u=\putps_\req(v)$, and $v^@=\putps_\self(v)$ (upper indexes are not shown as Powerpoint doesn't allow having upper and lower indexing together; subscripting $e$, $u$, $v^@$ with 2 would make notation heavy and we omitted it). Finally, 3) we add several derived elements (specified in the caption) needed later. Specifically, the diagram shows that two derived objects, $T^@$ (the target of $v^@$) and $\get(p', S')$ coincide and, moreover, the following equality called the PutGet law holds:
%$\get(e,S);\get(p',u)=v;v^@$ 
%\lawgap=1 ex
\noindent \begin{tabular}{l@{\hspace{4cm}}l}
%\\[0.5ex] 
\lawnamebr{PutGet}{
	} & %$_{~~~~~~}$
	$v.\putps_\req.\get_p =v;\amex{v} $ 
%	\\ [\lawgap]
\end{tabular}
For \bx, this is a fundamental requirement.....


==> ll-sections/overview.tex <==


\section{Overview of delta lenses with amendment and their compositionality}
%\section{Background: \bx\ world of model spaces and delta lenses}
\label{sec:backgr}


\subsection{Background: \bx\ world of model spaces and delta lenses}
In the (delta-based) \bx, the counterpart of values in Euclidean spaces dealt with in ML are complex artifacts called \bfem{models}. They can be seen as models of logical theories (of the first- or even higher-order) called \bfem{metamodels}. A typical way of specifying metamodels is to use graphs and constraints; in fact, metamodels can be seen as Makkai's generalized sketches \citemakkai, see also \cite{me-entcs08} for definitions and discussion in the MDE context. For our current discussion, it's enough to think about models as graphs with some (unspecified) extra structure, which behaves well enough to ensure the required categorical properties (the reader can think about {\em attributed typed graphs} as defined in \cite{ehrig-book06}); we will call them 'graphs'. In MDE applications, it normally does not make sense to distinguish isomorphic 'graphs' (indeed, objects identifiers are invisible) and thus we identify models with isomorphisms  classes of 'graphs' and assume categories of models to be strongly skeletal: the only isomorphisms are identity loops.  

Let \spG\ be a category of 'graphs'/models, $G, G'\in |\spG|$ are two objects, and \wrar{\tilde u}{G}{G'} is some informal notion of a model update (delta, change). We can formalize it by a span of monics $u=(G\lTo^i O\rTo^{i'} G')$ whose head $O$ specifies what part of $G$ is preserved in $G'$ so that the elements of $G$ beyond the image $i(O)$ are deleted, and the elements of $G'$ beyond $i'(O)$ are added during the update. % \frar{u}{G}{G'}.  
We assume that \spG\ has pullbacks so that spans are composable (and produce spans of monics), and we obtain a strongly skeletal category $\Span_{\mathsf{mon}}(\spG)$, %  (recall that \spG\ is skeletal and hence \Span(\spG) is a category rather than a bicategory), 
whose arrows are called \bfem{updates} or \bfem{deltas}. %Another way to specify informal updates $\tilde u$ is to use edit sequences describing what should be done with model $G$ to obtain model $G'$ step-by-step; such sequences are associatively composable and also produce a category (see, \eg, \citeeditlenses). 
The delta lens \fwk\ abstracts away these details and simply identifies model spaces with strongly skeletal categories and forward \trafon s between model spaces with functors; the latter are usually called \bfem{get functors}  or just \bfem{get}s (read `` get the view''): a detailed discussion and examples can be found in \cite{me-jot11}.%
\footnote{Not all useful \trafon s are functors, but many are, and it is a standard assumption in the delta lens \fwk.} 

Now we will schematically discuss how \alalens es work (and then will relate them to the ML setting in \citefst). %; precise definitions will be given in Sect.3. 
While an ordinary asymmetric  lens ``inverts'' a given functor \frar{\get}{\spA}{\spB} between model spaces, an \alalens\ ``inverts''  {\bf\em and} ``learns'' over a family of get functors \frar{\get_p}{\spA}{\spB} with $p$ being a parameter from a set $P$. We will actually consider a more general case with the parameter space also being a small category \spP, and the get family being a functor \frar{\get}{\spP}{[\spA, \spB]} into the category of functors from \spA\ to \spB\ and their natural transformations. %  (later we will consider a small category of parameters \spP\ whose set of objects is $P$). 
This implies that for \frar{e}{p}{p'} in \spP, and any two objects $A,A' \in \spA$, there is a mapping \frar{\get_e}{\spA(A,A')}{\spB(A.\get_p, A'.\get_{p'})} provided by the naturality of transformation $\get(e)$ (in the next section we will consider this in detail). 
We describe the data above in the top row of diagram \figri a, which provides the  ``types'' of the story, while the story itself is unravelled on the level of instances shown by the rectangular diagram below.   

Suppose given a model $A\in\spA$ and its view, model $A.\get_p= B \in\spB$, so that the state $(A,p,B)$ is consistent. 
Note our notation for the fact $A.\get_p=B$: bulleted arrows $x \rMapsto y$ don't have an internal structure and just visualize pairs $(x,y)$ --- the UML calls them {\em links}. The label over link $(A,B)$ in \figri(a) says that the link is an instance of function $\get_p$ (note the colon symbol), in more detail, this instance is fully determined by object $A$: it is the result of executing function  $\get_p$ at object $A$.%
\footnote{\label{fnote:storywithdefs} In a fuller version of the story with the type side explicitly given by a category \defcat\ of metamodels and \trafon\ definitions, over which a category of models is fibred,  link $(A,B)$ would be the Cartesian lifting of \trafon\ definition \flar{\niget_p}{\nim}{\nin} at object $A$ living in fibre \spA\ over metamodel \nim, and arriving at $B$ in the fibre \spB\ over \nin. Although the syntactical side is important for applications, lenses traditionally ignore it and we follow this style in the paper. 
}

\input{ll-figures/diags/bxmlPut-act19}
%\input{ll-figures/diags/bxmlPut-foss20}

Now suppose that $B$ is updated to $B'$ with delta (update) $\vii\in\spB(B,B')$ as shown. 
%We use numeric indexes for elements of the diagram to additionally convey the order of operations producing them, \eg, 1 means that production of link 1 by operation $\get_p$ is the first step of the story, and update $\vii$ is the second step. There is no intention to make this notation fully consistent (the more so formal); it is a syntactic sugar with some semantic connotations useful for reading complex diagrams further in the paper. %
%=== important remark for future thought
%\footnote{ 
%In the operational setting for updates (like in edit lenses), we would have a (partially defined) \trafon\ \frar{\vbf}{\spB}{\spB} so that update $\vii$ would be an instance of \vbf\ denoted by $2{:}\vbf$, but in the delta lens version used in this paper, vertical arrows are....}
In the asymmetric lens setting, any change of view $B$ destroys consistency (it's not so for the symmetric version of lenses), and an \alalens\ restores it by calling an operation \putl\ which a) changes the parameter with delta/update \frar{e}{p}{p'} (where $e$ refers to the {\em evolution} of the get), %from $p$ to $p'$, 
b) changes the source model $A$ with update \uiii,  and c) amends the update-violator $v$ with an {\em amendment} update $v^@$  so that the result of these changes is a consistent system $A'.\get_{p'}=B'^@$ as shown in the diagram (note the dashed arrows and index $p'$ near the bottom arrow). Thus, \putl\ is a triple of operations $(\putl^\upd, \putl^\req, \putl^\self)$, which for a given pair $(A,v)$ return a corresponding triple of updates \frar{e=\putl^\upd(A,v)}{p}{p'} (not shown in the diagram), \frar{u=\putl^\req(A,v)}{A}{A'}, \frar{v^@=\putl^\self(A,v)}{B'}{B'^@}; the superscripts \upd, \req\ abbreviate the corresponding names used in \citefst.   
%$u$, $v^@$.%and $\putl^\self$ that given $(A,v)$ 
%\footnote{Actually we will define even more categorical version in which the parameter space \spP\ is also a category and $\putl^\upd$ returns a parameter update \frar{e}{p}{p'}.}

Moreover, to ensure that operations \putl\ really invert functors \get, we require a much stronger consistency condition to hold:  %. Given  \frar{e}{p}{p'}, for any two objects $A,A' \in \spA$, there is a mapping \frar{\get_e}{\spA(A,A')}{\spB(A.\get_p, A'.\get_{p'})} provided by the naturality of transformation $\get(e)$ (in the next section we will consider this in detail). Now, 
for any $v$ as above, we require the equality $u.\get_{e}= v;v^@$ between updates---because it is update/delta $v;v^@$ that gives model $B'^@$ its real meaning in a typical MDE scenario.  
In the lens parlance, the last equation and its versions are called the Putget law: if we substitute $\putl(v)$ for $u$, we obtain equality $(\putl.v).\get_{p'} =v;v^@$ to hold for any $v$, hence, the name of the law. Another important law is {\em Stability}: if $v=\id_B$, then all three deltas, $e,u,v^@$ are also identities. A lens satisfying Stablity and Putget laws is called an {\em SP-alaLens}. 

Thus, an (SP) ala-lens is a pair $\ell=(\get,\putl)$ specified above, and we will write it as an arrow $\ell=(\get,\putl){:}\, \spA\stackrel{\spP}{\longrightarrow}\spB$ or just \frar{\ell=(\get,\putl)}{\spA}{\spB} keeping the parameter space \spP\ implicit. In the next section, we will show that SP-lenses can be composed sequentially and in parallel, and form an sm-category $\alalenscat$. 

An ala-lens \frar{\ell}{\spA}{\spB} is called {\em (elementarily) codiscrete} if all categories $\spA,\spP, \spB$ are codiscrete (below we will also consider non-elementarily codiscrete lenses). The full subcategory of (SP) codiscrete lenses will be denoted by $\alalenscat_0$ (and we have a full embedding $\alalenscat_0\rFEmb\alalenscat$).  

\subsection{Learners in the delta lens setting, I}

Diagram \figri(b) shows a specialization of the general ala-lens scenario in \figri(a) for ML-learners as defined in \citefst. Euclidean spaces are turned into categories whose arrows are differences: for any pair of tuples $a,a'\in\reals^m$, we have their componentwise difference $\del=(\del_i)_{i\le m}$, $\del_i=a'_i-a_i$, considered as an arrow \frar{\del}{a}{a'}.  Composition and identity are obvious, and any function \frar{f}{\reals^m}{\reals^n} gives rise to a functor \frar{\pmb f}{\rcat^m}{\rcat^n}.%
\footnote{A more refined model would be to consider monoids of differences as acting on values, say, monoid $\reals^m$ acts on $\reals^m$ so that given a value $a\in\reals^m$ and a difference (\textit{edit}, in the lens parlance) $\del\in\reals^m$, we compute $a'=a\odot\del$ where action $\odot$ is given by summation: $a\odot\del :=a+\del$. Thus, we have a monoid $\DDel^m=(\reals^m,+,0)$ that acts on $\reals^m$ by  \frar{\odot}{\DDel^m\timm\reals^m}{\reals^m}, and if function\frar{f}{\reals^m}{\reals^n} is differentiable, then its Jacobian matrix at point  $a$ can be seen as a monoid morphism \frar{\jacobf_a}{\DDel^m}{\DDel^n} so that for sufficiently small deltas, $f(a\odot\del)\approx f(a)\odot\jacobf_a(\del)$. Then functoriality of $f$ is based on its differentiability. We consider this model in more detail in \sectref{?}.
}
 The notation in diagram \figri(b) is borrowed from \citefst\ to ease seeing the parallelism (but note a discrepancy: $B'$ in \figri(a) corresponds to $b$  without prime in \figri(b)). Also note that for defining \putl, a special metrics is used: first, a differentiable error function \frar{\err}{\reals\timm\reals}{\reals} is defined, and then the total error is given by summation, $E_I(p,a,b):=\sum_{j\le n}\err(I_j(p,a), b_j)$ (see \citefst) so that $E_I(p,a,b)$ is a function of $\del_I(p,a,b)$ seen as an arrow. Finally, we can define update arrows using the gradient descent idea: \frar{\dellp}{p}{p'} with $\dellp=-\eps\nabla_p E_I(p,a,b)$ and \frar{\della}{a}{a'} with $\della=-\eps\nabla_a E_I(p,a,b)$ (of course, we can use different step sizes \eps\ for \dellp\ and \della).%
 \footnote{In \citefst, they define \della\ differently. First, function \frar{\prt_x\err(x_0,\_)}{\reals}{\reals} is considered invertible for all $x_0$, and let \flar{\rre_{x_0}}{\reals}{\reals} be its inverse (symbol \rre\ is the inversely read \err). Then for an $a\in\reals^m$, we have \flar{\rre_a}{\reals^m}{\reals^m}. Now  $\della$ can be defined as $\rre_a(\nabla_a E_I(p,a,b))$.} 
 Amendment is defined by differencing $\del^@=I(p',a')-b$. It easy to see that if $\del=0=\id_{I(p,a)}$, then $E_I(p,a,b)=0$ achieves its minimum and thus  $\dellp=\della=\del^@=0$ as well so that Stability holds. The Putget law trivially holds due to the definition of $\del^@$. Thus, learning based on the gradient descent gives us an SP-alaLens. 
 
 
%\clearpage
 \subsection{Functoriality of update policies}
% \input{ll-figures/diags/funofput}  old name of the sect
 \input{ll-figures/diags/policyfun-1}
 
 The diagram in \figrii\ illustrates compositionality of operations \get\ (trivial) and \putl\ (non-trivial) (nodes $\circ$ denote objects without names). Given a sequence of parameterized functors \frar{\get^i_{p_i}}{\spA_i}{\spA_{i+1}}, $p_i\in\spP_i$, $i\le n$ ($n=3$ in the diagram), it is easy to define their composition \frar{\get_p}{\spA_1}{\spA_n} for $p=(p_1...p_n)\in\spP{=}\spP_1\timm\ldots\timm\spP_n$ as $$A.\get_p=(...(A.\get^1_{p_1}).\;\ldots\;).\get^n_{p_n},$$ and show that it is associative (when functors are considered up to a suitable equivalence). Composition of $\putl^i$, $i\le n$ is more interesting: the diagram shows a simple projection of story, in which  arrows \frar{e_i{=}\putl^{i\,\upd}}{p_i}{p'_i} are not shown. Triple-arrow symbols $j{:}\putl^i$ denote three consecutive applications ($j=1,2,3$) of operations $\putl^i$ appropriately indexed. Double-arrows labelled $j{:}\get^i_{e_i}$ denote application of the corresponding \get-functors to arrows to demonstrate that the Putget law holds. 
 
 
 A pair $\ell_i=(\get^i,\putl^i)$ is an ala-lens \frar{\ell_i}{\spA_i}{\spA_{i+1}}, and the construction shown in the figure defines lens composition \frar{\ell_1;\ell_2;\ell_3}{A_1}{A_4} (it will be formally defined in \sectref{alalenscat}). %, we will prove that ala-lenses make an sm-category. 
 However, it's not the end of the story developed in \citefst. 
 %
 So far, in the lens formalism as such, two components of a lens $\ell=(\get, \putl)$ are considered given independently although their interaction is regulated by lens laws ensuring a weaker or stronger sense of \putl\ being an inverse to \get. However, in practice of both BX and ML, the \putl-component is built based on the \get-component. As there are many ways of inverting a {\bf general} functor, finding reasonable single-valued operation \putl\ (a so called {\em update policy})  is normally based on the {\bf specific} form of \get\ so that \putl\ is carefully ``tuned'' for a given specific \get. In other words, for a given specific domain context \nix, model spaces $\spA_i$ are special categories and functors \get s are special functors for which a reasonable single-valued operations \putl\ can be defined. For example, ML provides a special context, in which model spaces are Euclidean spaces (considered as categories $\rcat^m$), \get s are differentiable mappings \frar{f}{\rcat^k\timm\rcat^m}{\rcat^n}, and the gradient descent idea Gd provides a reasonable definition of \putl s. We will return for this discussion in \sectref{policyfun-2}
 
 \endinput
 
 \renewcommand\fu{}
 \renewcommand\wi{}
 
 % \input{ll-figures/diags/policyfun}
 %  \input{ll-figures/diags/policyfun-smallTri}
  %\input{ll-figures/diags/policyfun-bigTri-OLD(defVersion)} % future work
      \input{ll-figures/diags/policyfun-bigTri}
 %   \input{ll-figures/diags/policyfun-new}
 
 We can model the notion of a context \nix\ as an %sm-subcategory $\pgetcat_\nix$ of the sm-category of parametrized functors \pcatcat\ (see Appendix \sectref{pcatcat}) or, better, as an 
 sm-category $\pgetcat_\nix$ equipped with a faithful forgetful functor \frar{{-}\nix}{\pgetcat_\nix}{\pcatcat} (read symbol `${-}\nix$' as ``forget the \nix-structure'') into the category \pcatcat\ of all small categories and (equivalence classes of) parameterized functors between them (see Appendix \sectref{pcatcat}).  Now the process of building \putl\ based on \get\ can be formalized as a graph morphism \frar{\plusxput}{\pgetcat_\nix}{\alalenscat} from (the graph underlying) category $\pgetcat_\nix$ of parameterized \nix-functors to (the graph underlying) category of ala-lenses such that the internal triangle (*) in \figref{policyfun} commutes  %$({+}_\nix\putl);({-}\putl)={-}\nix$ 
 (read symbol `$\plusx{\nix}\putl$' as ``add \nix-determined operation \putl'' and `${-}\putl$' as ``forget operation \putl'' in a lens $\ell=(\get, \putl)$). 
 
 A central question of defining an update policy is whether it is functorial, that is, whether the graph morphism \plusxput\ is a functor. For example, a central result of \citefst\ is functoriality of \frar{\plusputx{Gd(\eps,\err)}}{\diffcat}{\learncat} where Gd refers to defining \putl\ via gradient descent with step size $\eps$ and  error function \err\ (see above), \diffcat\ denotes the category of (equivalence classes of) parameterized differentiable functions between Euclidean spaces, and \learncat\ is the category of codiscrete ala-lenses. The discussion above motivates the following formal definition.
 %\begin{defin}\label{def:policyfun}
 \par
 \smallskip\noindent
 {\bf Definition (Change propagation systems).}
 	An {\em asymmetric (parameterized, compositional) change propagation system (CPS)} is a triple $\nix=(\pgetcat_\nix, {-}\nix, \plusxput)$ with \pgetcat\ being an sm-category  equipped with two sm-functors, ${-}\nix$ and \plusxput\ as shown in \figref{policyfun}, such that ${-}\nix$ is faithful, and the triangle (*) commutes. % functor commutative diagram of functors 
 	
 	A CPS is called {\em codiscrete} if functor ${-}\nix$ factors through \psetcat\ and functor \plusxput\ factors through $\alalenscat_0$ as shown in \figref{policyfun}, where arrows with triangle tails denote full embeddings. Thus, a codiscrete CPS is a triple $\nix=(\pgetcat_\nix,{-}_0\nix, \plusxput_0)$ such that the external triangle (dashed arrows) in \figref{policyfun} commutes.
 %\end{defin}

One may think that ML-motivated CPS considered in \citefst\ is codiscrete  but .......

\zd{TWO sections are commented below:
	\\
ll-sections/ml-diff
\\
ll-sections/policyfun-ml2-piece
\\
but they are used elsewhere
}

\endinput

\input{ll-sections/ml-diff}
\input{ll-sections/policyfun-ml2-piece}

==> ll-sections/policy-as-functor.tex <==
\section{Propagation policy as  a functor
}

\input{ll-figures/diags/bigPicture}

==> ll-sections/policyfun-2.tex <==
\section{Functoriality of change propagation policies
	%Codiscrete lenses as Delta Lenses with Differencing 
}\label{sec:policyfun-2}

In this section, we discuss.....


\input{ll-sections/ddlenses}
\input{ll-sections/cpsystems}
\input{ll-sections/learners2lenses}



\zd{A HUGE outdated PIECE IS END-INPUTED}

\zd{But it seems that it is in the APPENDIX E now}

\endinput


\endinput
\input{ll-sections/derivatives-as-functors}
\section{Learners as delta lenses %: Functoriality of differentiation
}\label{sec:derifun}
%\newcommand\leefun{\enma{L_{\eps,\err}}}


In this section, we sketch  how the functor \frar{\leefun}{\paracat}{\learncat} specified in \citefst\ could be derived along the dd-lens lines described above as the composition $\leefun=({+}
\mathsf{deltas});!;\codifun$, where $!$ is the unique functor determined by pair $({+}\dif(pol), {+}\putl(pol))$ due to the universal property of products and the fact that the image of $!$ satisfies the condition of being a well-behaved dd-lens. 

\newcommand\figrcomp{\figref{difasfun}}
\subsubsection{Derivative as a functor.} Our first observation is that differentiability can be seen as functoriality. 
Let \frar{f}{\reals}{\reals} be a differentiable function, whose derivative is denoted by $\prt f$, $a,a'$ are two reals and $\del=a'-a$ is their difference treated as an arrow \frar{\del}{a}{a'}. %---subindex $a$ is used to suggest that we consider $a'-a$ as an action (we will also say {\em edit}) applied to value $a$ so that $(\reals, +, 0)$ becomes a monoid acting on \reals. 
%%(The difference $a'-a$ plays yet another role of a distance between $a$ and $a'$, below we will discuss it in more detail.) 
If \del\ is small enough, then $f(a')-f(a)\approx \del\cdot\prt f(a)$ and we can say that $\prt f(a)$ maps arrow \del\ to arrow \frar{\del.\prt f(a)}{a.f}{a'.f}. If function $f$ maps from the left to the right, we will often use the dot notation for function application so that \frar{\del.\prt f_a}{a.f}{a'.f}, where $\prt f_a$ denotes $\prtf(a)$. %the value of the differential $\prt f(a)$ at point $a$.

%-- the gradient version ---
%Let \frar{f}{\reals^m}{\reals} be a differentiable function, whose gradient is denoted by $\nabla f$, $a,a'$ are two $m$-tuples of real numbers, and $\del=(\del_1...\del_m)$ %a'-a=(a'_1-a-1,....,a'_m-a_m) is their componentwise difference, $\del_i=a'_i-a_i$, $i\le m$, treated as an arrow \frar{\del}{a}{a'}. If all $\del_i$ are small enough, then $f(a')-f(a)\approx \nabla f(a)\cdot\del$ (where $\cdot$ denotes the scalar product) and we can say that $\nabla f(a)$ maps arrow \del\ to arrow \frar{\nabla f(a)(\del)}{f(a)}{f(a')}. The generalization for the case \frar{f}{\reals^m}{\reals^n} is straightforward by considering $f$ a tuple $f_j, j\le n$ and Jacobian matrix $\jacobf=(\prt_if_j: i\le m, j\le n)$ replacing the gradient. To encompass all cases, we will call a linear operator mapping deltas from $a$ to deltas from $f(a)$ a {\em differential} and write  $\prtf(a)$ or often $\prtf_a$. If function $f$ maps from the left to the right, we will often use the dot notation for function application so that \frar{\del.\prt f_a}{a.f}{a'.f}, where $\prt f_a$ denotes the value of the differential $\prt f(a)$ at point $a$.

If deltas are not infinitely small, then $a'.f=a.f+\del.\prtf_a+o(\del)$ as shown by square (1) in diagram \figrcomp a, where \medadx{f} denotes $a.f+\del.\prtf_a$, and term $o(\del)$ converges to $0$ if \del\ converges to $0$. (If \frar{f}{\reals}{\reals} is an analytic function, then $o(\del)$ is the part of its Taylor series representation starting with the second order derivative, $o(\del)=\prt^2f_a\cdot\del^2/2!+\prt^3f_a\cdot\del^2/3!+\ldots$). If we consider \reals\ as a category \rcat\ whose arrows are triples $(a,\del,a')$ such that $a'=a+\del$, and composition $\del;\del'$ is given by addition, then differentiation becomes a functor-like mapping as shown by diagram  \figrcomp a. Diagram \figrcomp b, in which commutative ``rectangles'' (12) and (12') define $\prt(f;g)$, specifies the chain rule. 
\begin{remark}\label{rem:del-as-act}
	Commutativity of rectangle (11) in \figrcomp a is trivial as \rcat\ is a thin category. We can make it more interesting if....
\end{remark}
Generalization for the case \frar{f}{\reals^m}{\reals^n} is straightforward with $a,a'$ being $m$-tuples of real numbers, $\del=(\del_1...\del_m)$ %a'-a=(a'_1-a-1,....,a'_m-a_m) is 
their componentwise difference, Jacobian matrix $\jacobf=(\prt_i f_j: i\le m, j\le n)$ being the differential and $\jacobf\cdot\del$ is matrix-vector multiplication. If $n=1$, then \jacobf\ is gradient $\nabla f$. %, whose value at vector $a$ will be denoted by $\nabla_a$. 
To encompass all cases, we will call a linear operator mapping $m$-dimensional deltas from $a$ to $n$-dimensional deltas from $f(a)$ a {\em differential} and write  $\prtf(a)$ or often $\prtf_a$. 
%
An $m$-dimensional space $\reals^m$ is converted into category $\rcat^m$ componentwise. 

%======
%\input{figures/diags/difasfun1}
\input{figures/diags/difasfun3}
%====
%\input{figures/pdfs/getAmend-inR}
%====

\newcommand\couplarr[1]{\enma{#1^{\gg}}}
Now we define an abstract version of the above. %Given a category \spXX\ and an object $X\in|\spXX|$, we write $\spXX(X,\_)$ and $\spXX(\_,X)$ for classes \compr{\frar{u}{X}{X'}}{X'\in|\spXX|} and \compr{\frar{u}{X'}{X}}{X'\in|\spXX|} resp. 
Given a category \spXX\ and objects $X,X'\in|\spXX|$, we write $\couplarr{\spXX}(X,X')$ for the set of pairs of arrows 
%
\compr{(u,u')\in\spXX(X,Y)\timm\spXX(Y,X')}{Y\in|\spXX|} 
%
\noindent determined by the obvious pullback. 
\begin{defin}[Quasi-functors]\label{def:qfun}
Given categories \spA, \spB, a {\em quasi-functor} 
%$\spA\rightarrow\spB$ 
\frar{f^\gg}{\spA}{\spB} is given by i) an object function \frar{|f|}{|\spA|}{|\spB|} and ii) for any $A,A'\in|\spA|$, a mapping \frar{f^\gg_{AA'}}{\spA(A,A')}{\spB^\gg(B,B')} where $B=|f|(A)$, $B'=|f|(A')$. Given \frar{u}{A}{A'}, we consider the first component of pair $f^\gg_{AA'}(u)$ as the main value and denote it by $f_{AA'}(u)$ while the second component is called an {\em amendment} and denoted by $f_{AA'}^@(u)$. We say quasi-functor $f$ is {\em functorial at $u$} if $f_{AA'}^@(u)=\id_{B'}$, and {\em functorial at $A,A'$} if it is functorial at all \frar{u}{A}{A'}.  As a rule, we will omit indexes and write $f(u)$ for the main value and $f^@(u)$ for its amendments. %By an abuse of notation, 
The composition of pair $f^\gg_{AA'}(u)$, \ie, arrow $f(u);f^@(u)$, will be  denoted by $f^\gg(u)$. All this abuses notation but the context should make it clear.


Moreover, the following two functoriality conditions are required to hold for quasi-functors: unitality, \ie, for any $A$, $f(\id_A)=f^@(\id_A)=\id_{|f|(A)}$, and composition preservation  (cf. diagram \figrcomp a), which requires for any \frar{u}{A}{A'}, \frar{u'}{A'}{A''}, the following equation:
\begin{equation}\label{eq:qfun}
       f^\gg(u;u')=f^\gg(u);f^\gg(u') 
\end{equation}
%And for any $A$, $f(\id_A)=f^@(\id_A)=\id_{|f|(A)}$.
If $f$ maps from the left to the right, we will use the dot notation $u.f$, $u.f^@$. 
\end{defin}

The intuition that in the pair $u.f^\gg_{AA'}$, the component $u.f$ is the main value while $u.f^@$ is its amendment is formalized by the following definition of quasi-functor composition. Given two quasi-functors \frar{f}{\spA}{\spB} and \frar{g}{\spB}{\spC}, their {\em composition} $f;g$ or just $fg$ is defined by the following triple of mappings:  $|fg|:=|f|;|g|$ and, for any \frar{u}{A}{A'}, $u. fg := u.f .g$ and $u.(fg)^@:=(u.f.g^@);(u.f^@.g^\gg)$ (cf. diagram \figrcomp b). %Note that it is the definition of composition, which formalizes the intuition of the second component of a quasi-functor as an amendment.

Obviously, if $f$ and $g$ are unital, then $fg$ is such, and it is straightforward to check by multiple substitution, that if $f$ and $g$ preserve composition according to \eqref{qfun}, then $fg$ preserves composition too. Hence, $fg$ is a quasi-functor as soon as $f$ and $g$ are such. The identity functor on \spA\ is also the identity quasi-functor on \spA, and we thus have a category \qcatcat. Moreover, componentwise paring equips this category with an sm-structure: given parallel quasi-functors \frar{f_i}{\spA_i}{\spB_i}, $i=1,2$, we define $u_1\paar u_2.\,f_1\paar f_2=u_1. f_1\paar u_2.f_2$ and $u_1\paar u_2.\,(f_1\paar f_2)^@=u_1. f_1^@\paar u_2.f_2^@$. Checking sm-category axioms is straightforward. 
%\begin{lemma} The collection of all small categories and quasi-functors between them is a category \qcatcat. %Condition \eqref{qfun} holds for the above triple, and hence the latter determines a quasi-functor \frar{f;g}{\spA}{\spC}
%\end{lemma}

\subsubsection{Differentiating parameterized functions}
%====
\input{ll-figures/pdfs/getAmend-twoFig}
%====

Consider \frar{f}{\spP\timm\reals^m}{\reals^n}, where $\spP=\reals^k$ is a parameter space. Differentiating over parameters for a fixed $a\in\reals^m$, gives us an operator $\prt_p f(p,a)$ mapping parameter deltas \frar{e}{p}{p'} from $p$ into $\reals^n$-deltas from $a.f_p:=f(p,a)$ (as usual, we use symbol $p$ in two roles: as a variable running over \spP\ in $\prt_p f$ and as a fixed parameter value in other expressions). Similarly, differentiating over variables in $\reals^m$  for a fixed parameter $p\in\reals^k$, gives us an operator $\prt_a f(p,a)$ mapping deltas \frar{\del}{a}{a'} from $a$ into $\reals^n$-deltas from $a.f_p$. Diagram in \figgetam a describes the ingredients of the story as arrows. Intermediate vertical arrow from $a.e\prt_p$ has the same label as its counterpart on the left as we consider the delta $\hat \del :=\del.\prt_af(p,a)$ as acting on values in $\reals^n$, and we label the result of applying $\hat \del$ to $b\in \reals^n$ by $\hat \del$ so that different arrows from different $b$s get the same label. Similarly, two different horizontal arrows from $a.f_p$ and $a.\del\prt_a$ have the same action label too. 

An abstract delta lens formulation of the story is given by the following definition illustrated by diagram \figgetam b. 
\begin{defin}[incremental view system]\label{def:viewsys}
	Let \spS\ and \spT\ be model spaces. An {\em (incremental parametrized) view system} 	from \spS\ (the {\em source} of the view) to \spT\ (the {\em target}) is given by i) a category \spP\ of {\em parameters} (think about function/view definitions \parrd\ by objects of \spP) and ii) a quasi-functor \frar{\get}{\spP\timm\spA}{\spB}. A view system is called {\em codiscrete} if categories \spS, \spT, \spP\ are codiscrete.
\end{defin}

In the parametrized setting,  we have a differentiable function \frar{f}{P\times\reals^m}{\reals^n} with $P=\reals^k$ being the parameter space. %, and a differentiable error function \frar{\Err}{\reals^m}{\reals}, whose composition gives us differentiable  function \frar{E}{P\times\reals^m}{\reals}. 
We can convert this data into a double-indexed family of functors-as-monoid- homomorphisms  \frar{\get_{p,a}}{\DDel^m}{\DDel^n}, $p\in P, a\in \reals^m$ %, by, first, converting all Euclidean spaces into categories as described above, and then, 
by the two upper equations in \eqref{mlgetdef}: %as follows: for a given parameter $p$, parameter delta \frar{\Delp=(p'-p)}{p}{p'}, m-tuple of reals $a$ and input variables delta \frar{\Dela=(a'-a)}{a}{a'}, we define%
\footnote{as usual, by the abuse of notation we will denote variable and its fixed value by the same symbol $a$} 
%\begin{minipage}[t]{0.5\textwidth}
\begin{equation}\label{eq:mlgetdef}
\begin{array}{c}
\get_p(a)=f(p,a)
\\
\get_{p,a}(\dela)=\Dela*\nabla_af(p,a)
\\
\get_a(\Delp)=\Delp*\nabla_pf(p,a)
\end{array}
\end{equation}
%\end{minipage}
(where the last equation specifies natural transformation  $\get(\Delp)$). Thus, we have a parameterized functor or the \get-part of a dd-lens: the differencing operation is uniquely defined so that Difdif holds, and it is straightforward to check conditions \eqref{difget}.  In terms of diagram \figrcodi, we have built functors ${+}\mathsf{deltas(\pol)}$ and ${+}\dif(\pol)$.


\subsubsection{Gradient descent as an update propagation policy
	%Model spaces as metric spaces.
}
Metrics, \ie, setting a distance between values considered as an {\em error} is an important part of the story. %We will need also some metrics on differences considered as errors. 
Following \citefst, we assume that some  differentiable function \frar{\err}{\reals\times\reals}{\reals} is given, and %actions of monoid $\DDel=(\reals,+,0)$ are considered as opliftings: 
then given $a\in\reals$ and edit $\delta \in\DDel$, the result of applying $\delta$ to $a$ is an arrow \frar{\ovr{\delta}=\err(a,a')}{a}{a'}. For the multiple variables case $\reals^m$, a delta is a vector $\del=(\del_1,...,\del_m)$ acting componentwise, and the result of applying it to value $a=(a_1...a_m)$ is an arrow/distrance  \frar{\ovr{\del}=\Err(a,a')}{a}{a'} computed by summation: $\Err(a,a') :=\sum_{i\le m}\err(a_i,a'_i)=\sum_{i\le m}\err(a_i,a_i+\del_i)$.  
%considered as an arrow \frar{\ovr{\delb}}{b}{b'}
with $b=f(a)$ and $b'=f(a')$. Thus, an accurate setting would be to consider an asymmetric edit delta lens (see \cite{jr-unified} for a definition for the codiscrete case) whose model spaces are Lawvere categories (metric spaces). However, delta lenses subsume edit lenses (see \cite[sect.??]{me-jot11} for the idea and examples, and \cite{jr-unified} for formal results), and below we will work in the delta lens setting, in which deltas are pairs $(\del,\ovr{\del})$ where $\del=a'-a$ and $\ovr{\del}=\err(\del)$.  %As it was shown in \cite{jr-unified}, 

In the setting of \citefst,

For defining the \putl-part, we need a policy, and the gradient descent method gives us one. We can treat formulas in \citefst\ for computing the updated parameter $p'$ (for a given step size \eps) and updated input value $a'$ as $\putl^\upd$ and $\putl^\req$ operations mapping delta $\Del_b=b-E(p,a)$ to deltas $p'-p$ and $a'-a$ resp. (and conditions \eqref{difputupdself} (upper) and \eqref{difputreq} are automatically satisfied). We can also set $\putl^\self(\Del_b)=E(p',a') - b$ so that condition \eqref{difputupdself}(bottom) is also satisfied. Moreover, the Putget laws holds too. Thus, we have a (well-behaved) dd-lens. In terms of diagram in \figrcodi, we built functor ${+}\putl(\pol)$ and showed that the universal arrow $!=[{+}\dif(\pol), {+}\putl(\pol)]$ targets at the category of well-behaved dd-lenses as shown in the diagram.
%
%Probably, the entire construction would be more transparent and manageable (\eg, with respect to generalizations) if we consider this dd-lens as sequentially composed from two dd-lenses: \frar{\ell_\eps(f)}{\reals^m}{\reals^n} and \frar{\ell(\err)}{\reals^n}{\reals} (whose parameter space is \tcat). This elaboration is also left for future work. 

Finally, by applying the codiscretization functor, we arrive at the category of codiscrete ala-lenses, which gives us derived functor ${+}\putl0(\pol)$.   

%An Euclidean space $\reals^n$ can be seen as a category $\rcat^n$ enriched in $\niv=(\reals^n, +)$: given two tuples $a, a' \in \reals^n$, we define $\rcat^n(a,a')= (a'- a)$. A differentiable function \frar{f}{\reals^m}{\reals^n} can then be seen as a functor \frar{\get}{\rcat^m}{\rcat^n} whose object part is $f$, and the arrow part is the derivative: $\get(a'-a)=$

==> ll-sections/policyfun-ml2-piece.tex <==
  \subsection{UNKNOWN 1}
  
  
  %%==
 \input{ll-figures/diags/policyfun-ml}
 %%===
 
 
In this diagram, \pcatcat\ is the category of all small categories as objects and (equivalence classes of) parameterized functors between them as arrows.%
 \footnote{The latter are functors \frar{f}{\spP\timm\spA}{\spB} or, equivalently, functors \frar{f}{\spP}{[\spA, \spB]} from some small category \spP\ into the category of functors $\spA\rightarrow\spB$ and their natural transformations; see \sectref{pcatcat} for details.}
 

 
  The category of (small) sets and (equivalence classes of) parameterized functions, \psetcat, is fully embedded into \pcatcat\ by considering any set as a codiscrete category.  We name this embedding as \plusarrx{\pairing} to be read as ``add arrows by pairing'', \ie, by considering a pair $(a,a')\in A\timm A$ as an arrow $a\rightarrow a'$, which makes set $A$ a (codiscrete) category \spA.  Similarly, on the right side, we have a full embedding of the category of codiscrete ala-lenses into the category of delta ala-lenses. Finally, as any ala-lens is basically a pair $\get, \putl$ with \get\ a parameterized functor and \putl\ is its inversion in some special sense, we have a forgetful functor ${-}\putl$ (read ``forget \putl'') as shown in the diagram.  

  Now we consider the upper row of the diagram. We can convert any Euclidean space $\reals^n$ into a category $\rcat^n$ whose arrows, \frar{\del}{a}{a'}, are deltas defined componentwise: $a=(a_i)_{i\le n}$, $a'=(a'_i)_{i\le n}$, and $\del=(\del_i)_{i\le n}$ with $\del_i=a'_i-a_i$. Functors \frar{\pmb f}{\rcat^n}{\rcat^n} and functions \frar{f}{\reals^m}{\reals^n} are in bijective correspondence. This gives us the commutative square (1) in which $\paracatrcat$ is the category of parameterized differentiable maps considered as functors, the upper arrow is an isomorphism, and vertical arrows are functors that forget the rich structure of \reals\ and consider it as either a set (the left edge) or a category (the right edge).  The central part of the story is given by the central square (2). The gradient descent idea (Gd) allows us to add to any parameterized functor \fbf\  in \paracatrcat\ with its inverse (in a certain sense)  mapping \putl\ so that the pair $(\fbf,\putl)$ makes an ala-lens with an additional operation of differencing, which for any two objects $x,y$ in a general category \spXX\ selects an arrow/delta \frar{\dif(x,y)}{x}{y} %called adelta between $x$ and $y$ 
  (an accurate definition will be given in \sectref{codilens}). Forgetting first \dif\ and then \putl\ gives us a commutative square (2). Finally, a typical way of building codiscrete lenses in applications is to begin with a delta lens with differencing, which gives rise to a codiscrete lens in a functorial way--this gives us a general functor \codiscr\ (the right most edge in the diagram denotes equality: two different names for the same category). Note that square (actually, triangle) (3) is not %necessarily commutative and is not 
  commutative for a general delta lens with diff, whose underlying lens is not codiscrete. However, the lenses in the image of functor $\plusx{Gd(\eps,\err)}\putl$ relate thin categories, so that the rectangle (2)+(3) is commutative. 


==> ll-sections/prelimiaries.tex <==
%\section{Preliminaries}

%\input{ll-sections/back-act2foss}

\input{ll-sections/functOfLearning-act2foss}

%\input{ll-sections/aboutDefLens}
\input{ll-sections/aboutLaws}

%\input{ll-sections/notation}

%\input{ll-figures/diags/bigPicture}




==> ll-sections/remarks-on-laws-OLD.tex <==
In other words, we call an ala-lens wb if it is stable and satisfies Putget, \ie, is an SPg lens. 
%	{\emno A lens is {\em stable} if it satisfies Stability, and an {\em SPg-lens} if it satisfies Stability and Putget. 
%	\shortlong{Following the lens terminological traditions, in this paper  we will also call an SPg lens {\em well-behaved (wb)}. Note however that wb-lenses defined in \cite{me-fase18}  are stronger than SPg.}{}
%	\shortlong{}{A lens is called {\em Hippocratic} if the (Hippocr) law holds.%
%	\footnote{The term Hippocratic and its derivatives were coined for Bx by Perdita Stevens \cite{stevens-sosym10} to refer to a family of requirements sharing a common intention of doing nothing if consistency is not violated, which 
%	can be seen as an application of a major medical principle ``First, do no harm'' usually attributed to the Hippocratic oath --- see Wikipedia {\tt https://en.wikipedia.org/wiki/Hippocratic\_Oath} for details.} 
%An SPg Hippocratic lens is called {\em well-behaved (wb)}
%}  % end of long
%%	
%%	A target delta $v$, is {\em closed} if $v^@=\id_{B'}$; an \alalens\ is {\em closed} if each target delta is closed. %or {\em SPg-lens} if it also satisfies Putget and Closure resp. 
%}
%
Remarks \ref{rema:laws1}, \ref{rema:laws2},\ref{rema:putget4codi} are applicable for ala-lenses as well. 
}  %end LONG
% long remark about the laws, which is now partly in remarks 1 and 2.
%\begin{remark}\label{rema:alalenslaws}{\emno 
%%a) Condition Closure only requires full amendment deltas $v;v^@$ to be closed, which is  much weaker than the defining condition of closed lens requiring  {\em each} delta to be closed. %as to be fulfilled in closed lenses. 
%a) Stability says that the lens does nothing if nothing happens on the target side (no trigger--no action, hence, the name of the law) 
%
%b) Putget requires the goal of update propagation to be achieved after the propagation act is finished. 
%%\begin{remark}\label{rema:putget}%\zd{to be reworked}
%%	The Putget law 
%In the codiscrete setting, it is a notational trick rather than a law. We begin with delta $v=(A_p, B')$, which operation  $\putps^\req$  propagates  to delta $u=(A,A')$ and function $\get_{e}$ sends it to delta  $(A_p,A'_{p'})$. Also, $\putps^\self$ gives us an amendment delta $v^@=(B',A'_{p'})$ and $v;v^@=(A_p, A'_{p'})=\get_e(A,A')$ so that Putget always holds. %targeting at some model $A'_{p'}$ anyway. 
%But in the general delta setting, there are many possible deltas between models $B'$ and $A'_{p'}$, whereas the Putget law states the existence of some special delta \frar{v^@}{B'}{A'_{p'}} such that equation (\putget) holds. %Note also that Putget implies commutativity of the lower triangle in the right back face as the upper one is commutative by Putget. %much more certainty about $B''$ and precisely specifies the relationship between $B'$ and $B''$, namely, it says that they are related by a specified update $\amex{v}$.
%
%\shortlong{
%c) Besides Stability and Putget, the MDE context for ala-lenses suggests other laws; some of them are considered in \cite{me-fase18}% \eg, Hippocraticness described in the longer version \cite{me-act19-long}.
%}{
%c) Hippocraticness prohibits amending delta $v$ if consistency can be achieved for $v$ without amendment (hence, the name).  Note that neither equality $\putUL{\upd}{p,A}(v)=p$ nor $\putUL{\req}{p,A}(v)=u$ are required: the lens can improve consistency by changing $p$ and $u$ but changing $v$ is disallowed.  
%}} % end \em; end long
%\end{remark}

%==== the law pieces ends


%  law is a notational trick rather than a law. We begin with delta $v=(A.\get, B')$, which operation  $\putl^\spba_A$  propagates  to delta $u=(A,A')$,  and function $\get$ sends it to delta  $(B,B'')$ where $A'.\get=B''$. Also, $\putl^\spbb_A$ gives us an amendment delta $v^@=(B', B'^@)$ and $v;v^@=(S_p, S'_{p'})=\get_e(S,S')$ so that Putget always holds. %targeting at some model $S'_{p'}$ anyway. But in the general delta setting, there are many possible deltas between models $T'$ and $S'_{p'}$, whereas the Putget law states the existence of some special delta \frar{v^@}{T'}{S'_{p'}} such that equation (\putget) holds. %Note also that Putget implies commutativity of the lower triangle in the right back face as the upper one is commutative by Putget. %much more certainty about $T''$ and precisely specifies the relationship between $T'$ and $T''$, namely, it says that they are related by a specified update $\amex{v}$

\begin{remark}[On lens laws]\label{rema:laws2}
	\shortlong{}{b)}	
	Besides Stability and Putget, the MDE context for ala-lenses suggests other laws discussed in \cite{me-faoc19}, which were (somewhat recklessly) included into the \wbcodex. To avoid confusion, Johnson and Rosebrugh aptly proposed to call lenses satisfying Stability and Putget {\em SPg lenses} so that the name unambiguously conveys the meaning. In the present paper, wb will mean exactly SPg.   % \eg, Hippocraticness described in the longer version \cite{me-act19-long}.
	\shortlong{}{
		c) Hippocraticness prohibits amending delta $v$ if consistency can be achieved for $v$ without amendment (hence, the name).  Note that neither equality $\putUL{\upd}{p,S}(v)=p$ nor $\putUL{\req}{p,S}(v)=u$ are required: the lens can improve consistency by changing $p$ and $u$ but changing $v$ is disallowed.  
	} % end \em; end long
\end{remark}
\begin{remark}[Putget for codiscrete lenses]
	\label{rema:putget4codi}%\zd{to be reworked}
	%	The Putget law 
	In the codiscrete setting, the codiscrete Putget law, \putgetcodi, actually determines amendment in a unique way. The other way round, a codiscrete lens without the requirement to satisfy Putget, is a wb codiscrete lens with amendment (which satisfies the amended Putget). %    law is a notational trick rather than a law. We begin with delta $v=(A.\get, B')$, which operation  $\putl^\spba_A$  propagates  to delta $u=(A,A')$,  and function $\get$ sends it to delta  $(B,B'')$ where $A'.\get=B''$. Also, $\putl^\spbb_A$ gives us an amendment delta $v^@=(B', B'^@)$ and $v;v^@=(S_p, S'_{p'})=\get_e(S,S')$ so that Putget always holds. %targeting at some model $S'_{p'}$ anyway. But in the general delta setting, there are many possible deltas between models $T'$ and $S'_{p'}$, whereas the Putget law states the existence of some special delta \frar{v^@}{T'}{S'_{p'}} such that equation (\putget) holds. %Note also that Putget implies commutativity of the lower triangle in the right back face as the upper one is commutative by Putget. %much more certainty about $T''$ and precisely specifies the relationship between $T'$ and $T''$, namely, it says that they are related by a specified update $\amex{v}$.
\end{remark}

==> ll-sections/remarks-on-laws.tex <==
Remarks \ref{rema:putget4codi} (p.~\pageref{rema:putget4codi}) on lens laws  are applicable to ala-lenses as well.
\endinput
\begin{remark}[On lens laws]\label{rema:laws1}{\emno 
%		Condition Closure only requires full amendment deltas $v;v^@$ to be closed, which is  much weaker than the defining condition of closed lens requiring  {\em each} delta to be closed. %as to be fulfilled in closed lenses. 
Stability says that the lens does nothing if nothing happens on the target side (no trigger--no action, hence, the name of the law) 
		
Putget requires the goal of update propagation to be achieved after the propagation act is finished (see examples in \sectref{ex-updprop}). Note the distinction between the \putgetcodi\ condition included into the very definition of a lens, and the full Putget law required for the wb specialization of lenses. It is needed to ensure smooth tiling of \putl-squares (\ie, arrow squares describing application of \putl\ to a view update and its result) both horizontally and vertically (not considered in this paper). Also, if we want to accurately define operations \putl\ independently of the functor \get, we still need a function \frar{\get_0=|\get|}{|\spA|}{|\spB|} and the codiscrete Putget law to ensure smooth tiling (cf.\cite{bryce-act19}).
		%
Note also that 	in the codiscrete setting, the \putgetcodi\ condition actually determines amendment in a unique way. The other way round, a codiscrete lens without the requirement to satisfy Putget, is nevertheless a wb codiscrete lens with amendment (which trivially satisfies the amended Putget). 
}
\end{remark}
%\zd{see other remarks in the long version}
\endinput

\begin{remark}[On lens laws]\label{rema:laws2}
	\shortlong{}{b)}	
	Besides Stability and Putget, the MDE context for ala-lenses suggests other laws discussed in \cite{me-faoc19}, which were (somewhat recklessly) included into the \wbcodex. To avoid confusion, Johnson and Rosebrugh aptly proposed to call lenses satisfying Stability and Putget {\em SPg lenses} so that the name unambiguously conveys the meaning. In the present paper, wb will mean exactly SPg.   % \eg, Hippocraticness described in the longer version \cite{me-act19-long}.
	\shortlong{}{
		c) Hippocraticness prohibits amending delta $v$ if consistency can be achieved for $v$ without amendment (hence, the name).  Note that neither equality $\putUL{\upd}{p,S}(v)=p$ nor $\putUL{\req}{p,S}(v)=u$ are required: the lens can improve consistency by changing $p$ and $u$ but changing $v$ is disallowed.  
	} % end \em; end long
\end{remark}
\begin{remark}[Putget for codiscrete lenses]
	\label{rema:putget4codi}%\zd{to be reworked}
	%	The Putget law 
	In the codiscrete setting, the codiscrete Putget law, \putgetcodi, actually determines amendment in a unique way. The other way round, a codiscrete lens without the requirement to satisfy Putget, is a wb codiscrete lens with amendment (which satisfies the amended Putget). %    law is a notational trick rather than a law. We begin with delta $v=(A.\get, B')$, which operation  $\putl^\spba_A$  propagates  to delta $u=(A,A')$,  and function $\get$ sends it to delta  $(B,B'')$ where $A'.\get=B''$. Also, $\putl^\spbb_A$ gives us an amendment delta $v^@=(B', B'^@)$ and $v;v^@=(S_p, S'_{p'})=\get_e(S,S')$ so that Putget always holds. %targeting at some model $S'_{p'}$ anyway. But in the general delta setting, there are many possible deltas between models $T'$ and $S'_{p'}$, whereas the Putget law states the existence of some special delta \frar{v^@}{T'}{S'_{p'}} such that equation (\putget) holds. %Note also that Putget implies commutativity of the lower triangle in the right back face as the upper one is commutative by Putget. %much more certainty about $T''$ and precisely specifies the relationship between $T'$ and $T''$, namely, it says that they are related by a specified update $\amex{v}$.
\end{remark}

==> ll-sections/safety_buffer.tex <==
\section{Sequential and parallel composition of apa-lenses, and \smm\ category \apalenscat.}
\newcommand\figkl{\figref{kl-lens}}
\renewcommand\figrii{\figkl} %ref{kl-lens}}
\newcommand\defrii{\defref{def:aalens-hComp}}
\renewcommand\kl{\ensuremath{\ekk;\ell}}
%\renewcommand\figari{\figref{}}

\input{ll-figures/pdfs/aalens-hComp}
\begin{constr}[Sequential composition of apa-lenses]\label{con:apa-seq}{\em  
	Let \frar{\ekk}{\spA}{\spB} and \frar{\ell}{\spB}{\spC} be two apa-lenses with parameterized functors \frar{\get^\ekk}{\spP}{[\spA,\spB]} and \frar{\get^\ell}{\spQ}{[\spB,\spC]} resp. %spaces \spP\ and \spQ\ resp.  
	Their {\em composition}  is the following apa-lens \kl.
	
	Its parameter space is the product $\spP\times\spQ$, and the \get-family is defined as follows. For any pair of parameters $(p,q)$ (we will write \pq), %$\get^{(p,q)}$ or 
	\frar{\get^{\kl}_{pq}=\get^\ekk_p;\get^\ell_q}{\spA}{\spC}.
	%functor $\#(p,q)$ is the composed functor %\frar{\get^p;\get^q}{\spA}{\spC}, 
	%\frar{\#p;\#q}{\spA}{\spC}, and given 
	Given a pair of parameter deltas, \frar{e}{p}{p'} in \spP\ and \frar{h}{q}{q'} in \spQ, their $\get^{\kl}$-image is the Godement product of natural transformations, $\get^{\kl}(eh)=\get^\ekk(e)*\get^\ell(h)$. 
	
	
	Now we define \kl's propagation operations \putl s. Let $(A, pq, C_{pq})$ with $A\in\xob{\spA}$, $\pq\in |\spP\timm\spQ|$, $q\in|\spQ|$ be a \zdmodok{state}{state}{} of lens \kl, and  \frar{w}{C_\pq}{C'} is a target update as shown in \figrii. %\ with bold black lines.  %All stages of the definition are accurately described in \figrii. 
	For the first propagation step, we run lens $\ell$ as shown in \figrii\ with the blue colour for derived elements: this is just an instantiation of the pattern of \figari\ with the source object being $B_p=\get_p(A)$ and parameter $q$. The results are deltas %, being a given state of  lens $\ell$,  $w$ a given target update, and 
	\begin{equation}\label{eq:kldef1}
	\frar{h=\putxy{q}{B}^{\ell.\upd}(w)}{q}{q'}, \quad
	\frar{v=\putxy{q}{B}^{\ell.\req}(w)}{B_p}{B'}, \quad
%\mbox{ and }
	\frar{\amex{w}=\putxy{q}{B}^{\ell\self}(w)}{C'}{C^@}.
	\end{equation}
% three propagated updates. 
	%
	Next we run lens $\ekk$ at state $(p,A)$ and the target update $v$ produced by lens $\ell$; it is yet another instantiation of pattern in \figari\ (this time with the green colour for derived elements), which produces three deltas
	\begin{equation}\label{eq:kldef2}
	\frar{e=\putxy{p}{A}^{\ekk.\upd}(v)}{p}{p'},\quad
	\frar{u=\putxy{p}{A}^{\ekk.\req}(v)}{A}{A'}, \quad
% \mbox{ and }
	\frar{\amex{v}=\putxy{p}{A}^{\ekk\self}(v)}{B'}{B^@}.
\end{equation}
%or, after substituting the term for $v$, 
%	\begin{equation}\label{eq:kldef2}
%	\frar{e=\putxy{p}{A}^{\ekk.\upd}(\putxy{q}{B}^{\ell.\req}(w))}{p}{p'},\quad
%	\frar{u=\putxy{p}{A}^{\ekk.\req}(\putxy{q}{B}^{\ell.\req}(w))}{A}{A'}, \quad
%	% \mbox{ and }
%	\frar{\amex{v}=\putxy{p}{A}^{\ekk\self}(\putxy{q}{B}^{\ell.\req}(w))}{B'}{B^@}.
%\end{equation}
These data specify the green prism adjoint to the blue prism: the edge $v$ of the latter is half of the right back face diagonal $B_pB^@$ of the former. In order to make an instance of the pattern in \figari\ for lens \kl, we need to complete the blue-green diagram by filling-in the empty spaces below the diagonal and above the diagonal with appropriate arrows. These filling-in arrows are provided by functors $\get^\ell$ and $\get^\ekk$ and shown in orange  (where we have chosen one of the two equivalent ways of forming a Godement product -- note two curve brown arrows).
%By composing appropriate green and blue arrows with orange ones, 
In this way we obtain yet another instantiation of the pattern in \figari\ denoted by \kl:
\begin{equation}\label{eq:kldef3}
\putxy{A}{\pq}^{\klbr\upd}(w) = (e,h), \quad
\putxy{A}{\pq}^{\klbr\req}(w) = u, \quad
%\mbox{ and }
\putxy{A}{\pq}^{\klbr\self}(w) = w^{\klbr.@}    %\get_{q'}(v^@),
\end{equation}
where $w^{\klbr.@}=w^@;v^@_{q}$, and 
$v^@_{q'}$ denotes $v^@.\get_{q'}$. 
Thus, we built an apa-lens \kl, which satisfies equation \putgeto\ %\eqref{putget0} (Putget)$_0$ 
by construction.  %\ie, an apa-lens, which we denote by \kl.
}\end{constr}
%\input{ll-figures/pdfs/aalens-hComp}
%The following result is obvious.
The following result is important for practical applications: it ensures that a composed synchronizer satisfies its requirements automatically as soon as its components do, which allows significant reducing of the integration testing (only connectivity is to be checked).
%We will also need the following two derived constructs.
{\newcommand\xell{\enma{}}
\begin{defin}[Get and Put images of a lens]
	Given a lens from space \spS\ to space \spT, define %the following two sets of deltas: 
	$$
	\begin{array}{l}
	\Get^\xell(\spS)=\comprCol{u.\get_p\, }{u\in\Arr\spS, p\in|\spP|}\subset \Arr\spT
	\\ 
	\Putl^\xell(\spT)=\comprCol{\putl^\xell_{p,S}.v\,}{p\in|\spP|, S\in|\spS|, \frar{v}{\get_p(S)}{\_}\in\Arr\spT}\subset\Arr\spS
	\end{array}
	$$
\end{defin}} % end group
\begin{theorem} [Seq. composition and lens laws] Given are apa-lenses \frar{\ekk}{\spA}{\spB}, \frar{\ell}{\spB}{\spC}, and lens \frar{\kl}{\spA}{\spC} is their seq. composition as defined above. Then the following holds. 

(a)	Lens \kl\ is SPg  as soon as lenses $\ekk$ and $\ell$ are such.  

(b) If lenses \ekk\ and \elll\ are wb, and additionally are {\em well-matched} in the sense that $\Get^\ekk(\spA)\superset\Put^\ell(\spC)$, 
% functors $\get^\ell_q$, $q\in\spQ$ {\em preserve} closed deltas, \ie, map \ekk-closed deltas in \spB\ to $\ell$-closed deltas in \spC, 
then the lens \kl\ is wb as well.  %satisfies Closure law (and hence is wb) as soon as lenses $\ekk$ and $\ell$ are such.  
\end{theorem}
{\renewcommand\id{the identity}
{\em Proof.} a) Stability of \kl\ is obvious. To prove Putget for \kl, we first note that 
as $e_A$ is \id\ due to Putget for \ekk, then its image is also \id\ (functoriality of  $\get_{q'}$) and hence $(e*h)_A$ is \id\ as $h_B$ is \id\ due to Putget for \elll. It remains to prove $u.\get^{\kl}_{p'q'}=w;w^{\klbr.@}$ %(w^@;v^@_{q'})$, %where $v^@_{q'}$ denotes $v^@.\get_{q'}$. 
We compute:
%
\newcommand\getUL[2]{\enma{\get^{#1}_{#2}}}
	\newcommand\getekk[1]{\getUL{\ekk}{#1}}
		\newcommand\getell[1]{\getUL{\ell}{#1}}
		\newcommand\byx[1]{\mbox{\quad #1}}
\begin{eqnarray}
	u.\getUL{\kl}{p'q'}
	&=& 
	u.\getekk{p'}.\getell{q'}  \byx{by constr.}
	\\ &=&
	(v;v^@).\getell{q'} \byx{Putget for \ekk}
	\\ &=&
	(v.\getell{q'})\,;\,(v^2.\getell{q'}) \byx{functoriality}
	\\ &=&
	(w;w^@)\, ;\, v^@_{q'} \byx{Putget for \elll\ | def. of $v^@_{q'}$}
	\\ &=&
	w;(w^@;v^@_{q'}) \byx{associativity of ;}
	\\ &=& 
	w;w^{\klbr.@}
\end{eqnarray}
%
%note that $\ekk$'s and $\ell$'s Putgets provide commutativity of the triangles $B_pB_{p'}B^@$ and $C_{\pq}C_{q'}C^@$ resp., and functor $\get^\ell_{q'}$ maps the green triangle into a commutative triangle $C_{q'}C_{p'q'}C^{@@}$ (note the orange label [=]), which together with commutative blue provides Putget for \kl. 
%\begin{remark}
%	Note that in general, lens \kl\ does not satisfy Closure condition even if lenses \ekk\ and \elll\  do. Finding additional conditions on lens ``junction'', which would ensure Closure of lens \kl\ is a work in progress (cf. \cite{me-fase18}) 
%\end{remark}
Proof of (b). For any given $A, p, q$ in the respective spaces, and delta \frar{w}{A.\get^{\kl}_{pq}}{C'} such that $u.\get^{\kl}_{pq}=w$ for some \frar{u}{A}{\_}, we need to prove $w^{\klbr.@}=\id_{C'}$. We have seen that $$
w^{\klbr.@}=w^{\ell.@}{\bf \,;\;}\getell{q'}(v^{\ekk.@}) 
\mbox{\quad where $v=\putl^{\ell.\req}_{B_p,q}$}.
$$ We will prove that both components of ; are identities. The first one is identity due to $w=\getell{q}(u.\getekk{p})$ and \elll\ is Hippocratic. For the second component, $v^{\ekk.@}$ is identity as i) $v=\putl^{\ell.\req}_{B_p,q}$ and lenses are well-matched and ii) lens \ekk\ is Hippocratic. Now the second component is identity as functor $\getell{q'}$ preserves identities. 
} % ned of the group for \id 

%
%
%We need to prove that delta $w;w^{\klbr.@}$ is closed. 
%\begin{eqnarray}
%	w;w^{\klbr.@}
%	&=&u.\getUL{\kl}{p'q'} \byx{Putget for \kl\ proved above}
%	\\&=& (u.\getekk{p'}).\getell{q'} \byx{by constr. of \kl}
%	\\&=& (v;v^@).\getell{q'} \byx{by Putget for \ekk}
%%	\\&=& ....
%\end{eqnarray}
%Now, delta $v;v^@$ is closed due to Closure condition for lens \ekk, and \getell{q'} maps it to a delta closed in \elll\ by the preservation condition. Thus, $w;w^{\klbr.@}$ is closed in \elll.
%
%Due to Putget for \kl\ proved above, 


\begin{constr}[Parallel composition of apa-lenses]\label{con:apa-par}{\em 
Let \frar{\ell_i}{\spA_i}{\spB_i}, $i=1,2$ be two apa-lenses with parameter spaces $\spP_i$. The lens 
\frar{\ll}{\spA_1\timm\spA_2}{\spB_1\timm\spB_2} is defined as follows. (We will denote a pair of element $(x,y)$ by $x\paar y$.)
%
Parameter space $\ll.\spP=\spP_1\times\spP_2$. For any $p_1\paar p_2\in \spP_1\timm\spP_2$,  define $\getxy{\ll}{\pp}=\getxy{\ell_1}{p_1}\times\getxy{\ell_2}{p_2}$.
Further, for any $
\ss \in \spA_1 \times \spA_2
$ and delta 
\frar{v_1\paar v_2}%
       {\getxy{\ll}{\pp}(\ss)}
       {T'_1\paar T'_2},
       we define componentwise
       $$
       \frar{e=\putxyz{\llbr\upd}{\pp}{\ss}(v_1\paar v_2)}{\pp}{p'_1\paar p'_2} 
       \mbox{ by setting $e=e_1\paar e_2$ where %
       	$e_i=\putxyz{{\ell_i}}{p_i}{S_i}(v_i)$, $i=1,2$   }
$$
and similarly for $\putxyz{\llbr\req}{\pp}{\ss}$ and \putxyz{\llbr\self}{\pp}{\ss}
}\end{constr}
The following result is obvious but important (as any compositionality result-- see the remark about integration testing above).
\begin{theorem}[Parallel composition and lens laws]
Lens $\ell_1\paar\ell_2$ is wb as soon as lenses $\ell_1$ and $\ell_2$ are such.
\end{theorem}


%\subsection{\smm\ category \apalenscat\ of apa-lenses }

Now we are going top show that apa-lenses can be organized into an sm-category. 
To obtain an associative sequential  composition of apa-lenses, we need to consider them up to some equivalence (indeed, Cartesian product is not strictly associative).
\begin{defin}[Apa-lens Equivalence]
	Two parallel apa-lenses \frar{\ell, \hell}{\spS}{\spT} are called {\em equivalent} if their parameter spaces are isomorphic via a functor \frar{\isop}{\spP}{\hat\spP} such that for any $S\in\xob{\spS}$,  $p\in\spP$ and \frar{v}{(S.\get_p)}{T'} the following holds:
	$$
	S.\get_p=S.\hget_\hp,\quad
	\isop(\putps^\upd(v))=\hputl_{S,\hp}(v), \quad
		\mbox{ and }
	\putps^{\x}(v)=\hputl^\x_{S,\isop(p)}(v) 
	\mbox{ for $\x\inn\{\req,\self \}$} \quad 
	$$
\end{defin}
\begin{remark}In general, we should require isomorphisms rather than equalities above, but isos become equalities for skeletal categories.  
\end{remark}
\begin{lemma}\label{prop:eq-i-comp}
	Operations of lens' sequential and parallel composition are compatible with lens' equivalence. Hence, these operations are well-defined for equivalence classes.
\end{lemma}
Below we will identify lenses with their equivalence classes by default. 
%%	
%%	 together with an isomorphic natural transformation \dlar{i}{\#}{f;\hat\#} such that %$f;\hat\#=\#$ 
%	for all propagation operations $\putl^\x$, $x\in\{\upd,\req,\self\}$, and any \zdmod{state}{???}{} $(p,S)$, equality $$\putxy{p}{S}^x(v) = \puthatxy{\hat p}{S}_x(i_S;v)$$ holds for any target update \frar{v}{T}{T'} where $T=p^*(S)$, $\hat p=f(p)$, and  $\hat T=\hat p^*(S)$ (so that \flar{i_S}{T}{\hat T}). 
%	\zd{$\putl^\x$, $x\in\{\upd,\req,\self\}$ is to be introduced earlier!!}
%\begin{remark}\zd{Just for the record}A more categorically plausible definition would require just isomorphisms rather than equalities, but then we need 2-arrows between updates.
%\end{remark}
\begin{theorem}[Apa-lenses form an sm-category]
	Operations of sequential and parallel composition of apa-lenses defined above allow building an sm-category \apalenscat, whose objects are model spaces (= skeletal categories) and arrows are (equivalence classes) of apa-lenses.  
%	a) Model spaces as objects and equivalence classes of aa-lenses as arrows form a category denoted by \aalenscat. 
%	b) 	If \defri\ (\figri) is enriched with Cartesian monoidal product ($S_1\otimes S_2=(S_1, S_2)$ for objects and similarly for arrows), then  \aalenscat\ becomes a symmetric monoidal category. 
\end{theorem}
{\em Proof.} It is easy to check that identity lenses $\idl_\spA$ defined in \exref{idlens} are the units of the seq. lens composition defined above. The proof of associativity is rather involved and is placed into Appendix. Thus, \apalenscat\ is a category. 

\newcommand\isolensfun{\enma{\catname{isolens}}}
Next we define the monoidal structure. The monoidal product of objects is Cartesian product of categories (skeletality is preserved), and the monoidal product of arrows is lens' parallel composition defined above. The monoidal unit is the terminal category \tcat. Associators, left and right unitors, and braiding are iso-lenses generated by the respective isomorphism functors (\exref{isolens}). Moreover, it is easy to see that the iso-lens construction is actually a functor \frar{\catname{isolens}}{\catcat}{\apalenscat}. Then  as a) \catcat\ is \smm\ and fulfils all necessary monoidal equations, and b) \isolensfun\ is a functor, these equations hold for the apa-lens images of \catcat-arrows, and \apalenscat\ is \smm\ too (cf. a similar path in \citefst\ with $(\setcat,\times)$ instead of $(\catcat,\times)$.  
%\begin{corollary}Category \apalenscat\ has a full sm-subcategory of SPg apa-lenses and a full sm-subcategory 
%\end{corollary}

==> ll-sections/vert-compose.tex <==
\section{Compositionality of update propagation: K-Putput}

==> macros/4citations.tex <==
\newcommand\citebaezncat{\cite{?}}
\newcommand\citefjbx{\cite{fj-bx19}}
\newcommand\citefj{\cite{fj-bx19}}
\newcommand\citefst{\cite{fst-backprop}}
\newcommand\citefstx[1]{\cite[#1]{fst-backprop}}
\renewcommand\citell{\citefst}
\newcommand\citepiercetr{\cite{?}[TR2003]}
\newcommand\citemakkai{\cite{makkai-ske}}
\newcommand\citefetal{\cite{fst-backprop,fj-bx19}}
\newcommand\citeeditlenses{\cite{bpierce-editlens,jr-unified}}
\newcommand\citejrunified{\cite{jr-unified}}
\newcommand\citejrunifiedX[1]{\cite[#1]{jr-unified}}
\newcommand\citemtex{\cite{mtbe-kappel12}} %[MT from examples]}
\newcommand\citemtbe{\cite{mtbe-kappel12}} %[MT from examples]}
\newcommand\citeao{\cite{alv-ong}}
\newcommand\citeaotr{\cite{alv-ong-tr}}
\newcommand\citeaotrx[1]{\cite[#1]{alv-ong-tr}}
%\newcommand\citeeditlenses{\cite{?}}

==> macros/4fase17paper.tex <==
\newcommand\sameown{\textsf{sameOwn}}

\newcommand\mt{\textsc{mmt}}
\newcommand\mmt{\mt}
\newcommand\metatr{\ensuremath{T}} % {Tr_{\mathrm{def}}}}
\newcommand\modtr[1]{\ensuremath{Tr_{#1}}}
\newcommand{\emath}[1]{{\ensuremath{#1}}}
%\newcommand{\tobjnobr}[2]{\emath{\mathbf{T}^\bullet_{#1}(#2)}}

\newcommand\anmt{\ensuremath{{\mathbf T}}}

\newcommand\coveh{\ensuremath{\mathsf{Commut.Vehicle}}}
\newcommand\lveh{\ensuremath{\mathsf{LeisureVehicle}}}
\newcommand\veh{\ensuremath{\mathsf{Vehicle}}}
\newcommand\car{\textsf{Car}}
\newcommand\bcar{\textsf{bCar}}
\newcommand\wcar{\textsf{wCar}}
\newcommand\days{\textsc{Days}}
\newcommand\boat{\textsf{Boat}}
\newcommand\amph{\textsf{amph}}
\newcommand\cveh{\textsf{Commut}}
\newcommand\usedon{\textsf{usedOn}}
\newcommand\same{\textsf{same}}
\newcommand\inzz{\textsf{in}}


%------
%\newcommand\mydefin[2]{\par\noindent \textbf{Definition #1 (#2).}}
%\renewcommand\mydefin[2]{\par\noindent \textbf{Definition #1.}}
%\newenvironment{\mydefin}[2]% name
%{\par\noindent \textbf{Definition #1 (#2).}}% opening macros
%{{\qed}} %closing macros


\endinput



==> macros/4general-llncs.tex <==
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand*{\textcal}[1]{%
	% family qzc: Font TeX Gyre Chorus (package tgchorus)
	% family pzc: Font Zapf Chancery (package chancery)
	\textit{\fontfamily{qzc}\selectfont#1}%
}

\DeclareMathAlphabet{\mathantt}{OT1}{antt}{li}{it}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\newcommand\ensureamth[1]{\ensuremath{#1}}

% == rotation command
%\rotatebox[origin=c]{45}{$xxx$} 
\newcommand\qqquad{\qquad\quad}
\newcommand\qqqquad{\qquad\qquad}
%\newcommand{\tmapleft[2]}{\ensuremath{#1}}
%\newcommand\mysectpar{\par\medskip}
%\newcommand\mysection[1]{\mysectpar\noindent{\rm \bfseries{\large #1.}}}
%%\renewcommand\mysection[1]{\section{#1}}
%\newcommand\myitempar{\par}
%\newcommand\myitem[1]{\myitempar{\bf #1.}}
%
%\newcommand\mysubsection[1]{\vspace{-1.ex}\subsection{#1}\vspace{-0.65ex}}
%\newcommand\mysubsubsection[2]{\vspace{#2}\subsubsection{#1}} 
%%  another version
%%\renewcommand\mysubsubsection[1]{\par\smallskip\noindent {\bfseries\itshape{#1}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% == my font discipline for defs for Springer ==

%-- doesn't worl for Compisitinality
\newenvironment{defin}[1][]{\ifthenelse{\equal{#1}{}}{\definition}{\definition[#1]}\rm}{\enddefinition}
\newenvironment{propo}[1][]{\ifthenelse{\equal{#1}{}}{\proposition}{\proposition[#1]}\rm}{\endproposition}
\newenvironment{remar}[1][]{\ifthenelse{\equal{#1}{}}{\remark}{\remark[#1]}\rm}{\endremark}
% \newtheorem{defin}{Definition}
% \newtheorem{corol}{Corollary}
% \newtheorem{theorem}{Theorem}
% \newtheorem{propo}{Proposition}
% \newtheorem{rema}{\textit{Remark}}
% \newtheorem{example}{Example}

%% ATTENTION PLS !
%  for Elsevieer, the above macros don't work, but versions below do work
% \let\oldexample=\example
% \let\endoldexample=\endexample
% \renewenvironment{example}{\vspace{-0.6em}\begin{oldexample}}{\end{oldexample}\vspace{-0.35em}}

% \let\olddefin=\defin
% \let\endolddefin=\enddefin
% \renewenvironment{defin}{\vspace{-0.6em}\begin{olddefin}}{\end{olddefin}\vspace{-0.5em}}

% \let\oldpropo=\propo
% \let\endoldpropo=\endpropo
% \renewenvironment{propo}{\vspace{-0.6em}\begin{oldpropo}}{\end{oldpropo}\vspace{-0.5em}}

% \let\oldrema=\rema
% \let\endoldrema=\endrema
% \newenvironment{rema}{\vspace{-0.6em}\begin{oldrema}}{\end{oldrema}\vspace{-0.5em}}

% \let\oldcorol=\corol
% \let\endoldcorol=\endcorol
% \newenvironment{corol}{\vspace{-0.6em}\begin{oldcorol}}{\end{oldcorol}\vspace{-0.5em}}

% \let\oldtheorem=\theorem
% \let\endoldtheorem=\endtheorem
% \renewenvironment{theorem}{\vspace{-0.6em}\begin{oldtheorem}}{\end{oldtheorem}\vspace{-


% math operations

\newcommand\opname[1]{\ensuremath{\mathsf{#1}}}
\newcommand\colim{\opname{colim}}
\newcommand\limcat{\opname{lim}}

%===== Calligraph. Literals ======
\newcommand\niceletter[1]{\ensuremath{{\cal #1}}}
\newcommand\nicex[1]{\niceletter{#1}}
\newcommand\nia{\nicex{A}}
\newcommand\nib{\nicex{B}}
\newcommand\nid{\nicex{D}}
\newcommand\nie {\nicex{E}}
\newcommand\nik {\nicex{K}}
\newcommand\nil {\nicex{L}}
\newcommand\nim{\nicex{M}}

\newcommand\nio{\nicex{O}}
\newcommand\nip{\nicex{P}}
\newcommand\nir{\nicex{R}}
\newcommand\nit{\nicex{T}}
\newcommand\niu{\nicex{U}}
\newcommand\niw{\nicex{W}}
\newcommand\nix{\nicex{X}}


% Domain-codomain/source-target/ident
\newcommand\cod[1]{\ensuremath{{#1}^\bullet}}
\newcommand\dom[1]{\ensuremath{^\bullet{#1}}}
\newcommand\so{\ensuremath{\mathsf{src}}}
\newcommand\ta{\ensuremath{\mathsf{trg}}}
\renewcommand\so{\ensuremath{\mathsf{s}}} % was src
\renewcommand\ta{\ensuremath{\mathsf{t}}}  % was trg
\newcommand\ldom[1]{\ensuremath{$\Box #1 $}}
\newcommand\rdom[1]{\ensuremath{$#1 \Box $}}
\newcommand\id[1]{\opname{id}_{{#1}}}
\renewcommand\id{\opname{id}}

% fig and others references
\newcommand\figref[1]{Fig.~\ref{#1}}
\newcommand\exref[1]{Ex.~\ref{#1}}
\newcommand\defref[1]{Def.~\ref{#1}}
\newcommand\tabref[1]{Table~\ref{#1}}
\newcommand\diagref[1]{(\ref{#1})}
%\newcommand\eqref[1]{\ref{#1}}
\newcommand\sectref[1]{Sect.~\ref{#1}}
\newcommand\secref[1]{Sect.~\ref{#1}}
\newcommand\appref[1]{Appendix~\ref{#1}}
%\newcommand\eqref[1]{(\ref{#1})}
%===============================================


% my macros for Formulas 

% roman font in math formulas
\newcommand\rmand{\mbox{ and }}
\newcommand\rmor{\mbox{ or }}
\newcommand\rmxor{\mbox{ xor }}

\newcommand\eqdef{\ensuremath{\stackrel{\mathrm{def}}{=}}}

% semantic brackets 
\newcommand\respace{\!}%\!\!}
\newcommand\lsemm{\left[ \respace\left[ }
\newcommand\rsemm{\right]\respace\right]}
\newcommand\semm[1]{\mbox{$\lsemm\, \mathit{#1} \, \rsemm$}}

% less blank space
\newcommand\timm{{\times}}
\newcommand\inn{{\in}}
\newcommand\subsett{{\subset}}
\newcommand\supsett{{\superset}}

%Suggestive Names for MathSymbols
\newcommand\superset{\supset}
\newcommand\subeq{{\subseteq}}
\newcommand\supeq{{\supseteq}}
\newcommand\sqsubeq{{\sqsubseteq}}
\newcommand\sqsupeq{{\sqsupseteq}}
\newcommand\varno{{\varnothing}}
\newcommand\subsetarr{\ensuremath{\hookrightarrow}}
\newcommand\supsetarr{\ensuremath{\hookleftarrow}}

\newcommand\this{\ensuremath{\underline{\mathrm{this}}}}
\newcommand\self{\ensuremath{\underline{\mathrm{self}}}}


\newcommand\ovr[1]{\ensuremath{\overline{#1}}}
\newcommand\und[1]{\ensuremath{\underline{#1}}}


\newcommand\rarr{{\rightarrow}}
%\newcommand\lar{\leftarrow}
\newcommand\larr{{\leftarrow}}
\newcommand\ifff{\Leftrightarrow}
\newcommand\iffarrow{\Leftrightarrow}
\newcommand\bottom{\perp}
\newcommand\disj{\vee}
\newcommand\sdisj{\stackrel{!}{\vee} }
\newcommand\conj{\wedge}
%\newcommand\mathand{\,\&\,}
\renewcommand\neg{\sim}
\newcommand\ded{\vdash}
\newcommand\semded{\models}
\newcommand\synent{\ensuremath{\vdah}}
\newcommand\sement{\ensuremath{\models}}

\newcommand\njoin[2]{\mathbin{${#1}\triangleright\!\triangleleft\;{#2}$}}

%\newcommand\ifthenelse[3]{{\bf if}#1{\bf then}#2{\bf else}#3}


\newcommand\true{\nmf{true}}
\newcommand\false{\nmf{false}}

% Operations 

\newcommand\image[2]{\opname{Image}_{#1}{#2}}
\newcommand\img[2]{\image{#1}{#2}}
%\newcommand\range[2]{\Operation{Range}_{#1}({#2})}

%\newcommand\aut{\ensuremath{\operation{Aut}}}
\newcommand\isoind{\opname{iso}}
\newcommand\iso{\isoind}

\newcommand\coimage[2]{\opname{CoIm}_{#1}{#2}}
\newcommand\coim[2]{\coimage{#1}{#2}}

\renewcommand\restriction[2]{#1\left\lceil_{#2}\mathstrut\right.}
\renewcommand\restriction[2]{\ensuremath{#1{\upharpoonright}_{#2}\mathstrut}}
\newcommand\restr[2]{\restriction{#1}{#2}}

\newcommand\idmap[1]{\Operation{id}_{#1}}

\newcommand\Inverse[1]{\left (\mathstrut {#1} \right )^{-1}}
%\newcommand\inverse[1]

%  Comprehension

\newcommand\comprehension[2]{\ensuremath{\left\{{#1}\left|\;{#2}\right.\right\}}}
\renewcommand\comprehension[2]{\ensuremath{\left\{{#1}| \;{#2}\right\}}}  % big brackets
%\renewcommand\comprehension[2]{\ensuremath{\{{#1}| \;{#2}\}}} % small brackets
\newcommand\compr[2]{\comprehension{#1}{#2}}
\newcommand\tuplecompr[2]
{\left\langle{#1}\left|\;{#2}\right.\right\rangle}
\newcommand\tuple[1]{\left\langle\mathstrut {#1}\right\rangle}
\newcommand\cotuplecompr[2]
{\left\rangle\mathstrut {#1}\left|\;{#2}\right.\right\langle}
\newcommand\cotuple[1]{\left\rangle\mathstrut {#1}\right\langle\;}
\newcommand\family[2]{\left(\mathstrut #1 \right)_{#2}}
\newcommand\famm[2]{\family{#1}{#2}}
% big brackets
\newcommand\comprfam[2]{\left(\mathstrut{#1}\left|\;{#2}\right.\right)}
\newcommand\famcompr[2]{\left(\mathstrut{#1}\left|\;{#2}\right.\right)}
% normal brackets
\renewcommand\comprfam[2]{(\mathstrut{#1}\left|\;{#2}\right.)}
\renewcommand\famcompr[2]{(\mathstrut{#1}\left|\;{#2}\right.)}
\newcommand\newfamm[2]{\compfamily{#1}{#2}}
\newcommand\arrfamm[4]{\family{%
		\lar{#1}{#2}{#3}%
	}{#4}}


\newcommand\cotimes{+}
\newcommand\noteq{\ne}
\newcommand\mybigcup[2]{\bigcup\compr{#1}{#2}}
\newcommand\mybigcap[2]{\bigcap\compr{#1}{#2}}

\newcommand\myprod[1]{{#1 \prod}}



%-- categories names
\newcommand\catname[1]{\mbox{\bfseries\itshape #1}}
%\newcommand\cat[1]{\catname{#1}}
\newcommand\catnameind[1]{{\pmb #1}}
\newcommand\categoryop[1]{\mbox{\bfseries\itshape #1}$^{\mathrm{op}}$}



%\renewcommand\cat[1]{\catname{#1}}
\newcommand\CC{\catname{C}}

\newcommand\graphcat{\catname{Graph}}
\newcommand\setcat{\catname{Set}}
\newcommand\twocat{\catname{2}}
\newcommand\relcat{\catname{Rel}}
\newcommand\catcat{\catname{Cat}}
\newcommand\natset{\catname{Nat}}
\newcommand\gracat{\catname{Graph}}
\newcommand\rgracat{\catname{rGraph}}
\newcommand\twogracat{\catname{2Graph}}
\newcommand\dbgracat{\catname{dblGraph}}
\newcommand\posetcat{\catname{Poset}}
\newcommand\reprcat{\catname{Repr}}
\newcommand\schemacat{\catname{Schema}}
%\newcommand\catname[1]{\mbox{\boldmath $#1$}}



%=== word shorcuts
% \newcommand\eg{e.g.}
% \newcommand\ie{i.e.}
% \newcommand\etal{\textit{et al}}
%\newcommand\fwk{framework}
%\newcommand\traj{trajector}
%\newcommand\traj{trajector}
%\newcommand\syncon{synchronization}
%\newcommand\Syncon{Synchronization}
\newcommand\symmen{symmetrization}
\newcommand\Symmen{Symmetrization}


\endinput




\setlength{\marginparwidth}{3cm}
%\setlegth{\marginparsep}{1.5mm}
%\setlength{\marginparpush}{5mm}
%

\makeatletter
  \def\fps@figure{tp}
\makeatother

\newcommand{\backgro}[2]{\par\noindent\framebox[\textwidth]{
\begin{minipage}{0.98\textwidth}
\setlength{\parindent}{0.5cm} \noindent \textbf{Background: #1} #2
\end{minipage}}\smallskip}

%%%% macros %%%
%\newtheorem{defin}{Definition}%[section]
%\renewcommand{\thedefin}{\Alph{defin}}

\newcounter{defCounter}
\newenvironment{defin}[1][]{
\refstepcounter{defCounter}
\begin{trivlist}
\item[\hskip \labelsep {\bfseries Definition \arabic{defCounter} (#1) }]}%
{\end{trivlist}}



%\newcommand\xxx[4]{{\it #1}\mbox{$_{#3}^{#4}{#2}$}}
%\newcommand{\s}{\star}
%\newcommand\mrk[1]{\mbox{$\langle${\tt #1}$\rangle$}}
%=================================================
% 1  Fonts and letters
%============================================

%=====================================================
% 2  Mathematical shtuchki
%=========================================================


% New Symbols allowed to use in MathMode (!)
%========= General =============
\newcommand\mylist[2]{\mbox%
                          {$#1_1,\ldots,#1_{#2}$}}

\newcommand\iidots[2]{\mbox{
                            $#1=1,\ldots,#2$
                      }}
\newcommand\ijdots[3]{\mbox{
                            $#1=#2,\ldots,#3$
                      }}
\newcommand{\vare}{\varepsilon}
\newcommand\nr{\normalsize\rm}
\newcommand\tril{\triangleleft}
\newcommand\eqdef{\stackrel{\rm def}{=}}
\newcommand\trir{\triangleright}
\newcommand\bc{\bigcirc}







%(4)%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Abbreviations of words from pre_gen
%%%%%%%%%%%%%%%%%%%%%

%\newcommand\ql{query \lan} comment for ISMIS'96
\newcommand\sync{synchronous}
\newcommand\async{asynchronous}
\newcommand\syncn{synchronization}
\newcommand\syncd{synchronized}
\newcommand\Sync{Synchronous}
\newcommand\Async{Asynchronous}
\newcommand\Syncn{Synchronization}
\newcommand\Syncd{Synchronized}

\newcommand\sce{scenario}

\newcommand\eqe{equivalence}
\newcommand\eqt{equivalent}

\newcommand\intn{intuition}
\newcommand\intv{intuitive}
\newcommand\coa{coalgebra}
\newcommand\ispartof{\ittt{isPartOf}}
\newcommand\isPartOf{\ittt{isPartOf}}
\newcommand\IsPartOf{\ittt{isPartOf}}

\newcommand\of{\ittt{(isPart)Of}}
\newcommand\Of{\ittt{Of}}
\newcommand\arrdl{ArrDL}
\newcommand\elmsl{ElmSL}

\newcommand\isa{\ittt{isA}}
\newcommand\IsA{\ittt{isA}}
\newcommand\isA{\ittt{isA}}


\newcommand\subst{\ittt{subst}}


\newcommand\OOAD{OOA\&D}
\newcommand\oid{o-id}

\newcommand\pred{predicate}

\newcommand\interstan{interstate relation}
\newcommand\intrel{interstate relation}
\newcommand\demon{demonstration}
\newcommand\demoe{demonstrate}
\newcommand\asson{association}
\newcommand\config{configuration}
\newcommand\asscon{association configuration}
\newcommand\ass{associative}
\newcommand\assive{associative}
\newcommand\aggrn{aggregation}
\newcommand\attrn{attribution}
\newcommand\abbrn{abbreviation}
\newcommand\gen{generalization}
\newcommand{\iden}{identification}
\newcommand\idey{identity}
\newcommand\qualn{qualification}
\newcommand\reprn{representation}
\newcommand\situn{situation}
\newcommand\speln{specialization}
\newcommand\spen{specialization}
\newcommand\spel{specialization}
\newcommand\spec{specification}
\newcommand\implen{implmentation}
\newcommand\impleg{implmenting}
\newcommand\strul{structural} %\strul

\newcommand\spenisa{\spen\ \isa-arrow}
\newcommand\genisa {\gen\  \isa-arrow}

\newcommand\visun{visualization}


%\newcommand\gen{generalization}
\newcommand\repr{representation}

\newcommand\visn{visualization}


%\newcommand{\oid}{object identity}
\newcommand{\oids}{object identities}



\newcommand\datamod[1]{{\rm #1}}

\newcommand\ERC{\datamod{ERC\mbox{$^+$}}}
\newcommand\ercd{\ERC-diagram}
\newcommand\ER{\datamod{ER}}
\newcommand\EER{\datamod{EER}}
\newcommand\RM{\datamod{RM}}
\newcommand\RMT{\datamod{RM/T}}
\newcommand\RDM{\datamod{RDM}}
\newcommand\VO{\datamod{VO}}
\newcommand\OOO{\datamod{OO}}
\newcommand\SDM{\datamod{SDM}}
\newcommand\FDM{\datamod{FDM}}
\newcommand\IFO{\datamod{IFO}}
\newcommand\Oid{\datamod{Oid}}
\newcommand\RO{\datamod{RO}}
\newcommand\ROP{\datamod{RO\mbox{$^+$}}}
\newcommand\Flogic{\datamod{F-logic}}
\newcommand\SkeDM{\datamod{SkeDM}}
\newcommand\Diagr{\datamod{Diagrams}}

\newcommand\datatrend[1]{{\bf #1}}

\newcommand\eer{\datatrend{eer}}
\newcommand\ooo{\datatrend{oo}}
\newcommand\pl{\datatrend{pl}}
\newcommand\skeske{\datatrend{ske}}

\newcommand\msour{multisource}
\newcommand\sour{source}

\newcommand\abbr{abbreviat}
\newcommand\lega{legacyless}


\newcommand\Ass{Associative}



\newcommand{\ider}{identifier}
\newcommand{\deor}{descriptor}

\newcommand\dombs{domain-based sketch}
\newcommand\ms{multisource}
\newcommand\mt{multitarget}
\newcommand\refin{refinement}
\newcommand\db{database}
\newcommand{\grab}{graph-based }
\newcommand{\spef}{specification}
%\newcommand\spec{specification}
\newcommand{\grabs}{\grab\spef}
\newcommand{\lan}{language}
\newcommand{\sgd}{\spel$\!$/\gen distinction }
\newcommand\qr{query }
\newcommand\qrs{queries}

%%%%% Integration %%%%%%%%%%%%%

\newcommand{\integ}{integration}
\newcommand{\intd}{integrated}
\newcommand{\di}{data integration }
\newcommand{\dbi}{database integration }
\newcommand{\vi}{view integration }
\newcommand{\si}{schema integration}
\newcommand{\sdi}{schema and data integration }
%-------------------------------------
\newcommand{\cmod}{conceptual modeling}
\newcommand{\smod}{semantic modeling}
\newcommand{\dbs}{data base}
\newcommand{\dml}{data model}
%\newcommand{\dm}{data model}%{dm}%{DM} % an abbreviation
\newcommand\const{constraint}
\newcommand{\attr}{attribute}
%=====================================
\newcommand\cdb{component \db}
\newcommand\dincy{data inconsistency}
\newcommand\corr{correspondence}
\newcommand\lang{language}
%------
\newcommand\corinf{correspondence information}
\newcommand\corrinf{correspondence information}

\newcommand\coras{correspondence assertion}
\newcommand\corass{correspondence assertions}
\newcommand\corda{correspondence data}
\newcommand\coreq{\corr\ equation}
\newcommand\coreqs{\corr\ equations}

\newcommand\dacorr{data \corr}
\newcommand\cors{\corr\ \ske}
\newcommand\corss{\corr\ \skes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\relship}{relationship}
%----------------------------------------
\newcommand{\Spc}{Spaccapietra {\em et al} }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\ske{sketch}
\newcommand\skes{sketches}
\newcommand\cske{component sketch}
\newcommand\cskes{component sketches}
\newcommand\eroo{\cite{ER95}}
%%%%%%%%%%%% Romanic abbreviations  %%%%%%%%%%%%
\newcommand\eg{e.g.}
\newcommand\ie{i.e.}
\newcommand\wrt{w.r.t.}
\newcommand\etc{{\em etc}}
\newcommand\etal{{\em et al}}
\newcommand\ala{{\em a la }}
\newcommand\apriori{{\em a priori}}
\newcommand\adhoc{{\em ad hoc}}
\newcommand\dejure{{\em de jure}}
\newcommand\defacto{{\em de facto}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\sign}{signature}
%\newcommand{\constr}{constructivizab}% *le or *ility
%\newcommand{\cat}{category}
%\newcommand{\cats}{categories}
%\newcommand{\ct}{category theory\ } %y or ies
%\newcommand\mor{morphism}
%\newcommand\amor{automorphism}
%\newcommand\alg{algebra}
%%\newcommand\inst{institution}
%=============================

%(5)\newcommand\entails{\Rightarrow}
%\newcommand\implies{\Rightarrow}
%-------------------------------------
%\newcommand\dom[1]{\mathit{Dom}(#1)}
%\newcommand\cod[1]{\mathit{Cod}(#1)}
\newcommand\rg[1]{\mathit{Rg}(#1)}
\newcommand\DOM[1]{\Box #1}
\newcommand\COD[1]{#1 \Box}

\newcommand\tabname[1]{\mbox{$\ittt{Tab}\_#1$}}
%\newcommand\multisource[
\newcommand\mytilde[1]{\widetilde{#1}}
\newcommand\sempr[1]{\mytilde{\semm{#1}}}

\newcommand\mycount[1]{{\bf count}{(#1)}}
\newcommand\gragen[1]{\left[\mathstrut #1 \right]}

\newcommand\respace{\!}%\!\!}
\newcommand\lsemm{\left[ \respace\left[ }
\newcommand\rsemm{\right]\respace\right]}
\newcommand\semm[1]{\mbox{$\lsemm\, \mathit{#1} \, \rsemm$}}
\newcommand\semmind[2]{\mbox{$\lsemm\, \mathit{#1} \, \rsemm^{#2}$}}



\newcommand\semmindex[1]{\lsemm\, \mathit{#1} \, \rsemm}
\newcommand\semmstar[1]{\semm{#1}^{*}}
\newcommand\lbesemm{\left< \respace\left<}
\newcommand\rbesemm{\right> \respace\right>}
\newcommand\besemm[1]{\mbox{$\lbesemm\, \mathit{#1} \, \rbesemm$}}



%(6)%\newcommand\informalPar[1]{\nicex{{#1}$}}
%\newcommand\infParind[1]{\cal #1}
%Contents:
%--- semiotics
%--- Skesig
%--- Varset
%--- Behset



%%==== Semiotics =====
%
%%\newcommand\formalPar[1]{\mbox{$\mathrm{#1}$}}
%\newcommand\frmParind[1]{\mathrm{#1}}
%
%\newcommand\informalParBold[1]{\mbox{${\cal #1}$}}
%\newcommand\formalPar[1]{\mbox{$\mathrm #1$}}
%
%\newcommand\object[2]{\mbox{${\mathsf{#1}}_{#2}$}}
%%\newcommand\object[2]{\mbox{$#1_{#2}$}}
%\newcommand\universe[1]{\mbox{$\mathbf{#1}$}}
%%\newcommand\objectind[1]{\mathsf{#1}}
%\newcommand\objectind[1]{\mathsf{#1}}
%\newcommand\universeind[1]{\mathbf{#1}}
%
%\newcommand\proc[1]{\mbox{\sffamily\bfseries #1}}
%\newcommand\procind[2]{\mbox{${\mathrm{#1}}_{\mathrm #2}$}}
%\newcommand\linf{\informalParBold{L}}
%\newcommand\minf{\mbox{$\informalPar{M}(\diag{})$}}
%\newcommand\mdinf{\mbox{$\informalPar{M}(\diag{})$}} % the same as above
%\newcommand\mdfrm{\mbox{$\formalPar{M}(\diag{})$}} % the same as above
%\newcommand\uinf{\informalPar{U}}
%
%\newcommand\meaninf{\informalPar{M}}
%\newcommand\meanfrm[1]{\mbox{$\formalPar{M}_{#1}$}}
%\newcommand\diag[1]{\object{D}{#1}} %\mbox{$D$}}
%\newcommand\diagob[1]{\object{D}{#1}} %\mbox{$D$}}
%\newcommand\diags{\mbox{$\mathit{Diags}$}}
%\newcommand\graph{\mbox{$\mathit{Graph}$}}
%\newcommand\skeob[1]{\object{S}{#1}}
%\newcommand\modelob[1]{\object{M}{#1}}
%\newcommand\sigob[1]{\object{\mbox{$\Sigma$}}{#1}}
%\newcommand\skediag{\skeob{}[\diag{}]}
%\newcommand\meaninfdiag{\meaninf[\diag{}]}
%\newcommand\meanfrmdiag{\meanfrm[\diag{}]}
%% synonyms
%\newcommand\meanifdiag{\meaninf[\diag{}]}
%\newcommand\meanfdiag{\meanfrm[\diag{}]}

%=======================
%==== Skesig
%\newcommand\so[1]{source(#1)}
%\newcommand\ta[1]{target(#1)}
\newcommand\U{{\cal U}}
\newcommand\M{{\cal M}}
\newcommand\Set{{\mathbf Set}}
\newcommand\Varset{{\mathbf Varset}}
\newcommand\univ{\mbox{$\mathbf U$}}
\newcommand\univind{{\mathbf U}}
\newcommand\skesig{\mbox{$\Sigma$}}

%%%% macro\Skesig.tex %%%%  June 29

\newcommand\mrkid{\mrk{ID}}
\newcommand\imID{\mbox{ID?}} %$^*$}}
\newcommand\mrkidd{\imID} % marker of IDDeficient
\newcommand\prodid{\mbox{$\times$-\ider}}
\newcommand\plusid{\mbox{$+$-\ider}}
\newcommand\prodkey{\mbox{$\times$-key}}
\newcommand\pluskey{\mbox{$+$-key}}

\newcommand\ID{\mrk{ID}}
\newcommand\IDplus{\mrk{ID$^+$}}
\newcommand\IDprod{\mrk{ID$^\times$}}

\newcommand\andiden{\emph{and}-\iden}
\newcommand\oriden{\emph{or}-\iden}


\newcommand\ssta{\mbox{${\mathsf S}_{\mathrm sta}$}}
\newcommand\sdyn{\mbox{${\mathsf S}_{\mathrm dyn}$}}

%\newcommand\mrk[1]{\mbox{[${\tt #1}$]}}
%\newcommand\mrk[1]{\mbox{[${\mathbf{#1}}$]}}
%\newcommand\mrkop[1]{\mbox{$\langle{\tt #1}\rangle$}}
\newcommand\mrkop[1]{\mbox{$\langle{\mathbf{#1}}\rangle$}}
\newcommand\mrkopr[1]{\mbox{$\mathbf{[{#1}\rangle}$}}
\newcommand\mrkopl[1]{\mbox{$\mathbf{\langle{#1}]}$}}
\newcommand\mrksemiop[1]{\mbox{$\langle{\tt #1}]$}}
\newcommand\mrkNode[1]{\mbox{${\tt #1}$}}
\newcommand\mrkn[1]{\mrkNode{#1}}
\newcommand\mrktt[1]{{\tt #1}}
\newcommand\mrkopright[1]{\mbox{$[${\tt #1}$\rangle$}}
\newcommand\mrkopleft[1]{\mbox{$\langle${\tt #1}$]$}}
%%%%%%%%%%%%%  Begin Key commands %%%%%%%%%%%%%%%%%%%%%%%

\newcommand\PredicateSignature{\Pi}
\newcommand\OperationSignature{\Sigma}
\newcommand\predFromOperSig{\Sigma_{pr}}
\newcommand\BaseSignature{\bf B}
\newcommand\DomainBase{\bf B}

\newcommand\ConstraintLanguage{CL}
\newcommand\dolan%DomainLanguage{\Delta}
{\mbox{$\Delta $}}

\newcommand\dolanm{\Delta}

\newcommand\adtm{ADT}
\newcommand\adt{{\sl \adtm}}
\newcommand\dolanadt{\dolan_{\adtm}}
\newcommand\sigadt{{\it Sig}_{\adtm}}
\newcommand\semmadt{\semm{}_{\adtm}}

\newcommand\dbauxm{DBD}
\newcommand\dbaux{{\sl \dbauxm}}
\newcommand\dolandbaux{\dolan_{\dbauxm}}
\newcommand\sigdbaux{{\it Sig}_{\dbauxm}}
\newcommand\semmdbaux{\semm{}_{\dbauxm}}

\newcommand\ba{D}
\newcommand\domba{\mbox{$\Domain(\ba)$}}
\newcommand\bam{\BasicDomainMarkerSymbol}          %  B  for using in math mode
%\newcommand\V{\mbox{$\TheValueUniverse_{\dolanm}$}}%

\newcommand\Pred{{\it Pred}}
\newcommand\Oper{{\it Op}}
\newcommand\Base{{\it Base}}
\newcommand\Dom{{\it Dom}}
\newcommand\Domain{{\it Dom}}
\newcommand\pool{V}

\newcommand\ArityMap{{\it Shp}}
\newcommand\ArityGraph{D}
\newcommand\AritySketch{{\cal D}}
\newcommand\ArityInclusion{\mbox{\Large $\iota$}}

\newcommand\rms{\rm\scriptsize}   % for writing, eg, \D^{\rms in}

\newcommand\PredicateMarkerSymbol{P}
\newcommand\OperationMarkerSymbol{F}
\newcommand\BasicDomainMarkerSymbol{B}

\newcommand\PredicateDiagramSet[1]{\PredicateMarkerSymbol^{#1}}%P^#1}
\newcommand\OperationDiagramSet[1]{\OperationMarkerSymbol^{#1}}%F^#1}
\newcommand\BasicDomainDiagramSet[1]{\BasicDomainMarkerSymbol^{#1}}%B^#1}

\newcommand\AGraph{G}
\newcommand\g{\mbox{$\AGraph$}}
\newcommand\gm{\AGraph}

\newcommand\ASketchSymbol{S}
\newcommand\ASketch{\mathsf \ASketchSymbol}
\newcommand\s{\mbox{$\ASketch$}}
\newcommand\sind{\ASketch}
\newcommand\sm{\ASketch}
\newcommand\sprim{\mbox{$\ASketch'$}}
\newcommand\sbipr{\mbox{$\ASketch''$}}


\newcommand\TheUniverseSymbol{U}
\newcommand\TheUniverseSketch{\cal \TheUniverseSymbol}
\newcommand\TheObjectUniverse{Obj }%{\cal O}
\newcommand\TheTimeUniverse{\cal T}%{T}
\newcommand\TheHistoryUniverse{\cal \TheTimeUniverse^*}%}
\newcommand\TheValueUniverse{Val}%{\cal V}

\newcommand\ASketchAlgebra{\cal A}
\newcommand\ABaseSubSketch{\cal B}    % base subsketch of

\newcommand\APermutation{\pi}

%===================================================

\newcommand\Mod[1]{\mbox{{\bf Mod}$(#1)$}}
\newcommand\Ext[1]{\mbox{{\bf Ext}$(#1)$}}
\newcommand\Inst[1]{\mbox{{\bf Inst}$(#1)$}}

%%%%%%%%%%%%%   End Key commands %%%%%%%%%%%%%%%%%


%%%%%%%%%%%%    Useful Abbreviations %%%%%%%%%%%%

%%% Sketchi


\newcommand\sdom{\mbox{$\s_{\DomainBase}$}}
\newcommand\sdomm{\s_{\DomainBase}}

\newcommand\newb{\mbox{$\DomainBase$}}
\newcommand\bm{\DomainBase}

\newcommand{\bs}{\mbox{$\ABaseSubSketch$}}
\newcommand\bsm{\ABaseSubSketch}

\newcommand\skespe{{\bf \ASketchSymbol}}

\newcommand\gras{{\it Gra}\skeob}
\newcommand\doms{{\it Dom}\skeob}
\newcommand\clas{{\it Cla}\skeob}
\newcommand\rels{{\it Rel}(\skeob)}

\newcommand\R{\nicex{ R$}}
\newcommand\OO{\mbox{$\TheObjectUniverse$}}
%\newcommand\T{\mbox{$\TheTimeUniverse$}}
%\newcommand\Hist{\mbox{$\TheHistoryUniverse}}
%\newcommand\V{\mbox{$\TheValueUniverse_{\bm}$}}%

\renewcommand\u{\mbox{$\TheUniverseSketch$}}
\newcommand\um{\TheUniverseSketch}
\newcommand\upred{\mbox{$\TheUniverseSketch_{\predsigm}$}}
\newcommand\uoper{\mbox{$\TheUniverseSketch_{\opersigm}$}}

\newcommand\predsig{\mbox{$\PredicateSignature$}}
\newcommand\predsigm{\PredicateSignature}
\newcommand\opersig{\mbox{$\OperationSignature$}}
\newcommand\opersigm{\OperationSignature}
\newcommand\predopsig{\mbox{$\predFromOperSig$}}
%\newcommand\pros{\predopsig}
\newcommand\prosm{\predFromOperSig}
\newcommand\basesig{\mbox{\BaseSignature}}
\newcommand\basesigm{{\BaseSignature}}
\newcommand\clan{\mbox{$\ConstraintLanguage$}}
\newcommand\clanm{\ConstraintLanguage}
\newcommand\colan{\mbox{\ConstraintLanguage}}
\newcommand\clanform{\mbox{$\ConstraintLanguage=(\Pred,\arimap,\semm{})$}}
\newcommand\colanm{\ConstraintLanguage}
%\newcommand\dolan{\mbox{\DomainLanguage}}
%\newcommand\dolanm{\DomainLanguage}

\newcommand\pis{$\PredicateSignature $-sketch}
\newcommand\sis{$\OperationSignature $-sketch}
\newcommand\siprs{$\predFromOperSig$-sketch}
\newcommand\sia{$\OperationSignature $-algebra}
\newcommand\clans{$\Constraint Language$-sketch}

\newcommand\arimap{\ArityMap}
\newcommand\arimapin{\mbox{\ArityMap$^{\rms in}$}}

\newcommand\os{\mbox{$\overline{\s}$}}
%\newcommand\go{\mbox{$G_{({\cal O})}$}}

\newcommand\pip{\mbox{$\APermutation^{+}$}}
\newcommand\depipComp{\mbox{$\delta \comp\APermutation^{+}$}}
\newcommand\depip{\mbox{$\APermutation^{+}\delta $}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%                                  %%%%%%%%%%%%%%%%%
%%%%%%%%%%            A R I T I E S         %%%%%%%%%%%%%%%%%%
%%%%%%%%%%                                  %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\pr{\mbox{$\PredicateMarkerSymbol$}}  % $P$ for using in text mode
\newcommand\op{\mbox{$\OperationMarkerSymbol$}}  % $F$ for using in text mode
%\newcommand\ba{\mbox{$\BasicDomainMarkerSymbol$}}  % $P$ for using in text mode


\newcommand\myprm{\PredicateMarkerSymbol}        %  P  for using in math mode
\newcommand\opm{\OperationMarkerSymbol}          %  F  for using in math mode
%\newcommand\bam{\BasicDomainMarkerSymbol}       %  B  for using in math mode

%%%%   functions to put the arg
%%%%   as subindex near \pr,\op and \ba

\newcommand\prix[1]{\myprm_{#1}}
\newcommand\opix[1]{\opm_{#1}}
\newcommand\baix[1]{\bam_{#1}}

%%%----  end functions

\newcommand\pri{$\myprm_{i}$}    %  \pr_i for using in text mode
\newcommand\opi{$\opm_{j}$}      %  \op_j for using in text mode
\newcommand\bai{$\bam_{l}$}      %  \ba_l for using in text mode

\newcommand\prim{\myprm_{i}}     %  \pr_i for using in math mode
\newcommand\opim{\opm_{j}}       %  \op_j for using in math mode
\newcommand\baim{\bam_{l}}       %  \ba_l for using in text mode
%======================================
%  eto makrosy funcciy
\renewcommand\Pr[1]{\PredicateDiagramSet{#1}}  % P^#1
\newcommand\Op[1]{\OperationDiagramSet{#1}}    % F^#1
\newcommand\Ba[1]{\BasicDomainDiagramSet{#1}}  % B^#1
%  a eto ih znacheniya
\newcommand\PrS{\Pr{\s}}      % P^\s
\newcommand\OpS{\Op{\s}}      % F^\s
\newcommand\BaS{\Ba{\s}}      % B^\s
%\newcommand\domba{$\Domain(\ba)$}

\newcommand\PrU{\Pr{\u}}      % P^\u
\newcommand\OpU{\Op{\u}}      % F^\u
\newcommand\BaU{\Ba{\u}}      % B^\u

%------------------------------------------------
% eto makrosy funkciy s 2 argumwntami
\newcommand\Prix[2]{\Pr{#1}_{#2}}              % a set P^#1_#2
\newcommand\Opix[2]{\Op{#1}_{#2}}              % a set F^#1_#2
\newcommand\Baix[2]{\Ba{#1}_{#2}}              % a set B^#1_#2
% a eto b nih podstavleny indexy i ostalsya 1 argument
\newcommand\Pri[1]{$\Prix{#1}{i}$}             % a set og diag, P^#1_i
\newcommand\Opi[1]{$\Opix{#1}{j}$}             % a set of diag, F^#1_j
\newcommand\Bai[1]{$\Baix{#1}{l}$}             % a set of diag, B^#1_l
% a eto znacheniya
\newcommand\PriS{\Pri{\s}}      % Pi^\s
\newcommand\OpiS{\Opi{\s}}      % Fj^\s
\newcommand\BaiS{\Bai{\s}}      % Bl^\s

\newcommand\PriU{\Pri{\u}}      % Pi^\u
\newcommand\OpiU{\Opi{\u}}      % Fj^\u
\newcommand\BaiU{\Bai{\u}}      % Bl^\u

%  a eto dlya mat mode
\newcommand\Prim[1]{\Prix{#1}{i}}     %  a set of diagr,  P^#1_i for using in math mode
\newcommand\Opim[1]{\Opix{#1}{j}}     %  a set of diagr,  F^#1_j for using in math mode
\newcommand\Baim[1]{\Baix{#1}{l}}     %  a set of diagr,  B^#1_#2 for using in math mode
%====================================================

%\newcommand\pool{V}
\newcommand\vx[1]{\mbox                                  % D_arg
                      {$\pool_{#1}$}}
\newcommand\vinx[1]{\mbox                                % D^in_arg
                      {$\pool^{\mbox\rms in}_{#1}$}}
\newcommand\voutx[1]{\mbox                               % D^out_arg
                      {$\pool^{\mbox\rms out}_{#1}$}}
%============================================================

%\newcommand\ArityGraph{D}
%\newcommand\AritySketch{\D}                             % \D - nice D
\newcommand\sprx[1]{\mbox                                %  D_arg
                      {$\ArityGraph_{#1}$}}
\newcommand\sopx[1]{\mbox                                % \D_arg
                      {$\AritySketch_{#1}$}}
\newcommand\sinx[1]{\mbox                                % \D^in_arg
                      {$\AritySketch^{\rms in}_{#1}$}}
\newcommand\soutx[1]{\mbox                               % \D^out_arg
                      {$\AritySketch^{\rms out}_{#1}$}}

%-----   marker-subindex version
\newcommand\spr{\sprx{\myprm}}         %  D_{prop marker}
\newcommand\sop{\sopx{\opm}}         % \D_{oper marker}
\newcommand\sinop{\sinx{\opm}}       % \D^in_{oper mark}
%-----   i-subindex version
\newcommand\spri{\sprx{i}}          %  D_{i}
\newcommand\sopi{\sopx{j}}          % \D_{j}
\newcommand\sinopi{\sinx{j}}        % \D^in_{j}



\newcommand\opshaxy[2]{\inclar{#1_{#2}}  % arg1_arg2: D^in_arg2 -->D_arg2
                            {\sinx{#2}}
                              {\sopx{#2}}
                       }
%\newcommand\ArityInclusion{i}
\newcommand\opsha{\opshaxy{\ArityInclusion}{\opm}}   %i_f: D^in_f   --> D_f
\newcommand\opshai{\opshaxy{\ArityInclusion}{\opim}} %i_f: D^in_f_j --> D_f_j

%----------------------------------------

%\newcommand\ArityMap{{\it Shp}}
\newcommand\arix[1]{\mbox
                        {$\ArityMap({#1})$}}         % Shp(arg)
\newcommand\ariinx[1]{\mbox
                        {$\ArityInclusion_{#1}$}}    % \iota_{arg}

\newcommand\aripr{\arix{\myprm}}                  % Shp(p)
\newcommand\ariop{\arix{\opm}}                  % Shp(f)
\newcommand\arinc{\ariinx{\opm}}                % \iota_f

\newcommand\aripri{\arix{\prim}}                % Shp(p_i)
\newcommand\ariopi{\arix{\opim}}                % Shp(f_j)
\newcommand\arinci{\ariinx{\opim}}              % \iota_j

%-----------------------------------------
\newcommand\sepr{\semm{\pr}}
\newcommand\seop{\semm{\op}}
\newcommand\sepri{\semm{\pri}}
\newcommand\seopi{\semm{\op}}


\newcommand\opv{\mbox{\Oper$^+$}}

%\endinput

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%              %%%%%%%%%%%%%%%
%%%%%%%%%%%  Old Macros %%%%%%%%%%%%%%%%
%%%%%%%%%%              %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\newcommand\sig{\mbox{$\PredicateSignature$}}
%\newcommand\gra{{\bf G}}
%\newcommand\sigo{\mbox{$\Sigma_1$}}
%\newcommand\grao{\mbox{${\bf G}_1$}}
%% OOPS! \newcommand\inst{\mbox{$\lar{\vare }{S}{W}$}}
%%\newcommand\sch{\Category{Schema} }
%
%
%\newcommand\instVareps{\mbox{$\lar{\vare }{S}{W}$}}
%\newcommand\inste{\mbox{$\lar{e}{S}{W}$}}
%\newcommand\emor[1]{\lar{e}{#1}{\u}}
%\newcommand\sv{\mbox{$S_V$}}
%\newcommand\sr{\mbox{$S_R$}}
%\newcommand\vmor{\lar{v}{\sv}{\ovrs{}}}
%\newcommand\rmor{\lar{r}{S}{\ovrs{R}}}
%\newcommand\vpair{\mbox{$V=(\sv,v)$}}
%\newcommand\rpair{\mbox{$R=(\sr,r)$}}
%===
%==== Varset
%% macros for writing formulas with varsets and varfunctions

%%%%%%%%%    ..\dke96\macro\varset.tex    %%%%%%%
%\renewcommand\c{\mbox{$\AClass$}}                    %   C
%\newcommand\cm{\AClass}                              %   C
%\newcommand\ce{\mbox{$\semm{\AClass}$}}              % ||C||

%\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}   % ||C||^#1

%\newcommand\cindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
% apply:
%\newcommand\cet{\ceind{\ltt}}                         % ||C||^t
%\newcommand\ceu{\ceind{\ltu}}                         % ||C||^u
\newcommand\ObjStt{\ittt{ObjStt}}
\newcommand\C{\textit{C}}
\newcommand\D{\textit{D}}

\newcommand\ot[1]{\mbox{$o^{\ltt_{#1}}$}}
\newcommand\otm{o^\ltt}
\newcommand\ou[1]{\mbox{$o^{\ltu_{#1}}$}}
\newcommand\otu{o^\ltu}

\newcommand\cet{\mbox{$\semm{C}^{\ltt}$}}                         % ||C||^t
\newcommand\ceti{\mbox{$\semm{C}^{\ltt_i}$}}                         % ||C||^t
\newcommand\ceu{\mbox{$\semm{C}^{\ltu}$}}                         % ||C||^t
\newcommand\ceprt{\mbox{$\sempr{C}^{\ltt}$}}                         % ||C||^t
\newcommand\cepru{\mbox{$\sempr{C}^{\ltu}$}}                         % ||C||^t


\newcommand\cetu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\AClass}^{\ltu}$}}
\newcommand\ceut{\mbox{$\vphantom{\semm{AClass}}^{\ltu}\!\semm{\AClass}^{\ltt}$}}
\newcommand\detu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass}^{\ltu}$}}
\newcommand\fetu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass_f}^{\ltu}$}}
\newcommand\djetu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass_j}^{\ltu}$}}
\newcommand\dietu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass_i}^{\ltu}$}}
\newcommand\deut{\mbox{$\vphantom{\semm{AClass}}^{\ltu}\!\semm{\TargetClass}^{\ltt}$}}
\newcommand\ceprtu{\mbox{$\vphantom{\sempr{AClass}}^{\ltt}\sempr{\AClass}^{\ltu}$}}
\newcommand\deprtu{\mbox{$\vphantom{\sempr{AClass}}^{\ltt}\sempr{\TargetClass}^{\ltu}$}}



\newcommand\cesu{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\AClass}^{\ltu}$}}
\newcommand\cest{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\AClass}^{\ltt}$}}
\newcommand\cett{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\AClass}^{\ltt}$}}

\newcommand\dest{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\TargetClass}^{\ltt}$}}
\newcommand\desu{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\TargetClass}^{\ltu}$}}

\newcommand\cestart{\mbox{${\semmstar{C}}^{\ltt}$}}                         % ||C||^t
\newcommand\cestaru{\mbox{${\semmstar{C}}^{\ltu}$}}                         % ||C||^t
\newcommand\cestartu{\mbox{${}^{\ltt}{\semmstar{C}}^{\ltu}$}}

\newcommand\ceto{\mbox{$\semm{\AClass}^{\ltt}_{o}$}}
\newcommand\ceuo{\mbox{$\semm{\AClass}^{ \ltu}_{o}$}}

\newcommand\cestarto{\mbox{${\semmstar{\AClass}}^{\ltt}_{o}$}}
\newcommand\cestaruo{\mbox{${\semmstar{\AClass}}^{ \ltu}_{o}$}}

%======================================================================

%  ----  Basic Command -----------

\newcommand\LogicalTime{\cal T}
\newcommand\SetOfHistories{\LogicalTime^*}
\newcommand\AHistory{H}%J}

%\newcommand\IndexingXupYdownZ[3]{\mbox{$#1^{#2}_{#3}$}}
%\newcommand\IntRelSymb{\varepsilon}%rho}
%\newcommand\IntRelSymb{\mbox{\Large$\iota$}}%rho}
%\newcommand\IntersttMap{\mbox{\ittt same}}%rho}

\newcommand\AClass{C}
\newcommand\SourceClass{C}
\newcommand\TargetClass{D}
\newcommand\e{E}
\newcommand\AReference{f}
\newcommand\AnotherReference{g}
%\newcommand\Identifier{\mbox{\Large$\iota$}}
\renewcommand\g{g}
%\newcommand\h{h}
%\newcommand\hind{h}


\newcommand\farr{\lar{\AReference}{\SourceClass}{\TargetClass}}
\newcommand\farris{\lar{\AReference_i}{\SourceClass}{\TargetClass_i}}
\newcommand\farrit{\lar{\AReference_i}{\SourceClass_i}{\TargetClass}}
\newcommand\ffams{\mbox{$\f=\famm{\farris}{i\in I}$}}
\newcommand\ffamt{\mbox{$\f=\famm{\farrit}{i\in I}$}}

\newcommand\garr{\lar{\AnotherReference}{\SourceClass}{\TargetClass}}
\newcommand\garrit{\lar{\AnotherReference_i}{\SourceClass}{\TargetClass_i}}
\newcommand\garris{\lar{\AnotherReference_i}{\SourceClass_i}{\TargetClass} }
\newcommand\gfams{\mbox{$\g=\famm{\garris}{i\in I}$}}
\newcommand\gfamt{\mbox{$\g=\famm{\garrit}{i\in I}$}}


\newcommand\iarr{\lar{\AReference}{\SourceClass}{\TargetClass}}
\newcommand\iarris{\lar{\Identifier_j}{\SourceClass}{\TargetClass_j}}
\newcommand\iarrit{\lar{\Identifier_j}{\SourceClass_j}{\TargetClass} }
\newcommand\ifams{\mbox{$\Identifier=\famm{\iarris}{j\in J}$}}
\newcommand\ifamt{\mbox{$\Identifier=\famm{\iarrit}{j\in J}$}}


\newcommand\AMoment{t}%j}
\newcommand\EarlierMoment{t}%j}
\newcommand\LaterMoment{u}%k}
\newcommand\EarlierEarlierMoment{s}%i}
\newcommand\LaterLaterMoment{v}%l}

\newcommand\ttt{t1,t2}

\newcommand\IndexingXupYdownZ[3]{\mbox{$#1^{#2}_{#3}$}}

%%%%%%%%%%%%%%%%%%%%%%
% -- Abbreviations ----
%%%%%%%%%%%%%%%%%%%%%%%%%%                    sket}}


\newcommand\T{\mbox{$\LogicalTime$}}
\newcommand\Tm{\LogicalTime}
\newcommand\Hist{\mbox{$\SetOfHistories$}}
\newcommand\Histm{\SetOfHistories}
\newcommand\IntersttMap{\mbox{\ittt{same}}}%rho}
\newcommand\same[2]{\mbox{$\IntersttMap^{#1}_{#2}$}}
\newcommand\inter[2]{\same{#1}{#2}}
\newcommand\interpr[2]{\mbox{$\mytilde\IntersttMap^#1_#2$}}
% \IndexingXupYdownZ{\IntRelSymb}{#1}{#2}}  %\vare^#1_#2
%\newcommand\interpr[2]%
%      {\IndexingXupYdownZ{\mytilde{\IntRelSymb}}{#1}{#2}}  %\vare^#1_#2

%%% The new version t is denoted by \ltt, u is denoted by  \ltu etc

\newcommand\ttu{\EarlierMoment\LaterMoment}   %tu
\newcommand\logtimet{\EarlierMoment}               %t
\newcommand\ltt{\EarlierMoment}               %t
%\newcommand\tu{\LaterMoment}                  %u
\newcommand\ltu{\LaterMoment}                  %u
\newcommand\ttlu{\mbox{$\ltt\le\ltu$}}         % t =< u
\newcommand\tleu{\mbox{$\ltt\le\ltu$}}         % t =< u
\newcommand\tlu{\mbox{$\ltt<\ltu$}}            % t < u
\newcommand\logtimes{\EarlierEarlierMoment}        %s
\newcommand\lts{\EarlierEarlierMoment}               %t
\newcommand\ltv{\LaterLaterMoment}             %l
\newcommand\tv{\LaterLaterMoment}             %l

\newcommand\J{\AHistory}                      %J

\newcommand\intertu[1]{\inter{\ltt\to\ltu}{#1}}       % \eps^tu_#1
\newcommand\interut[1]{\inter{\ltt\gets\ltu}{#1}}       % \eps^tu_#1
\newcommand\intertuut[1]{\inter{\ltt\leftrightarrow\ltu}{#1}}       % \eps^tu_#1

\newcommand\intertt[1]{\inter{\ltt\to\ltt}{#1}}                 % \eps^tu_#1

\newcommand\interst[1]{\inter{\lts\to\ltt}{#1}}       % \eps^tu_#1
\newcommand\interts[1]{\inter{\lts\gets\ltt}{#1}}       % \eps^tu_#1

\newcommand\intersu[1]{\inter{\lts\to\ltu}{#1}}       % \eps^tu_#1
\newcommand\interus[1]{\inter{\ltu\gets\lts}{#1}}       % \eps^tu_#1

%\newcommand\interst[1]{\inter{\lts\to\ltt}{#1}}                 % \eps^tu_#1
%\newcommand\intersu[1]{\inter{\lts\to\ltu}{#1}}                 % \eps^tu_#1

\newcommand\domintertu[1]{\ldom{\intertu{#1}}}  %\Box\eps^tu_#1
\newcommand\codintertu[1]{\rdom{\intertu{#1}}}  %\eps^tu_#1\Box

\newcommand\sametuut[1]{\mbox{$\same{\ltt\leftrightarrow\ltu}{#1}$}}       % \eps^tu_#1
\newcommand\sametu[1]{\mbox{$\same{\ltt\to\ltu}{#1}$}}       % \eps^tu_#1
\newcommand\sameut[1]{\mbox{$\same{\ltt\gets\ltu}{#1}$}}       % \eps^tu_#1
\newcommand\samectu{\mbox{$\same{\ltt\to\ltu}{\cm}$}}       % \eps^tu_#1
\newcommand\samecut{\mbox{$\same{\ltt\gets\ltu}{\cm}$}}       % \eps^tu_#1
\newcommand\samedtu{\mbox{$\same{\ltt\to\ltu}{\dm}$}}       % \eps^tu_#1
\newcommand\samedut{\mbox{$\same{\ltt\gets\ltu}{\dm}$}}       % \eps^tu_#1

\newcommand\samett[1]{\same{\ltt\to\ltt}{#1}}                 % \eps^tu_#1

\newcommand\samest[1]{\same{\lts\to\ltt}{#1}}       % \eps^tu_#1
\newcommand\samets[1]{\same{\lts\gets\ltt}{#1}}       % \eps^tu_#1
\newcommand\samecst{\same{\lts\to\ltt}{\cm}}       % \eps^tu_#1
\newcommand\samects{\same{\lts\gets\ltt}{\cm}}       % \eps^tu_#1
\newcommand\samedst{\same{\lts\to\ltt}{\dm}}       % \eps^tu_#1
\newcommand\samedts{\same{\lts\gets\ltt}{\dm}}       % \eps^tu_#1



\newcommand\samesu[1]{\same{\lts\to\ltu}{#1}}       % \eps^tu_#1
\newcommand\sameus[1]{\same{\ltu\gets\lts}{#1}}       % \eps^tu_#1

%\newcommand\samest[1]{\same{\lts\to\ltt}{#1}}                 % \eps^tu_#1
%\newcommand\samesu[1]{\same{\lts\to\ltu}{#1}}                 % \eps^tu_#1

\newcommand\domsametu[1]{\ldom{\sametu{#1}}}  %\Box\eps^tu_#1
\newcommand\codsametu[1]{\rdom{\sametu{#1}}}  %\eps^tu_#1\Box


%  Apply:
\newcommand\interctt{\inter{\ltt\to\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\intercst{\inter{\lts\to\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\interctu{\inter{\ltt\to\ltu}{\cm}}                 % \eps^tu_#1
\newcommand\intercsu{\inter{\lts\to\ltu}{\cm}}                 % \eps^tu_#1

\newcommand\intercut{\inter{\ltt\leftarrow\ltu}{\cm}}                 % \eps^tu_#1

\newcommand\interprctt{\interpr{\ltt\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\interprcst{\interpr{\lts\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\interprctu{\interpr{\ltt\ltu}{\cm}}                 % \eps^tu_#1
\newcommand\interprcsu{\interpr{\lts\ltu}{\cm}}                 % \eps^tu_#1

\newcommand\dominterctu{\domintertu{\cm}}  %\Box\eps^tu_#1
\newcommand\codinterctu{\codintertu{\cm}}  %\eps^tu_#1\Box

%----------------------------------------------
%% Classes and arrows
%-------------------------------------------------

%\renewcommand\c{\mbox{$\AClass$}}                    %   C
\newcommand\cm{\AClass}                              %   C
\newcommand\ce{\mbox{$\semm{\AClass}$}}              % ||C||

%--- function:
\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}   % ||C||^#1

\newcommand\cindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
% apply:
%\newcommand\cet{\mbox{$\semm{C}^{\ltt}$}}                         % ||C||^t
%\newcommand\ceu{\mbox{$\semm{C}^{\ltu}$}}                         % ||C||^t
%\newcommand\cetu{\mbox{${}^{\ltt}\semm{\AClass}^{\ltu}$}}
\newcommand\ces{\ceind{\lts}}                         % ||C||^u
\newcommand\cev{\ceind{\tv}}                         % ||C||^u


\newcommand\ceJ{\ceind{\J}}

\newcommand\objeq[2]{\simeq^{#1}_{#2}}
\newcommand\eqJ[1]{\objeq{\J}{#1}}

\newcommand\ciet{\cindeind{i}{\ltt}}                         % ||C_i||^t
\newcommand\ctet{\cindeind{t}{\ltt}}                         % ||C_t||^t
\newcommand\cjet{\cindeind{j}{\ltt}}                         % ||C_i||^t
\newcommand\cket{\cindeind{k}{\ltt}}                         % ||C_t||^t
\newcommand\clet{\cindeind{l}{\ltt}}                         % ||C_i||^t


\newcommand\cieJ{\ceind{\J}}
%\newcommand\cjeJ{\ceind{\J}}

% function:
\newcommand\cind[1]{\mbox{$\AClass^{#1}$}}           %      C^#1
\newcommand\cindl[2]{\mbox{$_{#1}\AClass^{#2}$}}     % _{#1}C^{#2}
\newcommand\cindr[2]{\mbox{$\AClass_{#1}^{#2}$}}     %      C_{#1}^{#2}

%\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}           %      C^#1
\newcommand\ceindl[2]{\mbox{$_{#1}\semm{\AClass}^{#2}$}}     % _{#1}C^{#2}
\newcommand\ceindr[2]{\mbox{$\semm{\AClass}_{#1}^{#2}$}}     %      C_{#1}^{#2}

%  apply:
\newcommand\ctu{\mbox{$^{\ltt}\!\AClass^{\ltu}$}}
\newcommand\ctplusu{\cindr{+\ltu}{\ltt}}
\newcommand\ctnullu{\cindr{0\ltu}{\ltt}}
\newcommand\cuminust{\cindl{-\ltt}{\ltu}}
\newcommand\cunullt{\cindl{0\ltt}{\ltu}}

%\newcommand\cetu{\cind{\ltt\ltu}}
\newcommand\cetplusu{\ceindr{+\ltu}{\ltt}}
\newcommand\cetnullu{\ceindr{0\ltu}{\ltt}}
\newcommand\ceuminust{\ceindl{-\ltt}{\ltu}}
\newcommand\ceunullt{\ceindl{0\ltt}{\ltu}}

% the same for D

%\renewcommand\d{\mbox{$\TargetClass$}}                    %   D
\newcommand\dm{\TargetClass}                              %   D

\newcommand\de{\mbox{$\semm{\TargetClass}$}}              % ||D||
\newcommand\deind[1]{\mbox{$\semm{\TargetClass}^{#1}$}}   % ||D||^#1
\renewcommand\det{\deind{\ltt}}                         % ||C||^t
\newcommand\deu{\deind{\ltu}}                         % ||C||^u
\newcommand\des{\deind{\lts}}                         % ||C||^u
\newcommand\dev{\deind{\tv}}                         % ||C||^u

\newcommand\deJ{\deind{\J}}

\newcommand\dindeind[2]{\mbox{$\semm{\TargetClass_{#1}}^{#2}$}}
%  apply
\newcommand\dies{\dindeind{i}{\lts}}                         % ||C||^t
\newcommand\djet{\dindeind{j}{\ltt}}                         % ||C||^t
\newcommand\djeu{\dindeind{j}{\ltu}}                         % ||C||^t
%\newcommand\djetu{\dindeind{j}{\ltt}}                         % ||C||^t
\newcommand\dieJ{\deind{\J}}
\newcommand\djeJ{\deind{\J}}
\newcommand\diet{\dindeind{i}{\ltt}}                         % ||C||^t
\newcommand\dieu{\dindeind{i}{\ltu}}                         % ||C||^t
%\newcommand\djetu{\dindeind{j}{\ltt}}                         % ||C||^t


\newcommand\dind[1]{\mbox{$\TargetClass^{#1}$}}           %      C^#1
\newcommand\dindl[2]{\mbox{$_{#1}\TargetClass^{#2}$}}     % _{#1}D^{#2}
\newcommand\dindr[2]{\mbox{$\TargetClass_{#1}^{#2}$}}     %      D_{#1}^{#2}

%\newcommand\deind[1]{\mbox{$\semm{\TargetClass}^{#1}$}}           %      C^#1
\newcommand\deindl[2]{\mbox{$_{#1}\semm{\TargetClass}^{#2}$}}     % _{#1}D^{#2}
\newcommand\deindr[2]{\mbox{$\semm{\TargetClass}_{#1}^{#2}$}}     %      D_{#1}^{#2}


% apply
\newcommand\dtu{\mbox{$^{\ltt}\!\TargetClass^{\ltu}$}}
\newcommand\detplusu{\deindr{+\ltu}{\ltt}}
\newcommand\detnullu{\deindr{0\ltu}{\ltt}}
\newcommand\deuminust{\deindl{-\ltt}{\ltu}}
\newcommand\deunullt{\deindl{0\ltt}{\ltu}}


%\newcommand\f{\mbox{$\AReference$}}                    %   f
\newcommand\fm{\AReference}                              %   f
%\newcommand\find[1]{\mbox{$\AReference^{#1}$}}           %      f^#1
%\newcommand\findl[2]{\mbox{$_{#1}\AReference^{#2}$}}     % _{#1}C^{#2}
%\newcommand\findr[2]{\mbox{$\AReference_{#1}^{#2}$}}     %      C_{#1}^{#2}

\newcommand\feind[1]{\mbox{$\semm{\AReference}^{#1}$}}           %      f^#1
\newcommand\feindl[2]{\mbox{$_{#1}\semm{\AReference}^{#2}$}}     % _{#1}C^{#2}
\newcommand\feindr[2]{\mbox{$\semm{\AReference}_{#1}^{#2}$}}     %      C_{#1}^{#2}

\newcommand\ftu{\find{\ttu}}

\newcommand\fe{\mbox{$\semm{\AReference}$}}              % ||f||
\renewcommand\feind[1]{\mbox{$\semm{\AReference}^{#1}$}}   % ||f||^#1
\newcommand\fet{\feind{\ltt}}
\newcommand\fes{\feind{\lts}}
\newcommand\feu{\feind{\ltu}}
\newcommand\fev{\feind{\tv}}
\newcommand\feJ{\feind{\J}}

\newcommand\femt{\mbox{$\semm{\AReference^{-1}}^{\ltt}$}}


\newcommand\findeind[2]{\mbox{$\semm{\AReference_{#1}}^{#2}$}}
\newcommand\fieu[1]{\findeind{#1}{\ltu}}
\newcommand\fiet[1]{\findeind{#1}{\ltt}}
\newcommand\fies[1]{\findeind{#1}{\lts}}                         % ||C||^t
%\newcommand\fiet{\findeind{i}{\ltt}}                         % ||C||^t
\newcommand\fjet{\findeind{j}{\ltt}}                         % ||C||^t
\newcommand\fket{\findeind{k}{\ltt}}                         % ||C||^t
\newcommand\flet{\findeind{l}{\ltt}}                         % ||C||^t
\newcommand\fkeu{\findeind{k}{\ltu}}                         % ||C||^t

\newcommand\fetplusu{\feindr{+\ltu}{\ltt}}
\newcommand\fetnullu{\feindr{0\ltu}{\ltt}}
\newcommand\feuminust{\feindl{-\ltt}{\ltu}}
\newcommand\feunullt{\feindl{0\ltt}{\ltu}}



%\newcommand\diet{\dindeind{i}{\ltt}}                         % ||C||^t
%\newcommand\djes{\dindeind{j}{\lts}}                         % ||C||^t

\newcommand\fieJ{\feind{\J}}
\newcommand\fjeJ{\feind{\J}}

\newcommand\fgcomp{\mbox{$\f(\g_1,\ldots,\g_m)$}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% The old version where \tj denotes t, \tk denotes u  etc
%%% The new version see on line 185

\newcommand\tjk{\EarlierMoment\LaterMoment}   %jk
\newcommand\tj{\EarlierMoment}               %j
\newcommand\tk{\LaterMoment}                  %k
\newcommand\tjlk{\mbox{$\tj\le\kt$}}
\newcommand\ti{\EarlierEarlierMoment}        %i
\newcommand\tl{\LaterLaterMoment}             %l

%\newcommand\J{\AHistory}                      %J

\newcommand\interjk[1]{\inter{\tjk}{#1}}                 % \eps^jk_#1
\newcommand\dominterjk[1]{\ldom{\interjk{#1}}}  %\Box\eps^jk_#1
\newcommand\codinterjk[1]{\rdom{\interjk{#1}}}  %\eps^jk_#1\Box

\newcommand\interjj[1]{\inter{\tj\tj}{#1}}                 % \eps^jk_#1
\newcommand\interij[1]{\inter{\ti\tj}{#1}}                 % \eps^jk_#1
%\newcommand\interjk[1]{\inter{\tj\tk}{#1}}                 % \eps^jk_#1
\newcommand\interik[1]{\inter{\ti\tk}{#1}}                 % \eps^jk_#1


\newcommand\intercjj{\inter{\tj\tj}{\cm}}                 % \eps^jk_#1
\newcommand\intercij{\inter{\ti\tj}{\cm}}                 % \eps^jk_#1
\newcommand\intercjk{\inter{\tj\tk}{\cm}}                 % \eps^jk_#1
\newcommand\intercik{\inter{\ti\tk}{\cm}}                 % \eps^jk_#1

\newcommand\domintercjk{\dominterjk{\cm}}  %\Box\eps^jk_#1
\newcommand\codintercjk{\codinterjk{\cm}}  %\eps^jk_#1\Box

\newcommand\interdjj{\inter{\tj\tj}{\dm}}                 % \eps^jk_#1
\newcommand\interdij{\inter{\ti\tj}{\dm}}                 % \eps^jk_#1
\newcommand\interdjk{\inter{\tj\tk}{\dm}}                 % \eps^jk_#1
\newcommand\interdik{\inter{\ti\tk}{\dm}}                 % \eps^jk_#1

%----------------------------------------------
%% Classes and arrows
%-------------------------------------------------

%\renewcommand\c{\mbox{$\AClass$}}                    %   C
%\newcommand\cm{\AClass}                              %   C

%\newcommand\ce{\mbox{$\semm{\AClass}$}}              % ||C||
%\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}   % ||C||^#1
\newcommand\cej{\ceind{\tj}}                         % ||C||^j
\newcommand\cek{\ceind{\tk}}                         % ||C||^k
%\newcommand\ceJ{\ceind{\J}}
%--- function:
%\newcommand\cindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
% apply:
\newcommand\ciej{\cindeind{i}{\tj}}                         % ||C_i||^j
\newcommand\cjej{\cindeind{j}{\tj}}                         % ||C_j||^j
\renewcommand\cieJ{\ceind{\J}}
\newcommand\cjeJ{\ceind{\J}}

% function:
%\newcommand\cind[1]{\mbox{$\AClass^{#1}$}}           %      C^#1
%\newcommand\cindl[2]{\mbox{$_{#1}\AClass^{#2}$}}     % _{#1}C^{#2}
%\newcommand\cindr[2]{\mbox{$\AClass_{#1}^{#2}$}}     %      C_{#1}^{#2}
%  apply:
\newcommand\cjk{\cind{\tj\tk}}
\newcommand\cjplusk{\cindr{+\tk}{\tj}}
\newcommand\cjnullk{\cindr{0\tk}{\tj}}
\newcommand\ckminusj{\cindl{-\tj}{\tk}}
\newcommand\cknullj{\cindl{0\tj}{\tk}}


% the same for D

%\renewcommand\d{\mbox{$\TargetClass$}}                    %   D
%\renewcommand\dm{\TargetClass}                              %   D

%\newcommand\de{\mbox{$\semm{\TargetClass}$}}              % ||D||

%\newcommand\deind[1]{\mbox{$\semm{\TargetClass}^{#1}$}}   % ||D||^#1
%\newcommand\dindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}

%\newcommand\dind[1]{\mbox{$\TargetClass^{#1}$}}           %      C^#1
%\newcommand\dindl[2]{\mbox{$_{#1}\TargetClass^{#2}$}}     % _{#1}D^{#2}
%\newcommand\dindr[2]{\mbox{$\TargetClass_{#1}^{#2}$}}     %      D_{#1}^{#2}



%  Apply:
\newcommand\dej{\deind{\tj}}                         % ||C||^j
\newcommand\dek{\deind{\tk}}                         % ||C||^k
%\newcommand\deJ{\deind{\J}}

\newcommand\diei{\dindeind{i}{\ti}}                         % ||C||^j
\newcommand\djej{\dindeind{j}{\tj}}                         % ||C||^j
%\newcommand\dieJ{\deind{\J}}
%\newcommand\djeJ{\deind{\J}}

\newcommand\djk{\dind{\tj\tk}}
\newcommand\djplusk{\dindr{+\tk}{\tj}}
\newcommand\djnullk{\dindr{0\tk}{\tj}}
\newcommand\dkminusj{\dindl{-\tj}{\tk}}
\newcommand\dknullj{\dindl{0\tj}{\tk}}


%\renewcommand\f{\mbox{$\AReference$}}                    %   f
%\newcommand\fm{\AReference}                              %   f
%\newcommand\find[1]{\mbox{$\AReference^{#1}$}}           %      f^#1
\newcommand\fjk{\find{\tjk}}

%\newcommand\fe{\mbox{$\semm{\AReference}$}}              % ||f||
%\newcommand\feind[1]{\mbox{$\semm{\AReference}^{#1}$}}   % ||f||^#1
\newcommand\fej{\feind{\tj}}
\newcommand\fei{\feind{\ti}}
\newcommand\fek{\feind{\tk}}
\newcommand\fel{\feind{\tl}}

%\newcommand\feJ{\feind{\J}}

%\newcommand\findeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
%\newcommand\diei{\dindeind{i}{\ti}}                         % ||C||^j
%\newcommand\djej{\dindeind{j}{\tj}}                         % ||C||^j
 \newcommand\fiei{\findeind{i}{\ti}}                         % ||C||^j
 \newcommand\fjej{\findeind{j}{\tj}}                         % ||C||^j
%\newcommand\fieJ{\feind{\J}}
%\newcommand\fjeJ{\feind{\J}}

%\newcommand\fgcomp{\mbox{$\f(\g_1,\ldots,\g_m)$}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\Distinctctu{\mbox{$^{\ltt}\!\semm{\ittt{Distinct}_{\cm}}^{\ltu}$}}
\newcommand\Distinctcst{\mbox{$^{\lts}\!\semm{\ittt{Distinct}_{\cm}}^{\ltt}$}}
\newcommand\Samectu{\mbox{$^{\ltt}\!\semm{\ittt{Same}_{\cm}}^{\ltu}$}}
\newcommand\Samecst{\mbox{$^{\lts}\!\semm{\ittt{Same}_{\cm}}^{\ltt}$}}
%=============
%%%%% Behset
\newcommand\xstatei[3]{\mbox{${\mathit {#1}state}^{#3}_{#2}$}}
\newcommand\statei[2]{\xstatei{}{#1}{#2}}
\newcommand\xstate[2]{\xstatei{#1}{}{#2}}
%\newcommand\tstatei[1]{\statei{#1}{\ltt}}

\newcommand\attrName[1]{{\mathit #1}}
\newcommand\methName[1]{{\mathit #1}}
\newcommand\statepoint[1]{#1}

%%%%%
% discussing string-based  vs graph-based logics
\newcommand\cmlang{{\bf L}}
\newcommand\myindex[1]{\mbox{\scriptsize{#1}}}
\newcommand\mathsymbol[1]{\mbox{$#1$}}
%\newcommand\repr{\mathsymbol{r}}
\newcommand\world%{\ittt{world}}
{\mathsymbol{\cal W}}
\newcommand\cmter%{\ittt{computer}}
{\mathsymbol{\cal C}}
\newcommand\topos{\mathsymbol{\cal S}}


%----------------------
\newcommand\viewob[1]{\object{V}{#1}}
\newcommand\thob[1]{\object{T}{#1}}
\newcommand\uniob[1]{\object{U}{#1}}
\newcommand\uniobmath[1]{\objectmath{U}{#1}}
\newcommand\uniobind[1]{\objectind{U}{#1}}

\newcommand\UNI{\universe{U}}
\newcommand\UNIind{\universeind{U}}
\newcommand\UNImath{\universeind{U}} % the same
\newcommand\Setsind{\universeind{Sets}}

\newcommand\particularUni[1]{\mbox{$\mathbf{#1}$}}
\newcommand\particularUniInd[1]{\mathbf{#1}}
\newcommand\Sets{\particularUni{Sets}}
\newcommand\Varsets{\particularUni{VarSets}}
\newcommand\Behsets{\particularUni{BehSets}}
\newcommand\Sketches{\particularUni{Sketches}}


\newcommand\skeproc{\proc{ske}}
\newcommand\arrdlproc{\procind{Formal}{ArrDL}}
\newcommand\elmslproc{\procind{Formal}{ElmSL}}

%\newcommand\formalPar[1]{\mbox{$\mathrm #1$}}
\newcommand\formalParBold[1]{\mbox{$#1$}}
\newcommand\lf{\formalParBold{L}}
\newcommand\mf{\formalPar{M(D)}}
\newcommand\uf{\formalPar{U}}
\newcommand\df{\formalPar{D}}
\newcommand\tdf{\mbox{$\thob(\diag)$}}
\newcommand\sdf{\mbox{$\skeob{}(\diag)$}}

\newcommand\str{\formalPar{\sigma}}
%(7)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Created on May 4,2001
%============================================
% Part 1: pure italic writing of names
%        formerly file italic.tex
%--------------------------------------------
% Part 2: commands for semantics extensions of classes
%         like [[Person]]^t or {^t}[[SamePerson]]^{u}
%        formerly file employ.tex
%===========================================

\newcommand\operarrow[2]{\mbox{{\sffamily%\itshape
                                         #1}$_{#2}$}}
\newcommand\projop[1]{\operarrow{p}{#1}}
%\newcommand\concatop{\operarrow{concat}{}}
%\newcommand\pairop{\operarrow{pair}{}}
%\newcommand\idop[1]{\operarrow{id}{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\newcommand\ltt{\mbox{$t$}}
%\newcommand\ltu{\mbox{$u$}}
%\newcommand\lts{\mbox{$s$}}

%

\newcommand\Emplsem[1]{\mbox{$\semm{\Empl}^{#1}$}}
\newcommand\Emplt{\Emplsem{\ltt}}
\newcommand\Emplu{\Emplsem{\ltu}}
\newcommand\Empls{\Emplsem{\lts}}
\newcommand\Empltu{\mbox{$^{\ltt}\!\semm{\Empl}^{\ltu}$}}
\newcommand\Emplst{\mbox{$^{\lts}\!\semm{\Empl}^{\ltt}$}}
\newcommand\SameEmpltu{\mbox{$^{\ltt}\!\semm{\SameEmpl}^{\ltu}$}}
\newcommand\SameEmplst{\mbox{$^{\lts}\!\semm{\SameEmpl}^{\ltt}$}}

\newcommand\Compsem[1]{\mbox{$\semm{\Comp}^{#1}$}}
\newcommand\Compt{\Compsem{\ltt}}
\newcommand\Compu{\Compsem{\ltu}}
\newcommand\Comps{\Compsem{\lts}}
\newcommand\Comptu{\mbox{$^{\ltt}\!\semm{\Comp}^{\ltu}$}}
\newcommand\Compst{\mbox{$^{\lts}\!\semm{\Comp}^{\ltt}$}}
\newcommand\SameComptu{\mbox{$^{\ltt}\!\semm{\SameComp}^{\ltu}$}}
\newcommand\SameCompst{\mbox{$^{\lts}\!\semm{\SameComp}^{\ltt}$}}

\newcommand\Engrsem[1]{\mbox{$\semm{\Engr}^{#1}$}}
\newcommand\Engrt{\Engrsem{\ltt}}
\newcommand\Engru{\Engrsem{\ltu}}
\newcommand\Engrs{\Engrsem{\lts}}
\newcommand\Engrtu{\mbox{$^{\ltt}\!\semm{\Engr}^{\ltu}$}}
\newcommand\Engrst{\mbox{$^{\lts}\!\semm{\Engr}^{\ltt}$}}

\newcommand\Mngrsem[1]{\mbox{$\semm{\Mngr}^{#1}$}}
\newcommand\Mngrt{\Mngrsem{\ltt}}
\newcommand\Mngru{\Mngrsem{\ltu}}
\newcommand\Mngrs{\Mngrsem{\lts}}
\newcommand\Mngrtu{\mbox{$^{\ltt}\!\semm{\Mngr}^{\ltu}$}}
\newcommand\Mngrst{\mbox{$^{\lts}\!\semm{\Mngr}^{\ltt}$}}

\newcommand\John[1]{\mbox{$\ittt{John}^{#1}$}}

\newcommand\Marr{\ittt{Married}}
\newcommand\Marrsem[1]{\mbox{$\semm{\Marr}^{#1}$}}
\newcommand\Marrt{\Marrsem{\ltt}}
\newcommand\Marru{\Marrsem{\ltu}}
\newcommand\Marrs{\Marrsem{\lts}}
\newcommand\Marrtu{\mbox{$^{\ltt}\!\semm{\Marr}^{\ltu}$}}
\newcommand\Marrst{\mbox{$^{\lts}\!\semm{\Marr}^{\ltt}$}}

\newcommand\Famy{\ittt{Family}}
\newcommand\Famysem[1]{\mbox{$\semm{\Famy}^{#1}$}}
\newcommand\Famyt{\Famysem{\ltt}}
\newcommand\Famyu{\Famysem{\ltu}}
\newcommand\Famys{\Famysem{\lts}}
\newcommand\Famytu{\mbox{$^{\ltt}\!\semm{\Famy}^{\ltu}$}}
\newcommand\Famyst{\mbox{$^{\lts}\!\semm{\Famy}^{\ltt}$}}
\newcommand\Famytt{\mbox{$^{\ltt}\!\semm{\Famy}^{\ltt}$}}
\newcommand\Familytu{\mbox{$^{\ltt}\!\semm{\Famy}^{\ltu}$}}
\newcommand\Familyst{\mbox{$^{\lts}\!\semm{\Famy}^{\ltt}$}}

\newcommand\Friendship{\ittt{Friendship}}
\newcommand\Friship{\ittt{Friendship}}
\newcommand\Frishiptu{\mbox{$^{\ltt}\!\semm{\Friship}^{\ltu}$}}
\newcommand\Frishipst{\mbox{$^{\lts}\!\semm{\Friship}^{\ltt}$}}


\newcommand\Matr{\ittt{Matrimony}}
\newcommand\Matrsem[1]{\mbox{$\semm{\Matr}^{#1}$}}
\newcommand\Matrt{\Matrsem{\ltt}}
\newcommand\Matru{\Matrsem{\ltu}}
\newcommand\Matrs{\Matrsem{\lts}}
\newcommand\Matrtu{\mbox{$^{\ltt}\!\semm{\Matr}^{\ltu}$}}
\newcommand\Matrst{\mbox{$^{\lts}\!\semm{\Matr}^{\ltt}$}}

\newcommand\Distincttu{\mbox{$^{\ltt}\!\semm{\ittt{Distinct}}^{\ltu}$}}
\newcommand\Distinctst{\mbox{$^{\lts}\!\semm{\ittt{Distinct}}^{\ltt}$}}
\newcommand\Sametu{\mbox{$^{\ltt}\!\semm{\ittt{Same}}^{\ltu}$}}
\newcommand\Samest{\mbox{$^{\lts}\!\semm{\ittt{Same}}^{\ltt}$}}

\newcommand\Wom{\ittt{Woman}}
\newcommand\Womsem[1]{\mbox{$\semm{\Wom}^{#1}$}}
\newcommand\Womt{\Womsem{\ltt}}
\newcommand\Womu{\Womsem{\ltu}}
\newcommand\Woms{\Womsem{\lts}}
\newcommand\Womtu{\mbox{$^{\ltt}\!\semm{\Wom}^{\ltu}$}}
\newcommand\Womst{\mbox{$^{\lts}\!\semm{\Wom}^{\ltt}$}}

%\newcommand\Man{\ittt{Man}}
\newcommand\Mansem[1]{\mbox{$\semm{\Man}^{#1}$}}
\newcommand\Mant{\Mansem{\ltt}}
\newcommand\Manu{\Mansem{\ltu}}
\newcommand\Mans{\Mansem{\lts}}
\newcommand\Mantu{\mbox{$^{\ltt}\!\semm{\Man}^{\ltu}$}}
\newcommand\Manst{\mbox{$^{\lts}\!\semm{\Man}^{\ltt}$}}

\newcommand\Husbsem[1]{\mbox{$\semm{\Husb}^{#1}$}}
\newcommand\Husbt{\Husbsem{\ltt}}
\newcommand\Husbu{\Husbsem{\ltu}}
\newcommand\Husbs{\Husbsem{\lts}}
\newcommand\Husbtu{\mbox{$^{\ltt}\!\semm{\Husb}^{\ltu}$}}
\newcommand\Husbst{\mbox{$^{\lts}\!\semm{\Husb}^{\ltt}$}}


\newcommand\mysemm[2]{\mbox{$\semm{#1}^{#2}$}}

\newcommand\isarrt{\mysemm{\isa}{\ltt}}
\newcommand\isarru{\mysemm{\isa}{\ltu}}

\newcommand\wifet{\mysemm{\wife}{\ltt}}
\newcommand\wifeu{\mysemm{\wife}{\ltu}}

\newcommand\husbt{\mysemm{\husb}{\ltt}}
\newcommand\husbu{\mysemm{\husb}{\ltu}}

\newcommand\mdatet{\mysemm{\mDate}{\ltt}}
\newcommand\mdateu{\mysemm{\mDate}{\ltu}}

\newcommand\liveset{\mysemm{\livesAt}{\ltt}}
\newcommand\liveseu{\mysemm{\livesAt}{\ltu}}

\newcommand\income{\ittt{income}}
\newcommand\WMHsem[2]{\mbox{$
      (\semm{\Wom}^{#1}\times\semm{\Man}^{#1}\times\semm{\House}^{#1})
\times
      (\semm{\Wom}^{#2}\times\semm{\Man}^{#2}\times\semm{\House}^{#2})
                            $}
                     }
\newcommand\WMHtu{\WMHsem{\ltt}{\ltu}}


\newcommand\WMWMsem[2]{\mbox{$(\semm{\Wom}^{#1}\times\semm{\Man}^{#1})
                        \times(\semm{\Wom}^{#2}\times\semm{\Man}^{#2})
                             $}
                        }
\newcommand\WMWMtu{\WMWMsem{\ltt}{\ltu}}


\newcommand\myview[1]{\mbox{$V_{#1}$}}
\newcommand\IndI{1}
\newcommand\SWAggr{2}
\newcommand\AggrI{3}
\newcommand\TWAggrG{4}
\newcommand\IndII{5}
\newcommand\TWAggrS{6}
\newcommand\LAggr{7}
\newcommand\LLAggr{8}
\newcommand\SWLAggr{9}
\newcommand\STWAggr{10}
\newcommand\DelAggr{11}
\newcommand\TotAggr{12}
\newcommand\WQual{13}
 \newcommand\LQual{14}
\newcommand\AttrI{15}
\newcommand\SWLQual{16}
\newcommand\STWQual{17}
\newcommand\AttrII{18}



%(8)
%\newcommand\s{\mbox{$S$}}
%\newcommand\os{\mbox{$\overline{S}$}}
%\newcommand\ovr[1]{\mbox{$\overline{#1}$}}
\newcommand\into[1]{\stackrel{#1}{\hookrightarrow}}
\newcommand\repgra{\nicex{ R$}}
\newcommand\rgra{\repgra}
\newcommand\nds[1]{\mbox{$\mathit{Nds}#1$}}
\newcommand\arrs[1]{\mbox{$\mathit{Arrs}#1$}}
\newcommand\ndsr{\nds{\rgra}}
\newcommand\arrsr{\arrs{\rgra}}

\newcommand\dersetmath{\mathit{Der}}
\newcommand\derset{\mbox{$\dersetmath$}}
\newcommand\derop{\mbox{$\mathbf{der}$}}
\newcommand\algebra[1]{\mbox{$\alpha^{#1}$}}
\newcommand\algu{\algebra{\uskemath}}

%\newcommand\inss[1]{\lar{I}{\ske{#1}}{\uske}}
%\newcommand\ovri{\mbox{$\overline{I}$}}
%\newcommand\ovrinss[1]{\lar{\ovri_{#1}}{\ovrs{#1}}{\uske}}

\newcommand\ovrske[1]{\mbox{$\overline{\ske{#1}}$}}
\newcommand\ovrs[1]{\mbox{$\overline{\ske{#1}}$}}
%-----------------------------
\newcommand\sv{\mbox{$\ske{V}$}}
\newcommand\sr{\mbox{$\ske{R}$}}
\newcommand\vmor{\lar{v}{\sv}{\ovrske{}}}
\newcommand\rmor{\lar{r}{S}{\ovrske{R}}}
\newcommand\emor{\lar{e}{S}{\U}}
\newcommand\vpair{\mbox{$V=(\sv,v)$}}
\newcommand\rpair{\mbox{$R=(\sr,r)$}}



%\newcommand\dbinst{\lar{e}{S}{W} }

%---------------------------------------------------


\newcommand\ovrsig[1]{\mbox{$\overline{\sigma _{#1}}$}}
\newcommand\ovrg[1]{\mbox{$\overline{G_{#1}}$}}
%-----------------------------------------
\newcommand\ovrp{\mbox{$\overline{\pi }$}}%{#1}}$}}
\newcommand\ovreps{\mbox{$\overline{\vare}$}}     % overlined epsilon


%\renewcommand\endinput{}
%\newcommand\comp{\mathbin{\triangleright\!\!\triangleright}}
\newcommand\state[2]{\mbox{${\mathit{state}}^{#1}_{#2}$}}
\newcommand\starInherit{*-inherit}

\newcommand\sig{\mbox{$\Sigma $}}
\newcommand\sigm{\Sigma}
\newcommand\defitemotstup[1]{\par\smallskip\noindent (#1)}


\newcommand\arity[1]{\mbox{$\mathit{Arity}(#1)$}}
\newcommand\predsem[2]{\mbox{$\semm{#1}^{#2} $}}
\newcommand\psem[1]{\predsem{P}{#1}}
\newcommand\psemu{\psem{\ucatmath}}
\newcommand\lsig{\mbox{$\Lambda $}}

%%%
\newcommand\Attr{\mbox{$\mathit{Attr}$}}
\newcommand\Var{\mbox{$\mathit{Var}$}}
\newcommand\relcat{\mbox{$\categoryname{Rel}$}}
\newcommand\relske{\mbox{$\sketchname{Rel}$}}
\newcommand\itte[1]{\mbox{\textit{#1}}}
\newcommand\dbcat{\mbox{$\categoryname{DB}$}}

\newcommand\skecat[1]{\mbox{$\categoryname{Sketch}(\sig_{#1})$}}
\newcommand\sigcat{\mbox{$\categoryname{Sign}$}}

\newcommand\funor{\mbox{$\Phi$}}
\newcommand\funarr{\lar{f}{X}{Y}}
\newcommand\currfun{\mbox{\lar{\Map{A}{\_}}{\catset}{\catset}}}
\newcommand\curra{\Map{A}{\_}}

% \newcommand\ {\itte{ }}
\newcommand\target{\itte{target}}
\newcommand\source{\itte{source}}
\newcommand\conof{\itte{consistsOf}}
\newcommand\marker{\itte{marker}}
\newcommand\Node{\itte{Node}}
\newcommand\nodeit{\ittt{node}}
\newcommand\Arrow{\itte{Arrow}}
\newcommand\arrow{\ittt{arrow}}
\newcommand\diagramit{\itte{diagram}}
\newcommand\graphit{\itte{graph}}
\newcommand\shape{\itte{shape}}
\newcommand\predecl{\itte{predicate\_declarations}}
\newcommand\statements{\itte{statements}}
\newcommand\carrier{\itte{carrier}}
\newcommand\arityshape{\itte{arity\_shape}}


% semiotics
%% MACROS OF Dec 3
\newcommand\formalObj[1]{\mbox{\sffamily #1}}
\newcommand\formalOper[1]{\mbox{{\bfseries\sffamily #1}}}
\newcommand\informalObj[1]{\mbox{\textit #1}}
\newcommand\informalOper[1]{\mbox{{\bfseries\itshape #1}}}

\newcommand\lzzl{\formalObj{l}}  %logic
\newcommand\ml{\informalObj{ML}}  % modeling language

\newcommand\f{\formalObj{F}}
\renewcommand\c{\informalObj{C}}
\newcommand\derf{\formalOper{Der}}
\newcommand\deri{\informalOper{Un}}
\newcommand\derff{\derf.\f}
\newcommand\deric{\deri(\c)}
\newcommand\FormalInterpret[1]{\mbox{$\formalObj{i}_f$}}
\newcommand\SubstantInterpret[1]{\mbox{$\informalObj{i}_s$}}


%====================================

\newcommand\informalPar[1]{\nicex{{#1}$}}
\newcommand\infParind[1]{\cal #1}
\newcommand\formalPar[1]{\mbox{$\mathrm{#1}$}}
\newcommand\frmParind[1]{\mathrm{#1}}

\newcommand\informalParBold[1]{\mbox{${\cal #1}$}}
%\newcommand\formalPar[1]{\mbox{$\mathrm #1$}}

\newcommand\object[2]{\mbox{${\mathsf{#1}}_{#2}$}}
%\newcommand\object[2]{\mbox{$#1_{#2}$}}
\newcommand\universe[1]{\mbox{$\mathbf{#1}$}}
%\newcommand\objectind[1]{\mathsf{#1}}
\newcommand\objectind[1]{\mathsf{#1}}
\newcommand\objectmath[1]{\mathsf{#1}} % the same
\newcommand\universeind[1]{\mathbf{#1}}
\newcommand\umath[1]{\mathbf{U}_{#1}}

\newcommand\proc[1]{\mbox{\sffamily\bfseries #1}}
\newcommand\procind[2]{\mbox{${\mathrm{#1}}_{\mathrm #2}$}}
\newcommand\linf{\informalParBold{L}}
\newcommand\minf{\mbox{$\informalPar{M}(\diag{})$}}
\newcommand\mdinf{\mbox{$\informalPar{M}(\diag{})$}} % the same as above
\newcommand\mdfrm{\mbox{$\formalPar{M}(\diag{})$}} % the same as above
\newcommand\uinf{\informalPar{U}}

\newcommand\meaninf{\informalPar{M}}
\newcommand\meanfrm[1]{\mbox{$\formalPar{M}_{#1}$}}

\newcommand\diags{\mbox{$\mathit{Diags}$}}
\newcommand\graph{\mbox{$\mathit{Graph}$}}

\newcommand\diaob[1]{\object{D}{#1}} %\mbox{$D$}}
\newcommand\diagob[1]{\object{D}{#1}} %the same \mbox{$D$}}
\newcommand\diag[1]{\object{D}{#1}} %the same \mbox{$D$}}
\newcommand\diaind{\objectind{D}}

\newcommand\graob[1]{\object{G}{#1}}
\newcommand\graind{\objectind{G}}
\newcommand\gra[1]{\graob{#1}}

\newcommand\skeob[1]{\object{S}{#1}}
\newcommand\skeind{\objectind{S}}

\newcommand\modelob[1]{\object{M}{#1}}
\newcommand\modelind{\objectind{M}}

\newcommand\sigob[1]{\object{\mbox{$\Sigma$}}{#1}}
\newcommand\skediag{\skeob{}[\diag{}]}

\newcommand\meaninfdiag{\meaninf[\diag{}]}
\newcommand\meanfrmdiag{\meanfrm[\diag{}]}
% synonyms
\newcommand\meanifdiag{\meaninf[\diag{}]}
\newcommand\meanfdiag{\meanfrm[\diag{}]}

%%% diags, sketchs, specs, and their semantic interpretaions
\newcommand\objectWithInd[3]{\mbox{$\mathsf{#1}_{#2}^{#3}$}}
\newcommand\sketch[1]{\objectWithInd{S}{#1}{}}
\renewcommand\ske[1]{\sketch{#1}}
%\newcommand\graph[1]{\objectWithInd{S}{#1}{}}
\renewcommand\diag[1]{\objectWithInd{D}{#1}{}}
%\newcommand\inst[2]{\mbox{$\mathit{Inst}^{#2}{(#1)}$}}
%\newcommand\instob[2]{\mbox{$\mathit{Inst}^{#2}{(#1)}$}}


%\newcommand\diaob[1]{\mbox{$\diag{#1}$}}
%\newcommand\skeob{\mbox{$S$}}
\newcommand\graofske{\mbox{$G_\skeind$}}
\newcommand\graske{\graofske}
\newcommand\diaofske{\mbox{$D_\skeind$}}
\newcommand\diaske{\diaofske}


\renewcommand\eg{e.g.}
\renewcommand\C{\mbox{$C$}}

\newcommand\ext[1]{\mbox{$\mathit{Ext}(#1)$}}
\renewcommand\stt[1]{\mbox{$\mathit{Stt}(#1)$}}
\newcommand\GCS{{\bf (GCS)}}
\newcommand\AET{{\bf (AET)}}



%\newcommand\tuple[1]{\left [ \mathstrut {#1} \right ]}
\newcommand\pmrk[1]{\mbox{[{\sf #1}]}}
\newcommand\omrk[1]{\mbox{[{\sf #1} $\rangle $}}

% used in Intro
\newcommand\lanfrm{\formalPar{FL}}
\newcommand\flan{\formalPar{FL}} %the same
\newcommand\flanind{\frmParind{FL}}

\newcommand\x{\diag{}}   %\mbox{$D$}}
\renewcommand\s{\skeob{}}%\mbox{$S$}}
%\newcommand\mix{\mbox{$\meaninf$}} %(\x)
%\newcommand\mfx{\mbox{$\meanfrm{\flanind}$}} %(\x)
\newcommand\mix{\mbox{$\meaninf(\x)$}}
\newcommand\mfx{\mbox{$\meanfrm{}(\x)$}}

%\newcommand\flan{\mbox{$\meanfrm(\x)$}}

\newcommand\spex[1]{\mbox{$\skeob{#1}$}} %(\mix)$}}
\newcommand\spem[1]{\mbox{$\skeob{#1}$}} %(\mix)$}}
\newcommand\spexl  {\mbox{$\skeob{\flanind}$}} %(\x)$}}
\newcommand\speml  {\mbox{$\skeob{}$}} %(\mfx)$}}

\newcommand\dateit{\ittt{date}}

% used in dGetStartViaAss
\newcommand\nis{\nicex{ S$}}
\newcommand\niv{\nicex{ V$}}
\newcommand\nivind{{V}}
\newcommand\nisind{{S}}

\newcommand\mrkdual[3]{\mbox{${#2}\stackrel{{\cal\scriptsize #1}}{[><]}{#3}$}} %{[>^{\mathrm{#1}}<]}$}}
\newcommand\sgv{single-valued}
\newcommand\assgenpred{\mbox{$[\Uparrow]$}}
\newcommand\SepPred{\mrk{1-1}  }
\newcommand\CovPred{\mrk{cover}}
\newcommand\MemPred{\mrk{$\in$}}

\newcommand\binAss{1}
\newcommand\assCla{2}
\newcommand\reiAss{3}
\newcommand\terAss{4}
\newcommand\quaAss{5}
\newcommand\skeo{\skeob{\binAss}}
\newcommand\skei{\skeob{\assCla}}
\newcommand\skeii{\skeob{\reiAss}}
\newcommand\skeiii{\skeob{\terAss}}
\newcommand\skeiv{\skeob{\quaAss}}
%\newcommand\diaob[1]{\diag{#1}}
\newcommand\diao{\diaob{\binAss}}
\newcommand\diai{\diaob{\assCla}}
\newcommand\diaii{\diaob{\reiAss}}
\newcommand\diaiii{\diaob{\terAss}}
\newcommand\diaiv{\diaob{\quaAss}}


\newcommand\visfunctor{\mbox{{\sffamily\bfseries vis}}}
\newcommand\skefunctor{\mbox{{\sffamily\bfseries ske}}}

%used in eAssonBySke
\newcommand\sale{\ittt{sale}}
\newcommand\Show{\ittt{Show}}
\renewcommand\show{\ittt{show}}
\newcommand\seat{\ittt{seat}}
\newcommand\perf{\ittt{perf}}
\newcommand\Performance{\ittt{Performance}}
\newcommand\Ticket{\ittt{Ticket}}
\newcommand\ticket{\ittt{sale}}
\newcommand\Integer{\ittt{Integer}}

\newcommand\mastr[1]{\mbox{$\mathbf{#1}$}}
\newcommand\extofcla[1]{\mastr{\semm{\mathit #1}}}
\newcommand\behofcla[1]{\mastr{\besemm{\mathit{#1}}}}
\newcommand\sttofcla[1]{\lar{\statemap{}{\mathit{#1}}}{\extofcla{#1}}{\behofcla{#1}}}

%\newcommand\tlu{\mbox{$t<u$}}
%\newenvironment\mathitext%
%{
%\begin{displaymath}
%\mbox{ }
%\end{displaymath}
%} {}
\newcommand\cEngine{\ittt{carEngine}}
\newcommand\carEngine{\ittt{carEngine}}


\newcommand\mrkmon[2]{\mbox{\mrk{1-1}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkfro[2]{\mbox{\mrk{fro}$^{#1}_{\mathit{#2}}$}}
\renewcommand\mrkid[2]{\mbox{\mrk{id}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkstrongid[2]{\mbox{\mrk{id!}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkdel[2]{\mbox{\mrk{del}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkins[2]{\mbox{\mrk{ins}$^{#1}_{\mathit{#2}}$}}

\newcommand\mathand{\mbox{ and }}
\newcommand\mathor{\mbox{ or }}
\newcommand\mathif{\mbox{ if }}
\newcommand\maththen{\mbox{ then }}
\newcommand\mathiff{\mbox{ iff }}
%\newcommand\ofit{\ittt{of}}
\newcommand\wholeit{\ittt{whole}}
\newcommand\Wholeit{\ittt{Whole}}
\newcommand\partit{\ittt{part}}
\newcommand\stateit{\ittt{state}}
\newcommand\prokol{{\mathbf +}\!\!\!\!\circ}

\newcommand\mixsemm[1]{\mbox{$\lbesemm\, {\mathit #1} \, \rsemm$}}

\newcommand\logrule[2]{\frac{\mathstrut #1}{\mathstrut #2}}
\newcommand\logruleFig[2]{\frac{\mathstrut #1}{\mathstrut #2}}
\newcommand\logruleRow[2]{\mbox{if $#1$ then $#2$}}
\newcommand\logruleFigText[2]{\mbox{$
\frac{\mbox{\rule[-1ex]{0pt}{3ex} #1}}{\mbox{\rule{0pt}{3ex} #2}} $}
}
\newcommand\logruleRowText[2]{\mbox{if #1 then #2}}


\newcommand\ClassIndInd[3]{\mbox{$^{#1}\!\semm{\mathit{#2}}^{#3}$}}
\newcommand\ClassBeh[1]{\mbox{$\besemm{\mathit{#1}}$}}

\newcommand\refInd[2]{\mbox{$\semm{\mathit{#1}}^{\mathit{#2}}$}}
\newcommand\refBehInd[2]{\mbox{$\besemm{\mathit{#1}}^{\mathit{#2}}$}}
\newcommand\refIndBeh[2]{\mbox{$\besemm{\mathit{#1}}^{\mathit{#2}}$}}




\renewcommand\same[2]{\mbox{${\mathit{same}}^{#1}_{\mathit{#2}}$}}
\newcommand\samemap[2]{\mbox{${\mathit{same}}^{#1}_{\mathit{#2}}$}}
%\newcommand\sametu[1]{\samemap{tu}{#1}}
\newcommand\delset[3]{\mbox{$\semm{#3}^{#1}\mathsf{Del}^{#1\rightarrow #2}$}}
\newcommand\deltu[1]{\delset{t}{u}{#1}}
\newcommand\newset[3]{\mbox{$\semm{#3}^{#1}\mathsf{New}^{#2\rightarrow #1}$}}
\newcommand\newut[1]{\newset{u}{t}{#1}}
\newcommand\newts[1]{\newset{t}{s}{#1}}
%\newcommand\insut[1]{\newset{t}{u}{#1}}
%\newcommand\newut[1]{\newset{t\leftarrow u}{#1}} %  correct
%\newcommand\newtu[1]{\newset{t\leftarrow u}{#1}} % incorrect, to match old
%\newcommand\newts[1]{\newset{s\leftarrow t}{#1}} %correct,
%\newcommand\newst[1]{\newset{s\leftarrow t}{#1}} %incorrect, to match old
\newcommand\statemap[2]{\mbox{${\mathit{state}}^{#1}_{\mathit{#2}}$}}



\newcommand\ofit{\ittt{of}}
\newcommand\ofmap[1]{\refInd{of}{#1}}
%\newcommand\ofit{\ofmap{}}
\newcommand\oft{\ofmap{t}}
\newcommand\ofu{\ofmap{u}}

\newcommand\ofindit{\mbox{$\semm{{\mathit of}_i}^{t}$}}
%\newcommand\ofindiu{\mbox{$\semm{{\mathit of}_i}^{u}$}}
\newcommand\ofiu{\mbox{$\semm{{\mathit of}_i}^{u}$}}
%
\newcommand\isit{\ittt{is}}
\newcommand\ismap[1]{\refInd{is}{#1}}
%\newcommand\isit{\ismap{}}
\newcommand\ist{\ismap{t}}
\newcommand\isu{\ismap{u}}


\newcommand\isindt{\mbox{$\semm{{\mathit is}_i}^{t}$}}
\newcommand\isindu{\mbox{$\semm{{\mathit is}_i}^{u}$}}
%

\newcommand\hasit{\ittt{has}}
\newcommand\hasmapbeh{\besemm{has}}
\newcommand\hasbeh{\besemm{has}}
\newcommand\hasbehind[1]{\besemm{has}_{#1}}


\newcommand\supmap[1]{\refInd{sup}{#1}}
\newcommand\supit{\supmap{}}
\newcommand\supt{\supmap{t}}
\newcommand\supu{\supmap{u}}
%
\newcommand\supbeh{\besemm{sup}}
%
\newcommand\submap[1]{\refInd{sub}{#1}}
\newcommand\subit{\submap{}}
\newcommand\subt{\submap{t}}
\newcommand\subu{\submap{u}}

\newcommand\isamap[1]{\refInd{isA}{#1}}
\newcommand\isait{\isamap{}}
\newcommand\isat{\isamap{t}}
\newcommand\isau{\isamap{u}}
\newcommand\isabeh{\besemm{\isa}}

\newcommand\Persontu{\ClassIndInd{t}{Person}{u}}
\newcommand\Persont{\ClassIndInd{}{Person}{t}}
\newcommand\Personu{\ClassIndInd{}{Person}{u}}
\newcommand\PersonBeh{\ClassBeh{Person}}

\newcommand\Drivertu{\ClassIndInd{t}{Driver}{u}}
\newcommand\Drivert{\ClassIndInd{}{Driver}{t}}
\newcommand\Driveru{\ClassIndInd{}{Driver}{u}}



\newcommand\Cart{\ClassIndInd{}{Car}{t}}
\newcommand\Caru{\ClassIndInd{}{Car}{u}}
\newcommand\Cartu{\ClassIndInd{t}{Car}{u}}
\newcommand\SameCartu{\ClassIndInd{t}{SameCar}{u}}
\newcommand\CarBeh{\ClassBeh{Car}}
\newcommand\Carbeh{\ClassBeh{Car}}
\newcommand\Ownershiptu{\ClassIndInd{t}{Ownership}{u}}
\newcommand\Ownershipt{\ClassIndInd{}{Ownership}{t}}
\newcommand\Ownershipu{\ClassIndInd{}{Ownership}{u}}



\newcommand\Ownership{\ittt{Ownership}}
\newcommand\owner{\ittt{owner}}
%\newcommand\car{\ittt{car}}
%\newcommand\property{\ittt{property}}

%\newcommand\Engine{\ittt{Engine}}
%\newcommand\Eng{\ittt{Eng}}
\newcommand\Enginetu{\ClassIndInd{t}{Engine}{u}}
\newcommand\Enginet{\ClassIndInd{}{Engine}{t}}
\newcommand\Engineu{\ClassIndInd{}{Engine}{u}}
\newcommand\EngineBeh{\ClassBeh{Engine}}
\newcommand\Enginebeh{\ClassBeh{Engine}}
\newcommand\Engbeh{\ClassBeh{Engine}}
\newcommand\BodyBeh{\ClassBeh{Body}}
\newcommand\ChassisBeh{\ClassBeh{Chassis}}


%\newcommand\Engine{\ittt{Engine}}
%\newcommand\Eng{\ittt{Eng}}
%\newcommand\Body{\ittt{Body}}
%\newcommand\BodyBeh{\ClassBeh{Body}}
%\newcommand\Chassis{\ittt{Chassis}}
%\newcommand\ChassisBeh{\ClassBeh{Chassis}}
%%\newcommand\PartName{Part}

%\newcommand\drives{\ittt{drives}}
\newcommand\drivest{\refInd{drives}{t}}
\newcommand\drivesu{\refInd{drives}{u}}
\newcommand\drivesbeht{\refBehInd{drives}{t}}
\newcommand\drivesbehu{\refBehInd{drives}{u}}
\newcommand\drivesbehv{\refBehInd{drives}{v}}
\newcommand\drivesbeh{\refBehInd{drives}{}}

\newcommand\fuelat{\refInd{fuelAmount}{t}}
%\newcommand\fuelAm{\ittt{fuelAmount}}
%\newcommand\tankVo{\ittt{tankVolume}}
%\newcommand\fillTa{\ittt{fillTank}}
%\newcommand\car{\ittt{car}}

\newcommand\tankvt{\refInd{tankVolume}{t}}
\newcommand\tankvu{\refInd{tankVolume}{u}}

\newcommand\cart{\refInd{car}{t}}
\newcommand\caru{\refInd{car}{u}}

\newcommand\prst{\refInd{prs}{t}}
\newcommand\prsu{\refInd{prs}{u}}

\newcommand\enginet{\refInd{engine}{t}}
\newcommand\engineu{\refInd{engine}{u}}

\newcommand\persont{\refInd{person}{t}}
\newcommand\personu{\refInd{person}{u}}



\newcommand\PersonP{\Person$^+$}
\newcommand\PersonM{\Person$^-$}
\newcommand\CarP{\Car$^+$}
\newcommand\CarM{\Car$^-$}


\newcommand\floatRange[1]{\mrk{Float(#1)}}

%\newcommand\Car{\ittt{Car}}


\newcommand\becar{\besemm{\Car}}
\newcommand\beCar{\besemm{\Car}}
\newcommand\lt{$t$}
\newcommand\tstate{\statei{}{\ltt}}
\newcommand\stts{\statepoint{s}}



% === composition: begin
\newcommand\ipart[1]{\mbox{$\mathit{Part}_{#1}$}}
\newcommand\ipartmath[1]{\mathit{Part}_{#1}}
\newcommand\ipartbeh[1]{\mbox{$\besemm{\ipart{#1}}$}}

\newcommand\imeth[1]{\mbox{$\mathit{Meth}_{#1}$}}
\newcommand\imethbeh[1]{\mbox{$\besemm{\imeth{#1}}$}}
\renewcommand\imeth[1]{\mbox{$\mathit{Meth}_{#1}$}}
\newcommand\imethstar[1]{\mbox{$\mathit{Meth}^*_{#1}$}}
\newcommand\istameth[1]{\imethstar{#1}} %the same

\newcommand\iiface[1]{\mbox{$\mathbf{IFace}_{#1}$}}
\newcommand\iifacestar[1]{\mbox{$\mathbf{IFace}^*_{#1}$}}
\newcommand\iistaface[1]{\iifacestar{#1}} %the same


\newcommand\prodspace{\mbox{$\prod_{i}\ipartbeh{i}$}}
\newcommand\prodspa{\mbox{$\prod_{i}\ipartbeh{i}$}}
\newcommand\wholespace{\mbox{$\prod_{i}^*\ipartbeh{i}$}}

\newcommand\prodmeths{\mbox{$%\prod_{i}\imeth{i}
                             \methsset{prod}$}}
\newcommand\wholemeths{\mbox{$%\prod^*_{i}\imeth{i}
                             \someofmethsset{Prod}$}}
\newcommand\prodmethsbeh{\mbox{$\besemm{\prodmeths}$}}
\newcommand\wholemethsbeh[2]{\mbox{$\besemm{\someofmeths{#1}{#2}}$}}
\newcommand\prodiface{\mbox{$%\prod_{i}\iiface{i}
                              \iface{Prod}$}}
\newcommand\wholeiface{\mbox{$%\prod^*_{i}\iiface{i}
                               \ifacepartial{Prod}$}}



%\newcommand\reductmap[1]{\mbox{$\mathit{red}^*_{\mathit{#1}}$}}
\newcommand\reductmap[2]{\mbox{$\mathit{red}^{\mathit{#1}}_{\mathit{#2}}$}}
%\newcommand\reductmapstar[1]{\mbox{$\mathit{red}^*_{\mathit{#1}}$}}
\newcommand\red[2]{\reductmap{#1}{#2}}
\newcommand\redsta[1]{\reductmapstar{#1}}
\newcommand\projectmap[1]{\mbox{$\mathit{proj}_{\mathit{#1}}$}}
%\renewcommand\proj[1]{\projectmap{#1}}
\newcommand\fproj[1]{\mbox{$\pi_{#1}$}}


%==== composition: end =========

\renewcommand\Eng[1]{\mbox{$\mathit{Eng}^#1$}}
\renewcommand\eng[1]{\mbox{$\mathit{eng}^#1$}}
\newcommand\ETOC{\Eng{*}} %Engine methods transferred TO Cars
\newcommand\etoc{\eng{*}}
\newcommand\Etocbeh{\besemm{\Engine^*}}
\newcommand\etocind{EngIntoCar}
\newcommand\ctoeind{CarToEng}

\newcommand\me{\mbox{$m$}}
\newcommand\Me{\mbox{$\mathit{Meth}$}}

%\newcommand\meths1]{\mbox{$\mathit{meth}^{\mathit{#1}}$}}
\newcommand\methsset[1]{\mbox{$\mathit{#1}\mathsf{Meth}$}}
%the same
\newcommand\meths[1]{\mbox{$\mathit{#1}\mathsf{Meth}$}}
%  in short
\newcommand\mset[1]{\methsset{#1}}

\newcommand\imset[1]{\mbox{\methsset{}$_{#1}$}}
\newcommand\someofmethsset[1]{\mbox{$\mathit{#1}^{*}\mathsf{Meth}$}}
% in short
\newcommand\somset[1]{\someofmethsset{#1}}

\newcommand\iface[1]       {\mbox{$\mathit{#1}  \mathbf{IFace}$}}
\newcommand\ifacepartial[1]{\mbox{$\mathit{#1}^*\mathbf{IFace}$}}

\newcommand\methsbody[2]{\mbox{$\besemm{\mathit{#1}}^{\mathit{#2}}$}}
%  in short
\newcommand\mbody[2]{\methsbody{#1}{#2}}
\newcommand\msbody[2]{\mbox{$\besemm{\methsset{#1}}^{\mathit{#2}}$}} % the same
\newcommand\mmbody[1]{\msbody{#1}{}}



\newcommand\someofmethsiface[1]{\mbox{$\ifacepartial{#1}$}}
\newcommand\somface[1]{\someofmethsiface{#1}}

\newcommand\someofmethsbody[2]{\mbox{$\besemm{\someofmethsset{#1}}^{#2}$}}
\newcommand\sombody[2]{\someofmethsbody{#1}{#2}}

\newcommand\miface{\iface{\me}}

\newcommand\categoryname[1]{\mathbf{#1}}
\newcommand\sketchname[1]{\mathsf{#1}}

\newcommand\setcatmath{\categoryname{Sets}}
\newcommand\setskemath{\sketchname{Set}}
\newcommand\vsetcatmath{\categoryname{VarSet}}
\newcommand\bsetcatmath{\categoryname{BehSet}}
\newcommand\coalgcatmath{\categoryname{coAlg}}
\newcommand\coalgske{\sketchname{coAlg}}
\newcommand\erske{\sketchname{ER}}
\newcommand\ercat{\categoryname{ER}}
\newcommand\vsetske{\sketchname{VarSet}}
\newcommand\bsetske{\sketchname{BehSet}}

\newcommand\setcat{\mbox{$\setcatmath$}}
\renewcommand\setcat{\mbox{$\categoryname{Sets}$}}
\newcommand\gracat{\mbox{$\categoryname{Graphs}$}}
\newcommand\posetcat{\mbox{$\categoryname{Posets}$}}
\newcommand\catcat{\mbox{$\categoryname{Cats}$}}


\newcommand\vsetcat{\mbox{$\vsetcatmath$}}
\newcommand\bsetcat{\mbox{$\bsetcatmath$}}
\newcommand\coalgcat{\mbox{$\coalgcatmath$}}
\newcommand\setske{\mbox{$\setskemath$}}


\newcommand\univcat{\mbox{$\categoryname{U}$}}
\newcommand\ucatmath{\categoryname{U}}
\newcommand\univske{\mbox{$\sketchname{U}$}}
\newcommand\uskemath{\sketchname{U}}
\newcommand\ucat{\univcat}
\newcommand\uske{\univske}

\newcommand\instus[2]{\inst{\ske{#1}}{\ucatmath_{#2}}}
\newcommand\uni[1]{\mbox{$\univcat_{#1} $}}

\newcommand\reuniv{\univcat}
\newcommand\mapcatmath{\categoryname{Map}}
\newcommand\mapcat{\categoryname{Map}}
\newcommand\Map[2]{\mbox{$\mapcatmath(#1,#2)$}}
\newcommand\cariface{\iface{\car}}

\newcommand\rePlug{\ittt{rePlug}}
%=====================
%\input{../../Tools/Macros/m01-macroLogic.tex}

%=====================
%\input{../../Tools/Macros/m05-myStyle(razdels).tex}
\newtheorem{mydef}{\noindent Definition}
%\newtheorem{remark}{Remark}
\newtheorem{termin}{\noindent Terminology}

%% ===========================================================
%%the version where razdels are inside subsections not sections
%\newcounter{Razdel}[subsection]
%\newcommand\beginRazd[1]%
%{
%\renewcommand\theRazdel{\thesubsection.\arabic{Razdel}}
%\par%\smallskip
%\noindent\refstepcounter{Razdel}%
%{\bf \thesubsection.\arabic{Razdel} #1} %\mylabel{#2}
%}
%%==========================================================

%% =========================================================
%%the version where razdels are inside sections not subsections
%\newcounter{RazDel}[section]
%\newcommand\beginRazD[1]%  2nd argument is dummy and inherited from old verion
%{
%\renewcommand\theRazDel{\thesection.\arabic{RazDel}}
%\par%\smallskip
%\noindent\refstepcounter{RazDel}%
%{\bf \thesection.\arabic{RazDel} #1} %\mylabel{#2}
%}
%%==============================================================
%
%%\newcommand\EndRazD{\qquad\qquad\mbox{$\diamondsuit$}\par\medskip}
%%\newcommand\EndRazd{\qquad\qquad\mbox{$\diamondsuit$}\par\medskip}
%
%\newcommand\EndRazD{\par\smallskip}
%\newcommand\EndRazd{\par\smallskip}
%%\renewcommand\EndRazD{\mbox{\textbf{endRemark} $\blacktriangleright$}\par\smallskip}
%%\renewcommand\EndRazd{\mbox{\textbf{endRemark} $\blacktriangleright$}\par\smallskip}
%\newcommand\remends{\par\smallskip}
%                   %{\mbox{\textbf{endRemark} $\blacktriangleright$}}
%
%
%\newenvironment{razdel}[2]{\beginRazd{#1}{Razd#2}}{\endRazd}
%\newenvironment{razd}[2]{\beginRazd{{%\itshape
%                                      \bfseries #1}}}{\EndRazd}
%%\newenvironment{razD}[2]{\beginRazD{#1}{RazD#2}}{\EndRazD}
%\newenvironment{razD}[2]{\beginRazD{{%\itshape
%                                      \bfseries #1}}}{\EndRazD}
%\newenvironment{razzD}[1]{\beginRazD{{%\itshape
%                                      \bfseries #1}}}{\EndRazD}
%
%% 1st argument is the title of the razdel,
%% 2nd - dummy, formerly it was for the label
%
%
%\newenvironment{defi}[1]{\beginRazdel{Definition.}  {Defi#1}}{\endRazdel}
%\newenvironment{cons}[1]{\beginRazdel{Construction.}{Cons#1}}{\endRazdel}
%\newenvironment{prop}[1]{\beginRazdel{Proposition.} {Prop#1}}{\endRazdel}
%\newenvironment{theo}[1]{\beginRazdel{Theorem.}     {Theo#1}}{\endRazdel}
%\newenvironment{coro}[1]{\beginRazdel{Corollary.}   {Coro#1}}{\endRazdel}
%\newenvironment{exam}[1]{\beginRazdel{Example.}     {Exam#1}}{\endRazdel}
%%\newenvironment{rema}[1]{\beginRazdel{Remark.}      {Rema#1}}{\endRazdel}
%\newenvironment{warn}[1]{\beginRazdel{Warning.}     {Warn#1}}{\endRazdel}
%\newenvironment{desc}[1]{\beginRazdel{Description.} {Desc#1}}{\endRazdel}
%\newenvironment{disc}[1]{\beginRazdel{Discussion.}  {Disc#1}}{\endRazdel}
%\newenvironment{conv}[1]{\beginRazdel{Convention.}  {Conv#1}}{\endRazdel}
%\newenvironment{nota}[1]{\beginRazdel{Notation.}    {Nota#1}}{\endRazdel}
%
%\newcommand\equnref[1]{Equation~(\ref{Equn#1})}
%\newcommand\equlref[1]{equality~(\ref{Equl#1})}
%%\newcommand\diagref[1]{(\ref{#1})}
%\newcommand\consref[1]{Construction~\ref{Cons#1}}
%\newcommand\defref[1]{Definition~\ref{#1}}
%\newcommand\propref[1]{Proposition~\ref{Prop#1}}
%\newcommand\discref[1]{Discussion~\ref{Disc#1}}
%\newcommand\convref[1]{Convention~\ref{Conv#1}}
%\newcommand\notaref[1]{Notation~\ref{Nota#1}}
%\newcommand\descref[1]{Description~\ref{Desc#1}}
%\newcommand\remaref[1]{Remark~\ref{Rema#1}}
%\newcommand\examref[1]{Example~\ref{Exam#1}}
%\newcommand\cororef[1]{Corollary~\ref{Coro#1}}
%\newcommand\razdref[1]{Section~\ref{Razd#1}}
%%\newcommand\appref[1]{appendix~\ref{App#1}}    see pre_gen.tex
%%\newcommand\sectref[1]{section~\ref{Sect#1}}   ....
%%\newcommand\sectsectref[1]{sections~\ref{Razd#1}}
%%\newcounter{Razdel}[subsection]
%\newcommand\NachRazd[2]%
%{
%%\renewcommand\theRazdel{\thesubsection.\arabic{Razdel}}
%\par\medskip\noindent%\refstepcounter{Razdel}%
%{\it #1} \mylabel{#2} }
%%\newcommand\end{\qquad\qquad\mbox{$\diamondsuit$}\par\medskip}
%
%\newenvironment{Example}{\NachRazd{Example}}{\end}
%\newenvironment{Remark} {\NachRazd{Remark}}{\end}
%\newenvironment{Warning}{\NachRazd{Warning}}{\end}
%=====================
%\input{../../Tools/Macros/m10-MMt-CASCON-Macros.tex}
\newcommand\instarr[1]{\mbox{$\lar{\statemap}{\igra{}{}}{#1}$}}
\newcommand\instarrt[1]{\mbox{$ \lar{\statemap}{\igraph{t}{}}{#1}$}}

\newcommand\idop{\mrksemiop{\times id}}
\newcommand\idos{\mrksemiop{+id}}

\newcommand\idoP{\mrkop{prod}}
\newcommand\idoS{\mrkop{sum}}

\newcommand\recop{\mrkop{rec}}
\newcommand\varop{\mrkop{var}}
%\newcommand\sumop{\mrkop{var}}

\renewcommand\owner{\textit{owner}}
\newcommand\types{\nicex{ T$}}

%% for Kleisly arrows section

\newcommand\ssma{\mbox{$S$}}
\newcommand\tsma{\mbox{$T$}}
\newcommand\usma{\mbox{$U$$$}}
\newcommand\mapelement{\mbox{$\rightsquigarrow$}}
\newcommand\mapel{\mapelement}

\newcommand\klear[3]{\mbox{$#1\!: #2 \rightsquigarrow #3$}}
\newcommand\kleare[2]{\mbox{$#1 \rightsquigarrow #2$}}
\newcommand\lare[2]{\mbox{$#1 \rightarrow #2$}}
%==============================================

\newcommand\corrce{correspondence}






%%% 1. Collections
%
%==1.1 Categories
% macros for names moved to macros4names.tex
%\newcommand\catname[1]{\mbox{\bfseries\itshape #1}}
%%\newcommand\catname[1]{\mbox{\boldmath $#1$}}
%\newcommand\cat[1]{\catname{#1}}
%\newcommand\categoryop[1]{\mbox{\bfseries\itshape #1}$^{\mathrm{op}}$}
%\newcommand\catnamei[1]{{\pmb #1}}



%\newcommand\idmap[1]{\operator{id}_{#1}}
%\renewcommand\f{\mbox{$\phi$}}
%\renewcommand\c{\catname{C}}
%\renewcommand\b{\catname{B}}
%\renewcommand\r{\catname{R}}





\newcommand\clonet{\mbox{${\nia}_\mathrm{Top}$}}
\newcommand\clonem{\mbox{${\nia}_\mathrm{MMt}$}}
%
% -- overlined letters for clones ---
%\newcommand\clonet{\mbox{$\overline{\nia}_\mathrm{Top}$}}
%\newcommand\clonem{\mbox{$\overline{\nia}_\mathrm{MMt}$}}



%==1.2 Classes of nodes/arrows
\newcommand\indclassofitems[1]{{\cal #1}}
\newcommand\classofitems[1]{\mbox{$\indclassofitems{#1}$}}
\newcommand\coi[1]{\classofitems{#1}}
\newcommand\incls{\coi{I}}
\newcommand\covers{\coi{C}}
\newcommand\univs{\coi{U}}
%\renewcommand\diags{\classofitems{D}}
\renewcommand\diags{\mathit{Diags}}
\newcommand\inddiags{\indclassofitems{D}}

%\newcommand\attrset[1]{\mbox{\textit{attrs}$(#1)$}}
%\newcommand\refset[1]{\mbox{\textit{refs}$(#1)$}}
%\newcommand\varset[1]{\mbox{\textit{vars}$(#1)$}}
%\newcommand\classtab[1]{\mbox{\textsf{tab}$_#1$}}
%\newcommand\attrtab[1]{\mbox{\textsf{aTab}$_#1$}}
%\newcommand\reftab[1]{\mbox{\textsf{rTab}$_#1$}}



%===1.3 Languages
\newcommand\querylanguage[1]{\nicex{ QL_{#1}$}}
\newcommand\ql{\querylanguage}
\newcommand\qlmath[1]{{\cal QL}_{#1}}

%%% 2. MMt Objects
\renewcommand\modelob[1]{\mbox{$M_{#1}$}}
\newcommand\schemaobsymbol{S}
\newcommand\typeSyssymbol{Types}
\newcommand\instanceGraphSymbol{I}
\newcommand\relschemaobsymbol{R}
\newcommand\skeobsymbol{S}
\newcommand\universesymbol{U}
\newcommand\valueUniverseGraphSymbol{U}
\newcommand\UniverseGraphSymbol{U}
\newcommand\schemaob[1]{\mbox{${\mathit \schemaobsymbol}_{#1}$}}
%\newcommand\typesys[1]{\mbox{${\mathit \schemaobsymbol}_{#1}$}}
\newcommand\instgra[2]{\mbox{${\mathit \instanceGraphSymbol}_{#1}^{#2}$}}
\newcommand\igra[2]{\instgra{#1}{#2}}
\newcommand\itogra[1]{\instgra{}{#1}}
\newcommand\irefgra[1]{\instgra{ref}{#1}}
\newcommand\iattgra[1]{\instgra{attr}{#1}}
\newcommand\iobjgra[1]{\instgra{obj}{#1}}

\newcommand\uvalgra[1]{\mbox{$\mathit{\universesymbol Val}_{#1}$}}
\newcommand\utupgra[1]{\mbox{$\mathit{\universesymbol Tuple}_{#1}$}}
\newcommand\uval{\uvalgra{}}
\newcommand\utup{\utupgra{}}
\renewcommand\uniob[1]{\mbox{$\mathsf{\universesymbol}_{#1}$}}

\newcommand\relsob[1]{\mbox{${\mathit \relschemaobsymbol}_{#1}$}}
\newcommand\newrelske[1] {\mbox{${\mathsf R}_{#1}$}}
\newcommand\newrelinst[2]{\mbox{${\mathsf Q}_{#1}^{#2}$}}

\newcommand\schemaOB[2]{\mbox{${\mathit \schemaobsymbol}_{#1}^{#2}$}}

\newcommand\claske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{cla}#1}$}}
\newcommand\refske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{ref}#1}$}}
\newcommand\attrske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{attr}#1}$}}
\newcommand\objrefske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{objRef}#1}$}}


\renewcommand\skeob[1]{\mbox{${\mathsf\skeobsymbol}_{#1}$}}
\newcommand\skeobind[1]{{\mathsf \skeobsymbol}_{#1}}
\newcommand\indskeob[1]{\skeobind{#1}}

\newcommand\typeske[1]{\mbox{$\mathsf{Type}_{#1}$}}
\newcommand\typemap[1]{\mbox{$\mathsf{type}_{#1}$}}
\newcommand\typeskeind{\mathsf{Type}}
\newcommand\typemapind[1]{\mathsf{type}_{#1}}

\renewcommand\statemap{\mbox{$\sigma$}}
\newcommand\statemapind{\sigma}




%\newcommand\gs{\mbox{$G_{\indskeob{}}$}}
%\newcommand\ds{\mbox{$\diags_{\indskeob{}}$}}
%\newcommand\gsi[1]{\mbox{$G_{\indskeob{#1}}$}}
%\newcommand\dsi[1]{\mbox{$\G_{\indskeob{#1}}$}}

%%% 2.1  Vectors of objects (bold objects)
%\newcommand\fullvector[3]{}
%\newcommand\vectorobject[1]{\mbox{$\boldsymbol{#1}$}} % see macros4names
\newcommand\multisch{\vectorobject{\schemaobsymbol}}
\newcommand\multiSch{\vectorobject{\schemaobsymbol}}
\newcommand\multinst{\vectorobject{\instancesymbol}}
\newcommand\multinstoo[1]{\mbox{$\multinst=(\inst{1},\ldots,\inst{#1})$}}

\newcommand\multiUni{\vectorobject{\universesymbol}}
\newcommand\multiRel{\vectorobject{\relschemaobsymbol}}
\newcommand\multiuni{\vectorobject{u}}
\newcommand\multirel{\vectorobject{r}}
\newcommand\multiu{\vectorobject{u}}
\newcommand\multir{\vectorobject{r}}
\newcommand\multiroo[1]{\mbox{$\multir=(r_1,\ldots,r_{#1})$}}


%== Operators
\newcommand\operator[1]{\mbox{\sf #1}}
\newcommand\operatorInIndex[1]{{\sf #1}}

\newcommand\heoperator[1]{\mbox{\sf\bfseries #1}}
\newcommand\match{\operator{match}}

\newcommand\indexedoperator[3]{\mbox{\operator{#1}$_{#2}^{#3}$}}
\newcommand\indexedoperatorInIndex[3]{\operatorInIndex{#1}_{#2}^{#3}}

\newcommand\der[2]{\indexedoperator{der}{#1}{#2}}
\newcommand\dero[1]{\indexedoperator{der}{}{#1}}
\newcommand\derInIndex[2]{\indexedoperatorInIndex{der}{#1}{#2}}

%\newcommand\proj[1]{\indexedoperator{p}{#1}{}}
%\newcommand\merge{\operator{merge}}
%\newcommand\modgen{\operator{modelGen}}
%\newcommand\datatrans{\operator{dataTransf}}
%\renewcommand\self{\operator{self}}


\newcommand\SFW[3]{\mbox{\operator{Select} #1
                         \operator{from} #2
                         \operator{where} #3}
                         }

%=====================
%\input{../../Tools/Macros/m20-newMacros}
%\renewcommand\em[1]{\emph{#1}}

%\newcommand\vect[1]{\textbf{#1}}
\newcommand\veg{\vect{G}}
\newcommand\vef{\vect{f}}
\newcommand\ver{\vect{R}}
\newcommand\ves{\vect{S}}
\newcommand\vehh{\vect{H}}
\newcommand\veho{\vect{\ovr{H}}}
\newcommand\veh{\vect{h}}

\newcommand\ovr[1]{\mbox{$\overline{\mathstrut#1}$}}
\newcommand\ovri[1]{\overline{#1}}
\newcommand\ovh[1]{\ovr{H}_{#1}}
%\newcommand\ovri[1]{\mb{\ovr{\iota'}_{#1}}}

\newcommand\edge[1]{\ittt{Edge}\mb{_{#1}}}
\newcommand\Edge[2]{\ittt{Edge}\mb{_{#1}^{#2}}}


\newcommand\univarr[1]{\mb{!_{#1}}}
\newcommand\doublearrow[5]{\mbox{$#1\stackrel{#4}{\rightarrow}
                                 #2\stackrel{#5}{\rightarrow}#3$
}}
\newcommand\arrdou[5]{\doublearrow{#1}{#2}{#3}{#4}{#5}}
\newcommand\arrarr{\arrdou{\gra{2}}{\gra{3}}{\gra{4}}{h_2}{h_3}}
\newcommand\scearr{\arrdou{\gra{2}}{\gra{1}}{\gra{0}}{\tau_1}{\tau_0}}
\newcommand\arrsce{\arrdou{\gra{2}}{\gra{1}}{\gra{0}}{\tau_1}{\tau_0}} % the same as above

\newcommand\arrspan[5]{\fbox{$#1\stackrel{#4}{\leftarrow}
                                 #2\stackrel{#5}{\rightarrow}#3$
}}
\newcommand\arrcospan[5]{\fbox{$#1\stackrel{#4}{\rightarrow}
                                 #2\stackrel{#5}{\leftarrow}#3$
}}

%\renewcommand\span[1]{\textbf{R}\mb{_{#1}}}
\newcommand\cospan[1]{\textbf{S}\mb{_{#1}}}
\newcommand\set[2]{\mb{#1=\{#2\}}}

\newcommand\integr[3]{\mb{#1\bigoplus_#3 #2}}

\newcommand\gran[1]{\mb{G_{{#1}N}}}
\newcommand\gred[1]{\mb{G_{{#1}E}}}
\newcommand\graman[1]{\mb{f_{{#1}N}}}
\newcommand\gramed[1]{\mb{f_{{#1}E}}}
\newcommand\grinman[1]{\mb{\iota'_{{#1}N}}}
\newcommand\grinmed[1]{\mb{\iota'_{{#1}E}}}

% changing from \mathsl to \mathit
\renewcommand\object[2]{\mbox{${\mathit{#1}}_{#2}$}}
\renewcommand\objectind[1]{\mathit{#1}}
\renewcommand\objectmath[1]{\mathit{#1}}

%\newcommand\DOM[1]{\Box #1}
%\newcommand\COD[1]{#1 \Box}


\newcommand\mb[1]{\mbox{$#1$}}
\newcommand\nin{\mb{\cal N}}
\newcommand\nix{\mb{\cal X}}
\newcommand\nil{\mb{\cal L}}
\newcommand\nik{\mb{\cal K}}
\newcommand\dvet{\mbox{:}}
\newcommand\ddvet{\dvet\dvet}
%\newcommand\n{\mb{n}}

\renewcommand\x{\mb{X}}

\newcommand\proxx[2]{\mb{\prod_{#1}{#2}}}
\newcommand\prox{\proxx{}{\vex}}
\newcommand\proy{\proxx{}{\vey}}
\newcommand\prodxn{\proxx{\cal L}{\vex}}
\newcommand\prodxm{\proxx{\cal K}{\vex}}

\newcommand\unixx[2]{\mb{\bigcup_{#1}{#2}}}
\newcommand\unix{\unixx{}{\vex}}

\newcommand\proj[1]{\mb{\ell_{#1}}}
\newcommand\proji{\proj{i}}






\renewcommand\ext{\mbox{\textsf{ext}}}








\newcommand\oclar{\mbox{\footnotesize $>$}}
\newcommand\myendset[1]{\mbox{$\{#1_1..#1_m\}$}}
\newcommand\fens{\myendset{f}}





\newcommand\fulla[1]{\mbox{${\mathbf F}_{#1}$}}
\newcommand\rmap[1]{\mbox{$#1^\rightarrow$}}
\newcommand\lmap[1]{\mbox{$^\leftarrow #1$}}
\newcommand\basemap[1]{\mbox{\textit{base}$_{#1}$}}


\newcommand\seq[1]{\textsf{seq}\mbox{$#1$}}
\newcommand\coll[2]{\textsf{coll}\mbox{$_{#1}(#2)$}}

\newcommand\tabschema{\mbox{$D=\{a_1:D_1,...,a_n:D_n\}$}}
\newcommand\tabschemamap{\mbox{\lar{D}{\attrset{}}{\setcat}}}



%=====================
%\input{../../Tools/Macros/m21--labelsnewMacros}
%(left) labels for formulas
\newcommand\equationNumber[1]{(\textsf{#1})}
\newcommand\eqnumber[1]{\equationNumber{#1}}
\newcommand\eqn[1]{\equationNumber{#1}}


%\newcommand\mafo[2]\mathform{#1}{#2}
\newcommand\mathfo[2]{$$#2\leqno{\mbox{(\textsf{#1})}} $$}
\newcommand\mafo[2]{$$#2 \leqno{\mbox{\eqn{#1}}} $$}


\newcommand\selflab{\eqn{self}}
\newcommand\looplab{\eqn{loop}}
\newcommand\idlelab{\eqn{idle}}
\newcommand\dolab{\eqn{do}}
\newcommand\triglab{\eqn{trigger}}

\newcommand\assonla{\eqn{fullAsson}}
\newcommand\tabla{\eqn{TAB}}
\newcommand\invla{\eqn{inverse}}
\newcommand\extla{\eqn{extension}}
\newcommand\tablatup{\eqn{TABrow}}
\newcommand\tablapro{\eqn{TABattr}}
\newcommand\sepla{\eqn{1-1}}
%=====================================
\newcommand\classn{\eqnumber{classn}}
\newcommand\indexn{\eqnumber{indexng}}

\newcommand\igralabel{\eqnumber{instGra}}
\newcommand\schemaGeneralLabel{\eqnumber{schemaGen}}
\newcommand\stlabel{\schemaGeneralLabel}
\newcommand\itablabel{\eqnumber{instTab}}
%\renewcommand\uniob[1]{\mbox{${\mathsf\universesymbol}_{#1}$}}
\newcommand\igratablabel{\eqnumber{instGraTab}}
\newcommand\igragralabel{\eqnumber{instGraGra}}
\newcommand\itabtablabel{\eqnumber{instTabTab}}

%=====================
%\input{../Tools/Macros/m21--abbrev4formulas}
%\input{../Tools/Macros/m22--abbrev4text}
%--------------------------------
%\renewcommand\zdmargin[1]{}
%\renewenvironment{razd}[2]{\subsubsection{#1}}{}
%\nocite{}
\renewenvironment{razD}[2]{\beginRazD{{%\itshape
                                      \bfseries #1}}}{\EndRazD}

%% sle
%%%%%%%%%% sle09 macros
%\newcommand\diagi[1]{#1\mbox{$'$}}
%\newcommand\diagii[1]{#1\mbox{$''$}}
%
%\newcommand\ari[1]{\mbox{\textsl{ar}$(#1)$}}
%\newcommand\mmname[1]{\textsf{#1}}
%\newcommand\mmcd{\mmname{CD}}
%\newcommand\mmsd{\mmname{SD}}
%\newcommand\mmsc{\mmname{SC}}
%\newcommand\mmca{\mmname{CA}}
%\newcommand\mmamt{\mmname{CAT}}
%\newcommand\mmcat{\mmname{CAT}}
%\newcommand\cd{\mmname{cd}}
%\renewcommand\sd{\mmname{sd}}
%\renewcommand\sc{\mmname{sc}}
%\newcommand\ca{\mmname{ca}}
%\newcommand\amt{\mmname{cat}}
%\renewcommand\cat{\mmname{cat}}
%\newcommand\cdi{\diagi{\cd}}
%\renewcommand\sdi{\diagi{\sd}}
%\newcommand\sci{\diagi{\sc}}
%\newcommand\cdii{\diagii{\cd}}
%\newcommand\sdii{\diagii{\sd}}
%\newcommand\scii{\diagii{\sc}}





\newcommand\base{\mbox{$\pmb{MM}$}}
\newcommand\p{\textbf{P}}
\newcommand\ps{\mbox{$P$}}
\newcommand\leqnoo[1]{\leqno{\mbox{#1}}}

\newcommand\keyword[1]{{\itshape\textsf{#1}}}
\newcommand\nam{\keyword{name}}
\renewcommand\owner{\keyword{owner}}
\newcommand\type{\keyword{type}}
\newcommand\val{\keyword{value}}
\newcommand\Class{\keyword{Class}}
\renewcommand\Attr{\keyword{Attr}}
\newcommand\Type{\keyword{Type}}
\newcommand\elm[1]{\mbox{$\mathit{El}(#1)$}}

\newcommand\ueq{\mbox{$\leftrightarrow$}}
\newcommand\uneq{\mbox{$\rightsquigarrow$}}

\newcommand\meq{\mbox{$=$}}
\newcommand\mneq{\mbox{$\neq$}}


\newcommand\shot{\textsl{shot}}
\newcommand\reltile{\textsl{relTile}}
%\newcommand\tauh{\mbox{$\tau_{\textsf{h}}$}}
%\newcommand\tauv{\mbox{$\tau_{\textsf{v}}$}}



\newcommand\vso{\textsf{v}\mbox{$\partial_0$}}
\newcommand\vta{\textsf{v}\mbox{$\partial_1$}}
\newcommand\hso{\textsf{h}\mbox{$\partial_0$}}
\newcommand\hta{\textsf{h}\mbox{$\partial_1$}}

\newcommand\mmod{\nicex{ M$}}
\newcommand\id{\textsl{id}}
\renewcommand\id{\mbox{$\iota$}}
\newcommand\recon[1]{\mbox{$#1$\textbf{!}}}

\newcommand\oidd[1]{\mbox{$\overline{#1}$}}
\newcommand\oiddi[1]{\mbox{$\overline{#1}'$}}

\renewcommand\oidd[1]{\mbox{${#1}$}}
\renewcommand\oiddi[1]{\mbox{${#1}'$}}

\newcommand\oa{\oidd{a}}
\newcommand\ob{\oidd{b}}
\newcommand\oP{\oidd{P}}
\newcommand\oQ{\oidd{Q}}

\newcommand\oai{\oiddi{a}}
\newcommand\obi{\oiddi{b}}
\newcommand\oPi{\oiddi{P}}
\newcommand\oQi{\oiddi{Q}}

% icmt

%%% icmt09 macros
% the % piece below  was moved to newMacros ---
\newcommand\mrkoprr[1]{\mrkopr{\mrkopr{#1}}}
%\der{}{Q}
%\newcommand\mmview[1]{\mbox{$\textsl{v}_{#1}$}}
%\newcommand\mmarr{v}
\newcommand\mmf{\mbox{$m$}} % to be used in the row
%\renewcommand\mmview[1]{\mbox{$\pmb{\mmarr}_{#1}$}}
%%\newcommand\mmv[1]{{\pmb{\mmarr}_{#1}}} %for subscripts
%\newcommand\mmmap[1]{\mbox{$\pmb{\mmarr}_{#1}$}}
%\renewcommand\mmm{m}  % to be used for sub-sup-indexes
%\newcommand\mmap[1]{\mbox{${\mmarr}_{#1}$}}

\newcommand\unde[1]{\underline{#1}}

\newcommand\oversi[1]{\overline{\sigma}^{#1}}

\newcommand\oversig[1]{\overline{\sigma}^{Q#1}}
\newcommand\overtau[1]{\overline{\tau}^{Q#1}}
\newcommand\overover{\overline{\oversig{1}}}
\newcommand\doublesig{{\overover^{Q2}}} %
\newcommand\votono{{\overline{\oversig{}}^{R}}}

\newcommand\derqq[2]{\mbox{$\dero{Q#1}#2$}}
\newcommand\dermms[1]{\derqq{#1}{\mms}}
\newcommand\derms[1]{\derqq{#1}{\ms{}}}
\newcommand\derqmms{\derqq{}{\mms}}
\newcommand\derqms{\derqq{}{\ms{}}}
\newcommand\derq[1]{\mbox{$\der{}{Q}#1$}}
\newcommand\doubleder[1]{\derqq{1;Q2}{#1}}

\newcommand\augtymaps{\flar%
{\overline{\sigma}^{Q}}%
{\dero{Q}\ms{}}%
{\dero{Q}\mms}%
}
%\newcommand\mmarr{\mbox{$m$}}

%
\newcommand\tracemap[1]{\mbox{$\stackrel{\rightsquigarrow}{#1}$}}
\renewcommand\tracemap[1]{\mbox{$\mathit{tr}_{#1}$}}
\renewcommand\tracemap[1]{\mbox{$#1^{*}$}}
\newcommand\tram{\tracemap{\mmmap}}
%
\newcommand\reversemap[1]{\mbox{\spf$_{#1}$}}
%\newcommand\revem{\reversemap{\mmview{}}}
\newcommand\revem[1]{\mbox{$\semm{\mmmap{#1}}$}}

\renewcommand\s[1]{\mbox{$S_{#1}$}}
\renewcommand\ms[1]{\mbox{$S_{#1}$}}
\newcommand\mos[1]{\mbox{$\overline{S}_{#1}$}}
\renewcommand\mt[1]{\mbox{$T_{#1}$}}
\newcommand\mot[1]{\mbox{$\overline{T}_{#1}$}}
\newcommand\mh[1]{\mbox{$H_{#1}$}}
\renewcommand\ml[1]{\mbox{$L_{#1}$}}

\newcommand\pbop{\operator{PB}}

\newcommand\msarr{\flar{\sigma}{S}{\mms}}
\newcommand\msarrq{\flar{\overline{\sigma}^{Q}}{\der{}{Q}S}{\der{}{Q}\mms}}
\newcommand\mssym{\mbox{$\overline{\sigma}$}}
\newcommand\mssymq{\mbox{$\overline{\sigma}^Q$}}

\newcommand\mtarr{\flar{\tau}{T}{\mmt}}
\newcommand\srelarr{\flar{\sigma}{S}{\mmrel}}
\newcommand\erdarr{\flar{\tau}{D}{\mmer}}
\newcommand\srelderarr[1]{\flar{\overline{\sigma}^{Q#1}}{\der{}{Q#1}S}{\der{}{Q#1}\mmrel}}



\newcommand\ertorel[1]{\flar{\textsf{er2rel}_{#1}}{\mmer}{\mmrel}}
\newcommand\ertorelder[1]{\flar{\textsf{er2rel}_{#1}}{\mmer}{\der{}{{Q#1}}\mmrel}}

% gttse

%\renewcommand\mmname[1]{\mbox{$\pmb{\cal #1}$}}
%\newcommand\mmmapname[1]{\mbox{$\pmb{#1}$}}
%\newcommand\mma{\mmname{M}}
%\newcommand\mmb{\mmname{N}}
%\newcommand\mmc{\mmname{O}}
%\newcommand\mmr[1]{\mbox{\mmname{R}$_{#1}$}}
%\renewcommand\mmr[1]{\mbox{$\pmb{r}_{#1}$}}
%\newcommand\mmab{\mmname{MN}}
%\newcommand\mmac{\mmname{MO}}
%\newcommand\mmv{\mmmapname{v}}
%\newcommand\mmw{\mmmapname{w}}
%\newcommand\mmp{\mmmapname{p}}
%\newcommand\mmq{\mmmapname{q}}

\renewcommand\dvet{\mbox{:\,}}

\newcommand\newrevem[1]{\mbox{$\semm{\mmmapname{#1}}$}}
\newcommand\rev{\newrevem{v}}
\newcommand\rew{\newrevem{w}}
\newcommand\rep{\newrevem{p}}
\newcommand\req{\newrevem{q}}


\newcommand\mmnamei[1]{\pmb{\cal #1}}
\newcommand\mmabi{\mmnamei{MN}}
\newcommand\mmaci{\mmnamei{MO}}
\newcommand\amn{\mbox{$A_{\mmabi}$}}
\newcommand\bmn{\mbox{$B_{\mmabi}$}}
\newcommand\amnprim{\mbox{$A'_{\mmabi}$}}
\newcommand\bmnprim{\mbox{$B'_{\mmabi}$}}
\newcommand\amo{\mbox{$A_{\mmaci}$}}
\newcommand\cmo{\mbox{$C_{\mmaci}$}}
\newcommand\umn{\mbox{$u_{\mmabi}$}}
\newcommand\vmn{\mbox{$v_{\mmabi}$}}

\newcommand\lmmes{\left] \respace\left] }
\newcommand\rmmes{\right[\respace\right[}
\newcommand\mmes[1]{\mbox{$\lmmes\, \mathit{#1} \, \rmmes$}}

% spans

\newcommand\spancat{\category{Span}}
\newcommand\spansa{\scat\spancat}
\newcommand\spanset{\setcat\spancat}
\newcommand\cospancat{\category{Cospan}}
\newcommand\cospansa{\scat\cospancat}
\newcommand\cospanset{\setcat\cospancat}


\newcommand\spanfull[4]{\mbox{${\cal #1}$=(\flar{#2_i}{#3}{#4 i},
$i=1,2)$}}

\newcommand\lKleisly{\Leftarrow}
\newcommand\rKleisly{\Rightarrow}
\newcommand\spandiag[5]  {\fbox{$#1\lTo^{#2} #3 \rTo^{#4} #5$}}
\newcommand\kleispandiag[5]{\fbox{$#1\lKleisly^{#2} #3 \rKleisly^{#4} #5$}}
\newcommand\kleislispandiag[5]{\fbox{$#1\lKleisly^{#2} #3 \rKleisly^{#4} #5$}}
\newcommand\cospandiag[5]{\fbox{$#1\rTo^{#2} #3 \lTo^{#4} #5$}}
\newcommand\kleicospandiag[5]{\fbox{$#1\rKleisly^{#2} #3 \lKleisly^{#4} #5$}}
\newcommand\kleislicospandiag[5]{\fbox{$#1\rKleisly^{#2} #3 \lKleisly^{#4} #5$}}


\newcommand\flarsemm[3]{\flar{#1}{\semm{#2}}{\semm{#3}}}
\newcommand\spandiagsemm[5]{\fbox{$\semm{#1}\lTo^{#2} \semm{#3} \rTo^{#4} \semm{#5}$}}
\newcommand\cospandiagsemm[5]{\fbox{$\semm{#1}\rTo^{#2} \semm{#3} \lTo^{#4} \semm{#5}$}}


%=== with brackets
\newcommand\spandiagbra[5]
{\mbox{$%\left %
(#1\stackrel{~#2}{\leftarrow} #3
                                           \stackrel{#4~}{\rightarrow} #5%\right
)$}}
\renewcommand\kleispandiag[5]{\mbox{$\left(#1\stackrel{~#2}{\lKleisly} #3
                                             \stackrel{#4~}{\rKleisly} #5
                                             \right)$}}
\renewcommand\kleislispandiag[5]{\mbox{$\left(#1\stackrel{#2}{\lKleisly} #3
                                             \stackrel{#4}{\rKleisly} #5
                                             \right)$}}
\renewcommand\kleicospandiag[5]{\mbox{$\left(#1\stackrel{#2}{\rKleisly} #3
                                             \stackrel{#4}{\lKleisly} #5
                                             \right)$}}
\renewcommand\kleislicospandiag[5]{\mbox{$\left(#1\stackrel{#2}{\rKleisly} #3
                                             \stackrel{#4}{\lKleisly} #5
                                             \right)$}}

\renewcommand\cospandiag[5]{\mbox{$\left(#1\rTo^{#2} #3 \lTo^{#4} #5\right)$}}
\renewcommand\cospandiag[5]  {\mbox{$\left(#1\stackrel{~#2}{\rightarrow} #3
                                           \stackrel{#4~}{\leftarrow} #5\right)$}}

% without brackets
\renewcommand\spandiag[5]  {\mbox{$#1\stackrel{~#2}{\leftarrow} #3
                                           \stackrel{#4~}{\rightarrow} #5$}}
\renewcommand\cospandiag[5]  {\mbox{$#1\stackrel{~#2}{\rightarrow} #3
                                           \stackrel{#4~}{\leftarrow} #5$}}


%\renewcommand\kleislycospandiag[5]{\mbox{$\left(#1\rKleisly^{#2} #3 \lKleisly^{#4} #5\right)$}}

\renewcommand\flarsemm[3]{\flar{#1}{\semm{#2}}{\semm{#3}}}
\renewcommand\spandiagsemm[5]{\mbox{$\left(\semm{#1}\lTo^{#2} \semm{#3}\rTo^{#4} \semm{#5}\right)$}}
\renewcommand\cospandiagsemm[5]{\mbox{$\left(\semm{#1}\rTo^{#2} \semm{#3}\lTo^{#4} \semm{#5}\right)$}}


%% end macros



%%==== end newMacros


==> macros/4general-prev.tex <==
% == rotation command
%\rotatebox[origin=c]{45}{$xxx$} 
\newcommand\qqquad{\qquad\quad}
\newcommand\qqqquad{\qquad\qquad}
%\newcommand{\tmapleft[2]}{\ensuremath{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% == my font discipline for defs for Springer ==

\newenvironment{defin}[1][]{\ifthenelse{\equal{#1}{}}{\definition}{\definition[#1]}\rm}{\enddefinition}
\newenvironment{propo}[1][]{\ifthenelse{\equal{#1}{}}{\proposition}{\proposition[#1]}\rm}{\endproposition}
\newenvironment{remar}[1][]{\ifthenelse{\equal{#1}{}}{\remark}{\remark[#1]}\rm}{\endremark}
% \newtheorem{defin}{Definition}
% \newtheorem{corol}{Corollary}
% \newtheorem{theorem}{Theorem}
% \newtheorem{propo}{Proposition}
% \newtheorem{rema}{\textit{Remark}}
% \newtheorem{example}{Example}

%% ATTENTION PLS !
%  for Elsevieer, the above macros don't work, but versions below do work
% \let\oldexample=\example
% \let\endoldexample=\endexample
% \renewenvironment{example}{\vspace{-0.6em}\begin{oldexample}}{\end{oldexample}\vspace{-0.35em}}

% \let\olddefin=\defin
% \let\endolddefin=\enddefin
% \renewenvironment{defin}{\vspace{-0.6em}\begin{olddefin}}{\end{olddefin}\vspace{-0.5em}}

% \let\oldpropo=\propo
% \let\endoldpropo=\endpropo
% \renewenvironment{propo}{\vspace{-0.6em}\begin{oldpropo}}{\end{oldpropo}\vspace{-0.5em}}

% \let\oldrema=\rema
% \let\endoldrema=\endrema
% \newenvironment{rema}{\vspace{-0.6em}\begin{oldrema}}{\end{oldrema}\vspace{-0.5em}}

% \let\oldcorol=\corol
% \let\endoldcorol=\endcorol
% \newenvironment{corol}{\vspace{-0.6em}\begin{oldcorol}}{\end{oldcorol}\vspace{-0.5em}}

% \let\oldtheorem=\theorem
% \let\endoldtheorem=\endtheorem
% \renewenvironment{theorem}{\vspace{-0.6em}\begin{oldtheorem}}{\end{oldtheorem}\vspace{-


% math operations

\newcommand\opname[1]{\ensuremath{\mathsf{#1}}}
\newcommand\colim{\opname{colim}}
\newcommand\limcat{\opname{lim}}

%===== Calligraph. Literals ======
\newcommand\niceletter[1]{\ensuremath{{\cal #1}}}
\newcommand\nicex[1]{\niceletter{#1}}
\newcommand\nia{\nicex{A}}
\newcommand\nib{\nicex{B}}
\newcommand\nid{\nicex{D}}
\newcommand\nie {\nicex{E}}
\newcommand\nik {\nicex{K}}
\newcommand\nil {\nicex{L}}
\newcommand\nim{\nicex{M}}

\newcommand\nio{\nicex{O}}
\newcommand\nip{\nicex{P}}
\newcommand\nir{\nicex{R}}
\newcommand\nit{\nicex{T}}
\newcommand\niu{\nicex{U}}
\newcommand\niw{\nicex{W}}
\newcommand\nix{\nicex{X}}


% Domain-codomain/source-target/ident
\newcommand\cod[1]{\ensuremath{{#1}^\bullet}}
\newcommand\dom[1]{\ensuremath{^\bullet{#1}}}
\newcommand\so{\ensuremath{\mathsf{src}}}
\newcommand\ta{\ensuremath{\mathsf{trg}}}
\renewcommand\so{\ensuremath{\mathsf{s}}} % was src
\renewcommand\ta{\ensuremath{\mathsf{t}}}  % was trg
\newcommand\ldom[1]{\ensuremath{$\Box #1 $}}
\newcommand\rdom[1]{\ensuremath{$#1 \Box $}}
\newcommand\id[1]{\opname{id}_{{#1}}}
\renewcommand\id{\opname{id}}

% fig and others references
\newcommand\figref[1]{Fig.~\ref{#1}}
\newcommand\exref[1]{Ex.~\ref{#1}}
\newcommand\defref[1]{Definition~\ref{#1}}
\newcommand\tabref[1]{Table~\ref{#1}}
\newcommand\diagref[1]{(\ref{#1})}
%\newcommand\eqref[1]{\ref{#1}}
\newcommand\sectref[1]{Sect.~\ref{#1}}
\newcommand\secref[1]{Sect.~\ref{#1}}
\newcommand\appref[1]{Appendix~\ref{#1}}
%\newcommand\eqref[1]{(\ref{#1})}
%===============================================


% my macros for Formulas 

% roman font in math formulas
\newcommand\rmand{\mbox{ and }}
\newcommand\rmor{\mbox{ or }}
\newcommand\rmxor{\mbox{ xor }}

\newcommand\eqdef{\ensuremath{\stackrel{\mathrm{def}}{=}}}

% semantic brackets 
\newcommand\respace{\!}%\!\!}
\newcommand\lsemm{\left[ \respace\left[ }
\newcommand\rsemm{\right]\respace\right]}
\newcommand\semm[1]{\mbox{$\lsemm\, \mathit{#1} \, \rsemm$}}

% less blank space
\newcommand\timm{{\times}}
\newcommand\inn{{\in}}
\newcommand\subsett{{\subset}}
\newcommand\supsett{{\superset}}

%Suggestive Names for MathSymbols
\newcommand\superset{\supset}
\newcommand\subeq{{\subseteq}}
\newcommand\supeq{{\supseteq}}
\newcommand\sqsubeq{{\sqsubseteq}}
\newcommand\sqsupeq{{\sqsupseteq}}
\newcommand\varno{{\varnothing}}
\newcommand\subsetarr{\ensuremath{\hookrightarrow}}
\newcommand\supsetarr{\ensuremath{\hookleftarrow}}

\newcommand\this{\ensuremath{\underline{\mathrm{this}}}}
\newcommand\self{\ensuremath{\underline{\mathrm{self}}}}


\newcommand\ovr[1]{\ensuremath{\overline{#1}}}
\newcommand\und[1]{\ensuremath{\underline{#1}}}


\newcommand\rarr{{\rightarrow}}
%\newcommand\lar{\leftarrow}
\newcommand\larr{{\leftarrow}}
\newcommand\ifff{\Leftrightarrow}
\newcommand\iffarrow{\Leftrightarrow}
\newcommand\bottom{\perp}
\newcommand\disj{\vee}
\newcommand\sdisj{\stackrel{!}{\vee} }
\newcommand\conj{\wedge}
%\newcommand\mathand{\,\&\,}
\renewcommand\neg{\sim}
\newcommand\ded{\vdash}
\newcommand\semded{\models}
\newcommand\synent{\ensuremath{\vdah}}
\newcommand\sement{\ensuremath{\models}}

\newcommand\njoin[2]{\mathbin{${#1}\triangleright\!\triangleleft\;{#2}$}}

%\newcommand\ifthenelse[3]{{\bf if}#1{\bf then}#2{\bf else}#3}


\newcommand\true{\nmf{true}}
\newcommand\false{\nmf{false}}

% Operations 

\newcommand\image[2]{\opname{Image}_{#1}{#2}}
\newcommand\img[2]{\image{#1}{#2}}
%\newcommand\range[2]{\Operation{Range}_{#1}({#2})}

%\newcommand\aut{\ensuremath{\operation{Aut}}}
\newcommand\isoind{\opname{iso}}
\newcommand\iso{\isoind}

\newcommand\coimage[2]{\opname{CoIm}_{#1}{#2}}
\newcommand\coim[2]{\coimage{#1}{#2}}

\renewcommand\restriction[2]{#1\left\lceil_{#2}\mathstrut\right.}
\renewcommand\restriction[2]{#1\upharpoonright_{#2}\mathstrut}
\newcommand\restr[2]{\restriction{#1}{#2}}

\newcommand\idmap[1]{\Operation{id}_{#1}}

\newcommand\Inverse[1]{\left (\mathstrut {#1} \right )^{-1}}
%\newcommand\inverse[1]

%  Comprehension

\newcommand\comprehension[2]{\ensuremath{\left\{{#1}\left|\;{#2}\right.\right\}}}
\renewcommand\comprehension[2]{\ensuremath{\left\{{#1}| \;{#2}\right\}}}  % big brackets
\renewcommand\comprehension[2]{\ensuremath{\{{#1}| \;{#2}\}}}
\newcommand\compr[2]{\comprehension{#1}{#2}}
\newcommand\tuplecompr[2]
{\left\langle{#1}\left|\;{#2}\right.\right\rangle}
\newcommand\tuple[1]{\left\langle\mathstrut {#1}\right\rangle}
\newcommand\cotuplecompr[2]
{\left\rangle\mathstrut {#1}\left|\;{#2}\right.\right\langle}
\newcommand\cotuple[1]{\left\rangle\mathstrut {#1}\right\langle\;}
\newcommand\family[2]{\left(\mathstrut #1 \right)_{#2}}
\newcommand\famm[2]{\family{#1}{#2}}
% big brackets
\newcommand\comprfam[2]{\left(\mathstrut{#1}\left|\;{#2}\right.\right)}
\newcommand\famcompr[2]{\left(\mathstrut{#1}\left|\;{#2}\right.\right)}
% normal brackets
\renewcommand\comprfam[2]{(\mathstrut{#1}\left|\;{#2}\right.)}
\renewcommand\famcompr[2]{(\mathstrut{#1}\left|\;{#2}\right.)}
\newcommand\newfamm[2]{\compfamily{#1}{#2}}
\newcommand\arrfamm[4]{\family{%
		\lar{#1}{#2}{#3}%
	}{#4}}


\newcommand\cotimes{+}
\newcommand\noteq{\ne}
\newcommand\mybigcup[2]{\bigcup\compr{#1}{#2}}
\newcommand\mybigcap[2]{\bigcap\compr{#1}{#2}}

\newcommand\myprod[1]{{#1 \prod}}



%-- categories names
\newcommand\catname[1]{\mbox{\bfseries\itshape #1}}
%\newcommand\cat[1]{\catname{#1}}
\newcommand\catnameind[1]{{\pmb #1}}
\newcommand\categoryop[1]{\mbox{\bfseries\itshape #1}$^{\mathrm{op}}$}



%\renewcommand\cat[1]{\catname{#1}}
\newcommand\CC{\catname{C}}

\newcommand\graphcat{\catname{Graphs}}
\newcommand\setcat{\catname{Set}}
\newcommand\twocat{\catname{2}}
\newcommand\relcat{\catname{Rel}}
\newcommand\catcat{\catname{Cat}}
\newcommand\natset{\catname{Nat}}
\newcommand\gracat{\catname{Graphs}}
\newcommand\rgracat{\catname{rGraphs}}
\newcommand\twogracat{\catname{2Graphs}}
\newcommand\dbgracat{\catname{dblGraphs}}
\newcommand\posetcat{\catname{Posets}}
\newcommand\reprcat{\catname{Repr}}
\newcommand\schemacat{\catname{Schema}}
%\newcommand\catname[1]{\mbox{\boldmath $#1$}}



%=== word shorcuts
% \newcommand\eg{e.g.}
% \newcommand\ie{i.e.}
% \newcommand\etal{\textit{et al}}
%\newcommand\fwk{framework}
%\newcommand\traj{trajector}
%\newcommand\traj{trajector}
%\newcommand\syncon{synchronization}
%\newcommand\Syncon{Synchronization}
\newcommand\symmen{symmetrization}
\newcommand\Symmen{Symmetrization}


\endinput




\setlength{\marginparwidth}{3cm}
%\setlegth{\marginparsep}{1.5mm}
%\setlength{\marginparpush}{5mm}
%

\makeatletter
  \def\fps@figure{tp}
\makeatother

\newcommand{\backgro}[2]{\par\noindent\framebox[\textwidth]{
\begin{minipage}{0.98\textwidth}
\setlength{\parindent}{0.5cm} \noindent \textbf{Background: #1} #2
\end{minipage}}\smallskip}

%%%% macros %%%
%\newtheorem{defin}{Definition}%[section]
%\renewcommand{\thedefin}{\Alph{defin}}

\newcounter{defCounter}
\newenvironment{defin}[1][]{
\refstepcounter{defCounter}
\begin{trivlist}
\item[\hskip \labelsep {\bfseries Definition \arabic{defCounter} (#1) }]}%
{\end{trivlist}}



%\newcommand\xxx[4]{{\it #1}\mbox{$_{#3}^{#4}{#2}$}}
%\newcommand{\s}{\star}
%\newcommand\mrk[1]{\mbox{$\langle${\tt #1}$\rangle$}}
%=================================================
% 1  Fonts and letters
%============================================

%=====================================================
% 2  Mathematical shtuchki
%=========================================================


% New Symbols allowed to use in MathMode (!)
%========= General =============
\newcommand\mylist[2]{\mbox%
                          {$#1_1,\ldots,#1_{#2}$}}

\newcommand\iidots[2]{\mbox{
                            $#1=1,\ldots,#2$
                      }}
\newcommand\ijdots[3]{\mbox{
                            $#1=#2,\ldots,#3$
                      }}
\newcommand{\vare}{\varepsilon}
\newcommand\nr{\normalsize\rm}
\newcommand\tril{\triangleleft}
\newcommand\eqdef{\stackrel{\rm def}{=}}
\newcommand\trir{\triangleright}
\newcommand\bc{\bigcirc}







%(4)%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Abbreviations of words from pre_gen
%%%%%%%%%%%%%%%%%%%%%

%\newcommand\ql{query \lan} comment for ISMIS'96
\newcommand\sync{synchronous}
\newcommand\async{asynchronous}
\newcommand\syncn{synchronization}
\newcommand\syncd{synchronized}
\newcommand\Sync{Synchronous}
\newcommand\Async{Asynchronous}
\newcommand\Syncn{Synchronization}
\newcommand\Syncd{Synchronized}

\newcommand\sce{scenario}

\newcommand\eqe{equivalence}
\newcommand\eqt{equivalent}

\newcommand\intn{intuition}
\newcommand\intv{intuitive}
\newcommand\coa{coalgebra}
\newcommand\ispartof{\ittt{isPartOf}}
\newcommand\isPartOf{\ittt{isPartOf}}
\newcommand\IsPartOf{\ittt{isPartOf}}

\newcommand\of{\ittt{(isPart)Of}}
\newcommand\Of{\ittt{Of}}
\newcommand\arrdl{ArrDL}
\newcommand\elmsl{ElmSL}

\newcommand\isa{\ittt{isA}}
\newcommand\IsA{\ittt{isA}}
\newcommand\isA{\ittt{isA}}


\newcommand\subst{\ittt{subst}}


\newcommand\OOAD{OOA\&D}
\newcommand\oid{o-id}

\newcommand\pred{predicate}

\newcommand\interstan{interstate relation}
\newcommand\intrel{interstate relation}
\newcommand\demon{demonstration}
\newcommand\demoe{demonstrate}
\newcommand\asson{association}
\newcommand\config{configuration}
\newcommand\asscon{association configuration}
\newcommand\ass{associative}
\newcommand\assive{associative}
\newcommand\aggrn{aggregation}
\newcommand\attrn{attribution}
\newcommand\abbrn{abbreviation}
\newcommand\gen{generalization}
\newcommand{\iden}{identification}
\newcommand\idey{identity}
\newcommand\qualn{qualification}
\newcommand\reprn{representation}
\newcommand\situn{situation}
\newcommand\speln{specialization}
\newcommand\spen{specialization}
\newcommand\spel{specialization}
\newcommand\spec{specification}
\newcommand\implen{implmentation}
\newcommand\impleg{implmenting}
\newcommand\strul{structural} %\strul

\newcommand\spenisa{\spen\ \isa-arrow}
\newcommand\genisa {\gen\  \isa-arrow}

\newcommand\visun{visualization}


%\newcommand\gen{generalization}
\newcommand\repr{representation}

\newcommand\visn{visualization}


%\newcommand{\oid}{object identity}
\newcommand{\oids}{object identities}



\newcommand\datamod[1]{{\rm #1}}

\newcommand\ERC{\datamod{ERC\mbox{$^+$}}}
\newcommand\ercd{\ERC-diagram}
\newcommand\ER{\datamod{ER}}
\newcommand\EER{\datamod{EER}}
\newcommand\RM{\datamod{RM}}
\newcommand\RMT{\datamod{RM/T}}
\newcommand\RDM{\datamod{RDM}}
\newcommand\VO{\datamod{VO}}
\newcommand\OOO{\datamod{OO}}
\newcommand\SDM{\datamod{SDM}}
\newcommand\FDM{\datamod{FDM}}
\newcommand\IFO{\datamod{IFO}}
\newcommand\Oid{\datamod{Oid}}
\newcommand\RO{\datamod{RO}}
\newcommand\ROP{\datamod{RO\mbox{$^+$}}}
\newcommand\Flogic{\datamod{F-logic}}
\newcommand\SkeDM{\datamod{SkeDM}}
\newcommand\Diagr{\datamod{Diagrams}}

\newcommand\datatrend[1]{{\bf #1}}

\newcommand\eer{\datatrend{eer}}
\newcommand\ooo{\datatrend{oo}}
\newcommand\pl{\datatrend{pl}}
\newcommand\skeske{\datatrend{ske}}

\newcommand\msour{multisource}
\newcommand\sour{source}

\newcommand\abbr{abbreviat}
\newcommand\lega{legacyless}


\newcommand\Ass{Associative}



\newcommand{\ider}{identifier}
\newcommand{\deor}{descriptor}

\newcommand\dombs{domain-based sketch}
\newcommand\ms{multisource}
\newcommand\mt{multitarget}
\newcommand\refin{refinement}
\newcommand\db{database}
\newcommand{\grab}{graph-based }
\newcommand{\spef}{specification}
%\newcommand\spec{specification}
\newcommand{\grabs}{\grab\spef}
\newcommand{\lan}{language}
\newcommand{\sgd}{\spel$\!$/\gen distinction }
\newcommand\qr{query }
\newcommand\qrs{queries}

%%%%% Integration %%%%%%%%%%%%%

\newcommand{\integ}{integration}
\newcommand{\intd}{integrated}
\newcommand{\di}{data integration }
\newcommand{\dbi}{database integration }
\newcommand{\vi}{view integration }
\newcommand{\si}{schema integration}
\newcommand{\sdi}{schema and data integration }
%-------------------------------------
\newcommand{\cmod}{conceptual modeling}
\newcommand{\smod}{semantic modeling}
\newcommand{\dbs}{data base}
\newcommand{\dml}{data model}
%\newcommand{\dm}{data model}%{dm}%{DM} % an abbreviation
\newcommand\const{constraint}
\newcommand{\attr}{attribute}
%=====================================
\newcommand\cdb{component \db}
\newcommand\dincy{data inconsistency}
\newcommand\corr{correspondence}
\newcommand\lang{language}
%------
\newcommand\corinf{correspondence information}
\newcommand\corrinf{correspondence information}

\newcommand\coras{correspondence assertion}
\newcommand\corass{correspondence assertions}
\newcommand\corda{correspondence data}
\newcommand\coreq{\corr\ equation}
\newcommand\coreqs{\corr\ equations}

\newcommand\dacorr{data \corr}
\newcommand\cors{\corr\ \ske}
\newcommand\corss{\corr\ \skes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\relship}{relationship}
%----------------------------------------
\newcommand{\Spc}{Spaccapietra {\em et al} }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\ske{sketch}
\newcommand\skes{sketches}
\newcommand\cske{component sketch}
\newcommand\cskes{component sketches}
\newcommand\eroo{\cite{ER95}}
%%%%%%%%%%%% Romanic abbreviations  %%%%%%%%%%%%
\newcommand\eg{e.g.}
\newcommand\ie{i.e.}
\newcommand\wrt{w.r.t.}
\newcommand\etc{{\em etc}}
\newcommand\etal{{\em et al}}
\newcommand\ala{{\em a la }}
\newcommand\apriori{{\em a priori}}
\newcommand\adhoc{{\em ad hoc}}
\newcommand\dejure{{\em de jure}}
\newcommand\defacto{{\em de facto}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\sign}{signature}
%\newcommand{\constr}{constructivizab}% *le or *ility
%\newcommand{\cat}{category}
%\newcommand{\cats}{categories}
%\newcommand{\ct}{category theory\ } %y or ies
%\newcommand\mor{morphism}
%\newcommand\amor{automorphism}
%\newcommand\alg{algebra}
%%\newcommand\inst{institution}
%=============================

%(5)\newcommand\entails{\Rightarrow}
%\newcommand\implies{\Rightarrow}
%-------------------------------------
%\newcommand\dom[1]{\mathit{Dom}(#1)}
%\newcommand\cod[1]{\mathit{Cod}(#1)}
\newcommand\rg[1]{\mathit{Rg}(#1)}
\newcommand\DOM[1]{\Box #1}
\newcommand\COD[1]{#1 \Box}

\newcommand\tabname[1]{\mbox{$\ittt{Tab}\_#1$}}
%\newcommand\multisource[
\newcommand\mytilde[1]{\widetilde{#1}}
\newcommand\sempr[1]{\mytilde{\semm{#1}}}

\newcommand\mycount[1]{{\bf count}{(#1)}}
\newcommand\gragen[1]{\left[\mathstrut #1 \right]}

\newcommand\respace{\!}%\!\!}
\newcommand\lsemm{\left[ \respace\left[ }
\newcommand\rsemm{\right]\respace\right]}
\newcommand\semm[1]{\mbox{$\lsemm\, \mathit{#1} \, \rsemm$}}
\newcommand\semmind[2]{\mbox{$\lsemm\, \mathit{#1} \, \rsemm^{#2}$}}



\newcommand\semmindex[1]{\lsemm\, \mathit{#1} \, \rsemm}
\newcommand\semmstar[1]{\semm{#1}^{*}}
\newcommand\lbesemm{\left< \respace\left<}
\newcommand\rbesemm{\right> \respace\right>}
\newcommand\besemm[1]{\mbox{$\lbesemm\, \mathit{#1} \, \rbesemm$}}



%(6)%\newcommand\informalPar[1]{\nicex{{#1}$}}
%\newcommand\infParind[1]{\cal #1}
%Contents:
%--- semiotics
%--- Skesig
%--- Varset
%--- Behset



%%==== Semiotics =====
%
%%\newcommand\formalPar[1]{\mbox{$\mathrm{#1}$}}
%\newcommand\frmParind[1]{\mathrm{#1}}
%
%\newcommand\informalParBold[1]{\mbox{${\cal #1}$}}
%\newcommand\formalPar[1]{\mbox{$\mathrm #1$}}
%
%\newcommand\object[2]{\mbox{${\mathsf{#1}}_{#2}$}}
%%\newcommand\object[2]{\mbox{$#1_{#2}$}}
%\newcommand\universe[1]{\mbox{$\mathbf{#1}$}}
%%\newcommand\objectind[1]{\mathsf{#1}}
%\newcommand\objectind[1]{\mathsf{#1}}
%\newcommand\universeind[1]{\mathbf{#1}}
%
%\newcommand\proc[1]{\mbox{\sffamily\bfseries #1}}
%\newcommand\procind[2]{\mbox{${\mathrm{#1}}_{\mathrm #2}$}}
%\newcommand\linf{\informalParBold{L}}
%\newcommand\minf{\mbox{$\informalPar{M}(\diag{})$}}
%\newcommand\mdinf{\mbox{$\informalPar{M}(\diag{})$}} % the same as above
%\newcommand\mdfrm{\mbox{$\formalPar{M}(\diag{})$}} % the same as above
%\newcommand\uinf{\informalPar{U}}
%
%\newcommand\meaninf{\informalPar{M}}
%\newcommand\meanfrm[1]{\mbox{$\formalPar{M}_{#1}$}}
%\newcommand\diag[1]{\object{D}{#1}} %\mbox{$D$}}
%\newcommand\diagob[1]{\object{D}{#1}} %\mbox{$D$}}
%\newcommand\diags{\mbox{$\mathit{Diags}$}}
%\newcommand\graph{\mbox{$\mathit{Graph}$}}
%\newcommand\skeob[1]{\object{S}{#1}}
%\newcommand\modelob[1]{\object{M}{#1}}
%\newcommand\sigob[1]{\object{\mbox{$\Sigma$}}{#1}}
%\newcommand\skediag{\skeob{}[\diag{}]}
%\newcommand\meaninfdiag{\meaninf[\diag{}]}
%\newcommand\meanfrmdiag{\meanfrm[\diag{}]}
%% synonyms
%\newcommand\meanifdiag{\meaninf[\diag{}]}
%\newcommand\meanfdiag{\meanfrm[\diag{}]}

%=======================
%==== Skesig
%\newcommand\so[1]{source(#1)}
%\newcommand\ta[1]{target(#1)}
\newcommand\U{{\cal U}}
\newcommand\M{{\cal M}}
\newcommand\Set{{\mathbf Set}}
\newcommand\Varset{{\mathbf Varset}}
\newcommand\univ{\mbox{$\mathbf U$}}
\newcommand\univind{{\mathbf U}}
\newcommand\skesig{\mbox{$\Sigma$}}

%%%% macro\Skesig.tex %%%%  June 29

\newcommand\mrkid{\mrk{ID}}
\newcommand\imID{\mbox{ID?}} %$^*$}}
\newcommand\mrkidd{\imID} % marker of IDDeficient
\newcommand\prodid{\mbox{$\times$-\ider}}
\newcommand\plusid{\mbox{$+$-\ider}}
\newcommand\prodkey{\mbox{$\times$-key}}
\newcommand\pluskey{\mbox{$+$-key}}

\newcommand\ID{\mrk{ID}}
\newcommand\IDplus{\mrk{ID$^+$}}
\newcommand\IDprod{\mrk{ID$^\times$}}

\newcommand\andiden{\emph{and}-\iden}
\newcommand\oriden{\emph{or}-\iden}


\newcommand\ssta{\mbox{${\mathsf S}_{\mathrm sta}$}}
\newcommand\sdyn{\mbox{${\mathsf S}_{\mathrm dyn}$}}

%\newcommand\mrk[1]{\mbox{[${\tt #1}$]}}
%\newcommand\mrk[1]{\mbox{[${\mathbf{#1}}$]}}
%\newcommand\mrkop[1]{\mbox{$\langle{\tt #1}\rangle$}}
\newcommand\mrkop[1]{\mbox{$\langle{\mathbf{#1}}\rangle$}}
\newcommand\mrkopr[1]{\mbox{$\mathbf{[{#1}\rangle}$}}
\newcommand\mrkopl[1]{\mbox{$\mathbf{\langle{#1}]}$}}
\newcommand\mrksemiop[1]{\mbox{$\langle{\tt #1}]$}}
\newcommand\mrkNode[1]{\mbox{${\tt #1}$}}
\newcommand\mrkn[1]{\mrkNode{#1}}
\newcommand\mrktt[1]{{\tt #1}}
\newcommand\mrkopright[1]{\mbox{$[${\tt #1}$\rangle$}}
\newcommand\mrkopleft[1]{\mbox{$\langle${\tt #1}$]$}}
%%%%%%%%%%%%%  Begin Key commands %%%%%%%%%%%%%%%%%%%%%%%

\newcommand\PredicateSignature{\Pi}
\newcommand\OperationSignature{\Sigma}
\newcommand\predFromOperSig{\Sigma_{pr}}
\newcommand\BaseSignature{\bf B}
\newcommand\DomainBase{\bf B}

\newcommand\ConstraintLanguage{CL}
\newcommand\dolan%DomainLanguage{\Delta}
{\mbox{$\Delta $}}

\newcommand\dolanm{\Delta}

\newcommand\adtm{ADT}
\newcommand\adt{{\sl \adtm}}
\newcommand\dolanadt{\dolan_{\adtm}}
\newcommand\sigadt{{\it Sig}_{\adtm}}
\newcommand\semmadt{\semm{}_{\adtm}}

\newcommand\dbauxm{DBD}
\newcommand\dbaux{{\sl \dbauxm}}
\newcommand\dolandbaux{\dolan_{\dbauxm}}
\newcommand\sigdbaux{{\it Sig}_{\dbauxm}}
\newcommand\semmdbaux{\semm{}_{\dbauxm}}

\newcommand\ba{D}
\newcommand\domba{\mbox{$\Domain(\ba)$}}
\newcommand\bam{\BasicDomainMarkerSymbol}          %  B  for using in math mode
%\newcommand\V{\mbox{$\TheValueUniverse_{\dolanm}$}}%

\newcommand\Pred{{\it Pred}}
\newcommand\Oper{{\it Op}}
\newcommand\Base{{\it Base}}
\newcommand\Dom{{\it Dom}}
\newcommand\Domain{{\it Dom}}
\newcommand\pool{V}

\newcommand\ArityMap{{\it Shp}}
\newcommand\ArityGraph{D}
\newcommand\AritySketch{{\cal D}}
\newcommand\ArityInclusion{\mbox{\Large $\iota$}}

\newcommand\rms{\rm\scriptsize}   % for writing, eg, \D^{\rms in}

\newcommand\PredicateMarkerSymbol{P}
\newcommand\OperationMarkerSymbol{F}
\newcommand\BasicDomainMarkerSymbol{B}

\newcommand\PredicateDiagramSet[1]{\PredicateMarkerSymbol^{#1}}%P^#1}
\newcommand\OperationDiagramSet[1]{\OperationMarkerSymbol^{#1}}%F^#1}
\newcommand\BasicDomainDiagramSet[1]{\BasicDomainMarkerSymbol^{#1}}%B^#1}

\newcommand\AGraph{G}
\newcommand\g{\mbox{$\AGraph$}}
\newcommand\gm{\AGraph}

\newcommand\ASketchSymbol{S}
\newcommand\ASketch{\mathsf \ASketchSymbol}
\newcommand\s{\mbox{$\ASketch$}}
\newcommand\sind{\ASketch}
\newcommand\sm{\ASketch}
\newcommand\sprim{\mbox{$\ASketch'$}}
\newcommand\sbipr{\mbox{$\ASketch''$}}


\newcommand\TheUniverseSymbol{U}
\newcommand\TheUniverseSketch{\cal \TheUniverseSymbol}
\newcommand\TheObjectUniverse{Obj }%{\cal O}
\newcommand\TheTimeUniverse{\cal T}%{T}
\newcommand\TheHistoryUniverse{\cal \TheTimeUniverse^*}%}
\newcommand\TheValueUniverse{Val}%{\cal V}

\newcommand\ASketchAlgebra{\cal A}
\newcommand\ABaseSubSketch{\cal B}    % base subsketch of

\newcommand\APermutation{\pi}

%===================================================

\newcommand\Mod[1]{\mbox{{\bf Mod}$(#1)$}}
\newcommand\Ext[1]{\mbox{{\bf Ext}$(#1)$}}
\newcommand\Inst[1]{\mbox{{\bf Inst}$(#1)$}}

%%%%%%%%%%%%%   End Key commands %%%%%%%%%%%%%%%%%


%%%%%%%%%%%%    Useful Abbreviations %%%%%%%%%%%%

%%% Sketchi


\newcommand\sdom{\mbox{$\s_{\DomainBase}$}}
\newcommand\sdomm{\s_{\DomainBase}}

\newcommand\newb{\mbox{$\DomainBase$}}
\newcommand\bm{\DomainBase}

\newcommand{\bs}{\mbox{$\ABaseSubSketch$}}
\newcommand\bsm{\ABaseSubSketch}

\newcommand\skespe{{\bf \ASketchSymbol}}

\newcommand\gras{{\it Gra}\skeob}
\newcommand\doms{{\it Dom}\skeob}
\newcommand\clas{{\it Cla}\skeob}
\newcommand\rels{{\it Rel}(\skeob)}

\newcommand\R{\nicex{ R$}}
\newcommand\OO{\mbox{$\TheObjectUniverse$}}
%\newcommand\T{\mbox{$\TheTimeUniverse$}}
%\newcommand\Hist{\mbox{$\TheHistoryUniverse}}
%\newcommand\V{\mbox{$\TheValueUniverse_{\bm}$}}%

\renewcommand\u{\mbox{$\TheUniverseSketch$}}
\newcommand\um{\TheUniverseSketch}
\newcommand\upred{\mbox{$\TheUniverseSketch_{\predsigm}$}}
\newcommand\uoper{\mbox{$\TheUniverseSketch_{\opersigm}$}}

\newcommand\predsig{\mbox{$\PredicateSignature$}}
\newcommand\predsigm{\PredicateSignature}
\newcommand\opersig{\mbox{$\OperationSignature$}}
\newcommand\opersigm{\OperationSignature}
\newcommand\predopsig{\mbox{$\predFromOperSig$}}
%\newcommand\pros{\predopsig}
\newcommand\prosm{\predFromOperSig}
\newcommand\basesig{\mbox{\BaseSignature}}
\newcommand\basesigm{{\BaseSignature}}
\newcommand\clan{\mbox{$\ConstraintLanguage$}}
\newcommand\clanm{\ConstraintLanguage}
\newcommand\colan{\mbox{\ConstraintLanguage}}
\newcommand\clanform{\mbox{$\ConstraintLanguage=(\Pred,\arimap,\semm{})$}}
\newcommand\colanm{\ConstraintLanguage}
%\newcommand\dolan{\mbox{\DomainLanguage}}
%\newcommand\dolanm{\DomainLanguage}

\newcommand\pis{$\PredicateSignature $-sketch}
\newcommand\sis{$\OperationSignature $-sketch}
\newcommand\siprs{$\predFromOperSig$-sketch}
\newcommand\sia{$\OperationSignature $-algebra}
\newcommand\clans{$\Constraint Language$-sketch}

\newcommand\arimap{\ArityMap}
\newcommand\arimapin{\mbox{\ArityMap$^{\rms in}$}}

\newcommand\os{\mbox{$\overline{\s}$}}
%\newcommand\go{\mbox{$G_{({\cal O})}$}}

\newcommand\pip{\mbox{$\APermutation^{+}$}}
\newcommand\depipComp{\mbox{$\delta \comp\APermutation^{+}$}}
\newcommand\depip{\mbox{$\APermutation^{+}\delta $}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%                                  %%%%%%%%%%%%%%%%%
%%%%%%%%%%            A R I T I E S         %%%%%%%%%%%%%%%%%%
%%%%%%%%%%                                  %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\pr{\mbox{$\PredicateMarkerSymbol$}}  % $P$ for using in text mode
\newcommand\op{\mbox{$\OperationMarkerSymbol$}}  % $F$ for using in text mode
%\newcommand\ba{\mbox{$\BasicDomainMarkerSymbol$}}  % $P$ for using in text mode


\newcommand\myprm{\PredicateMarkerSymbol}        %  P  for using in math mode
\newcommand\opm{\OperationMarkerSymbol}          %  F  for using in math mode
%\newcommand\bam{\BasicDomainMarkerSymbol}       %  B  for using in math mode

%%%%   functions to put the arg
%%%%   as subindex near \pr,\op and \ba

\newcommand\prix[1]{\myprm_{#1}}
\newcommand\opix[1]{\opm_{#1}}
\newcommand\baix[1]{\bam_{#1}}

%%%----  end functions

\newcommand\pri{$\myprm_{i}$}    %  \pr_i for using in text mode
\newcommand\opi{$\opm_{j}$}      %  \op_j for using in text mode
\newcommand\bai{$\bam_{l}$}      %  \ba_l for using in text mode

\newcommand\prim{\myprm_{i}}     %  \pr_i for using in math mode
\newcommand\opim{\opm_{j}}       %  \op_j for using in math mode
\newcommand\baim{\bam_{l}}       %  \ba_l for using in text mode
%======================================
%  eto makrosy funcciy
\renewcommand\Pr[1]{\PredicateDiagramSet{#1}}  % P^#1
\newcommand\Op[1]{\OperationDiagramSet{#1}}    % F^#1
\newcommand\Ba[1]{\BasicDomainDiagramSet{#1}}  % B^#1
%  a eto ih znacheniya
\newcommand\PrS{\Pr{\s}}      % P^\s
\newcommand\OpS{\Op{\s}}      % F^\s
\newcommand\BaS{\Ba{\s}}      % B^\s
%\newcommand\domba{$\Domain(\ba)$}

\newcommand\PrU{\Pr{\u}}      % P^\u
\newcommand\OpU{\Op{\u}}      % F^\u
\newcommand\BaU{\Ba{\u}}      % B^\u

%------------------------------------------------
% eto makrosy funkciy s 2 argumwntami
\newcommand\Prix[2]{\Pr{#1}_{#2}}              % a set P^#1_#2
\newcommand\Opix[2]{\Op{#1}_{#2}}              % a set F^#1_#2
\newcommand\Baix[2]{\Ba{#1}_{#2}}              % a set B^#1_#2
% a eto b nih podstavleny indexy i ostalsya 1 argument
\newcommand\Pri[1]{$\Prix{#1}{i}$}             % a set og diag, P^#1_i
\newcommand\Opi[1]{$\Opix{#1}{j}$}             % a set of diag, F^#1_j
\newcommand\Bai[1]{$\Baix{#1}{l}$}             % a set of diag, B^#1_l
% a eto znacheniya
\newcommand\PriS{\Pri{\s}}      % Pi^\s
\newcommand\OpiS{\Opi{\s}}      % Fj^\s
\newcommand\BaiS{\Bai{\s}}      % Bl^\s

\newcommand\PriU{\Pri{\u}}      % Pi^\u
\newcommand\OpiU{\Opi{\u}}      % Fj^\u
\newcommand\BaiU{\Bai{\u}}      % Bl^\u

%  a eto dlya mat mode
\newcommand\Prim[1]{\Prix{#1}{i}}     %  a set of diagr,  P^#1_i for using in math mode
\newcommand\Opim[1]{\Opix{#1}{j}}     %  a set of diagr,  F^#1_j for using in math mode
\newcommand\Baim[1]{\Baix{#1}{l}}     %  a set of diagr,  B^#1_#2 for using in math mode
%====================================================

%\newcommand\pool{V}
\newcommand\vx[1]{\mbox                                  % D_arg
                      {$\pool_{#1}$}}
\newcommand\vinx[1]{\mbox                                % D^in_arg
                      {$\pool^{\mbox\rms in}_{#1}$}}
\newcommand\voutx[1]{\mbox                               % D^out_arg
                      {$\pool^{\mbox\rms out}_{#1}$}}
%============================================================

%\newcommand\ArityGraph{D}
%\newcommand\AritySketch{\D}                             % \D - nice D
\newcommand\sprx[1]{\mbox                                %  D_arg
                      {$\ArityGraph_{#1}$}}
\newcommand\sopx[1]{\mbox                                % \D_arg
                      {$\AritySketch_{#1}$}}
\newcommand\sinx[1]{\mbox                                % \D^in_arg
                      {$\AritySketch^{\rms in}_{#1}$}}
\newcommand\soutx[1]{\mbox                               % \D^out_arg
                      {$\AritySketch^{\rms out}_{#1}$}}

%-----   marker-subindex version
\newcommand\spr{\sprx{\myprm}}         %  D_{prop marker}
\newcommand\sop{\sopx{\opm}}         % \D_{oper marker}
\newcommand\sinop{\sinx{\opm}}       % \D^in_{oper mark}
%-----   i-subindex version
\newcommand\spri{\sprx{i}}          %  D_{i}
\newcommand\sopi{\sopx{j}}          % \D_{j}
\newcommand\sinopi{\sinx{j}}        % \D^in_{j}



\newcommand\opshaxy[2]{\inclar{#1_{#2}}  % arg1_arg2: D^in_arg2 -->D_arg2
                            {\sinx{#2}}
                              {\sopx{#2}}
                       }
%\newcommand\ArityInclusion{i}
\newcommand\opsha{\opshaxy{\ArityInclusion}{\opm}}   %i_f: D^in_f   --> D_f
\newcommand\opshai{\opshaxy{\ArityInclusion}{\opim}} %i_f: D^in_f_j --> D_f_j

%----------------------------------------

%\newcommand\ArityMap{{\it Shp}}
\newcommand\arix[1]{\mbox
                        {$\ArityMap({#1})$}}         % Shp(arg)
\newcommand\ariinx[1]{\mbox
                        {$\ArityInclusion_{#1}$}}    % \iota_{arg}

\newcommand\aripr{\arix{\myprm}}                  % Shp(p)
\newcommand\ariop{\arix{\opm}}                  % Shp(f)
\newcommand\arinc{\ariinx{\opm}}                % \iota_f

\newcommand\aripri{\arix{\prim}}                % Shp(p_i)
\newcommand\ariopi{\arix{\opim}}                % Shp(f_j)
\newcommand\arinci{\ariinx{\opim}}              % \iota_j

%-----------------------------------------
\newcommand\sepr{\semm{\pr}}
\newcommand\seop{\semm{\op}}
\newcommand\sepri{\semm{\pri}}
\newcommand\seopi{\semm{\op}}


\newcommand\opv{\mbox{\Oper$^+$}}

%\endinput

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%              %%%%%%%%%%%%%%%
%%%%%%%%%%%  Old Macros %%%%%%%%%%%%%%%%
%%%%%%%%%%              %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\newcommand\sig{\mbox{$\PredicateSignature$}}
%\newcommand\gra{{\bf G}}
%\newcommand\sigo{\mbox{$\Sigma_1$}}
%\newcommand\grao{\mbox{${\bf G}_1$}}
%% OOPS! \newcommand\inst{\mbox{$\lar{\vare }{S}{W}$}}
%%\newcommand\sch{\Category{Schema} }
%
%
%\newcommand\instVareps{\mbox{$\lar{\vare }{S}{W}$}}
%\newcommand\inste{\mbox{$\lar{e}{S}{W}$}}
%\newcommand\emor[1]{\lar{e}{#1}{\u}}
%\newcommand\sv{\mbox{$S_V$}}
%\newcommand\sr{\mbox{$S_R$}}
%\newcommand\vmor{\lar{v}{\sv}{\ovrs{}}}
%\newcommand\rmor{\lar{r}{S}{\ovrs{R}}}
%\newcommand\vpair{\mbox{$V=(\sv,v)$}}
%\newcommand\rpair{\mbox{$R=(\sr,r)$}}
%===
%==== Varset
%% macros for writing formulas with varsets and varfunctions

%%%%%%%%%    ..\dke96\macro\varset.tex    %%%%%%%
%\renewcommand\c{\mbox{$\AClass$}}                    %   C
%\newcommand\cm{\AClass}                              %   C
%\newcommand\ce{\mbox{$\semm{\AClass}$}}              % ||C||

%\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}   % ||C||^#1

%\newcommand\cindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
% apply:
%\newcommand\cet{\ceind{\ltt}}                         % ||C||^t
%\newcommand\ceu{\ceind{\ltu}}                         % ||C||^u
\newcommand\ObjStt{\ittt{ObjStt}}
\newcommand\C{\textit{C}}
\newcommand\D{\textit{D}}

\newcommand\ot[1]{\mbox{$o^{\ltt_{#1}}$}}
\newcommand\otm{o^\ltt}
\newcommand\ou[1]{\mbox{$o^{\ltu_{#1}}$}}
\newcommand\otu{o^\ltu}

\newcommand\cet{\mbox{$\semm{C}^{\ltt}$}}                         % ||C||^t
\newcommand\ceti{\mbox{$\semm{C}^{\ltt_i}$}}                         % ||C||^t
\newcommand\ceu{\mbox{$\semm{C}^{\ltu}$}}                         % ||C||^t
\newcommand\ceprt{\mbox{$\sempr{C}^{\ltt}$}}                         % ||C||^t
\newcommand\cepru{\mbox{$\sempr{C}^{\ltu}$}}                         % ||C||^t


\newcommand\cetu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\AClass}^{\ltu}$}}
\newcommand\ceut{\mbox{$\vphantom{\semm{AClass}}^{\ltu}\!\semm{\AClass}^{\ltt}$}}
\newcommand\detu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass}^{\ltu}$}}
\newcommand\fetu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass_f}^{\ltu}$}}
\newcommand\djetu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass_j}^{\ltu}$}}
\newcommand\dietu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass_i}^{\ltu}$}}
\newcommand\deut{\mbox{$\vphantom{\semm{AClass}}^{\ltu}\!\semm{\TargetClass}^{\ltt}$}}
\newcommand\ceprtu{\mbox{$\vphantom{\sempr{AClass}}^{\ltt}\sempr{\AClass}^{\ltu}$}}
\newcommand\deprtu{\mbox{$\vphantom{\sempr{AClass}}^{\ltt}\sempr{\TargetClass}^{\ltu}$}}



\newcommand\cesu{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\AClass}^{\ltu}$}}
\newcommand\cest{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\AClass}^{\ltt}$}}
\newcommand\cett{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\AClass}^{\ltt}$}}

\newcommand\dest{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\TargetClass}^{\ltt}$}}
\newcommand\desu{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\TargetClass}^{\ltu}$}}

\newcommand\cestart{\mbox{${\semmstar{C}}^{\ltt}$}}                         % ||C||^t
\newcommand\cestaru{\mbox{${\semmstar{C}}^{\ltu}$}}                         % ||C||^t
\newcommand\cestartu{\mbox{${}^{\ltt}{\semmstar{C}}^{\ltu}$}}

\newcommand\ceto{\mbox{$\semm{\AClass}^{\ltt}_{o}$}}
\newcommand\ceuo{\mbox{$\semm{\AClass}^{ \ltu}_{o}$}}

\newcommand\cestarto{\mbox{${\semmstar{\AClass}}^{\ltt}_{o}$}}
\newcommand\cestaruo{\mbox{${\semmstar{\AClass}}^{ \ltu}_{o}$}}

%======================================================================

%  ----  Basic Command -----------

\newcommand\LogicalTime{\cal T}
\newcommand\SetOfHistories{\LogicalTime^*}
\newcommand\AHistory{H}%J}

%\newcommand\IndexingXupYdownZ[3]{\mbox{$#1^{#2}_{#3}$}}
%\newcommand\IntRelSymb{\varepsilon}%rho}
%\newcommand\IntRelSymb{\mbox{\Large$\iota$}}%rho}
%\newcommand\IntersttMap{\mbox{\ittt same}}%rho}

\newcommand\AClass{C}
\newcommand\SourceClass{C}
\newcommand\TargetClass{D}
\newcommand\e{E}
\newcommand\AReference{f}
\newcommand\AnotherReference{g}
%\newcommand\Identifier{\mbox{\Large$\iota$}}
\renewcommand\g{g}
%\newcommand\h{h}
%\newcommand\hind{h}


\newcommand\farr{\lar{\AReference}{\SourceClass}{\TargetClass}}
\newcommand\farris{\lar{\AReference_i}{\SourceClass}{\TargetClass_i}}
\newcommand\farrit{\lar{\AReference_i}{\SourceClass_i}{\TargetClass}}
\newcommand\ffams{\mbox{$\f=\famm{\farris}{i\in I}$}}
\newcommand\ffamt{\mbox{$\f=\famm{\farrit}{i\in I}$}}

\newcommand\garr{\lar{\AnotherReference}{\SourceClass}{\TargetClass}}
\newcommand\garrit{\lar{\AnotherReference_i}{\SourceClass}{\TargetClass_i}}
\newcommand\garris{\lar{\AnotherReference_i}{\SourceClass_i}{\TargetClass} }
\newcommand\gfams{\mbox{$\g=\famm{\garris}{i\in I}$}}
\newcommand\gfamt{\mbox{$\g=\famm{\garrit}{i\in I}$}}


\newcommand\iarr{\lar{\AReference}{\SourceClass}{\TargetClass}}
\newcommand\iarris{\lar{\Identifier_j}{\SourceClass}{\TargetClass_j}}
\newcommand\iarrit{\lar{\Identifier_j}{\SourceClass_j}{\TargetClass} }
\newcommand\ifams{\mbox{$\Identifier=\famm{\iarris}{j\in J}$}}
\newcommand\ifamt{\mbox{$\Identifier=\famm{\iarrit}{j\in J}$}}


\newcommand\AMoment{t}%j}
\newcommand\EarlierMoment{t}%j}
\newcommand\LaterMoment{u}%k}
\newcommand\EarlierEarlierMoment{s}%i}
\newcommand\LaterLaterMoment{v}%l}

\newcommand\ttt{t1,t2}

\newcommand\IndexingXupYdownZ[3]{\mbox{$#1^{#2}_{#3}$}}

%%%%%%%%%%%%%%%%%%%%%%
% -- Abbreviations ----
%%%%%%%%%%%%%%%%%%%%%%%%%%                    sket}}


\newcommand\T{\mbox{$\LogicalTime$}}
\newcommand\Tm{\LogicalTime}
\newcommand\Hist{\mbox{$\SetOfHistories$}}
\newcommand\Histm{\SetOfHistories}
\newcommand\IntersttMap{\mbox{\ittt{same}}}%rho}
\newcommand\same[2]{\mbox{$\IntersttMap^{#1}_{#2}$}}
\newcommand\inter[2]{\same{#1}{#2}}
\newcommand\interpr[2]{\mbox{$\mytilde\IntersttMap^#1_#2$}}
% \IndexingXupYdownZ{\IntRelSymb}{#1}{#2}}  %\vare^#1_#2
%\newcommand\interpr[2]%
%      {\IndexingXupYdownZ{\mytilde{\IntRelSymb}}{#1}{#2}}  %\vare^#1_#2

%%% The new version t is denoted by \ltt, u is denoted by  \ltu etc

\newcommand\ttu{\EarlierMoment\LaterMoment}   %tu
\newcommand\logtimet{\EarlierMoment}               %t
\newcommand\ltt{\EarlierMoment}               %t
%\newcommand\tu{\LaterMoment}                  %u
\newcommand\ltu{\LaterMoment}                  %u
\newcommand\ttlu{\mbox{$\ltt\le\ltu$}}         % t =< u
\newcommand\tleu{\mbox{$\ltt\le\ltu$}}         % t =< u
\newcommand\tlu{\mbox{$\ltt<\ltu$}}            % t < u
\newcommand\logtimes{\EarlierEarlierMoment}        %s
\newcommand\lts{\EarlierEarlierMoment}               %t
\newcommand\ltv{\LaterLaterMoment}             %l
\newcommand\tv{\LaterLaterMoment}             %l

\newcommand\J{\AHistory}                      %J

\newcommand\intertu[1]{\inter{\ltt\to\ltu}{#1}}       % \eps^tu_#1
\newcommand\interut[1]{\inter{\ltt\gets\ltu}{#1}}       % \eps^tu_#1
\newcommand\intertuut[1]{\inter{\ltt\leftrightarrow\ltu}{#1}}       % \eps^tu_#1

\newcommand\intertt[1]{\inter{\ltt\to\ltt}{#1}}                 % \eps^tu_#1

\newcommand\interst[1]{\inter{\lts\to\ltt}{#1}}       % \eps^tu_#1
\newcommand\interts[1]{\inter{\lts\gets\ltt}{#1}}       % \eps^tu_#1

\newcommand\intersu[1]{\inter{\lts\to\ltu}{#1}}       % \eps^tu_#1
\newcommand\interus[1]{\inter{\ltu\gets\lts}{#1}}       % \eps^tu_#1

%\newcommand\interst[1]{\inter{\lts\to\ltt}{#1}}                 % \eps^tu_#1
%\newcommand\intersu[1]{\inter{\lts\to\ltu}{#1}}                 % \eps^tu_#1

\newcommand\domintertu[1]{\ldom{\intertu{#1}}}  %\Box\eps^tu_#1
\newcommand\codintertu[1]{\rdom{\intertu{#1}}}  %\eps^tu_#1\Box

\newcommand\sametuut[1]{\mbox{$\same{\ltt\leftrightarrow\ltu}{#1}$}}       % \eps^tu_#1
\newcommand\sametu[1]{\mbox{$\same{\ltt\to\ltu}{#1}$}}       % \eps^tu_#1
\newcommand\sameut[1]{\mbox{$\same{\ltt\gets\ltu}{#1}$}}       % \eps^tu_#1
\newcommand\samectu{\mbox{$\same{\ltt\to\ltu}{\cm}$}}       % \eps^tu_#1
\newcommand\samecut{\mbox{$\same{\ltt\gets\ltu}{\cm}$}}       % \eps^tu_#1
\newcommand\samedtu{\mbox{$\same{\ltt\to\ltu}{\dm}$}}       % \eps^tu_#1
\newcommand\samedut{\mbox{$\same{\ltt\gets\ltu}{\dm}$}}       % \eps^tu_#1

\newcommand\samett[1]{\same{\ltt\to\ltt}{#1}}                 % \eps^tu_#1

\newcommand\samest[1]{\same{\lts\to\ltt}{#1}}       % \eps^tu_#1
\newcommand\samets[1]{\same{\lts\gets\ltt}{#1}}       % \eps^tu_#1
\newcommand\samecst{\same{\lts\to\ltt}{\cm}}       % \eps^tu_#1
\newcommand\samects{\same{\lts\gets\ltt}{\cm}}       % \eps^tu_#1
\newcommand\samedst{\same{\lts\to\ltt}{\dm}}       % \eps^tu_#1
\newcommand\samedts{\same{\lts\gets\ltt}{\dm}}       % \eps^tu_#1



\newcommand\samesu[1]{\same{\lts\to\ltu}{#1}}       % \eps^tu_#1
\newcommand\sameus[1]{\same{\ltu\gets\lts}{#1}}       % \eps^tu_#1

%\newcommand\samest[1]{\same{\lts\to\ltt}{#1}}                 % \eps^tu_#1
%\newcommand\samesu[1]{\same{\lts\to\ltu}{#1}}                 % \eps^tu_#1

\newcommand\domsametu[1]{\ldom{\sametu{#1}}}  %\Box\eps^tu_#1
\newcommand\codsametu[1]{\rdom{\sametu{#1}}}  %\eps^tu_#1\Box


%  Apply:
\newcommand\interctt{\inter{\ltt\to\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\intercst{\inter{\lts\to\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\interctu{\inter{\ltt\to\ltu}{\cm}}                 % \eps^tu_#1
\newcommand\intercsu{\inter{\lts\to\ltu}{\cm}}                 % \eps^tu_#1

\newcommand\intercut{\inter{\ltt\leftarrow\ltu}{\cm}}                 % \eps^tu_#1

\newcommand\interprctt{\interpr{\ltt\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\interprcst{\interpr{\lts\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\interprctu{\interpr{\ltt\ltu}{\cm}}                 % \eps^tu_#1
\newcommand\interprcsu{\interpr{\lts\ltu}{\cm}}                 % \eps^tu_#1

\newcommand\dominterctu{\domintertu{\cm}}  %\Box\eps^tu_#1
\newcommand\codinterctu{\codintertu{\cm}}  %\eps^tu_#1\Box

%----------------------------------------------
%% Classes and arrows
%-------------------------------------------------

%\renewcommand\c{\mbox{$\AClass$}}                    %   C
\newcommand\cm{\AClass}                              %   C
\newcommand\ce{\mbox{$\semm{\AClass}$}}              % ||C||

%--- function:
\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}   % ||C||^#1

\newcommand\cindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
% apply:
%\newcommand\cet{\mbox{$\semm{C}^{\ltt}$}}                         % ||C||^t
%\newcommand\ceu{\mbox{$\semm{C}^{\ltu}$}}                         % ||C||^t
%\newcommand\cetu{\mbox{${}^{\ltt}\semm{\AClass}^{\ltu}$}}
\newcommand\ces{\ceind{\lts}}                         % ||C||^u
\newcommand\cev{\ceind{\tv}}                         % ||C||^u


\newcommand\ceJ{\ceind{\J}}

\newcommand\objeq[2]{\simeq^{#1}_{#2}}
\newcommand\eqJ[1]{\objeq{\J}{#1}}

\newcommand\ciet{\cindeind{i}{\ltt}}                         % ||C_i||^t
\newcommand\ctet{\cindeind{t}{\ltt}}                         % ||C_t||^t
\newcommand\cjet{\cindeind{j}{\ltt}}                         % ||C_i||^t
\newcommand\cket{\cindeind{k}{\ltt}}                         % ||C_t||^t
\newcommand\clet{\cindeind{l}{\ltt}}                         % ||C_i||^t


\newcommand\cieJ{\ceind{\J}}
%\newcommand\cjeJ{\ceind{\J}}

% function:
\newcommand\cind[1]{\mbox{$\AClass^{#1}$}}           %      C^#1
\newcommand\cindl[2]{\mbox{$_{#1}\AClass^{#2}$}}     % _{#1}C^{#2}
\newcommand\cindr[2]{\mbox{$\AClass_{#1}^{#2}$}}     %      C_{#1}^{#2}

%\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}           %      C^#1
\newcommand\ceindl[2]{\mbox{$_{#1}\semm{\AClass}^{#2}$}}     % _{#1}C^{#2}
\newcommand\ceindr[2]{\mbox{$\semm{\AClass}_{#1}^{#2}$}}     %      C_{#1}^{#2}

%  apply:
\newcommand\ctu{\mbox{$^{\ltt}\!\AClass^{\ltu}$}}
\newcommand\ctplusu{\cindr{+\ltu}{\ltt}}
\newcommand\ctnullu{\cindr{0\ltu}{\ltt}}
\newcommand\cuminust{\cindl{-\ltt}{\ltu}}
\newcommand\cunullt{\cindl{0\ltt}{\ltu}}

%\newcommand\cetu{\cind{\ltt\ltu}}
\newcommand\cetplusu{\ceindr{+\ltu}{\ltt}}
\newcommand\cetnullu{\ceindr{0\ltu}{\ltt}}
\newcommand\ceuminust{\ceindl{-\ltt}{\ltu}}
\newcommand\ceunullt{\ceindl{0\ltt}{\ltu}}

% the same for D

%\renewcommand\d{\mbox{$\TargetClass$}}                    %   D
\newcommand\dm{\TargetClass}                              %   D

\newcommand\de{\mbox{$\semm{\TargetClass}$}}              % ||D||
\newcommand\deind[1]{\mbox{$\semm{\TargetClass}^{#1}$}}   % ||D||^#1
\renewcommand\det{\deind{\ltt}}                         % ||C||^t
\newcommand\deu{\deind{\ltu}}                         % ||C||^u
\newcommand\des{\deind{\lts}}                         % ||C||^u
\newcommand\dev{\deind{\tv}}                         % ||C||^u

\newcommand\deJ{\deind{\J}}

\newcommand\dindeind[2]{\mbox{$\semm{\TargetClass_{#1}}^{#2}$}}
%  apply
\newcommand\dies{\dindeind{i}{\lts}}                         % ||C||^t
\newcommand\djet{\dindeind{j}{\ltt}}                         % ||C||^t
\newcommand\djeu{\dindeind{j}{\ltu}}                         % ||C||^t
%\newcommand\djetu{\dindeind{j}{\ltt}}                         % ||C||^t
\newcommand\dieJ{\deind{\J}}
\newcommand\djeJ{\deind{\J}}
\newcommand\diet{\dindeind{i}{\ltt}}                         % ||C||^t
\newcommand\dieu{\dindeind{i}{\ltu}}                         % ||C||^t
%\newcommand\djetu{\dindeind{j}{\ltt}}                         % ||C||^t


\newcommand\dind[1]{\mbox{$\TargetClass^{#1}$}}           %      C^#1
\newcommand\dindl[2]{\mbox{$_{#1}\TargetClass^{#2}$}}     % _{#1}D^{#2}
\newcommand\dindr[2]{\mbox{$\TargetClass_{#1}^{#2}$}}     %      D_{#1}^{#2}

%\newcommand\deind[1]{\mbox{$\semm{\TargetClass}^{#1}$}}           %      C^#1
\newcommand\deindl[2]{\mbox{$_{#1}\semm{\TargetClass}^{#2}$}}     % _{#1}D^{#2}
\newcommand\deindr[2]{\mbox{$\semm{\TargetClass}_{#1}^{#2}$}}     %      D_{#1}^{#2}


% apply
\newcommand\dtu{\mbox{$^{\ltt}\!\TargetClass^{\ltu}$}}
\newcommand\detplusu{\deindr{+\ltu}{\ltt}}
\newcommand\detnullu{\deindr{0\ltu}{\ltt}}
\newcommand\deuminust{\deindl{-\ltt}{\ltu}}
\newcommand\deunullt{\deindl{0\ltt}{\ltu}}


%\newcommand\f{\mbox{$\AReference$}}                    %   f
\newcommand\fm{\AReference}                              %   f
%\newcommand\find[1]{\mbox{$\AReference^{#1}$}}           %      f^#1
%\newcommand\findl[2]{\mbox{$_{#1}\AReference^{#2}$}}     % _{#1}C^{#2}
%\newcommand\findr[2]{\mbox{$\AReference_{#1}^{#2}$}}     %      C_{#1}^{#2}

\newcommand\feind[1]{\mbox{$\semm{\AReference}^{#1}$}}           %      f^#1
\newcommand\feindl[2]{\mbox{$_{#1}\semm{\AReference}^{#2}$}}     % _{#1}C^{#2}
\newcommand\feindr[2]{\mbox{$\semm{\AReference}_{#1}^{#2}$}}     %      C_{#1}^{#2}

\newcommand\ftu{\find{\ttu}}

\newcommand\fe{\mbox{$\semm{\AReference}$}}              % ||f||
\renewcommand\feind[1]{\mbox{$\semm{\AReference}^{#1}$}}   % ||f||^#1
\newcommand\fet{\feind{\ltt}}
\newcommand\fes{\feind{\lts}}
\newcommand\feu{\feind{\ltu}}
\newcommand\fev{\feind{\tv}}
\newcommand\feJ{\feind{\J}}

\newcommand\femt{\mbox{$\semm{\AReference^{-1}}^{\ltt}$}}


\newcommand\findeind[2]{\mbox{$\semm{\AReference_{#1}}^{#2}$}}
\newcommand\fieu[1]{\findeind{#1}{\ltu}}
\newcommand\fiet[1]{\findeind{#1}{\ltt}}
\newcommand\fies[1]{\findeind{#1}{\lts}}                         % ||C||^t
%\newcommand\fiet{\findeind{i}{\ltt}}                         % ||C||^t
\newcommand\fjet{\findeind{j}{\ltt}}                         % ||C||^t
\newcommand\fket{\findeind{k}{\ltt}}                         % ||C||^t
\newcommand\flet{\findeind{l}{\ltt}}                         % ||C||^t
\newcommand\fkeu{\findeind{k}{\ltu}}                         % ||C||^t

\newcommand\fetplusu{\feindr{+\ltu}{\ltt}}
\newcommand\fetnullu{\feindr{0\ltu}{\ltt}}
\newcommand\feuminust{\feindl{-\ltt}{\ltu}}
\newcommand\feunullt{\feindl{0\ltt}{\ltu}}



%\newcommand\diet{\dindeind{i}{\ltt}}                         % ||C||^t
%\newcommand\djes{\dindeind{j}{\lts}}                         % ||C||^t

\newcommand\fieJ{\feind{\J}}
\newcommand\fjeJ{\feind{\J}}

\newcommand\fgcomp{\mbox{$\f(\g_1,\ldots,\g_m)$}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% The old version where \tj denotes t, \tk denotes u  etc
%%% The new version see on line 185

\newcommand\tjk{\EarlierMoment\LaterMoment}   %jk
\newcommand\tj{\EarlierMoment}               %j
\newcommand\tk{\LaterMoment}                  %k
\newcommand\tjlk{\mbox{$\tj\le\kt$}}
\newcommand\ti{\EarlierEarlierMoment}        %i
\newcommand\tl{\LaterLaterMoment}             %l

%\newcommand\J{\AHistory}                      %J

\newcommand\interjk[1]{\inter{\tjk}{#1}}                 % \eps^jk_#1
\newcommand\dominterjk[1]{\ldom{\interjk{#1}}}  %\Box\eps^jk_#1
\newcommand\codinterjk[1]{\rdom{\interjk{#1}}}  %\eps^jk_#1\Box

\newcommand\interjj[1]{\inter{\tj\tj}{#1}}                 % \eps^jk_#1
\newcommand\interij[1]{\inter{\ti\tj}{#1}}                 % \eps^jk_#1
%\newcommand\interjk[1]{\inter{\tj\tk}{#1}}                 % \eps^jk_#1
\newcommand\interik[1]{\inter{\ti\tk}{#1}}                 % \eps^jk_#1


\newcommand\intercjj{\inter{\tj\tj}{\cm}}                 % \eps^jk_#1
\newcommand\intercij{\inter{\ti\tj}{\cm}}                 % \eps^jk_#1
\newcommand\intercjk{\inter{\tj\tk}{\cm}}                 % \eps^jk_#1
\newcommand\intercik{\inter{\ti\tk}{\cm}}                 % \eps^jk_#1

\newcommand\domintercjk{\dominterjk{\cm}}  %\Box\eps^jk_#1
\newcommand\codintercjk{\codinterjk{\cm}}  %\eps^jk_#1\Box

\newcommand\interdjj{\inter{\tj\tj}{\dm}}                 % \eps^jk_#1
\newcommand\interdij{\inter{\ti\tj}{\dm}}                 % \eps^jk_#1
\newcommand\interdjk{\inter{\tj\tk}{\dm}}                 % \eps^jk_#1
\newcommand\interdik{\inter{\ti\tk}{\dm}}                 % \eps^jk_#1

%----------------------------------------------
%% Classes and arrows
%-------------------------------------------------

%\renewcommand\c{\mbox{$\AClass$}}                    %   C
%\newcommand\cm{\AClass}                              %   C

%\newcommand\ce{\mbox{$\semm{\AClass}$}}              % ||C||
%\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}   % ||C||^#1
\newcommand\cej{\ceind{\tj}}                         % ||C||^j
\newcommand\cek{\ceind{\tk}}                         % ||C||^k
%\newcommand\ceJ{\ceind{\J}}
%--- function:
%\newcommand\cindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
% apply:
\newcommand\ciej{\cindeind{i}{\tj}}                         % ||C_i||^j
\newcommand\cjej{\cindeind{j}{\tj}}                         % ||C_j||^j
\renewcommand\cieJ{\ceind{\J}}
\newcommand\cjeJ{\ceind{\J}}

% function:
%\newcommand\cind[1]{\mbox{$\AClass^{#1}$}}           %      C^#1
%\newcommand\cindl[2]{\mbox{$_{#1}\AClass^{#2}$}}     % _{#1}C^{#2}
%\newcommand\cindr[2]{\mbox{$\AClass_{#1}^{#2}$}}     %      C_{#1}^{#2}
%  apply:
\newcommand\cjk{\cind{\tj\tk}}
\newcommand\cjplusk{\cindr{+\tk}{\tj}}
\newcommand\cjnullk{\cindr{0\tk}{\tj}}
\newcommand\ckminusj{\cindl{-\tj}{\tk}}
\newcommand\cknullj{\cindl{0\tj}{\tk}}


% the same for D

%\renewcommand\d{\mbox{$\TargetClass$}}                    %   D
%\renewcommand\dm{\TargetClass}                              %   D

%\newcommand\de{\mbox{$\semm{\TargetClass}$}}              % ||D||

%\newcommand\deind[1]{\mbox{$\semm{\TargetClass}^{#1}$}}   % ||D||^#1
%\newcommand\dindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}

%\newcommand\dind[1]{\mbox{$\TargetClass^{#1}$}}           %      C^#1
%\newcommand\dindl[2]{\mbox{$_{#1}\TargetClass^{#2}$}}     % _{#1}D^{#2}
%\newcommand\dindr[2]{\mbox{$\TargetClass_{#1}^{#2}$}}     %      D_{#1}^{#2}



%  Apply:
\newcommand\dej{\deind{\tj}}                         % ||C||^j
\newcommand\dek{\deind{\tk}}                         % ||C||^k
%\newcommand\deJ{\deind{\J}}

\newcommand\diei{\dindeind{i}{\ti}}                         % ||C||^j
\newcommand\djej{\dindeind{j}{\tj}}                         % ||C||^j
%\newcommand\dieJ{\deind{\J}}
%\newcommand\djeJ{\deind{\J}}

\newcommand\djk{\dind{\tj\tk}}
\newcommand\djplusk{\dindr{+\tk}{\tj}}
\newcommand\djnullk{\dindr{0\tk}{\tj}}
\newcommand\dkminusj{\dindl{-\tj}{\tk}}
\newcommand\dknullj{\dindl{0\tj}{\tk}}


%\renewcommand\f{\mbox{$\AReference$}}                    %   f
%\newcommand\fm{\AReference}                              %   f
%\newcommand\find[1]{\mbox{$\AReference^{#1}$}}           %      f^#1
\newcommand\fjk{\find{\tjk}}

%\newcommand\fe{\mbox{$\semm{\AReference}$}}              % ||f||
%\newcommand\feind[1]{\mbox{$\semm{\AReference}^{#1}$}}   % ||f||^#1
\newcommand\fej{\feind{\tj}}
\newcommand\fei{\feind{\ti}}
\newcommand\fek{\feind{\tk}}
\newcommand\fel{\feind{\tl}}

%\newcommand\feJ{\feind{\J}}

%\newcommand\findeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
%\newcommand\diei{\dindeind{i}{\ti}}                         % ||C||^j
%\newcommand\djej{\dindeind{j}{\tj}}                         % ||C||^j
 \newcommand\fiei{\findeind{i}{\ti}}                         % ||C||^j
 \newcommand\fjej{\findeind{j}{\tj}}                         % ||C||^j
%\newcommand\fieJ{\feind{\J}}
%\newcommand\fjeJ{\feind{\J}}

%\newcommand\fgcomp{\mbox{$\f(\g_1,\ldots,\g_m)$}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\Distinctctu{\mbox{$^{\ltt}\!\semm{\ittt{Distinct}_{\cm}}^{\ltu}$}}
\newcommand\Distinctcst{\mbox{$^{\lts}\!\semm{\ittt{Distinct}_{\cm}}^{\ltt}$}}
\newcommand\Samectu{\mbox{$^{\ltt}\!\semm{\ittt{Same}_{\cm}}^{\ltu}$}}
\newcommand\Samecst{\mbox{$^{\lts}\!\semm{\ittt{Same}_{\cm}}^{\ltt}$}}
%=============
%%%%% Behset
\newcommand\xstatei[3]{\mbox{${\mathit {#1}state}^{#3}_{#2}$}}
\newcommand\statei[2]{\xstatei{}{#1}{#2}}
\newcommand\xstate[2]{\xstatei{#1}{}{#2}}
%\newcommand\tstatei[1]{\statei{#1}{\ltt}}

\newcommand\attrName[1]{{\mathit #1}}
\newcommand\methName[1]{{\mathit #1}}
\newcommand\statepoint[1]{#1}

%%%%%
% discussing string-based  vs graph-based logics
\newcommand\cmlang{{\bf L}}
\newcommand\myindex[1]{\mbox{\scriptsize{#1}}}
\newcommand\mathsymbol[1]{\mbox{$#1$}}
%\newcommand\repr{\mathsymbol{r}}
\newcommand\world%{\ittt{world}}
{\mathsymbol{\cal W}}
\newcommand\cmter%{\ittt{computer}}
{\mathsymbol{\cal C}}
\newcommand\topos{\mathsymbol{\cal S}}


%----------------------
\newcommand\viewob[1]{\object{V}{#1}}
\newcommand\thob[1]{\object{T}{#1}}
\newcommand\uniob[1]{\object{U}{#1}}
\newcommand\uniobmath[1]{\objectmath{U}{#1}}
\newcommand\uniobind[1]{\objectind{U}{#1}}

\newcommand\UNI{\universe{U}}
\newcommand\UNIind{\universeind{U}}
\newcommand\UNImath{\universeind{U}} % the same
\newcommand\Setsind{\universeind{Sets}}

\newcommand\particularUni[1]{\mbox{$\mathbf{#1}$}}
\newcommand\particularUniInd[1]{\mathbf{#1}}
\newcommand\Sets{\particularUni{Sets}}
\newcommand\Varsets{\particularUni{VarSets}}
\newcommand\Behsets{\particularUni{BehSets}}
\newcommand\Sketches{\particularUni{Sketches}}


\newcommand\skeproc{\proc{ske}}
\newcommand\arrdlproc{\procind{Formal}{ArrDL}}
\newcommand\elmslproc{\procind{Formal}{ElmSL}}

%\newcommand\formalPar[1]{\mbox{$\mathrm #1$}}
\newcommand\formalParBold[1]{\mbox{$#1$}}
\newcommand\lf{\formalParBold{L}}
\newcommand\mf{\formalPar{M(D)}}
\newcommand\uf{\formalPar{U}}
\newcommand\df{\formalPar{D}}
\newcommand\tdf{\mbox{$\thob(\diag)$}}
\newcommand\sdf{\mbox{$\skeob{}(\diag)$}}

\newcommand\str{\formalPar{\sigma}}
%(7)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Created on May 4,2001
%============================================
% Part 1: pure italic writing of names
%        formerly file italic.tex
%--------------------------------------------
% Part 2: commands for semantics extensions of classes
%         like [[Person]]^t or {^t}[[SamePerson]]^{u}
%        formerly file employ.tex
%===========================================

\newcommand\operarrow[2]{\mbox{{\sffamily%\itshape
                                         #1}$_{#2}$}}
\newcommand\projop[1]{\operarrow{p}{#1}}
%\newcommand\concatop{\operarrow{concat}{}}
%\newcommand\pairop{\operarrow{pair}{}}
%\newcommand\idop[1]{\operarrow{id}{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\newcommand\ltt{\mbox{$t$}}
%\newcommand\ltu{\mbox{$u$}}
%\newcommand\lts{\mbox{$s$}}

%

\newcommand\Emplsem[1]{\mbox{$\semm{\Empl}^{#1}$}}
\newcommand\Emplt{\Emplsem{\ltt}}
\newcommand\Emplu{\Emplsem{\ltu}}
\newcommand\Empls{\Emplsem{\lts}}
\newcommand\Empltu{\mbox{$^{\ltt}\!\semm{\Empl}^{\ltu}$}}
\newcommand\Emplst{\mbox{$^{\lts}\!\semm{\Empl}^{\ltt}$}}
\newcommand\SameEmpltu{\mbox{$^{\ltt}\!\semm{\SameEmpl}^{\ltu}$}}
\newcommand\SameEmplst{\mbox{$^{\lts}\!\semm{\SameEmpl}^{\ltt}$}}

\newcommand\Compsem[1]{\mbox{$\semm{\Comp}^{#1}$}}
\newcommand\Compt{\Compsem{\ltt}}
\newcommand\Compu{\Compsem{\ltu}}
\newcommand\Comps{\Compsem{\lts}}
\newcommand\Comptu{\mbox{$^{\ltt}\!\semm{\Comp}^{\ltu}$}}
\newcommand\Compst{\mbox{$^{\lts}\!\semm{\Comp}^{\ltt}$}}
\newcommand\SameComptu{\mbox{$^{\ltt}\!\semm{\SameComp}^{\ltu}$}}
\newcommand\SameCompst{\mbox{$^{\lts}\!\semm{\SameComp}^{\ltt}$}}

\newcommand\Engrsem[1]{\mbox{$\semm{\Engr}^{#1}$}}
\newcommand\Engrt{\Engrsem{\ltt}}
\newcommand\Engru{\Engrsem{\ltu}}
\newcommand\Engrs{\Engrsem{\lts}}
\newcommand\Engrtu{\mbox{$^{\ltt}\!\semm{\Engr}^{\ltu}$}}
\newcommand\Engrst{\mbox{$^{\lts}\!\semm{\Engr}^{\ltt}$}}

\newcommand\Mngrsem[1]{\mbox{$\semm{\Mngr}^{#1}$}}
\newcommand\Mngrt{\Mngrsem{\ltt}}
\newcommand\Mngru{\Mngrsem{\ltu}}
\newcommand\Mngrs{\Mngrsem{\lts}}
\newcommand\Mngrtu{\mbox{$^{\ltt}\!\semm{\Mngr}^{\ltu}$}}
\newcommand\Mngrst{\mbox{$^{\lts}\!\semm{\Mngr}^{\ltt}$}}

\newcommand\John[1]{\mbox{$\ittt{John}^{#1}$}}

\newcommand\Marr{\ittt{Married}}
\newcommand\Marrsem[1]{\mbox{$\semm{\Marr}^{#1}$}}
\newcommand\Marrt{\Marrsem{\ltt}}
\newcommand\Marru{\Marrsem{\ltu}}
\newcommand\Marrs{\Marrsem{\lts}}
\newcommand\Marrtu{\mbox{$^{\ltt}\!\semm{\Marr}^{\ltu}$}}
\newcommand\Marrst{\mbox{$^{\lts}\!\semm{\Marr}^{\ltt}$}}

\newcommand\Famy{\ittt{Family}}
\newcommand\Famysem[1]{\mbox{$\semm{\Famy}^{#1}$}}
\newcommand\Famyt{\Famysem{\ltt}}
\newcommand\Famyu{\Famysem{\ltu}}
\newcommand\Famys{\Famysem{\lts}}
\newcommand\Famytu{\mbox{$^{\ltt}\!\semm{\Famy}^{\ltu}$}}
\newcommand\Famyst{\mbox{$^{\lts}\!\semm{\Famy}^{\ltt}$}}
\newcommand\Famytt{\mbox{$^{\ltt}\!\semm{\Famy}^{\ltt}$}}
\newcommand\Familytu{\mbox{$^{\ltt}\!\semm{\Famy}^{\ltu}$}}
\newcommand\Familyst{\mbox{$^{\lts}\!\semm{\Famy}^{\ltt}$}}

\newcommand\Friendship{\ittt{Friendship}}
\newcommand\Friship{\ittt{Friendship}}
\newcommand\Frishiptu{\mbox{$^{\ltt}\!\semm{\Friship}^{\ltu}$}}
\newcommand\Frishipst{\mbox{$^{\lts}\!\semm{\Friship}^{\ltt}$}}


\newcommand\Matr{\ittt{Matrimony}}
\newcommand\Matrsem[1]{\mbox{$\semm{\Matr}^{#1}$}}
\newcommand\Matrt{\Matrsem{\ltt}}
\newcommand\Matru{\Matrsem{\ltu}}
\newcommand\Matrs{\Matrsem{\lts}}
\newcommand\Matrtu{\mbox{$^{\ltt}\!\semm{\Matr}^{\ltu}$}}
\newcommand\Matrst{\mbox{$^{\lts}\!\semm{\Matr}^{\ltt}$}}

\newcommand\Distincttu{\mbox{$^{\ltt}\!\semm{\ittt{Distinct}}^{\ltu}$}}
\newcommand\Distinctst{\mbox{$^{\lts}\!\semm{\ittt{Distinct}}^{\ltt}$}}
\newcommand\Sametu{\mbox{$^{\ltt}\!\semm{\ittt{Same}}^{\ltu}$}}
\newcommand\Samest{\mbox{$^{\lts}\!\semm{\ittt{Same}}^{\ltt}$}}

\newcommand\Wom{\ittt{Woman}}
\newcommand\Womsem[1]{\mbox{$\semm{\Wom}^{#1}$}}
\newcommand\Womt{\Womsem{\ltt}}
\newcommand\Womu{\Womsem{\ltu}}
\newcommand\Woms{\Womsem{\lts}}
\newcommand\Womtu{\mbox{$^{\ltt}\!\semm{\Wom}^{\ltu}$}}
\newcommand\Womst{\mbox{$^{\lts}\!\semm{\Wom}^{\ltt}$}}

%\newcommand\Man{\ittt{Man}}
\newcommand\Mansem[1]{\mbox{$\semm{\Man}^{#1}$}}
\newcommand\Mant{\Mansem{\ltt}}
\newcommand\Manu{\Mansem{\ltu}}
\newcommand\Mans{\Mansem{\lts}}
\newcommand\Mantu{\mbox{$^{\ltt}\!\semm{\Man}^{\ltu}$}}
\newcommand\Manst{\mbox{$^{\lts}\!\semm{\Man}^{\ltt}$}}

\newcommand\Husbsem[1]{\mbox{$\semm{\Husb}^{#1}$}}
\newcommand\Husbt{\Husbsem{\ltt}}
\newcommand\Husbu{\Husbsem{\ltu}}
\newcommand\Husbs{\Husbsem{\lts}}
\newcommand\Husbtu{\mbox{$^{\ltt}\!\semm{\Husb}^{\ltu}$}}
\newcommand\Husbst{\mbox{$^{\lts}\!\semm{\Husb}^{\ltt}$}}


\newcommand\mysemm[2]{\mbox{$\semm{#1}^{#2}$}}

\newcommand\isarrt{\mysemm{\isa}{\ltt}}
\newcommand\isarru{\mysemm{\isa}{\ltu}}

\newcommand\wifet{\mysemm{\wife}{\ltt}}
\newcommand\wifeu{\mysemm{\wife}{\ltu}}

\newcommand\husbt{\mysemm{\husb}{\ltt}}
\newcommand\husbu{\mysemm{\husb}{\ltu}}

\newcommand\mdatet{\mysemm{\mDate}{\ltt}}
\newcommand\mdateu{\mysemm{\mDate}{\ltu}}

\newcommand\liveset{\mysemm{\livesAt}{\ltt}}
\newcommand\liveseu{\mysemm{\livesAt}{\ltu}}

\newcommand\income{\ittt{income}}
\newcommand\WMHsem[2]{\mbox{$
      (\semm{\Wom}^{#1}\times\semm{\Man}^{#1}\times\semm{\House}^{#1})
\times
      (\semm{\Wom}^{#2}\times\semm{\Man}^{#2}\times\semm{\House}^{#2})
                            $}
                     }
\newcommand\WMHtu{\WMHsem{\ltt}{\ltu}}


\newcommand\WMWMsem[2]{\mbox{$(\semm{\Wom}^{#1}\times\semm{\Man}^{#1})
                        \times(\semm{\Wom}^{#2}\times\semm{\Man}^{#2})
                             $}
                        }
\newcommand\WMWMtu{\WMWMsem{\ltt}{\ltu}}


\newcommand\myview[1]{\mbox{$V_{#1}$}}
\newcommand\IndI{1}
\newcommand\SWAggr{2}
\newcommand\AggrI{3}
\newcommand\TWAggrG{4}
\newcommand\IndII{5}
\newcommand\TWAggrS{6}
\newcommand\LAggr{7}
\newcommand\LLAggr{8}
\newcommand\SWLAggr{9}
\newcommand\STWAggr{10}
\newcommand\DelAggr{11}
\newcommand\TotAggr{12}
\newcommand\WQual{13}
 \newcommand\LQual{14}
\newcommand\AttrI{15}
\newcommand\SWLQual{16}
\newcommand\STWQual{17}
\newcommand\AttrII{18}



%(8)
%\newcommand\s{\mbox{$S$}}
%\newcommand\os{\mbox{$\overline{S}$}}
%\newcommand\ovr[1]{\mbox{$\overline{#1}$}}
\newcommand\into[1]{\stackrel{#1}{\hookrightarrow}}
\newcommand\repgra{\nicex{ R$}}
\newcommand\rgra{\repgra}
\newcommand\nds[1]{\mbox{$\mathit{Nds}#1$}}
\newcommand\arrs[1]{\mbox{$\mathit{Arrs}#1$}}
\newcommand\ndsr{\nds{\rgra}}
\newcommand\arrsr{\arrs{\rgra}}

\newcommand\dersetmath{\mathit{Der}}
\newcommand\derset{\mbox{$\dersetmath$}}
\newcommand\derop{\mbox{$\mathbf{der}$}}
\newcommand\algebra[1]{\mbox{$\alpha^{#1}$}}
\newcommand\algu{\algebra{\uskemath}}

%\newcommand\inss[1]{\lar{I}{\ske{#1}}{\uske}}
%\newcommand\ovri{\mbox{$\overline{I}$}}
%\newcommand\ovrinss[1]{\lar{\ovri_{#1}}{\ovrs{#1}}{\uske}}

\newcommand\ovrske[1]{\mbox{$\overline{\ske{#1}}$}}
\newcommand\ovrs[1]{\mbox{$\overline{\ske{#1}}$}}
%-----------------------------
\newcommand\sv{\mbox{$\ske{V}$}}
\newcommand\sr{\mbox{$\ske{R}$}}
\newcommand\vmor{\lar{v}{\sv}{\ovrske{}}}
\newcommand\rmor{\lar{r}{S}{\ovrske{R}}}
\newcommand\emor{\lar{e}{S}{\U}}
\newcommand\vpair{\mbox{$V=(\sv,v)$}}
\newcommand\rpair{\mbox{$R=(\sr,r)$}}



%\newcommand\dbinst{\lar{e}{S}{W} }

%---------------------------------------------------


\newcommand\ovrsig[1]{\mbox{$\overline{\sigma _{#1}}$}}
\newcommand\ovrg[1]{\mbox{$\overline{G_{#1}}$}}
%-----------------------------------------
\newcommand\ovrp{\mbox{$\overline{\pi }$}}%{#1}}$}}
\newcommand\ovreps{\mbox{$\overline{\vare}$}}     % overlined epsilon


%\renewcommand\endinput{}
%\newcommand\comp{\mathbin{\triangleright\!\!\triangleright}}
\newcommand\state[2]{\mbox{${\mathit{state}}^{#1}_{#2}$}}
\newcommand\starInherit{*-inherit}

\newcommand\sig{\mbox{$\Sigma $}}
\newcommand\sigm{\Sigma}
\newcommand\defitemotstup[1]{\par\smallskip\noindent (#1)}


\newcommand\arity[1]{\mbox{$\mathit{Arity}(#1)$}}
\newcommand\predsem[2]{\mbox{$\semm{#1}^{#2} $}}
\newcommand\psem[1]{\predsem{P}{#1}}
\newcommand\psemu{\psem{\ucatmath}}
\newcommand\lsig{\mbox{$\Lambda $}}

%%%
\newcommand\Attr{\mbox{$\mathit{Attr}$}}
\newcommand\Var{\mbox{$\mathit{Var}$}}
\newcommand\relcat{\mbox{$\categoryname{Rel}$}}
\newcommand\relske{\mbox{$\sketchname{Rel}$}}
\newcommand\itte[1]{\mbox{\textit{#1}}}
\newcommand\dbcat{\mbox{$\categoryname{DB}$}}

\newcommand\skecat[1]{\mbox{$\categoryname{Sketch}(\sig_{#1})$}}
\newcommand\sigcat{\mbox{$\categoryname{Sign}$}}

\newcommand\funor{\mbox{$\Phi$}}
\newcommand\funarr{\lar{f}{X}{Y}}
\newcommand\currfun{\mbox{\lar{\Map{A}{\_}}{\catset}{\catset}}}
\newcommand\curra{\Map{A}{\_}}

% \newcommand\ {\itte{ }}
\newcommand\target{\itte{target}}
\newcommand\source{\itte{source}}
\newcommand\conof{\itte{consistsOf}}
\newcommand\marker{\itte{marker}}
\newcommand\Node{\itte{Node}}
\newcommand\nodeit{\ittt{node}}
\newcommand\Arrow{\itte{Arrow}}
\newcommand\arrow{\ittt{arrow}}
\newcommand\diagramit{\itte{diagram}}
\newcommand\graphit{\itte{graph}}
\newcommand\shape{\itte{shape}}
\newcommand\predecl{\itte{predicate\_declarations}}
\newcommand\statements{\itte{statements}}
\newcommand\carrier{\itte{carrier}}
\newcommand\arityshape{\itte{arity\_shape}}


% semiotics
%% MACROS OF Dec 3
\newcommand\formalObj[1]{\mbox{\sffamily #1}}
\newcommand\formalOper[1]{\mbox{{\bfseries\sffamily #1}}}
\newcommand\informalObj[1]{\mbox{\textit #1}}
\newcommand\informalOper[1]{\mbox{{\bfseries\itshape #1}}}

\newcommand\lzzl{\formalObj{l}}  %logic
\newcommand\ml{\informalObj{ML}}  % modeling language

\newcommand\f{\formalObj{F}}
\renewcommand\c{\informalObj{C}}
\newcommand\derf{\formalOper{Der}}
\newcommand\deri{\informalOper{Un}}
\newcommand\derff{\derf.\f}
\newcommand\deric{\deri(\c)}
\newcommand\FormalInterpret[1]{\mbox{$\formalObj{i}_f$}}
\newcommand\SubstantInterpret[1]{\mbox{$\informalObj{i}_s$}}


%====================================

\newcommand\informalPar[1]{\nicex{{#1}$}}
\newcommand\infParind[1]{\cal #1}
\newcommand\formalPar[1]{\mbox{$\mathrm{#1}$}}
\newcommand\frmParind[1]{\mathrm{#1}}

\newcommand\informalParBold[1]{\mbox{${\cal #1}$}}
%\newcommand\formalPar[1]{\mbox{$\mathrm #1$}}

\newcommand\object[2]{\mbox{${\mathsf{#1}}_{#2}$}}
%\newcommand\object[2]{\mbox{$#1_{#2}$}}
\newcommand\universe[1]{\mbox{$\mathbf{#1}$}}
%\newcommand\objectind[1]{\mathsf{#1}}
\newcommand\objectind[1]{\mathsf{#1}}
\newcommand\objectmath[1]{\mathsf{#1}} % the same
\newcommand\universeind[1]{\mathbf{#1}}
\newcommand\umath[1]{\mathbf{U}_{#1}}

\newcommand\proc[1]{\mbox{\sffamily\bfseries #1}}
\newcommand\procind[2]{\mbox{${\mathrm{#1}}_{\mathrm #2}$}}
\newcommand\linf{\informalParBold{L}}
\newcommand\minf{\mbox{$\informalPar{M}(\diag{})$}}
\newcommand\mdinf{\mbox{$\informalPar{M}(\diag{})$}} % the same as above
\newcommand\mdfrm{\mbox{$\formalPar{M}(\diag{})$}} % the same as above
\newcommand\uinf{\informalPar{U}}

\newcommand\meaninf{\informalPar{M}}
\newcommand\meanfrm[1]{\mbox{$\formalPar{M}_{#1}$}}

\newcommand\diags{\mbox{$\mathit{Diags}$}}
\newcommand\graph{\mbox{$\mathit{Graph}$}}

\newcommand\diaob[1]{\object{D}{#1}} %\mbox{$D$}}
\newcommand\diagob[1]{\object{D}{#1}} %the same \mbox{$D$}}
\newcommand\diag[1]{\object{D}{#1}} %the same \mbox{$D$}}
\newcommand\diaind{\objectind{D}}

\newcommand\graob[1]{\object{G}{#1}}
\newcommand\graind{\objectind{G}}
\newcommand\gra[1]{\graob{#1}}

\newcommand\skeob[1]{\object{S}{#1}}
\newcommand\skeind{\objectind{S}}

\newcommand\modelob[1]{\object{M}{#1}}
\newcommand\modelind{\objectind{M}}

\newcommand\sigob[1]{\object{\mbox{$\Sigma$}}{#1}}
\newcommand\skediag{\skeob{}[\diag{}]}

\newcommand\meaninfdiag{\meaninf[\diag{}]}
\newcommand\meanfrmdiag{\meanfrm[\diag{}]}
% synonyms
\newcommand\meanifdiag{\meaninf[\diag{}]}
\newcommand\meanfdiag{\meanfrm[\diag{}]}

%%% diags, sketchs, specs, and their semantic interpretaions
\newcommand\objectWithInd[3]{\mbox{$\mathsf{#1}_{#2}^{#3}$}}
\newcommand\sketch[1]{\objectWithInd{S}{#1}{}}
\renewcommand\ske[1]{\sketch{#1}}
%\newcommand\graph[1]{\objectWithInd{S}{#1}{}}
\renewcommand\diag[1]{\objectWithInd{D}{#1}{}}
%\newcommand\inst[2]{\mbox{$\mathit{Inst}^{#2}{(#1)}$}}
%\newcommand\instob[2]{\mbox{$\mathit{Inst}^{#2}{(#1)}$}}


%\newcommand\diaob[1]{\mbox{$\diag{#1}$}}
%\newcommand\skeob{\mbox{$S$}}
\newcommand\graofske{\mbox{$G_\skeind$}}
\newcommand\graske{\graofske}
\newcommand\diaofske{\mbox{$D_\skeind$}}
\newcommand\diaske{\diaofske}


\renewcommand\eg{e.g.}
\renewcommand\C{\mbox{$C$}}

\newcommand\ext[1]{\mbox{$\mathit{Ext}(#1)$}}
\renewcommand\stt[1]{\mbox{$\mathit{Stt}(#1)$}}
\newcommand\GCS{{\bf (GCS)}}
\newcommand\AET{{\bf (AET)}}



%\newcommand\tuple[1]{\left [ \mathstrut {#1} \right ]}
\newcommand\pmrk[1]{\mbox{[{\sf #1}]}}
\newcommand\omrk[1]{\mbox{[{\sf #1} $\rangle $}}

% used in Intro
\newcommand\lanfrm{\formalPar{FL}}
\newcommand\flan{\formalPar{FL}} %the same
\newcommand\flanind{\frmParind{FL}}

\newcommand\x{\diag{}}   %\mbox{$D$}}
\renewcommand\s{\skeob{}}%\mbox{$S$}}
%\newcommand\mix{\mbox{$\meaninf$}} %(\x)
%\newcommand\mfx{\mbox{$\meanfrm{\flanind}$}} %(\x)
\newcommand\mix{\mbox{$\meaninf(\x)$}}
\newcommand\mfx{\mbox{$\meanfrm{}(\x)$}}

%\newcommand\flan{\mbox{$\meanfrm(\x)$}}

\newcommand\spex[1]{\mbox{$\skeob{#1}$}} %(\mix)$}}
\newcommand\spem[1]{\mbox{$\skeob{#1}$}} %(\mix)$}}
\newcommand\spexl  {\mbox{$\skeob{\flanind}$}} %(\x)$}}
\newcommand\speml  {\mbox{$\skeob{}$}} %(\mfx)$}}

\newcommand\dateit{\ittt{date}}

% used in dGetStartViaAss
\newcommand\nis{\nicex{ S$}}
\newcommand\niv{\nicex{ V$}}
\newcommand\nivind{{V}}
\newcommand\nisind{{S}}

\newcommand\mrkdual[3]{\mbox{${#2}\stackrel{{\cal\scriptsize #1}}{[><]}{#3}$}} %{[>^{\mathrm{#1}}<]}$}}
\newcommand\sgv{single-valued}
\newcommand\assgenpred{\mbox{$[\Uparrow]$}}
\newcommand\SepPred{\mrk{1-1}  }
\newcommand\CovPred{\mrk{cover}}
\newcommand\MemPred{\mrk{$\in$}}

\newcommand\binAss{1}
\newcommand\assCla{2}
\newcommand\reiAss{3}
\newcommand\terAss{4}
\newcommand\quaAss{5}
\newcommand\skeo{\skeob{\binAss}}
\newcommand\skei{\skeob{\assCla}}
\newcommand\skeii{\skeob{\reiAss}}
\newcommand\skeiii{\skeob{\terAss}}
\newcommand\skeiv{\skeob{\quaAss}}
%\newcommand\diaob[1]{\diag{#1}}
\newcommand\diao{\diaob{\binAss}}
\newcommand\diai{\diaob{\assCla}}
\newcommand\diaii{\diaob{\reiAss}}
\newcommand\diaiii{\diaob{\terAss}}
\newcommand\diaiv{\diaob{\quaAss}}


\newcommand\visfunctor{\mbox{{\sffamily\bfseries vis}}}
\newcommand\skefunctor{\mbox{{\sffamily\bfseries ske}}}

%used in eAssonBySke
\newcommand\sale{\ittt{sale}}
\newcommand\Show{\ittt{Show}}
\renewcommand\show{\ittt{show}}
\newcommand\seat{\ittt{seat}}
\newcommand\perf{\ittt{perf}}
\newcommand\Performance{\ittt{Performance}}
\newcommand\Ticket{\ittt{Ticket}}
\newcommand\ticket{\ittt{sale}}
\newcommand\Integer{\ittt{Integer}}

\newcommand\mastr[1]{\mbox{$\mathbf{#1}$}}
\newcommand\extofcla[1]{\mastr{\semm{\mathit #1}}}
\newcommand\behofcla[1]{\mastr{\besemm{\mathit{#1}}}}
\newcommand\sttofcla[1]{\lar{\statemap{}{\mathit{#1}}}{\extofcla{#1}}{\behofcla{#1}}}

%\newcommand\tlu{\mbox{$t<u$}}
%\newenvironment\mathitext%
%{
%\begin{displaymath}
%\mbox{ }
%\end{displaymath}
%} {}
\newcommand\cEngine{\ittt{carEngine}}
\newcommand\carEngine{\ittt{carEngine}}


\newcommand\mrkmon[2]{\mbox{\mrk{1-1}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkfro[2]{\mbox{\mrk{fro}$^{#1}_{\mathit{#2}}$}}
\renewcommand\mrkid[2]{\mbox{\mrk{id}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkstrongid[2]{\mbox{\mrk{id!}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkdel[2]{\mbox{\mrk{del}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkins[2]{\mbox{\mrk{ins}$^{#1}_{\mathit{#2}}$}}

\newcommand\mathand{\mbox{ and }}
\newcommand\mathor{\mbox{ or }}
\newcommand\mathif{\mbox{ if }}
\newcommand\maththen{\mbox{ then }}
\newcommand\mathiff{\mbox{ iff }}
%\newcommand\ofit{\ittt{of}}
\newcommand\wholeit{\ittt{whole}}
\newcommand\Wholeit{\ittt{Whole}}
\newcommand\partit{\ittt{part}}
\newcommand\stateit{\ittt{state}}
\newcommand\prokol{{\mathbf +}\!\!\!\!\circ}

\newcommand\mixsemm[1]{\mbox{$\lbesemm\, {\mathit #1} \, \rsemm$}}

\newcommand\logrule[2]{\frac{\mathstrut #1}{\mathstrut #2}}
\newcommand\logruleFig[2]{\frac{\mathstrut #1}{\mathstrut #2}}
\newcommand\logruleRow[2]{\mbox{if $#1$ then $#2$}}
\newcommand\logruleFigText[2]{\mbox{$
\frac{\mbox{\rule[-1ex]{0pt}{3ex} #1}}{\mbox{\rule{0pt}{3ex} #2}} $}
}
\newcommand\logruleRowText[2]{\mbox{if #1 then #2}}


\newcommand\ClassIndInd[3]{\mbox{$^{#1}\!\semm{\mathit{#2}}^{#3}$}}
\newcommand\ClassBeh[1]{\mbox{$\besemm{\mathit{#1}}$}}

\newcommand\refInd[2]{\mbox{$\semm{\mathit{#1}}^{\mathit{#2}}$}}
\newcommand\refBehInd[2]{\mbox{$\besemm{\mathit{#1}}^{\mathit{#2}}$}}
\newcommand\refIndBeh[2]{\mbox{$\besemm{\mathit{#1}}^{\mathit{#2}}$}}




\renewcommand\same[2]{\mbox{${\mathit{same}}^{#1}_{\mathit{#2}}$}}
\newcommand\samemap[2]{\mbox{${\mathit{same}}^{#1}_{\mathit{#2}}$}}
%\newcommand\sametu[1]{\samemap{tu}{#1}}
\newcommand\delset[3]{\mbox{$\semm{#3}^{#1}\mathsf{Del}^{#1\rightarrow #2}$}}
\newcommand\deltu[1]{\delset{t}{u}{#1}}
\newcommand\newset[3]{\mbox{$\semm{#3}^{#1}\mathsf{New}^{#2\rightarrow #1}$}}
\newcommand\newut[1]{\newset{u}{t}{#1}}
\newcommand\newts[1]{\newset{t}{s}{#1}}
%\newcommand\insut[1]{\newset{t}{u}{#1}}
%\newcommand\newut[1]{\newset{t\leftarrow u}{#1}} %  correct
%\newcommand\newtu[1]{\newset{t\leftarrow u}{#1}} % incorrect, to match old
%\newcommand\newts[1]{\newset{s\leftarrow t}{#1}} %correct,
%\newcommand\newst[1]{\newset{s\leftarrow t}{#1}} %incorrect, to match old
\newcommand\statemap[2]{\mbox{${\mathit{state}}^{#1}_{\mathit{#2}}$}}



\newcommand\ofit{\ittt{of}}
\newcommand\ofmap[1]{\refInd{of}{#1}}
%\newcommand\ofit{\ofmap{}}
\newcommand\oft{\ofmap{t}}
\newcommand\ofu{\ofmap{u}}

\newcommand\ofindit{\mbox{$\semm{{\mathit of}_i}^{t}$}}
%\newcommand\ofindiu{\mbox{$\semm{{\mathit of}_i}^{u}$}}
\newcommand\ofiu{\mbox{$\semm{{\mathit of}_i}^{u}$}}
%
\newcommand\isit{\ittt{is}}
\newcommand\ismap[1]{\refInd{is}{#1}}
%\newcommand\isit{\ismap{}}
\newcommand\ist{\ismap{t}}
\newcommand\isu{\ismap{u}}


\newcommand\isindt{\mbox{$\semm{{\mathit is}_i}^{t}$}}
\newcommand\isindu{\mbox{$\semm{{\mathit is}_i}^{u}$}}
%

\newcommand\hasit{\ittt{has}}
\newcommand\hasmapbeh{\besemm{has}}
\newcommand\hasbeh{\besemm{has}}
\newcommand\hasbehind[1]{\besemm{has}_{#1}}


\newcommand\supmap[1]{\refInd{sup}{#1}}
\newcommand\supit{\supmap{}}
\newcommand\supt{\supmap{t}}
\newcommand\supu{\supmap{u}}
%
\newcommand\supbeh{\besemm{sup}}
%
\newcommand\submap[1]{\refInd{sub}{#1}}
\newcommand\subit{\submap{}}
\newcommand\subt{\submap{t}}
\newcommand\subu{\submap{u}}

\newcommand\isamap[1]{\refInd{isA}{#1}}
\newcommand\isait{\isamap{}}
\newcommand\isat{\isamap{t}}
\newcommand\isau{\isamap{u}}
\newcommand\isabeh{\besemm{\isa}}

\newcommand\Persontu{\ClassIndInd{t}{Person}{u}}
\newcommand\Persont{\ClassIndInd{}{Person}{t}}
\newcommand\Personu{\ClassIndInd{}{Person}{u}}
\newcommand\PersonBeh{\ClassBeh{Person}}

\newcommand\Drivertu{\ClassIndInd{t}{Driver}{u}}
\newcommand\Drivert{\ClassIndInd{}{Driver}{t}}
\newcommand\Driveru{\ClassIndInd{}{Driver}{u}}



\newcommand\Cart{\ClassIndInd{}{Car}{t}}
\newcommand\Caru{\ClassIndInd{}{Car}{u}}
\newcommand\Cartu{\ClassIndInd{t}{Car}{u}}
\newcommand\SameCartu{\ClassIndInd{t}{SameCar}{u}}
\newcommand\CarBeh{\ClassBeh{Car}}
\newcommand\Carbeh{\ClassBeh{Car}}
\newcommand\Ownershiptu{\ClassIndInd{t}{Ownership}{u}}
\newcommand\Ownershipt{\ClassIndInd{}{Ownership}{t}}
\newcommand\Ownershipu{\ClassIndInd{}{Ownership}{u}}



\newcommand\Ownership{\ittt{Ownership}}
\newcommand\owner{\ittt{owner}}
%\newcommand\car{\ittt{car}}
%\newcommand\property{\ittt{property}}

%\newcommand\Engine{\ittt{Engine}}
%\newcommand\Eng{\ittt{Eng}}
\newcommand\Enginetu{\ClassIndInd{t}{Engine}{u}}
\newcommand\Enginet{\ClassIndInd{}{Engine}{t}}
\newcommand\Engineu{\ClassIndInd{}{Engine}{u}}
\newcommand\EngineBeh{\ClassBeh{Engine}}
\newcommand\Enginebeh{\ClassBeh{Engine}}
\newcommand\Engbeh{\ClassBeh{Engine}}
\newcommand\BodyBeh{\ClassBeh{Body}}
\newcommand\ChassisBeh{\ClassBeh{Chassis}}


%\newcommand\Engine{\ittt{Engine}}
%\newcommand\Eng{\ittt{Eng}}
%\newcommand\Body{\ittt{Body}}
%\newcommand\BodyBeh{\ClassBeh{Body}}
%\newcommand\Chassis{\ittt{Chassis}}
%\newcommand\ChassisBeh{\ClassBeh{Chassis}}
%%\newcommand\PartName{Part}

%\newcommand\drives{\ittt{drives}}
\newcommand\drivest{\refInd{drives}{t}}
\newcommand\drivesu{\refInd{drives}{u}}
\newcommand\drivesbeht{\refBehInd{drives}{t}}
\newcommand\drivesbehu{\refBehInd{drives}{u}}
\newcommand\drivesbehv{\refBehInd{drives}{v}}
\newcommand\drivesbeh{\refBehInd{drives}{}}

\newcommand\fuelat{\refInd{fuelAmount}{t}}
%\newcommand\fuelAm{\ittt{fuelAmount}}
%\newcommand\tankVo{\ittt{tankVolume}}
%\newcommand\fillTa{\ittt{fillTank}}
%\newcommand\car{\ittt{car}}

\newcommand\tankvt{\refInd{tankVolume}{t}}
\newcommand\tankvu{\refInd{tankVolume}{u}}

\newcommand\cart{\refInd{car}{t}}
\newcommand\caru{\refInd{car}{u}}

\newcommand\prst{\refInd{prs}{t}}
\newcommand\prsu{\refInd{prs}{u}}

\newcommand\enginet{\refInd{engine}{t}}
\newcommand\engineu{\refInd{engine}{u}}

\newcommand\persont{\refInd{person}{t}}
\newcommand\personu{\refInd{person}{u}}



\newcommand\PersonP{\Person$^+$}
\newcommand\PersonM{\Person$^-$}
\newcommand\CarP{\Car$^+$}
\newcommand\CarM{\Car$^-$}


\newcommand\floatRange[1]{\mrk{Float(#1)}}

%\newcommand\Car{\ittt{Car}}


\newcommand\becar{\besemm{\Car}}
\newcommand\beCar{\besemm{\Car}}
\newcommand\lt{$t$}
\newcommand\tstate{\statei{}{\ltt}}
\newcommand\stts{\statepoint{s}}



% === composition: begin
\newcommand\ipart[1]{\mbox{$\mathit{Part}_{#1}$}}
\newcommand\ipartmath[1]{\mathit{Part}_{#1}}
\newcommand\ipartbeh[1]{\mbox{$\besemm{\ipart{#1}}$}}

\newcommand\imeth[1]{\mbox{$\mathit{Meth}_{#1}$}}
\newcommand\imethbeh[1]{\mbox{$\besemm{\imeth{#1}}$}}
\renewcommand\imeth[1]{\mbox{$\mathit{Meth}_{#1}$}}
\newcommand\imethstar[1]{\mbox{$\mathit{Meth}^*_{#1}$}}
\newcommand\istameth[1]{\imethstar{#1}} %the same

\newcommand\iiface[1]{\mbox{$\mathbf{IFace}_{#1}$}}
\newcommand\iifacestar[1]{\mbox{$\mathbf{IFace}^*_{#1}$}}
\newcommand\iistaface[1]{\iifacestar{#1}} %the same


\newcommand\prodspace{\mbox{$\prod_{i}\ipartbeh{i}$}}
\newcommand\prodspa{\mbox{$\prod_{i}\ipartbeh{i}$}}
\newcommand\wholespace{\mbox{$\prod_{i}^*\ipartbeh{i}$}}

\newcommand\prodmeths{\mbox{$%\prod_{i}\imeth{i}
                             \methsset{prod}$}}
\newcommand\wholemeths{\mbox{$%\prod^*_{i}\imeth{i}
                             \someofmethsset{Prod}$}}
\newcommand\prodmethsbeh{\mbox{$\besemm{\prodmeths}$}}
\newcommand\wholemethsbeh[2]{\mbox{$\besemm{\someofmeths{#1}{#2}}$}}
\newcommand\prodiface{\mbox{$%\prod_{i}\iiface{i}
                              \iface{Prod}$}}
\newcommand\wholeiface{\mbox{$%\prod^*_{i}\iiface{i}
                               \ifacepartial{Prod}$}}



%\newcommand\reductmap[1]{\mbox{$\mathit{red}^*_{\mathit{#1}}$}}
\newcommand\reductmap[2]{\mbox{$\mathit{red}^{\mathit{#1}}_{\mathit{#2}}$}}
%\newcommand\reductmapstar[1]{\mbox{$\mathit{red}^*_{\mathit{#1}}$}}
\newcommand\red[2]{\reductmap{#1}{#2}}
\newcommand\redsta[1]{\reductmapstar{#1}}
\newcommand\projectmap[1]{\mbox{$\mathit{proj}_{\mathit{#1}}$}}
%\renewcommand\proj[1]{\projectmap{#1}}
\newcommand\fproj[1]{\mbox{$\pi_{#1}$}}


%==== composition: end =========

\renewcommand\Eng[1]{\mbox{$\mathit{Eng}^#1$}}
\renewcommand\eng[1]{\mbox{$\mathit{eng}^#1$}}
\newcommand\ETOC{\Eng{*}} %Engine methods transferred TO Cars
\newcommand\etoc{\eng{*}}
\newcommand\Etocbeh{\besemm{\Engine^*}}
\newcommand\etocind{EngIntoCar}
\newcommand\ctoeind{CarToEng}

\newcommand\me{\mbox{$m$}}
\newcommand\Me{\mbox{$\mathit{Meth}$}}

%\newcommand\meths1]{\mbox{$\mathit{meth}^{\mathit{#1}}$}}
\newcommand\methsset[1]{\mbox{$\mathit{#1}\mathsf{Meth}$}}
%the same
\newcommand\meths[1]{\mbox{$\mathit{#1}\mathsf{Meth}$}}
%  in short
\newcommand\mset[1]{\methsset{#1}}

\newcommand\imset[1]{\mbox{\methsset{}$_{#1}$}}
\newcommand\someofmethsset[1]{\mbox{$\mathit{#1}^{*}\mathsf{Meth}$}}
% in short
\newcommand\somset[1]{\someofmethsset{#1}}

\newcommand\iface[1]       {\mbox{$\mathit{#1}  \mathbf{IFace}$}}
\newcommand\ifacepartial[1]{\mbox{$\mathit{#1}^*\mathbf{IFace}$}}

\newcommand\methsbody[2]{\mbox{$\besemm{\mathit{#1}}^{\mathit{#2}}$}}
%  in short
\newcommand\mbody[2]{\methsbody{#1}{#2}}
\newcommand\msbody[2]{\mbox{$\besemm{\methsset{#1}}^{\mathit{#2}}$}} % the same
\newcommand\mmbody[1]{\msbody{#1}{}}



\newcommand\someofmethsiface[1]{\mbox{$\ifacepartial{#1}$}}
\newcommand\somface[1]{\someofmethsiface{#1}}

\newcommand\someofmethsbody[2]{\mbox{$\besemm{\someofmethsset{#1}}^{#2}$}}
\newcommand\sombody[2]{\someofmethsbody{#1}{#2}}

\newcommand\miface{\iface{\me}}

\newcommand\categoryname[1]{\mathbf{#1}}
\newcommand\sketchname[1]{\mathsf{#1}}

\newcommand\setcatmath{\categoryname{Sets}}
\newcommand\setskemath{\sketchname{Set}}
\newcommand\vsetcatmath{\categoryname{VarSet}}
\newcommand\bsetcatmath{\categoryname{BehSet}}
\newcommand\coalgcatmath{\categoryname{coAlg}}
\newcommand\coalgske{\sketchname{coAlg}}
\newcommand\erske{\sketchname{ER}}
\newcommand\ercat{\categoryname{ER}}
\newcommand\vsetske{\sketchname{VarSet}}
\newcommand\bsetske{\sketchname{BehSet}}

\newcommand\setcat{\mbox{$\setcatmath$}}
\renewcommand\setcat{\mbox{$\categoryname{Sets}$}}
\newcommand\gracat{\mbox{$\categoryname{Graphs}$}}
\newcommand\posetcat{\mbox{$\categoryname{Posets}$}}
\newcommand\catcat{\mbox{$\categoryname{Cats}$}}


\newcommand\vsetcat{\mbox{$\vsetcatmath$}}
\newcommand\bsetcat{\mbox{$\bsetcatmath$}}
\newcommand\coalgcat{\mbox{$\coalgcatmath$}}
\newcommand\setske{\mbox{$\setskemath$}}


\newcommand\univcat{\mbox{$\categoryname{U}$}}
\newcommand\ucatmath{\categoryname{U}}
\newcommand\univske{\mbox{$\sketchname{U}$}}
\newcommand\uskemath{\sketchname{U}}
\newcommand\ucat{\univcat}
\newcommand\uske{\univske}

\newcommand\instus[2]{\inst{\ske{#1}}{\ucatmath_{#2}}}
\newcommand\uni[1]{\mbox{$\univcat_{#1} $}}

\newcommand\reuniv{\univcat}
\newcommand\mapcatmath{\categoryname{Map}}
\newcommand\mapcat{\categoryname{Map}}
\newcommand\Map[2]{\mbox{$\mapcatmath(#1,#2)$}}
\newcommand\cariface{\iface{\car}}

\newcommand\rePlug{\ittt{rePlug}}
%=====================
%\input{../../Tools/Macros/m01-macroLogic.tex}

%=====================
%\input{../../Tools/Macros/m05-myStyle(razdels).tex}
\newtheorem{mydef}{\noindent Definition}
%\newtheorem{remark}{Remark}
\newtheorem{termin}{\noindent Terminology}

%% ===========================================================
%%the version where razdels are inside subsections not sections
%\newcounter{Razdel}[subsection]
%\newcommand\beginRazd[1]%
%{
%\renewcommand\theRazdel{\thesubsection.\arabic{Razdel}}
%\par%\smallskip
%\noindent\refstepcounter{Razdel}%
%{\bf \thesubsection.\arabic{Razdel} #1} %\mylabel{#2}
%}
%%==========================================================

%% =========================================================
%%the version where razdels are inside sections not subsections
%\newcounter{RazDel}[section]
%\newcommand\beginRazD[1]%  2nd argument is dummy and inherited from old verion
%{
%\renewcommand\theRazDel{\thesection.\arabic{RazDel}}
%\par%\smallskip
%\noindent\refstepcounter{RazDel}%
%{\bf \thesection.\arabic{RazDel} #1} %\mylabel{#2}
%}
%%==============================================================
%
%%\newcommand\EndRazD{\qquad\qquad\mbox{$\diamondsuit$}\par\medskip}
%%\newcommand\EndRazd{\qquad\qquad\mbox{$\diamondsuit$}\par\medskip}
%
%\newcommand\EndRazD{\par\smallskip}
%\newcommand\EndRazd{\par\smallskip}
%%\renewcommand\EndRazD{\mbox{\textbf{endRemark} $\blacktriangleright$}\par\smallskip}
%%\renewcommand\EndRazd{\mbox{\textbf{endRemark} $\blacktriangleright$}\par\smallskip}
%\newcommand\remends{\par\smallskip}
%                   %{\mbox{\textbf{endRemark} $\blacktriangleright$}}
%
%
%\newenvironment{razdel}[2]{\beginRazd{#1}{Razd#2}}{\endRazd}
%\newenvironment{razd}[2]{\beginRazd{{%\itshape
%                                      \bfseries #1}}}{\EndRazd}
%%\newenvironment{razD}[2]{\beginRazD{#1}{RazD#2}}{\EndRazD}
%\newenvironment{razD}[2]{\beginRazD{{%\itshape
%                                      \bfseries #1}}}{\EndRazD}
%\newenvironment{razzD}[1]{\beginRazD{{%\itshape
%                                      \bfseries #1}}}{\EndRazD}
%
%% 1st argument is the title of the razdel,
%% 2nd - dummy, formerly it was for the label
%
%
%\newenvironment{defi}[1]{\beginRazdel{Definition.}  {Defi#1}}{\endRazdel}
%\newenvironment{cons}[1]{\beginRazdel{Construction.}{Cons#1}}{\endRazdel}
%\newenvironment{prop}[1]{\beginRazdel{Proposition.} {Prop#1}}{\endRazdel}
%\newenvironment{theo}[1]{\beginRazdel{Theorem.}     {Theo#1}}{\endRazdel}
%\newenvironment{coro}[1]{\beginRazdel{Corollary.}   {Coro#1}}{\endRazdel}
%\newenvironment{exam}[1]{\beginRazdel{Example.}     {Exam#1}}{\endRazdel}
%%\newenvironment{rema}[1]{\beginRazdel{Remark.}      {Rema#1}}{\endRazdel}
%\newenvironment{warn}[1]{\beginRazdel{Warning.}     {Warn#1}}{\endRazdel}
%\newenvironment{desc}[1]{\beginRazdel{Description.} {Desc#1}}{\endRazdel}
%\newenvironment{disc}[1]{\beginRazdel{Discussion.}  {Disc#1}}{\endRazdel}
%\newenvironment{conv}[1]{\beginRazdel{Convention.}  {Conv#1}}{\endRazdel}
%\newenvironment{nota}[1]{\beginRazdel{Notation.}    {Nota#1}}{\endRazdel}
%
%\newcommand\equnref[1]{Equation~(\ref{Equn#1})}
%\newcommand\equlref[1]{equality~(\ref{Equl#1})}
%%\newcommand\diagref[1]{(\ref{#1})}
%\newcommand\consref[1]{Construction~\ref{Cons#1}}
%\newcommand\defref[1]{Definition~\ref{#1}}
%\newcommand\propref[1]{Proposition~\ref{Prop#1}}
%\newcommand\discref[1]{Discussion~\ref{Disc#1}}
%\newcommand\convref[1]{Convention~\ref{Conv#1}}
%\newcommand\notaref[1]{Notation~\ref{Nota#1}}
%\newcommand\descref[1]{Description~\ref{Desc#1}}
%\newcommand\remaref[1]{Remark~\ref{Rema#1}}
%\newcommand\examref[1]{Example~\ref{Exam#1}}
%\newcommand\cororef[1]{Corollary~\ref{Coro#1}}
%\newcommand\razdref[1]{Section~\ref{Razd#1}}
%%\newcommand\appref[1]{appendix~\ref{App#1}}    see pre_gen.tex
%%\newcommand\sectref[1]{section~\ref{Sect#1}}   ....
%%\newcommand\sectsectref[1]{sections~\ref{Razd#1}}
%%\newcounter{Razdel}[subsection]
%\newcommand\NachRazd[2]%
%{
%%\renewcommand\theRazdel{\thesubsection.\arabic{Razdel}}
%\par\medskip\noindent%\refstepcounter{Razdel}%
%{\it #1} \mylabel{#2} }
%%\newcommand\end{\qquad\qquad\mbox{$\diamondsuit$}\par\medskip}
%
%\newenvironment{Example}{\NachRazd{Example}}{\end}
%\newenvironment{Remark} {\NachRazd{Remark}}{\end}
%\newenvironment{Warning}{\NachRazd{Warning}}{\end}
%=====================
%\input{../../Tools/Macros/m10-MMt-CASCON-Macros.tex}
\newcommand\instarr[1]{\mbox{$\lar{\statemap}{\igra{}{}}{#1}$}}
\newcommand\instarrt[1]{\mbox{$ \lar{\statemap}{\igraph{t}{}}{#1}$}}

\newcommand\idop{\mrksemiop{\times id}}
\newcommand\idos{\mrksemiop{+id}}

\newcommand\idoP{\mrkop{prod}}
\newcommand\idoS{\mrkop{sum}}

\newcommand\recop{\mrkop{rec}}
\newcommand\varop{\mrkop{var}}
%\newcommand\sumop{\mrkop{var}}

\renewcommand\owner{\textit{owner}}
\newcommand\types{\nicex{ T$}}

%% for Kleisly arrows section

\newcommand\ssma{\mbox{$S$}}
\newcommand\tsma{\mbox{$T$}}
\newcommand\usma{\mbox{$U$$$}}
\newcommand\mapelement{\mbox{$\rightsquigarrow$}}
\newcommand\mapel{\mapelement}

\newcommand\klear[3]{\mbox{$#1\!: #2 \rightsquigarrow #3$}}
\newcommand\kleare[2]{\mbox{$#1 \rightsquigarrow #2$}}
\newcommand\lare[2]{\mbox{$#1 \rightarrow #2$}}
%==============================================

\newcommand\corrce{correspondence}






%%% 1. Collections
%
%==1.1 Categories
% macros for names moved to macros4names.tex
%\newcommand\catname[1]{\mbox{\bfseries\itshape #1}}
%%\newcommand\catname[1]{\mbox{\boldmath $#1$}}
%\newcommand\cat[1]{\catname{#1}}
%\newcommand\categoryop[1]{\mbox{\bfseries\itshape #1}$^{\mathrm{op}}$}
%\newcommand\catnamei[1]{{\pmb #1}}



%\newcommand\idmap[1]{\operator{id}_{#1}}
%\renewcommand\f{\mbox{$\phi$}}
%\renewcommand\c{\catname{C}}
%\renewcommand\b{\catname{B}}
%\renewcommand\r{\catname{R}}





\newcommand\clonet{\mbox{${\nia}_\mathrm{Top}$}}
\newcommand\clonem{\mbox{${\nia}_\mathrm{MMt}$}}
%
% -- overlined letters for clones ---
%\newcommand\clonet{\mbox{$\overline{\nia}_\mathrm{Top}$}}
%\newcommand\clonem{\mbox{$\overline{\nia}_\mathrm{MMt}$}}



%==1.2 Classes of nodes/arrows
\newcommand\indclassofitems[1]{{\cal #1}}
\newcommand\classofitems[1]{\mbox{$\indclassofitems{#1}$}}
\newcommand\coi[1]{\classofitems{#1}}
\newcommand\incls{\coi{I}}
\newcommand\covers{\coi{C}}
\newcommand\univs{\coi{U}}
%\renewcommand\diags{\classofitems{D}}
\renewcommand\diags{\mathit{Diags}}
\newcommand\inddiags{\indclassofitems{D}}

%\newcommand\attrset[1]{\mbox{\textit{attrs}$(#1)$}}
%\newcommand\refset[1]{\mbox{\textit{refs}$(#1)$}}
%\newcommand\varset[1]{\mbox{\textit{vars}$(#1)$}}
%\newcommand\classtab[1]{\mbox{\textsf{tab}$_#1$}}
%\newcommand\attrtab[1]{\mbox{\textsf{aTab}$_#1$}}
%\newcommand\reftab[1]{\mbox{\textsf{rTab}$_#1$}}



%===1.3 Languages
\newcommand\querylanguage[1]{\nicex{ QL_{#1}$}}
\newcommand\ql{\querylanguage}
\newcommand\qlmath[1]{{\cal QL}_{#1}}

%%% 2. MMt Objects
\renewcommand\modelob[1]{\mbox{$M_{#1}$}}
\newcommand\schemaobsymbol{S}
\newcommand\typeSyssymbol{Types}
\newcommand\instanceGraphSymbol{I}
\newcommand\relschemaobsymbol{R}
\newcommand\skeobsymbol{S}
\newcommand\universesymbol{U}
\newcommand\valueUniverseGraphSymbol{U}
\newcommand\UniverseGraphSymbol{U}
\newcommand\schemaob[1]{\mbox{${\mathit \schemaobsymbol}_{#1}$}}
%\newcommand\typesys[1]{\mbox{${\mathit \schemaobsymbol}_{#1}$}}
\newcommand\instgra[2]{\mbox{${\mathit \instanceGraphSymbol}_{#1}^{#2}$}}
\newcommand\igra[2]{\instgra{#1}{#2}}
\newcommand\itogra[1]{\instgra{}{#1}}
\newcommand\irefgra[1]{\instgra{ref}{#1}}
\newcommand\iattgra[1]{\instgra{attr}{#1}}
\newcommand\iobjgra[1]{\instgra{obj}{#1}}

\newcommand\uvalgra[1]{\mbox{$\mathit{\universesymbol Val}_{#1}$}}
\newcommand\utupgra[1]{\mbox{$\mathit{\universesymbol Tuple}_{#1}$}}
\newcommand\uval{\uvalgra{}}
\newcommand\utup{\utupgra{}}
\renewcommand\uniob[1]{\mbox{$\mathsf{\universesymbol}_{#1}$}}

\newcommand\relsob[1]{\mbox{${\mathit \relschemaobsymbol}_{#1}$}}
\newcommand\newrelske[1] {\mbox{${\mathsf R}_{#1}$}}
\newcommand\newrelinst[2]{\mbox{${\mathsf Q}_{#1}^{#2}$}}

\newcommand\schemaOB[2]{\mbox{${\mathit \schemaobsymbol}_{#1}^{#2}$}}

\newcommand\claske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{cla}#1}$}}
\newcommand\refske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{ref}#1}$}}
\newcommand\attrske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{attr}#1}$}}
\newcommand\objrefske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{objRef}#1}$}}


\renewcommand\skeob[1]{\mbox{${\mathsf\skeobsymbol}_{#1}$}}
\newcommand\skeobind[1]{{\mathsf \skeobsymbol}_{#1}}
\newcommand\indskeob[1]{\skeobind{#1}}

\newcommand\typeske[1]{\mbox{$\mathsf{Type}_{#1}$}}
\newcommand\typemap[1]{\mbox{$\mathsf{type}_{#1}$}}
\newcommand\typeskeind{\mathsf{Type}}
\newcommand\typemapind[1]{\mathsf{type}_{#1}}

\renewcommand\statemap{\mbox{$\sigma$}}
\newcommand\statemapind{\sigma}




%\newcommand\gs{\mbox{$G_{\indskeob{}}$}}
%\newcommand\ds{\mbox{$\diags_{\indskeob{}}$}}
%\newcommand\gsi[1]{\mbox{$G_{\indskeob{#1}}$}}
%\newcommand\dsi[1]{\mbox{$\G_{\indskeob{#1}}$}}

%%% 2.1  Vectors of objects (bold objects)
%\newcommand\fullvector[3]{}
%\newcommand\vectorobject[1]{\mbox{$\boldsymbol{#1}$}} % see macros4names
\newcommand\multisch{\vectorobject{\schemaobsymbol}}
\newcommand\multiSch{\vectorobject{\schemaobsymbol}}
\newcommand\multinst{\vectorobject{\instancesymbol}}
\newcommand\multinstoo[1]{\mbox{$\multinst=(\inst{1},\ldots,\inst{#1})$}}

\newcommand\multiUni{\vectorobject{\universesymbol}}
\newcommand\multiRel{\vectorobject{\relschemaobsymbol}}
\newcommand\multiuni{\vectorobject{u}}
\newcommand\multirel{\vectorobject{r}}
\newcommand\multiu{\vectorobject{u}}
\newcommand\multir{\vectorobject{r}}
\newcommand\multiroo[1]{\mbox{$\multir=(r_1,\ldots,r_{#1})$}}


%== Operators
\newcommand\operator[1]{\mbox{\sf #1}}
\newcommand\operatorInIndex[1]{{\sf #1}}

\newcommand\heoperator[1]{\mbox{\sf\bfseries #1}}
\newcommand\match{\operator{match}}

\newcommand\indexedoperator[3]{\mbox{\operator{#1}$_{#2}^{#3}$}}
\newcommand\indexedoperatorInIndex[3]{\operatorInIndex{#1}_{#2}^{#3}}

\newcommand\der[2]{\indexedoperator{der}{#1}{#2}}
\newcommand\dero[1]{\indexedoperator{der}{}{#1}}
\newcommand\derInIndex[2]{\indexedoperatorInIndex{der}{#1}{#2}}

%\newcommand\proj[1]{\indexedoperator{p}{#1}{}}
%\newcommand\merge{\operator{merge}}
%\newcommand\modgen{\operator{modelGen}}
%\newcommand\datatrans{\operator{dataTransf}}
%\renewcommand\self{\operator{self}}


\newcommand\SFW[3]{\mbox{\operator{Select} #1
                         \operator{from} #2
                         \operator{where} #3}
                         }

%=====================
%\input{../../Tools/Macros/m20-newMacros}
%\renewcommand\em[1]{\emph{#1}}

%\newcommand\vect[1]{\textbf{#1}}
\newcommand\veg{\vect{G}}
\newcommand\vef{\vect{f}}
\newcommand\ver{\vect{R}}
\newcommand\ves{\vect{S}}
\newcommand\vehh{\vect{H}}
\newcommand\veho{\vect{\ovr{H}}}
\newcommand\veh{\vect{h}}

\newcommand\ovr[1]{\mbox{$\overline{\mathstrut#1}$}}
\newcommand\ovri[1]{\overline{#1}}
\newcommand\ovh[1]{\ovr{H}_{#1}}
%\newcommand\ovri[1]{\mb{\ovr{\iota'}_{#1}}}

\newcommand\edge[1]{\ittt{Edge}\mb{_{#1}}}
\newcommand\Edge[2]{\ittt{Edge}\mb{_{#1}^{#2}}}


\newcommand\univarr[1]{\mb{!_{#1}}}
\newcommand\doublearrow[5]{\mbox{$#1\stackrel{#4}{\rightarrow}
                                 #2\stackrel{#5}{\rightarrow}#3$
}}
\newcommand\arrdou[5]{\doublearrow{#1}{#2}{#3}{#4}{#5}}
\newcommand\arrarr{\arrdou{\gra{2}}{\gra{3}}{\gra{4}}{h_2}{h_3}}
\newcommand\scearr{\arrdou{\gra{2}}{\gra{1}}{\gra{0}}{\tau_1}{\tau_0}}
\newcommand\arrsce{\arrdou{\gra{2}}{\gra{1}}{\gra{0}}{\tau_1}{\tau_0}} % the same as above

\newcommand\arrspan[5]{\fbox{$#1\stackrel{#4}{\leftarrow}
                                 #2\stackrel{#5}{\rightarrow}#3$
}}
\newcommand\arrcospan[5]{\fbox{$#1\stackrel{#4}{\rightarrow}
                                 #2\stackrel{#5}{\leftarrow}#3$
}}

%\renewcommand\span[1]{\textbf{R}\mb{_{#1}}}
\newcommand\cospan[1]{\textbf{S}\mb{_{#1}}}
\newcommand\set[2]{\mb{#1=\{#2\}}}

\newcommand\integr[3]{\mb{#1\bigoplus_#3 #2}}

\newcommand\gran[1]{\mb{G_{{#1}N}}}
\newcommand\gred[1]{\mb{G_{{#1}E}}}
\newcommand\graman[1]{\mb{f_{{#1}N}}}
\newcommand\gramed[1]{\mb{f_{{#1}E}}}
\newcommand\grinman[1]{\mb{\iota'_{{#1}N}}}
\newcommand\grinmed[1]{\mb{\iota'_{{#1}E}}}

% changing from \mathsl to \mathit
\renewcommand\object[2]{\mbox{${\mathit{#1}}_{#2}$}}
\renewcommand\objectind[1]{\mathit{#1}}
\renewcommand\objectmath[1]{\mathit{#1}}

%\newcommand\DOM[1]{\Box #1}
%\newcommand\COD[1]{#1 \Box}


\newcommand\mb[1]{\mbox{$#1$}}
\newcommand\nin{\mb{\cal N}}
\newcommand\nix{\mb{\cal X}}
\newcommand\nil{\mb{\cal L}}
\newcommand\nik{\mb{\cal K}}
\newcommand\dvet{\mbox{:}}
\newcommand\ddvet{\dvet\dvet}
%\newcommand\n{\mb{n}}

\renewcommand\x{\mb{X}}

\newcommand\proxx[2]{\mb{\prod_{#1}{#2}}}
\newcommand\prox{\proxx{}{\vex}}
\newcommand\proy{\proxx{}{\vey}}
\newcommand\prodxn{\proxx{\cal L}{\vex}}
\newcommand\prodxm{\proxx{\cal K}{\vex}}

\newcommand\unixx[2]{\mb{\bigcup_{#1}{#2}}}
\newcommand\unix{\unixx{}{\vex}}

\newcommand\proj[1]{\mb{\ell_{#1}}}
\newcommand\proji{\proj{i}}






\renewcommand\ext{\mbox{\textsf{ext}}}








\newcommand\oclar{\mbox{\footnotesize $>$}}
\newcommand\myendset[1]{\mbox{$\{#1_1..#1_m\}$}}
\newcommand\fens{\myendset{f}}





\newcommand\fulla[1]{\mbox{${\mathbf F}_{#1}$}}
\newcommand\rmap[1]{\mbox{$#1^\rightarrow$}}
\newcommand\lmap[1]{\mbox{$^\leftarrow #1$}}
\newcommand\basemap[1]{\mbox{\textit{base}$_{#1}$}}


\newcommand\seq[1]{\textsf{seq}\mbox{$#1$}}
\newcommand\coll[2]{\textsf{coll}\mbox{$_{#1}(#2)$}}

\newcommand\tabschema{\mbox{$D=\{a_1:D_1,...,a_n:D_n\}$}}
\newcommand\tabschemamap{\mbox{\lar{D}{\attrset{}}{\setcat}}}



%=====================
%\input{../../Tools/Macros/m21--labelsnewMacros}
%(left) labels for formulas
\newcommand\equationNumber[1]{(\textsf{#1})}
\newcommand\eqnumber[1]{\equationNumber{#1}}
\newcommand\eqn[1]{\equationNumber{#1}}


%\newcommand\mafo[2]\mathform{#1}{#2}
\newcommand\mathfo[2]{$$#2\leqno{\mbox{(\textsf{#1})}} $$}
\newcommand\mafo[2]{$$#2 \leqno{\mbox{\eqn{#1}}} $$}


\newcommand\selflab{\eqn{self}}
\newcommand\looplab{\eqn{loop}}
\newcommand\idlelab{\eqn{idle}}
\newcommand\dolab{\eqn{do}}
\newcommand\triglab{\eqn{trigger}}

\newcommand\assonla{\eqn{fullAsson}}
\newcommand\tabla{\eqn{TAB}}
\newcommand\invla{\eqn{inverse}}
\newcommand\extla{\eqn{extension}}
\newcommand\tablatup{\eqn{TABrow}}
\newcommand\tablapro{\eqn{TABattr}}
\newcommand\sepla{\eqn{1-1}}
%=====================================
\newcommand\classn{\eqnumber{classn}}
\newcommand\indexn{\eqnumber{indexng}}

\newcommand\igralabel{\eqnumber{instGra}}
\newcommand\schemaGeneralLabel{\eqnumber{schemaGen}}
\newcommand\stlabel{\schemaGeneralLabel}
\newcommand\itablabel{\eqnumber{instTab}}
%\renewcommand\uniob[1]{\mbox{${\mathsf\universesymbol}_{#1}$}}
\newcommand\igratablabel{\eqnumber{instGraTab}}
\newcommand\igragralabel{\eqnumber{instGraGra}}
\newcommand\itabtablabel{\eqnumber{instTabTab}}

%=====================
%\input{../Tools/Macros/m21--abbrev4formulas}
%\input{../Tools/Macros/m22--abbrev4text}
%--------------------------------
%\renewcommand\zdmargin[1]{}
%\renewenvironment{razd}[2]{\subsubsection{#1}}{}
%\nocite{}
\renewenvironment{razD}[2]{\beginRazD{{%\itshape
                                      \bfseries #1}}}{\EndRazD}

%% sle
%%%%%%%%%% sle09 macros
%\newcommand\diagi[1]{#1\mbox{$'$}}
%\newcommand\diagii[1]{#1\mbox{$''$}}
%
%\newcommand\ari[1]{\mbox{\textsl{ar}$(#1)$}}
%\newcommand\mmname[1]{\textsf{#1}}
%\newcommand\mmcd{\mmname{CD}}
%\newcommand\mmsd{\mmname{SD}}
%\newcommand\mmsc{\mmname{SC}}
%\newcommand\mmca{\mmname{CA}}
%\newcommand\mmamt{\mmname{CAT}}
%\newcommand\mmcat{\mmname{CAT}}
%\newcommand\cd{\mmname{cd}}
%\renewcommand\sd{\mmname{sd}}
%\renewcommand\sc{\mmname{sc}}
%\newcommand\ca{\mmname{ca}}
%\newcommand\amt{\mmname{cat}}
%\renewcommand\cat{\mmname{cat}}
%\newcommand\cdi{\diagi{\cd}}
%\renewcommand\sdi{\diagi{\sd}}
%\newcommand\sci{\diagi{\sc}}
%\newcommand\cdii{\diagii{\cd}}
%\newcommand\sdii{\diagii{\sd}}
%\newcommand\scii{\diagii{\sc}}





\newcommand\base{\mbox{$\pmb{MM}$}}
\newcommand\p{\textbf{P}}
\newcommand\ps{\mbox{$P$}}
\newcommand\leqnoo[1]{\leqno{\mbox{#1}}}

\newcommand\keyword[1]{{\itshape\textsf{#1}}}
\newcommand\nam{\keyword{name}}
\renewcommand\owner{\keyword{owner}}
\newcommand\type{\keyword{type}}
\newcommand\val{\keyword{value}}
\newcommand\Class{\keyword{Class}}
\renewcommand\Attr{\keyword{Attr}}
\newcommand\Type{\keyword{Type}}
\newcommand\elm[1]{\mbox{$\mathit{El}(#1)$}}

\newcommand\ueq{\mbox{$\leftrightarrow$}}
\newcommand\uneq{\mbox{$\rightsquigarrow$}}

\newcommand\meq{\mbox{$=$}}
\newcommand\mneq{\mbox{$\neq$}}


\newcommand\shot{\textsl{shot}}
\newcommand\reltile{\textsl{relTile}}
%\newcommand\tauh{\mbox{$\tau_{\textsf{h}}$}}
%\newcommand\tauv{\mbox{$\tau_{\textsf{v}}$}}



\newcommand\vso{\textsf{v}\mbox{$\partial_0$}}
\newcommand\vta{\textsf{v}\mbox{$\partial_1$}}
\newcommand\hso{\textsf{h}\mbox{$\partial_0$}}
\newcommand\hta{\textsf{h}\mbox{$\partial_1$}}

\newcommand\mmod{\nicex{ M$}}
\newcommand\id{\textsl{id}}
\renewcommand\id{\mbox{$\iota$}}
\newcommand\recon[1]{\mbox{$#1$\textbf{!}}}

\newcommand\oidd[1]{\mbox{$\overline{#1}$}}
\newcommand\oiddi[1]{\mbox{$\overline{#1}'$}}

\renewcommand\oidd[1]{\mbox{${#1}$}}
\renewcommand\oiddi[1]{\mbox{${#1}'$}}

\newcommand\oa{\oidd{a}}
\newcommand\ob{\oidd{b}}
\newcommand\oP{\oidd{P}}
\newcommand\oQ{\oidd{Q}}

\newcommand\oai{\oiddi{a}}
\newcommand\obi{\oiddi{b}}
\newcommand\oPi{\oiddi{P}}
\newcommand\oQi{\oiddi{Q}}

% icmt

%%% icmt09 macros
% the % piece below  was moved to newMacros ---
\newcommand\mrkoprr[1]{\mrkopr{\mrkopr{#1}}}
%\der{}{Q}
%\newcommand\mmview[1]{\mbox{$\textsl{v}_{#1}$}}
%\newcommand\mmarr{v}
\newcommand\mmf{\mbox{$m$}} % to be used in the row
%\renewcommand\mmview[1]{\mbox{$\pmb{\mmarr}_{#1}$}}
%%\newcommand\mmv[1]{{\pmb{\mmarr}_{#1}}} %for subscripts
%\newcommand\mmmap[1]{\mbox{$\pmb{\mmarr}_{#1}$}}
%\renewcommand\mmm{m}  % to be used for sub-sup-indexes
%\newcommand\mmap[1]{\mbox{${\mmarr}_{#1}$}}

\newcommand\unde[1]{\underline{#1}}

\newcommand\oversi[1]{\overline{\sigma}^{#1}}

\newcommand\oversig[1]{\overline{\sigma}^{Q#1}}
\newcommand\overtau[1]{\overline{\tau}^{Q#1}}
\newcommand\overover{\overline{\oversig{1}}}
\newcommand\doublesig{{\overover^{Q2}}} %
\newcommand\votono{{\overline{\oversig{}}^{R}}}

\newcommand\derqq[2]{\mbox{$\dero{Q#1}#2$}}
\newcommand\dermms[1]{\derqq{#1}{\mms}}
\newcommand\derms[1]{\derqq{#1}{\ms{}}}
\newcommand\derqmms{\derqq{}{\mms}}
\newcommand\derqms{\derqq{}{\ms{}}}
\newcommand\derq[1]{\mbox{$\der{}{Q}#1$}}
\newcommand\doubleder[1]{\derqq{1;Q2}{#1}}

\newcommand\augtymaps{\flar%
{\overline{\sigma}^{Q}}%
{\dero{Q}\ms{}}%
{\dero{Q}\mms}%
}
%\newcommand\mmarr{\mbox{$m$}}

%
\newcommand\tracemap[1]{\mbox{$\stackrel{\rightsquigarrow}{#1}$}}
\renewcommand\tracemap[1]{\mbox{$\mathit{tr}_{#1}$}}
\renewcommand\tracemap[1]{\mbox{$#1^{*}$}}
\newcommand\tram{\tracemap{\mmmap}}
%
\newcommand\reversemap[1]{\mbox{\spf$_{#1}$}}
%\newcommand\revem{\reversemap{\mmview{}}}
\newcommand\revem[1]{\mbox{$\semm{\mmmap{#1}}$}}

\renewcommand\s[1]{\mbox{$S_{#1}$}}
\renewcommand\ms[1]{\mbox{$S_{#1}$}}
\newcommand\mos[1]{\mbox{$\overline{S}_{#1}$}}
\renewcommand\mt[1]{\mbox{$T_{#1}$}}
\newcommand\mot[1]{\mbox{$\overline{T}_{#1}$}}
\newcommand\mh[1]{\mbox{$H_{#1}$}}
\renewcommand\ml[1]{\mbox{$L_{#1}$}}

\newcommand\pbop{\operator{PB}}

\newcommand\msarr{\flar{\sigma}{S}{\mms}}
\newcommand\msarrq{\flar{\overline{\sigma}^{Q}}{\der{}{Q}S}{\der{}{Q}\mms}}
\newcommand\mssym{\mbox{$\overline{\sigma}$}}
\newcommand\mssymq{\mbox{$\overline{\sigma}^Q$}}

\newcommand\mtarr{\flar{\tau}{T}{\mmt}}
\newcommand\srelarr{\flar{\sigma}{S}{\mmrel}}
\newcommand\erdarr{\flar{\tau}{D}{\mmer}}
\newcommand\srelderarr[1]{\flar{\overline{\sigma}^{Q#1}}{\der{}{Q#1}S}{\der{}{Q#1}\mmrel}}



\newcommand\ertorel[1]{\flar{\textsf{er2rel}_{#1}}{\mmer}{\mmrel}}
\newcommand\ertorelder[1]{\flar{\textsf{er2rel}_{#1}}{\mmer}{\der{}{{Q#1}}\mmrel}}

% gttse

%\renewcommand\mmname[1]{\mbox{$\pmb{\cal #1}$}}
%\newcommand\mmmapname[1]{\mbox{$\pmb{#1}$}}
%\newcommand\mma{\mmname{M}}
%\newcommand\mmb{\mmname{N}}
%\newcommand\mmc{\mmname{O}}
%\newcommand\mmr[1]{\mbox{\mmname{R}$_{#1}$}}
%\renewcommand\mmr[1]{\mbox{$\pmb{r}_{#1}$}}
%\newcommand\mmab{\mmname{MN}}
%\newcommand\mmac{\mmname{MO}}
%\newcommand\mmv{\mmmapname{v}}
%\newcommand\mmw{\mmmapname{w}}
%\newcommand\mmp{\mmmapname{p}}
%\newcommand\mmq{\mmmapname{q}}

\renewcommand\dvet{\mbox{:\,}}

\newcommand\newrevem[1]{\mbox{$\semm{\mmmapname{#1}}$}}
\newcommand\rev{\newrevem{v}}
\newcommand\rew{\newrevem{w}}
\newcommand\rep{\newrevem{p}}
\newcommand\req{\newrevem{q}}


\newcommand\mmnamei[1]{\pmb{\cal #1}}
\newcommand\mmabi{\mmnamei{MN}}
\newcommand\mmaci{\mmnamei{MO}}
\newcommand\amn{\mbox{$A_{\mmabi}$}}
\newcommand\bmn{\mbox{$B_{\mmabi}$}}
\newcommand\amnprim{\mbox{$A'_{\mmabi}$}}
\newcommand\bmnprim{\mbox{$B'_{\mmabi}$}}
\newcommand\amo{\mbox{$A_{\mmaci}$}}
\newcommand\cmo{\mbox{$C_{\mmaci}$}}
\newcommand\umn{\mbox{$u_{\mmabi}$}}
\newcommand\vmn{\mbox{$v_{\mmabi}$}}

\newcommand\lmmes{\left] \respace\left] }
\newcommand\rmmes{\right[\respace\right[}
\newcommand\mmes[1]{\mbox{$\lmmes\, \mathit{#1} \, \rmmes$}}

% spans

\newcommand\spancat{\category{Span}}
\newcommand\spansa{\scat\spancat}
\newcommand\spanset{\setcat\spancat}
\newcommand\cospancat{\category{Cospan}}
\newcommand\cospansa{\scat\cospancat}
\newcommand\cospanset{\setcat\cospancat}


\newcommand\spanfull[4]{\mbox{${\cal #1}$=(\flar{#2_i}{#3}{#4 i},
$i=1,2)$}}

\newcommand\lKleisly{\Leftarrow}
\newcommand\rKleisly{\Rightarrow}
\newcommand\spandiag[5]  {\fbox{$#1\lTo^{#2} #3 \rTo^{#4} #5$}}
\newcommand\kleispandiag[5]{\fbox{$#1\lKleisly^{#2} #3 \rKleisly^{#4} #5$}}
\newcommand\kleislispandiag[5]{\fbox{$#1\lKleisly^{#2} #3 \rKleisly^{#4} #5$}}
\newcommand\cospandiag[5]{\fbox{$#1\rTo^{#2} #3 \lTo^{#4} #5$}}
\newcommand\kleicospandiag[5]{\fbox{$#1\rKleisly^{#2} #3 \lKleisly^{#4} #5$}}
\newcommand\kleislicospandiag[5]{\fbox{$#1\rKleisly^{#2} #3 \lKleisly^{#4} #5$}}


\newcommand\flarsemm[3]{\flar{#1}{\semm{#2}}{\semm{#3}}}
\newcommand\spandiagsemm[5]{\fbox{$\semm{#1}\lTo^{#2} \semm{#3} \rTo^{#4} \semm{#5}$}}
\newcommand\cospandiagsemm[5]{\fbox{$\semm{#1}\rTo^{#2} \semm{#3} \lTo^{#4} \semm{#5}$}}


%=== with brackets
\newcommand\spandiagbra[5]
{\mbox{$%\left %
(#1\stackrel{~#2}{\leftarrow} #3
                                           \stackrel{#4~}{\rightarrow} #5%\right
)$}}
\renewcommand\kleispandiag[5]{\mbox{$\left(#1\stackrel{~#2}{\lKleisly} #3
                                             \stackrel{#4~}{\rKleisly} #5
                                             \right)$}}
\renewcommand\kleislispandiag[5]{\mbox{$\left(#1\stackrel{#2}{\lKleisly} #3
                                             \stackrel{#4}{\rKleisly} #5
                                             \right)$}}
\renewcommand\kleicospandiag[5]{\mbox{$\left(#1\stackrel{#2}{\rKleisly} #3
                                             \stackrel{#4}{\lKleisly} #5
                                             \right)$}}
\renewcommand\kleislicospandiag[5]{\mbox{$\left(#1\stackrel{#2}{\rKleisly} #3
                                             \stackrel{#4}{\lKleisly} #5
                                             \right)$}}

\renewcommand\cospandiag[5]{\mbox{$\left(#1\rTo^{#2} #3 \lTo^{#4} #5\right)$}}
\renewcommand\cospandiag[5]  {\mbox{$\left(#1\stackrel{~#2}{\rightarrow} #3
                                           \stackrel{#4~}{\leftarrow} #5\right)$}}

% without brackets
\renewcommand\spandiag[5]  {\mbox{$#1\stackrel{~#2}{\leftarrow} #3
                                           \stackrel{#4~}{\rightarrow} #5$}}
\renewcommand\cospandiag[5]  {\mbox{$#1\stackrel{~#2}{\rightarrow} #3
                                           \stackrel{#4~}{\leftarrow} #5$}}


%\renewcommand\kleislycospandiag[5]{\mbox{$\left(#1\rKleisly^{#2} #3 \lKleisly^{#4} #5\right)$}}

\renewcommand\flarsemm[3]{\flar{#1}{\semm{#2}}{\semm{#3}}}
\renewcommand\spandiagsemm[5]{\mbox{$\left(\semm{#1}\lTo^{#2} \semm{#3}\rTo^{#4} \semm{#5}\right)$}}
\renewcommand\cospandiagsemm[5]{\mbox{$\left(\semm{#1}\rTo^{#2} \semm{#3}\lTo^{#4} \semm{#5}\right)$}}


%% end macros



%%==== end newMacros


==> macros/4lenses/macros4drawingTiles.tex <==
%\newcommand\xx{\!\!}
%\newcommand\xxx{\!\!\!}
%\newcommand\xxxx{\xxx\xx}

\newcommand\qryincl[2]{\mathsf{i}_{#1}^{#2}}
\newcommand\qryinclq[1]{\qryincl{#1}{Q}}
\newcommand\liftqryincl[2]{\ovr{\mathsf{i}_{#1}^{#2}}}
\newcommand\liftqryinclq[1]{\liftqryincl{#1}{Q}}


\newcommand\arrONarr{\stackrel{\mbox{$\longrightarrow$}}{\smash{\longrightarrow}}}
\newcommand\eeTilearrow[1]{\stackrel{#1}{\smash{\arrONarr}}}
%\newcommand\seTilearrow[2]{\searrow\xxx\xx\searrow{\mathsf{#1}_{#2}^{\mathstrut}}}

% NE staff
%\newcommand\mrklab[1]{\diagopername{#1}}
\newcommand\neTilearrowAB[2]{\mrklab{#1}
           \lefteqn{\,\nearrow\xxx\xx\nearrow}{\mrklab{#2}}
}
\newcommand\neqExeLabel{\neTilearrow{qEx}{e}}
\newcommand\seqExeLabel{\seTilearrow{qEx}{e}}
\newcommand\sevExeLabel{\seTilearrow{vEx}{e}}
\newcommand\nevExeLabel{\neTilearrow{vEx}{e}}
\newcommand\nePBLabel{\neTilearrow{p}{b}}
\newcommand\sePBLabel{\seTilearrow{p}{b}}
\newcommand\neCommLabel{\neTilearrow{[;]}{\xx}}
% SE staff
%\newcommand\seTilearrow[2]{\mrklab{#1}
%           \lefteqn{\searrow\xxx\xx\searrow}{\mrklab{#2}}
%}



\newcommand\seTilearrowHru[1]{%\mrklab{#1}
%           \lefteqn{\searrow\xxx\xx\searrow}{\mrklab{#2}}
 \lefteqn%
 {~~#1}{\searrow\xxx\xx\searrow}
} %
%%%% Oct 13 %%%%%
%\renewcommand\seTilearrowHru[1]{%\mrklab{#1}
%%           \lefteqn{\searrow\xxx\xx\searrow}{\mrklab{#2}}
% \lefteqn%
% {#1}{\searrow\xxx\xx\searrow}
%} %
%%%%%%%%%%%%%%%



%\newcommand\swTilearrowHru[1]{%\mrklab{#1}
%%           \lefteqn{\searrow\xxx\xx\searrow}{\mrklab{#2}}
% \lefteqn%
%         {~~#1}{\swarrow\xxx\xx\swarrow}
%}

\newcommand\ssTilearrow[2]{\downarrow\xxx\xx\downarrow^{#1_{#2}^{\mathstrut}}}
\newcommand\ssTilearrowHru[1]{\lefteqn%
{~~#1} \downarrow\xx\xx\downarrow}

% short names
\newcommand\seTilelabel[1]{\seTilearrowHru{#1}}
\newcommand\swTilelabel[1]{\swTilearrowHru{#1}}
\newcommand\ssTilelabel[2]{\ssTilearrowHru{#1}}


\newcommand\sefPrpLabel{\seTilearrow{[fPp}{]}}

% SW stuff
%\newcommand\swTilearrow[2]{\mrklab{#1}
%           \lefteqn{\mrklab{#2}}{\swarrow\xxx\xx\swarrow}
%}

%\renewcommand\swTilearrow[2]{{#1}
%           %\lefteqn
%           {\swarrow\xxx\xx\swarrow}{{#2}}
%}

\newcommand\swbPrpLabel{\swTilearrow{[bPp}{]}}

%\newcommand\swTilearrow[2]{\swarrow\xxx\xx\swarrow^{#1_{#2}^{\mathstrut}}}
% NN stuff
\newcommand\nnTilearrow[2]{\downarrow\xxx\xxx\xx\downarrow^{#1_{#2}^{\mathstrut}}}
\renewcommand\nnTilearrow[2]{\mrklab{#1}\!
           \lefteqn{\uparrow\xxx\xx\uparrow}{\mrklab{#2}}
}
%\renewcommand\nnTilearrow[2]{\mrklab{#1}^{
%              {\uparrow}\!{\uparrow}
%            } %{\mrklab{#2}}
%}
\newcommand\nnsubstLabel{\nnTilearrow{subst~}{}}

\newcommand\seselabel{~~~\seTilearrow{}{}~~~}
\newcommand\swswlabel{~~~\swTilearrow{}{}~~~}



\newcommand\rBlockarrow{\rule{0.25pt}{4.pt}\xx\Rrightarrow}
\newcommand\lBlockarrow{\Lleftarrow\xx\rule{0.25pt}{4.pt}}
\newcommand\sBlockarrow{\downarrow\xx\downarrow\xx\downarrow}
\renewcommand\sBlockarrow{\Downarrow\xxx\Downarrow}
\newcommand\rBlockarrowII{\mbox{$\sqsubset\xx\sqsupset$}\xx\LARGE{\rhd}}


==> macros/4lenses/macros4spaceNames.tex <==
\newcommand\colfunct{\ensuremath{\mathsf{Col}}}

% now spaces
\newcommand\metamodname[1]{\ensuremath{\mathsf{#1}}}
\renewcommand\metamodname[1]{\ensuremath{{\pmb{#1}}}}
\newcommand\metamapsymb[1]{\ensuremath{\pmb{#1}}}
\newcommand\classname[1]{\ensuremath{\pmb{#1}}}  %\itshape{\textbf{#1}}}
\newcommand\spacenam[1]{\ensuremath{\mathbf{#1}}}
%\newcommand\spacenamind[1]{\mathbf{#1}}
%\newcommand\arralgnam[1]{\ensuremath{{\pmb #1}}}
%\newcommand\spaalt{\arralgnam{alt}}

\newcommand\cfwkclass{\classname{CFwk}}
\newcommand\scclass{\classname{SCase}}
\newcommand\T{\classname{T}}

\newcommand\spaA{\ensuremath{\spacenam{A}}}
\newcommand\spaB{\ensuremath{\spacenam{B}}}
\newcommand\spaC{\ensuremath{\spacenam{C}}}

\newcommand\mmm{\ensuremath{\metamodname{M}}}
\newcommand\mmmd{\ensuremath{\mmm_\Delta}}
\newcommand\mmmdpri{\ensuremath{\mmm_\Delta^\priv}}
\newcommand\mmmdpub{\ensuremath{\mmm_\Delta^\pub}}
\newcommand\mmmob{\ensuremath{\mmm_\bullet}}
\newcommand\mmn{\ensuremath{\metamodname{N}}}
\newcommand\mmmn{\ensuremath{\metamodname{N}}}
\newcommand\mmnd{\ensuremath{\mmn_\Delta}}
\newcommand\mmndpri{\ensuremath{\mmn_\Delta^\priv}}
\newcommand\mmndpub{\ensuremath{\mmn_\Delta^\pub}}
\newcommand\mmnob{\ensuremath{\mmn_\bullet}}
\newcommand\mmmnob{\mmnob}
\newcommand\mmi{\ensuremath{\metamodname{I}}}
\newcommand\mmid{\ensuremath{\mmi_\Delta}}
\newcommand\mmiob{\ensuremath{\mmi_\bullet}}
\newcommand\mmj{\ensuremath{\metamodname{J}}}
\newcommand\mmjd{\ensuremath{\mmj_\Delta}}
\newcommand\mmjob{\ensuremath{\mmj_\bullet}}
\newcommand\mmo{\ensuremath{\metamodname{O}}}
\newcommand\mmr{\ensuremath{\metamodname{R}}}
\newcommand\mmrop{\ensuremath{\metamodname{R}^{{\circ}}}}
\newcommand\mmkop{\ensuremath{\metamodname{K}^{{\circ}}}}
\newcommand\mmrr{\ensuremath{\mmr_\bullet}}
\newcommand\mmrl{\ensuremath{{_\bullet}\mmr}}
\newcommand\mmk{\ensuremath{\metamodname{K}}}
\newcommand\mmkr{\ensuremath{\mmk_\bullet}}
\newcommand\mmkl{\ensuremath{{_\bullet}\mmk}}

\newcommand\mml{\ensuremath{\metamodname{L}}}
\newcommand\mms{\ensuremath{\metamodname{S}}}
\newcommand\mmsd{\ensuremath{\mms_\Delta}}
\newcommand\mmsob{\ensuremath{\mms_\bullet}}
\newcommand\mmv{\ensuremath{\metamodname{V}}}
\newcommand\mmvd{\ensuremath{\mmv_\Delta}}
\newcommand\mmld{\ensuremath{\mml_\Delta}}
\newcommand\mmrd{\ensuremath{\mmr_\Delta}}
\newcommand\mmvob{\ensuremath{\mmv_\bullet}}
\newcommand\mmrob{\ensuremath{\mmr_\bullet}}
\newcommand\mmlob{\ensuremath{\mml_\bullet}}
%\newcommand\ma{\trajectname{A}}
%\newcommand\mb{\trajectname{B}}

\newcommand\mmq{\metamodname{Q}}
%\newcommand\mmr{\metamodname{R}}
\newcommand\mmmrn{\metamodname{MRN}}

\endinput

\newcommand\mma[1]{\ensuremath{\metamodname{A}_{#1}}}
\newcommand\mmb[1]{\ensuremath{\metamodname{B}_{#1}}}
\newcommand\mmc[1]{\ensuremath{\metamodname{C}_{#1}}}
\newcommand\mmm[1]{\ensuremath{\metamodname{M}_{#1}}}
\renewcommand\mmm[1]{\ensuremath{\metamodname{V}_{#1}}}
\newcommand\mmn[1]{\ensuremath{\metamodname{N}_{#1}}}
\renewcommand\mmn[1]{\ensuremath{\metamodname{S}_{#1}}}
\newcommand\mmo[1]{\ensuremath{\metamodname{O}_{#1}}}
\newcommand\mmr[1]{\ensuremath{\metamodname{R}_{#1}}}
\newcommand\mmk[1]{\ensuremath{\metamodname{K}_{#1}}}
\newcommand\mms[1]{\ensuremath{\metamodname{S}_{#1}}}
\newcommand\mmv[1]{\ensuremath{\metamodname{V}_{#1}}}



\newcommand\mmmsub[1]{\ensuremath{\metamodname{M}^-_{#1}}}
\newcommand\mmnsub[1]{\ensuremath{\metamodname{N}^-_{#1}}}

\newcommand\mmmton{\metamodname{M_N}}
\newcommand\mmmx{\metamodname{M_N}}



%\newcommand\mmo{\metamapsymb{O}}
%\newcommand\mmr{\metamapsymb{r}}
%\newcommand\mmu{\metamapsymb{u}}
%\newcommand\mmv{\metamapsymb{v}}

% dyn metamod
\newcommand\dmmm[1]{\ensuremath{\spacenam{M}_{#1}}}
\newcommand\dmmn[1]{\ensuremath{\spacenam{N}_{#1}}}
\newcommand\dmmo[1]{\ensuremath{\spacenam{O}_{#1}}}


==> macros/4thisPaper-0.tex <==
\newcommand\incal{incremental}
\newcommand\mbcon{\ensuremath{\sim}}
\newcommand\hgg[1]{}
\newcommand\info{\ensuremath{\mathrm{inf}}}



\newcommand\boldsubsubsection[1]{\subsubsection*{\textbf{#1}}}
\renewcommand\boldsubsubsection[1]{\subsubsection*{{#1}}}
\newcommand\goup{\vspace{-7.5pt}}
\newcommand\rich{\ensuremath{\mathrm{+}}}
\newcommand\poor{\ensuremath{\mathrm{-}}}
\newcommand\ohtri{\ensuremath{(\ohafra\ohafra\ohafra)}}



\newcommand\alens{\ensuremath{\lambda}}
\newcommand\dbox[1]{\fbox{$#1$}}
% sub and super scripts
\newcommand\indname[1]{\ensuremath\mathrm{#1}}
\newcommand\priv{{\indname{prv}}}
\newcommand\pub{{\indname{pub}}}

\endinput













==> macros/citations.tex <==
%Tuy\'eras
\newcommand\citelongver[1]{\cite[#1]{myX-learning19}  }
\newcommand\citebaezncat{\cite{?}}
\newcommand\citefjbx{\cite{fj-bx19}}
\newcommand\citefj{\cite{fj-bx19}}
\newcommand\citefst{\cite{fst-backprop}}
\newcommand\citefstx[1]{\cite[#1]{fst-backprop}}
\renewcommand\citell{\citefst}
\newcommand\citepiercetr{\cite{?}[TR2003]}
\newcommand\citemakkai{\cite{makkai-ske}}
\newcommand\citefetal{\cite{fst-backprop,fj-bx19}}
\newcommand\citeeditlenses{\cite{bpierce-editlens,jr-unified}}
\newcommand\citejrunified{\cite{jr-unified}}
\newcommand\citejrunifiedX[1]{\cite[#1]{jr-unified}}
\newcommand\citemtex{\cite{mtbe-kappel12}} %[MT from examples]}
\newcommand\citemtbe{\cite{mtbe-kappel12}} %[MT from examples]}
\newcommand\citeao{\cite{alv-ong}}
\newcommand\citeaotr{\cite{alv-ong-tr}}
\newcommand\citeaotrx[1]{\cite[#1]{alv-ong-tr}}
%\newcommand\citeeditlenses{\cite{?}}
\newcommand\citedlenstgg{\cite{?}}
\newcommand\citebob{\cite{?}} % perrsonal comm. about pare
\newcommand\citeorsets{\cite{?}}

==> macros/macros-general.tex <==
\newcommand\bfem[1]{{\bf\em #1}}
\newcounter{defCounter}
\newenvironment{defin}[1][]{
	\refstepcounter{defCounter}
	\begin{trivlist}
		\item[\hskip \labelsep {\bfseries Definition \arabic{defCounter} (#1) }]
	}%
	{\end{trivlist}}

\newcommand\tcat{\catname{I\!\!I}}
\renewcommand\tcat{\enma{\mathbf{\large 1}}}
\newcommand\tfun{\enma{\mathit{1}}}

\newcommand\mono{\enma{\nmf{monic}}}
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand*{\textcal}[1]{%
	% family qzc: Font TeX Gyre Chorus (package tgchorus)
	% family pzc: Font Zapf Chancery (package chancery)
	\textit{\fontfamily{qzc}\selectfont#1}%
}

\DeclareMathAlphabet{\mathantt}{OT1}{antt}{li}{it}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\newcommand\ensureamth[1]{\ensuremath{#1}}

% == rotation command
%\rotatebox[origin=c]{45}{$xxx$} 
\newcommand\qqquad{\qquad\quad}
\newcommand\qqqquad{\qquad\qquad}
%\newcommand{\tmapleft[2]}{\ensuremath{#1}}
%\newcommand\mysectpar{\par\medskip}
%\newcommand\mysection[1]{\mysectpar\noindent{\rm \bfseries{\large #1.}}}
%%\renewcommand\mysection[1]{\section{#1}}
%\newcommand\myitempar{\par}
%\newcommand\myitem[1]{\myitempar{\bf #1.}}
%
%\newcommand\mysubsection[1]{\vspace{-1.ex}\subsection{#1}\vspace{-0.65ex}}
%\newcommand\mysubsubsection[2]{\vspace{#2}\subsubsection{#1}} 
%%  another version
%%\renewcommand\mysubsubsection[1]{\par\smallskip\noindent {\bfseries\itshape{#1}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% == my font discipline for defs for Springer ==

%-- doesn't worl for Compisitinality
%\newenvironment{defin}[1][]{\ifthenelse{\equal{#1}{}}{\definition}{\definition[#1]}\rm}{\enddefinition}
%\newenvironment{propo}[1][]{\ifthenelse{\equal{#1}{}}{\proposition}{\proposition[#1]}\rm}{\endproposition}
%\newenvironment{remar}[1][]{\ifthenelse{\equal{#1}{}}{\remark}{\remark[#1]}\rm}{\endremark}
% \newtheorem{defin}{Definition}
% \newtheorem{corol}{Corollary}
% \newtheorem{theorem}{Theorem}
% \newtheorem{propo}{Proposition}
% \newtheorem{rema}{\textit{Remark}}
% \newtheorem{example}{Example}

%% ATTENTION PLS !
%  for Elsevieer, the above macros don't work, but versions below do work
% \let\oldexample=\example
% \let\endoldexample=\endexample
% \renewenvironment{example}{\vspace{-0.6em}\begin{oldexample}}{\end{oldexample}\vspace{-0.35em}}

% \let\olddefin=\defin
% \let\endolddefin=\enddefin
% \renewenvironment{defin}{\vspace{-0.6em}\begin{olddefin}}{\end{olddefin}\vspace{-0.5em}}

% \let\oldpropo=\propo
% \let\endoldpropo=\endpropo
% \renewenvironment{propo}{\vspace{-0.6em}\begin{oldpropo}}{\end{oldpropo}\vspace{-0.5em}}

% \let\oldrema=\rema
% \let\endoldrema=\endrema
% \newenvironment{rema}{\vspace{-0.6em}\begin{oldrema}}{\end{oldrema}\vspace{-0.5em}}

% \let\oldcorol=\corol
% \let\endoldcorol=\endcorol
% \newenvironment{corol}{\vspace{-0.6em}\begin{oldcorol}}{\end{oldcorol}\vspace{-0.5em}}

% \let\oldtheorem=\theorem
% \let\endoldtheorem=\endtheorem
% \renewenvironment{theorem}{\vspace{-0.6em}\begin{oldtheorem}}{\end{oldtheorem}\vspace{-


% math operations

\newcommand\opname[1]{\ensuremath{\mathsf{#1}}}
\newcommand\colim{\opname{colim}}
\newcommand\limcat{\opname{lim}}

%===== Calligraph. Literals ======
\newcommand\niceletter[1]{\ensuremath{{\cal #1}}}
\newcommand\nicex[1]{\niceletter{#1}}
\newcommand\nia{\nicex{A}}
\newcommand\nib{\nicex{B}}
\newcommand\nid{\nicex{D}}
\newcommand\nie {\nicex{E}}
\newcommand\nik {\nicex{K}}
\newcommand\nil {\nicex{L}}
\newcommand\nim{\nicex{M}}

\newcommand\nio{\nicex{O}}
\newcommand\nip{\nicex{P}}
\newcommand\nir{\nicex{R}}
\newcommand\nit{\nicex{T}}
\newcommand\niu{\nicex{U}}
\newcommand\niv{\nicex{V}}
\newcommand\niw{\nicex{W}}
\newcommand\nix{\nicex{X}}


% Domain-codomain/source-target/ident
\newcommand\cod[1]{\ensuremath{{#1}^\bullet}}
\newcommand\dom[1]{\ensuremath{^\bullet{#1}}}
\newcommand\so{\ensuremath{\mathsf{src}}}
\newcommand\ta{\ensuremath{\mathsf{trg}}}
\renewcommand\so{\ensuremath{\mathsf{s}}} % was src
\renewcommand\ta{\ensuremath{\mathsf{t}}}  % was trg
\newcommand\ldom[1]{\ensuremath{$\Box #1 $}}
\newcommand\rdom[1]{\ensuremath{$#1 \Box $}}
\newcommand\id[1]{\opname{id}_{{#1}}}
\renewcommand\id{\opname{id}}
\newcommand\Id[1]{\opname{Id}_{{#1}}}
\renewcommand\Id{\opname{Id}}

% fig and others references
\newcommand\figref[1]{Fig.~\ref{fig:#1}}
\newcommand\exref[1]{Example~\ref{ex:#1}}
\newcommand\defref[1]{Def.~\ref{def:#1}}
\newcommand\conref[1]{Constr.~\ref{con:#1}}
\newcommand\tabref[1]{Table~\ref{tab:#1}}
\newcommand\diagref[1]{(\ref{diag:#1})}
%\newcommand\eqref[1]{\ref{#1}}
\newcommand\sectref[1]{Sect.~\ref{sec:#1}}
\newcommand\secref[1]{Sect.~\ref{sec:#1}}
\newcommand\appref[1]{Appendix~\ref{#1}}
\renewcommand\eqref[1]{(\ref{eq:#1})}
%===============================================


% my macros for Formulas 

% roman font in math formulas
\newcommand\rmand{\mbox{ and }}
\newcommand\rmor{\mbox{ or }}
\newcommand\rmxor{\mbox{ xor }}

\newcommand\eqdef{\ensuremath{\stackrel{\mathrm{def}}{=}}}

% semantic brackets 
\newcommand\respace{\!}%\!\!}
\newcommand\lsemm{\left[ \respace\left[ }
\newcommand\rsemm{\right]\respace\right]}
\newcommand\semm[1]{\mbox{$\lsemm\, \mathit{#1} \, \rsemm$}}

% less blank space
\newcommand\timm{{\times}}
\newcommand\inn{{\in}}
\newcommand\subsett{{\subset}}
\newcommand\supsett{{\superset}}

%Suggestive Names for MathSymbols
\newcommand\superset{\supset}
\newcommand\subeq{{\subseteq}}
\newcommand\supeq{{\supseteq}}
\newcommand\sqsubeq{{\sqsubseteq}}
\newcommand\sqsupeq{{\sqsupseteq}}
\newcommand\varno{{\varnothing}}
\newcommand\subsetarr{\ensuremath{\hookrightarrow}}
\newcommand\supsetarr{\ensuremath{\hookleftarrow}}

\newcommand\this{\ensuremath{\underline{\mathrm{this}}}}
\newcommand\self{\ensuremath{\underline{\mathrm{self}}}}


\newcommand\ovr[1]{\ensuremath{\overline{#1}}}
\newcommand\und[1]{\ensuremath{\underline{#1}}}


\newcommand\rarr{{\rightarrow}}
%\newcommand\lar{\leftarrow}
\newcommand\larr{{\leftarrow}}
\newcommand\ifff{\Leftrightarrow}
\newcommand\iffarrow{\Leftrightarrow}
\newcommand\bottom{\perp}
\newcommand\disj{\vee}
\newcommand\sdisj{\stackrel{!}{\vee} }
\newcommand\conj{\wedge}
%\newcommand\mathand{\,\&\,}
\renewcommand\neg{\sim}
\newcommand\ded{\vdash}
\newcommand\semded{\models}
\newcommand\synent{\ensuremath{\vdah}}
\newcommand\sement{\ensuremath{\models}}

\newcommand\njoin[2]{\mathbin{${#1}\triangleright\!\triangleleft\;{#2}$}}

%\newcommand\ifthenelse[3]{{\bf if}#1{\bf then}#2{\bf else}#3}


\newcommand\true{\nmf{true}}
\newcommand\false{\nmf{false}}

% Operations 

\newcommand\image[2]{\opname{Image}_{#1}{#2}}
\newcommand\img[2]{\image{#1}{#2}}
%\newcommand\range[2]{\Operation{Range}_{#1}({#2})}

%\newcommand\aut{\ensuremath{\operation{Aut}}}
\newcommand\isoind{\opname{iso}}
\newcommand\iso{\isoind}

\newcommand\coimage[2]{\opname{CoIm}_{#1}{#2}}
\newcommand\coim[2]{\coimage{#1}{#2}}

\renewcommand\restriction[2]{#1\left\lceil_{#2}\mathstrut\right.}
\renewcommand\restriction[2]{\ensuremath{#1{\upharpoonright}_{#2}\mathstrut}}
\newcommand\restr[2]{\restriction{#1}{#2}}

\newcommand\idmap[1]{\Operation{id}_{#1}}

\newcommand\Inverse[1]{\left (\mathstrut {#1} \right )^{-1}}
%\newcommand\inverse[1]

%  Comprehension

\newcommand\comprehension[2]{\ensuremath{\left\{{#1}\left|\;{#2}\right.\right\}}}
\renewcommand\comprehension[2]{\ensuremath{\left\{{#1}| \;{#2}\right\}}}  % big brackets
\newcommand\comprehensionColon[2]{\ensuremath{\left\{{#1}{:} \;{#2}\right\}}}  % big brackets
%\renewcommand\comprehension[2]{\ensuremath{\{{#1}| \;{#2}\}}} % small brackets
\newcommand\compr[2]{\comprehension{#1}{#2}}
\newcommand\comprCol[2]{\comprehensionColon{#1}{#2}}
\newcommand\tuplecompr[2]
{\left\langle{#1}\left|\;{#2}\right.\right\rangle}
\newcommand\tuple[1]{\left\langle\mathstrut {#1}\right\rangle}
\newcommand\cotuplecompr[2]
{\left\rangle\mathstrut {#1}\left|\;{#2}\right.\right\langle}
\newcommand\cotuple[1]{\left\rangle\mathstrut {#1}\right\langle\;}
\newcommand\family[2]{\left(\mathstrut #1 \right)_{#2}}
\newcommand\famm[2]{\family{#1}{#2}}
% big brackets
\newcommand\comprfam[2]{\enma{\left(\mathstrut{#1}\left|\;{#2}\right.\right)}}
\newcommand\famcompr[2]{\left(\mathstrut{#1}\left|\;{#2}\right.\right)}
% normal brackets
\renewcommand\comprfam[2]{\enma{(\mathstrut{#1}\left|\;{#2}\right.)}}
\renewcommand\famcompr[2]{(\mathstrut{#1}\left|\;{#2}\right.)}
\newcommand\newfamm[2]{\compfamily{#1}{#2}}
\newcommand\arrfamm[4]{\family{%
		\lar{#1}{#2}{#3}%
	}{#4}}


\newcommand\cotimes{+}
\newcommand\noteq{\ne}
\newcommand\mybigcup[2]{\bigcup\compr{#1}{#2}}
\newcommand\mybigcap[2]{\bigcap\compr{#1}{#2}}

\newcommand\myprod[1]{{#1 \prod}}



%-- categories names
\newcommand\catname[1]{\mbox{\bfseries\itshape #1}}
\renewcommand\catname[1]{\enma{\pmb{#1}}}
%\newcommand\cat[1]{\catname{#1}}
\newcommand\catnameind[1]{{\pmb #1}}
\newcommand\categoryop[1]{\mbox{\bfseries\itshape #1}$^{\mathrm{op}}$}



%\renewcommand\cat[1]{\catname{#1}}
\newcommand\CC{\catname{C}}

\newcommand\graphcat{\catname{Graph}}
\newcommand\setcat{\catname{Set}}
\newcommand\twocat{\catname{2}}
\newcommand\relcat{\catname{Rel}}
\newcommand\catcat{\catname{Cat}}
\newcommand\natset{\catname{Nat}}
\newcommand\gracat{\catname{Graph}}
\newcommand\rgracat{\catname{rGraph}}
\newcommand\twogracat{\catname{2Graph}}
\newcommand\dbgracat{\catname{dblGraph}}
\newcommand\posetcat{\catname{Poset}}
\newcommand\reprcat{\catname{Repr}}
\newcommand\schemacat{\catname{Schema}}
%\newcommand\catname[1]{\mbox{\boldmath $#1$}}



%=== word shorcuts
% \newcommand\eg{e.g.}
% \newcommand\ie{i.e.}
% \newcommand\etal{\textit{et al}}
%\newcommand\fwk{framework}
%\newcommand\traj{trajector}
%\newcommand\traj{trajector}
%\newcommand\syncon{synchronization}
%\newcommand\Syncon{Synchronization}
\newcommand\symmen{symmetrization}
\newcommand\Symmen{Symmetrization}


\endinput




\setlength{\marginparwidth}{3cm}
%\setlegth{\marginparsep}{1.5mm}
%\setlength{\marginparpush}{5mm}
%

\makeatletter
  \def\fps@figure{tp}
\makeatother

\newcommand{\backgro}[2]{\par\noindent\framebox[\textwidth]{
\begin{minipage}{0.98\textwidth}
\setlength{\parindent}{0.5cm} \noindent \textbf{Background: #1} #2
\end{minipage}}\smallskip}

%%%% macros %%%
%\newtheorem{defin}{Definition}%[section]
%\renewcommand{\thedefin}{\Alph{defin}}





%\newcommand\xxx[4]{{\it #1}\mbox{$_{#3}^{#4}{#2}$}}
%\newcommand{\s}{\star}
%\newcommand\mrk[1]{\mbox{$\langle${\tt #1}$\rangle$}}
%=================================================
% 1  Fonts and letters
%============================================

%=====================================================
% 2  Mathematical shtuchki
%=========================================================


% New Symbols allowed to use in MathMode (!)
%========= General =============
\newcommand\mylist[2]{\mbox%
                          {$#1_1,\ldots,#1_{#2}$}}

\newcommand\iidots[2]{\mbox{
                            $#1=1,\ldots,#2$
                      }}
\newcommand\ijdots[3]{\mbox{
                            $#1=#2,\ldots,#3$
                      }}
\newcommand{\vare}{\varepsilon}
\newcommand\nr{\normalsize\rm}
\newcommand\tril{\triangleleft}
\newcommand\eqdef{\stackrel{\rm def}{=}}
\newcommand\trir{\triangleright}
\newcommand\bc{\bigcirc}







%(4)%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Abbreviations of words from pre_gen
%%%%%%%%%%%%%%%%%%%%%

%\newcommand\ql{query \lan} comment for ISMIS'96
\newcommand\sync{synchronous}
\newcommand\async{asynchronous}
\newcommand\syncn{synchronization}
\newcommand\syncd{synchronized}
\newcommand\Sync{Synchronous}
\newcommand\Async{Asynchronous}
\newcommand\Syncn{Synchronization}
\newcommand\Syncd{Synchronized}

\newcommand\sce{scenario}

\newcommand\eqe{equivalence}
\newcommand\eqt{equivalent}

\newcommand\intn{intuition}
\newcommand\intv{intuitive}
\newcommand\coa{coalgebra}
\newcommand\ispartof{\ittt{isPartOf}}
\newcommand\isPartOf{\ittt{isPartOf}}
\newcommand\IsPartOf{\ittt{isPartOf}}

\newcommand\of{\ittt{(isPart)Of}}
\newcommand\Of{\ittt{Of}}
\newcommand\arrdl{ArrDL}
\newcommand\elmsl{ElmSL}

\newcommand\isa{\ittt{isA}}
\newcommand\IsA{\ittt{isA}}
\newcommand\isA{\ittt{isA}}


\newcommand\subst{\ittt{subst}}


\newcommand\OOAD{OOA\&D}
\newcommand\oid{o-id}

\newcommand\pred{predicate}

\newcommand\interstan{interstate relation}
\newcommand\intrel{interstate relation}
\newcommand\demon{demonstration}
\newcommand\demoe{demonstrate}
\newcommand\asson{association}
\newcommand\config{configuration}
\newcommand\asscon{association configuration}
\newcommand\ass{associative}
\newcommand\assive{associative}
\newcommand\aggrn{aggregation}
\newcommand\attrn{attribution}
\newcommand\abbrn{abbreviation}
\newcommand\gen{generalization}
\newcommand{\iden}{identification}
\newcommand\idey{identity}
\newcommand\qualn{qualification}
\newcommand\reprn{representation}
\newcommand\situn{situation}
\newcommand\speln{specialization}
\newcommand\spen{specialization}
\newcommand\spel{specialization}
\newcommand\spec{specification}
\newcommand\implen{implmentation}
\newcommand\impleg{implmenting}
\newcommand\strul{structural} %\strul

\newcommand\spenisa{\spen\ \isa-arrow}
\newcommand\genisa {\gen\  \isa-arrow}

\newcommand\visun{visualization}


%\newcommand\gen{generalization}
\newcommand\repr{representation}

\newcommand\visn{visualization}


%\newcommand{\oid}{object identity}
\newcommand{\oids}{object identities}



\newcommand\datamod[1]{{\rm #1}}

\newcommand\ERC{\datamod{ERC\mbox{$^+$}}}
\newcommand\ercd{\ERC-diagram}
\newcommand\ER{\datamod{ER}}
\newcommand\EER{\datamod{EER}}
\newcommand\RM{\datamod{RM}}
\newcommand\RMT{\datamod{RM/T}}
\newcommand\RDM{\datamod{RDM}}
\newcommand\VO{\datamod{VO}}
\newcommand\OOO{\datamod{OO}}
\newcommand\SDM{\datamod{SDM}}
\newcommand\FDM{\datamod{FDM}}
\newcommand\IFO{\datamod{IFO}}
\newcommand\Oid{\datamod{Oid}}
\newcommand\RO{\datamod{RO}}
\newcommand\ROP{\datamod{RO\mbox{$^+$}}}
\newcommand\Flogic{\datamod{F-logic}}
\newcommand\SkeDM{\datamod{SkeDM}}
\newcommand\Diagr{\datamod{Diagrams}}

\newcommand\datatrend[1]{{\bf #1}}

\newcommand\eer{\datatrend{eer}}
\newcommand\ooo{\datatrend{oo}}
\newcommand\pl{\datatrend{pl}}
\newcommand\skeske{\datatrend{ske}}

\newcommand\msour{multisource}
\newcommand\sour{source}

\newcommand\abbr{abbreviat}
\newcommand\lega{legacyless}


\newcommand\Ass{Associative}



\newcommand{\ider}{identifier}
\newcommand{\deor}{descriptor}

\newcommand\dombs{domain-based sketch}
\newcommand\ms{multisource}
\newcommand\mt{multitarget}
\newcommand\refin{refinement}
\newcommand\db{database}
\newcommand{\grab}{graph-based }
\newcommand{\spef}{specification}
%\newcommand\spec{specification}
\newcommand{\grabs}{\grab\spef}
\newcommand{\lan}{language}
\newcommand{\sgd}{\spel$\!$/\gen distinction }
\newcommand\qr{query }
\newcommand\qrs{queries}

%%%%% Integration %%%%%%%%%%%%%

\newcommand{\integ}{integration}
\newcommand{\intd}{integrated}
\newcommand{\di}{data integration }
\newcommand{\dbi}{database integration }
\newcommand{\vi}{view integration }
\newcommand{\si}{schema integration}
\newcommand{\sdi}{schema and data integration }
%-------------------------------------
\newcommand{\cmod}{conceptual modeling}
\newcommand{\smod}{semantic modeling}
\newcommand{\dbs}{data base}
\newcommand{\dml}{data model}
%\newcommand{\dm}{data model}%{dm}%{DM} % an abbreviation
\newcommand\const{constraint}
\newcommand{\attr}{attribute}
%=====================================
\newcommand\cdb{component \db}
\newcommand\dincy{data inconsistency}
\newcommand\corr{correspondence}
\newcommand\lang{language}
%------
\newcommand\corinf{correspondence information}
\newcommand\corrinf{correspondence information}

\newcommand\coras{correspondence assertion}
\newcommand\corass{correspondence assertions}
\newcommand\corda{correspondence data}
\newcommand\coreq{\corr\ equation}
\newcommand\coreqs{\corr\ equations}

\newcommand\dacorr{data \corr}
\newcommand\cors{\corr\ \ske}
\newcommand\corss{\corr\ \skes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\relship}{relationship}
%----------------------------------------
\newcommand{\Spc}{Spaccapietra {\em et al} }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\ske{sketch}
\newcommand\skes{sketches}
\newcommand\cske{component sketch}
\newcommand\cskes{component sketches}
\newcommand\eroo{\cite{ER95}}
%%%%%%%%%%%% Romanic abbreviations  %%%%%%%%%%%%
\newcommand\eg{e.g.}
\newcommand\ie{i.e.}
\newcommand\wrt{w.r.t.}
\newcommand\etc{{\em etc}}
\newcommand\etal{{\em et al}}
\newcommand\ala{{\em a la }}
\newcommand\apriori{{\em a priori}}
\newcommand\adhoc{{\em ad hoc}}
\newcommand\dejure{{\em de jure}}
\newcommand\defacto{{\em de facto}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\sign}{signature}
%\newcommand{\constr}{constructivizab}% *le or *ility
%\newcommand{\cat}{category}
%\newcommand{\cats}{categories}
%\newcommand{\ct}{category theory\ } %y or ies
%\newcommand\mor{morphism}
%\newcommand\amor{automorphism}
%\newcommand\alg{algebra}
%%\newcommand\inst{institution}
%=============================

%(5)\newcommand\entails{\Rightarrow}
%\newcommand\implies{\Rightarrow}
%-------------------------------------
%\newcommand\dom[1]{\mathit{Dom}(#1)}
%\newcommand\cod[1]{\mathit{Cod}(#1)}
\newcommand\rg[1]{\mathit{Rg}(#1)}
\newcommand\DOM[1]{\Box #1}
\newcommand\COD[1]{#1 \Box}

\newcommand\tabname[1]{\mbox{$\ittt{Tab}\_#1$}}
%\newcommand\multisource[
\newcommand\mytilde[1]{\widetilde{#1}}
\newcommand\sempr[1]{\mytilde{\semm{#1}}}

\newcommand\mycount[1]{{\bf count}{(#1)}}
\newcommand\gragen[1]{\left[\mathstrut #1 \right]}

\newcommand\respace{\!}%\!\!}
\newcommand\lsemm{\left[ \respace\left[ }
\newcommand\rsemm{\right]\respace\right]}
\newcommand\semm[1]{\enma{$\lsemm\, \mathit{#1} \, \rsemm$}}
\newcommand\semmind[2]{\mbox{$\lsemm\, \mathit{#1} \, \rsemm^{#2}$}}
\newcommand\semmx[2]{\enma{$\lsemm\, \mathit{#2} \, \rsemm^{#1}$}}
\newcommand\semmA[2]{\enma{$\lsemm\, \mathit{#2} \, \rsemm^{A}$}}
\newcommand\semmB[2]{\enma{$\lsemm\, \mathit{#2} \, \rsemm^{B}$}}

\newcommand\semmindex[1]{\lsemm\, \mathit{#1} \, \rsemm}
\newcommand\semmstar[1]{\semm{#1}^{*}}
\newcommand\lbesemm{\left< \respace\left<}
\newcommand\rbesemm{\right> \respace\right>}
\newcommand\besemm[1]{\mbox{$\lbesemm\, \mathit{#1} \, \rbesemm$}}



%(6)%\newcommand\informalPar[1]{\nicex{{#1}$}}
%\newcommand\infParind[1]{\cal #1}
%Contents:
%--- semiotics
%--- Skesig
%--- Varset
%--- Behset



%%==== Semiotics =====
%
%%\newcommand\formalPar[1]{\mbox{$\mathrm{#1}$}}
%\newcommand\frmParind[1]{\mathrm{#1}}
%
%\newcommand\informalParBold[1]{\mbox{${\cal #1}$}}
%\newcommand\formalPar[1]{\mbox{$\mathrm #1$}}
%
%\newcommand\object[2]{\mbox{${\mathsf{#1}}_{#2}$}}
%%\newcommand\object[2]{\mbox{$#1_{#2}$}}
%\newcommand\universe[1]{\mbox{$\mathbf{#1}$}}
%%\newcommand\objectind[1]{\mathsf{#1}}
%\newcommand\objectind[1]{\mathsf{#1}}
%\newcommand\universeind[1]{\mathbf{#1}}
%
%\newcommand\proc[1]{\mbox{\sffamily\bfseries #1}}
%\newcommand\procind[2]{\mbox{${\mathrm{#1}}_{\mathrm #2}$}}
%\newcommand\linf{\informalParBold{L}}
%\newcommand\minf{\mbox{$\informalPar{M}(\diag{})$}}
%\newcommand\mdinf{\mbox{$\informalPar{M}(\diag{})$}} % the same as above
%\newcommand\mdfrm{\mbox{$\formalPar{M}(\diag{})$}} % the same as above
%\newcommand\uinf{\informalPar{U}}
%
%\newcommand\meaninf{\informalPar{M}}
%\newcommand\meanfrm[1]{\mbox{$\formalPar{M}_{#1}$}}
%\newcommand\diag[1]{\object{D}{#1}} %\mbox{$D$}}
%\newcommand\diagob[1]{\object{D}{#1}} %\mbox{$D$}}
%\newcommand\diags{\mbox{$\mathit{Diags}$}}
%\newcommand\graph{\mbox{$\mathit{Graph}$}}
%\newcommand\skeob[1]{\object{S}{#1}}
%\newcommand\modelob[1]{\object{M}{#1}}
%\newcommand\sigob[1]{\object{\mbox{$\Sigma$}}{#1}}
%\newcommand\skediag{\skeob{}[\diag{}]}
%\newcommand\meaninfdiag{\meaninf[\diag{}]}
%\newcommand\meanfrmdiag{\meanfrm[\diag{}]}
%% synonyms
%\newcommand\meanifdiag{\meaninf[\diag{}]}
%\newcommand\meanfdiag{\meanfrm[\diag{}]}

%=======================
%==== Skesig
%\newcommand\so[1]{source(#1)}
%\newcommand\ta[1]{target(#1)}
\newcommand\U{{\cal U}}
\newcommand\M{{\cal M}}
\newcommand\Set{{\mathbf Set}}
\newcommand\Varset{{\mathbf Varset}}
\newcommand\univ{\mbox{$\mathbf U$}}
\newcommand\univind{{\mathbf U}}
\newcommand\skesig{\mbox{$\Sigma$}}

%%%% macro\Skesig.tex %%%%  June 29

\newcommand\mrkid{\mrk{ID}}
\newcommand\imID{\mbox{ID?}} %$^*$}}
\newcommand\mrkidd{\imID} % marker of IDDeficient
\newcommand\prodid{\mbox{$\times$-\ider}}
\newcommand\plusid{\mbox{$+$-\ider}}
\newcommand\prodkey{\mbox{$\times$-key}}
\newcommand\pluskey{\mbox{$+$-key}}

\newcommand\ID{\mrk{ID}}
\newcommand\IDplus{\mrk{ID$^+$}}
\newcommand\IDprod{\mrk{ID$^\times$}}

\newcommand\andiden{\emph{and}-\iden}
\newcommand\oriden{\emph{or}-\iden}


\newcommand\ssta{\mbox{${\mathsf S}_{\mathrm sta}$}}
\newcommand\sdyn{\mbox{${\mathsf S}_{\mathrm dyn}$}}

%\newcommand\mrk[1]{\mbox{[${\tt #1}$]}}
%\newcommand\mrk[1]{\mbox{[${\mathbf{#1}}$]}}
%\newcommand\mrkop[1]{\mbox{$\langle{\tt #1}\rangle$}}
\newcommand\mrkop[1]{\mbox{$\langle{\mathbf{#1}}\rangle$}}
\newcommand\mrkopr[1]{\mbox{$\mathbf{[{#1}\rangle}$}}
\newcommand\mrkopl[1]{\mbox{$\mathbf{\langle{#1}]}$}}
\newcommand\mrksemiop[1]{\mbox{$\langle{\tt #1}]$}}
\newcommand\mrkNode[1]{\mbox{${\tt #1}$}}
\newcommand\mrkn[1]{\mrkNode{#1}}
\newcommand\mrktt[1]{{\tt #1}}
\newcommand\mrkopright[1]{\mbox{$[${\tt #1}$\rangle$}}
\newcommand\mrkopleft[1]{\mbox{$\langle${\tt #1}$]$}}
%%%%%%%%%%%%%  Begin Key commands %%%%%%%%%%%%%%%%%%%%%%%

\newcommand\PredicateSignature{\Pi}
\newcommand\OperationSignature{\Sigma}
\newcommand\predFromOperSig{\Sigma_{pr}}
\newcommand\BaseSignature{\bf B}
\newcommand\DomainBase{\bf B}

\newcommand\ConstraintLanguage{CL}
\newcommand\dolan%DomainLanguage{\Delta}
{\mbox{$\Delta $}}

\newcommand\dolanm{\Delta}

\newcommand\adtm{ADT}
\newcommand\adt{{\sl \adtm}}
\newcommand\dolanadt{\dolan_{\adtm}}
\newcommand\sigadt{{\it Sig}_{\adtm}}
\newcommand\semmadt{\semm{}_{\adtm}}

\newcommand\dbauxm{DBD}
\newcommand\dbaux{{\sl \dbauxm}}
\newcommand\dolandbaux{\dolan_{\dbauxm}}
\newcommand\sigdbaux{{\it Sig}_{\dbauxm}}
\newcommand\semmdbaux{\semm{}_{\dbauxm}}

\newcommand\ba{D}
\newcommand\domba{\mbox{$\Domain(\ba)$}}
\newcommand\bam{\BasicDomainMarkerSymbol}          %  B  for using in math mode
%\newcommand\V{\mbox{$\TheValueUniverse_{\dolanm}$}}%

\newcommand\Pred{{\it Pred}}
\newcommand\Oper{{\it Op}}
\newcommand\Base{{\it Base}}
\newcommand\Dom{{\it Dom}}
\newcommand\Domain{{\it Dom}}
\newcommand\pool{V}

\newcommand\ArityMap{{\it Shp}}
\newcommand\ArityGraph{D}
\newcommand\AritySketch{{\cal D}}
\newcommand\ArityInclusion{\mbox{\Large $\iota$}}

\newcommand\rms{\rm\scriptsize}   % for writing, eg, \D^{\rms in}

\newcommand\PredicateMarkerSymbol{P}
\newcommand\OperationMarkerSymbol{F}
\newcommand\BasicDomainMarkerSymbol{B}

\newcommand\PredicateDiagramSet[1]{\PredicateMarkerSymbol^{#1}}%P^#1}
\newcommand\OperationDiagramSet[1]{\OperationMarkerSymbol^{#1}}%F^#1}
\newcommand\BasicDomainDiagramSet[1]{\BasicDomainMarkerSymbol^{#1}}%B^#1}

\newcommand\AGraph{G}
\newcommand\g{\mbox{$\AGraph$}}
\newcommand\gm{\AGraph}

\newcommand\ASketchSymbol{S}
\newcommand\ASketch{\mathsf \ASketchSymbol}
\newcommand\s{\mbox{$\ASketch$}}
\newcommand\sind{\ASketch}
\newcommand\sm{\ASketch}
\newcommand\sprim{\mbox{$\ASketch'$}}
\newcommand\sbipr{\mbox{$\ASketch''$}}


\newcommand\TheUniverseSymbol{U}
\newcommand\TheUniverseSketch{\cal \TheUniverseSymbol}
\newcommand\TheObjectUniverse{Obj }%{\cal O}
\newcommand\TheTimeUniverse{\cal T}%{T}
\newcommand\TheHistoryUniverse{\cal \TheTimeUniverse^*}%}
\newcommand\TheValueUniverse{Val}%{\cal V}

\newcommand\ASketchAlgebra{\cal A}
\newcommand\ABaseSubSketch{\cal B}    % base subsketch of

\newcommand\APermutation{\pi}

%===================================================

\newcommand\Mod[1]{\mbox{{\bf Mod}$(#1)$}}
\newcommand\Ext[1]{\mbox{{\bf Ext}$(#1)$}}
\newcommand\Inst[1]{\mbox{{\bf Inst}$(#1)$}}

%%%%%%%%%%%%%   End Key commands %%%%%%%%%%%%%%%%%


%%%%%%%%%%%%    Useful Abbreviations %%%%%%%%%%%%

%%% Sketchi


\newcommand\sdom{\mbox{$\s_{\DomainBase}$}}
\newcommand\sdomm{\s_{\DomainBase}}

\newcommand\newb{\mbox{$\DomainBase$}}
\newcommand\bm{\DomainBase}

\newcommand{\bs}{\mbox{$\ABaseSubSketch$}}
\newcommand\bsm{\ABaseSubSketch}

\newcommand\skespe{{\bf \ASketchSymbol}}

\newcommand\gras{{\it Gra}\skeob}
\newcommand\doms{{\it Dom}\skeob}
\newcommand\clas{{\it Cla}\skeob}
\newcommand\rels{{\it Rel}(\skeob)}

\newcommand\R{\nicex{ R$}}
\newcommand\OO{\mbox{$\TheObjectUniverse$}}
%\newcommand\T{\mbox{$\TheTimeUniverse$}}
%\newcommand\Hist{\mbox{$\TheHistoryUniverse}}
%\newcommand\V{\mbox{$\TheValueUniverse_{\bm}$}}%

\renewcommand\u{\mbox{$\TheUniverseSketch$}}
\newcommand\um{\TheUniverseSketch}
\newcommand\upred{\mbox{$\TheUniverseSketch_{\predsigm}$}}
\newcommand\uoper{\mbox{$\TheUniverseSketch_{\opersigm}$}}

\newcommand\predsig{\mbox{$\PredicateSignature$}}
\newcommand\predsigm{\PredicateSignature}
\newcommand\opersig{\mbox{$\OperationSignature$}}
\newcommand\opersigm{\OperationSignature}
\newcommand\predopsig{\mbox{$\predFromOperSig$}}
%\newcommand\pros{\predopsig}
\newcommand\prosm{\predFromOperSig}
\newcommand\basesig{\mbox{\BaseSignature}}
\newcommand\basesigm{{\BaseSignature}}
\newcommand\clan{\mbox{$\ConstraintLanguage$}}
\newcommand\clanm{\ConstraintLanguage}
\newcommand\colan{\mbox{\ConstraintLanguage}}
\newcommand\clanform{\mbox{$\ConstraintLanguage=(\Pred,\arimap,\semm{})$}}
\newcommand\colanm{\ConstraintLanguage}
%\newcommand\dolan{\mbox{\DomainLanguage}}
%\newcommand\dolanm{\DomainLanguage}

\newcommand\pis{$\PredicateSignature $-sketch}
\newcommand\sis{$\OperationSignature $-sketch}
\newcommand\siprs{$\predFromOperSig$-sketch}
\newcommand\sia{$\OperationSignature $-algebra}
\newcommand\clans{$\Constraint Language$-sketch}

\newcommand\arimap{\ArityMap}
\newcommand\arimapin{\mbox{\ArityMap$^{\rms in}$}}

\newcommand\os{\mbox{$\overline{\s}$}}
%\newcommand\go{\mbox{$G_{({\cal O})}$}}

\newcommand\pip{\mbox{$\APermutation^{+}$}}
\newcommand\depipComp{\mbox{$\delta \comp\APermutation^{+}$}}
\newcommand\depip{\mbox{$\APermutation^{+}\delta $}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%                                  %%%%%%%%%%%%%%%%%
%%%%%%%%%%            A R I T I E S         %%%%%%%%%%%%%%%%%%
%%%%%%%%%%                                  %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\pr{\mbox{$\PredicateMarkerSymbol$}}  % $P$ for using in text mode
\newcommand\op{\mbox{$\OperationMarkerSymbol$}}  % $F$ for using in text mode
%\newcommand\ba{\mbox{$\BasicDomainMarkerSymbol$}}  % $P$ for using in text mode


\newcommand\myprm{\PredicateMarkerSymbol}        %  P  for using in math mode
\newcommand\opm{\OperationMarkerSymbol}          %  F  for using in math mode
%\newcommand\bam{\BasicDomainMarkerSymbol}       %  B  for using in math mode

%%%%   functions to put the arg
%%%%   as subindex near \pr,\op and \ba

\newcommand\prix[1]{\myprm_{#1}}
\newcommand\opix[1]{\opm_{#1}}
\newcommand\baix[1]{\bam_{#1}}

%%%----  end functions

\newcommand\pri{$\myprm_{i}$}    %  \pr_i for using in text mode
\newcommand\opi{$\opm_{j}$}      %  \op_j for using in text mode
\newcommand\bai{$\bam_{l}$}      %  \ba_l for using in text mode

\newcommand\prim{\myprm_{i}}     %  \pr_i for using in math mode
\newcommand\opim{\opm_{j}}       %  \op_j for using in math mode
\newcommand\baim{\bam_{l}}       %  \ba_l for using in text mode
%======================================
%  eto makrosy funcciy
\renewcommand\Pr[1]{\PredicateDiagramSet{#1}}  % P^#1
\newcommand\Op[1]{\OperationDiagramSet{#1}}    % F^#1
\newcommand\Ba[1]{\BasicDomainDiagramSet{#1}}  % B^#1
%  a eto ih znacheniya
\newcommand\PrS{\Pr{\s}}      % P^\s
\newcommand\OpS{\Op{\s}}      % F^\s
\newcommand\BaS{\Ba{\s}}      % B^\s
%\newcommand\domba{$\Domain(\ba)$}

\newcommand\PrU{\Pr{\u}}      % P^\u
\newcommand\OpU{\Op{\u}}      % F^\u
\newcommand\BaU{\Ba{\u}}      % B^\u

%------------------------------------------------
% eto makrosy funkciy s 2 argumwntami
\newcommand\Prix[2]{\Pr{#1}_{#2}}              % a set P^#1_#2
\newcommand\Opix[2]{\Op{#1}_{#2}}              % a set F^#1_#2
\newcommand\Baix[2]{\Ba{#1}_{#2}}              % a set B^#1_#2
% a eto b nih podstavleny indexy i ostalsya 1 argument
\newcommand\Pri[1]{$\Prix{#1}{i}$}             % a set og diag, P^#1_i
\newcommand\Opi[1]{$\Opix{#1}{j}$}             % a set of diag, F^#1_j
\newcommand\Bai[1]{$\Baix{#1}{l}$}             % a set of diag, B^#1_l
% a eto znacheniya
\newcommand\PriS{\Pri{\s}}      % Pi^\s
\newcommand\OpiS{\Opi{\s}}      % Fj^\s
\newcommand\BaiS{\Bai{\s}}      % Bl^\s

\newcommand\PriU{\Pri{\u}}      % Pi^\u
\newcommand\OpiU{\Opi{\u}}      % Fj^\u
\newcommand\BaiU{\Bai{\u}}      % Bl^\u

%  a eto dlya mat mode
\newcommand\Prim[1]{\Prix{#1}{i}}     %  a set of diagr,  P^#1_i for using in math mode
\newcommand\Opim[1]{\Opix{#1}{j}}     %  a set of diagr,  F^#1_j for using in math mode
\newcommand\Baim[1]{\Baix{#1}{l}}     %  a set of diagr,  B^#1_#2 for using in math mode
%====================================================

%\newcommand\pool{V}
\newcommand\vx[1]{\mbox                                  % D_arg
                      {$\pool_{#1}$}}
\newcommand\vinx[1]{\mbox                                % D^in_arg
                      {$\pool^{\mbox\rms in}_{#1}$}}
\newcommand\voutx[1]{\mbox                               % D^out_arg
                      {$\pool^{\mbox\rms out}_{#1}$}}
%============================================================

%\newcommand\ArityGraph{D}
%\newcommand\AritySketch{\D}                             % \D - nice D
\newcommand\sprx[1]{\mbox                                %  D_arg
                      {$\ArityGraph_{#1}$}}
\newcommand\sopx[1]{\mbox                                % \D_arg
                      {$\AritySketch_{#1}$}}
\newcommand\sinx[1]{\mbox                                % \D^in_arg
                      {$\AritySketch^{\rms in}_{#1}$}}
\newcommand\soutx[1]{\mbox                               % \D^out_arg
                      {$\AritySketch^{\rms out}_{#1}$}}

%-----   marker-subindex version
\newcommand\spr{\sprx{\myprm}}         %  D_{prop marker}
\newcommand\sop{\sopx{\opm}}         % \D_{oper marker}
\newcommand\sinop{\sinx{\opm}}       % \D^in_{oper mark}
%-----   i-subindex version
\newcommand\spri{\sprx{i}}          %  D_{i}
\newcommand\sopi{\sopx{j}}          % \D_{j}
\newcommand\sinopi{\sinx{j}}        % \D^in_{j}



\newcommand\opshaxy[2]{\inclar{#1_{#2}}  % arg1_arg2: D^in_arg2 -->D_arg2
                            {\sinx{#2}}
                              {\sopx{#2}}
                       }
%\newcommand\ArityInclusion{i}
\newcommand\opsha{\opshaxy{\ArityInclusion}{\opm}}   %i_f: D^in_f   --> D_f
\newcommand\opshai{\opshaxy{\ArityInclusion}{\opim}} %i_f: D^in_f_j --> D_f_j

%----------------------------------------

%\newcommand\ArityMap{{\it Shp}}
\newcommand\arix[1]{\mbox
                        {$\ArityMap({#1})$}}         % Shp(arg)
\newcommand\ariinx[1]{\mbox
                        {$\ArityInclusion_{#1}$}}    % \iota_{arg}

\newcommand\aripr{\arix{\myprm}}                  % Shp(p)
\newcommand\ariop{\arix{\opm}}                  % Shp(f)
\newcommand\arinc{\ariinx{\opm}}                % \iota_f

\newcommand\aripri{\arix{\prim}}                % Shp(p_i)
\newcommand\ariopi{\arix{\opim}}                % Shp(f_j)
\newcommand\arinci{\ariinx{\opim}}              % \iota_j

%-----------------------------------------
\newcommand\sepr{\semm{\pr}}
\newcommand\seop{\semm{\op}}
\newcommand\sepri{\semm{\pri}}
\newcommand\seopi{\semm{\op}}


\newcommand\opv{\mbox{\Oper$^+$}}

%\endinput

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%              %%%%%%%%%%%%%%%
%%%%%%%%%%%  Old Macros %%%%%%%%%%%%%%%%
%%%%%%%%%%              %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\newcommand\sig{\mbox{$\PredicateSignature$}}
%\newcommand\gra{{\bf G}}
%\newcommand\sigo{\mbox{$\Sigma_1$}}
%\newcommand\grao{\mbox{${\bf G}_1$}}
%% OOPS! \newcommand\inst{\mbox{$\lar{\vare }{S}{W}$}}
%%\newcommand\sch{\Category{Schema} }
%
%
%\newcommand\instVareps{\mbox{$\lar{\vare }{S}{W}$}}
%\newcommand\inste{\mbox{$\lar{e}{S}{W}$}}
%\newcommand\emor[1]{\lar{e}{#1}{\u}}
%\newcommand\sv{\mbox{$S_V$}}
%\newcommand\sr{\mbox{$S_R$}}
%\newcommand\vmor{\lar{v}{\sv}{\ovrs{}}}
%\newcommand\rmor{\lar{r}{S}{\ovrs{R}}}
%\newcommand\vpair{\mbox{$V=(\sv,v)$}}
%\newcommand\rpair{\mbox{$R=(\sr,r)$}}
%===
%==== Varset
%% macros for writing formulas with varsets and varfunctions

%%%%%%%%%    ..\dke96\macro\varset.tex    %%%%%%%
%\renewcommand\c{\mbox{$\AClass$}}                    %   C
%\newcommand\cm{\AClass}                              %   C
%\newcommand\ce{\mbox{$\semm{\AClass}$}}              % ||C||

%\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}   % ||C||^#1

%\newcommand\cindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
% apply:
%\newcommand\cet{\ceind{\ltt}}                         % ||C||^t
%\newcommand\ceu{\ceind{\ltu}}                         % ||C||^u
\newcommand\ObjStt{\ittt{ObjStt}}
\newcommand\C{\textit{C}}
\newcommand\D{\textit{D}}

\newcommand\ot[1]{\mbox{$o^{\ltt_{#1}}$}}
\newcommand\otm{o^\ltt}
\newcommand\ou[1]{\mbox{$o^{\ltu_{#1}}$}}
\newcommand\otu{o^\ltu}

\newcommand\cet{\mbox{$\semm{C}^{\ltt}$}}                         % ||C||^t
\newcommand\ceti{\mbox{$\semm{C}^{\ltt_i}$}}                         % ||C||^t
\newcommand\ceu{\mbox{$\semm{C}^{\ltu}$}}                         % ||C||^t
\newcommand\ceprt{\mbox{$\sempr{C}^{\ltt}$}}                         % ||C||^t
\newcommand\cepru{\mbox{$\sempr{C}^{\ltu}$}}                         % ||C||^t


\newcommand\cetu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\AClass}^{\ltu}$}}
\newcommand\ceut{\mbox{$\vphantom{\semm{AClass}}^{\ltu}\!\semm{\AClass}^{\ltt}$}}
\newcommand\detu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass}^{\ltu}$}}
\newcommand\fetu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass_f}^{\ltu}$}}
\newcommand\djetu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass_j}^{\ltu}$}}
\newcommand\dietu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass_i}^{\ltu}$}}
\newcommand\deut{\mbox{$\vphantom{\semm{AClass}}^{\ltu}\!\semm{\TargetClass}^{\ltt}$}}
\newcommand\ceprtu{\mbox{$\vphantom{\sempr{AClass}}^{\ltt}\sempr{\AClass}^{\ltu}$}}
\newcommand\deprtu{\mbox{$\vphantom{\sempr{AClass}}^{\ltt}\sempr{\TargetClass}^{\ltu}$}}



\newcommand\cesu{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\AClass}^{\ltu}$}}
\newcommand\cest{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\AClass}^{\ltt}$}}
\newcommand\cett{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\AClass}^{\ltt}$}}

\newcommand\dest{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\TargetClass}^{\ltt}$}}
\newcommand\desu{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\TargetClass}^{\ltu}$}}

\newcommand\cestart{\mbox{${\semmstar{C}}^{\ltt}$}}                         % ||C||^t
\newcommand\cestaru{\mbox{${\semmstar{C}}^{\ltu}$}}                         % ||C||^t
\newcommand\cestartu{\mbox{${}^{\ltt}{\semmstar{C}}^{\ltu}$}}

\newcommand\ceto{\mbox{$\semm{\AClass}^{\ltt}_{o}$}}
\newcommand\ceuo{\mbox{$\semm{\AClass}^{ \ltu}_{o}$}}

\newcommand\cestarto{\mbox{${\semmstar{\AClass}}^{\ltt}_{o}$}}
\newcommand\cestaruo{\mbox{${\semmstar{\AClass}}^{ \ltu}_{o}$}}

%======================================================================

%  ----  Basic Command -----------

\newcommand\LogicalTime{\cal T}
\newcommand\SetOfHistories{\LogicalTime^*}
\newcommand\AHistory{H}%J}

%\newcommand\IndexingXupYdownZ[3]{\mbox{$#1^{#2}_{#3}$}}
%\newcommand\IntRelSymb{\varepsilon}%rho}
%\newcommand\IntRelSymb{\mbox{\Large$\iota$}}%rho}
%\newcommand\IntersttMap{\mbox{\ittt same}}%rho}

\newcommand\AClass{C}
\newcommand\SourceClass{C}
\newcommand\TargetClass{D}
\newcommand\e{E}
\newcommand\AReference{f}
\newcommand\AnotherReference{g}
%\newcommand\Identifier{\mbox{\Large$\iota$}}
\renewcommand\g{g}
%\newcommand\h{h}
%\newcommand\hind{h}


\newcommand\farr{\lar{\AReference}{\SourceClass}{\TargetClass}}
\newcommand\farris{\lar{\AReference_i}{\SourceClass}{\TargetClass_i}}
\newcommand\farrit{\lar{\AReference_i}{\SourceClass_i}{\TargetClass}}
\newcommand\ffams{\mbox{$\f=\famm{\farris}{i\in I}$}}
\newcommand\ffamt{\mbox{$\f=\famm{\farrit}{i\in I}$}}

\newcommand\garr{\lar{\AnotherReference}{\SourceClass}{\TargetClass}}
\newcommand\garrit{\lar{\AnotherReference_i}{\SourceClass}{\TargetClass_i}}
\newcommand\garris{\lar{\AnotherReference_i}{\SourceClass_i}{\TargetClass} }
\newcommand\gfams{\mbox{$\g=\famm{\garris}{i\in I}$}}
\newcommand\gfamt{\mbox{$\g=\famm{\garrit}{i\in I}$}}


\newcommand\iarr{\lar{\AReference}{\SourceClass}{\TargetClass}}
\newcommand\iarris{\lar{\Identifier_j}{\SourceClass}{\TargetClass_j}}
\newcommand\iarrit{\lar{\Identifier_j}{\SourceClass_j}{\TargetClass} }
\newcommand\ifams{\mbox{$\Identifier=\famm{\iarris}{j\in J}$}}
\newcommand\ifamt{\mbox{$\Identifier=\famm{\iarrit}{j\in J}$}}


\newcommand\AMoment{t}%j}
\newcommand\EarlierMoment{t}%j}
\newcommand\LaterMoment{u}%k}
\newcommand\EarlierEarlierMoment{s}%i}
\newcommand\LaterLaterMoment{v}%l}

\newcommand\ttt{t1,t2}

\newcommand\IndexingXupYdownZ[3]{\mbox{$#1^{#2}_{#3}$}}

%%%%%%%%%%%%%%%%%%%%%%
% -- Abbreviations ----
%%%%%%%%%%%%%%%%%%%%%%%%%%                    sket}}


\newcommand\T{\mbox{$\LogicalTime$}}
\newcommand\Tm{\LogicalTime}
\newcommand\Hist{\mbox{$\SetOfHistories$}}
\newcommand\Histm{\SetOfHistories}
\newcommand\IntersttMap{\mbox{\ittt{same}}}%rho}
\newcommand\same[2]{\mbox{$\IntersttMap^{#1}_{#2}$}}
\newcommand\inter[2]{\same{#1}{#2}}
\newcommand\interpr[2]{\mbox{$\mytilde\IntersttMap^#1_#2$}}
% \IndexingXupYdownZ{\IntRelSymb}{#1}{#2}}  %\vare^#1_#2
%\newcommand\interpr[2]%
%      {\IndexingXupYdownZ{\mytilde{\IntRelSymb}}{#1}{#2}}  %\vare^#1_#2

%%% The new version t is denoted by \ltt, u is denoted by  \ltu etc

\newcommand\ttu{\EarlierMoment\LaterMoment}   %tu
\newcommand\logtimet{\EarlierMoment}               %t
\newcommand\ltt{\EarlierMoment}               %t
%\newcommand\tu{\LaterMoment}                  %u
\newcommand\ltu{\LaterMoment}                  %u
\newcommand\ttlu{\mbox{$\ltt\le\ltu$}}         % t =< u
\newcommand\tleu{\mbox{$\ltt\le\ltu$}}         % t =< u
\newcommand\tlu{\mbox{$\ltt<\ltu$}}            % t < u
\newcommand\logtimes{\EarlierEarlierMoment}        %s
\newcommand\lts{\EarlierEarlierMoment}               %t
\newcommand\ltv{\LaterLaterMoment}             %l
\newcommand\tv{\LaterLaterMoment}             %l

\newcommand\J{\AHistory}                      %J

\newcommand\intertu[1]{\inter{\ltt\to\ltu}{#1}}       % \eps^tu_#1
\newcommand\interut[1]{\inter{\ltt\gets\ltu}{#1}}       % \eps^tu_#1
\newcommand\intertuut[1]{\inter{\ltt\leftrightarrow\ltu}{#1}}       % \eps^tu_#1

\newcommand\intertt[1]{\inter{\ltt\to\ltt}{#1}}                 % \eps^tu_#1

\newcommand\interst[1]{\inter{\lts\to\ltt}{#1}}       % \eps^tu_#1
\newcommand\interts[1]{\inter{\lts\gets\ltt}{#1}}       % \eps^tu_#1

\newcommand\intersu[1]{\inter{\lts\to\ltu}{#1}}       % \eps^tu_#1
\newcommand\interus[1]{\inter{\ltu\gets\lts}{#1}}       % \eps^tu_#1

%\newcommand\interst[1]{\inter{\lts\to\ltt}{#1}}                 % \eps^tu_#1
%\newcommand\intersu[1]{\inter{\lts\to\ltu}{#1}}                 % \eps^tu_#1

\newcommand\domintertu[1]{\ldom{\intertu{#1}}}  %\Box\eps^tu_#1
\newcommand\codintertu[1]{\rdom{\intertu{#1}}}  %\eps^tu_#1\Box

\newcommand\sametuut[1]{\mbox{$\same{\ltt\leftrightarrow\ltu}{#1}$}}       % \eps^tu_#1
\newcommand\sametu[1]{\mbox{$\same{\ltt\to\ltu}{#1}$}}       % \eps^tu_#1
\newcommand\sameut[1]{\mbox{$\same{\ltt\gets\ltu}{#1}$}}       % \eps^tu_#1
\newcommand\samectu{\mbox{$\same{\ltt\to\ltu}{\cm}$}}       % \eps^tu_#1
\newcommand\samecut{\mbox{$\same{\ltt\gets\ltu}{\cm}$}}       % \eps^tu_#1
\newcommand\samedtu{\mbox{$\same{\ltt\to\ltu}{\dm}$}}       % \eps^tu_#1
\newcommand\samedut{\mbox{$\same{\ltt\gets\ltu}{\dm}$}}       % \eps^tu_#1

\newcommand\samett[1]{\same{\ltt\to\ltt}{#1}}                 % \eps^tu_#1

\newcommand\samest[1]{\same{\lts\to\ltt}{#1}}       % \eps^tu_#1
\newcommand\samets[1]{\same{\lts\gets\ltt}{#1}}       % \eps^tu_#1
\newcommand\samecst{\same{\lts\to\ltt}{\cm}}       % \eps^tu_#1
\newcommand\samects{\same{\lts\gets\ltt}{\cm}}       % \eps^tu_#1
\newcommand\samedst{\same{\lts\to\ltt}{\dm}}       % \eps^tu_#1
\newcommand\samedts{\same{\lts\gets\ltt}{\dm}}       % \eps^tu_#1



\newcommand\samesu[1]{\same{\lts\to\ltu}{#1}}       % \eps^tu_#1
\newcommand\sameus[1]{\same{\ltu\gets\lts}{#1}}       % \eps^tu_#1

%\newcommand\samest[1]{\same{\lts\to\ltt}{#1}}                 % \eps^tu_#1
%\newcommand\samesu[1]{\same{\lts\to\ltu}{#1}}                 % \eps^tu_#1

\newcommand\domsametu[1]{\ldom{\sametu{#1}}}  %\Box\eps^tu_#1
\newcommand\codsametu[1]{\rdom{\sametu{#1}}}  %\eps^tu_#1\Box


%  Apply:
\newcommand\interctt{\inter{\ltt\to\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\intercst{\inter{\lts\to\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\interctu{\inter{\ltt\to\ltu}{\cm}}                 % \eps^tu_#1
\newcommand\intercsu{\inter{\lts\to\ltu}{\cm}}                 % \eps^tu_#1

\newcommand\intercut{\inter{\ltt\leftarrow\ltu}{\cm}}                 % \eps^tu_#1

\newcommand\interprctt{\interpr{\ltt\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\interprcst{\interpr{\lts\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\interprctu{\interpr{\ltt\ltu}{\cm}}                 % \eps^tu_#1
\newcommand\interprcsu{\interpr{\lts\ltu}{\cm}}                 % \eps^tu_#1

\newcommand\dominterctu{\domintertu{\cm}}  %\Box\eps^tu_#1
\newcommand\codinterctu{\codintertu{\cm}}  %\eps^tu_#1\Box

%----------------------------------------------
%% Classes and arrows
%-------------------------------------------------

%\renewcommand\c{\mbox{$\AClass$}}                    %   C
\newcommand\cm{\AClass}                              %   C
\newcommand\ce{\mbox{$\semm{\AClass}$}}              % ||C||

%--- function:
\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}   % ||C||^#1

\newcommand\cindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
% apply:
%\newcommand\cet{\mbox{$\semm{C}^{\ltt}$}}                         % ||C||^t
%\newcommand\ceu{\mbox{$\semm{C}^{\ltu}$}}                         % ||C||^t
%\newcommand\cetu{\mbox{${}^{\ltt}\semm{\AClass}^{\ltu}$}}
\newcommand\ces{\ceind{\lts}}                         % ||C||^u
\newcommand\cev{\ceind{\tv}}                         % ||C||^u


\newcommand\ceJ{\ceind{\J}}

\newcommand\objeq[2]{\simeq^{#1}_{#2}}
\newcommand\eqJ[1]{\objeq{\J}{#1}}

\newcommand\ciet{\cindeind{i}{\ltt}}                         % ||C_i||^t
\newcommand\ctet{\cindeind{t}{\ltt}}                         % ||C_t||^t
\newcommand\cjet{\cindeind{j}{\ltt}}                         % ||C_i||^t
\newcommand\cket{\cindeind{k}{\ltt}}                         % ||C_t||^t
\newcommand\clet{\cindeind{l}{\ltt}}                         % ||C_i||^t


\newcommand\cieJ{\ceind{\J}}
%\newcommand\cjeJ{\ceind{\J}}

% function:
\newcommand\cind[1]{\mbox{$\AClass^{#1}$}}           %      C^#1
\newcommand\cindl[2]{\mbox{$_{#1}\AClass^{#2}$}}     % _{#1}C^{#2}
\newcommand\cindr[2]{\mbox{$\AClass_{#1}^{#2}$}}     %      C_{#1}^{#2}

%\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}           %      C^#1
\newcommand\ceindl[2]{\mbox{$_{#1}\semm{\AClass}^{#2}$}}     % _{#1}C^{#2}
\newcommand\ceindr[2]{\mbox{$\semm{\AClass}_{#1}^{#2}$}}     %      C_{#1}^{#2}

%  apply:
\newcommand\ctu{\mbox{$^{\ltt}\!\AClass^{\ltu}$}}
\newcommand\ctplusu{\cindr{+\ltu}{\ltt}}
\newcommand\ctnullu{\cindr{0\ltu}{\ltt}}
\newcommand\cuminust{\cindl{-\ltt}{\ltu}}
\newcommand\cunullt{\cindl{0\ltt}{\ltu}}

%\newcommand\cetu{\cind{\ltt\ltu}}
\newcommand\cetplusu{\ceindr{+\ltu}{\ltt}}
\newcommand\cetnullu{\ceindr{0\ltu}{\ltt}}
\newcommand\ceuminust{\ceindl{-\ltt}{\ltu}}
\newcommand\ceunullt{\ceindl{0\ltt}{\ltu}}

% the same for D

%\renewcommand\d{\mbox{$\TargetClass$}}                    %   D
\newcommand\dm{\TargetClass}                              %   D

\newcommand\de{\mbox{$\semm{\TargetClass}$}}              % ||D||
\newcommand\deind[1]{\mbox{$\semm{\TargetClass}^{#1}$}}   % ||D||^#1
\renewcommand\det{\deind{\ltt}}                         % ||C||^t
\newcommand\deu{\deind{\ltu}}                         % ||C||^u
\newcommand\des{\deind{\lts}}                         % ||C||^u
\newcommand\dev{\deind{\tv}}                         % ||C||^u

\newcommand\deJ{\deind{\J}}

\newcommand\dindeind[2]{\mbox{$\semm{\TargetClass_{#1}}^{#2}$}}
%  apply
\newcommand\dies{\dindeind{i}{\lts}}                         % ||C||^t
\newcommand\djet{\dindeind{j}{\ltt}}                         % ||C||^t
\newcommand\djeu{\dindeind{j}{\ltu}}                         % ||C||^t
%\newcommand\djetu{\dindeind{j}{\ltt}}                         % ||C||^t
\newcommand\dieJ{\deind{\J}}
\newcommand\djeJ{\deind{\J}}
\newcommand\diet{\dindeind{i}{\ltt}}                         % ||C||^t
\newcommand\dieu{\dindeind{i}{\ltu}}                         % ||C||^t
%\newcommand\djetu{\dindeind{j}{\ltt}}                         % ||C||^t


\newcommand\dind[1]{\mbox{$\TargetClass^{#1}$}}           %      C^#1
\newcommand\dindl[2]{\mbox{$_{#1}\TargetClass^{#2}$}}     % _{#1}D^{#2}
\newcommand\dindr[2]{\mbox{$\TargetClass_{#1}^{#2}$}}     %      D_{#1}^{#2}

%\newcommand\deind[1]{\mbox{$\semm{\TargetClass}^{#1}$}}           %      C^#1
\newcommand\deindl[2]{\mbox{$_{#1}\semm{\TargetClass}^{#2}$}}     % _{#1}D^{#2}
\newcommand\deindr[2]{\mbox{$\semm{\TargetClass}_{#1}^{#2}$}}     %      D_{#1}^{#2}


% apply
\newcommand\dtu{\mbox{$^{\ltt}\!\TargetClass^{\ltu}$}}
\newcommand\detplusu{\deindr{+\ltu}{\ltt}}
\newcommand\detnullu{\deindr{0\ltu}{\ltt}}
\newcommand\deuminust{\deindl{-\ltt}{\ltu}}
\newcommand\deunullt{\deindl{0\ltt}{\ltu}}


%\newcommand\f{\mbox{$\AReference$}}                    %   f
\newcommand\fm{\AReference}                              %   f
%\newcommand\find[1]{\mbox{$\AReference^{#1}$}}           %      f^#1
%\newcommand\findl[2]{\mbox{$_{#1}\AReference^{#2}$}}     % _{#1}C^{#2}
%\newcommand\findr[2]{\mbox{$\AReference_{#1}^{#2}$}}     %      C_{#1}^{#2}

\newcommand\feind[1]{\mbox{$\semm{\AReference}^{#1}$}}           %      f^#1
\newcommand\feindl[2]{\mbox{$_{#1}\semm{\AReference}^{#2}$}}     % _{#1}C^{#2}
\newcommand\feindr[2]{\mbox{$\semm{\AReference}_{#1}^{#2}$}}     %      C_{#1}^{#2}

\newcommand\ftu{\find{\ttu}}

\newcommand\fe{\mbox{$\semm{\AReference}$}}              % ||f||
\renewcommand\feind[1]{\mbox{$\semm{\AReference}^{#1}$}}   % ||f||^#1
\newcommand\fet{\feind{\ltt}}
\newcommand\fes{\feind{\lts}}
\newcommand\feu{\feind{\ltu}}
\newcommand\fev{\feind{\tv}}
\newcommand\feJ{\feind{\J}}

\newcommand\femt{\mbox{$\semm{\AReference^{-1}}^{\ltt}$}}


\newcommand\findeind[2]{\mbox{$\semm{\AReference_{#1}}^{#2}$}}
\newcommand\fieu[1]{\findeind{#1}{\ltu}}
\newcommand\fiet[1]{\findeind{#1}{\ltt}}
\newcommand\fies[1]{\findeind{#1}{\lts}}                         % ||C||^t
%\newcommand\fiet{\findeind{i}{\ltt}}                         % ||C||^t
\newcommand\fjet{\findeind{j}{\ltt}}                         % ||C||^t
\newcommand\fket{\findeind{k}{\ltt}}                         % ||C||^t
\newcommand\flet{\findeind{l}{\ltt}}                         % ||C||^t
\newcommand\fkeu{\findeind{k}{\ltu}}                         % ||C||^t

\newcommand\fetplusu{\feindr{+\ltu}{\ltt}}
\newcommand\fetnullu{\feindr{0\ltu}{\ltt}}
\newcommand\feuminust{\feindl{-\ltt}{\ltu}}
\newcommand\feunullt{\feindl{0\ltt}{\ltu}}



%\newcommand\diet{\dindeind{i}{\ltt}}                         % ||C||^t
%\newcommand\djes{\dindeind{j}{\lts}}                         % ||C||^t

\newcommand\fieJ{\feind{\J}}
\newcommand\fjeJ{\feind{\J}}

\newcommand\fgcomp{\mbox{$\f(\g_1,\ldots,\g_m)$}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% The old version where \tj denotes t, \tk denotes u  etc
%%% The new version see on line 185

\newcommand\tjk{\EarlierMoment\LaterMoment}   %jk
\newcommand\tj{\EarlierMoment}               %j
\newcommand\tk{\LaterMoment}                  %k
\newcommand\tjlk{\mbox{$\tj\le\kt$}}
\newcommand\ti{\EarlierEarlierMoment}        %i
\newcommand\tl{\LaterLaterMoment}             %l

%\newcommand\J{\AHistory}                      %J

\newcommand\interjk[1]{\inter{\tjk}{#1}}                 % \eps^jk_#1
\newcommand\dominterjk[1]{\ldom{\interjk{#1}}}  %\Box\eps^jk_#1
\newcommand\codinterjk[1]{\rdom{\interjk{#1}}}  %\eps^jk_#1\Box

\newcommand\interjj[1]{\inter{\tj\tj}{#1}}                 % \eps^jk_#1
\newcommand\interij[1]{\inter{\ti\tj}{#1}}                 % \eps^jk_#1
%\newcommand\interjk[1]{\inter{\tj\tk}{#1}}                 % \eps^jk_#1
\newcommand\interik[1]{\inter{\ti\tk}{#1}}                 % \eps^jk_#1


\newcommand\intercjj{\inter{\tj\tj}{\cm}}                 % \eps^jk_#1
\newcommand\intercij{\inter{\ti\tj}{\cm}}                 % \eps^jk_#1
\newcommand\intercjk{\inter{\tj\tk}{\cm}}                 % \eps^jk_#1
\newcommand\intercik{\inter{\ti\tk}{\cm}}                 % \eps^jk_#1

\newcommand\domintercjk{\dominterjk{\cm}}  %\Box\eps^jk_#1
\newcommand\codintercjk{\codinterjk{\cm}}  %\eps^jk_#1\Box

\newcommand\interdjj{\inter{\tj\tj}{\dm}}                 % \eps^jk_#1
\newcommand\interdij{\inter{\ti\tj}{\dm}}                 % \eps^jk_#1
\newcommand\interdjk{\inter{\tj\tk}{\dm}}                 % \eps^jk_#1
\newcommand\interdik{\inter{\ti\tk}{\dm}}                 % \eps^jk_#1

%----------------------------------------------
%% Classes and arrows
%-------------------------------------------------

%\renewcommand\c{\mbox{$\AClass$}}                    %   C
%\newcommand\cm{\AClass}                              %   C

%\newcommand\ce{\mbox{$\semm{\AClass}$}}              % ||C||
%\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}   % ||C||^#1
\newcommand\cej{\ceind{\tj}}                         % ||C||^j
\newcommand\cek{\ceind{\tk}}                         % ||C||^k
%\newcommand\ceJ{\ceind{\J}}
%--- function:
%\newcommand\cindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
% apply:
\newcommand\ciej{\cindeind{i}{\tj}}                         % ||C_i||^j
\newcommand\cjej{\cindeind{j}{\tj}}                         % ||C_j||^j
\renewcommand\cieJ{\ceind{\J}}
\newcommand\cjeJ{\ceind{\J}}

% function:
%\newcommand\cind[1]{\mbox{$\AClass^{#1}$}}           %      C^#1
%\newcommand\cindl[2]{\mbox{$_{#1}\AClass^{#2}$}}     % _{#1}C^{#2}
%\newcommand\cindr[2]{\mbox{$\AClass_{#1}^{#2}$}}     %      C_{#1}^{#2}
%  apply:
\newcommand\cjk{\cind{\tj\tk}}
\newcommand\cjplusk{\cindr{+\tk}{\tj}}
\newcommand\cjnullk{\cindr{0\tk}{\tj}}
\newcommand\ckminusj{\cindl{-\tj}{\tk}}
\newcommand\cknullj{\cindl{0\tj}{\tk}}


% the same for D

%\renewcommand\d{\mbox{$\TargetClass$}}                    %   D
%\renewcommand\dm{\TargetClass}                              %   D

%\newcommand\de{\mbox{$\semm{\TargetClass}$}}              % ||D||

%\newcommand\deind[1]{\mbox{$\semm{\TargetClass}^{#1}$}}   % ||D||^#1
%\newcommand\dindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}

%\newcommand\dind[1]{\mbox{$\TargetClass^{#1}$}}           %      C^#1
%\newcommand\dindl[2]{\mbox{$_{#1}\TargetClass^{#2}$}}     % _{#1}D^{#2}
%\newcommand\dindr[2]{\mbox{$\TargetClass_{#1}^{#2}$}}     %      D_{#1}^{#2}



%  Apply:
\newcommand\dej{\deind{\tj}}                         % ||C||^j
\newcommand\dek{\deind{\tk}}                         % ||C||^k
%\newcommand\deJ{\deind{\J}}

\newcommand\diei{\dindeind{i}{\ti}}                         % ||C||^j
\newcommand\djej{\dindeind{j}{\tj}}                         % ||C||^j
%\newcommand\dieJ{\deind{\J}}
%\newcommand\djeJ{\deind{\J}}

\newcommand\djk{\dind{\tj\tk}}
\newcommand\djplusk{\dindr{+\tk}{\tj}}
\newcommand\djnullk{\dindr{0\tk}{\tj}}
\newcommand\dkminusj{\dindl{-\tj}{\tk}}
\newcommand\dknullj{\dindl{0\tj}{\tk}}


%\renewcommand\f{\mbox{$\AReference$}}                    %   f
%\newcommand\fm{\AReference}                              %   f
%\newcommand\find[1]{\mbox{$\AReference^{#1}$}}           %      f^#1
\newcommand\fjk{\find{\tjk}}

%\newcommand\fe{\mbox{$\semm{\AReference}$}}              % ||f||
%\newcommand\feind[1]{\mbox{$\semm{\AReference}^{#1}$}}   % ||f||^#1
\newcommand\fej{\feind{\tj}}
\newcommand\fei{\feind{\ti}}
\newcommand\fek{\feind{\tk}}
\newcommand\fel{\feind{\tl}}

%\newcommand\feJ{\feind{\J}}

%\newcommand\findeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
%\newcommand\diei{\dindeind{i}{\ti}}                         % ||C||^j
%\newcommand\djej{\dindeind{j}{\tj}}                         % ||C||^j
 \newcommand\fiei{\findeind{i}{\ti}}                         % ||C||^j
 \newcommand\fjej{\findeind{j}{\tj}}                         % ||C||^j
%\newcommand\fieJ{\feind{\J}}
%\newcommand\fjeJ{\feind{\J}}

%\newcommand\fgcomp{\mbox{$\f(\g_1,\ldots,\g_m)$}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\Distinctctu{\mbox{$^{\ltt}\!\semm{\ittt{Distinct}_{\cm}}^{\ltu}$}}
\newcommand\Distinctcst{\mbox{$^{\lts}\!\semm{\ittt{Distinct}_{\cm}}^{\ltt}$}}
\newcommand\Samectu{\mbox{$^{\ltt}\!\semm{\ittt{Same}_{\cm}}^{\ltu}$}}
\newcommand\Samecst{\mbox{$^{\lts}\!\semm{\ittt{Same}_{\cm}}^{\ltt}$}}
%=============
%%%%% Behset
\newcommand\xstatei[3]{\mbox{${\mathit {#1}state}^{#3}_{#2}$}}
\newcommand\statei[2]{\xstatei{}{#1}{#2}}
\newcommand\xstate[2]{\xstatei{#1}{}{#2}}
%\newcommand\tstatei[1]{\statei{#1}{\ltt}}

\newcommand\attrName[1]{{\mathit #1}}
\newcommand\methName[1]{{\mathit #1}}
\newcommand\statepoint[1]{#1}

%%%%%
% discussing string-based  vs graph-based logics
\newcommand\cmlang{{\bf L}}
\newcommand\myindex[1]{\mbox{\scriptsize{#1}}}
\newcommand\mathsymbol[1]{\mbox{$#1$}}
%\newcommand\repr{\mathsymbol{r}}
\newcommand\world%{\ittt{world}}
{\mathsymbol{\cal W}}
\newcommand\cmter%{\ittt{computer}}
{\mathsymbol{\cal C}}
\newcommand\topos{\mathsymbol{\cal S}}


%----------------------
\newcommand\viewob[1]{\object{V}{#1}}
\newcommand\thob[1]{\object{T}{#1}}
\newcommand\uniob[1]{\object{U}{#1}}
\newcommand\uniobmath[1]{\objectmath{U}{#1}}
\newcommand\uniobind[1]{\objectind{U}{#1}}

\newcommand\UNI{\universe{U}}
\newcommand\UNIind{\universeind{U}}
\newcommand\UNImath{\universeind{U}} % the same
\newcommand\Setsind{\universeind{Sets}}

\newcommand\particularUni[1]{\mbox{$\mathbf{#1}$}}
\newcommand\particularUniInd[1]{\mathbf{#1}}
\newcommand\Sets{\particularUni{Sets}}
\newcommand\Varsets{\particularUni{VarSets}}
\newcommand\Behsets{\particularUni{BehSets}}
\newcommand\Sketches{\particularUni{Sketches}}


\newcommand\skeproc{\proc{ske}}
\newcommand\arrdlproc{\procind{Formal}{ArrDL}}
\newcommand\elmslproc{\procind{Formal}{ElmSL}}

%\newcommand\formalPar[1]{\mbox{$\mathrm #1$}}
\newcommand\formalParBold[1]{\mbox{$#1$}}
\newcommand\lf{\formalParBold{L}}
\newcommand\mf{\formalPar{M(D)}}
\newcommand\uf{\formalPar{U}}
\newcommand\df{\formalPar{D}}
\newcommand\tdf{\mbox{$\thob(\diag)$}}
\newcommand\sdf{\mbox{$\skeob{}(\diag)$}}

\newcommand\str{\formalPar{\sigma}}
%(7)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Created on May 4,2001
%============================================
% Part 1: pure italic writing of names
%        formerly file italic.tex
%--------------------------------------------
% Part 2: commands for semantics extensions of classes
%         like [[Person]]^t or {^t}[[SamePerson]]^{u}
%        formerly file employ.tex
%===========================================

\newcommand\operarrow[2]{\mbox{{\sffamily%\itshape
                                         #1}$_{#2}$}}
\newcommand\projop[1]{\operarrow{p}{#1}}
%\newcommand\concatop{\operarrow{concat}{}}
%\newcommand\pairop{\operarrow{pair}{}}
%\newcommand\idop[1]{\operarrow{id}{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\newcommand\ltt{\mbox{$t$}}
%\newcommand\ltu{\mbox{$u$}}
%\newcommand\lts{\mbox{$s$}}

%

\newcommand\Emplsem[1]{\mbox{$\semm{\Empl}^{#1}$}}
\newcommand\Emplt{\Emplsem{\ltt}}
\newcommand\Emplu{\Emplsem{\ltu}}
\newcommand\Empls{\Emplsem{\lts}}
\newcommand\Empltu{\mbox{$^{\ltt}\!\semm{\Empl}^{\ltu}$}}
\newcommand\Emplst{\mbox{$^{\lts}\!\semm{\Empl}^{\ltt}$}}
\newcommand\SameEmpltu{\mbox{$^{\ltt}\!\semm{\SameEmpl}^{\ltu}$}}
\newcommand\SameEmplst{\mbox{$^{\lts}\!\semm{\SameEmpl}^{\ltt}$}}

\newcommand\Compsem[1]{\mbox{$\semm{\Comp}^{#1}$}}
\newcommand\Compt{\Compsem{\ltt}}
\newcommand\Compu{\Compsem{\ltu}}
\newcommand\Comps{\Compsem{\lts}}
\newcommand\Comptu{\mbox{$^{\ltt}\!\semm{\Comp}^{\ltu}$}}
\newcommand\Compst{\mbox{$^{\lts}\!\semm{\Comp}^{\ltt}$}}
\newcommand\SameComptu{\mbox{$^{\ltt}\!\semm{\SameComp}^{\ltu}$}}
\newcommand\SameCompst{\mbox{$^{\lts}\!\semm{\SameComp}^{\ltt}$}}

\newcommand\Engrsem[1]{\mbox{$\semm{\Engr}^{#1}$}}
\newcommand\Engrt{\Engrsem{\ltt}}
\newcommand\Engru{\Engrsem{\ltu}}
\newcommand\Engrs{\Engrsem{\lts}}
\newcommand\Engrtu{\mbox{$^{\ltt}\!\semm{\Engr}^{\ltu}$}}
\newcommand\Engrst{\mbox{$^{\lts}\!\semm{\Engr}^{\ltt}$}}

\newcommand\Mngrsem[1]{\mbox{$\semm{\Mngr}^{#1}$}}
\newcommand\Mngrt{\Mngrsem{\ltt}}
\newcommand\Mngru{\Mngrsem{\ltu}}
\newcommand\Mngrs{\Mngrsem{\lts}}
\newcommand\Mngrtu{\mbox{$^{\ltt}\!\semm{\Mngr}^{\ltu}$}}
\newcommand\Mngrst{\mbox{$^{\lts}\!\semm{\Mngr}^{\ltt}$}}

\newcommand\John[1]{\mbox{$\ittt{John}^{#1}$}}

\newcommand\Marr{\ittt{Married}}
\newcommand\Marrsem[1]{\mbox{$\semm{\Marr}^{#1}$}}
\newcommand\Marrt{\Marrsem{\ltt}}
\newcommand\Marru{\Marrsem{\ltu}}
\newcommand\Marrs{\Marrsem{\lts}}
\newcommand\Marrtu{\mbox{$^{\ltt}\!\semm{\Marr}^{\ltu}$}}
\newcommand\Marrst{\mbox{$^{\lts}\!\semm{\Marr}^{\ltt}$}}

\newcommand\Famy{\ittt{Family}}
\newcommand\Famysem[1]{\mbox{$\semm{\Famy}^{#1}$}}
\newcommand\Famyt{\Famysem{\ltt}}
\newcommand\Famyu{\Famysem{\ltu}}
\newcommand\Famys{\Famysem{\lts}}
\newcommand\Famytu{\mbox{$^{\ltt}\!\semm{\Famy}^{\ltu}$}}
\newcommand\Famyst{\mbox{$^{\lts}\!\semm{\Famy}^{\ltt}$}}
\newcommand\Famytt{\mbox{$^{\ltt}\!\semm{\Famy}^{\ltt}$}}
\newcommand\Familytu{\mbox{$^{\ltt}\!\semm{\Famy}^{\ltu}$}}
\newcommand\Familyst{\mbox{$^{\lts}\!\semm{\Famy}^{\ltt}$}}

\newcommand\Friendship{\ittt{Friendship}}
\newcommand\Friship{\ittt{Friendship}}
\newcommand\Frishiptu{\mbox{$^{\ltt}\!\semm{\Friship}^{\ltu}$}}
\newcommand\Frishipst{\mbox{$^{\lts}\!\semm{\Friship}^{\ltt}$}}


\newcommand\Matr{\ittt{Matrimony}}
\newcommand\Matrsem[1]{\mbox{$\semm{\Matr}^{#1}$}}
\newcommand\Matrt{\Matrsem{\ltt}}
\newcommand\Matru{\Matrsem{\ltu}}
\newcommand\Matrs{\Matrsem{\lts}}
\newcommand\Matrtu{\mbox{$^{\ltt}\!\semm{\Matr}^{\ltu}$}}
\newcommand\Matrst{\mbox{$^{\lts}\!\semm{\Matr}^{\ltt}$}}

\newcommand\Distincttu{\mbox{$^{\ltt}\!\semm{\ittt{Distinct}}^{\ltu}$}}
\newcommand\Distinctst{\mbox{$^{\lts}\!\semm{\ittt{Distinct}}^{\ltt}$}}
\newcommand\Sametu{\mbox{$^{\ltt}\!\semm{\ittt{Same}}^{\ltu}$}}
\newcommand\Samest{\mbox{$^{\lts}\!\semm{\ittt{Same}}^{\ltt}$}}

\newcommand\Wom{\ittt{Woman}}
\newcommand\Womsem[1]{\mbox{$\semm{\Wom}^{#1}$}}
\newcommand\Womt{\Womsem{\ltt}}
\newcommand\Womu{\Womsem{\ltu}}
\newcommand\Woms{\Womsem{\lts}}
\newcommand\Womtu{\mbox{$^{\ltt}\!\semm{\Wom}^{\ltu}$}}
\newcommand\Womst{\mbox{$^{\lts}\!\semm{\Wom}^{\ltt}$}}

%\newcommand\Man{\ittt{Man}}
\newcommand\Mansem[1]{\mbox{$\semm{\Man}^{#1}$}}
\newcommand\Mant{\Mansem{\ltt}}
\newcommand\Manu{\Mansem{\ltu}}
\newcommand\Mans{\Mansem{\lts}}
\newcommand\Mantu{\mbox{$^{\ltt}\!\semm{\Man}^{\ltu}$}}
\newcommand\Manst{\mbox{$^{\lts}\!\semm{\Man}^{\ltt}$}}

\newcommand\Husbsem[1]{\mbox{$\semm{\Husb}^{#1}$}}
\newcommand\Husbt{\Husbsem{\ltt}}
\newcommand\Husbu{\Husbsem{\ltu}}
\newcommand\Husbs{\Husbsem{\lts}}
\newcommand\Husbtu{\mbox{$^{\ltt}\!\semm{\Husb}^{\ltu}$}}
\newcommand\Husbst{\mbox{$^{\lts}\!\semm{\Husb}^{\ltt}$}}


\newcommand\mysemm[2]{\mbox{$\semm{#1}^{#2}$}}

\newcommand\isarrt{\mysemm{\isa}{\ltt}}
\newcommand\isarru{\mysemm{\isa}{\ltu}}

\newcommand\wifet{\mysemm{\wife}{\ltt}}
\newcommand\wifeu{\mysemm{\wife}{\ltu}}

\newcommand\husbt{\mysemm{\husb}{\ltt}}
\newcommand\husbu{\mysemm{\husb}{\ltu}}

\newcommand\mdatet{\mysemm{\mDate}{\ltt}}
\newcommand\mdateu{\mysemm{\mDate}{\ltu}}

\newcommand\liveset{\mysemm{\livesAt}{\ltt}}
\newcommand\liveseu{\mysemm{\livesAt}{\ltu}}

\newcommand\income{\ittt{income}}
\newcommand\WMHsem[2]{\mbox{$
      (\semm{\Wom}^{#1}\times\semm{\Man}^{#1}\times\semm{\House}^{#1})
\times
      (\semm{\Wom}^{#2}\times\semm{\Man}^{#2}\times\semm{\House}^{#2})
                            $}
                     }
\newcommand\WMHtu{\WMHsem{\ltt}{\ltu}}


\newcommand\WMWMsem[2]{\mbox{$(\semm{\Wom}^{#1}\times\semm{\Man}^{#1})
                        \times(\semm{\Wom}^{#2}\times\semm{\Man}^{#2})
                             $}
                        }
\newcommand\WMWMtu{\WMWMsem{\ltt}{\ltu}}


\newcommand\myview[1]{\mbox{$V_{#1}$}}
\newcommand\IndI{1}
\newcommand\SWAggr{2}
\newcommand\AggrI{3}
\newcommand\TWAggrG{4}
\newcommand\IndII{5}
\newcommand\TWAggrS{6}
\newcommand\LAggr{7}
\newcommand\LLAggr{8}
\newcommand\SWLAggr{9}
\newcommand\STWAggr{10}
\newcommand\DelAggr{11}
\newcommand\TotAggr{12}
\newcommand\WQual{13}
 \newcommand\LQual{14}
\newcommand\AttrI{15}
\newcommand\SWLQual{16}
\newcommand\STWQual{17}
\newcommand\AttrII{18}



%(8)
%\newcommand\s{\mbox{$S$}}
%\newcommand\os{\mbox{$\overline{S}$}}
%\newcommand\ovr[1]{\mbox{$\overline{#1}$}}
\newcommand\into[1]{\stackrel{#1}{\hookrightarrow}}
\newcommand\repgra{\nicex{ R$}}
\newcommand\rgra{\repgra}
\newcommand\nds[1]{\mbox{$\mathit{Nds}#1$}}
\newcommand\arrs[1]{\mbox{$\mathit{Arrs}#1$}}
\newcommand\ndsr{\nds{\rgra}}
\newcommand\arrsr{\arrs{\rgra}}

\newcommand\dersetmath{\mathit{Der}}
\newcommand\derset{\mbox{$\dersetmath$}}
\newcommand\derop{\mbox{$\mathbf{der}$}}
\newcommand\algebra[1]{\mbox{$\alpha^{#1}$}}
\newcommand\algu{\algebra{\uskemath}}

%\newcommand\inss[1]{\lar{I}{\ske{#1}}{\uske}}
%\newcommand\ovri{\mbox{$\overline{I}$}}
%\newcommand\ovrinss[1]{\lar{\ovri_{#1}}{\ovrs{#1}}{\uske}}

\newcommand\ovrske[1]{\mbox{$\overline{\ske{#1}}$}}
\newcommand\ovrs[1]{\mbox{$\overline{\ske{#1}}$}}
%-----------------------------
\newcommand\sv{\mbox{$\ske{V}$}}
\newcommand\sr{\mbox{$\ske{R}$}}
\newcommand\vmor{\lar{v}{\sv}{\ovrske{}}}
\newcommand\rmor{\lar{r}{S}{\ovrske{R}}}
\newcommand\emor{\lar{e}{S}{\U}}
\newcommand\vpair{\mbox{$V=(\sv,v)$}}
\newcommand\rpair{\mbox{$R=(\sr,r)$}}



%\newcommand\dbinst{\lar{e}{S}{W} }

%---------------------------------------------------


\newcommand\ovrsig[1]{\mbox{$\overline{\sigma _{#1}}$}}
\newcommand\ovrg[1]{\mbox{$\overline{G_{#1}}$}}
%-----------------------------------------
\newcommand\ovrp{\mbox{$\overline{\pi }$}}%{#1}}$}}
\newcommand\ovreps{\mbox{$\overline{\vare}$}}     % overlined epsilon


%\renewcommand\endinput{}
%\newcommand\comp{\mathbin{\triangleright\!\!\triangleright}}
\newcommand\state[2]{\mbox{${\mathit{state}}^{#1}_{#2}$}}
\newcommand\starInherit{*-inherit}

\newcommand\sig{\mbox{$\Sigma $}}
\newcommand\sigm{\Sigma}
\newcommand\defitemotstup[1]{\par\smallskip\noindent (#1)}


\newcommand\arity[1]{\mbox{$\mathit{Arity}(#1)$}}
\newcommand\predsem[2]{\mbox{$\semm{#1}^{#2} $}}
\newcommand\psem[1]{\predsem{P}{#1}}
\newcommand\psemu{\psem{\ucatmath}}
\newcommand\lsig{\mbox{$\Lambda $}}

%%%
\newcommand\Attr{\mbox{$\mathit{Attr}$}}
\newcommand\Var{\mbox{$\mathit{Var}$}}
\newcommand\relcat{\mbox{$\categoryname{Rel}$}}
\newcommand\relske{\mbox{$\sketchname{Rel}$}}
\newcommand\itte[1]{\mbox{\textit{#1}}}
\newcommand\dbcat{\mbox{$\categoryname{DB}$}}

\newcommand\skecat[1]{\mbox{$\categoryname{Sketch}(\sig_{#1})$}}
\newcommand\sigcat{\mbox{$\categoryname{Sign}$}}

\newcommand\funor{\mbox{$\Phi$}}
\newcommand\funarr{\lar{f}{X}{Y}}
\newcommand\currfun{\mbox{\lar{\Map{A}{\_}}{\catset}{\catset}}}
\newcommand\curra{\Map{A}{\_}}

% \newcommand\ {\itte{ }}
\newcommand\target{\itte{target}}
\newcommand\source{\itte{source}}
\newcommand\conof{\itte{consistsOf}}
\newcommand\marker{\itte{marker}}
\newcommand\Node{\itte{Node}}
\newcommand\nodeit{\ittt{node}}
\newcommand\Arrow{\itte{Arrow}}
\newcommand\arrow{\ittt{arrow}}
\newcommand\diagramit{\itte{diagram}}
\newcommand\graphit{\itte{graph}}
\newcommand\shape{\itte{shape}}
\newcommand\predecl{\itte{predicate\_declarations}}
\newcommand\statements{\itte{statements}}
\newcommand\carrier{\itte{carrier}}
\newcommand\arityshape{\itte{arity\_shape}}


% semiotics
%% MACROS OF Dec 3
\newcommand\formalObj[1]{\mbox{\sffamily #1}}
\newcommand\formalOper[1]{\mbox{{\bfseries\sffamily #1}}}
\newcommand\informalObj[1]{\mbox{\textit #1}}
\newcommand\informalOper[1]{\mbox{{\bfseries\itshape #1}}}

\newcommand\lzzl{\formalObj{l}}  %logic
\newcommand\ml{\informalObj{ML}}  % modeling language

\newcommand\f{\formalObj{F}}
\renewcommand\c{\informalObj{C}}
\newcommand\derf{\formalOper{Der}}
\newcommand\deri{\informalOper{Un}}
\newcommand\derff{\derf.\f}
\newcommand\deric{\deri(\c)}
\newcommand\FormalInterpret[1]{\mbox{$\formalObj{i}_f$}}
\newcommand\SubstantInterpret[1]{\mbox{$\informalObj{i}_s$}}


%====================================

\newcommand\informalPar[1]{\nicex{{#1}$}}
\newcommand\infParind[1]{\cal #1}
\newcommand\formalPar[1]{\mbox{$\mathrm{#1}$}}
\newcommand\frmParind[1]{\mathrm{#1}}

\newcommand\informalParBold[1]{\mbox{${\cal #1}$}}
%\newcommand\formalPar[1]{\mbox{$\mathrm #1$}}

\newcommand\object[2]{\mbox{${\mathsf{#1}}_{#2}$}}
%\newcommand\object[2]{\mbox{$#1_{#2}$}}
\newcommand\universe[1]{\mbox{$\mathbf{#1}$}}
%\newcommand\objectind[1]{\mathsf{#1}}
\newcommand\objectind[1]{\mathsf{#1}}
\newcommand\objectmath[1]{\mathsf{#1}} % the same
\newcommand\universeind[1]{\mathbf{#1}}
\newcommand\umath[1]{\mathbf{U}_{#1}}

\newcommand\proc[1]{\mbox{\sffamily\bfseries #1}}
\newcommand\procind[2]{\mbox{${\mathrm{#1}}_{\mathrm #2}$}}
\newcommand\linf{\informalParBold{L}}
\newcommand\minf{\mbox{$\informalPar{M}(\diag{})$}}
\newcommand\mdinf{\mbox{$\informalPar{M}(\diag{})$}} % the same as above
\newcommand\mdfrm{\mbox{$\formalPar{M}(\diag{})$}} % the same as above
\newcommand\uinf{\informalPar{U}}

\newcommand\meaninf{\informalPar{M}}
\newcommand\meanfrm[1]{\mbox{$\formalPar{M}_{#1}$}}

\newcommand\diags{\mbox{$\mathit{Diags}$}}
\newcommand\graph{\mbox{$\mathit{Graph}$}}

\newcommand\diaob[1]{\object{D}{#1}} %\mbox{$D$}}
\newcommand\diagob[1]{\object{D}{#1}} %the same \mbox{$D$}}
\newcommand\diag[1]{\object{D}{#1}} %the same \mbox{$D$}}
\newcommand\diaind{\objectind{D}}

\newcommand\graob[1]{\object{G}{#1}}
\newcommand\graind{\objectind{G}}
\newcommand\gra[1]{\graob{#1}}

\newcommand\skeob[1]{\object{S}{#1}}
\newcommand\skeind{\objectind{S}}

\newcommand\modelob[1]{\object{M}{#1}}
\newcommand\modelind{\objectind{M}}

\newcommand\sigob[1]{\object{\mbox{$\Sigma$}}{#1}}
\newcommand\skediag{\skeob{}[\diag{}]}

\newcommand\meaninfdiag{\meaninf[\diag{}]}
\newcommand\meanfrmdiag{\meanfrm[\diag{}]}
% synonyms
\newcommand\meanifdiag{\meaninf[\diag{}]}
\newcommand\meanfdiag{\meanfrm[\diag{}]}

%%% diags, sketchs, specs, and their semantic interpretaions
\newcommand\objectWithInd[3]{\mbox{$\mathsf{#1}_{#2}^{#3}$}}
\newcommand\sketch[1]{\objectWithInd{S}{#1}{}}
\renewcommand\ske[1]{\sketch{#1}}
%\newcommand\graph[1]{\objectWithInd{S}{#1}{}}
\renewcommand\diag[1]{\objectWithInd{D}{#1}{}}
%\newcommand\inst[2]{\mbox{$\mathit{Inst}^{#2}{(#1)}$}}
%\newcommand\instob[2]{\mbox{$\mathit{Inst}^{#2}{(#1)}$}}


%\newcommand\diaob[1]{\mbox{$\diag{#1}$}}
%\newcommand\skeob{\mbox{$S$}}
\newcommand\graofske{\mbox{$G_\skeind$}}
\newcommand\graske{\graofske}
\newcommand\diaofske{\mbox{$D_\skeind$}}
\newcommand\diaske{\diaofske}


\renewcommand\eg{e.g.}
\renewcommand\C{\mbox{$C$}}

\newcommand\ext[1]{\mbox{$\mathit{Ext}(#1)$}}
\renewcommand\stt[1]{\mbox{$\mathit{Stt}(#1)$}}
\newcommand\GCS{{\bf (GCS)}}
\newcommand\AET{{\bf (AET)}}



%\newcommand\tuple[1]{\left [ \mathstrut {#1} \right ]}
\newcommand\pmrk[1]{\mbox{[{\sf #1}]}}
\newcommand\omrk[1]{\mbox{[{\sf #1} $\rangle $}}

% used in Intro
\newcommand\lanfrm{\formalPar{FL}}
\newcommand\flan{\formalPar{FL}} %the same
\newcommand\flanind{\frmParind{FL}}

\newcommand\x{\diag{}}   %\mbox{$D$}}
\renewcommand\s{\skeob{}}%\mbox{$S$}}
%\newcommand\mix{\mbox{$\meaninf$}} %(\x)
%\newcommand\mfx{\mbox{$\meanfrm{\flanind}$}} %(\x)
\newcommand\mix{\mbox{$\meaninf(\x)$}}
\newcommand\mfx{\mbox{$\meanfrm{}(\x)$}}

%\newcommand\flan{\mbox{$\meanfrm(\x)$}}

\newcommand\spex[1]{\mbox{$\skeob{#1}$}} %(\mix)$}}
\newcommand\spem[1]{\mbox{$\skeob{#1}$}} %(\mix)$}}
\newcommand\spexl  {\mbox{$\skeob{\flanind}$}} %(\x)$}}
\newcommand\speml  {\mbox{$\skeob{}$}} %(\mfx)$}}

\newcommand\dateit{\ittt{date}}

% used in dGetStartViaAss
\newcommand\nis{\nicex{ S$}}
\newcommand\niv{\nicex{ V$}}
\newcommand\nivind{{V}}
\newcommand\nisind{{S}}

\newcommand\mrkdual[3]{\mbox{${#2}\stackrel{{\cal\scriptsize #1}}{[><]}{#3}$}} %{[>^{\mathrm{#1}}<]}$}}
\newcommand\sgv{single-valued}
\newcommand\assgenpred{\mbox{$[\Uparrow]$}}
\newcommand\SepPred{\mrk{1-1}  }
\newcommand\CovPred{\mrk{cover}}
\newcommand\MemPred{\mrk{$\in$}}

\newcommand\binAss{1}
\newcommand\assCla{2}
\newcommand\reiAss{3}
\newcommand\terAss{4}
\newcommand\quaAss{5}
\newcommand\skeo{\skeob{\binAss}}
\newcommand\skei{\skeob{\assCla}}
\newcommand\skeii{\skeob{\reiAss}}
\newcommand\skeiii{\skeob{\terAss}}
\newcommand\skeiv{\skeob{\quaAss}}
%\newcommand\diaob[1]{\diag{#1}}
\newcommand\diao{\diaob{\binAss}}
\newcommand\diai{\diaob{\assCla}}
\newcommand\diaii{\diaob{\reiAss}}
\newcommand\diaiii{\diaob{\terAss}}
\newcommand\diaiv{\diaob{\quaAss}}


\newcommand\visfunctor{\mbox{{\sffamily\bfseries vis}}}
\newcommand\skefunctor{\mbox{{\sffamily\bfseries ske}}}

%used in eAssonBySke
\newcommand\sale{\ittt{sale}}
\newcommand\Show{\ittt{Show}}
\renewcommand\show{\ittt{show}}
\newcommand\seat{\ittt{seat}}
\newcommand\perf{\ittt{perf}}
\newcommand\Performance{\ittt{Performance}}
\newcommand\Ticket{\ittt{Ticket}}
\newcommand\ticket{\ittt{sale}}
\newcommand\Integer{\ittt{Integer}}

\newcommand\mastr[1]{\mbox{$\mathbf{#1}$}}
\newcommand\extofcla[1]{\mastr{\semm{\mathit #1}}}
\newcommand\behofcla[1]{\mastr{\besemm{\mathit{#1}}}}
\newcommand\sttofcla[1]{\lar{\statemap{}{\mathit{#1}}}{\extofcla{#1}}{\behofcla{#1}}}

%\newcommand\tlu{\mbox{$t<u$}}
%\newenvironment\mathitext%
%{
%\begin{displaymath}
%\mbox{ }
%\end{displaymath}
%} {}
\newcommand\cEngine{\ittt{carEngine}}
\newcommand\carEngine{\ittt{carEngine}}


\newcommand\mrkmon[2]{\mbox{\mrk{1-1}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkfro[2]{\mbox{\mrk{fro}$^{#1}_{\mathit{#2}}$}}
\renewcommand\mrkid[2]{\mbox{\mrk{id}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkstrongid[2]{\mbox{\mrk{id!}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkdel[2]{\mbox{\mrk{del}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkins[2]{\mbox{\mrk{ins}$^{#1}_{\mathit{#2}}$}}

\newcommand\mathand{\mbox{ and }}
\newcommand\mathor{\mbox{ or }}
\newcommand\mathif{\mbox{ if }}
\newcommand\maththen{\mbox{ then }}
\newcommand\mathiff{\mbox{ iff }}
%\newcommand\ofit{\ittt{of}}
\newcommand\wholeit{\ittt{whole}}
\newcommand\Wholeit{\ittt{Whole}}
\newcommand\partit{\ittt{part}}
\newcommand\stateit{\ittt{state}}
\newcommand\prokol{{\mathbf +}\!\!\!\!\circ}

\newcommand\mixsemm[1]{\mbox{$\lbesemm\, {\mathit #1} \, \rsemm$}}

\newcommand\logrule[2]{\frac{\mathstrut #1}{\mathstrut #2}}
\newcommand\logruleFig[2]{\frac{\mathstrut #1}{\mathstrut #2}}
\newcommand\logruleRow[2]{\mbox{if $#1$ then $#2$}}
\newcommand\logruleFigText[2]{\mbox{$
\frac{\mbox{\rule[-1ex]{0pt}{3ex} #1}}{\mbox{\rule{0pt}{3ex} #2}} $}
}
\newcommand\logruleRowText[2]{\mbox{if #1 then #2}}


\newcommand\ClassIndInd[3]{\mbox{$^{#1}\!\semm{\mathit{#2}}^{#3}$}}
\newcommand\ClassBeh[1]{\mbox{$\besemm{\mathit{#1}}$}}

\newcommand\refInd[2]{\mbox{$\semm{\mathit{#1}}^{\mathit{#2}}$}}
\newcommand\refBehInd[2]{\mbox{$\besemm{\mathit{#1}}^{\mathit{#2}}$}}
\newcommand\refIndBeh[2]{\mbox{$\besemm{\mathit{#1}}^{\mathit{#2}}$}}




\renewcommand\same[2]{\mbox{${\mathit{same}}^{#1}_{\mathit{#2}}$}}
\newcommand\samemap[2]{\mbox{${\mathit{same}}^{#1}_{\mathit{#2}}$}}
%\newcommand\sametu[1]{\samemap{tu}{#1}}
\newcommand\delset[3]{\mbox{$\semm{#3}^{#1}\mathsf{Del}^{#1\rightarrow #2}$}}
\newcommand\deltu[1]{\delset{t}{u}{#1}}
\newcommand\newset[3]{\mbox{$\semm{#3}^{#1}\mathsf{New}^{#2\rightarrow #1}$}}
\newcommand\newut[1]{\newset{u}{t}{#1}}
\newcommand\newts[1]{\newset{t}{s}{#1}}
%\newcommand\insut[1]{\newset{t}{u}{#1}}
%\newcommand\newut[1]{\newset{t\leftarrow u}{#1}} %  correct
%\newcommand\newtu[1]{\newset{t\leftarrow u}{#1}} % incorrect, to match old
%\newcommand\newts[1]{\newset{s\leftarrow t}{#1}} %correct,
%\newcommand\newst[1]{\newset{s\leftarrow t}{#1}} %incorrect, to match old
\newcommand\statemap[2]{\mbox{${\mathit{state}}^{#1}_{\mathit{#2}}$}}



\newcommand\ofit{\ittt{of}}
\newcommand\ofmap[1]{\refInd{of}{#1}}
%\newcommand\ofit{\ofmap{}}
\newcommand\oft{\ofmap{t}}
\newcommand\ofu{\ofmap{u}}

\newcommand\ofindit{\mbox{$\semm{{\mathit of}_i}^{t}$}}
%\newcommand\ofindiu{\mbox{$\semm{{\mathit of}_i}^{u}$}}
\newcommand\ofiu{\mbox{$\semm{{\mathit of}_i}^{u}$}}
%
\newcommand\isit{\ittt{is}}
\newcommand\ismap[1]{\refInd{is}{#1}}
%\newcommand\isit{\ismap{}}
\newcommand\ist{\ismap{t}}
\newcommand\isu{\ismap{u}}


\newcommand\isindt{\mbox{$\semm{{\mathit is}_i}^{t}$}}
\newcommand\isindu{\mbox{$\semm{{\mathit is}_i}^{u}$}}
%

\newcommand\hasit{\ittt{has}}
\newcommand\hasmapbeh{\besemm{has}}
\newcommand\hasbeh{\besemm{has}}
\newcommand\hasbehind[1]{\besemm{has}_{#1}}


\newcommand\supmap[1]{\refInd{sup}{#1}}
\newcommand\supit{\supmap{}}
\newcommand\supt{\supmap{t}}
\newcommand\supu{\supmap{u}}
%
\newcommand\supbeh{\besemm{sup}}
%
\newcommand\submap[1]{\refInd{sub}{#1}}
\newcommand\subit{\submap{}}
\newcommand\subt{\submap{t}}
\newcommand\subu{\submap{u}}

\newcommand\isamap[1]{\refInd{isA}{#1}}
\newcommand\isait{\isamap{}}
\newcommand\isat{\isamap{t}}
\newcommand\isau{\isamap{u}}
\newcommand\isabeh{\besemm{\isa}}

\newcommand\Persontu{\ClassIndInd{t}{Person}{u}}
\newcommand\Persont{\ClassIndInd{}{Person}{t}}
\newcommand\Personu{\ClassIndInd{}{Person}{u}}
\newcommand\PersonBeh{\ClassBeh{Person}}

\newcommand\Drivertu{\ClassIndInd{t}{Driver}{u}}
\newcommand\Drivert{\ClassIndInd{}{Driver}{t}}
\newcommand\Driveru{\ClassIndInd{}{Driver}{u}}



\newcommand\Cart{\ClassIndInd{}{Car}{t}}
\newcommand\Caru{\ClassIndInd{}{Car}{u}}
\newcommand\Cartu{\ClassIndInd{t}{Car}{u}}
\newcommand\SameCartu{\ClassIndInd{t}{SameCar}{u}}
\newcommand\CarBeh{\ClassBeh{Car}}
\newcommand\Carbeh{\ClassBeh{Car}}
\newcommand\Ownershiptu{\ClassIndInd{t}{Ownership}{u}}
\newcommand\Ownershipt{\ClassIndInd{}{Ownership}{t}}
\newcommand\Ownershipu{\ClassIndInd{}{Ownership}{u}}



\newcommand\Ownership{\ittt{Ownership}}
\newcommand\owner{\ittt{owner}}
%\newcommand\car{\ittt{car}}
%\newcommand\property{\ittt{property}}

%\newcommand\Engine{\ittt{Engine}}
%\newcommand\Eng{\ittt{Eng}}
\newcommand\Enginetu{\ClassIndInd{t}{Engine}{u}}
\newcommand\Enginet{\ClassIndInd{}{Engine}{t}}
\newcommand\Engineu{\ClassIndInd{}{Engine}{u}}
\newcommand\EngineBeh{\ClassBeh{Engine}}
\newcommand\Enginebeh{\ClassBeh{Engine}}
\newcommand\Engbeh{\ClassBeh{Engine}}
\newcommand\BodyBeh{\ClassBeh{Body}}
\newcommand\ChassisBeh{\ClassBeh{Chassis}}


%\newcommand\Engine{\ittt{Engine}}
%\newcommand\Eng{\ittt{Eng}}
%\newcommand\Body{\ittt{Body}}
%\newcommand\BodyBeh{\ClassBeh{Body}}
%\newcommand\Chassis{\ittt{Chassis}}
%\newcommand\ChassisBeh{\ClassBeh{Chassis}}
%%\newcommand\PartName{Part}

%\newcommand\drives{\ittt{drives}}
\newcommand\drivest{\refInd{drives}{t}}
\newcommand\drivesu{\refInd{drives}{u}}
\newcommand\drivesbeht{\refBehInd{drives}{t}}
\newcommand\drivesbehu{\refBehInd{drives}{u}}
\newcommand\drivesbehv{\refBehInd{drives}{v}}
\newcommand\drivesbeh{\refBehInd{drives}{}}

\newcommand\fuelat{\refInd{fuelAmount}{t}}
%\newcommand\fuelAm{\ittt{fuelAmount}}
%\newcommand\tankVo{\ittt{tankVolume}}
%\newcommand\fillTa{\ittt{fillTank}}
%\newcommand\car{\ittt{car}}

\newcommand\tankvt{\refInd{tankVolume}{t}}
\newcommand\tankvu{\refInd{tankVolume}{u}}

\newcommand\cart{\refInd{car}{t}}
\newcommand\caru{\refInd{car}{u}}

\newcommand\prst{\refInd{prs}{t}}
\newcommand\prsu{\refInd{prs}{u}}

\newcommand\enginet{\refInd{engine}{t}}
\newcommand\engineu{\refInd{engine}{u}}

\newcommand\persont{\refInd{person}{t}}
\newcommand\personu{\refInd{person}{u}}



\newcommand\PersonP{\Person$^+$}
\newcommand\PersonM{\Person$^-$}
\newcommand\CarP{\Car$^+$}
\newcommand\CarM{\Car$^-$}


\newcommand\floatRange[1]{\mrk{Float(#1)}}

%\newcommand\Car{\ittt{Car}}


\newcommand\becar{\besemm{\Car}}
\newcommand\beCar{\besemm{\Car}}
\newcommand\lt{$t$}
\newcommand\tstate{\statei{}{\ltt}}
\newcommand\stts{\statepoint{s}}



% === composition: begin
\newcommand\ipart[1]{\mbox{$\mathit{Part}_{#1}$}}
\newcommand\ipartmath[1]{\mathit{Part}_{#1}}
\newcommand\ipartbeh[1]{\mbox{$\besemm{\ipart{#1}}$}}

\newcommand\imeth[1]{\mbox{$\mathit{Meth}_{#1}$}}
\newcommand\imethbeh[1]{\mbox{$\besemm{\imeth{#1}}$}}
\renewcommand\imeth[1]{\mbox{$\mathit{Meth}_{#1}$}}
\newcommand\imethstar[1]{\mbox{$\mathit{Meth}^*_{#1}$}}
\newcommand\istameth[1]{\imethstar{#1}} %the same

\newcommand\iiface[1]{\mbox{$\mathbf{IFace}_{#1}$}}
\newcommand\iifacestar[1]{\mbox{$\mathbf{IFace}^*_{#1}$}}
\newcommand\iistaface[1]{\iifacestar{#1}} %the same


\newcommand\prodspace{\mbox{$\prod_{i}\ipartbeh{i}$}}
\newcommand\prodspa{\mbox{$\prod_{i}\ipartbeh{i}$}}
\newcommand\wholespace{\mbox{$\prod_{i}^*\ipartbeh{i}$}}

\newcommand\prodmeths{\mbox{$%\prod_{i}\imeth{i}
                             \methsset{prod}$}}
\newcommand\wholemeths{\mbox{$%\prod^*_{i}\imeth{i}
                             \someofmethsset{Prod}$}}
\newcommand\prodmethsbeh{\mbox{$\besemm{\prodmeths}$}}
\newcommand\wholemethsbeh[2]{\mbox{$\besemm{\someofmeths{#1}{#2}}$}}
\newcommand\prodiface{\mbox{$%\prod_{i}\iiface{i}
                              \iface{Prod}$}}
\newcommand\wholeiface{\mbox{$%\prod^*_{i}\iiface{i}
                               \ifacepartial{Prod}$}}



%\newcommand\reductmap[1]{\mbox{$\mathit{red}^*_{\mathit{#1}}$}}
\newcommand\reductmap[2]{\mbox{$\mathit{red}^{\mathit{#1}}_{\mathit{#2}}$}}
%\newcommand\reductmapstar[1]{\mbox{$\mathit{red}^*_{\mathit{#1}}$}}
\newcommand\red[2]{\reductmap{#1}{#2}}
\newcommand\redsta[1]{\reductmapstar{#1}}
\newcommand\projectmap[1]{\mbox{$\mathit{proj}_{\mathit{#1}}$}}
%\renewcommand\proj[1]{\projectmap{#1}}
\newcommand\fproj[1]{\mbox{$\pi_{#1}$}}


%==== composition: end =========

\renewcommand\Eng[1]{\mbox{$\mathit{Eng}^#1$}}
\renewcommand\eng[1]{\mbox{$\mathit{eng}^#1$}}
\newcommand\ETOC{\Eng{*}} %Engine methods transferred TO Cars
\newcommand\etoc{\eng{*}}
\newcommand\Etocbeh{\besemm{\Engine^*}}
\newcommand\etocind{EngIntoCar}
\newcommand\ctoeind{CarToEng}

\newcommand\me{\mbox{$m$}}
\newcommand\Me{\mbox{$\mathit{Meth}$}}

%\newcommand\meths1]{\mbox{$\mathit{meth}^{\mathit{#1}}$}}
\newcommand\methsset[1]{\mbox{$\mathit{#1}\mathsf{Meth}$}}
%the same
\newcommand\meths[1]{\mbox{$\mathit{#1}\mathsf{Meth}$}}
%  in short
\newcommand\mset[1]{\methsset{#1}}

\newcommand\imset[1]{\mbox{\methsset{}$_{#1}$}}
\newcommand\someofmethsset[1]{\mbox{$\mathit{#1}^{*}\mathsf{Meth}$}}
% in short
\newcommand\somset[1]{\someofmethsset{#1}}

\newcommand\iface[1]       {\mbox{$\mathit{#1}  \mathbf{IFace}$}}
\newcommand\ifacepartial[1]{\mbox{$\mathit{#1}^*\mathbf{IFace}$}}

\newcommand\methsbody[2]{\mbox{$\besemm{\mathit{#1}}^{\mathit{#2}}$}}
%  in short
\newcommand\mbody[2]{\methsbody{#1}{#2}}
\newcommand\msbody[2]{\mbox{$\besemm{\methsset{#1}}^{\mathit{#2}}$}} % the same
\newcommand\mmbody[1]{\msbody{#1}{}}



\newcommand\someofmethsiface[1]{\mbox{$\ifacepartial{#1}$}}
\newcommand\somface[1]{\someofmethsiface{#1}}

\newcommand\someofmethsbody[2]{\mbox{$\besemm{\someofmethsset{#1}}^{#2}$}}
\newcommand\sombody[2]{\someofmethsbody{#1}{#2}}

\newcommand\miface{\iface{\me}}

\newcommand\categoryname[1]{\mathbf{#1}}
\newcommand\sketchname[1]{\mathsf{#1}}

\newcommand\setcatmath{\categoryname{Sets}}
\newcommand\setskemath{\sketchname{Set}}
\newcommand\vsetcatmath{\categoryname{VarSet}}
\newcommand\bsetcatmath{\categoryname{BehSet}}
\newcommand\coalgcatmath{\categoryname{coAlg}}
\newcommand\coalgske{\sketchname{coAlg}}
\newcommand\erske{\sketchname{ER}}
\newcommand\ercat{\categoryname{ER}}
\newcommand\vsetske{\sketchname{VarSet}}
\newcommand\bsetske{\sketchname{BehSet}}

\newcommand\setcat{\mbox{$\setcatmath$}}
\renewcommand\setcat{\mbox{$\categoryname{Sets}$}}
\newcommand\gracat{\mbox{$\categoryname{Graphs}$}}
\newcommand\posetcat{\mbox{$\categoryname{Posets}$}}
\newcommand\catcat{\mbox{$\categoryname{Cats}$}}


\newcommand\vsetcat{\mbox{$\vsetcatmath$}}
\newcommand\bsetcat{\mbox{$\bsetcatmath$}}
\newcommand\coalgcat{\mbox{$\coalgcatmath$}}
\newcommand\setske{\mbox{$\setskemath$}}


\newcommand\univcat{\mbox{$\categoryname{U}$}}
\newcommand\ucatmath{\categoryname{U}}
\newcommand\univske{\mbox{$\sketchname{U}$}}
\newcommand\uskemath{\sketchname{U}}
\newcommand\ucat{\univcat}
\newcommand\uske{\univske}

\newcommand\instus[2]{\inst{\ske{#1}}{\ucatmath_{#2}}}
\newcommand\uni[1]{\mbox{$\univcat_{#1} $}}

\newcommand\reuniv{\univcat}
\newcommand\mapcatmath{\categoryname{Map}}
\newcommand\mapcat{\categoryname{Map}}
\newcommand\Map[2]{\mbox{$\mapcatmath(#1,#2)$}}
\newcommand\cariface{\iface{\car}}

\newcommand\rePlug{\ittt{rePlug}}
%=====================
%\input{../../Tools/Macros/m01-macroLogic.tex}

%=====================
%\input{../../Tools/Macros/m05-myStyle(razdels).tex}
\newtheorem{mydef}{\noindent Definition}
%\newtheorem{remark}{Remark}
\newtheorem{termin}{\noindent Terminology}

%% ===========================================================
%%the version where razdels are inside subsections not sections
%\newcounter{Razdel}[subsection]
%\newcommand\beginRazd[1]%
%{
%\renewcommand\theRazdel{\thesubsection.\arabic{Razdel}}
%\par%\smallskip
%\noindent\refstepcounter{Razdel}%
%{\bf \thesubsection.\arabic{Razdel} #1} %\mylabel{#2}
%}
%%==========================================================

%% =========================================================
%%the version where razdels are inside sections not subsections
%\newcounter{RazDel}[section]
%\newcommand\beginRazD[1]%  2nd argument is dummy and inherited from old verion
%{
%\renewcommand\theRazDel{\thesection.\arabic{RazDel}}
%\par%\smallskip
%\noindent\refstepcounter{RazDel}%
%{\bf \thesection.\arabic{RazDel} #1} %\mylabel{#2}
%}
%%==============================================================
%
%%\newcommand\EndRazD{\qquad\qquad\mbox{$\diamondsuit$}\par\medskip}
%%\newcommand\EndRazd{\qquad\qquad\mbox{$\diamondsuit$}\par\medskip}
%
%\newcommand\EndRazD{\par\smallskip}
%\newcommand\EndRazd{\par\smallskip}
%%\renewcommand\EndRazD{\mbox{\textbf{endRemark} $\blacktriangleright$}\par\smallskip}
%%\renewcommand\EndRazd{\mbox{\textbf{endRemark} $\blacktriangleright$}\par\smallskip}
%\newcommand\remends{\par\smallskip}
%                   %{\mbox{\textbf{endRemark} $\blacktriangleright$}}
%
%
%\newenvironment{razdel}[2]{\beginRazd{#1}{Razd#2}}{\endRazd}
%\newenvironment{razd}[2]{\beginRazd{{%\itshape
%                                      \bfseries #1}}}{\EndRazd}
%%\newenvironment{razD}[2]{\beginRazD{#1}{RazD#2}}{\EndRazD}
%\newenvironment{razD}[2]{\beginRazD{{%\itshape
%                                      \bfseries #1}}}{\EndRazD}
%\newenvironment{razzD}[1]{\beginRazD{{%\itshape
%                                      \bfseries #1}}}{\EndRazD}
%
%% 1st argument is the title of the razdel,
%% 2nd - dummy, formerly it was for the label
%
%
%\newenvironment{defi}[1]{\beginRazdel{Definition.}  {Defi#1}}{\endRazdel}
%\newenvironment{cons}[1]{\beginRazdel{Construction.}{Cons#1}}{\endRazdel}
%\newenvironment{prop}[1]{\beginRazdel{Proposition.} {Prop#1}}{\endRazdel}
%\newenvironment{theo}[1]{\beginRazdel{Theorem.}     {Theo#1}}{\endRazdel}
%\newenvironment{coro}[1]{\beginRazdel{Corollary.}   {Coro#1}}{\endRazdel}
%\newenvironment{exam}[1]{\beginRazdel{Example.}     {Exam#1}}{\endRazdel}
%%\newenvironment{rema}[1]{\beginRazdel{Remark.}      {Rema#1}}{\endRazdel}
%\newenvironment{warn}[1]{\beginRazdel{Warning.}     {Warn#1}}{\endRazdel}
%\newenvironment{desc}[1]{\beginRazdel{Description.} {Desc#1}}{\endRazdel}
%\newenvironment{disc}[1]{\beginRazdel{Discussion.}  {Disc#1}}{\endRazdel}
%\newenvironment{conv}[1]{\beginRazdel{Convention.}  {Conv#1}}{\endRazdel}
%\newenvironment{nota}[1]{\beginRazdel{Notation.}    {Nota#1}}{\endRazdel}
%
%\newcommand\equnref[1]{Equation~(\ref{Equn#1})}
%\newcommand\equlref[1]{equality~(\ref{Equl#1})}
%%\newcommand\diagref[1]{(\ref{#1})}
%\newcommand\consref[1]{Construction~\ref{Cons#1}}
%\newcommand\defref[1]{Definition~\ref{#1}}
%\newcommand\propref[1]{Proposition~\ref{Prop#1}}
%\newcommand\discref[1]{Discussion~\ref{Disc#1}}
%\newcommand\convref[1]{Convention~\ref{Conv#1}}
%\newcommand\notaref[1]{Notation~\ref{Nota#1}}
%\newcommand\descref[1]{Description~\ref{Desc#1}}
%\newcommand\remaref[1]{Remark~\ref{Rema#1}}
%\newcommand\examref[1]{Example~\ref{Exam#1}}
%\newcommand\cororef[1]{Corollary~\ref{Coro#1}}
%\newcommand\razdref[1]{Section~\ref{Razd#1}}
%%\newcommand\appref[1]{appendix~\ref{App#1}}    see pre_gen.tex
%%\newcommand\sectref[1]{section~\ref{Sect#1}}   ....
%%\newcommand\sectsectref[1]{sections~\ref{Razd#1}}
%%\newcounter{Razdel}[subsection]
%\newcommand\NachRazd[2]%
%{
%%\renewcommand\theRazdel{\thesubsection.\arabic{Razdel}}
%\par\medskip\noindent%\refstepcounter{Razdel}%
%{\it #1} \mylabel{#2} }
%%\newcommand\end{\qquad\qquad\mbox{$\diamondsuit$}\par\medskip}
%
%\newenvironment{Example}{\NachRazd{Example}}{\end}
%\newenvironment{Remark} {\NachRazd{Remark}}{\end}
%\newenvironment{Warning}{\NachRazd{Warning}}{\end}
%=====================
%\input{../../Tools/Macros/m10-MMt-CASCON-Macros.tex}
\newcommand\instarr[1]{\mbox{$\lar{\statemap}{\igra{}{}}{#1}$}}
\newcommand\instarrt[1]{\mbox{$ \lar{\statemap}{\igraph{t}{}}{#1}$}}

\newcommand\idop{\mrksemiop{\times id}}
\newcommand\idos{\mrksemiop{+id}}

\newcommand\idoP{\mrkop{prod}}
\newcommand\idoS{\mrkop{sum}}

\newcommand\recop{\mrkop{rec}}
\newcommand\varop{\mrkop{var}}
%\newcommand\sumop{\mrkop{var}}

\renewcommand\owner{\textit{owner}}
\newcommand\types{\nicex{ T$}}

%% for Kleisly arrows section

\newcommand\ssma{\mbox{$S$}}
\newcommand\tsma{\mbox{$T$}}
\newcommand\usma{\mbox{$U$$$}}
\newcommand\mapelement{\mbox{$\rightsquigarrow$}}
\newcommand\mapel{\mapelement}

\newcommand\klear[3]{\mbox{$#1\!: #2 \rightsquigarrow #3$}}
\newcommand\kleare[2]{\mbox{$#1 \rightsquigarrow #2$}}
\newcommand\lare[2]{\mbox{$#1 \rightarrow #2$}}
%==============================================

\newcommand\corrce{correspondence}






%%% 1. Collections
%
%==1.1 Categories
% macros for names moved to macros4names.tex
%\newcommand\catname[1]{\mbox{\bfseries\itshape #1}}
%%\newcommand\catname[1]{\mbox{\boldmath $#1$}}
%\newcommand\cat[1]{\catname{#1}}
%\newcommand\categoryop[1]{\mbox{\bfseries\itshape #1}$^{\mathrm{op}}$}
%\newcommand\catnamei[1]{{\pmb #1}}



%\newcommand\idmap[1]{\operator{id}_{#1}}
%\renewcommand\f{\mbox{$\phi$}}
%\renewcommand\c{\catname{C}}
%\renewcommand\b{\catname{B}}
%\renewcommand\r{\catname{R}}





\newcommand\clonet{\mbox{${\nia}_\mathrm{Top}$}}
\newcommand\clonem{\mbox{${\nia}_\mathrm{MMt}$}}
%
% -- overlined letters for clones ---
%\newcommand\clonet{\mbox{$\overline{\nia}_\mathrm{Top}$}}
%\newcommand\clonem{\mbox{$\overline{\nia}_\mathrm{MMt}$}}



%==1.2 Classes of nodes/arrows
\newcommand\indclassofitems[1]{{\cal #1}}
\newcommand\classofitems[1]{\mbox{$\indclassofitems{#1}$}}
\newcommand\coi[1]{\classofitems{#1}}
\newcommand\incls{\coi{I}}
\newcommand\covers{\coi{C}}
\newcommand\univs{\coi{U}}
%\renewcommand\diags{\classofitems{D}}
\renewcommand\diags{\mathit{Diags}}
\newcommand\inddiags{\indclassofitems{D}}

%\newcommand\attrset[1]{\mbox{\textit{attrs}$(#1)$}}
%\newcommand\refset[1]{\mbox{\textit{refs}$(#1)$}}
%\newcommand\varset[1]{\mbox{\textit{vars}$(#1)$}}
%\newcommand\classtab[1]{\mbox{\textsf{tab}$_#1$}}
%\newcommand\attrtab[1]{\mbox{\textsf{aTab}$_#1$}}
%\newcommand\reftab[1]{\mbox{\textsf{rTab}$_#1$}}



%===1.3 Languages
\newcommand\querylanguage[1]{\nicex{ QL_{#1}$}}
\newcommand\ql{\querylanguage}
\newcommand\qlmath[1]{{\cal QL}_{#1}}

%%% 2. MMt Objects
\renewcommand\modelob[1]{\mbox{$M_{#1}$}}
\newcommand\schemaobsymbol{S}
\newcommand\typeSyssymbol{Types}
\newcommand\instanceGraphSymbol{I}
\newcommand\relschemaobsymbol{R}
\newcommand\skeobsymbol{S}
\newcommand\universesymbol{U}
\newcommand\valueUniverseGraphSymbol{U}
\newcommand\UniverseGraphSymbol{U}
\newcommand\schemaob[1]{\mbox{${\mathit \schemaobsymbol}_{#1}$}}
%\newcommand\typesys[1]{\mbox{${\mathit \schemaobsymbol}_{#1}$}}
\newcommand\instgra[2]{\mbox{${\mathit \instanceGraphSymbol}_{#1}^{#2}$}}
\newcommand\igra[2]{\instgra{#1}{#2}}
\newcommand\itogra[1]{\instgra{}{#1}}
\newcommand\irefgra[1]{\instgra{ref}{#1}}
\newcommand\iattgra[1]{\instgra{attr}{#1}}
\newcommand\iobjgra[1]{\instgra{obj}{#1}}

\newcommand\uvalgra[1]{\mbox{$\mathit{\universesymbol Val}_{#1}$}}
\newcommand\utupgra[1]{\mbox{$\mathit{\universesymbol Tuple}_{#1}$}}
\newcommand\uval{\uvalgra{}}
\newcommand\utup{\utupgra{}}
\renewcommand\uniob[1]{\mbox{$\mathsf{\universesymbol}_{#1}$}}

\newcommand\relsob[1]{\mbox{${\mathit \relschemaobsymbol}_{#1}$}}
\newcommand\newrelske[1] {\mbox{${\mathsf R}_{#1}$}}
\newcommand\newrelinst[2]{\mbox{${\mathsf Q}_{#1}^{#2}$}}

\newcommand\schemaOB[2]{\mbox{${\mathit \schemaobsymbol}_{#1}^{#2}$}}

\newcommand\claske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{cla}#1}$}}
\newcommand\refske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{ref}#1}$}}
\newcommand\attrske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{attr}#1}$}}
\newcommand\objrefske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{objRef}#1}$}}


\renewcommand\skeob[1]{\mbox{${\mathsf\skeobsymbol}_{#1}$}}
\newcommand\skeobind[1]{{\mathsf \skeobsymbol}_{#1}}
\newcommand\indskeob[1]{\skeobind{#1}}

\newcommand\typeske[1]{\mbox{$\mathsf{Type}_{#1}$}}
\newcommand\typemap[1]{\mbox{$\mathsf{type}_{#1}$}}
\newcommand\typeskeind{\mathsf{Type}}
\newcommand\typemapind[1]{\mathsf{type}_{#1}}

\renewcommand\statemap{\mbox{$\sigma$}}
\newcommand\statemapind{\sigma}




%\newcommand\gs{\mbox{$G_{\indskeob{}}$}}
%\newcommand\ds{\mbox{$\diags_{\indskeob{}}$}}
%\newcommand\gsi[1]{\mbox{$G_{\indskeob{#1}}$}}
%\newcommand\dsi[1]{\mbox{$\G_{\indskeob{#1}}$}}

%%% 2.1  Vectors of objects (bold objects)
%\newcommand\fullvector[3]{}
%\newcommand\vectorobject[1]{\mbox{$\boldsymbol{#1}$}} % see macros4names
\newcommand\multisch{\vectorobject{\schemaobsymbol}}
\newcommand\multiSch{\vectorobject{\schemaobsymbol}}
\newcommand\multinst{\vectorobject{\instancesymbol}}
\newcommand\multinstoo[1]{\mbox{$\multinst=(\inst{1},\ldots,\inst{#1})$}}

\newcommand\multiUni{\vectorobject{\universesymbol}}
\newcommand\multiRel{\vectorobject{\relschemaobsymbol}}
\newcommand\multiuni{\vectorobject{u}}
\newcommand\multirel{\vectorobject{r}}
\newcommand\multiu{\vectorobject{u}}
\newcommand\multir{\vectorobject{r}}
\newcommand\multiroo[1]{\mbox{$\multir=(r_1,\ldots,r_{#1})$}}


%== Operators
\newcommand\operator[1]{\mbox{\sf #1}}
\newcommand\operatorInIndex[1]{{\sf #1}}

\newcommand\heoperator[1]{\mbox{\sf\bfseries #1}}
\newcommand\match{\operator{match}}

\newcommand\indexedoperator[3]{\mbox{\operator{#1}$_{#2}^{#3}$}}
\newcommand\indexedoperatorInIndex[3]{\operatorInIndex{#1}_{#2}^{#3}}

\newcommand\der[2]{\indexedoperator{der}{#1}{#2}}
\newcommand\dero[1]{\indexedoperator{der}{}{#1}}
\newcommand\derInIndex[2]{\indexedoperatorInIndex{der}{#1}{#2}}

%\newcommand\proj[1]{\indexedoperator{p}{#1}{}}
%\newcommand\merge{\operator{merge}}
%\newcommand\modgen{\operator{modelGen}}
%\newcommand\datatrans{\operator{dataTransf}}
%\renewcommand\self{\operator{self}}


\newcommand\SFW[3]{\mbox{\operator{Select} #1
                         \operator{from} #2
                         \operator{where} #3}
                         }

%=====================
%\input{../../Tools/Macros/m20-newMacros}
%\renewcommand\em[1]{\emph{#1}}

%\newcommand\vect[1]{\textbf{#1}}
\newcommand\veg{\vect{G}}
\newcommand\vef{\vect{f}}
\newcommand\ver{\vect{R}}
\newcommand\ves{\vect{S}}
\newcommand\vehh{\vect{H}}
\newcommand\veho{\vect{\ovr{H}}}
\newcommand\veh{\vect{h}}

\newcommand\ovr[1]{\mbox{$\overline{\mathstrut#1}$}}
\newcommand\ovri[1]{\overline{#1}}
\newcommand\ovh[1]{\ovr{H}_{#1}}
%\newcommand\ovri[1]{\mb{\ovr{\iota'}_{#1}}}

\newcommand\edge[1]{\ittt{Edge}\mb{_{#1}}}
\newcommand\Edge[2]{\ittt{Edge}\mb{_{#1}^{#2}}}


\newcommand\univarr[1]{\mb{!_{#1}}}
\newcommand\doublearrow[5]{\mbox{$#1\stackrel{#4}{\rightarrow}
                                 #2\stackrel{#5}{\rightarrow}#3$
}}
\newcommand\arrdou[5]{\doublearrow{#1}{#2}{#3}{#4}{#5}}
\newcommand\arrarr{\arrdou{\gra{2}}{\gra{3}}{\gra{4}}{h_2}{h_3}}
\newcommand\scearr{\arrdou{\gra{2}}{\gra{1}}{\gra{0}}{\tau_1}{\tau_0}}
\newcommand\arrsce{\arrdou{\gra{2}}{\gra{1}}{\gra{0}}{\tau_1}{\tau_0}} % the same as above

\newcommand\arrspan[5]{\fbox{$#1\stackrel{#4}{\leftarrow}
                                 #2\stackrel{#5}{\rightarrow}#3$
}}
\newcommand\arrcospan[5]{\fbox{$#1\stackrel{#4}{\rightarrow}
                                 #2\stackrel{#5}{\leftarrow}#3$
}}

%\renewcommand\span[1]{\textbf{R}\mb{_{#1}}}
\newcommand\cospan[1]{\textbf{S}\mb{_{#1}}}
\newcommand\set[2]{\mb{#1=\{#2\}}}

\newcommand\integr[3]{\mb{#1\bigoplus_#3 #2}}

\newcommand\gran[1]{\mb{G_{{#1}N}}}
\newcommand\gred[1]{\mb{G_{{#1}E}}}
\newcommand\graman[1]{\mb{f_{{#1}N}}}
\newcommand\gramed[1]{\mb{f_{{#1}E}}}
\newcommand\grinman[1]{\mb{\iota'_{{#1}N}}}
\newcommand\grinmed[1]{\mb{\iota'_{{#1}E}}}

% changing from \mathsl to \mathit
\renewcommand\object[2]{\mbox{${\mathit{#1}}_{#2}$}}
\renewcommand\objectind[1]{\mathit{#1}}
\renewcommand\objectmath[1]{\mathit{#1}}

%\newcommand\DOM[1]{\Box #1}
%\newcommand\COD[1]{#1 \Box}


\newcommand\mb[1]{\mbox{$#1$}}
\newcommand\nin{\mb{\cal N}}
\newcommand\nix{\mb{\cal X}}
\newcommand\nil{\mb{\cal L}}
\newcommand\nik{\mb{\cal K}}
\newcommand\dvet{\mbox{:}}
\newcommand\ddvet{\dvet\dvet}
%\newcommand\n{\mb{n}}

\renewcommand\x{\mb{X}}

\newcommand\proxx[2]{\mb{\prod_{#1}{#2}}}
\newcommand\prox{\proxx{}{\vex}}
\newcommand\proy{\proxx{}{\vey}}
\newcommand\prodxn{\proxx{\cal L}{\vex}}
\newcommand\prodxm{\proxx{\cal K}{\vex}}

\newcommand\unixx[2]{\mb{\bigcup_{#1}{#2}}}
\newcommand\unix{\unixx{}{\vex}}

\newcommand\proj[1]{\mb{\ell_{#1}}}
\newcommand\proji{\proj{i}}






\renewcommand\ext{\mbox{\textsf{ext}}}








\newcommand\oclar{\mbox{\footnotesize $>$}}
\newcommand\myendset[1]{\mbox{$\{#1_1..#1_m\}$}}
\newcommand\fens{\myendset{f}}





\newcommand\fulla[1]{\mbox{${\mathbf F}_{#1}$}}
\newcommand\rmap[1]{\mbox{$#1^\rightarrow$}}
\newcommand\lmap[1]{\mbox{$^\leftarrow #1$}}
\newcommand\basemap[1]{\mbox{\textit{base}$_{#1}$}}


\newcommand\seq[1]{\textsf{seq}\mbox{$#1$}}
\newcommand\coll[2]{\textsf{coll}\mbox{$_{#1}(#2)$}}

\newcommand\tabschema{\mbox{$D=\{a_1:D_1,...,a_n:D_n\}$}}
\newcommand\tabschemamap{\mbox{\lar{D}{\attrset{}}{\setcat}}}



%=====================
%\input{../../Tools/Macros/m21--labelsnewMacros}
%(left) labels for formulas
\newcommand\equationNumber[1]{(\textsf{#1})}
\newcommand\eqnumber[1]{\equationNumber{#1}}
\newcommand\eqn[1]{\equationNumber{#1}}


%\newcommand\mafo[2]\mathform{#1}{#2}
\newcommand\mathfo[2]{$$#2\leqno{\mbox{(\textsf{#1})}} $$}
\newcommand\mafo[2]{$$#2 \leqno{\mbox{\eqn{#1}}} $$}


\newcommand\selflab{\eqn{self}}
\newcommand\looplab{\eqn{loop}}
\newcommand\idlelab{\eqn{idle}}
\newcommand\dolab{\eqn{do}}
\newcommand\triglab{\eqn{trigger}}

\newcommand\assonla{\eqn{fullAsson}}
\newcommand\tabla{\eqn{TAB}}
\newcommand\invla{\eqn{inverse}}
\newcommand\extla{\eqn{extension}}
\newcommand\tablatup{\eqn{TABrow}}
\newcommand\tablapro{\eqn{TABattr}}
\newcommand\sepla{\eqn{1-1}}
%=====================================
\newcommand\classn{\eqnumber{classn}}
\newcommand\indexn{\eqnumber{indexng}}

\newcommand\igralabel{\eqnumber{instGra}}
\newcommand\schemaGeneralLabel{\eqnumber{schemaGen}}
\newcommand\stlabel{\schemaGeneralLabel}
\newcommand\itablabel{\eqnumber{instTab}}
%\renewcommand\uniob[1]{\mbox{${\mathsf\universesymbol}_{#1}$}}
\newcommand\igratablabel{\eqnumber{instGraTab}}
\newcommand\igragralabel{\eqnumber{instGraGra}}
\newcommand\itabtablabel{\eqnumber{instTabTab}}

%=====================
%\input{../Tools/Macros/m21--abbrev4formulas}
%\input{../Tools/Macros/m22--abbrev4text}
%--------------------------------
%\renewcommand\zdmargin[1]{}
%\renewenvironment{razd}[2]{\subsubsection{#1}}{}
%\nocite{}
\renewenvironment{razD}[2]{\beginRazD{{%\itshape
                                      \bfseries #1}}}{\EndRazD}

%% sle
%%%%%%%%%% sle09 macros
%\newcommand\diagi[1]{#1\mbox{$'$}}
%\newcommand\diagii[1]{#1\mbox{$''$}}
%
%\newcommand\ari[1]{\mbox{\textsl{ar}$(#1)$}}
%\newcommand\mmname[1]{\textsf{#1}}
%\newcommand\mmcd{\mmname{CD}}
%\newcommand\mmsd{\mmname{SD}}
%\newcommand\mmsc{\mmname{SC}}
%\newcommand\mmca{\mmname{CA}}
%\newcommand\mmamt{\mmname{CAT}}
%\newcommand\mmcat{\mmname{CAT}}
%\newcommand\cd{\mmname{cd}}
%\renewcommand\sd{\mmname{sd}}
%\renewcommand\sc{\mmname{sc}}
%\newcommand\ca{\mmname{ca}}
%\newcommand\amt{\mmname{cat}}
%\renewcommand\cat{\mmname{cat}}
%\newcommand\cdi{\diagi{\cd}}
%\renewcommand\sdi{\diagi{\sd}}
%\newcommand\sci{\diagi{\sc}}
%\newcommand\cdii{\diagii{\cd}}
%\newcommand\sdii{\diagii{\sd}}
%\newcommand\scii{\diagii{\sc}}





\newcommand\base{\mbox{$\pmb{MM}$}}
\newcommand\p{\textbf{P}}
\newcommand\ps{\mbox{$P$}}
\newcommand\leqnoo[1]{\leqno{\mbox{#1}}}

\newcommand\keyword[1]{{\itshape\textsf{#1}}}
\newcommand\nam{\keyword{name}}
\renewcommand\owner{\keyword{owner}}
\newcommand\type{\keyword{type}}
\newcommand\val{\keyword{value}}
\newcommand\Class{\keyword{Class}}
\renewcommand\Attr{\keyword{Attr}}
\newcommand\Type{\keyword{Type}}
\newcommand\elm[1]{\mbox{$\mathit{El}(#1)$}}

\newcommand\ueq{\mbox{$\leftrightarrow$}}
\newcommand\uneq{\mbox{$\rightsquigarrow$}}

\newcommand\meq{\mbox{$=$}}
\newcommand\mneq{\mbox{$\neq$}}


\newcommand\shot{\textsl{shot}}
\newcommand\reltile{\textsl{relTile}}
%\newcommand\tauh{\mbox{$\tau_{\textsf{h}}$}}
%\newcommand\tauv{\mbox{$\tau_{\textsf{v}}$}}



\newcommand\vso{\textsf{v}\mbox{$\partial_0$}}
\newcommand\vta{\textsf{v}\mbox{$\partial_1$}}
\newcommand\hso{\textsf{h}\mbox{$\partial_0$}}
\newcommand\hta{\textsf{h}\mbox{$\partial_1$}}

\newcommand\mmod{\nicex{ M$}}
\newcommand\id{\textsl{id}}
\renewcommand\id{\mbox{$\iota$}}
\newcommand\recon[1]{\mbox{$#1$\textbf{!}}}

\newcommand\oidd[1]{\mbox{$\overline{#1}$}}
\newcommand\oiddi[1]{\mbox{$\overline{#1}'$}}

\renewcommand\oidd[1]{\mbox{${#1}$}}
\renewcommand\oiddi[1]{\mbox{${#1}'$}}

\newcommand\oa{\oidd{a}}
\newcommand\ob{\oidd{b}}
\newcommand\oP{\oidd{P}}
\newcommand\oQ{\oidd{Q}}

\newcommand\oai{\oiddi{a}}
\newcommand\obi{\oiddi{b}}
\newcommand\oPi{\oiddi{P}}
\newcommand\oQi{\oiddi{Q}}

% icmt

%%% icmt09 macros
% the % piece below  was moved to newMacros ---
\newcommand\mrkoprr[1]{\mrkopr{\mrkopr{#1}}}
%\der{}{Q}
%\newcommand\mmview[1]{\mbox{$\textsl{v}_{#1}$}}
%\newcommand\mmarr{v}
\newcommand\mmf{\mbox{$m$}} % to be used in the row
%\renewcommand\mmview[1]{\mbox{$\pmb{\mmarr}_{#1}$}}
%%\newcommand\mmv[1]{{\pmb{\mmarr}_{#1}}} %for subscripts
%\newcommand\mmmap[1]{\mbox{$\pmb{\mmarr}_{#1}$}}
%\renewcommand\mmm{m}  % to be used for sub-sup-indexes
%\newcommand\mmap[1]{\mbox{${\mmarr}_{#1}$}}

\newcommand\unde[1]{\underline{#1}}

\newcommand\oversi[1]{\overline{\sigma}^{#1}}

\newcommand\oversig[1]{\overline{\sigma}^{Q#1}}
\newcommand\overtau[1]{\overline{\tau}^{Q#1}}
\newcommand\overover{\overline{\oversig{1}}}
\newcommand\doublesig{{\overover^{Q2}}} %
\newcommand\votono{{\overline{\oversig{}}^{R}}}

\newcommand\derqq[2]{\mbox{$\dero{Q#1}#2$}}
\newcommand\dermms[1]{\derqq{#1}{\mms}}
\newcommand\derms[1]{\derqq{#1}{\ms{}}}
\newcommand\derqmms{\derqq{}{\mms}}
\newcommand\derqms{\derqq{}{\ms{}}}
\newcommand\derq[1]{\mbox{$\der{}{Q}#1$}}
\newcommand\doubleder[1]{\derqq{1;Q2}{#1}}

\newcommand\augtymaps{\flar%
{\overline{\sigma}^{Q}}%
{\dero{Q}\ms{}}%
{\dero{Q}\mms}%
}
%\newcommand\mmarr{\mbox{$m$}}

%
\newcommand\tracemap[1]{\mbox{$\stackrel{\rightsquigarrow}{#1}$}}
\renewcommand\tracemap[1]{\mbox{$\mathit{tr}_{#1}$}}
\renewcommand\tracemap[1]{\mbox{$#1^{*}$}}
\newcommand\tram{\tracemap{\mmmap}}
%
\newcommand\reversemap[1]{\mbox{\spf$_{#1}$}}
%\newcommand\revem{\reversemap{\mmview{}}}
\newcommand\revem[1]{\mbox{$\semm{\mmmap{#1}}$}}

\renewcommand\s[1]{\mbox{$S_{#1}$}}
\renewcommand\ms[1]{\mbox{$S_{#1}$}}
\newcommand\mos[1]{\mbox{$\overline{S}_{#1}$}}
\renewcommand\mt[1]{\mbox{$T_{#1}$}}
\newcommand\mot[1]{\mbox{$\overline{T}_{#1}$}}
\newcommand\mh[1]{\mbox{$H_{#1}$}}
\renewcommand\ml[1]{\mbox{$L_{#1}$}}

\newcommand\pbop{\operator{PB}}

\newcommand\msarr{\flar{\sigma}{S}{\mms}}
\newcommand\msarrq{\flar{\overline{\sigma}^{Q}}{\der{}{Q}S}{\der{}{Q}\mms}}
\newcommand\mssym{\mbox{$\overline{\sigma}$}}
\newcommand\mssymq{\mbox{$\overline{\sigma}^Q$}}

\newcommand\mtarr{\flar{\tau}{T}{\mmt}}
\newcommand\srelarr{\flar{\sigma}{S}{\mmrel}}
\newcommand\erdarr{\flar{\tau}{D}{\mmer}}
\newcommand\srelderarr[1]{\flar{\overline{\sigma}^{Q#1}}{\der{}{Q#1}S}{\der{}{Q#1}\mmrel}}



\newcommand\ertorel[1]{\flar{\textsf{er2rel}_{#1}}{\mmer}{\mmrel}}
\newcommand\ertorelder[1]{\flar{\textsf{er2rel}_{#1}}{\mmer}{\der{}{{Q#1}}\mmrel}}

% gttse

%\renewcommand\mmname[1]{\mbox{$\pmb{\cal #1}$}}
%\newcommand\mmmapname[1]{\mbox{$\pmb{#1}$}}
%\newcommand\mma{\mmname{M}}
%\newcommand\mmb{\mmname{N}}
%\newcommand\mmc{\mmname{O}}
%\newcommand\mmr[1]{\mbox{\mmname{R}$_{#1}$}}
%\renewcommand\mmr[1]{\mbox{$\pmb{r}_{#1}$}}
%\newcommand\mmab{\mmname{MN}}
%\newcommand\mmac{\mmname{MO}}
%\newcommand\mmv{\mmmapname{v}}
%\newcommand\mmw{\mmmapname{w}}
%\newcommand\mmp{\mmmapname{p}}
%\newcommand\mmq{\mmmapname{q}}

\renewcommand\dvet{\mbox{:\,}}

\newcommand\newrevem[1]{\mbox{$\semm{\mmmapname{#1}}$}}
\newcommand\rev{\newrevem{v}}
\newcommand\rew{\newrevem{w}}
\newcommand\rep{\newrevem{p}}
\newcommand\req{\newrevem{q}}


\newcommand\mmnamei[1]{\pmb{\cal #1}}
\newcommand\mmabi{\mmnamei{MN}}
\newcommand\mmaci{\mmnamei{MO}}
\newcommand\amn{\mbox{$A_{\mmabi}$}}
\newcommand\bmn{\mbox{$B_{\mmabi}$}}
\newcommand\amnprim{\mbox{$A'_{\mmabi}$}}
\newcommand\bmnprim{\mbox{$B'_{\mmabi}$}}
\newcommand\amo{\mbox{$A_{\mmaci}$}}
\newcommand\cmo{\mbox{$C_{\mmaci}$}}
\newcommand\umn{\mbox{$u_{\mmabi}$}}
\newcommand\vmn{\mbox{$v_{\mmabi}$}}

\newcommand\lmmes{\left] \respace\left] }
\newcommand\rmmes{\right[\respace\right[}
\newcommand\mmes[1]{\mbox{$\lmmes\, \mathit{#1} \, \rmmes$}}

% spans

\newcommand\spancat{\category{Span}}
\newcommand\spansa{\scat\spancat}
\newcommand\spanset{\setcat\spancat}
\newcommand\cospancat{\category{Cospan}}
\newcommand\cospansa{\scat\cospancat}
\newcommand\cospanset{\setcat\cospancat}


\newcommand\spanfull[4]{\mbox{${\cal #1}$=(\flar{#2_i}{#3}{#4 i},
$i=1,2)$}}

\newcommand\lKleisly{\Leftarrow}
\newcommand\rKleisly{\Rightarrow}
\newcommand\spandiag[5]  {\fbox{$#1\lTo^{#2} #3 \rTo^{#4} #5$}}
\newcommand\kleispandiag[5]{\fbox{$#1\lKleisly^{#2} #3 \rKleisly^{#4} #5$}}
\newcommand\kleislispandiag[5]{\fbox{$#1\lKleisly^{#2} #3 \rKleisly^{#4} #5$}}
\newcommand\cospandiag[5]{\fbox{$#1\rTo^{#2} #3 \lTo^{#4} #5$}}
\newcommand\kleicospandiag[5]{\fbox{$#1\rKleisly^{#2} #3 \lKleisly^{#4} #5$}}
\newcommand\kleislicospandiag[5]{\fbox{$#1\rKleisly^{#2} #3 \lKleisly^{#4} #5$}}


\newcommand\flarsemm[3]{\flar{#1}{\semm{#2}}{\semm{#3}}}
\newcommand\spandiagsemm[5]{\fbox{$\semm{#1}\lTo^{#2} \semm{#3} \rTo^{#4} \semm{#5}$}}
\newcommand\cospandiagsemm[5]{\fbox{$\semm{#1}\rTo^{#2} \semm{#3} \lTo^{#4} \semm{#5}$}}


%=== with brackets
\newcommand\spandiagbra[5]
{\mbox{$%\left %
(#1\stackrel{~#2}{\leftarrow} #3
                                           \stackrel{#4~}{\rightarrow} #5%\right
)$}}
\renewcommand\kleispandiag[5]{\mbox{$\left(#1\stackrel{~#2}{\lKleisly} #3
                                             \stackrel{#4~}{\rKleisly} #5
                                             \right)$}}
\renewcommand\kleislispandiag[5]{\mbox{$\left(#1\stackrel{#2}{\lKleisly} #3
                                             \stackrel{#4}{\rKleisly} #5
                                             \right)$}}
\renewcommand\kleicospandiag[5]{\mbox{$\left(#1\stackrel{#2}{\rKleisly} #3
                                             \stackrel{#4}{\lKleisly} #5
                                             \right)$}}
\renewcommand\kleislicospandiag[5]{\mbox{$\left(#1\stackrel{#2}{\rKleisly} #3
                                             \stackrel{#4}{\lKleisly} #5
                                             \right)$}}

\renewcommand\cospandiag[5]{\mbox{$\left(#1\rTo^{#2} #3 \lTo^{#4} #5\right)$}}
\renewcommand\cospandiag[5]  {\mbox{$\left(#1\stackrel{~#2}{\rightarrow} #3
                                           \stackrel{#4~}{\leftarrow} #5\right)$}}

% without brackets
\renewcommand\spandiag[5]  {\mbox{$#1\stackrel{~#2}{\leftarrow} #3
                                           \stackrel{#4~}{\rightarrow} #5$}}
\renewcommand\cospandiag[5]  {\mbox{$#1\stackrel{~#2}{\rightarrow} #3
                                           \stackrel{#4~}{\leftarrow} #5$}}


%\renewcommand\kleislycospandiag[5]{\mbox{$\left(#1\rKleisly^{#2} #3 \lKleisly^{#4} #5\right)$}}

\renewcommand\flarsemm[3]{\flar{#1}{\semm{#2}}{\semm{#3}}}
\renewcommand\spandiagsemm[5]{\mbox{$\left(\semm{#1}\lTo^{#2} \semm{#3}\rTo^{#4} \semm{#5}\right)$}}
\renewcommand\cospandiagsemm[5]{\mbox{$\left(\semm{#1}\rTo^{#2} \semm{#3}\lTo^{#4} \semm{#5}\right)$}}


%% end macros



%%==== end newMacros


==> macros/macros4diagArrows.tex <==
\usepackage{diagrams}
%\diagramstyle[PostScript=dvips] % to print inclined arrows properly

%%%%%%%%%%%%%%%%%%
% some useful arrow segments missed by Taylor
%%%%%%%%%%%%%%%%%%
\newarrowhead{bt}\blacktriangleright\blacktriangleright\blacktriangleright\blacktriangleright
\newarrowtail{bt}\blacktriangleleft\blacktriangleleft\blacktriangleleft\blacktriangleleft
\newarrowmiddle{bar}\rtbar\ltbar\dtbar\utbar
\newarrowmiddle{|}\vert\vert--
\newarrowmiddle{||}\Vert\Vert==
\newarrowmiddle{=}==\Vert\Vert
\newarrowtail{=}==\Vert\Vert
\newarrowhead{l}\langle\langle\langle\langle %\Vert\Vert
\newarrowhead{r}\rangle\rangle\rangle\rangle %\Vert\Vert
\newarrowfiller{=}==\Vert\Vert
\newarrowfiller{d}\cdot\cdot\cdot\cdot
\newarrowmiddle{x}****
\newarrowmiddle{b}\bullet\bullet\bullet\bullet
\newarrowtail{b}\bullet\bullet\bullet\bullet
\newarrowmiddle{3}\equiv\equiv\vfthree\vfthree
\newarrowfiller{3}\equiv\equiv\vfthree\vfthree
\newarrowtail{3}\equiv\equiv\vfthree\vfthree
\newarrowtail{<=}\Leftarrow\Rightarrow{\@cmex7E}{\@cmex7F}
\newarrowfiller{bold}{\bf-}{\bf-}{\bf|}{\bf|}  % no effect!
\newarrowfiller{o}{\hho}{\circ}{\circ}{\circ}  % is \circ == hho?
\newarrowmiddle{>}\rtla\ltla\dtla\utla
%\newarrowfiller{>}\rtla\ltla\dtla\utla       it hangs the machine
\newarrowmiddle{d}\cdot\cdot\cdot\cdot

% Taylor defines only rightwise => -> ->> harpoon etc.
% If one needs the opposite (e.g. for bidirected arrows),
% copy the corresponding lines from diagrams.tex and modify them!
\newarrow{To}----{>}
\newarrow{Toang}----{->}
\newarrow{BMapsto}b---{>}
\newarrow{Mapsto}{|}---{>}
\newarrow{Mapsto}{b}---{>}
\newarrow{Dermapsto}{|}{dash}{}{dash}{>}
\newarrow{Dermapsto}{b}{dash}{}{dash}{>}
\newarrow{Dashmapsto}{b}{dash}{dash}{dash}{>}
\newarrow{Dotmapsto}{b}...{>}
\newarrow{Maps}b----
\newarrow{ID}33333

\newarrow{Dashes}{}{dash}{}{dash}{}
\newarrow{Dots}.....

\newarrow{EQ}=====
\newarrow{NRelto}--+-{->}
\newarrow{Relto}--b-{->}
\newarrow{BSpanto}--b-{->} % bulleted span arrow
\newarrow{Embed}>---{>}
\newarrow{Embed}{blacktriangle}---{>}
\newarrow{EmbedDashed}{blacktriangle}{dash}{dash}{dash}{>}
\newarrow{FEmb}{blacktriangle}---{>}
\newarrow{WEmb}{blacktriangle}---{>}
\newarrow{WEmbDot}{blacktriangle}...{>}
\newarrow{FEmbDot}{blacktriangle}...{>}
%%%%---> redef with bold heads
\newarrow{FEmb}{blacktriangle}---{blacktriangle}
\newarrow{WEmb}{blacktriangle}---{blacktriangle}
\newarrow{WEmbDot}{blacktriangle}...{blacktriangle}
\newarrow{FEmbDot}{blacktriangle}...{blacktriangle}
\newarrow{WEmbDash}{blacktriangle}{dash}{dash}{dash}{blacktriangle}
\newarrow{FEmbDash}{blacktriangle}{dash}{dash}{dash}{blacktriangle}
%=====

\newarrow{Dashto}{}{dash}{}{dash}{>} %or {->}
\newarrow{Dotto}....{>} %or {->}
% because of a bug, i need to have two diff commands
% for right and left triple arrow
\newarrow{RDiagto}3333{r}
\newarrow{RDiagderto}{}{3}{}{3}{r}
\newarrow{LDiagto}3333{l}
\newarrow{LDiagderto}{}{3}{}{3}{l}
\newarrow{Mapsderto}{b}{dash}{}{dash}{>}
\newarrow{Into}C---{>}
\newarrow{Indashto}C{dash}{}{dash}{>}
\newarrow{Derinto}C{dash}{}{dash}{>}
\newarrow{Congruent}33333
\newarrow{Cover}----{blacktriangle}
\newarrow{Monic}{>}--->
\newarrow{Isoto}{>}---{triangle}
\newarrow{ISA}===={=>}
\newarrow{Isato}===={=>}
\newarrow{Doubleto}===={=>}
\newarrow{ClassicMapsto}{|}--->
\newarrow{Entail}{|}----
\newarrow{PArrow}{o}--->
\newarrow{MArrow}----{>>}
\newarrow{MPArrow}{o}---{>>}
\newarrow{Ogogoto}oooo{->}
\newarrow{Metato}--3->
\newarrow{MetaMapto}{|}-3->
\newarrow{OneToMany}+---{o}
\newarrow{HalfDashTo}{}{dash}{}-{>>}
\newarrow{DLine}=====
\newarrow{Line}-----
\newarrow{Tline}33333
\newarrow{Dashline}{}{dash}{}{dash}{}
\newarrow{Dotline}{}{o}{}{o}{}
\newarrow{Curlyto}{curlyvee}--->           % Without AMS-TeX Only Horisontal
\newarrow{Bito}<--->
\newarrow{Bito}{<}---{>}
\newarrow{Bidito}{<}==={>}
\newarrow{Bitrito}{bt}333{bt}
\newarrow{Corrto}<--->
\newarrow{Dercorrto}{<}{dash}{}{dash}{>}
%\newarrow{Dercorrto}{<}{d}{d}{d}{>}
%\newarrow{Infer}----{|}
%\newarrow{Black}{blacktriangle}---{blacktriangle} %  AMS needed

%%%%%%%%%%%%%%%%
\newarrow{Instofto}{curlyvee}...{>}
%\newarrow{Instofto}{curlyvee}---{->}
\newarrow{Instofderto}{curlyvee}{dash}{}{dash}{->}
% update, match and view arrows in Taylor's Diags
\newarrow{Updto}----{>}
\newarrow{Derupdto}{}{dash}{}{dash}{>}
\newarrow{Mchto}----{>}
\newarrow{Dermchto}{}{dash}{}{dash}{>}
\newarrow{Viewto}----{>->}
\newarrow{Derviewto}{}{dash}{}{dash}{>>}
% better version
\newarrow{Viewto}===={=>}
\newarrow{Hetmchto}===={=>}
\newarrow{Derviewto}{=}{}{=}{}{=>}
%\newarrow{Derviewto}{}{=}{}{=}{=>}
\newarrow{Idleto}===={=>}
\newarrow{Deridleto}{=}{}{=}{}{=>}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\coverarrowhead{triangle}
%\newcommand\coverarrowhead{blacktriangle}  % needs AMS-package !!!
\newcommand\partialarrowtail{{\Large \bullet}}
\newlength{\StatArrBody}
\newlength{\NodeFrameThickness}
\setlength{\NodeFrameThickness}{1.5pt}
\setlength{\StatArrBody}{0.9\NodeFrameThickness}%{1.25pt}
%\newcommand{\tch}[2]{\begin{picture}(0,0)
%                        \put(#1,#2){\circle*{3}}
%                        \end{picture}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> macros/macros4fase17paper.tex <==
\newcommand\sameown{\textsf{sameOwn}}

\newcommand\mt{\textsc{mmt}}
\newcommand\mmt{\mt}
\newcommand\metatr{\ensuremath{T}} % {Tr_{\mathrm{def}}}}
\newcommand\modtr[1]{\ensuremath{Tr_{#1}}}
\newcommand{\emath}[1]{{\ensuremath{#1}}}
%\newcommand{\tobjnobr}[2]{\emath{\mathbf{T}^\bullet_{#1}(#2)}}

\newcommand\anmt{\ensuremath{{\mathbf T}}}

\newcommand\coveh{\ensuremath{\mathsf{Commut.Vehicle}}}
\newcommand\lveh{\ensuremath{\mathsf{LeisureVehicle}}}
\newcommand\veh{\ensuremath{\mathsf{Vehicle}}}
\newcommand\car{\textsf{Car}}
\newcommand\days{\textsc{Days}}
\newcommand\boat{\textsf{Boat}}
\newcommand\amph{\textsf{amph}}
\newcommand\cveh{\textsf{Commut}}
\newcommand\usedon{\textsf{usedOn}}
\newcommand\same{\textsf{same}}

\newlength{\figwidth}
\newlength{\onemodwid}
\newlength{\twomodwid}
\setlength{\figwidth}{0.48\textwidth} % was 0.55
\setlength{\onemodwid}{0.205\textwidth} % was 0.25
\setlength{\twomodwid}{0.295\textwidth} %was 0.325
%------
%\newcommand\mydefin[2]{\par\noindent \textbf{Definition #1 (#2).}}
%\renewcommand\mydefin[2]{\par\noindent \textbf{Definition #1.}}
%\newenvironment{\mydefin}[2]% name
%{\par\noindent \textbf{Definition #1 (#2).}}% opening macros
%{{\qed}} %closing macros


\endinput



==> macros/macros4textArrows.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Arrows in diagrams and formulas
% normal functional arrow f: X-->Y
%\newcommand\frar[3]{\ensuremath{#1{:}\;#2\rightarrow #3}}
%\newcommand\trisprar{---}%[3]{\ensuremath{#1{:}\;#2\rightarrow #3}}
%\newcommand\fprar[4]{\ensuremath{#1{:}\;#2\stackrel{#4}{\rightarrow} #3}}
%\renewcommand\fprar[4]{\ensuremath{#1{:}\;#2\rTo^{#4} #3}}
\newcommand\fprarlong[4]{\ensuremath{#1{:}\;#2\stackrel{#4}{\longrightarrow} #3}} %functional arrow
\newcommand\wrar[3]{\ensuremath{#1{:}\;#2\rightsquigarrow #3}} %wavy arrow
\newcommand\wbiar[3]{\ensuremath{#1{:}\;#2\leftrightsquigarrow #3}} %wavy arrow
\newcommand\farr[3]{\frar{#1}{#2}{#3}}% if typo occurs
%\newcommand\lar[3]{\flar{#1}{#2}{#3}}%
\newcommand\updar[3]{\frar{#1}{#2}{#3}}
%\newcommand\viewlar[4]{\mbox{$#1\!:#2\rightarrow^{#4} #3$}}
%\newcommand\flarcat[4]{\mbox{$#1\!:#2\rightarrow #3{:}{:}\,#4$}}

% variants
%-----------
%long
\newcommand\frarr[3]{\mbox{$#1\!:#2\longrightarrow #3$}} % long arrow
\renewcommand\larr[3]{\mbox{$#1\!:#2\longrightarrow #3$}} % the same
%\newcommand\lari[4]{\mbox{$#1_{i}\!:\:#2\:\longrightarrow\:#3_{i},\;i=1,\ldots,#4$}}%

%multihead
\newcommand\mlar[3]{\larlar{#1}{#2}{#3}} %multiarrow
\newcommand\larlar[3]{\mbox{$#1\!:#2\twoheadrightarrow#3$}} %needs AMS
% double body
\newcommand\drar[3]{\mbox{$#1\!:#2\Rightarrow #3$}} %double arrow
\newcommand\dlarcat[4]{\mbox{$#1\!:#2\Rightarrow #3{:}{:}\,#4$}}
\newcommand\trar[3]{\mbox{$#1\!:\,#2\Rightarrow #3$}}
% inclusions
\newcommand\inclarr[3]{\mbox{$#1\!:\:#2\:\rInto\:#3$}}       %$key=<AltShftRT>
\newcommand\inclar[3] {\mbox{$#1\!:\:#2\:\hookrightarrow\:#3$}}
\newcommand\binclar[3] {\mbox{$#1\!:\:#2\:\hookleftarrow\:#3$}}
%triple body
\newcommand\trilar[3]{\mbox{$#1\!:#2\Rrightarrow #3$}} % triple
% profunctor/span
\newcommand\spanar[3]{\mbox{$#1\!:#2\nrightarrow#3$}}
\newcommand\trispar[3]{\spanar{#1}{#2}{#3}}  %synonym
\newcommand\backspanar[3]{\mbox{$#1\!:#2\nleftarrow#3$}}
%spans
\newcommand\spanlar[5]{\mbox{$#1\!:#2\leftarrow #3\rightarrow #4 :#5$}} %double arrow%
% -- bidir arrows version
\renewcommand\spanar[3]{\mbox{$#1\!:#2\nleftrightarrow #3$}}
\renewcommand\backspanar[3]{\mbox{$#1\!:#3\nleftrightarrow #2$}}
%----  triple spaces
\newcommand\tri{\enma{{\rightarrow}}}
\newcommand\trisprar[3]{\mbox{$#1\!:#2\trisparrow#3$}}


%-- backward arrow
\newcommand\flar[3]{\ensuremath{#1\!:#2\leftarrow #3}} %backward functional arrow
%\newcommand\bflar[3]{\mbox{$#1\!:#2\leftarrow #3$}} %backward functional arrow
\newcommand\dlar[3]{\mbox{$#1\!:#2\Leftarrow #3$}} %double arrow
%\newcommand\bdlar[3]{\mbox{$#1\!:#2\Leftarrow #3$}} %double arrow

% two directional
\newcommand\bilar[3]{\mbox{$#1\!:#2\leftrightarrow #3$}}%
\newcommand\biarr[3]{\mbox{$#1\!:#2\leftrightarrow #3$}}%
\newcommand\bidlar[3]{\mbox{$#1\!:#2\Leftrightarrow #3$}}
\newcommand\corar[3]{\bilar{#1}{#2}{#3}}
\newcommand\lelar[3]{\mbox{$#1\!:#2\rightleftarrows #3$}} %double arrow

\newcommand\lensar[3]{\mbox{$#1\!:#2\leftrightharpoons #3$}}%
\newcommand\lensarleft[3]{\mbox{$#1\!:#2\rightleftharpoons #3$}}%
\newcommand\lensarright[3]{\lensar{#1}{#2}{#3}}
%\renewcommand\lensar[3]{\mbox{$#1\!:#2\asymdoublearrow#3$}}
\newcommand\asymdoublearrow{%
\begin{array}{c}
~\rightarrow\\[-9pt]
\leftharpoondown
\end{array}}%

%%%%%%%%%%%%%%%%%%%%%%%
%---stackrel versions

% backward arrow
\newcommand\bfrarstack[3]{\mbox{$#3 \stackrel{~#1}{\longleftarrow} #2$}}
\newcommand\frarstack[3]{\bfrarstack{#1}{#2}{#3}}
\newcommand\flarstack[3]{\mbox{$#2\stackrel{#1~}{\longrightarrow} #3$}} %functyional arrow
\newcommand\spanlarstack[5]{\mbox{$#2\stackrel{~#1}{\longleftarrow} #3 %
                                                                       \stackrel{#5~}{\longrightarrow} #4$}} %double arrow%

% bidirectional

\newcommand\bilarsy[3]{\mbox{$#2\stackrel{#1}{\leftrightarrow}#3$}}
\newcommand\bidlarsy[3]{\mbox{$\left(#2\stackrel{#1}{\Leftrightarrow}#3\right)$}}
\newcommand\bixxlar[4]{\mbox{$#1\!:#2\stackrel{#3}{\longleftrightarrow} #4$}}%
\newcommand\bixlar[3]{\mbox{$#1\stackrel{#2}{\longleftrightarrow} #3$}}%
\newcommand\xxlar[4]{\mbox{$#1\!:#2\stackrel{#3}{\longrightarrow} #4$}}

%-- Now instances of the macros above for particular names of maps, thjeir sources and targets
\newcommand\updaraaa{\flar{a}{A}{A'}}
\newcommand\updarbbb{\flar{b}{B}{B'}}
\newcommand\corarrab{\bilar{r}{A}{B}}
\newcommand\corrarrab{\bilar{r}{A}{B}}
\newcommand\trisparrmn{\trispar{R}{\mmm}{\mmn}}
%
\newcommand\alifar[3]{\spanar{#1}{#2}{#3}}
\newcommand\backalifar[3]{\backspanar{#1}{#2}{#3}}
\newcommand\alifarrmn{\spanar{\mmr}{\mmm}{\mmn}}
\newcommand\genalifarrmn{\spanar{\mmr}{\mmm}{\mmn}}
\newcommand\symalifarrmn{\spanar{\mmr^{>\!<}}{\mmm}{\mmn}}
\newcommand\asalifarrmn{\spanar{\mmr^\le}{\mmm}{\mmn}}
\newcommand\asymLalifarrmn{\spanar{\mmr^<}{\mmm}{\mmn}}
\newcommand\asymLEalifarrmn{\spanar{\mmr^\le}{\mmm}{\mmn}}
\newcommand\asymGalifarrmn{\spanar{\mmr^>}{\mmm}{\mmn}}
\newcommand\asymGEalifarrmn{\spanar{\mmr^\ge}{\mmm}{\mmn}}
\newcommand\bialifarrmn{\spanar{\mmr^{\cong}}{\mmm}{\mmn}}

\newcommand\backgenalifarrmn{\backspanar{\mmr}{\mmm}{\mmn}}
\newcommand\backsymalifarrmn{\backspanar{\mmr^{>\!<}}{\mmm}{\mmn}}
\newcommand\backasalifarrmn{\backspanar{\mmr^\le}{\mmm}{\mmn}}
\newcommand\backasymLalifarrmn{\backspanar{\mmr^<}{\mmm}{\mmn}}
\newcommand\backasymGalifarrmn{\backspanar{\mmr^>}{\mmm}{\mmn}}

\newcommand\confar[3]{\spanar{#1}{#2}{#3}}
\newcommand\backconfar[3]{\backspanar{#1}{#2}{#3}}
\newcommand\confarkmn{\spanar{\mmk}{\mmm}{\mmn}}
\newcommand\genconfarkmn{\spanar{\mmk}{\mmm}{\mmn}}
\newcommand\symconfarkmn{\spanar{\mmk^{>\!<}}{\mmm}{\mmn}}
\newcommand\asconfarkmn{\spanar{\mmk^\le}{\mmm}{\mmn}}
\newcommand\asymLconfarkmn{\spanar{\mmk^<}{\mmm}{\mmn}}
\newcommand\asymLEconfarkmn{\spanar{\mmk^\le}{\mmm}{\mmn}}
\newcommand\asymGconfarkmn{\spanar{\mmk^>}{\mmm}{\mmn}}
\newcommand\asymGEconfarkmn{\spanar{\mmk^\ge}{\mmm}{\mmn}}
\newcommand\biconfarkmn{\spanar{\mmk^{\cong}}{\mmm}{\mmn}}
%--- outdated with *rmn instead of *kmn in the name of macros
%\newcommand\confar[3]{\spanar{#1}{#2}{#3}}
%\newcommand\backconfar[3]{\backspanar{#1}{#2}{#3}}
\newcommand\confarrmn{\spanar{\mmk}{\mmm}{\mmn}}
\newcommand\genconfarrmn{\spanar{\mmk}{\mmm}{\mmn}}
\newcommand\symconfarrmn{\spanar{\mmk^{>\!<}}{\mmm}{\mmn}}
\newcommand\asconfarrmn{\spanar{\mmk^\le}{\mmm}{\mmn}}
\newcommand\asymLconfarrmn{\spanar{\mmk^<}{\mmm}{\mmn}}
\newcommand\asymLEconfarrmn{\spanar{\mmk^\le}{\mmm}{\mmn}}
\newcommand\asymGconfarrmn{\spanar{\mmk^>}{\mmm}{\mmn}}
\newcommand\asymGEconfarrmn{\spanar{\mmk^\ge}{\mmm}{\mmn}}
\newcommand\biconfarrmn{\spanar{\mmk^{\cong}}{\mmm}{\mmn}}

\newcommand\backgenconfarkmn{\backspanar{\mmk}{\mmm}{\mmn}}
\newcommand\backsymconfarkmn{\backspanar{\mmk^{>\!<}}{\mmm}{\mmn}}
\newcommand\backasconfarkmn{\backspanar{\mmk^\le}{\mmm}{\mmn}}
\newcommand\backasymLconfarkmn{\backspanar{\mmk^<}{\mmm}{\mmn}}
\newcommand\backasymGconfarkmn{\backspanar{\mmk^>}{\mmm}{\mmn}}
%--%--- outdated with *rmn instead of *kmn in the name of macros
\newcommand\backgenconfarrmn{\backspanar{\mmk}{\mmm}{\mmn}}
\newcommand\backopgenconfarrmn{\backspanar{\mmk^\circ}{\mmm}{\mmn}}
\newcommand\backopgenalifarrmn{\backspanar{\mmr^\circ}{\mmm}{\mmn}}
\newcommand\backsymconfarrmn{\backspanar{\mmk^{>\!<}}{\mmm}{\mmn}}
\newcommand\backasconfarrmn{\backspanar{\mmk^\le}{\mmm}{\mmn}}
\newcommand\backasymLconfarrmn{\backspanar{\mmk^<}{\mmm}{\mmn}}
\newcommand\backasymGconfarrmn{\backspanar{\mmk^>}{\mmm}{\mmn}}



%
\newcommand\lensarlmn{\lensar{\alens}{\mmm}{\mmn}}
\newcommand\genlensarlmn{\lensar{\alens}{\mmm}{\mmn}}
\newcommand\aslensarlmn{\lensar{\alens^\leq}{\mmm}{\mmn}}
\newcommand\asymLElensarlmn{\lensar{\alens^\leq}{\mmm}{\mmn}}
\newcommand\asymGElensarlmn{\lensar{\alens^\geq}{\mmm}{\mmn}}
\newcommand\symlensarlmn{\lensar{\alens^\gtlt}{\mmm}{\mmn}}
\newcommand\lesnarlmn{\lensar{\alens}{\mmm}{\mmn}} % the same in case of typo

\newcommand\lenssupx[1]{\lensar{\alens^{{#1}}}{\mmm}{\mmn}}
\newcommand\lenssubx[1]{\lensar{\alens_{{#1}}}{\mmm}{\mmn}}
\newcommand\lensopsupx[1]{\lensar{\alens^{\circ{#1}}}{\mmn}{\mmm}}
\newcommand\lensopsubx[1]{\lensar{\alens^{\circ_{#1}}{\mmn}{\mmm}}}
\newcommand\lenssupsubx[2]{\lensar{\alens^{#1}_{#2}}{\mmm}{\mmn}}

\newcommand\cfwksubx[1]{\spanar{\mmk_{{#1}}}{\mmm}{\mmn}}
\newcommand\cfwkopsubx[1]{\spanar{\mmk^{\circ}_{{#1}}}{\mmm}{\mmn}}

\newcommand\syncar[3]{\mbox{$#1\!:#2 \rightleftarrows #3$}}%
\newcommand\syncarleft[3]{\mbox{$#1\!:#2 \leftrightarrows #3$}}%
\newcommand\syncaright[3]{\syncar{#1}{#2}{#3}}
\newcommand\async{\ensuremath{\sigma}}
\newcommand\aSync{\ensuremath{\Sigma}}
\renewcommand\aSync{\ensuremath{\Pi}}
\newcommand\syncarsab{\syncar{\async}{A}{B}}
\newcommand\gensyncarsab{\syncar{\async}{A}{B}}
\newcommand\genSyncarsab{\syncar{\async}{A}{B}}
\newcommand\gensynctypearsab{\syncar{\async}{A}{B}}
\newcommand\genSynctypearsab{\syncar{\async}{A}{B}}
\newcommand\assyncarsab{\syncar{\async^\leq}{A}{B}}
\newcommand\asymGLEsyncarsab{\syncar{\aSync_{>\!\le}}{A}{B}}
\newcommand\asymGELsyncarsab{\syncar{\aSync_{\ge\!<}}{A}{B}}
\newcommand\asymGsyncarsab{\syncar{\aSync_{>}}{A}{B}}
\newcommand\asymLsyncarsab{\syncar{\aSync_{<}}{A}{B}}
\newcommand\symsyncarsab{\syncar{\async_\gtlt}{A}{B}}
\newcommand\symsyncarsabPoor{\syncar{\async_{\ge\!\le}}{A}{B}}
\newcommand\symSyncarsab{\syncar{\aSync_\gtlt}{A}{B}}
\newcommand\symSyncarsabPoor{\syncar{\aSync_{\ge\!\le}}{A}{B}}
\newcommand\lesnarsab{\syncar{\async}{A}{B}} % the same in case of typo



\newcommand\noninclensarlmn{\lensar{\alens_\noninc}{\mmm}{\mmn}}
\newcommand\fullinclensarlmn{\lensar{\alens_\fullinc}{\mmm}{\mmn}}


\endinput










\newcommand\vilar[3]{\dlar{#1}{#2}{#3}}
\newcommand\vlar[3]{\vilar{#1}{#2}{#3}}
\newcommand\malar[3]{\flar{#1}{#2}{#3}}
\newcommand\uplar[3]{\flar{#1}{#2}{#3}}
\newcommand\ular[3]{\uplar{#1}{#2}{#3}}
%  adding :: Graph,Set,Cat etc as the 4th parameter
\newcommand\vilarcat[4]{\dlarcat{#1}{#2}{#3}{#4}} % .. ::#4
\newcommand\malarcat[4]{\flarcat{#1}{#2}{#3}{#4}}
\newcommand\uplarcat[4]{\flarcat{#1}{#2}{#3}{#4}}

\newcommand\viewOfrel{{\prec}}
\newcommand\viewofar[3]{\mbox{$#1\!:#2\Rightarrow #3$}}
\newcommand\mmvmn{\vilar{\mmv}{\mms}{\mmt}}
\newcommand\mmvab{\vilar{\mmv}{\mms}{\mmt}}
\newcommand\mmvabcat{\vilarcat{\mmv}{\mms}{\mmt}{\mmodcat}}
\newcommand\mmvmncat{\vilarcat{\mmv}{\mms}{\mmt}{\mmodcat}}
\newcommand\mvab {\vilar{\mv}{A}{B}}
\newcommand\mvabcat{\vilarcat{\mv}{A}{B}{\modcath}}


\newcommand\vrelar[3]{\mbox{$#1\stackrel{#3}{\leftarrow}#2$}}
\newcommand\mmvrel[3]{\vrelar{#1}{#2}{#3}}
\newcommand\mmabv{\mmvrel{\mma}{\mmb}{\mmv}}


==> macros/thisPaper-compy.tex <==
\newcommand\Uml{\enma{\mathcal{U}}}
%\newtheorem{example}{{\em Example}}
\newtheorem{propo}{Proposition}
%\newtheorem{remark}{Remark}
%\newtheorem{theorem}{Theorem}
%\newtheorem{defin}{Definition}
\newtheorem{constr}{Construction}
%\newtheorem{constr}[defin]{Construction}
%\newtheorem{lemma}{Lemma}
\newtheorem{coro}{Corollary}
\newtheorem{discuss}{Discussion}
%\newenvironment{proof}{{\em Proof.}}{\qed\par\smallskip\indent}
%\newcommand\qed{\hbox to 0.45\textwidth {\hfill $\square$}}

\newcommand\minusspaprop{\enma{
\begin{array}{l}
	{-}\mathsf{space}
	\\ [-7.5pt]
	\mathsf{properties}
\end{array}
}%>{\qqquad(4)}
}

\newcommand\spXXcodi{\enma{\spXX^0}}
\renewcommand\spXXcodi{\enma{||\spXX||}}
\newcommand\spapro{\enma{\footnotesize{\mathrm{spaceProp.}}}}
\newcommand\minusspa{\enma{({-}\spapro)}}
\newcommand\arrows{\enma{\mathsf{arrows}}}
\newcommand\paracaterr{\paracatx{\err}}
\newcommand\ints{\enma{\mathbb{N}}}
% + put and Co stuff
\newcommand\ponix{\enma{\breve{\nix}}}
\renewcommand\ponix{\enma{\ovr{\nix}}}
\renewcommand\ponix{\enma{\pi\!\nix}}
\renewcommand\ponix{\nix}
%\renewcommand\onix{\enma{\widetilde{\nix}}}
%\renewcommand\onix{\enma{\widehat{\nix}}}
%\renewcommand\onix{\enma{\stackrel{\circ}{\nix}}}

\newcommand\xyz{\enma{\mathsf{xxx}}}
\newcommand\lowlowindex[2]{\enma{#1_{\!_{#2}}}}
%\renewcommand\lowlowindex[2]{\enma{#1_{{#2}}}}

\newcommand\lowindxyz[3]{\enma{#1_{#2_{#3}}}}
%\renewcommand\lowlowindex[2]{\enma{#1_{{#2}}}}
\newcommand\plusx[1]{\lowlowindex{+}{#1}}
%\newcommand\plusx[1]{\lowindxyz{+}{}{#1}}
\newcommand\minusx[1]{\lowlowindex{-}{#1}}
\newcommand\minusnix{\enma{{-}\nix}}
\newcommand\minusnixbra{\enma{[{-}\nix]}}
\newcommand\minusnixcodi{\enma{({-}\nix)^0}}
\newcommand\minusnixcodibra{\enma{[({-}\nix)^0]}}
\newcommand\minusput{\enma{{-}\putl}}
\newcommand\minusdif{\enma{{-}\dif}}
\newcommand\minuswbdif{\enma{{-}\mathrm{wbdif}}}
	\renewcommand\minuswbdif{\enma{{-}\mathrm{Difputdif}}}
\newcommand\minusputcodi{\enma{{-}\putl^0}}
%\newcommand\minusx[1]{\enma{-_{\!_{#1}}}}
\newcommand\congx[1]{\lowlowindex{\cong}{#1}}

\newcommand\plusputx[1]{\enma{\plusx{#1}\putl}}
% + dif
\newcommand\plusxput{\enma{\plusx{\ponix}\putl}} 
\newcommand\plusxputcodi{\enma{\plusxput^0}} 
\newcommand\plusxdif{\enma{\plusx{\ponix}\dif}} 
\newcommand\plusxdel{\enma{\plusx{\ponix}\deltas}} 
%  delta
\newcommand\plusdelx[1]{\enma{\plusx{#1}\deltas}}
\newcommand\plusarrx[1]{\enma{\plusx{#1}\mathsf{arr}}}



%\newcommand\plusdifx[1]{\enma{\plusx{#1}\dif}}
%\newcommand\plusxdif{\plusdifx{\ponix}} 
%\newcommand\minusdifx[1]{\enma{\minusx{#1}\dif}}
\newcommand\minusxdel{\minusx{\ponix}\deltas}

% colors
\newcommand\diff{\enma{\diagopername{diff}}}
\newcommand\diffind{\enma{\diagopername{diff}}}
\newcommand\differ{\enma{\diagopername{differ}}}
\newcommand\pairing{\enma{\diagopername{pairing}}}
\newcommand\lens{\enma{\diagopername{lens}}}
\newcommand\grt[1]{\textcolor{caribbeangreen}{#1}}
\newcommand\grgrt[1]{\textcolor{caribbeangreen}{#1}}
\newcommand\blt[1]{\textcolor{blue}{#1}}
\newcommand\redt[1]{\textcolor{red}{#1}}

%\newcommand\plusxdel[1]{\enma{\plusx{#1}\deltas}}
%\newcoo
%\newcommand\lensarrp


%\newcommand\plusxdel{\plusdelx{\onix}} 

\newcommand\pind{\enma{\tilde{p}}}
\newcommand\odash{\enma{\circleddash}}
\newcommand\ovre{\ovr{e}}
\newcommand\medxyz[3]{\enma{#1^{#2#3}}}  % #1 is arg, #2 delta, #3 fun
\newcommand\medaxy[2]{\medxyz{a}{#1}{#2}}
\newcommand\medfxy[2]{\medxyz{#1}{#2}{f}}
\newcommand\medadx[1]{\medxyz{a}{\del}{#1}}
\newcommand\medafx[1]{\medxyz{a}{#1}{f}}

	\newcommand\medxy[2]{\enma{{#1}^{\prt{#2}}}}
	%\renewcommand\medxy[2]{\medxyz{}{}}
	\newcommand\medfx[1]{\medxy{#1}{f}}
	
			\newcommand\getobx[1]{\enma{|\get|_{#1}}}
	\newcommand\getobp{\getobx{p}}
	
	
\newcommand\Del{\enma{\mathit{\Delta}}}
\newcommand\Dela{\enma{\Delta_a}}
\newcommand\Delp{\enma{\Delta_p}}
\newcommand\ffun{\enma{\mathbf{f}}}
\renewcommand\ffun{\enma{\widehat{f}}}
\newcommand\DDel{\enma{{\pmb \Delta}}}
\newcommand\DDela{\enma{{\pmb \Delta}_\spA}}
\newcommand\DDelb{\enma{{\pmb \Delta}_\spB}}
\newcommand\del{\enma{\delta}}
%\renewcommand\del{\Del}
\newcommand\dela{\enma{\delta_a}}
\newcommand\della{\enma{\hat{\del}}}
\newcommand\dellp{\enma{\check{\del}}}
\newcommand\delb{\enma{\delta_b}}
\newcommand\jacobx[1]{\enma{\mathbf{J}#1}}
\newcommand\jacobf{\jacobx{f}}
\newcommand\prtx[1]{\enma{\prt #1}}
\newcommand\prtf{\prtx{f}}
\renewcommand\cod{\diagopername{cod}}
\renewcommand\cod{\diagopername{codomain}}
\newcommand\fu{\nmf{f}}
\newcommand\wi{\nmf{w}}
\newcommand\emb{\nmf{e}}
\newcommand\rcat{\enma{\mathbf{R}}}
\newcommand\bx{BX}%\hfill}}
\newcommand\bxl{BX\enma{_\mathrm{L}}}%\hfill}}
\newcommand\Bx{BX\ }%\hfill}}
\newcommand\Bxs{BX}%\hfill}}
\newcommand\alalens{ala-lens}
\newcommand\Alalens{Ala-lens}
\newcommand\alaalens{alaa-lens}
\newcommand\Alalaens{Alaa-lens}
\newcommand\mlo{ML$_{\mathsf{noBp}}$}
\newcommand\mlbp{ML}%$_{\mathsf{bp}}$}
\newcommand\bxo{Bx}%$_{\mathsf{no{-}ev}}$}
\newcommand\bxev{Bx$_{\mathsf{Ev}}$}

\newcommand\warr{\enma{\rightsquigarrow}}
\newcommand\warrxy[2]{\enma{#1\warr#2}}
\newcommand\warraa{\warrxy{a}{a'}} 
\newcommand\warrbb{\warrxy{b}{b'}}
\newcommand\warrbba{\warrxy{b'}{b'^@}}
\newcommand\warrpp{\warrxy{p}{p'}}

\newcommand\byx[1]{\mbox{\quad #1}}
\newcommand\byeq[2]{\mbox{\quad #1 \eqref{#2}}}
\newcommand\byeqna[2]{\mbox{\quad #1 \eqref{eqna-#2}}}
\newcommand\byeqnaa[3]{\mbox{\quad #1 \eqref{eqna-#2}~#3  }}

%\renewcommand\xxx{\enma{\mathsf{xxx}}}
\renewcommand\xob[1]{\enma{|#1|}}
\newcommand\Arr{\enma{\mathsf{Arr}}}
\newcommand\elll{\enma{\ell}}
\newcommand\vii{\enma{v^{}}}
\newcommand\uiii{\enma{u^{}}}
\newcommand\viii{\enma{v^{@}}}
\newcommand\niget{\enma{\mathpzc{get}}}
\newcommand\nifo[1]{\enma{\mathcal{#1}}}
%\newcommand\nim{\nifo{M}}
\newcommand\nin{\nifo{N}}
\newcommand\defcat{\catfont{Def}}
\renewcommand\defcat{\enma{\mathpzc{Def}}}
\newcommand\vbf{\enma{\mathbf{v}}}
\newcommand\smm{symmetric monoidal}
\newcommand\sm{sm}
\newcommand\ome{\enma{\omega}}
\newcommand\isop{\enma{\iota}}
\newcommand\hell{\enma{\hat\ell}}
\newcommand\hp{{\enma{\hat p}}}
\renewcommand\hp{{\enma{\isop(p)}}}
\newcommand\hget{\enma{\widehat{\get}}}
\newcommand\hputl{\enma{\widehat{\putl}}}

\newcommand\Err{\nmf{Err}}
\newcommand\rreals{\enma{\reals\timm\reals}}
\newcommand\prtfrac[2]{\enma{\frac{\prt#1}{\prt#2}}}
\newcommand\breals{\enma{\mathbf{R}}}
\newcommand\enma[1]{{\ensuremath{#1}}}
\newcommand\brealsx[1]{\enma{\mathbf{R}^{#1}}}
\newcommand\rcatx[1]{\enma{\rcat^{{#1}}}}
\newcommand\realsx[1]{\enma{\mathbb{R}^{#1}}}
%\renewcommand\xob[1]{\enma{|#1|}}
%\newcommand\bx{Bx}
\renewcommand\f{\enma{I(p,\_)}}
\newcommand\parr{parameter}
\newcommand\parrd{parameterized}
\newcommand\Parrd{Parameterized}
\newcommand\parrn{parameterization}
\newcommand\Parrn{Parameterization}
\newcommand\pard{parameterized}
\newcommand\Pard{Parameterized}
\newcommand\parn{parameterization}
\newcommand\Parn{Parameterization}


\newcommand\Reals{\enma{\mathbb{R}}}
\newcommand\reals{\enma{\mathbb{R}}}
%\newcommand\realsx[1]{\enma{\mathbb{R}^{{#1}}}
\newcommand\prpol{\nmf{policy}}
\newcommand\pol{\nmf{pol}}
\newcommand\Pol{\nmf{Pol}}
\newcommand\ipol{\nmf{inv}}
\renewcommand\pol{\enma{\mathit{pol}}}

\newcommand\err{\nmf{err}}
\newcommand\rre{\nmf{r\!r\!e}}
\newcommand\errx{\nmf{errx}}
\newcommand\sym{\nmf{sym}}
\newcommand\eps{\enma{\varepsilon}}
\newcommand\ptol{\catname{p2l}}
\newcommand\aplenscat{\catname{alLens}}
\newcommand\apalenscat{\catname{aaLLens}}
\newcommand\allenscat{\catname{alLens}}
\newcommand\alalenscat{\catname{alaLens}}
\newcommand\aladlenscat{\catname{alaLensDif}}
\newcommand\alalenscatcodi{\enma{\catname{alaLens}}\!\,\mbox{\bf\em 0}}
\renewcommand\alalenscatcodi{\enma{\catname{alaLens}^0}}
\newcommand\pgetnixcatcodi{\enma{\catname{pGet}_\nix^0}}
\newcommand\putlcodi{\enma{\putl^0}}
\newcommand\allenscatcodi{\enma{\catname{alLens}^0}}
\newcommand\alalensdifcat{\catname{alaLensDif}}
\newcommand\alalenscatdif{\alalensdifcat}
\newcommand\diffcat{\catname{Dif\!f}}
% amedamend
\newcommand\alaalenscat{\catname{alaaLens}}
\newcommand\alaalenscatcodi{\enma{\catname{alaaLens}}\!\,\mbox{\bf\em 0}}
\newcommand\alaalenscatdif{\catname{alaaLensDif}}
\newcommand\codiscr{\diagopername{codiscr}}
\renewcommand\codiscr{\catname{codiscr}}
\newcommand\codifun{\codiscr}
\newcommand\pgetcat{\catname{pGet}}
\newcommand\pgetdifcat{\catname{pGetDif}}
\newcommand\pgetcatnix{\enma{\pgetcat_\nix}} %catname{pGet}}

\newcommand\lift{\nmf{lift}}
\newcommand\fun{\nmf{fun}}
\newcommand\grd{\nmf{grd}}
\newcommand\Grd{\nmf{Grd}}
\newcommand\gdbp{\nmf{GdBp}}
\newcommand\gd{\nmf{Gd}}
\renewcommand\lawnamebr[1]{\lawname{(#1)}}
\newcommand\amend{amendment}
\newcommand\prop{proposition}
\newcommand\icorr{\ensuremath{\mathsf{indCorr}}}
\newcommand\lner{learner}
\newcommand\Lner{Learner}
\newcommand\learncat{\catname{Learn}}
\newcommand\learnfun{\catname{learner}}
\newcommand\learncatcon{\enma{\mathbb{L}\mathbf{earn}}}
\newcommand\paracatcon{\enma{\mathbb{P}\mathbf{ara}}}
%\newcommand\learnfun{\catname{learner}}




\newcommand\bxfun{\catname{bx}}
\newcommand\bxcat{\catname{PView}}
\newcommand\ptracat{\catname{PTransf}}
\newcommand\tracat{\catname{Transf}}
\newcommand\pviewcat{\catname{PGet}}
\newcommand\viewcat{\catname{Get}}

\newcommand\paarr{\enma{\;\paar\;}} 
\newcommand\lm{\enma{\ell;\emm}}
\newcommand\lmbr{\enma{(\ell;\emm)}}
\newcommand\paarrx[1]{\paarr} %\enma{\;\paar^{#1}\;  }}

\newcommand\paar{\enma{\!\,|\!|}}
\renewcommand\ll{\enma{\ell_1\!|\!|\ell_2}}
\newcommand\pp{{p_1\paar p_2}}
\renewcommand\ss{{S_1\paar S_2}}

\renewcommand\ll{\enma{\ell_1\paar\ell_2}}
\newcommand\llbr{\enma{(\ll)}}
\newcommand\putpsi{\putxyz{(1)}{p_1}{S_1}}
\newcommand\putpsii{\putxyz{(2)}{p_2}{S_2}}
\newcommand\getpi{\getxy{{\ell_1}}{{p_1}}} 
\newcommand\getpii{\getxy{{\ell_2}}{p_2}}
\newcommand\difputdif{\lawname{Difputdif}}
\renewcommand\difputlaw{\lawname{Difput}} % must be the same
\newcommand\catcattimm{\enma{(\catcat,\!\timm)}}
\newcommand\setcattimm{\enma{(\setcat,\!\timm)}}
\newcommand\Hom{\enma{\mathit{Hom}}}
\newcommand\codd{\enma{\mathsf{cod}}}
\newcommand\xcatcat[1]{\enma{\catname{#1}\catname{Cat}}}
\newcommand\pcatcat{\catname{pCat}}
\newcommand\smcatcat{\catname{smCat}}
\newcommand\qcatcat{\catname{QCat}}
\newcommand\pcatcatdif{\catname{pCatDif}}
\newcommand\pspadifcat{\catname{pSpaceDif}}
\newcommand\psetcat{\catname{pSet}}
\newcommand\paracat{\catname{Para}}
\newcommand\paracatre{\catname{Para_\reals}}
\newcommand\paracatrcat{\catname{Para_\rcat}}
  \newcommand\fbf{\enma{\pmb f}}
\newcommand\leefun{\enma{L_{\eps,\err}}}
\newcommand\leefunovr{\ovr{\leefun}}
\newcommand\pfuncat{\catname{pFun}}
\newcommand\pmtcat{\catname{pTransf}}
\newcommand\lnercat{\learncat}
\newcommand\slenscat{\catname{sLens}}
\newcommand\alenscat{\catname{aLens}}
\newcommand\alenscattgg{\mathbb{V}\catname{TGGLens}}
\newcommand\viewcattgg{\mathbb{V}\catname{iewTGG}}
\newcommand\bprules{\nmf{Rules}}
\newcommand\bppol{\nmf{bpPolicy}}
\newcommand\mboxsmall[1]{\mbox{\small#1}}


\newcommand\aalenscat{\catname{aaLens}}
\renewcommand\apalenscat{\catname{alaLens}}
\renewcommand\alalenscat{\catname{alaLens}}
\newcommand\ltol{\catname{l2l}}
\newcommand\pq{\enma{{pq}}}
\newcommand\eh{\enma{{eh}}}
\newcommand\klbr{\enma{(\kl)}}

\newcommand\citell{\cite{ll-bx19}[ll@bx19]}



% Must add these macros here, because tex does not compile, if they are moved to macro files
\newcommand\figri{} 
\newcommand\figrii{}
\newcommand\figriii{}
\newcommand\figriia{}
\newcommand\figriv{}
\newcommand\figrv{}
\newcommand\PP{\ensuremath{\mathit{PUT}}}
\newcommand\figrsdlens{Fig.??}
\newcommand\diarefi{}
\newcommand\diarefii{}
\newcommand\diarefiii{}

\newcommand\putgeto{\enma{\putget_0}}

%\newcommand\putxyz[3]{\ensuremath{#3.\putl^{(#1,#2)}}}
\newcommand\putxyz[3]{\ensuremath{\putl^{#1}_{{#2},{#3}}}}
\newcommand\putUL[2]{\ensuremath{\putl^{#1}_{#2}}}
\newcommand\getxy[2]{\ensuremath{\get^{{#1}}_{{#2}} }}
\newcommand\putqbx[1]{\putxyz{#1}{q}{B_p}}
%\newcommand\putqb{\putxy{q}{B}}
\newcommand\puthatxy[2]{\ensuremath{\widehat{\putl}^{(#1,#2)}}}

\newcommand\putxy[2]{\ensuremath{\putl_{(#1,#2)}}}
\renewcommand\putxy[2]{\ensuremath{\putl_{#1,#2}}}
\newcommand\putpa{\putxy{p}{A}}
\newcommand\putqb{\putxy{q}{B}}
\newcommand\putps{\putxy{p}{S}}
\newcommand\putqbp{\putxy{q}{B_p}}
%\newcommand\putqb{\putxy{q}{B}}
%--- for gets
\newcommand\gettxy[2]{\ensuremath{\get_{#1,#2}}}
\newcommand\getamxy[2]{\ensuremath{\get^{@}_{#1,#2}}}
%\renewcommand\putxy[2]{\ensuremath{\putl_{#1,#2}}}
\newcommand\getpa{\gettxy{p}{A}}
\newcommand\getqb{\gettxy{q}{B}}
\newcommand\getps{\gettxy{p}{S}}
\newcommand\getamps{\getamxy{p}{S}}

\newcommand\xdeldel[3]{\enma{#1_{#2,#3}}}
\newcommand\sue{\xdeldel{S}{u}{e}}



\renewcommand\indb{\ensuremath{\mathsf{req}}}
\newcommand\upd{\ensuremath{\mathsf{upd}}}
\newcommand\req{\ensuremath{\mathsf{req}}}
\renewcommand\self{\ensuremath{\mathsf{self}}}

\newcommand\niuu{\ensuremath{\mathbf{u}}}
\newcommand\thissec{\ref{sec:somesection}}
\newcommand\fakeob{\strut}
\newcommand\npmargin[1]{\mymarginnew{NewSubsect\# #1}}
\newcommand\npmarginn[2]{\mymarginNew{NewSubsect\##1}{#2}}

\renewcommand\x{\enma{\mathbf{x}}}

\renewcommand\newpi[2]{\hlight{#1}{NewPiece\#\! #2}}
\renewcommand\newpii[3]{\hlightNew{#1}{NewPiece\#\! #2}{#3}}
\newcommand\newsec[3]{\hlightNew{#1}{This is entirely new sect\! #2}{#3}}

\newcommand\prodx[1]{\ensuremath{\small{\prod}\!#1}}
\renewcommand\xstar[1]{\Corrsx{#1}}
%\renewcommand\xob[1]{\ensuremath{\mathsf{Ob}(#1)}}

\renewcommand\R[1]{\ensuremath{\mspA^{\bigstar}_{#1}}}
\renewcommand\xarr[1]{\ensuremath{#1%
		^{\footnotesize{\RHD}}}}
	\renewcommand\xarr[1]{\ensuremath{#1%
			^{\mathbf{\rightarrow}}}}
\renewcommand\xarr[1]{\ensuremath{\mathsf{Ar}(#1)}}
\newcommand\xar[1]{\ensuremath{\mathsf{Ar}(#1)}}

\newcommand\setop{\ensuremath{\diagopername{set}}}
\newcommand\Corrsx[1]{\ensuremath{#1^\bigstar}}
\renewcommand\Corrsx[1]{\ensuremath{\mathsf{Corr}(#1)}}
\newcommand\corrsx[1]{\ensuremath{\mathsf{corr}(#1)}}
\newcommand\Corrsma{\Corrsx{\mspA}}
\newcommand\Corrsa{\Corrsx{\spA}}
\newcommand\Korrsma{\Corrsx{\spK}}
\newcommand\corr{\ensuremath{\mathsf{corr}}}
\newcommand\corrx[1]{\corrsx{#1}}
\newcommand\Corr{\ensuremath{\mathsf{Corr}}}
\newcommand\Corrcat{\ensuremath{\mathbf{Corr}}}
\newcommand\Corrx[1]{\Corrsx{#1}}

\newcommand\amdx[1]{\ensuremath{#1^{@}}}
\newcommand\amex[1]{\amdx{#1}}
\newcommand\ameui{\amex{u_i}}

\newcommand\reflectzero{Reflect0}

\newcommand\kputput{\lawname{KPutput}}
\newcommand\kputputlaw{\lawname{\kputput} law}
\newcommand\ppgrx[1]{\ensuremath{\ppg^{#1}}}
\newcommand\ppgr{\ppgrx{\acorr}}
\newcommand\ppgB{\ppgrx{B}}
\newcommand\ppghB{\ppgrx{\hat B}}

\newcommand\elementToSingleton[1]{\ensuremath{\widehat{#1}}}
\newcommand\etosing[1]{\elementToSingleton{#1}}
\newcommand\sing{\ensuremath{\mathrm{sing}}}
\newcommand\prosing{\ensuremath{\prod}}
\newcommand\allm{\ensuremath{(M_{123})}}
\newcommand\spE{\ensuremath{\spacenam{E}}}
%-- the upper taken from macros-general
\renewcommand\comprfam[2]{\left(\mathstrut{#1}\left|\;{#2}\right.)}
\renewcommand\comprfam[2]{\left(\mathstrut{#1}\,| \;{#2}\right)}
%\renewcommand\comprfam[2]{\left(\mathstrut{#1}\right)_{{#2}}}

%= tuples
\newcommand\tuplenam[1]{\ensuremath{\pmb{#1}}}
\renewcommand\tuplenam[1]{\ensuremath{{#1}}}
\newcommand\tupX[1]{\ensuremath{\tuplenam{#1}}}
\newcommand\tupA{\tupX{A}}
\newcommand\tupu{\tupX{u}}
\newcommand\tupB{\tupX{B}}
\newcommand\tupv{\tupX{v}}

\newcommand\prodX[1]{\ensuremath{\prtbf^{\Pi}\!\!#1}}
\renewcommand\prodX[1]{\ensuremath{#1^{\Pi}}}
\newcommand\prodmspA{\prodX{\mspA}}
\newcommand\prodmspB{\prodX{\mspB}}

\newcommand\bounX[1]{\ensuremath{\prtbf#1}}
\newcommand\bounmspA{\bounX{\mspA}}




\newcommand\xconfig[1]{\ensuremath{\mathsf{#1}}}
\newcommand\Span{\xconfig{Span}}
\newcommand\Cospan{\xconfig{Cospan}}
%\newcommand\K{\spaR}
% -- conseq compatible updates
\newcommand\compUpd[2]{\ensuremath{\mathsf{#1}^{{#2}}}}
\newcommand\seqK{\compUpd{K}{\RHD\!\!\RHD}}
\newcommand\parK{\compUpd{K}{{|}{|}{}}}
\newcommand\spanK[1]{\compUpd{K}{\blacktriangle{#1}}}
\newcommand\disjK[1]{\compUpd{K}{\blacktriangle{#1}}}
\newcommand\Kupd{\seqK}
\newcommand\Kseq{\seqK}
%--space of conflict-free/concurr compatible updates
\newcommand\cofrK{\parK}

\newcommand\Kpar{\parK}
\newcommand\Kspan[1]{\spanK{#1}}
\newcommand\Kdisj[1]{\disjK{#1}}

%\endinput

% space of consist corrs
\newcommand\consK{\mspX{K^\bigstar}}
\newcommand\Kcorr{\compUpd{K}{\bigstar}}
%\renewcommand\Kcorr{\mspX{K^{\bigstar}}}
%\renewcommand\Kcorr{\ensuremath{{\spaR}^{}}}






\newcommand\prospa[1]{\ensuremath{\Pi#1}}
\newcommand\exIntro{$\ast$}
\renewcommand\exIntro{\textit{Running example}}
\newcommand\bad{\ensuremath{\dagger}}
\newcommand\prt{\ensuremath{\partial}}
\newcommand\prtbf{\ensuremath{\boldsymbol{\partial}}}
\renewcommand\ta{\ensuremath{\mathsf{t}}}
\renewcommand\so{\ensuremath{\mathsf{s}}}
\cornersize{.5} 
\newcommand\dbox[1]{\fbox{$#1$}}
\renewcommand\dbox[1]{\ovalbox{$#1$}}

\newcommand\mmcol{\ensuremath{{M^{++}}}}
\newcommand\aacol{\ensuremath{{A^{++}}}}

\newcommand\Mplus{\ensuremath{{M^+}}}
\newcommand\Aplus{\ensuremath{{A^+}}}
\newcommand\mmplus{\Mplus}
\newcommand\aaplus{\Aplus}
\newcommand\Mpluss{\ensuremath{{M^{++}}}}
\newcommand\Apluss{\ensuremath{{A^{++}}}}

\newcommand\mmap[1]{\ensuremath{{\mathsf{m}_{#1}}}}
\newcommand\amap[1] {\ensuremath{{\mathsf{a}_{#1}}}}
\newcommand\mplus[1]{\ensuremath{{\mathsf{m}^+_{#1}}}}
\newcommand\aplus[1]{\ensuremath{{\mathsf{a}^+_{#1}}}}


\newcommand\undn{\und{n}}


\newcommand\scenum[1]{\ensuremath{\mathbf{(S#1)}}}
\newcommand\Scenum[1]{\textbf{(Scenario #1)}}
\renewcommand\Scenum[1]{(scenario \scenum{#1})}

\newcommand\xmi[1]{\ensuremath{M_{#1}}}
\newcommand\mo{\xmi{}}
\newcommand\mi{\xmi{1}}
\newcommand\mii{\xmi{2}}
\newcommand\miii{\xmi{3}}
\newcommand\xai[1]{\ensuremath{A_{#1}}}
\newcommand\yai[1]{\ensuremath{R_{#1}}}
\newcommand\ao{\xai{}}
\newcommand\ai{{\xai{1}}}
\newcommand\aii{{\xai{2}}}
\newcommand\aiii{{\xai{3}}}
\newcommand\ri{{\yai{1}}}
\newcommand\rii{{(\yai{12})}}
\newcommand\riii{{(\yai{123})}}


%-- proper names --
\newcommand\addr{\nmf{Addr}}
\newcommand\name{\nmf{name}}
\newcommand\String{\nmf{String}}
\newcommand{\Person}{\nmf{Person}}
\newcommand{\Comp}{\nmf{Company}}
\newcommand{\Company}{\nmf{Company}}
\newcommand{\Commute}{\nmf{Route}}
\newcommand{\Comm}{\nmf{Route}}
\newcommand{\Route}{\nmf{Route}}
\newcommand\Addr{\nmf{Addr}}
\newcommand\from{\nmf{from}}
\newcommand\lives{\nmf{livesAt}}
\newcommand\loc{\nmf{locAt}}
\newcommand\toattr{\nmf{to}}
%\newcommand\Empl{\nmf{Empl\textrm{-}ment}}
%\newcommand{\eer}{\nmf{empl}\textrm{-}\nmf{er}}
%\newcommand{\eee}{\nmf{empl}\textrm{-}\nmf{ee}}
\newcommand\Empl{\nmf{Employment}}
\newcommand{\eer}{\nmf{employer}}
\newcommand{\eee}{\nmf{employee}}
\newcommand{\etor}{\nmf{(e2r)}}
\newcommand{\ptop}{\nmf{(p2p)}}
\newcommand{\ctoc}{\nmf{(c2c)}}


\newcommand\namefont[1]{\ensuremath{\mathsf{#1}}}
\newcommand\nmf[1]{\namefont{#1}}
\newcommand\ittt[1]{\ensuremath\mathit{#1}} 

\newcommand{\netw}{\nmf{Network}}
\newcommand{\network}{\nmf{Network}}
\newcommand{\person}{\nmf{Person}}
\newcommand{\member}{\nmf{Member}}

\renewcommand\phone{\nmf{Phone}}
\newcommand\EMail{\nmf{Email}}
\newcommand\contact{\nmf{Contact}}
\newcommand{\topic}{\nmf{Topic}}
\newcommand{\str}{\nmf{Str}}
\renewcommand{\inv}{\nmf{inv}}
\newcommand{\PM}{\nmf{P/M}}

\newcommand{\cp}{\nmf{c/p}}
\newcommand{\memb}{\nmf{memb}}
\newcommand{\ident}{\nmf{ident}}
\newcommand{\cell}{\nmf{cell}}
\newcommand{\emails}{\nmf{emails}}
\newcommand{\logins}{\nmf{logins}}
\newcommand{\comm}{\nmf{comm}}
\newcommand{\privv}{\nmf{priv}}
%\newcommand{\from}{\nmf{from}}
\newcommand{\too}{\nmf{to}}
\newcommand{\scope}{\nmf{scope}}
\newcommand{\escope}{\nmf{e}\textrm{-}\nmf{scope}}
\newcommand{\on}{\nmf{on}}
\newcommand{\ret}{\nmf{re}}
\newcommand{\re}{\nmf{re}}
\newcommand{\subj}{\nmf{subj}}
\newcommand{\eon}{\nmf{e}\textrm{-}\nmf{on}}
%===
%\newlength{\cellH}
%\newlength{\cellW}



%=== from JSS paper
\newcommand\incal{incremental}
\newcommand\mbcon{\ensuremath{\sim}}
\newcommand\hgg[1]{}
\newcommand\info{\ensuremath{\mathrm{inf}}}

\newcommand\boldsubsubsection[1]{\subsubsection*{\textbf{#1}}}
\renewcommand\boldsubsubsection[1]{\subsubsection*{{#1}}}
\newcommand\goup{\vspace{-7.5pt}}
\newcommand\rich{\ensuremath{\mathrm{+}}}
\newcommand\poor{\ensuremath{\mathrm{-}}}
\newcommand\ohtri{\ensuremath{(\ohafra\ohafra\ohafra)}}

\newcommand\alens{\ensuremath{\lambda}}

% sub and super scripts
\newcommand\indname[1]{\ensuremath\mathrm{#1}}
\newcommand\priv{{\indname{prv}}}
\newcommand\pub{{\indname{pub}}}

\endinput

% Domain-codomain/source-target/ident
\newcommand\cod[1]{\ensuremath{{#1}^\bullet}}
\newcommand\dom[1]{\ensuremath{^\bullet{#1}}}
\newcommand\so{\ensuremath{\mathsf{src}}}
\newcommand\ta{\ensuremath{\mathsf{trg}}}
\renewcommand\so{\ensuremath{\mathsf{s}}} % was src
\renewcommand\ta{\ensuremath{\mathsf{t}}}  % was trg
\newcommand\ldom[1]{\ensuremath{$\Box #1 $}}
\newcommand\rdom[1]{\ensuremath{$#1 \Box $}}
\newcommand\id[1]{\opname{id}_{{#1}}}
\renewcommand\id{\opname{id}}


==> macros/thisPaper-llncs.tex <==
% Must add these macros here, because tex does not compile, if they are moved to macro files
\newcommand\figri{} 
\newcommand\figrii{}
\newcommand\figriii{}
\newcommand\figriia{}
\newcommand\figriv{}
\newcommand\figrv{}
\newcommand\PP{\ensuremath{\mathit{PUT}}}
\newcommand\figrsdlens{Fig.??}


\newcommand\putxy[2]{\ensuremath{\putl^{(#1,#2)}}}
\newcommand\putpa{\putxy{p}{A}}
\newcommand\putqb{\putxy{q}{B}}
\renewcommand\indb{\ensuremath{\mathsf{req}}}
\newcommand\upd{\ensuremath{\mathsf{Upd}}}
\newcommand\req{\ensuremath{\mathsf{req}}}
\renewcommand\self{\ensuremath{\mathsf{self}}}

\newcommand\niuu{\ensuremath{\mathcal{u}}}
\newcommand\thissec{\ref{sec:somesection}}
\newcommand\fakeob{\strut}
\newcommand\npmargin[1]{\mymarginnew{NewSubsect\# #1}}
\newcommand\npmarginn[2]{\mymarginNew{NewSubsect\##1}{#2}}
\newcommand\newsec[3]{\hlightNew{#1}{This is entirely new sect\! #2}{#3}}
%\newcommand\npmarginn[2]{\mymarginNew{NewSubsect\##1}{#2}}

\renewcommand\xstar[1]{\Corrsx{#1}}
\renewcommand\xob[1]{\ensuremath{\mathsf{Ob}(#1)}}

\renewcommand\R[1]{\ensuremath{\mspA^{\bigstar}_{#1}}}
\renewcommand\xarr[1]{\ensuremath{#1%
		^{\footnotesize{\RHD}}}}
	\renewcommand\xarr[1]{\ensuremath{#1%
			^{\mathbf{\rightarrow}}}}
\renewcommand\xarr[1]{\ensuremath{\mathsf{Ar}(#1)}}

\newcommand\setop{\ensuremath{\diagopername{set}}}
\newcommand\Corrsx[1]{\ensuremath{#1^\bigstar}}
\renewcommand\Corrsx[1]{\ensuremath{\mathsf{Corr}(#1)}}
\newcommand\corrsx[1]{\ensuremath{\mathsf{corr}(#1)}}
\newcommand\Corrsma{\Corrsx{\mspA}}
\newcommand\Corrsa{\Corrsx{\spA}}
\newcommand\Korrsma{\Corrsx{\spK}}
\newcommand\corr{\ensuremath{\mathsf{corr}}}
\newcommand\corrx[1]{\corrsx{#1}}
\newcommand\Corr{\ensuremath{\mathsf{Corr}}}
\newcommand\Corrcat{\ensuremath{\mathbf{Corr}}}
\newcommand\Corrx[1]{\Corrsx{#1}}

\newcommand\amdx[1]{\ensuremath{#1^{@}}}
\newcommand\amex[1]{\amdx{#1}}
\newcommand\ameui{\amex{u_i}}

\newcommand\reflectzero{Reflect0}

\newcommand\kputput{\lawname{KPutput}}
\newcommand\kputputlaw{\lawname{\kputput} law}
\newcommand\ppgrx[1]{\ensuremath{\ppg^{#1}}}
\newcommand\ppgr{\ppgrx{\acorr}}
\newcommand\ppgB{\ppgrx{B}}
\newcommand\ppghB{\ppgrx{\hat B}}

\newcommand\elementToSingleton[1]{\ensuremath{\widehat{#1}}}
\newcommand\etosing[1]{\elementToSingleton{#1}}
\newcommand\sing{\ensuremath{\mathrm{sing}}}
\newcommand\prosing{\ensuremath{\prod}}
\newcommand\allm{\ensuremath{(M_{123})}}
\newcommand\spE{\ensuremath{\spacenam{E}}}
%-- the upper taken from macros-general
\renewcommand\comprfam[2]{\left(\mathstrut{#1}\left|\;{#2}\right.)}
\renewcommand\comprfam[2]{\left(\mathstrut{#1}\,| \;{#2}\right)}
%\renewcommand\comprfam[2]{\left(\mathstrut{#1}\right)_{{#2}}}

%= tuples
\newcommand\tuplenam[1]{\ensuremath{\pmb{#1}}}
\renewcommand\tuplenam[1]{\ensuremath{{#1}}}
\newcommand\tupX[1]{\ensuremath{\tuplenam{#1}}}
\newcommand\tupA{\tupX{A}}
\newcommand\tupu{\tupX{u}}
\newcommand\tupB{\tupX{B}}
\newcommand\tupv{\tupX{v}}

\newcommand\prodX[1]{\ensuremath{\prtbf^{\Pi}\!\!#1}}
\renewcommand\prodX[1]{\ensuremath{#1^{\Pi}}}
\newcommand\prodmspA{\prodX{\mspA}}
\newcommand\prodmspB{\prodX{\mspB}}

\newcommand\bounX[1]{\ensuremath{\prtbf#1}}
\newcommand\bounmspA{\bounX{\mspA}}




\newcommand\xconfig[1]{\ensuremath{\mathsf{#1}}}
\newcommand\Span{\xconfig{Span}}
\newcommand\Cospan{\xconfig{Cospan}}
%\newcommand\K{\spaR}
% -- conseq compatible updates
\newcommand\compUpd[2]{\ensuremath{\mathsf{#1}^{{#2}}}}
\newcommand\seqK{\compUpd{K}{\RHD\!\!\RHD}}
\newcommand\parK{\compUpd{K}{{|}{|}{}}}
\newcommand\spanK[1]{\compUpd{K}{\blacktriangle{#1}}}
\newcommand\disjK[1]{\compUpd{K}{\blacktriangle{#1}}}
\newcommand\Kupd{\seqK}
\newcommand\Kseq{\seqK}
%--space of conflict-free/concurr compatible updates
\newcommand\cofrK{\parK}

\newcommand\Kpar{\parK}
\newcommand\Kspan[1]{\spanK{#1}}
\newcommand\Kdisj[1]{\disjK{#1}}

%\endinput

% space of consist corrs
\newcommand\consK{\mspX{K^\bigstar}}
\newcommand\Kcorr{\compUpd{K}{\bigstar}}
%\renewcommand\Kcorr{\mspX{K^{\bigstar}}}
%\renewcommand\Kcorr{\ensuremath{{\spaR}^{}}}





\newcommand\prospa[1]{\ensuremath{\Pi#1}}
\newcommand{\kl}{\ekk\timm \ell}
\newcommand\exIntro{$\ast$}
\renewcommand\exIntro{\textit{Running example}}
\newcommand\bad{\ensuremath{\dagger}}
\newcommand\prt{\ensuremath{\partial}}
\newcommand\prtbf{\ensuremath{\boldsymbol{\partial}}}
\renewcommand\ta{\ensuremath{\mathsf{t}}}
\renewcommand\so{\ensuremath{\mathsf{s}}}
\cornersize{.5} 
\newcommand\dbox[1]{\fbox{$#1$}}
\renewcommand\dbox[1]{\ovalbox{$#1$}}

\newcommand\mmcol{\ensuremath{{M^{++}}}}
\newcommand\aacol{\ensuremath{{A^{++}}}}

\newcommand\Mplus{\ensuremath{{M^+}}}
\newcommand\Aplus{\ensuremath{{A^+}}}
\newcommand\mmplus{\Mplus}
\newcommand\aaplus{\Aplus}
\newcommand\Mpluss{\ensuremath{{M^{++}}}}
\newcommand\Apluss{\ensuremath{{A^{++}}}}

\newcommand\mmap[1]{\ensuremath{{\mathsf{m}_{#1}}}}
\newcommand\amap[1] {\ensuremath{{\mathsf{a}_{#1}}}}
\newcommand\mplus[1]{\ensuremath{{\mathsf{m}^+_{#1}}}}
\newcommand\aplus[1]{\ensuremath{{\mathsf{a}^+_{#1}}}}


\newcommand\undn{\und{n}}


\newcommand\scenum[1]{\ensuremath{\mathbf{(S#1)}}}
\newcommand\Scenum[1]{\textbf{(Scenario #1)}}
\renewcommand\Scenum[1]{(scenario \scenum{#1})}

\newcommand\xmi[1]{\ensuremath{M_{#1}}}
\newcommand\mo{\xmi{}}
\newcommand\mi{\xmi{1}}
\newcommand\mii{\xmi{2}}
\newcommand\miii{\xmi{3}}
\newcommand\xai[1]{\ensuremath{A_{#1}}}
\newcommand\yai[1]{\ensuremath{R_{#1}}}
\newcommand\ao{\xai{}}
\newcommand\ai{{\xai{1}}}
\newcommand\aii{{\xai{2}}}
\newcommand\aiii{{\xai{3}}}
\newcommand\ri{{\yai{1}}}
\newcommand\rii{{(\yai{12})}}
\newcommand\riii{{(\yai{123})}}


%-- proper names --
\newcommand\addr{\nmf{Addr}}
\newcommand\name{\nmf{name}}
\newcommand\String{\nmf{String}}
\newcommand{\Person}{\nmf{Person}}
\newcommand{\Comp}{\nmf{Company}}
\newcommand{\Company}{\nmf{Company}}
\newcommand{\Commute}{\nmf{Route}}
\newcommand{\Comm}{\nmf{Route}}
\newcommand{\Route}{\nmf{Route}}
\newcommand\Addr{\nmf{Addr}}
\newcommand\from{\nmf{from}}
\newcommand\lives{\nmf{livesAt}}
\newcommand\loc{\nmf{locAt}}
\newcommand\toattr{\nmf{to}}
%\newcommand\Empl{\nmf{Empl\textrm{-}ment}}
%\newcommand{\eer}{\nmf{empl}\textrm{-}\nmf{er}}
%\newcommand{\eee}{\nmf{empl}\textrm{-}\nmf{ee}}
\newcommand\Empl{\nmf{Employment}}
\newcommand{\eer}{\nmf{employer}}
\newcommand{\eee}{\nmf{employee}}
\newcommand{\etor}{\nmf{(e2r)}}
\newcommand{\ptop}{\nmf{(p2p)}}
\newcommand{\ctoc}{\nmf{(c2c)}}


\newcommand\namefont[1]{\ensuremath{\mathsf{#1}}}
\newcommand\nmf[1]{\namefont{#1}}
\newcommand\ittt[1]{\ensuremath\mathit{#1}} 

\newcommand{\netw}{\nmf{Network}}
\newcommand{\network}{\nmf{Network}}
\newcommand{\person}{\nmf{Person}}
\newcommand{\member}{\nmf{Member}}

\renewcommand\phone{\nmf{Phone}}
\newcommand\EMail{\nmf{Email}}
\newcommand\contact{\nmf{Contact}}
\newcommand{\topic}{\nmf{Topic}}
\newcommand{\str}{\nmf{Str}}
\renewcommand{\inv}{\nmf{inv}}
\newcommand{\PM}{\nmf{P/M}}

\newcommand{\cp}{\nmf{c/p}}
\newcommand{\memb}{\nmf{memb}}
\newcommand{\ident}{\nmf{ident}}
\newcommand{\cell}{\nmf{cell}}
\newcommand{\emails}{\nmf{emails}}
\newcommand{\logins}{\nmf{logins}}
\newcommand{\comm}{\nmf{comm}}
\newcommand{\privv}{\nmf{priv}}
%\newcommand{\from}{\nmf{from}}
\newcommand{\too}{\nmf{to}}
\newcommand{\scope}{\nmf{scope}}
\newcommand{\escope}{\nmf{e}\textrm{-}\nmf{scope}}
\newcommand{\on}{\nmf{on}}
\newcommand{\ret}{\nmf{re}}
\newcommand{\re}{\nmf{re}}
\newcommand{\subj}{\nmf{subj}}
\newcommand{\eon}{\nmf{e}\textrm{-}\nmf{on}}
%===
%\newlength{\cellH}
%\newlength{\cellW}



%=== from JSS paper
\newcommand\incal{incremental}
\newcommand\mbcon{\ensuremath{\sim}}
\newcommand\hgg[1]{}
\newcommand\info{\ensuremath{\mathrm{inf}}}



\newcommand\boldsubsubsection[1]{\subsubsection*{\textbf{#1}}}
\renewcommand\boldsubsubsection[1]{\subsubsection*{{#1}}}
\newcommand\goup{\vspace{-7.5pt}}
\newcommand\rich{\ensuremath{\mathrm{+}}}
\newcommand\poor{\ensuremath{\mathrm{-}}}
\newcommand\ohtri{\ensuremath{(\ohafra\ohafra\ohafra)}}

\newcommand\alens{\ensuremath{\lambda}}

% sub and super scripts
\newcommand\indname[1]{\ensuremath\mathrm{#1}}
\newcommand\priv{{\indname{prv}}}
\newcommand\pub{{\indname{pub}}}

\endinput

% Domain-codomain/source-target/ident
\newcommand\cod[1]{\ensuremath{{#1}^\bullet}}
\newcommand\dom[1]{\ensuremath{^\bullet{#1}}}
\newcommand\so{\ensuremath{\mathsf{src}}}
\newcommand\ta{\ensuremath{\mathsf{trg}}}
\renewcommand\so{\ensuremath{\mathsf{s}}} % was src
\renewcommand\ta{\ensuremath{\mathsf{t}}}  % was trg
\newcommand\ldom[1]{\ensuremath{$\Box #1 $}}
\newcommand\rdom[1]{\ensuremath{$#1 \Box $}}
\newcommand\id[1]{\opname{id}_{{#1}}}
\renewcommand\id{\opname{id}}


==> macros/thisPaper-llncsNew.tex <==
\newcommand\modcat{\catname{Mod}}
\newcommand\semmx[2]{\enma{\lsemm\, \mathit{#2}\,\rsemm^{#1}}}
\newcommand\semmA[1]{\semmx{A}{#1}}
\newcommand\semmB[1]{\semmx{B}{#1}}
\newcommand\semmX[1]{\semmx{X}{#1}}
\newcommand\semmAp[1]{\semmx{A'}{#1}}
\newcommand\semmBp[1]{\semmx{B'}{#1}}
\newcommand\semmXp[1]{\semmx{X'}{#1}}

\newcommand\bxl{BX\enma{_\mathrm{L}}}%\hfill}}
\newcommand\Bx{Bx\ }%\hfill}}
\newcommand\Bxs{BX}%\hfill}}
\newcommand\mlo{ML$_{\mathsf{noBp}}$}
\newcommand\mlbp{ML}%$_{\mathsf{bp}}$}
\newcommand\Bxo{\Bx}%$_{\mathsf{no{-}ev}}$}
\newcommand\Bxev{\Bx$_{\mathsf{Ev}}$}

%--> new theorems and such
% strange but for compy style, a;; macros below are needed
% but for llncs, on four of them
%-----
%\newtheorem{example}{{\em Example}}
\newtheorem{propo}{Proposition}
%\newtheorem{remark}{Remark}
%\newtheorem{theorem}{Theorem}
%\newtheorem{defin}{Definition}
\newtheorem{constr}{Construction}
%\newtheorem{constr}[defin]{Construction}
%\newtheorem{lemma}{Lemma}
\newtheorem{coro}{Corollary}
\newtheorem{discuss}{Discussion}
%\newenvironment{proof}{{\em Proof.}}{\qed\par\smallskip\indent}
%\newcommand\qed{\hbox to 0.45\textwidth {\hfill $\square$}}
%===

\newcommand\emno{} % created to easily remove many {\em xxxx} in the compy style defs
\newcommand\minusspaprop{\enma{
\begin{array}{l}
	{-}\mathsf{space}
	\\ [-7.5pt]
	\mathsf{properties}
\end{array}
}%>{\qqquad(4)}
}

\newcommand\nivv{\enma{\mathpzc{v}}}
\newcommand\spXXcodi{\enma{\spXX^0}}
\renewcommand\spXXcodi{\enma{||\spXX||}}
\newcommand\spapro{\enma{\footnotesize{\mathrm{spaceProp.}}}}
\newcommand\minusspa{\enma{({-}\spapro)}}
\newcommand\arrows{\enma{\mathsf{arrows}}}
\newcommand\paracaterr{\paracatx{\err}}
\newcommand\ints{\enma{\mathbb{N}}}
% + put and Co stuff
\newcommand\ponix{\enma{\breve{\nix}}}
\renewcommand\ponix{\enma{\ovr{\nix}}}
\renewcommand\ponix{\enma{\pi\!\nix}}
\renewcommand\ponix{\nix}
%\renewcommand\onix{\enma{\widetilde{\nix}}}
%\renewcommand\onix{\enma{\widehat{\nix}}}
%\renewcommand\onix{\enma{\stackrel{\circ}{\nix}}}

\newcommand\xyz{\enma{\mathsf{xxx}}}
\newcommand\lowlowindex[2]{\enma{#1_{\!_{#2}}}}
%\renewcommand\lowlowindex[2]{\enma{#1_{{#2}}}}

\newcommand\lowindxyz[3]{\enma{#1_{#2_{#3}}}}
%\renewcommand\lowlowindex[2]{\enma{#1_{{#2}}}}
\newcommand\plusx[1]{\lowlowindex{+}{#1}}
%\newcommand\plusx[1]{\lowindxyz{+}{}{#1}}
\newcommand\minusx[1]{\lowlowindex{-}{#1}}
\newcommand\minusnix{\enma{{-}\nix}}
\newcommand\minusnixbra{\enma{[{-}\nix]}}
\newcommand\minusnixcodi{\enma{({-}\nix)^0}}
\newcommand\minusnixcodibra{\enma{[({-}\nix)^0]}}
\newcommand\minusput{\enma{{-}\putl}}
\newcommand\minusdif{\enma{{-}\dif}}
\newcommand\minuswbdif{\enma{{-}\mathrm{wbdif}}}
	\renewcommand\minuswbdif{\enma{{-}\mathrm{Difputdif}}}
\newcommand\minusputcodi{\enma{{-}\putl^0}}
%\newcommand\minusx[1]{\enma{-_{\!_{#1}}}}
\newcommand\congx[1]{\lowlowindex{\cong}{#1}}

\newcommand\plusputx[1]{\enma{\plusx{#1}\putl}}
% + dif
\newcommand\plusxput{\enma{\plusx{\ponix}\putl}} 
\newcommand\plusxputcodi{\enma{\plusxput^0}} 
\newcommand\plusxdif{\enma{\plusx{\ponix}\dif}} 
\newcommand\plusxdel{\enma{\plusx{\ponix}\deltas}} 
%  delta
\newcommand\plusdelx[1]{\enma{\plusx{#1}\deltas}}
\newcommand\plusarrx[1]{\enma{\plusx{#1}\mathsf{arr}}}



%\newcommand\plusdifx[1]{\enma{\plusx{#1}\dif}}
%\newcommand\plusxdif{\plusdifx{\ponix}} 
%\newcommand\minusdifx[1]{\enma{\minusx{#1}\dif}}
\newcommand\minusxdel{\minusx{\ponix}\deltas}

% colors
\newcommand\diff{\enma{\diagopername{diff}}}
\newcommand\diffind{\enma{\diagopername{diff}}}
\newcommand\differ{\enma{\diagopername{differ}}}
\newcommand\pairing{\enma{\diagopername{pairing}}}
\newcommand\lens{\enma{\diagopername{lens}}}
\newcommand\grt[1]{\textcolor{caribbeangreen}{#1}}
\newcommand\grgrt[1]{\textcolor{caribbeangreen}{#1}}
\newcommand\blt[1]{\textcolor{blue}{#1}}
\newcommand\redt[1]{\textcolor{red}{#1}}

%\newcommand\plusxdel[1]{\enma{\plusx{#1}\deltas}}
%\newcoo
%\newcommand\lensarrp


%\newcommand\plusxdel{\plusdelx{\onix}} 

\newcommand\pind{\enma{\tilde{p}}}
\newcommand\odash{\enma{\circleddash}}
\newcommand\ovre{\ovr{e}}
\newcommand\medxyz[3]{\enma{#1^{#2#3}}}  % #1 is arg, #2 delta, #3 fun
\newcommand\medaxy[2]{\medxyz{a}{#1}{#2}}
\newcommand\medfxy[2]{\medxyz{#1}{#2}{f}}
\newcommand\medadx[1]{\medxyz{a}{\del}{#1}}
\newcommand\medafx[1]{\medxyz{a}{#1}{f}}

	\newcommand\medxy[2]{\enma{{#1}^{\prt{#2}}}}
	%\renewcommand\medxy[2]{\medxyz{}{}}
	\newcommand\medfx[1]{\medxy{#1}{f}}
	
			\newcommand\getobx[1]{\enma{|\get|_{#1}}}
	\newcommand\getobp{\getobx{p}}
	
	
\newcommand\Del{\enma{\mathit{\Delta}}}
\newcommand\Dela{\enma{\Delta_a}}
\newcommand\Delp{\enma{\Delta_p}}
\newcommand\ffun{\enma{\mathbf{f}}}
\renewcommand\ffun{\enma{\widehat{f}}}
\newcommand\DDel{\enma{{\pmb \Delta}}}
\newcommand\DDela{\enma{{\pmb \Delta}_\spA}}
\newcommand\DDelb{\enma{{\pmb \Delta}_\spB}}
\newcommand\del{\enma{\delta}}
%\renewcommand\del{\Del}
\newcommand\dela{\enma{\delta_a}}
\newcommand\della{\enma{\hat{\del}}}
\newcommand\dellp{\enma{\check{\del}}}
\newcommand\delb{\enma{\delta_b}}
\newcommand\jacobx[1]{\enma{\mathbf{J}#1}}
\newcommand\jacobf{\jacobx{f}}
\newcommand\prtx[1]{\enma{\prt #1}}
\newcommand\prtf{\prtx{f}}
\renewcommand\cod{\diagopername{cod}}
\renewcommand\cod{\diagopername{codomain}}
\newcommand\fu{\nmf{f}}
\newcommand\wi{\nmf{w}}
\newcommand\emb{\nmf{e}}
\newcommand\rcat{\enma{\mathbf{R}}}
\newcommand\bx{BX}%\hfill}}
\newcommand\alalens{ala-lens}
\newcommand\Alalens{Ala-lens}
\newcommand\alaalens{alaa-lens}
\newcommand\Alalaens{Alaa-lens}
%\newcommand\mlo{ML$_{\mathsf{noBp}}$}
%\newcommand\mlbp{ML}%$_{\mathsf{bp}}$}
\newcommand\bxo{Bx}%$_{\mathsf{no{-}ev}}$}
\newcommand\bxev{Bx$_{\mathsf{Ev}}$}

\newcommand\warr{\enma{\rightsquigarrow}}
\newcommand\warrxy[2]{\enma{#1\warr#2}}
\newcommand\warraa{\warrxy{a}{a'}} 
\newcommand\warrbb{\warrxy{b}{b'}}
\newcommand\warrbba{\warrxy{b'}{b'^@}}
\newcommand\warrpp{\warrxy{p}{p'}}

\newcommand\byx[1]{\mbox{\quad #1}}
\newcommand\byeq[2]{\mbox{\quad #1 \eqref{#2}}}
\newcommand\byeqna[2]{\mbox{\quad #1 \eqref{eqna-#2}}}
\newcommand\byeqnaa[3]{\mbox{\quad #1 \eqref{eqna-#2}~#3  }}

%\renewcommand\xxx{\enma{\mathsf{xxx}}}
\renewcommand\xob[1]{\enma{|#1|}}
\newcommand\Arr{\enma{\mathsf{Arr}}}
\newcommand\elll{\enma{\ell}}
\newcommand\vii{\enma{v^{}}}
\newcommand\uiii{\enma{u^{}}}
\newcommand\viii{\enma{v^{@}}}
\newcommand\niget{\enma{\mathpzc{get}}}
\newcommand\nifo[1]{\enma{\mathcal{#1}}}
%\newcommand\nim{\nifo{M}}
\newcommand\nin{\nifo{N}}
%\newcommand\defcat{\catfont{Def}}
\newcommand\defcat{\enma{\mathpzc{Def}}}
\newcommand\vbf{\enma{\mathbf{v}}}
\newcommand\smm{symmetric monoidal}
\newcommand\sm{sm}
\newcommand\ome{\enma{\omega}}
\newcommand\isop{\enma{\iota}}
\newcommand\hell{\enma{\hat\ell}}
\newcommand\hp{{\enma{\hat p}}}
\renewcommand\hp{{\enma{\isop(p)}}}
\newcommand\hget{\enma{\widehat{\get}}}
\newcommand\hputl{\enma{\widehat{\putl}}}

\newcommand\Err{\nmf{Err}}
\newcommand\rreals{\enma{\reals\timm\reals}}
\newcommand\prtfrac[2]{\enma{\frac{\prt#1}{\prt#2}}}
\newcommand\breals{\enma{\mathbf{R}}}
\newcommand\enma[1]{{\ensuremath{#1}}}
\newcommand\brealsx[1]{\enma{\mathbf{R}^{#1}}}
\newcommand\rcatx[1]{\enma{\rcat^{{#1}}}}
\newcommand\realsx[1]{\enma{\mathbb{R}^{#1}}}
%\renewcommand\xob[1]{\enma{|#1|}}
%\newcommand\bx{Bx}
\renewcommand\f{\enma{I(p,\_)}}
\newcommand\parr{parameter}
\newcommand\parrd{parameterized}
\newcommand\Parrd{Parameterized}
\newcommand\parrn{parameterization}
\newcommand\Parrn{Parameterization}
\newcommand\pard{parameterized}
\newcommand\Pard{Parameterized}
\newcommand\parn{parameterization}
\newcommand\Parn{Parameterization}


\newcommand\Reals{\enma{\mathbb{R}}}
\newcommand\reals{\enma{\mathbb{R}}}
%\newcommand\realsx[1]{\enma{\mathbb{R}^{{#1}}}
\newcommand\prpol{\nmf{policy}}
\newcommand\pol{\nmf{pol}}
\newcommand\Pol{\nmf{Pol}}
\newcommand\ipol{\nmf{inv}}
\renewcommand\pol{\enma{\mathit{pol}}}

\newcommand\err{\nmf{err}}
\newcommand\rre{\nmf{r\!r\!e}}
\newcommand\errx{\nmf{errx}}
\newcommand\sym{\nmf{sym}}
\newcommand\eps{\enma{\varepsilon}}
\newcommand\ptol{\catname{p2l}}
\newcommand\aplenscat{\catname{alLens}}
\newcommand\apalenscat{\catname{aaLLens}}
\newcommand\allenscat{\catname{alLens}}
\newcommand\alalenscat{\catname{alaLens}}
\newcommand\aladlenscat{\catname{alaLensDif}}
\newcommand\alalenscatcodi{\enma{\catname{alaLens}}\!\,\mbox{\bf\em 0}}
\renewcommand\alalenscatcodi{\enma{\catname{alaLens}^0}}
\newcommand\pgetnixcatcodi{\enma{\catname{pGet}_\nix^0}}
\newcommand\putlcodi{\enma{\putl^0}}
\newcommand\allenscatcodi{\enma{\catname{alLens}^0}}
\newcommand\alalensdifcat{\catname{alaLensDif}}
\newcommand\alalenscatdif{\alalensdifcat}
\newcommand\diffcat{\catname{Dif\!f}}
% amedamend
\newcommand\alaalenscat{\catname{alaaLens}}
\newcommand\alaalenscatcodi{\enma{\catname{alaaLens}}\!\,\mbox{\bf\em 0}}
\newcommand\alaalenscatdif{\catname{alaaLensDif}}
\newcommand\codiscr{\diagopername{codiscr}}
\renewcommand\codiscr{\catname{codiscr}}
\newcommand\codifun{\codiscr}
\newcommand\pgetcat{\catname{pGet}}
\newcommand\pgetdifcat{\catname{pGetDif}}
\newcommand\pgetcatnix{\enma{\pgetcat_\nix}} %catname{pGet}}

\newcommand\lift{\nmf{lift}}
\newcommand\fun{\nmf{fun}}
\newcommand\grd{\nmf{grd}}
\newcommand\Grd{\nmf{Grd}}
\newcommand\gdbp{\nmf{GdBp}}
\newcommand\gd{\nmf{Gd}}
\renewcommand\lawnamebr[1]{\lawname{(#1)}}
\newcommand\amend{amendment}
\newcommand\prop{proposition}
\newcommand\icorr{\ensuremath{\mathsf{indCorr}}}
\newcommand\lner{learner}
\newcommand\Lner{Learner}
\newcommand\learncat{\catname{Learn}}
\newcommand\learnfun{\catname{learner}}
\newcommand\learncatcon{\enma{\mathbb{L}\mathbf{earn}}}
\newcommand\paracatcon{\enma{\mathbb{P}\mathbf{ara}}}
%\newcommand\learnfun{\catname{learner}}




\newcommand\bxfun{\catname{bx}}
\newcommand\bxcat{\catname{PView}}
\newcommand\ptracat{\catname{PTransf}}
\newcommand\tracat{\catname{Transf}}
\newcommand\pviewcat{\catname{PGet}}
\newcommand\viewcat{\catname{Get}}

\newcommand\paarr{\enma{\;\paar\;}} 
\newcommand\lm{\enma{\ell;\emm}}
\newcommand\lmbr{\enma{(\ell;\emm)}}
\newcommand\paarrx[1]{\paarr} %\enma{\;\paar^{#1}\;  }}

\newcommand\paar{\enma{\!\,|\!|}}
\renewcommand\ll{\enma{\ell_1\!|\!|\ell_2}}
\newcommand\pp{{p_1\paar p_2}}
\renewcommand\ss{{S_1\paar S_2}}

\renewcommand\ll{\enma{\ell_1\paar\ell_2}}
\newcommand\llbr{\enma{(\ll)}}
\newcommand\putpsi{\putxyz{(1)}{p_1}{S_1}}
\newcommand\putpsii{\putxyz{(2)}{p_2}{S_2}}
\newcommand\getpi{\getxy{{\ell_1}}{{p_1}}} 
\newcommand\getpii{\getxy{{\ell_2}}{p_2}}
\newcommand\difputdif{\lawname{Difputdif}}
\renewcommand\difputlaw{\lawname{Difput}} % must be the same
\newcommand\catcattimm{\enma{(\catcat,\!\timm)}}
\newcommand\setcattimm{\enma{(\setcat,\!\timm)}}
\newcommand\Hom{\enma{\mathit{Hom}}}
\newcommand\codd{\enma{\mathsf{cod}}}
\newcommand\xcatcat[1]{\enma{\catname{#1}\catname{Cat}}}
\newcommand\pcatcat{\catname{pCat}}
\newcommand\smcatcat{\catname{smCat}}
\newcommand\qcatcat{\catname{QCat}}
\newcommand\pcatcatdif{\catname{pCatDif}}
\newcommand\pspadifcat{\catname{pSpaceDif}}
\newcommand\psetcat{\catname{pSet}}
\newcommand\paracat{\catname{Para}}
\newcommand\paracatre{\catname{Para_\reals}}
\newcommand\paracatrcat{\catname{Para_\rcat}}
  \newcommand\fbf{\enma{\pmb f}}
\newcommand\leefun{\enma{L_{\eps,\err}}}
\newcommand\leefunovr{\ovr{\leefun}}
\newcommand\pfuncat{\catname{pFun}}
\newcommand\pmtcat{\catname{pTransf}}
\newcommand\lnercat{\learncat}
\newcommand\slenscat{\catname{sLens}}
\newcommand\alenscat{\catname{aLens}}
\newcommand\alenscattgg{\mathbb{V}\catname{TGGLens}}
\newcommand\viewcattgg{\mathbb{V}\catname{iewTGG}}
\newcommand\bprules{\nmf{Rules}}
\newcommand\bppol{\nmf{bpPolicy}}
\newcommand\mboxsmall[1]{\mbox{\small#1}}


\newcommand\aalenscat{\catname{aaLens}}
\renewcommand\apalenscat{\catname{alaLens}}
\renewcommand\alalenscat{\catname{alaLens}}
\newcommand\ltol{\catname{l2l}}
\newcommand\pq{\enma{{pq}}}
\newcommand\eh{\enma{{eh}}}
\newcommand\klbr{\enma{(\kl)}}

\newcommand\citell{\cite{ll-bx19}[ll@bx19]}



% Must add these macros here, because tex does not compile, if they are moved to macro files
\newcommand\figri{} 
\newcommand\figrii{}
\newcommand\figriii{}
\newcommand\figriia{}
\newcommand\figriv{}
\newcommand\figrv{}
\newcommand\PP{\ensuremath{\mathit{PUT}}}
\newcommand\figrsdlens{Fig.??}
\newcommand\diarefi{}
\newcommand\diarefii{}
\newcommand\diarefiii{}

\newcommand\putgeto{\enma{\putget_0}}

%\newcommand\putxyz[3]{\ensuremath{#3.\putl^{(#1,#2)}}}
\newcommand\putxyz[3]{\ensuremath{\putl^{#1}_{{#2},{#3}}}}
\newcommand\putUL[2]{\ensuremath{\putl^{#1}_{#2}}}
\newcommand\getxy[2]{\ensuremath{\get^{{#1}}_{{#2}} }}
\newcommand\putqbx[1]{\putxyz{#1}{q}{B_p}}
%\newcommand\putqb{\putxy{q}{B}}
\newcommand\puthatxy[2]{\ensuremath{\widehat{\putl}^{(#1,#2)}}}

\newcommand\putxy[2]{\ensuremath{\putl_{(#1,#2)}}}
\renewcommand\putxy[2]{\ensuremath{\putl_{#1,#2}}}
\newcommand\putpa{\putxy{p}{A}}
\newcommand\putqb{\putxy{q}{B}}
\newcommand\putps{\putxy{p}{S}}
\newcommand\putqbp{\putxy{q}{B_p}}
%\newcommand\putqb{\putxy{q}{B}}
%--- for gets
\newcommand\gettxy[2]{\ensuremath{\get_{#1,#2}}}
\newcommand\getamxy[2]{\ensuremath{\get^{@}_{#1,#2}}}
%\renewcommand\putxy[2]{\ensuremath{\putl_{#1,#2}}}
\newcommand\getpa{\gettxy{p}{A}}
\newcommand\getqb{\gettxy{q}{B}}
\newcommand\getps{\gettxy{p}{S}}
\newcommand\getamps{\getamxy{p}{S}}

\newcommand\xdeldel[3]{\enma{#1_{#2,#3}}}
\newcommand\sue{\xdeldel{S}{u}{e}}



\renewcommand\indb{\ensuremath{\mathsf{req}}}
\newcommand\upd{\ensuremath{\mathsf{upd}}}
\newcommand\req{\ensuremath{\mathsf{req}}}
\renewcommand\self{\ensuremath{\mathsf{self}}}

\newcommand\niuu{\ensuremath{\mathbf{u}}}
\newcommand\thissec{\ref{sec:somesection}}
\newcommand\fakeob{\strut}
\newcommand\npmargin[1]{\mymarginnew{NewSubsect\# #1}}
\newcommand\npmarginn[2]{\mymarginNew{NewSubsect\##1}{#2}}

\renewcommand\x{\enma{\mathbf{x}}}

\renewcommand\newpi[2]{\hlight{#1}{NewPiece\#\! #2}}
\renewcommand\newpii[3]{\hlightNew{#1}{NewPiece\#\! #2}{#3}}
\newcommand\newsec[3]{\hlightNew{#1}{This is entirely new sect\! #2}{#3}}

\newcommand\prodx[1]{\ensuremath{\small{\prod}\!#1}}
\renewcommand\xstar[1]{\Corrsx{#1}}
%\renewcommand\xob[1]{\ensuremath{\mathsf{Ob}(#1)}}

\renewcommand\R[1]{\ensuremath{\mspA^{\bigstar}_{#1}}}
\renewcommand\xarr[1]{\ensuremath{#1%
		^{\footnotesize{\RHD}}}}
	\renewcommand\xarr[1]{\ensuremath{#1%
			^{\mathbf{\rightarrow}}}}
\renewcommand\xarr[1]{\ensuremath{\mathsf{Ar}(#1)}}
\newcommand\xar[1]{\ensuremath{\mathsf{Ar}(#1)}}

\newcommand\setop{\ensuremath{\diagopername{set}}}
\newcommand\Corrsx[1]{\ensuremath{#1^\bigstar}}
\renewcommand\Corrsx[1]{\ensuremath{\mathsf{Corr}(#1)}}
\newcommand\corrsx[1]{\ensuremath{\mathsf{corr}(#1)}}
\newcommand\Corrsma{\Corrsx{\mspA}}
\newcommand\Corrsa{\Corrsx{\spA}}
\newcommand\Korrsma{\Corrsx{\spK}}
\newcommand\corr{\ensuremath{\mathsf{corr}}}
\newcommand\corrx[1]{\corrsx{#1}}
\newcommand\Corr{\ensuremath{\mathsf{Corr}}}
\newcommand\Corrcat{\ensuremath{\mathbf{Corr}}}
\newcommand\Corrx[1]{\Corrsx{#1}}

\newcommand\amdx[1]{\ensuremath{#1^{@}}}
\newcommand\amex[1]{\amdx{#1}}
\newcommand\ameui{\amex{u_i}}

\newcommand\reflectzero{Reflect0}

\newcommand\kputput{\lawname{KPutput}}
\newcommand\kputputlaw{\lawname{\kputput} law}
\newcommand\ppgrx[1]{\ensuremath{\ppg^{#1}}}
\newcommand\ppgr{\ppgrx{\acorr}}
\newcommand\ppgB{\ppgrx{B}}
\newcommand\ppghB{\ppgrx{\hat B}}

\newcommand\elementToSingleton[1]{\ensuremath{\widehat{#1}}}
\newcommand\etosing[1]{\elementToSingleton{#1}}
\newcommand\sing{\ensuremath{\mathrm{sing}}}
\newcommand\prosing{\ensuremath{\prod}}
\newcommand\allm{\ensuremath{(M_{123})}}
\newcommand\spE{\ensuremath{\spacenam{E}}}
%-- the upper taken from macros-general
\renewcommand\comprfam[2]{\left(\mathstrut{#1}\left|\;{#2}\right.)}
\renewcommand\comprfam[2]{\left(\mathstrut{#1}\,| \;{#2}\right)}
%\renewcommand\comprfam[2]{\left(\mathstrut{#1}\right)_{{#2}}}

%= tuples
\newcommand\tuplenam[1]{\ensuremath{\pmb{#1}}}
\renewcommand\tuplenam[1]{\ensuremath{{#1}}}
\newcommand\tupX[1]{\ensuremath{\tuplenam{#1}}}
\newcommand\tupA{\tupX{A}}
\newcommand\tupu{\tupX{u}}
\newcommand\tupB{\tupX{B}}
\newcommand\tupv{\tupX{v}}

\newcommand\prodX[1]{\ensuremath{\prtbf^{\Pi}\!\!#1}}
\renewcommand\prodX[1]{\ensuremath{#1^{\Pi}}}
\newcommand\prodmspA{\prodX{\mspA}}
\newcommand\prodmspB{\prodX{\mspB}}

\newcommand\bounX[1]{\ensuremath{\prtbf#1}}
\newcommand\bounmspA{\bounX{\mspA}}




\newcommand\xconfig[1]{\ensuremath{\mathsf{#1}}}
\newcommand\Span{\xconfig{Span}}
\newcommand\Cospan{\xconfig{Cospan}}
%\newcommand\K{\spaR}
% -- conseq compatible updates
\newcommand\compUpd[2]{\ensuremath{\mathsf{#1}^{{#2}}}}
\newcommand\seqK{\compUpd{K}{\RHD\!\!\RHD}}
\newcommand\parK{\compUpd{K}{{|}{|}{}}}
\newcommand\spanK[1]{\compUpd{K}{\blacktriangle{#1}}}
\newcommand\disjK[1]{\compUpd{K}{\blacktriangle{#1}}}
\newcommand\Kupd{\seqK}
\newcommand\Kseq{\seqK}
%--space of conflict-free/concurr compatible updates
\newcommand\cofrK{\parK}

\newcommand\Kpar{\parK}
\newcommand\Kspan[1]{\spanK{#1}}
\newcommand\Kdisj[1]{\disjK{#1}}

%\endinput

% space of consist corrs
\newcommand\consK{\mspX{K^\bigstar}}
\newcommand\Kcorr{\compUpd{K}{\bigstar}}
%\renewcommand\Kcorr{\mspX{K^{\bigstar}}}
%\renewcommand\Kcorr{\ensuremath{{\spaR}^{}}}






\newcommand\prospa[1]{\ensuremath{\Pi#1}}
\newcommand\exIntro{$\ast$}
\renewcommand\exIntro{\textit{Running example}}
\newcommand\bad{\ensuremath{\dagger}}
\newcommand\prt{\ensuremath{\partial}}
\newcommand\prtbf{\ensuremath{\boldsymbol{\partial}}}
\renewcommand\ta{\ensuremath{\mathsf{t}}}
\renewcommand\so{\ensuremath{\mathsf{s}}}
\cornersize{.5} 
\newcommand\dbox[1]{\fbox{$#1$}}
\renewcommand\dbox[1]{\ovalbox{$#1$}}

\newcommand\mmcol{\ensuremath{{M^{++}}}}
\newcommand\aacol{\ensuremath{{A^{++}}}}

\newcommand\Mplus{\ensuremath{{M^+}}}
\newcommand\Aplus{\ensuremath{{A^+}}}
\newcommand\mmplus{\Mplus}
\newcommand\aaplus{\Aplus}
\newcommand\Mpluss{\ensuremath{{M^{++}}}}
\newcommand\Apluss{\ensuremath{{A^{++}}}}

\newcommand\mmap[1]{\ensuremath{{\mathsf{m}_{#1}}}}
\newcommand\amap[1] {\ensuremath{{\mathsf{a}_{#1}}}}
\newcommand\mplus[1]{\ensuremath{{\mathsf{m}^+_{#1}}}}
\newcommand\aplus[1]{\ensuremath{{\mathsf{a}^+_{#1}}}}


\newcommand\undn{\und{n}}


\newcommand\scenum[1]{\ensuremath{\mathbf{(S#1)}}}
\newcommand\Scenum[1]{\textbf{(Scenario #1)}}
\renewcommand\Scenum[1]{(scenario \scenum{#1})}

\newcommand\xmi[1]{\ensuremath{M_{#1}}}
\newcommand\mo{\xmi{}}
\newcommand\mi{\xmi{1}}
\newcommand\mii{\xmi{2}}
\newcommand\miii{\xmi{3}}
\newcommand\xai[1]{\ensuremath{A_{#1}}}
\newcommand\yai[1]{\ensuremath{R_{#1}}}
\newcommand\ao{\xai{}}
\newcommand\ai{{\xai{1}}}
\newcommand\aii{{\xai{2}}}
\newcommand\aiii{{\xai{3}}}
\newcommand\ri{{\yai{1}}}
\newcommand\rii{{(\yai{12})}}
\newcommand\riii{{(\yai{123})}}


%-- proper names --
\newcommand\addr{\nmf{Addr}}
\newcommand\name{\nmf{name}}
\newcommand\String{\nmf{String}}
\newcommand{\Person}{\nmf{Person}}
\newcommand{\Comp}{\nmf{Company}}
\newcommand{\Company}{\nmf{Company}}
\newcommand{\Commute}{\nmf{Route}}
\newcommand{\Comm}{\nmf{Route}}
\newcommand{\Route}{\nmf{Route}}
\newcommand\Addr{\nmf{Addr}}
\newcommand\from{\nmf{from}}
\newcommand\lives{\nmf{livesAt}}
\newcommand\loc{\nmf{locAt}}
\newcommand\toattr{\nmf{to}}
%\newcommand\Empl{\nmf{Empl\textrm{-}ment}}
%\newcommand{\eer}{\nmf{empl}\textrm{-}\nmf{er}}
%\newcommand{\eee}{\nmf{empl}\textrm{-}\nmf{ee}}
\newcommand\Empl{\nmf{Employment}}
\newcommand{\eer}{\nmf{employer}}
\newcommand{\eee}{\nmf{employee}}
\newcommand{\etor}{\nmf{(e2r)}}
\newcommand{\ptop}{\nmf{(p2p)}}
\newcommand{\ctoc}{\nmf{(c2c)}}


\newcommand\namefont[1]{\ensuremath{\mathsf{#1}}}
\newcommand\nmf[1]{\namefont{#1}}
\newcommand\ittt[1]{\ensuremath\mathit{#1}} 

\newcommand{\netw}{\nmf{Network}}
\newcommand{\network}{\nmf{Network}}
\newcommand{\person}{\nmf{Person}}
\newcommand{\member}{\nmf{Member}}

\renewcommand\phone{\nmf{Phone}}
\newcommand\EMail{\nmf{Email}}
\newcommand\contact{\nmf{Contact}}
\newcommand{\topic}{\nmf{Topic}}
\newcommand{\str}{\nmf{Str}}
\renewcommand{\inv}{\nmf{inv}}
\newcommand{\PM}{\nmf{P/M}}

\newcommand{\cp}{\nmf{c/p}}
\newcommand{\memb}{\nmf{memb}}
\newcommand{\ident}{\nmf{ident}}
\newcommand{\cell}{\nmf{cell}}
\newcommand{\emails}{\nmf{emails}}
\newcommand{\logins}{\nmf{logins}}
\newcommand{\comm}{\nmf{comm}}
\newcommand{\privv}{\nmf{priv}}
%\newcommand{\from}{\nmf{from}}
\newcommand{\too}{\nmf{to}}
\newcommand{\scope}{\nmf{scope}}
\newcommand{\escope}{\nmf{e}\textrm{-}\nmf{scope}}
\newcommand{\on}{\nmf{on}}
\newcommand{\ret}{\nmf{re}}
\newcommand{\re}{\nmf{re}}
\newcommand{\subj}{\nmf{subj}}
\newcommand{\eon}{\nmf{e}\textrm{-}\nmf{on}}
%===
%\newlength{\cellH}
%\newlength{\cellW}



%=== from JSS paper
\newcommand\incal{incremental}
\newcommand\mbcon{\ensuremath{\sim}}
\newcommand\hgg[1]{}
\newcommand\info{\ensuremath{\mathrm{inf}}}

\newcommand\boldsubsubsection[1]{\subsubsection*{\textbf{#1}}}
\renewcommand\boldsubsubsection[1]{\subsubsection*{{#1}}}
\newcommand\goup{\vspace{-7.5pt}}
\newcommand\rich{\ensuremath{\mathrm{+}}}
\newcommand\poor{\ensuremath{\mathrm{-}}}
\newcommand\ohtri{\ensuremath{(\ohafra\ohafra\ohafra)}}

\newcommand\alens{\ensuremath{\lambda}}

% sub and super scripts
\newcommand\indname[1]{\ensuremath\mathrm{#1}}
\newcommand\priv{{\indname{prv}}}
\newcommand\pub{{\indname{pub}}}

\endinput

% Domain-codomain/source-target/ident
\newcommand\cod[1]{\ensuremath{{#1}^\bullet}}
\newcommand\dom[1]{\ensuremath{^\bullet{#1}}}
\newcommand\so{\ensuremath{\mathsf{src}}}
\newcommand\ta{\ensuremath{\mathsf{trg}}}
\renewcommand\so{\ensuremath{\mathsf{s}}} % was src
\renewcommand\ta{\ensuremath{\mathsf{t}}}  % was trg
\newcommand\ldom[1]{\ensuremath{$\Box #1 $}}
\newcommand\rdom[1]{\ensuremath{$#1 \Box $}}
\newcommand\id[1]{\opname{id}_{{#1}}}
\renewcommand\id{\opname{id}}


==> macros/thisPaper.tex <==
% Must add these macros here, because tex does not compile, if they are moved to macro files
\newcommand\figri{} 
\newcommand\figrii{}
\newcommand\figriii{}
\newcommand\figriia{}
\newcommand\figriv{}
\newcommand\figrv{}
\newcommand\PP{\ensuremath{\mathit{PUT}}}
\newcommand\figrsdlens{Fig.??}


\newcommand\putxy[2]{\ensuremath{\putl^{(#1,#2)}}}
\newcommand\putpa{\putxy{p}{A}}
\newcommand\putqb{\putxy{q}{B}}
\renewcommand\indb{\ensuremath{\mathsf{req}}}
\newcommand\upd{\ensuremath{\mathsf{Upd}}}
\newcommand\req{\ensuremath{\mathsf{req}}}
\renewcommand\self{\ensuremath{\mathsf{self}}}

\newcommand\niuu{\ensuremath{\mathcal{u}}}
\newcommand\thissec{\ref{sec:somesection}}
\newcommand\fakeob{\strut}
\newcommand\npmargin[1]{\mymarginnew{NewSubsect\# #1}}
\newcommand\npmarginn[2]{\mymarginNew{NewSubsect\##1}{#2}}

\renewcommand\newpi[2]{\hlight{#1}{NewPiece\#\! #2}}
\newcommand\newsec[3]{\hlightNew{#1}{This is entirely new sect\! #2}{#3}}
\renewcommand\newpii[3]{\hlightNew{#1}{NewPiece\#\! #2}{#3}}
\newcommand\prodx[1]{\ensuremath{\small{\prod}\!#1}}
\renewcommand\xstar[1]{\Corrsx{#1}}
\renewcommand\xob[1]{\ensuremath{\mathsf{Ob}(#1)}}

\renewcommand\R[1]{\ensuremath{\mspA^{\bigstar}_{#1}}}
\renewcommand\xarr[1]{\ensuremath{#1%
		^{\footnotesize{\RHD}}}}
	\renewcommand\xarr[1]{\ensuremath{#1%
			^{\mathbf{\rightarrow}}}}
\renewcommand\xarr[1]{\ensuremath{\mathsf{Ar}(#1)}}

\newcommand\setop{\ensuremath{\diagopername{set}}}
\newcommand\Corrsx[1]{\ensuremath{#1^\bigstar}}
\renewcommand\Corrsx[1]{\ensuremath{\mathsf{Corr}(#1)}}
\newcommand\corrsx[1]{\ensuremath{\mathsf{corr}(#1)}}
\newcommand\Corrsma{\Corrsx{\mspA}}
\newcommand\Corrsa{\Corrsx{\spA}}
\newcommand\Korrsma{\Corrsx{\spK}}
\newcommand\corr{\ensuremath{\mathsf{corr}}}
\newcommand\corrx[1]{\corrsx{#1}}
\newcommand\Corr{\ensuremath{\mathsf{Corr}}}
\newcommand\Corrcat{\ensuremath{\mathbf{Corr}}}
\newcommand\Corrx[1]{\Corrsx{#1}}
\newcommand\Korr{\ensuremath{\mathsf{K}}}

\newcommand\amdx[1]{\ensuremath{#1^{@}}}
\newcommand\amex[1]{\amdx{#1}}
\newcommand\ameui{\amex{u_i}}

\newcommand\reflectzero{Reflect0}

\newcommand\kputput{\lawname{KPutput}}
\newcommand\kputputlaw{\lawname{\kputput} law}
\newcommand\ppgrx[1]{\ensuremath{\ppg^{#1}}}
\newcommand\ppgr{\ppgrx{\acorr}}
\newcommand\ppgB{\ppgrx{B}}
\newcommand\ppghB{\ppgrx{\hat B}}

\newcommand\elementToSingleton[1]{\ensuremath{\widehat{#1}}}
\newcommand\etosing[1]{\elementToSingleton{#1}}
\newcommand\sing{\ensuremath{\mathrm{sing}}}
\newcommand\prosing{\ensuremath{\prod}}
\newcommand\allm{\ensuremath{(M_{123})}}
\newcommand\spE{\ensuremath{\spacenam{E}}}
%-- the upper taken from macros-general
\renewcommand\comprfam[2]{\left(\mathstrut{#1}\left|\;{#2}\right.)}
\renewcommand\comprfam[2]{\left(\mathstrut{#1}\,| \;{#2}\right)}
%\renewcommand\comprfam[2]{\left(\mathstrut{#1}\right)_{{#2}}}

%= tuples
\newcommand\tuplenam[1]{\ensuremath{\pmb{#1}}}
\renewcommand\tuplenam[1]{\ensuremath{{#1}}}
\newcommand\tupX[1]{\ensuremath{\tuplenam{#1}}}
\newcommand\tupA{\tupX{A}}
\newcommand\tupu{\tupX{u}}
\newcommand\tupB{\tupX{B}}
\newcommand\tupv{\tupX{v}}

\newcommand\prodX[1]{\ensuremath{\prtbf^{\Pi}\!\!#1}}
\renewcommand\prodX[1]{\ensuremath{#1^{\Pi}}}
\newcommand\prodmspA{\prodX{\mspA}}
\newcommand\prodmspB{\prodX{\mspB}}

\newcommand\bounX[1]{\ensuremath{\prtbf#1}}
\newcommand\bounmspA{\bounX{\mspA}}




\newcommand\xconfig[1]{\ensuremath{\mathsf{#1}}}
\newcommand\Span{\xconfig{Span}}
\newcommand\Cospan{\xconfig{Cospan}}
%\newcommand\K{\spaR}
% -- conseq compatible updates
\newcommand\compUpd[2]{\ensuremath{\mathsf{#1}^{{#2}}}}
\newcommand\seqK{\compUpd{K}{\RHD\!\!\RHD}}
\newcommand\parK{\compUpd{K}{{|}{|}{}}}
\newcommand\spanK[1]{\compUpd{K}{\blacktriangle{#1}}}
\newcommand\disjK[1]{\compUpd{K}{\blacktriangle{#1}}}
\newcommand\Kupd{\seqK}
\newcommand\Kseq{\seqK}
%--space of conflict-free/concurr compatible updates
\newcommand\cofrK{\parK}

\newcommand\Kpar{\parK}
\newcommand\Kspan[1]{\spanK{#1}}
\newcommand\Kdisj[1]{\disjK{#1}}

%\endinput

% space of consist corrs
\newcommand\consK{\mspX{K^\bigstar}}
\newcommand\Kcorr{\compUpd{K}{\bigstar}}
%\renewcommand\Kcorr{\mspX{K^{\bigstar}}}
%\renewcommand\Kcorr{\ensuremath{{\spaR}^{}}}





\newcommand\prospa[1]{\ensuremath{\Pi#1}}
\newcommand{\kl}{\ekk\timm \ell}
\newcommand\exIntro{$\ast$}
\renewcommand\exIntro{\textit{Running example}}
\newcommand\bad{\ensuremath{\dagger}}
\newcommand\prt{\ensuremath{\partial}}
\newcommand\prtbf{\ensuremath{\boldsymbol{\partial}}}
\renewcommand\ta{\ensuremath{\mathsf{t}}}
\renewcommand\so{\ensuremath{\mathsf{s}}}
\cornersize{.5} 
\newcommand\dbox[1]{\fbox{$#1$}}
\renewcommand\dbox[1]{\ovalbox{$#1$}}

\newcommand\mmcol{\ensuremath{{M^{++}}}}
\newcommand\aacol{\ensuremath{{A^{++}}}}

\newcommand\Mplus{\ensuremath{{M^+}}}
\newcommand\Aplus{\ensuremath{{A^+}}}
\newcommand\mmplus{\Mplus}
\newcommand\aaplus{\Aplus}
\newcommand\Mpluss{\ensuremath{{M^{++}}}}
\newcommand\Apluss{\ensuremath{{A^{++}}}}

\newcommand\mmap[1]{\ensuremath{{\mathsf{m}_{#1}}}}
\newcommand\amap[1] {\ensuremath{{\mathsf{a}_{#1}}}}
\newcommand\mplus[1]{\ensuremath{{\mathsf{m}^+_{#1}}}}
\newcommand\aplus[1]{\ensuremath{{\mathsf{a}^+_{#1}}}}


\newcommand\undn{\und{n}}


\newcommand\scenum[1]{\ensuremath{\mathbf{(S#1)}}}
\newcommand\Scenum[1]{\textbf{(Scenario #1)}}
\renewcommand\Scenum[1]{(scenario \scenum{#1})}

\newcommand\xmi[1]{\ensuremath{M_{#1}}}
\newcommand\mo{\xmi{}}
\newcommand\mi{\xmi{1}}
\newcommand\mii{\xmi{2}}
\newcommand\miii{\xmi{3}}
\newcommand\xai[1]{\ensuremath{A_{#1}}}
\newcommand\yai[1]{\ensuremath{R_{#1}}}
\newcommand\ao{\xai{}}
\newcommand\ai{{\xai{1}}}
\newcommand\aii{{\xai{2}}}
\newcommand\aiii{{\xai{3}}}
\newcommand\ri{{\yai{1}}}
\newcommand\rii{{(\yai{12})}}
\newcommand\riii{{(\yai{123})}}


%-- proper names --
\newcommand\addr{\nmf{Addr}}
\newcommand\name{\nmf{name}}
\newcommand\String{\nmf{String}}
\newcommand{\Person}{\nmf{Person}}
\newcommand{\Comp}{\nmf{Company}}
\newcommand{\Company}{\nmf{Company}}
\newcommand{\Commute}{\nmf{Route}}
\newcommand{\Comm}{\nmf{Route}}
\newcommand{\Route}{\nmf{Route}}
\newcommand\Addr{\nmf{Addr}}
\newcommand\from{\nmf{from}}
\newcommand\lives{\nmf{livesAt}}
\newcommand\loc{\nmf{locAt}}
\newcommand\toattr{\nmf{to}}
%\newcommand\Empl{\nmf{Empl\textrm{-}ment}}
%\newcommand{\eer}{\nmf{empl}\textrm{-}\nmf{er}}
%\newcommand{\eee}{\nmf{empl}\textrm{-}\nmf{ee}}
\newcommand\Empl{\nmf{Employment}}
\newcommand{\eer}{\nmf{employer}}
\newcommand{\eee}{\nmf{employee}}
\newcommand{\etor}{\nmf{(e2r)}}
\newcommand{\ptop}{\nmf{(p2p)}}
\newcommand{\ctoc}{\nmf{(c2c)}}


\newcommand\namefont[1]{\ensuremath{\mathsf{#1}}}
\newcommand\nmf[1]{\namefont{#1}}
\newcommand\ittt[1]{\ensuremath\mathit{#1}} 

\newcommand{\netw}{\nmf{Network}}
\newcommand{\network}{\nmf{Network}}
\newcommand{\person}{\nmf{Person}}
\newcommand{\member}{\nmf{Member}}

\renewcommand\phone{\nmf{Phone}}
\newcommand\EMail{\nmf{Email}}
\newcommand\contact{\nmf{Contact}}
\newcommand{\topic}{\nmf{Topic}}
\newcommand{\str}{\nmf{Str}}
\renewcommand{\inv}{\nmf{inv}}
\newcommand{\PM}{\nmf{P/M}}

\newcommand{\cp}{\nmf{c/p}}
\newcommand{\memb}{\nmf{memb}}
\newcommand{\ident}{\nmf{ident}}
\newcommand{\cell}{\nmf{cell}}
\newcommand{\emails}{\nmf{emails}}
\newcommand{\logins}{\nmf{logins}}
\newcommand{\comm}{\nmf{comm}}
\newcommand{\privv}{\nmf{priv}}
%\newcommand{\from}{\nmf{from}}
\newcommand{\too}{\nmf{to}}
\newcommand{\scope}{\nmf{scope}}
\newcommand{\escope}{\nmf{e}\textrm{-}\nmf{scope}}
\newcommand{\on}{\nmf{on}}
\newcommand{\ret}{\nmf{re}}
\newcommand{\re}{\nmf{re}}
\newcommand{\subj}{\nmf{subj}}
\newcommand{\eon}{\nmf{e}\textrm{-}\nmf{on}}
%===
%\newlength{\cellH}
%\newlength{\cellW}



%=== from JSS paper
\newcommand\incal{incremental}
\newcommand\mbcon{\ensuremath{\sim}}
\newcommand\hgg[1]{}
\newcommand\info{\ensuremath{\mathrm{inf}}}



\newcommand\boldsubsubsection[1]{\subsubsection*{\textbf{#1}}}
\renewcommand\boldsubsubsection[1]{\subsubsection*{{#1}}}
\newcommand\goup{\vspace{-7.5pt}}
\newcommand\rich{\ensuremath{\mathrm{+}}}
\newcommand\poor{\ensuremath{\mathrm{-}}}
\newcommand\ohtri{\ensuremath{(\ohafra\ohafra\ohafra)}}

\newcommand\alens{\ensuremath{\lambda}}

% sub and super scripts
\newcommand\indname[1]{\ensuremath\mathrm{#1}}
\newcommand\priv{{\indname{prv}}}
\newcommand\pub{{\indname{pub}}}

\endinput

% Domain-codomain/source-target/ident
\newcommand\cod[1]{\ensuremath{{#1}^\bullet}}
\newcommand\dom[1]{\ensuremath{^\bullet{#1}}}
\newcommand\so{\ensuremath{\mathsf{src}}}
\newcommand\ta{\ensuremath{\mathsf{trg}}}
\renewcommand\so{\ensuremath{\mathsf{s}}} % was src
\renewcommand\ta{\ensuremath{\mathsf{t}}}  % was trg
\newcommand\ldom[1]{\ensuremath{$\Box #1 $}}
\newcommand\rdom[1]{\ensuremath{$#1 \Box $}}
\newcommand\id[1]{\opname{id}_{{#1}}}
\renewcommand\id{\opname{id}}


==> macros4thisPaper.tex <==
%-- the upper taken from macros-general
\renewcommand\comprfam[2]{(\mathstrut{#1}\left|\;{#2}\right.)}
\renewcommand\comprfam[2]{\left(\mathstrut{#1}{:}\,\;{#2}\right)}
%\renewcommand\comprfam[2]{\left(\mathstrut{#1}\right)_{{#2}}}

%= tuples
\newcommand\tuplenam[1]{\ensuremath{\pmb{#1}}}
\renewcommand\tuplenam[1]{\ensuremath{{#1}}}
\newcommand\tupX[1]{\ensuremath{\tuplenam{#1}}}
\newcommand\tupA{\tupX{A}}
\newcommand\tupu{\tupX{u}}
\newcommand\tupB{\tupX{B}}
\newcommand\tupv{\tupX{v}}

\newcommand\prodX[1]{\ensuremath{\prtbf^{\Pi}\!\!#1}}
\renewcommand\prodX[1]{\ensuremath{#1^{\Pi}}}
\newcommand\prodmspA{\prodX{\mspA}}
\newcommand\prodmspB{\prodX{\mspB}}

\newcommand\bounX[1]{\ensuremath{\prtbf#1}}
\newcommand\bounmspA{\bounX{\mspA}}




\newcommand\xconfig[1]{\ensuremath{\mathsf{#1}}}
\newcommand\Span{\xconfig{Span}}
\newcommand\Cospan{\xconfig{Cospan}}
%\newcommand\K{\spaR}
% -- conseq compatible updates
\newcommand\compUpd[2]{\ensuremath{\mathsf{#1}^{{#2}}}}
\newcommand\seqK{\compUpd{K}{\RHD\!\!\RHD}}
\newcommand\parK{\compUpd{K}{{|}{|}{}}}
\newcommand\spanK[1]{\compUpd{K}{\blacktriangle{#1}}}
\newcommand\disjK[1]{\compUpd{K}{\vartriangle{#1}}}
\newcommand\Kupd{\seqK}
\newcommand\Kseq{\seqK}
%--space of conflict-free/concurr compatible updates
\newcommand\cofrK{\parK}
\newcommand\Kpar{\parK}
\newcommand\Kspan[1]{\spanK{#1}}
\newcommand\Kdisj[1]{\disjK{#1}}

%\endinput

% space of consist corrs
\newcommand\consK{\mspX{K^\bigstar}}
\newcommand\Kcorr{\compUpd{K}{\bigstar}}
%\renewcommand\Kcorr{\mspX{K^{\bigstar}}}
%\renewcommand\Kcorr{\ensuremath{{\spaR}^{}}}




\renewcommand\R[1]{\ensuremath{\mspA^{\bigstar}_{#1}}}
\renewcommand\xarr[1]{\ensuremath{#1%
		^{\footnotesize{\RHD}}}}
\newcommand\prospa[1]{\ensuremath{\Pi#1}}
\newcommand{\kl}{\ekk\times \ell}
\newcommand\exIntro{$\ast$}
\renewcommand\exIntro{\textit{Running example}}
\newcommand\bad{\ensuremath{\dagger}}
\newcommand\prt{\ensuremath{\partial}}
\newcommand\prtbf{\ensuremath{\boldsymbol{\partial}}}
\renewcommand\ta{\ensuremath{\mathsf{t}}}
\renewcommand\so{\ensuremath{\mathsf{s}}}
\cornersize{.5} 
\newcommand\dbox[1]{\fbox{$#1$}}
\renewcommand\dbox[1]{\ovalbox{$#1$}}

\newcommand\mmcol{\ensuremath{{M^{++}}}}
\newcommand\aacol{\ensuremath{{A^{++}}}}

\newcommand\Mplus{\ensuremath{{M^+}}}
\newcommand\Aplus{\ensuremath{{A^+}}}
\newcommand\mmplus{\Mplus}
\newcommand\aaplus{\Aplus}
\newcommand\Mpluss{\ensuremath{{M^{++}}}}
\newcommand\Apluss{\ensuremath{{A^{++}}}}

\newcommand\mmap[1]{\ensuremath{{\mathsf{m}_{#1}}}}
\newcommand\amap[1] {\ensuremath{{\mathsf{a}_{#1}}}}
\newcommand\mplus[1]{\ensuremath{{\mathsf{m}^+_{#1}}}}
\newcommand\aplus[1]{\ensuremath{{\mathsf{a}^+_{#1}}}}


\newcommand\undn{\und{n}}


\newcommand\scenum[1]{\ensuremath{\mathbf{(S#1)}}}
\newcommand\Scenum[1]{\textbf{(Scenario #1)}}
\renewcommand\Scenum[1]{(scenario \scenum{#1})}

\newcommand\xmi[1]{\ensuremath{M_{#1}}}
\newcommand\mo{\xmi{}}
\newcommand\mi{\xmi{1}}
\newcommand\mii{\xmi{2}}
\newcommand\miii{\xmi{3}}
\newcommand\xai[1]{\ensuremath{A_{#1}}}
\newcommand\ao{\xai{}}
\newcommand\ai{{\xai{1}}}
\newcommand\aii{{\xai{2}}}
\newcommand\aiii{{\xai{3}}}


%-- proper names --
\newcommand\addr{\nmf{Addr}}
\newcommand\name{\nmf{name}}
\newcommand\String{\nmf{String}}
\newcommand{\Person}{\nmf{Person}}
\newcommand{\Comp}{\nmf{Company}}
\newcommand{\Company}{\nmf{Company}}
\newcommand{\Commute}{\nmf{Commute}}
\newcommand{\Comm}{\nmf{Commute}}
\newcommand\Addr{\nmf{Addr}}
\newcommand\from{\nmf{from}}
\newcommand\lives{\nmf{lives}}
\newcommand\loc{\nmf{located}}
\newcommand\Empl{\nmf{Empl}}
\newcommand{\eer}{\nmf{empl}\textrm{-}\nmf{er}}
\newcommand{\eee}{\nmf{empl}\textrm{-}\nmf{ee}}
%\newcommand\eer{\nmf{empl{-}er}}
%\newcommand\eee{\nmf{empl{-}ee}}

\newcommand\namefont[1]{\ensuremath{\mathsf{#1}}}
\newcommand\nmf[1]{\namefont{#1}}
\newcommand\ittt[1]{\ensuremath\mathit{#1}} 

\newcommand{\netw}{\nmf{Network}}
\newcommand{\network}{\nmf{Network}}
\newcommand{\person}{\nmf{Person}}
\newcommand{\member}{\nmf{Member}}

\renewcommand\phone{\nmf{Phone}}
\newcommand\EMail{\nmf{Email}}
\newcommand\contact{\nmf{Contact}}
\newcommand{\topic}{\nmf{Topic}}
\newcommand{\str}{\nmf{Str}}
\renewcommand{\inv}{\nmf{inv}}
\newcommand{\PM}{\nmf{P/M}}

\newcommand{\cp}{\nmf{c/p}}
\newcommand{\memb}{\nmf{memb}}
\newcommand{\ident}{\nmf{ident}}
\newcommand{\cell}{\nmf{cell}}
\newcommand{\emails}{\nmf{emails}}
\newcommand{\logins}{\nmf{logins}}
\newcommand{\comm}{\nmf{comm}}
\newcommand{\privv}{\nmf{priv}}
%\newcommand{\from}{\nmf{from}}
\newcommand{\too}{\nmf{to}}
\newcommand{\scope}{\nmf{scope}}
\newcommand{\escope}{\nmf{e}\textrm{-}\nmf{scope}}
\newcommand{\on}{\nmf{on}}
\newcommand{\ret}{\nmf{re}}
\newcommand{\re}{\nmf{re}}
\newcommand{\subj}{\nmf{subj}}
\newcommand{\eon}{\nmf{e}\textrm{-}\nmf{on}}
%===
%\newlength{\cellH}
%\newlength{\cellW}



%=== from JSS paper
\newcommand\incal{incremental}
\newcommand\mbcon{\ensuremath{\sim}}
\newcommand\hgg[1]{}
\newcommand\info{\ensuremath{\mathrm{inf}}}



\newcommand\boldsubsubsection[1]{\subsubsection*{\textbf{#1}}}
\renewcommand\boldsubsubsection[1]{\subsubsection*{{#1}}}
\newcommand\goup{\vspace{-7.5pt}}
\newcommand\rich{\ensuremath{\mathrm{+}}}
\newcommand\poor{\ensuremath{\mathrm{-}}}
\newcommand\ohtri{\ensuremath{(\ohafra\ohafra\ohafra)}}

\newcommand\alens{\ensuremath{\lambda}}

% sub and super scripts
\newcommand\indname[1]{\ensuremath\mathrm{#1}}
\newcommand\priv{{\indname{prv}}}
\newcommand\pub{{\indname{pub}}}

\endinput

% Domain-codomain/source-target/ident
\newcommand\cod[1]{\ensuremath{{#1}^\bullet}}
\newcommand\dom[1]{\ensuremath{^\bullet{#1}}}
\newcommand\so{\ensuremath{\mathsf{src}}}
\newcommand\ta{\ensuremath{\mathsf{trg}}}
\renewcommand\so{\ensuremath{\mathsf{s}}} % was src
\renewcommand\ta{\ensuremath{\mathsf{t}}}  % was trg
\newcommand\ldom[1]{\ensuremath{$\Box #1 $}}
\newcommand\rdom[1]{\ensuremath{$#1 \Box $}}
\newcommand\id[1]{\opname{id}_{{#1}}}
\renewcommand\id{\opname{id}}


==> model-spaces.tex <==
\section{Model spaces}

\subsection{Definitions}

Let's call a cat {\em strongly skeletal} if all its isos are identities. This is stronger than being just a skeletal cat as the latter allows non-identity isomorphic loops on an objects. 
\newcommand\editcat{\catname{Edit}}
\newcommand\editx[1]{\enma{\editcat_{#1}}}
\newcommand\edita{\enma{\editcat_{\spA}}}
\newcommand\editb{\enma{\editcat_{\spB}}}
\newcommand\tracecat{\catname{Trace}}
\newcommand\tracex[1]{\enma{\tracecat_{#1}}}
\newcommand\tracea{\enma{\tracecat_{\spA}}}
\newcommand\traceb{\enma{\tracecat_{\spB}}}
\newcommand\trfunx[1]{\enma{{\pmb f}_{#1}}}
\newcommand\trfuna{\enma{{\pmb f}_{\spA}}}
\newcommand\trfun{\trfunx{}} %{\enma{\pmb f}}
\newcommand\edit{\editx{}} %{\enma{\editcat_{\spA}}}
\newcommand\trace{\tracex{}}

\begin{defin}[Model spaces] A model space \spA\ is given by an 
	%lax but identity preserving and 
	identity on objects functor between small categories, \frar{\trfuna}{\edita}{\tracea} satisfying some conditions specified below. Elements in the set $|\edita|=|\tracea|$ are called {\em models}, arrows in \edita\ are {\em edits} and arrows in \tracea\ are {\em traceabillity mappings} or just {\em traces}. We will omit the index \spA\ if it's clear from the context.  
	
	Now the list of additional conditions.
	\begin{itemize}
\item (Skeletality) We require \trace\ to be strongly skeletal
\item (Laxity) We require \edit\ and \trace\ to be 2-categories and \trfun\ be a lax but identity preserving 2-functor  
\item (Dagger)  Functor \trfun\ is a dagger functor between dagger categories (see, \eg, Peter Selinger's paper for a def.) We need a suitable generalization for 2-cats but it's straightforward
\item (Undo) Moreover, we require \edit\ to be a groupoid, \ie, for any edit \frar{e}{A}{A'}, we have $e^\dagger=e^{-1}$ so that $e;e^\dagger=\id_A$ and $e^\dagger;e=\id_{A'}$.
\item (Lifting) Functor \trfun\ is an opfibration, that is,
\begin{itemize}
\item For any $A\in|\edit|$, and each trace \frar{u}{A}{A'}, there is its lifting \frar{\ovr{u}}{A}{A'} which is universal (initial) amongst all edits \frar{e}{A}{A'} mapped to $u$ (\ie, such that $\trfun(e)=u$). That is, \ovr{u} is a weak opcartesian lifting of $u$. Note that this implies $\ovr{\id_A}=\id_A$.
\item Lifting is compositional: for any $A$ and \frar{u}{A}{A'}, \frar{u'}{A'}{A''}, we have $\ovr{u;u'}=\ovr{u};\ovr{u'}$. 
\item The 2-structure. Lifting should also be somehow compatible with the 2 structure and lift 2-arrows too, but I never worked/read about such things. Probably, n-lab should have something about this, and then we're fortunate -- making this accurate ourselves would be a hassle. 
\item Moreover, we require lifting to be dagger-compatible: $\ovr{u^\dagger}=\ovr{u}^\dagger$
\end{itemize}
\item (Connectedness)
Category \edit\ (and hence \trace) is connected: for any pair of models $(A,A')$ there is some \frar{e}{A}{A'} (and hence \frar{e.\trfun}{A}{A'}). We could equivalently require \trace\ to connected and then lifting would make \edit\ connected as well. 
%
\zd{But am not sure we need this condition.}	
\end{itemize} \qed
\end{defin} 
\subsection{Remarks}
Our goal number one is to show that a set of production rules over typed graphs gives rise to a model space. Let's begin with just graphs, then see how it carries on for typed graphs, then for types attributed graphs, and finally for models over arbitrary metamodels. 

For GT, arrows in \edit\ are DPOs with \trfun\ being the projection, but we need to show that DPOs are composable -- it may turn out a hassle as we will face interaction between PBs and POs, but I hope that nice features of adhesive cats would make it more or less doable. 

Lifting should be given by the initial pushout construction (I remember something of this kind in the Fundamentals of Alg GT book). 

The 2-cat structure needs care, but should be straightforward. If it will get complicated. let's consider the 2-arrow to be monics. 

The dagger structure should be easy. 

Overall, it looks doable (hopefully) but making it accurate is quite a bit of work.  


\end{document}

==> sections/backgr-deltalenses-full.tex <==
\subsection{Delta lenses and their composition}
Our discussion of the example can be summarized in the following algebraic terms. We have two categories of {\em models} and {\em updates}, \spA\ and \spB, and a functor \frar{\get}{\spA}{\spB} incrementally computing \spB-views of \spA-models (we will often write $A.\get$ for $\get(A)$). We also suppose that for a chosen update policy, we have worked out precise procedures for how to propagate any view update backwards. This gives us 
%an operation 
%\flar{\putl}{|\spA|\times_{\frompb}\arrofa} {|\spA|\times_{\frompb}\arrofb}
a family of operations 
\flar{\putl_A}{\spA(A,\_)}{\spB(A.\get, \_)}
indexed by \spA-objects, $A\in\obj{\spA}$, for which we write $\putl_A.v$ or $\putl_A(v)$ interchangeably. 
{% renewcommands to reuse the old def
\renewcommand\spS{\spA}  % tweaking the def from the old version
\renewcommand\spT{\spB}
%\renewcommand\ell{{}}
%\newcommand\S{{S}}
\renewcommand\S{{A}}
%\newcommand\T{{T}}
\renewcommand\T{{B}}
%\renewcommand\elll{\enma{\ell}}
\begin{defin}[Delta Lenses (\cite{me-jot11})]\label{def:alens} 
	Let \spS, \spT\ be two categories. An {\em (asymmetric delta) lens} from \spS\ to \spT\ is a pair $\ell=(\get, \putl)$, where \frar{\get}{\spS}{\spT} is a functor and $\putl$ is a family of operations 
	\flar{\putl_A}{\spA(A,\_)}{\spB(A.\get, \_)}
	indexed by objects of \spS, $\S\in\obj{\spS}$. Given $\S$, operation $\putl_\S$ maps any arrow \frar{v}{\S.\get}{\T'} %where $\S.\get=\T$ 
	to an arrow \frar{u}{\S}{\S'} such that $\S'.\get=B'$. The last condition is called (co)discrete Putget law:
		\\ [5pt]
%\lawgap=0.5 ex
%	\noindent 
	\begin{tabular}{l@{\quad}l}
	%	\\ [\lawgap] 
\lawnamebr{Putget}{0}
		& 
		\mbox{ 
			$(\putl_\S.v).\ta.\get_0  = v.\ta$ for all $\S\in|\spS|$ and $v\in\spT(\S.\get,\_)$
		} 
	\end{tabular}
\\ [5pt]	
	%We will often omit the script \elll, and write a lens as \frar{(\get,\putl)}{\spS}{\spT} 
where $\get_0$ denotes the object function of functor \get.	We will write a lens as an arrow \frar{\ell}{\spS}{\spT} going in the direction of \get.
\end{defin}
Note that family \putl\ corresponds to a chosen update policy, \eg, in terms of the example above, for the same view functor \get, we have two families of operations \putl, $\putl^\quit$ and $\putl^\trans$, corresponding to the two updated policies we discussed. %over the same view functor \get.
%a family \flar{\putl_A^\quit}{\spA(A,\_)}{\spB(A.\get, \_)} and another family \flar{\putl_A^\trans}{\spA(A,\_)}{\spB(A.\get, \_)},
 %A pair $\ell=(\get,\putl^A)$ is called an {\em asymmetric delta lens} from \spA\ to \spB.  
These two policies determine two lenses $\ell^\quit=(\get,\putl^\quit)$ and $\ell^\trans=(\get,\putl^\trans)$ sharing the same \get. %
%\shortlong{
%\zd{in the long version, the notions of ..... are described} 	
%	\endinput
%}{
%		
%}

%\zd{a piece about laws and wb is to be written!! Define \wbcodex!!!}
%\zdhl{---\vspace{2cm}---}{to eb written }
Besides a clear ontology of change propagation, practical applications of the lens \fwk\ are due to several constructs of lens composition that preserve some important lens properties. Lenses possessing those properties are often called {\em well-behaved (wb)}, and lenses' compositionality means that composition of wb lenses is again wb. This allows the designer of a complex \syncon\ system to avoid integration testing: if elementary \syncer s possess the required properties and tested, then their composition automatically possesses the required properties. The set of properties ensuring a lens is wb depends on the type of the lens as hand, and the \syncon\ problem it is intended to solve. Hence, well-behavedness is a loose term whose exact meaning is to be defined. We may say that there is a {\em Lens Codex of Wb} (in short, \wbcodex)  that needs a concrete technical interpretation for a special \syncon\ task at hand. 
\begin{defin}[\shortlong%{Equational laws} 
	{Well-behavedness}{Well-behavedness of a-lenses}]\label{def:wbalens}{\emno 
		A {\em (lens) equational law} is an equation to hold for all values of two variables: %$p\in \xob{\spP}$, 
		$\S\in\xob{\spS}$ and \frar{v}{\S.\get}{T'}} (as in the laws below).	
	A lens is called {\em well-behaved (wb)} if the following two equational laws hold:
	\\[1ex]
	\lawgap=1 ex
	\noindent \begin{tabular}{l@{\quad}l}
		\lawnamebr{Stability}{
		}	& \mbox{ 
			$\id_\S = \putl_\S.\id_{\S.\get}$ for all $\S\in|\spS|$ }
		\\ [\lawgap] \lawnamebr{Putget}{} 
		& 
		\mbox{ 
			$(\putl_\S.v).\get  = v$ for all $\S\in|\spS|$ and all $v\in\spT(\S.\get,\_)$
		} 
		%		\shortlong{}{
		%			\\ [\lawgap]
		%			\lawnamebr{Hippocr}{
		%			}	& \mbox{\em 
		%				if $\get_p(u)=v$ for some \frar{u}{S}{S'}, 
		%				then $v^@=\id_{T'}$
		%			}
		%		} %end long 
	\end{tabular}  %\\[10pt] 
\end{defin} 
} %----------------------------> end new command
%%%%%%%%
%\footnote{ 
%Note the distinction between the Putget$_0$ condition included into the very definition of a lens, and the full Putget law required for the wb specialization of lenses. It is needed if we want to define  operations \putl\ separately from the functor \get: then we still need a function \frar{\get_0=|\get|}{|\spA|}{|\spB|} and the codiscrete Putget law to ensure a reasonable behaviour of \putl\ (cf.\cite{bryce-act19}).
%}
%\vspace{-5em}
\begin{remark}%[On lens laws]
	\label{rema:lenslaws}
	{\emno 
a) Stability law says that a wb lens does nothing if nothing happens on the target side 
(no actions without triggers). 

b) Putget requires consistency after the backward propagation is finished. Note the distinction between the Putget$_0$ condition included into the very definition of a lens, and the full Putget law required for the wb lenses. The former is needed to ensure smooth tiling of \putl-squares (\ie, arrow squares describing application of \putl\ to a view update and its result) both horizontally (for sequential composition) and vertically (not considered in the paper). The full Putget assures true consistency as considering a state $B'$ alone does not say much about the real update and elements of $B'$ cannot be properly interpreted. The real story is specified by delta \frar{v}{B}{B'}, and consistency restoration needs the full (\putgetlaw)  law as above.  
\footnote{As shown in \cite{bryce-act19}, the Putget$_0$ condition  is needed if we want to define  operations \putl\ separately from the functor \get: then we still need a function \frar{\obj{\get}}{\obj{\spA}}{\obj{\spB}} and the codiscrete Putget law to ensure a reasonable behaviour of \putl.} 

c) A natural requirement for the family \putl\ would be its  compatibility with update composition: %, \eg, for requests in the absence of amendments, the following law is to hold 
for any \frar{v}{A.\get}{B'}, \frar{v'}{B'}{\_} the following is to hold:
        
        \smallskip
        \noindent \begin{tabular}{l@{\quad}l}
        %	\\ [5pt] 
        \lawnamebr{Putput}{} 
        	& 
        	\mbox{ 
        		$\putl_A.(v;v') = (\putl_A.v);(\putl_{A'}.v')$ where $A'=\ta(\putl_A.v)$
        	} 
        \\ [5pt]
        \end{tabular} 

\noindent (note that $A'.\get=B'$ due to \putgetcodi\ law).   However, this law does not hold in typical \Bx\ applications (see \cite{me-bx17} for examples and discussion) and thus is excluded from the  \wbcodex.%{\sc Lens Codex of Wb}.    
    } % end \emno
\end{remark}
  %\input{ll-figures/diags/viewSys-triangle}
%\medskip
%\vspace{5cm}
\newcommand\figalenscomp{\figref{alens-compose}}
\begin{minipage}{1.\linewidth}
\input{ll-figures/diags/diag-alens-compose}
Asymmetric lenses are sequentially associatively composable. % as shown in the inset figure: 
Having two lenses \frar{\ell1=(\get1,\putl1)}{\spA}{\spB} and \frar{\ell2=(\get2,\putl2)}{\spB}{\spC}, we build a lens \frar{\ell=(\get,\putl)}{\spA}{\spC} with $\get = \get1;\get2$ and $\putl$ being the family defined by composition as shown in \figref{alenscompose} (where objects produced by functors \get s are non-framed, arrows are dashed, and arrows produced by \putl s are dotted): for $A\in|\spA|$ and \frar{w}{A.\get}{C'}, 
$\putl_A.w=\putl1_A.\putl2_B.w$.  The identity lens is given by identity mappings, and we thus have a category \alenscat\ of asymmetric delta lenses \cite{me-jot11,jr-unified}. It's easy to see that sequential  composition preserves well-behavedness; we thus have an embedding $\alenscat_\wbind\subset\alenscat$.
\end{minipage}
% equipped with a ioo forgetful functor \frar{(\minusput)}{\alenscat}{\catcat} defined in the obvious way.
%\\

\bigskip
Next we will briefly outline the notion of an asymmetric lens with amendment (aa-lens): a detailed discussion and motivation can be found in \cite{me-faoc19}

\noindent
\begin{minipage}{1.\textwidth}
{% renewcommands to reuse the old def
	\renewcommand\spS{\spA}  % tweaking the def from the old version
	\renewcommand\spT{\spB}
	%\renewcommand\ell{{}}
	%\newcommand\S{{S}}
	\renewcommand\S{{A}}
	%\newcommand\T{{T}}
	\renewcommand\T{{B}}
	%\renewcommand\elll{\enma{\ell}}
	\vspace{2ex}
	\begin{defin}[Lenses with amendment ]\label{def:aalens} 
		Let \spS, \spT\ be two categories. An {\em (asymmetric delta) lens with amendment (aa-lens)} from \spS\ to \spT\ is a triple $\ell=(\get, \putl^\spba,\putl^\spbb)$, where \frar{\get}{\spS}{\spT} is a functor, $\putl^\spba$ is a family of operations 
		\flar{\putl^\spba_A}{\spA(A,\_)}{\spB(A.\get, \_)}
		indexed by objects of \spS, $\S\in|\spS|$ exactly like in \defref{alens} and 
		$\putl^\spbb$ is a family of operations 
		\frar{\putl^\spbb_A}{\spB(A.\get, \_)}{\spB(A.\get.\ta,\_)}
		also indexed by objects of \spS\ but now mapping an arrow \frar{v}{A.\get}{B'} to an arrow \frar{v^@}{B'}{B'^@} called an {\em amendment} to $v$. We require for all $\S\in|\spS|$,  $v\in\spT(\S.\get,\_)$: 
				\\ [5pt]
		%\lawgap=0.5 ex
		%	\noindent 
		\begin{tabular}{l@{\quad}l}
			%	\\ [\lawgap] 
			\lawnamebr{Putget}{0}
			& 
			\mbox{ 
				$(\putl^\spba_\S.v).\ta.\get_0  = (v;\putl^\spbb_A).\ta$ 
				%for all $\S\in|\spS|$,  $v\in\spT(\S.\get,\_)$
			} 
		\end{tabular}
		\\ [5pt]
	%		. Given $\S$, operation $\putl_\S$ maps any arrow \frar{v}{\T}{\T'} where $\S.\get=\T$ to an arrow \frar{u}{\S}{\S'}. 
		%We will often omit the script \elll, and write a lens as \frar{(\get,\putl)}{\spS}{\spT} 
	%	We will write a lens as an arrow \frar{\ell}{\spS}{\spT} going in the direction of \get.
%	\end{defin} 
	%	
		An aa-lens is called {\em well-behaved (wb)} if the following two equational laws hold:
		\\[1ex]
		\lawgap=1 ex
		\noindent \begin{tabular}{l@{\quad}l}
			\lawnamebr{Stability}{
			}	& \mbox{ 
				$\putl^\spba_\S(\id_{\S.\get})=\id_\S $ and}
			%\\ & 
				\mbox{$\putl_\S^\spbb(\id_{\S.\get})=\id_{\S.\get}$ %for all $\S\in|\spS|$ 
				}
			\\ [5pt] \lawnamebr{Putget}{} 
			& 
			\mbox{ 
				$(\putl^\spba_\S.v).\get  = v;(\putl^\spbb_A.v)$
			       }
		%	\\ &\mbox{ for all $\S\in|\spS|$ and all $v\in\spT(\S.\get,\_)$	} 
					\hippoOutin{}{
						\\ [\lawgap]
						\lawnamebr{Hippocr}{}	& \mbox{\em 
							if $\get_p(u)=v$ for some \frar{u}{S}{S'}, 
							then $v^@=\id_{T'}$
						}
					} %end hippoOutin
		\end{tabular}  
	\\[5pt] 
	for all $\S\in|\spS|$ and all $v\in\spT(\S.\get,\_)$.
	We will sometimes refer to the Putget law for aa-lenses as the {\em amended} Putget.
\end{defin}
 %} ----- %%\caption{Functoriality of update propagation policies: doubleLane}
%%\label{fig:policyfun-doubleLane}
}  % end renew command
\end{minipage}
%\begin{minipage}{0.45\textwidth}
%	\input{ll-figures/diags/lens-compose(a+aa)}
%\end{minipage}
 \hippoOutin{}{
\begin{remark}[Lens laws cont'd]\label{rema:lenslaws2}
	The name ``Hippocraticness'' refers to the famous principle ``First do no harm'' attributed to an ancient Greek physician Hippocrates. Technically, the law above says that if consistency could be achieved without amendment, then consistency is to be restored without amendment. 
 	% The latter prohibits amending delta $v$ if consistency can be achieved for $v$ without amendment (hence, the name).  
 	Note that neither equality $\putUL{\upd}{p,S}(v)=p$ nor $\putUL{\req}{p,S}(v)=u$ are required: changing $v$ is disallowed if consistency can be achieved with a triple $(e,u,\id_{B"})$. 
 
 Besides Stability and Putget, the MDE context for ala-lenses suggests other laws discussed in \cite{me-faoc19}, which were (somewhat recklessly) included into the \wbcodex\ for aa-lenses. To avoid confusion, Johnson and Rosebrugh aptly proposed to call lenses satisfying Stability and Putget {\em SPg lenses} so that the name unambiguously conveys the meaning. In the present paper, wb will mean SPg plus Hippocraticness.  % \eg, Hippocraticness described in the 
\end{remark}
} % END HippoOutin
\begin{remark}[Putget for codiscrete lenses]
	\label{rema:putget4codi}%\zd{to be reworked}
%	The Putget law 
In the codiscrete setting, the codiscrete Putget law, \putgetcodi, actually determines amendment in a unique way. The other way round, a codiscrete lens without the requirement to satisfy Putget, is a wb codiscrete lens with amendment (which satisfies the amended Putget). %    law is a notational trick rather than a law. We begin with delta $v=(A.\get, B')$, which operation  $\putl^\spba_A$  propagates  to delta $u=(A,A')$,  and function $\get$ sends it to delta  $(B,B'')$ where $A'.\get=B''$. Also, $\putl^\spbb_A$ gives us an amendment delta $v^@=(B', B'^@)$ and $v;v^@=(S_p, S'_{p'})=\get_e(S,S')$ so that Putget always holds. %targeting at some model $S'_{p'}$ anyway. But in the general delta setting, there are many possible deltas between models $T'$ and $S'_{p'}$, whereas the Putget law states the existence of some special delta \frar{v^@}{T'}{S'_{p'}} such that equation (\putget) holds. %Note also that Putget implies commutativity of the lower triangle in the right back face as the upper one is commutative by Putget. %much more certainty about $T''$ and precisely specifies the relationship between $T'$ and $T''$, namely, it says that they are related by a specified update $\amex{v}$.
\end{remark}


%}  % end renew command
%\end{minipage}

%\input{ll-figures/diags/policyfun-doubleLane}
%\input{ll-figures/diags/lens-compose(a+aa)}

\noindent
\begin{minipage}{1.\linewidth}
\input{ll-figures/diags/diag-aalens-compose-new}
\noindent Composition of aa-lenses, say, \frar{\ell1}{\spA}{\spB} and \frar{\ell2}{\spB}{\spC} is specified by diagram in \figref{aalenscompose} (objects produced by functors \get s are non-framed, arrows are dashed, and arrows produced by \putl s are dotted).  Operation invocation numbers 1-3 show the order of applying operations to produce the composed \putl: 
$\putl^\spca_A.w=\putl^\spba_A.\putl^\spcb_B.w$ and 
the composed lens amendment $\putl^{\spcc}=w^@$ is defined by composition $w^{@2};(v^{@1}.\get2)$.  In 
%\sectref{alalenscat} 
\sectref{seqlensass-proof}, 
we will see that composition of aa-lenses is associative (in the more general setting of ala-lenses, \ie, aa-lenses with learning) and they form a category \aalenscat\ with a subcategory of wb aa-lenses $\aalenscat_\wbind\subset\aalenscat$. Also, an ordinary a-lens can be seen as a special aa-lens, for which all amendments are identities, and aa-lens composition specified in \figref{aalenscompose} coincides with a-lens composition in \figref{alenscompose}; moreover, the aa-lens wb conditions become a-lens wb conditions. Thus, we have embeddings $\alenscat\subset\aalenscat$ and $\alenscat_\wbind\subset\aalenscat_\wbind$.
\end{minipage}

==> sections/backgr-deltalenses-short.tex <==
\subsection{Delta lenses and their composition}
Our discussion of the example can be summarized in the following algebraic terms. We have two categories of {\em models} and {\em updates}, \spA\ and \spB, and a functor \frar{\get}{\spA}{\spB} incrementally computing \spB-views of \spA-models (we will often write $A.\get$ for $\get(A)$). We also suppose that for a chosen update policy, we have worked out precise procedures for how to propagate any view update backwards. This gives us 
%an operation 
%\flar{\putl}{|\spA|\times_{\frompb}\arrofa} {|\spA|\times_{\frompb}\arrofb}
a family of operations 
\flar{\putl_A}{\spA(A,\_)}{\spB(A.\get, \_)}
indexed by \spA-objects, $A\in\obj{\spA}$, for which we write $\putl_A.v$ or $\putl_A(v)$ interchangeably. 
{% renewcommands to reuse the old def
\renewcommand\spS{\spA}  % tweaking the def from the old version
\renewcommand\spT{\spB}
%\renewcommand\ell{{}}
%\newcommand\S{{S}}
\renewcommand\S{{A}}
%\newcommand\T{{T}}
\renewcommand\T{{B}}
%\renewcommand\elll{\enma{\ell}}
\begin{defin}[Delta Lenses (\cite{me-jot11})]\label{def:alens} 
	Let \spS, \spT\ be two categories. An {\em (asymmetric delta) lens} from \spS\ to \spT\ is a pair $\ell=(\get, \putl)$, where \frar{\get}{\spS}{\spT} is a functor and $\putl$ is a family of operations 
	\flar{\putl_A}{\spA(A,\_)}{\spB(A.\get, \_)}
	indexed by objects of \spS, $\S\in\obj{\spS}$. Given $\S$, operation $\putl_\S$ maps any arrow \frar{v}{\S.\get}{\T'} %where $\S.\get=\T$ 
	to an arrow \frar{u}{\S}{\S'} such that $\S'.\get=B'$. The last condition is called (co)discrete Putget law:
		\\ [5pt]
%\lawgap=0.5 ex
%	\noindent 
	\begin{tabular}{l@{\quad}l}
	%	\\ [\lawgap] 
\lawnamebr{Putget}{0}
		& 
		\mbox{ 
			$(\putl_\S.v).\ta.\get_0  = v.\ta$ for all $\S\in|\spS|$ and $v\in\spT(\S.\get,\_)$
		} 
	\end{tabular}
\\ [5pt]	
	%We will often omit the script \elll, and write a lens as \frar{(\get,\putl)}{\spS}{\spT} 
where $\get_0$ denotes the object function of functor \get.	We will write a lens as an arrow \frar{\ell}{\spS}{\spT} going in the direction of \get.
\end{defin}
Note that family \putl\ corresponds to a chosen update policy, \eg, in terms of the example above, for the same view functor \get, we have two families of operations \putl, $\putl^\quit$ and $\putl^\trans$, corresponding to the two updated policies we discussed. %over the same view functor \get.
%a family \flar{\putl_A^\quit}{\spA(A,\_)}{\spB(A.\get, \_)} and another family \flar{\putl_A^\trans}{\spA(A,\_)}{\spB(A.\get, \_)},
 %A pair $\ell=(\get,\putl^A)$ is called an {\em asymmetric delta lens} from \spA\ to \spB.  
These two policies determine two lenses $\ell^\quit=(\get,\putl^\quit)$ and $\ell^\trans=(\get,\putl^\trans)$ sharing the same \get. %

% commented for the short version
%
%\begin{defin}[\shortlong%{Equational laws} 
%	{Well-behavedness}{Well-behavedness}]\label{def:wbalens}{\emno 
%		A {\em (lens) equational law} is an equation to hold for all values of two variables: %$p\in \xob{\spP}$, 
%		$\S\in\xob{\spS}$ and \frar{v}{\S.\get}{T'}} (as in the laws below).	
%	A lens is called {\em well-behaved (wb)} if the following two equational laws hold:
%	\\[1ex]
%	\lawgap=1 ex
%	\noindent \begin{tabular}{l@{\quad}l}
%		\lawnamebr{Stability}{
%		}	& \mbox{ 
%			$\id_\S = \putl_\S.\id_{\S.\get}$ for all $\S\in|\spS|$ }
%		\\ [\lawgap] \lawnamebr{Putget}{} 
%		& 
%		\mbox{ 
%			$(\putl_\S.v).\get  = v$ for all $\S\in|\spS|$ and all $v\in\spT(\S.\get,\_)$
%		} 
%		%		\shortlong{}{
%		%			\\ [\lawgap]
%		%			\lawnamebr{Hippocr}{
%		%			}	& \mbox{\em 
%		%				if $\get_p(u)=v$ for some \frar{u}{S}{S'}, 
%		%				then $v^@=\id_{T'}$
%		%			}
%		%		} %end long 
%	\end{tabular}  %\\[10pt] 
%\end{defin} 
%} %----------------------------> end new command
%%%%%%%%%
%%\footnote{ 
%%Note the distinction between the Putget$_0$ condition included into the very definition of a lens, and the full Putget law required for the wb specialization of lenses. It is needed if we want to define  operations \putl\ separately from the functor \get: then we still need a function \frar{\get_0=|\get|}{|\spA|}{|\spB|} and the codiscrete Putget law to ensure a reasonable behaviour of \putl\ (cf.\cite{bryce-act19}).
%%}
%%\vspace{-5em}
%\begin{remark}[On lens laws]\label{rema:laws1}{\emno 
%		%a) Condition Closure only requires full amendment deltas $v;v^@$ to be closed, which is  much weaker than the defining condition of closed lens requiring  {\em each} delta to be closed. %as to be fulfilled in closed lenses. 
%		a) Stability says that the lens does nothing if nothing happens on the target side (no trigger--no action, hence, the name of the law) 
%		
%		b) 	Putget requires the goal of update propagation to be achieved after the propagation act is finished (see examples in \sectref{ex-updprop}). Note the distinction between the Putget$_0$ condition included into the very definition of a lens, and the full Putget law required for the wb specialization of lenses. It is needed to ensure smooth tiling of \putl-squares (\ie, arrow squares describing application of \putl\ to a view update and its result) both horizontally and vertically (not considered in this paper). Also, if we want to accurately define operations \putl\ independently of the functor \get, we still need a function \frar{\get_0=|\get|}{|\spA|}{|\spB|} and the codiscrete Putget law to ensure smooth tiling (cf.\cite{bryce-act19}).
%
%        c) A natural requirement for the family \putl\ would be its  compatibility with update composition: %, \eg, for requests in the absence of amendments, the following law is to hold 
%        for any \frar{v}{A.\get}{B'}, \frar{v'}{B'}{\_} the following is to hold:
%        
%        \medskip
%        \noindent \begin{tabular}{l@{\quad}l}
%        %	\\ [5pt] 
%        \lawnamebr{Putput}{} 
%        	& 
%        	\mbox{ 
%        		$\putl_A.(v;v') = (\putl_A.v);(\putl_{A'}.v')$ where $A'=(\putl_A.v)^\ta$
%        	} 
%        \\ [5pt]
%        \end{tabular} 
%
%\noindent (note that $A'.\get=B'$ due to \putgetcodi\ law).   However, this law does not hold in typical \Bx applications (see \cite{me-bx17} for examples and discussion) and thus is excluded from the  \wbcodex. %{\sc Lens Codex of Wb}.    
%    } % end \emno
%\end{remark}
%   END short commented
 
 %\input{ll-figures/diags/viewSys-triangle}
\medskip
\newcommand\figalenscomp{\figref{alens-compose}}
\input{ll-figures/diags/diag-alens-compose}
Asymmetric lenses are sequentially associatively composable. % as shown in the inset figure: 
Having two lenses \frar{\ell1=(\get1,\putl1)}{\spA}{\spB} and \frar{\ell2=(\get2,\putl2)}{\spB}{\spC}, we build a lens \frar{\ell=(\get,\putl)}{\spA}{\spC} with $\get = \get1;\get2$ and $\putl$ being the family defined by composition as shown in \figref{alenscompose} (where objects produced by functors \get s are non-framed, arrows are dashed, and arrows produced by \putl s are dotted): for $A\in|\spA|$ and \frar{w}{A.\get}{C'}, $\putl_A.w=\putl1_A.\putl2_B.w$.  The identity lens is given by identity mappings, and we thus have a category \alenscat\ of asymmetric delta lenses \cite{me-jot11,jr-unified}. It's easy to see that sequential  composition preserves well-behavedness; we thus have an embedding $\alenscat_\wbind\subset\alenscat$.
% equipped with a ioo forgetful functor \frar{(\minusput)}{\alenscat}{\catcat} defined in the obvious way.
%\\

Next we will briefly outline the notion of an asymmetric lens with amendment (aa-lens): a detailed discussion and motivation can be found in \cite{me-faoc19}

\noindent
\begin{minipage}{1.\textwidth}
{% renewcommands to reuse the old def
	\renewcommand\spS{\spA}  % tweaking the def from the old version
	\renewcommand\spT{\spB}
	%\renewcommand\ell{{}}
	%\newcommand\S{{S}}
	\renewcommand\S{{A}}
	%\newcommand\T{{T}}
	\renewcommand\T{{B}}
	%\renewcommand\elll{\enma{\ell}}
	\begin{defin}[Lenses with amendment ]\label{def:aalens} 
		Let \spS, \spT\ be two categories. An {\em (asymmetric delta) lens with amendment (aa-lens)} from \spS\ to \spT\ is a triple $\ell=(\get, \putl^\spba,\putl^\spbb)$, where \frar{\get}{\spS}{\spT} is a functor, $\putl^\spba$ is a family of operations 
		\flar{\putl^\spba_A}{\spA(A,\_)}{\spB(A.\get, \_)}
		indexed by objects of \spS, $\S\in|\spS|$ exactly like in \defref{alens} and 
		$\putl^\spbb$ is a family of operations 
		\frar{\putl^\spbb_A}{\spB(A.\get, \_)}{\spB(A.\get.\ta,\_)}
		also indexed by objects of \spS\ but now mapping an arrow \frar{v}{A.\get}{B'} to an arrow \frar{v^@}{B'}{B'^@} called an {\em amendment} to $v$. We require for all $\S\in|\spS|$,  $v\in\spT(\S.\get,\_)$: 
				\\ [5pt]
		%\lawgap=0.5 ex
		%	\noindent 
		\begin{tabular}{l@{\quad}l}
			%	\\ [\lawgap] 
			\lawnamebr{Putget}{0}
			& 
			\mbox{ 
				$(\putl^\spba_\S.v).\ta.\get_0  = (v;\putl^\spbb_A).\ta$ 
				%for all $\S\in|\spS|$,  $v\in\spT(\S.\get,\_)$
			} 
		\end{tabular}
		\\ [5pt]
%	% Given $\S$, operation $\putl_\S$ maps any arrow \frar{v}{\T}{\T'} where $\S.\get=\T$ to an arrow \frar{u}{\S}{\S'}. We will often omit the script \elll, and write a lens as an arrow in the direction of \get, \frar{(\get,\putl)}{\spS}{\spT} 
%%  commented fro short
%		An aa-lens is called {\em well-behaved (wb)} if the following two equational laws hold:
%		\\[1ex]
%		\lawgap=1 ex
%		\noindent \begin{tabular}{l@{\quad}l}
%			\lawnamebr{Stability}{
%			}	& \mbox{ 
%				$\putl^\spba_\S(\id_{\S.\get})=\id_\S $ and}
%			%\\ & 
%				\mbox{$\putl_\S^\spbb(\id_{\S.\get})=\id_{\S.\get}$ %for all $\S\in|\spS|$ 
%				}
%			\\ [5pt] \lawnamebr{Putget}{} 
%			& 
%			\mbox{ 
%				$(\putl^\spba_\S.v).\get  = v;(\putl^\spbb_A.v)$}
%		%	\\ &\mbox{ for all $\S\in|\spS|$ and all $v\in\spT(\S.\get,\_)$	} 
%			%		\shortlong{}{
%			%			\\ [\lawgap]
%			%			\lawnamebr{Hippocr}{
%			%			}	& \mbox{\em 
%			%				if $\get_p(u)=v$ for some \frar{u}{S}{S'}, 
%			%				then $v^@=\id_{T'}$
%			%			}
%			%		} %end long 
%		\end{tabular}  
%	\\[5pt] 
%	for all $\S\in|\spS|$ and all $v\in\spT(\S.\get,\_)$.
%	We will sometimes refer to the Putget law for aa-lenses as the {\em amended} Putget.
%	\end{defin} 
% %} ----- %%\caption{Functoriality of update propagation policies: doubleLane}
%%%\label{fig:policyfun-doubleLane}
%}  % end renew command
%\end{minipage}
%%\begin{minipage}{0.45\textwidth}
%%	\input{ll-figures/diags/lens-compose(a+aa)}
%%\end{minipage}
%\begin{remark}[On lens laws]\label{rema:laws2}
%\shortlong{}{b)}	
%Besides Stability and Putget, the MDE context for ala-lenses suggests other laws discussed in \cite{me-faoc19}, which were (somewhat recklessly) included into the \wbcodex. To avoid confusion, Johnson and Rosebrugh aptly proposed to call lenses satisfying Stability and Putget {\em SPg lenses} so that the name unambiguously conveys the meaning. In the present paper, wb will mean exactly SPg.   % \eg, Hippocraticness described in the longer version \cite{me-act19-long}.
%\shortlong{}{
%	c) Hippocraticness prohibits amending delta $v$ if consistency can be achieved for $v$ without amendment (hence, the name).  Note that neither equality $\putUL{\upd}{p,S}(v)=p$ nor $\putUL{\req}{p,S}(v)=u$ are required: the lens can improve consistency by changing $p$ and $u$ but changing $v$ is disallowed.  
%} % end \em; end long
%\end{remark}
%\begin{remark}[Putget for codiscrete lenses]
%	\label{rema:putget4codi}%\zd{to be reworked}
%%	The Putget law 
%In the codiscrete setting, the codiscrete Putget law, \putgetcodi, actually determines amendment in a unique way. The other way round, a codiscrete lens without the requirement to satisfy Putget, is a wb codiscrete lens with amendment (which satisfies the amended Putget). %    law is a notational trick rather than a law. We begin with delta $v=(A.\get, B')$, which operation  $\putl^\spba_A$  propagates  to delta $u=(A,A')$,  and function $\get$ sends it to delta  $(B,B'')$ where $A'.\get=B''$. Also, $\putl^\spbb_A$ gives us an amendment delta $v^@=(B', B'^@)$ and $v;v^@=(S_p, S'_{p'})=\get_e(S,S')$ so that Putget always holds. %targeting at some model $S'_{p'}$ anyway. But in the general delta setting, there are many possible deltas between models $T'$ and $S'_{p'}$, whereas the Putget law states the existence of some special delta \frar{v^@}{T'}{S'_{p'}} such that equation (\putget) holds. %Note also that Putget implies commutativity of the lower triangle in the right back face as the upper one is commutative by Putget. %much more certainty about $T''$ and precisely specifies the relationship between $T'$ and $T''$, namely, it says that they are related by a specified update $\amex{v}$.
%\end{remark}
%
%
%%}  % end renew command
%%\end{minipage}
% END short commented


%\input{ll-figures/diags/policyfun-doubleLane}
%\input{ll-figures/diags/lens-compose(a+aa)}
\input{ll-figures/diags/diag-aalens-compose-new}
\noindent Composition of aa-lenses, say, \frar{\ell1}{\spA}{\spB} and \frar{\ell2}{\spB}{\spC} is specified by diagram in \figref{aalenscompose} (objects produced by functors \get s are non-framed, arrows are dashed, and arrows produced by \putl s are dotted).  Operation invocation numbers 1-3 show the order of applying operations to produce the composed \putl: 
$\putl^\spca_A.w=\putl^\spba_A.\putl^\spcb_B.w$ and 
the composed lens amendment $\putl^{\spcc}=w^@$ is defined by composition $w^{@2};(v^{@1}.\get2)$.  In 
%\sectref{alalenscat} 
\sectref{seqlensass-proof}, 
we will see that composition of aa-lenses is associative (in the more general setting of ala-lenses, \ie, aa-lenses with learning) and they form a category \aalenscat\ with a subcategory of wb aa-lenses $\aalenscat_\wbind\subset\aalenscat$. Also, an ordinary a-lens can be seen as a special aa-lens, for which all amendments are identities, and aa-lens composition specified in \figref{aalenscompose} coincides with a-lens composition in \figref{alenscompose}; moreover, the aa-lens wb conditions become a-lens wb conditions. Thus, we have embeddings $\alenscat\subset\aalenscat$ and $\alenscat_\wbind\subset\aalenscat_\wbind$.


==> sections/backgr-deltalenses-shortt.tex <==
\subsection{Delta lenses } %and their composition}
Our discussion of the example can be summarized in the following algebraic terms. We have two categories of {\em models} and {\em updates}, \spA\ and \spB, and a functor \frar{\get}{\spA}{\spB} incrementally computing \spB-views of \spA-models (we will often write $A.\get$ for $\get(A)$). We also suppose that for a chosen update policy, we have worked out precise procedures for how to propagate any view update backwards. This gives us 
%an operation 
%\flar{\putl}{|\spA|\times_{\frompb}\arrofa} {|\spA|\times_{\frompb}\arrofb}
a family of operations 
\flar{\putl_A}{\spA(A,\_)}{\spB(A.\get, \_)}
indexed by \spA-objects, $A\in\obj{\spA}$, for which we write $\putl_A.v$ or $\putl_A(v)$ interchangeably. 
{% renewcommands to reuse the old def
\renewcommand\spS{\spA}  % tweaking the def from the old version
\renewcommand\spT{\spB}
%\renewcommand\ell{{}}
%\newcommand\S{{S}}
\renewcommand\S{{A}}
%\newcommand\T{{T}}
\renewcommand\T{{B}}
%\renewcommand\elll{\enma{\ell}}
\begin{defin}[Delta Lenses (\cite{me-jot11})]\label{def:alens} 
	Let \spS, \spT\ be two categories. An {\em (asymmetric delta) lens} from \spS\ (the source of the lens) to \spT\ (the target) is a pair $\ell=(\get, \putl)$, where \frar{\get}{\spS}{\spT} is a functor and $\putl$ is a family of operations 
	\flar{\putl_A}{\spA(A,\_)}{\spB(A.\get, \_)}
	indexed by objects of \spS, $\S\in\obj{\spS}$. Given $\S$, operation $\putl_\S$ maps any arrow \frar{v}{\S.\get}{\T'} %where $\S.\get=\T$ 
	to an arrow \frar{u}{\S}{\S'} such that $\S'.\get=B'$. The last condition is called (co)discrete Putget law:
		\\ [5pt]
%\lawgap=0.5 ex
%	\noindent 
	\begin{tabular}{l@{\quad}l}
	%	\\ [\lawgap] 
\lawnamebr{Putget}{0}
		& 
		\mbox{ 
			$(\putl_\S.v).\ta.\get_0  = v.\ta$ for all $\S\in\obj{\spS}$ and $v\in\spT(\S.\get,\_)$
		} 
	\end{tabular}
\\ [5pt]	
	%We will often omit the script \elll, and write a lens as \frar{(\get,\putl)}{\spS}{\spT} 
where $\get_0$ denotes the object function of functor \get.	We will write a lens as an arrow \frar{\ell}{\spS}{\spT} going in the direction of \get.
\end{defin}
Note that family \putl\ corresponds to a chosen update policy, \eg, in terms of the example above, for the same view functor \get, we have two families of \putl-operations, $\putl^\quit$ and $\putl^\trans$, corresponding to the two updated policies we discussed. %over the same view functor \get.
%a family \flar{\putl_A^\quit}{\spA(A,\_)}{\spB(A.\get, \_)} and another family \flar{\putl_A^\trans}{\spA(A,\_)}{\spB(A.\get, \_)},
 %A pair $\ell=(\get,\putl^A)$ is called an {\em asymmetric delta lens} from \spA\ to \spB.  
These two policies determine two lenses $\ell^\quit=(\get,\putl^\quit)$ and $\ell^\trans=(\get,\putl^\trans)$ sharing the same \get. %
%\shortlong{
%\zd{in the long version, the notions of ..... are described} 	
%	\endinput
%}{
%		
%}
\begin{defin}[\shortlong%{Equational laws} 
	{Well-behavedness}{Well-behavedness}]\label{def:wbalens}{\emno 
		A {\em (lens) equational law} is an equation to hold for all values of two variables: %$p\in \xob{\spP}$, 
		$\S\in\xob{\spS}$ and \frar{v}{\S.\get}{T'}}. % (as in the laws below).	
	A lens is called {\em well-behaved (wb)} if the following two laws hold:
	\\[1ex]
	\lawgap=1 ex
	\noindent \begin{tabular}{l@{\quad}l}
		\lawnamebr{Stability}{
		}	& \mbox{ 
			$\id_\S = \putl_\S.\id_{\S.\get}$ for all $\S\in\obj{\spS}$ }
		\\ [\lawgap] \lawnamebr{Putget}{} 
		& 
		\mbox{ 
			$(\putl_\S.v).\get  = v$ for all $\S\in\obj{\spS}$ and all $v\in\spT(\S.\get,\_)$
		} 
		%		\shortlong{}{
		%			\\ [\lawgap]
		%			\lawnamebr{Hippocr}{
		%			}	& \mbox{\em 
		%				if $\get_p(u)=v$ for some \frar{u}{S}{S'}, 
		%				then $v^@=\id_{T'}$
		%			}
		%		} %end long 
	\end{tabular}  %\\[10pt] 
\end{defin} 
} %----------------------------> end new command
%%%%%%%%
\input{sections/remark-lensLaws}

\endinput
%%\vspace{-5em}
%\begin{remark}[On lens laws]\label{rema:laws1}{\emno 
%		%a) Condition Closure only requires full amendment deltas $v;v^@$ to be closed, which is  much weaker than the defining condition of closed lens requiring  {\em each} delta to be closed. %as to be fulfilled in closed lenses. 
%		a) Stability says that the lens does nothing if nothing happens on the target side (no trigger--no action, hence, the name of the law) 
%		
%		b) 	Putget requires the goal of update propagation to be achieved after the propagation act is finished (see examples in \sectref{ex-updprop}). Note the distinction between the Putget$_0$ condition included into the very definition of a lens, and the full Putget law required for the wb specialization of lenses. It is needed to ensure smooth tiling of \putl-squares (\ie, arrow squares describing application of \putl\ to a view update and its result) both horizontally and vertically (not considered in this paper). Also, if we want to accurately define operations \putl\ independently of the functor \get, we still need a function \frar{\get_0=|\get|}{|\spA|}{|\spB|} and the codiscrete Putget law to ensure smooth tiling (cf.\cite{bryce-act19}).
%
%        c) A natural requirement for the family \putl\ would be its  compatibility with update composition: %, \eg, for requests in the absence of amendments, the following law is to hold 
%        for any \frar{v}{A.\get}{B'}, \frar{v'}{B'}{\_} the following is to hold:
%        
%        \medskip
%        \noindent \begin{tabular}{l@{\quad}l}
%        %	\\ [5pt] 
%        \lawnamebr{Putput}{} 
%        	& 
%        	\mbox{ 
%        		$\putl_A.(v;v') = (\putl_A.v);(\putl_{A'}.v')$ where $A'=(\putl_A.v)^\ta$
%        	} 
%        \\ [5pt]
%        \end{tabular} 
%
%\noindent (note that $A'.\get=B'$ due to \putgetcodi\ law).   However, this law does not hold in typical \Bx applications (see \cite{me-bx17} for examples and discussion) and thus is excluded from the  \wbcodex. %{\sc Lens Codex of Wb}.    
%    } % end \emno
%\end{remark}
% END commented for short 
 
% % another commented for short
% %\input{ll-figures/diags/viewSys-triangle}
%\medskip
%\newcommand\figalenscomp{\figref{alens-compose}}
%\input{ll-figures/diags/diag-alens-compose}
%Asymmetric lenses are sequentially associatively composable. % as shown in the inset figure: 
%Having two lenses \frar{\ell1=(\get1,\putl1)}{\spA}{\spB} and \frar{\ell2=(\get2,\putl2)}{\spB}{\spC}, we build a lens \frar{\ell=(\get,\putl)}{\spA}{\spC} with $\get = \get1;\get2$ and $\putl$ being the family defined by composition as shown in \figref{alenscompose} (where objects produced by functors \get s are non-framed, arrows are dashed, and arrows produced by \putl s are dotted): for $A\in|\spA|$ and \frar{w}{A.\get}{C'}, $\putl_A.w=\putl1_A.\putl2_B.w$.  The identity lens is given by identity mappings, and we thus have a category \alenscat\ of asymmetric delta lenses \cite{me-jot11,jr-unified}. It's easy to see that sequential  composition preserves well-behavedness; we thus have an embedding $\alenscat_\wbind\subset\alenscat$.
%% equipped with a ioo forgetful functor \frar{(\minusput)}{\alenscat}{\catcat} defined in the obvious way.
%%\\

Next we will briefly discuss the notion of an asymmetric lens with amendment (aa-lens): a detailed discussion and motivation can be found in \cite{me-faoc19}

\noindent
\begin{minipage}{1.\textwidth}
{% renewcommands to reuse the old def
	\renewcommand\spS{\spA}  % tweaking the def from the old version
	\renewcommand\spT{\spB}
	%\renewcommand\ell{{}}
	%\newcommand\S{{S}}
	\renewcommand\S{{A}}
	%\newcommand\T{{T}}
	\renewcommand\T{{B}}
	%\renewcommand\elll{\enma{\ell}}
	\vspace{1ex}
	\begin{defin}[Lenses with amendment ]\label{def:aalens} 
		%Let \spS, \spT\ be two categories. 
		An {\em (asymmetric delta) lens with amendment (aa-lens)} from \spS\ to \spT\ is a triple $\ell=(\get, \putl^\spba,\putl^\spbb)$, where \frar{\get}{\spS}{\spT} is a functor, $\putl^\spba$ is a family of operations 
		\flar{\putl^\spba_A}{\spA(A,\_)}{\spB(A.\get, \_)}
		indexed by objects of \spS, $\S\in\obj{\spS}$ exactly like in \defref{alens} and 
		$\putl^\spbb$ is a family of operations 
		\frar{\putl^\spbb_A}{\spB(A.\get, \_)}{\spB(A.\get.\ta,\_)}
		also indexed by objects of \spS\ but now mapping an arrow \frar{v}{A.\get}{B'} to an arrow \frar{v^@}{B'}{B'^@} called an {\em amendment} to $v$. We require for all $\S\in\obj{\spS}$,  $v\in\spT(\S.\get,\_)$: 
				\\ [5pt]
		%\lawgap=0.5 ex
		%	\noindent 
		\begin{tabular}{l@{\quad}l}
			%	\\ [\lawgap] 
			\lawnamebr{Putget}{0}
			& 
			\mbox{ 
				$(\putl^\spba_\S.v).\ta.\get_0  = (v;\putl^\spbb_A).\ta$ 
				%for all $\S\in\obj{\spS}$,  $v\in\spT(\S.\get,\_)$
			} 
		\end{tabular}
		\\ [5pt]
	%		. Given $\S$, operation $\putl_\S$ maps any arrow \frar{v}{\T}{\T'} where $\S.\get=\T$ to an arrow \frar{u}{\S}{\S'}. 
		%We will often omit the script \elll, and write a lens as \frar{(\get,\putl)}{\spS}{\spT} 
	%	We will write a lens as an arrow \frar{\ell}{\spS}{\spT} going in the direction of \get.
%	\end{defin} 
		An aa-lens is called {\em well-behaved (wb)} if the following two equational laws hold:
		\\[1ex]
		\lawgap=1 ex
		\noindent \begin{tabular}{l@{\quad}l}
			\lawnamebr{Stability}{
			}	& \mbox{ 
				$\putl^\spba_\S(\id_{\S.\get})=\id_\S $ and}
			%\\ & 
				\mbox{$\putl_\S^\spbb(\id_{\S.\get})=\id_{\S.\get}$ %for all $\S\in\obj{\spS}$ 
				}
			\\ [5pt] \lawnamebr{Putget}{} 
			& 
			\mbox{ 
				$(\putl^\spba_\S.v).\get  = v;(\putl^\spbb_A.v)$}
		%	\\ &\mbox{ for all $\S\in\obj{\spS}$ and all $v\in\spT(\S.\get,\_)$	} 
			%		\shortlong{}{
			%			\\ [\lawgap]
			%			\lawnamebr{Hippocr}{
			%			}	& \mbox{\em 
			%				if $\get_p(u)=v$ for some \frar{u}{S}{S'}, 
			%				then $v^@=\id_{T'}$
			%			}
			%		} %end long 
		\end{tabular}  
	\\[5pt] 
	for all $\S\in\obj{\spS}$ and all $v\in\spT(\S.\get,\_)$.
	We will sometimes refer to the Putget law for aa-lenses as the {\em amended} Putget.	\end{defin} 
 %} ----- %%\caption{Functoriality of update propagation policies: doubleLane}
%%\label{fig:policyfun-doubleLane}
}  % end renew command
\end{minipage}
%\begin{minipage}{0.45\textwidth}
%	\input{ll-figures/diags/lens-compose(a+aa)}
%\end{minipage}
% commented for short
%\begin{remark}[On lens laws]\label{rema:laws2}
%\shortlong{}{b)}	
%Besides Stability and Putget, the MDE context for ala-lenses suggests other laws discussed in \cite{me-faoc19}, which were (somewhat recklessly) included into the \wbcodex. To avoid confusion, Johnson and Rosebrugh aptly proposed to call lenses satisfying Stability and Putget {\em SPg lenses} so that the name unambiguously conveys the meaning. In the present paper, wb will mean exactly SPg.   % \eg, Hippocraticness described in the longer version \cite{me-act19-long}.
%\shortlong{}{
%	c) Hippocraticness prohibits amending delta $v$ if consistency can be achieved for $v$ without amendment (hence, the name).  Note that neither equality $\putUL{\upd}{p,S}(v)=p$ nor $\putUL{\req}{p,S}(v)=u$ are required: the lens can improve consistency by changing $p$ and $u$ but changing $v$ is disallowed.  
%} % end \em; end long
%\end{remark}
\begin{remark}[On lens laws] %Putget for codiscrete lenses]
	\label{rema:putget4codi}%\zd{to be reworked}
%	The Putget law 
Stability law says that a wb lens does nothing if nothing happens on the target side 
(no actions without triggers). Putget requires consistency %the goal of update propagation to be achieved 
after the propagation act is finished. Note the distinction between the Putget$_0$ condition included into the very definition of a lens, and the full Putget law required for the wb lenses. The former is needed to ensure smooth tiling of \putl-squares (\ie, arrow squares describing application of \putl\ to a view update and its result) both horizontally and vertically (the latter is not considered in this paper). In the codiscrete setting, the codiscrete Putget law, \putgetcodi, actually determines amendment in a unique way. The other way round, a codiscrete lens without the requirement to satisfy Putget, is a wb codiscrete lens with amendment (which trivially satisfies the amended Putget). 
%  law is a notational trick rather than a law. We begin with delta $v=(A.\get, B')$, which operation  $\putl^\spba_A$  propagates  to delta $u=(A,A')$,  and function $\get$ sends it to delta  $(B,B'')$ where $A'.\get=B''$. Also, $\putl^\spbb_A$ gives us an amendment delta $v^@=(B', B'^@)$ and $v;v^@=(S_p, S'_{p'})=\get_e(S,S')$ so that Putget always holds. %targeting at some model $S'_{p'}$ anyway. But in the general delta setting, there are many possible deltas between models $T'$ and $S'_{p'}$, whereas the Putget law states the existence of some special delta \frar{v^@}{T'}{S'_{p'}} such that equation (\putget) holds. %Note also that Putget implies commutativity of the lower triangle in the right back face as the upper one is commutative by Putget. %much more certainty about $T''$ and precisely specifies the relationship between $T'$ and $T''$, namely, it says that they are related by a specified update $\amex{v}$.
\end{remark}

\endinput

%}  % end renew command
%\end{minipage}

%\input{ll-figures/diags/policyfun-doubleLane}
%\input{ll-figures/diags/lens-compose(a+aa)}
\input{ll-figures/diags/diag-aalens-compose-new}
\noindent Composition of aa-lenses, \frar{\ell1}{\spA}{\spB} and \frar{\ell2}{\spB}{\spC} is specified in \figref{aalenscompose} (objects produced by functors \get s are non-framed, arrows are dashed, and arrows produced by \putl s are dotted).  Operation invocation numbers 1-3 show the order of applying operations to produce the composed \putl: 
$\putl^\spca_A.w=\putl^\spba_A.\putl^\spcb_B.w$ and 
the composed lens amendment $\putl^{\spcc}=w^@$ is defined by composition $w^{@2};(v^{@1}.\get2)$.  In 
%\sectref{alalenscat} 
\sectref{alalenscat}, 
we will see that composition of aa-lenses is associative (in the more general setting of ala-lenses, \ie, aa-lenses with learning) and they form a category \aalenscat\ with a subcategory of wb aa-lenses $\aalenscat_\wbind\subset\aalenscat$. %Also, an ordinary a-lens can be seen as a special aa-lens, for which all amendments are identities, and aa-lens composition specified in \figref{aalenscompose} coincides with a-lens composition in \figref{alenscompose}; moreover, the aa-lens wb conditions become a-lens wb conditions. Thus, we have embeddings $\alenscat\subset\aalenscat$ and $\alenscat_\wbind\subset\aalenscat_\wbind$.


==> sections/functOfUpdpol.tex <==
\subsection{Functoriality of  update policies: An example }\label{sec:backgr-policyfun}
\renewcommand\figrii{\figref{ex-policyfun}}
\newcommand\figrsch{\figref{ex-sixlenses}}

The notion of an update policy transcends individual lenses. \figrii\  extends  the example in \figri\ with a new model space \spC\ whose schema consists of the only attribute \name, and a view of the IT-view, in which only employees of the ML department are to be shown. Thus, we  now have two functors, \frar{\get1}{\spA}{\spB} and \frar{\get2}{\spB}{\spC}, and their composition \frar{\Get}{\spA}{\spC} (referred to as the {\em long} get). The top part of \figrii\ shows how it works for model $A$ considered above. 

\input{ll-figures/pdfs/ex-policyfun}   % now it goes



\input{ll-figures/pdfs/ex-sixlenses}   % now it goes
Each of the two policies,  %considered above: 
\quit\ (green)  and \trans\  (orange), in which person's disappearance from the view are interpreted, resp., as quiting the company and transitioning to a department not included into the view, is applicable to the new view mappings $\get2$ and $\Get$, thus giving us six lenses shown in \figrsch\ with solid arrows; amongst them, lenses, $\nil^{\quit}$ and  $\nil^\trans$  are obtained by applying policy \pol\ to the (long) functor \Get;, and we will refer to them {\em long} lenses. In addition, we can compose lenses of the same colour 
as shown in \figrsch\ by dashed arrows (and we can also compose lenses of different colours ($\ell_1^\quit$ with $\ell_2^\trans$ and $\ell_1^\trans$ with $\ell_2^\quit$) but we do not need them). Now an important question is how long and composed lenses are related: whether $\nil^\pol$ and $\ell_1^\pol;\ell_2^\pol$ for
$\pol\in\{\quit,\trans\}$, are equal (perhaps up to some equivalence) or different?  
%$\pol\in\{\quit, \trans\}$: 

%\input{ll-figures/pdfs/ex-sixlenses}   % now it goes
\figrii\ demonstrates how the mechanisms work with a simple example. 
We begin with an update $w$ of the view $C$ that says that Mary $\#M$ left the ML department, and a new Mary $\#M'$ was hired for ML. Policy \quit\ interprets Mary's disappearance as quiting the company, and hence this Mary doesn't appear in view $B'^\quit$ produced by $\putl2^\quit$ nor in view $A'^\quit_{12}$ produced from $B'^\quit$ by $\putl1^\quit$, and updates $v^\quit$ and $u^\quit_{12}$ are written accordingly. Obviously, Mary also does not appear in view $A^{'\quit}$ produced by the long lens's $\Putl^\quit$. Thus, $\putl1_A^\quit(\putl2_A^\quit(w))=\Putl_A^\quit(w)$, and it is easy to understand that such equality will hold for any source model $A$ and any update \frar{w}{C}{C'} due to the nature of our two views $\get1$ and $\get2$. Hence, %$(\putl1^\quit ; \putl2^\quit) = \Putl^\quit$ and 
    $\nil^\quit=\ell_1^\quit ; \ell_2^\quit$ where $\nil^\quit=(\Get, \Putl^\quit)$ and $\ell_i^\quit=(\get i, \putl{i}^\quit)$. 
    
    The situation with policy \trans\ is more interesting. Model $A^{'\trans}_{12}$ produced by the composed lens $\ell_1^\trans ; \ell_2^\trans$, and model  $A^{'\trans}$ produced by the long lens $\nil^\trans=(\Get, \Putl^\trans)$ are different as shown in the figure  (notice the two different values for Mary's department framed with red ovals in the models). Indeed, the composed lens has more information about the old employee Mary---it knows that Mary was in the IT view, and hence can propagate the update more accurately. The comparison update \frar{\delta_{A,w}^\trans}{A'^\trans}{A'^\trans_{12}} adds this missing information so that equality $u^\trans ; \delta^\trans_{A,w}=u^\trans_{12}$ holds.  This is a general phenomenon: functor composition looses information and, in general, functor $\Get=\get1;\get2$ knows less than the pair $(\get1,\get2)$. Hence, operation $\Putl$ back-propagating updates over \Get\ (we will also say  {\em inverting} \Get) will, in general, result in less certain models than composition $\putl1\circ\putl2$ that inverts the composition $\get1;\get2$ (a discussion and examples of this phenomenon in the context of vertical composition of updates can be found in \cite{me-bx17}). Hence, comparison updates such as $\delta^\trans_{A,w}$ should exist for any $A$ and any \frar{w}{A.\Get}{C'}, and together they should give rise to something like a natural transformation between lenses, 
    \drar{\delta^\trans_{\spA,\spB,\spC} }%
    {\nil^\trans}%
    {\ell^\trans_1;\ell^\trans_2}. To make this notion precise, we need a notion of natural transformation between ``functors'' \putl, which we leave for future work. In the present paper, we will consider policies like \quit, for which strict equality holds.
   %----> very important piece for the next paper   
    \zdpar{----> very important piece for the next paper is endinputed<-----}    
  
  \endinput
  

==> sections/remark-lensLaws.tex <==
\begin{remark}%[On lens laws] %Putget for codiscrete lenses]
	\label{rema:putget4codi}%\zd{to be reworked}
%	The Putget law 
Stability law says that a wb lens does nothing if nothing happens on the target side 
(no actions without triggers). Putget requires consistency after the backward propagation is finished. Note the distinction between the Putget$_0$ condition included into the very definition of a lens, and the full Putget law required for the wb lenses. The former is needed to ensure smooth tiling of \putl-squares (\ie, arrow squares describing application of \putl\ to a view update and its result) both horizontally (for sequential composition) and vertically (not considered in the paper). The full Putget assures true consistency as considering a state $B'$ alone does not say much about the real update and elements of $B'$ cannot be properly interpreted. The real story is specified by delta \frar{v}{B}{B'}, and consistency restoration needs the full (\putgetlaw)  law as above.  
\footnote{As shown in \cite{bryce-act19}, the Putget$_0$ condition  is needed if we want to define  operations \putl\ separately from the functor \get: then we still need a function \frar{\obj{\get}}{\obj{\spA}}{\obj{\spB}} and the codiscrete Putget law to ensure a reasonable behaviour of \putl. 
}
\end{remark}
A more detailed trailer of lenses can be found in the long version \cite{myX-learning19}.
\endinput

In the codiscrete setting, the codiscrete Putget law, \putgetcodi, actually determines amendment in a unique way. The other way round, a codiscrete lens without the requirement to satisfy Putget, is a wb codiscrete lens with amendment (which trivially satisfies the amended Putget). 
%  law is a notational trick rather than a law. We begin with delta $v=(A.\get, B')$, which operation  $\putl^\spba_A$  propagates  to delta $u=(A,A')$,  and function $\get$ sends it to delta  $(B,B'')$ where $A'.\get=B''$. Also, $\putl^\spbb_A$ gives us an amendment delta $v^@=(B', B'^@)$ and $v;v^@=(S_p, S'_{p'})=\get_e(S,S')$ so that Putget always holds. %targeting at some model $S'_{p'}$ anyway. But in the general delta setting, there are many possible deltas between models $T'$ and $S'_{p'}$, whereas the Putget law states the existence of some special delta \frar{v^@}{T'}{S'_{p'}} such that equation (\putget) holds. %Note also that Putget implies commutativity of the lower triangle in the right back face as the upper one is commutative by Putget. %much more certainty about $T''$ and precisely specifies the relationship between $T'$ and $T''$, namely, it says that they are related by a specified update $\amex{v}$.


